Identification of Gaussian Process State Space Models

The Gaussian process state space model (GPSSM) is a non-linear dynamical system, where unknown transition and/or measurement mappings are described by GPs. Most research in GPSSMs has focussed on the state estimation problem, i.e., computing a posterior of the latent state given the model. However, the key challenge in GPSSMs has not been satisfactorily addressed yet: system identification, i.e., learning the model. To address this challenge, we impose a structured Gaussian variational posterior distribution over the latent states, which is parameterised by a recognition model in the form of a bi-directional recurrent neural network. Inference with this structure allows us to recover a posterior smoothed over sequences of data. We provide a practical algorithm for efficiently computing a lower bound on the marginal likelihood using the reparameterisation trick. This further allows for the use of arbitrary kernels within the GPSSM. We demonstrate that the learnt GPSSM can efficiently generate plausible future trajectories of the identified system after only observing a small number of episodes from the true system.

==> experiments/figs/cart_pole/tikz_samples_ep-15-all.tex <==
\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}

\begin{groupplot}[group style={group size=1 by 3}]
\nextgroupplot[
xshift=-8,
title={15 episodes (600 time steps in total)},
title style={font=\large},
xmin=-1.95, xmax=40.95,
%ymin=-0.886000303881668, ymax=0.688703126668518,
ymin=-0.45, ymax=0.45,
width=\figurewidth,
height=\figureheight,
xtick={},
xticklabels={},
yticklabels={},
tick align=outside,
tick pos=left,
x grid style={lightgray!92.026143790849673!black},
y grid style={lightgray!92.026143790849673!black}
]
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.014846076617963
1 0.100461952842589
2 0.260726659261027
3 0.2824492105806
4 0.22398827293092
5 0.0588433707005604
6 -0.0488796608865085
7 -0.115912861665624
8 -0.202868637580512
9 -0.271160301896775
10 -0.26763808386325
11 -0.32859390079
12 -0.282465896304055
13 -0.245298553810735
14 -0.135416004139912
15 -0.0800736528274948
16 -0.0658911166857852
17 -0.0597105016926545
18 -0.0274511281592034
19 -0.0346522892308503
20 -0.0212419602153417
21 -0.0215876763360194
22 -0.0234790688202553
23 -0.0258603081133604
24 -0.0302000384706362
25 -0.0313623720221861
26 -0.012837727073582
27 -0.0420921107397492
28 -0.00512756612439258
29 -0.00115923504458859
30 -0.00158568444861995
31 -0.0129017156877191
32 -0.00538799424687664
33 -0.00534414194975597
34 -0.0281248951658428
35 -0.00388720486309868
36 0.00730785433539971
37 0.00843748010544587
38 -0.00120454458777886
39 -0.0166119049807758
40 0.00158559711675732
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0847707696227165
1 0.0664750210357621
2 0.195076220664519
3 0.22083205857775
4 0.143296415034817
5 0.0104934705878241
6 -0.105614512145792
7 -0.198851922887476
8 -0.27269411095032
9 -0.322517867589121
10 -0.31591203297669
11 -0.373634989614987
12 -0.352305029239165
13 -0.276261909795982
14 -0.137159756373399
15 -0.0511959394782675
16 -0.0378181889779814
17 -0.0643514688040439
18 -0.048985851183037
19 -0.0303116422936425
20 -0.0485958477094766
21 -0.0305162461626569
22 -0.0334678285432695
23 -0.0329623009162692
24 -0.0518813408208469
25 -0.0689403249227718
26 -0.0514754349580562
27 -0.0829771051266937
28 -0.0584138232429137
29 -0.0603644136206309
30 -0.0459686620682627
31 -0.0944088721027931
32 -0.0888103095343107
33 -0.0715824986077802
34 -0.119398034105897
35 -0.122708422152279
36 -0.106590416500752
37 -0.122013274907401
38 -0.144582086211792
39 -0.17622688691316
40 -0.16024286525677
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0732522573716388
1 0.0684200750087038
2 0.248447101859337
3 0.29309085342362
4 0.245515448228272
5 0.118787909477099
6 -0.0183403474389801
7 -0.0628521795972494
8 -0.149443445332998
9 -0.19197491767841
10 -0.17750976613578
11 -0.190631606095018
12 -0.191396893836863
13 -0.165800601544147
14 -0.0528510242552249
15 0.0203587428946994
16 0.0306419107122329
17 0.0274255562110177
18 0.0421815478867549
19 0.0560814018964972
20 0.0423927585624684
21 0.0393712632165588
22 0.036490768678334
23 0.0485934271764776
24 0.0263978755082785
25 0.0242517913839997
26 0.0161315802832007
27 -0.00148279722445466
28 0.0191491251521771
29 0.0116572075353485
30 0.0292289535243357
31 -0.0026527876503204
32 0.0153009047125847
33 0.0246770174888935
34 -0.000128882766214033
35 0.00633501985194318
36 0.00479607445739383
37 -0.0152147194571173
38 -0.0193126268040613
39 -0.0394779084165382
40 -0.0338998516396121
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.033431878492209
1 0.094970123770171
2 0.233683714598099
3 0.269138441092298
4 0.20932029282551
5 0.0521507751358881
6 -0.0704260567742168
7 -0.145014018641827
8 -0.231522547967584
9 -0.301904329794127
10 -0.286739764383757
11 -0.306639600985777
12 -0.287183087411107
13 -0.261343176990266
14 -0.125407747703719
15 -0.0427663422558471
16 -0.0408403853270851
17 -0.0234747601035652
18 -0.0160743065374449
19 -0.00253522651146376
20 -0.00311777589577655
21 0.0169190745314172
22 0.0144328726525469
23 0.0243742218907563
24 0.0140515370149465
25 0.0281706759746569
26 0.031550113544335
27 0.0256313292418806
28 0.0511801630510984
29 0.0542055884482213
30 0.0660371609631891
31 0.0214249661781745
32 0.0409520125710348
33 0.0251870522405788
34 -0.0159240056302883
35 -0.0135434630513362
36 -0.0264704951703356
37 -0.00218443228551379
38 -0.0087382488696699
39 -0.0197797783287958
40 0.0145803411689078
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0376071097179365
1 0.098819184198053
2 0.233647171237585
3 0.264496709943409
4 0.200956405025161
5 0.0676487430531774
6 -0.0656657465641404
7 -0.151888590703583
8 -0.214345823797013
9 -0.277653677232077
10 -0.26416534507218
11 -0.311568207735448
12 -0.298534825202426
13 -0.245267309245865
14 -0.118417442351774
15 -0.0571557686876627
16 -0.0491790075927669
17 -0.0408082595861012
18 -0.0111601295304435
19 -0.00969496554971805
20 -0.0185276334661628
21 -0.00335455818239527
22 -0.00798834923865677
23 -0.00846299884847479
24 -0.0312809503540263
25 -0.0154667060526616
26 0.00903876859953723
27 -0.0174314523487222
28 0.0063188646196215
29 0.00657644900480658
30 -0.00612055546006918
31 -0.0348556802733988
32 -0.0268023981438139
33 -0.0340395023291888
34 -0.0628262419235615
35 -0.0497104756801541
36 -0.0410482767202858
37 -0.055663016281791
38 -0.0531769642067026
39 -0.0517562645605585
40 -0.0312020554083388
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0283432062780591
1 0.137708900617683
2 0.279120760575741
3 0.304345205240227
4 0.23006718671645
5 0.0951712115009524
6 -0.0177153745520835
7 -0.120881089950114
8 -0.203653075034057
9 -0.270898619055411
10 -0.25122363148553
11 -0.263648415819803
12 -0.255761992566483
13 -0.194765769483788
14 -0.0665263350967527
15 0.018361428808034
16 0.0010506877566554
17 -0.00484388653518586
18 0.0213942139970138
19 0.0432502404441726
20 0.0416235975474644
21 0.0740163502002842
22 0.0746706203633583
23 0.0679326473757786
24 0.0451557670264897
25 0.0488324074504085
26 0.0662107879714142
27 0.0481768470326882
28 0.0823279513232906
29 0.0809360303397417
30 0.0701641383938574
31 0.0394232032360566
32 0.0292301392484786
33 0.0265796967368459
34 -0.0143792367442339
35 -0.0345090973620561
36 -0.0117882534175617
37 -0.00316659199278302
38 -0.00228247002457316
39 -0.017797589273
40 -0.0205884401215242
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0586110238225528
1 0.0691670921451655
2 0.201564203301778
3 0.23911488467859
4 0.162812533911242
5 0.0227170627444018
6 -0.0868372768684083
7 -0.170727133460055
8 -0.250005290353231
9 -0.331899743122335
10 -0.315047693118001
11 -0.361423483968542
12 -0.345586391375502
13 -0.32908856210644
14 -0.20097896866712
15 -0.117269672990457
16 -0.131085433761716
17 -0.0948270066005783
18 -0.0771249714721218
19 -0.0757552159854287
20 -0.0614538667769047
21 -0.0505129949597345
22 -0.0426772086360092
23 -0.0326620716358548
24 -0.0503311907369923
25 -0.0266204185693093
26 -0.00983183256331444
27 -0.0178420835335045
28 0.0321424851384275
29 0.0464892465270728
30 0.0502339300030803
31 0.022454963030639
32 0.0232073976880631
33 0.0333740864824392
34 0.0292756596954264
35 0.0550146533010372
36 0.0718004830711507
37 0.0822089749631578
38 0.0643631200319303
39 0.053997413708565
40 0.085837559553287
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0505412382424044
1 0.08954151148773
2 0.235265803078786
3 0.263590494597963
4 0.205973716216044
5 0.0711674867183021
6 -0.0485030220494309
7 -0.14936494337546
8 -0.213971420724846
9 -0.271142600033067
10 -0.276156070246911
11 -0.308793076359334
12 -0.294580488402643
13 -0.274372609773147
14 -0.154791170464905
15 -0.0946711266386719
16 -0.111491865293369
17 -0.119575173971865
18 -0.0925142091847544
19 -0.0854586093242213
20 -0.0892668674477335
21 -0.0744203718690981
22 -0.0686183668820783
23 -0.0289229577346157
24 -0.0464922319986787
25 -0.0565173382953379
26 -0.030841620343292
27 -0.0336777889358979
28 -0.0208028783626197
29 -0.0136843431250169
30 -0.0143436957368479
31 -0.0377783858123122
32 -0.0375197922465169
33 -0.0327998823120659
34 -0.0486341785847673
35 -0.0490370080549196
36 -0.0182130691313072
37 -0.0090094938299794
38 -0.0152583437419267
39 -0.0117810257407074
40 0.00431862162047025
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0128584347377636
1 0.129617567190135
2 0.268510951757616
3 0.294183050665948
4 0.209364885660571
5 0.062422819481152
6 -0.0699782342422974
7 -0.143424648235976
8 -0.190330168694506
9 -0.257070878012151
10 -0.23487280168802
11 -0.21195560000147
12 -0.189307218557755
13 -0.146846759429923
14 0.0175197234941908
15 0.109750935158062
16 0.14889207676565
17 0.154312470988254
18 0.182565761243964
19 0.199206057445347
20 0.218437586543413
21 0.240366427230386
22 0.24517694303556
23 0.278941588895412
24 0.284282826544907
25 0.327099593825271
26 0.358806703645287
27 0.371238625322951
28 0.433609502404036
29 0.501976539660484
30 0.55506949560078
31 0.594554382519621
32 0.638098431173129
33 0.711541552438859
34 0.861560355809978
35 0.996805927180278
36 1.14118683486291
37 1.28265739549433
38 1.44316657607262
39 1.58363070291133
40 1.75747969892167
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0403290352347465
1 0.0905662959708957
2 0.214092415791705
3 0.231325306039928
4 0.18000674482172
5 0.0376219438501328
6 -0.0874793910045213
7 -0.185568401251226
8 -0.288152921258838
9 -0.346908589446421
10 -0.335425196094388
11 -0.363186892667437
12 -0.348137543045417
13 -0.310597198275722
14 -0.175891719750919
15 -0.136575120386923
16 -0.123661943168289
17 -0.112481995054289
18 -0.0812755995105645
19 -0.0516194876767617
20 -0.0481317925555649
21 -0.0272462740448924
22 -0.0167133447939412
23 -0.00480199314316554
24 -0.0225256929495616
25 -0.0280669289435016
26 0.00178218723191037
27 -0.025549033984773
28 -0.00751508101246046
29 -0.00116568173328169
30 0.0102828838842459
31 -0.000987462443688969
32 0.0171780156971373
33 0.0488024385282495
34 0.0274899516941112
35 0.0398172902320901
36 0.053248210149401
37 0.0409418950895999
38 0.0390122064440064
39 0.0376462440935859
40 0.0705914204383387
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0190824173716839
1 0.10842895170507
2 0.243683520540261
3 0.30553120593212
4 0.235112255725642
5 0.119102188015201
6 0.0133711622007935
7 -0.0641319393921256
8 -0.162452931562295
9 -0.226871761800854
10 -0.184313725594651
11 -0.227543729938391
12 -0.230634914658105
13 -0.188224741339317
14 -0.0891987692152449
15 -0.0169710765762812
16 -0.0330072873383171
17 -0.0413804500786297
18 -0.0292357605183939
19 -0.0261025519908777
20 -0.0149394879729039
21 -0.01345198080387
22 -0.0295783899119391
23 -0.0267504303816883
24 -0.0489865243778098
25 -0.0368614624442225
26 -0.0412731484288242
27 -0.0496225568025856
28 0.000160869204102632
29 0.0221025518849363
30 0.0170412983644992
31 0.0109086966037468
32 -0.00887199512286241
33 -0.0149708678367055
34 -0.0392561661618993
35 -0.0404255040011412
36 -0.0329641632907096
37 -0.0367673516439408
38 -0.0323210538666885
39 -0.0364226695696654
40 0.0152849038864966
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0588214210406885
1 0.0713947039136631
2 0.209276787554557
3 0.235939725570908
4 0.173525848793025
5 0.029937656643038
6 -0.137510065509271
7 -0.226358558864186
8 -0.305982268859187
9 -0.371079909678193
10 -0.354274724109954
11 -0.391468174394323
12 -0.398894978774826
13 -0.34821957597265
14 -0.257716242657077
15 -0.22305573822532
16 -0.206853268023432
17 -0.224901568752551
18 -0.206553849064845
19 -0.182100733870947
20 -0.176760969415978
21 -0.150603295215978
22 -0.140928729046911
23 -0.115720710589438
24 -0.14063927959863
25 -0.142552859049255
26 -0.119810149008387
27 -0.114558673189844
28 -0.0854307467317277
29 -0.0746537604597268
30 -0.0790425641322985
31 -0.0891065121664418
32 -0.0711221470887251
33 -0.0631632604065864
34 -0.0689710863236677
35 -0.0495531760414742
36 -0.0342192515420772
37 -0.00585890162644631
38 -0.0170368218310566
39 -0.0228568325019216
40 -0.0121096530346012
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.000672788696027382
1 0.128497260511284
2 0.272340157653971
3 0.302460830430134
4 0.256802898132805
5 0.133204909688808
6 0.0151025786582206
7 -0.0590926214326979
8 -0.158506335322864
9 -0.187163171181264
10 -0.165503465067219
11 -0.223960893479011
12 -0.212950817777537
13 -0.193288541578628
14 -0.0769426813302188
15 -0.0205194727599238
16 -0.011357198564899
17 -0.00694917272351248
18 0.0162997593804626
19 0.0483124952992293
20 0.0525352248842248
21 0.0482016436200059
22 0.0224046888330482
23 -0.0168292925613267
24 -0.0172457383807085
25 -0.0401879657573465
26 -0.0666388322476363
27 -0.078705777667242
28 -0.0790475168687994
29 -0.108479955807559
30 -0.107445137478431
31 -0.13641820666792
32 -0.173144523002834
33 -0.171017916681015
34 -0.202042056795784
35 -0.208878037773377
36 -0.204097514778876
37 -0.209976070264675
38 -0.243220171169241
39 -0.256977482029334
40 -0.259105679411265
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0709501469875446
1 0.0277379085346077
2 0.147729470810397
3 0.192700361719504
4 0.134676998886446
5 -0.00691389204747583
6 -0.121903323723327
7 -0.197822881941724
8 -0.279428707253953
9 -0.326796175430185
10 -0.294098792889947
11 -0.318815816372509
12 -0.30624113564383
13 -0.276466185918134
14 -0.144519831581902
15 -0.0306568688314286
16 -0.0320193993173028
17 -0.0233792574568357
18 -0.0153598377320252
19 -0.028624614353312
20 -0.000328479459501985
21 0.00281956730573363
22 0.00375128002476544
23 0.0211403141828912
24 0.0106236652480716
25 0.0166132676544892
26 0.0107473594161531
27 0.00779759407484359
28 0.0220467198882304
29 0.0106221730172837
30 0.00292351855246586
31 -0.0418562161004807
32 -0.0483071793400969
33 -0.0385160302237164
34 -0.0449748649794834
35 -0.0301929044141644
36 -0.0337771749031175
37 -0.0604801713147198
38 -0.0626493000537289
39 -0.06526323897201
40 -0.0528096445107531
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.00323155676220388
1 0.137880046519223
2 0.289068566389865
3 0.312882698647313
4 0.246058889579522
5 0.112066529680905
6 -0.0105596775677848
7 -0.0514833248007198
8 -0.10554429984392
9 -0.194683538730837
10 -0.197094545251952
11 -0.217693538875068
12 -0.199361370066462
13 -0.172080568321628
14 -0.0209363044638033
15 0.0454571945042082
16 0.0323004078481404
17 0.0277323410260131
18 0.0284833901076871
19 0.0491452473210439
20 0.0439939865033452
21 0.0530760540929345
22 0.0400063375006674
23 0.0474485558049702
24 0.024565336460566
25 0.0193571557107433
26 0.0319199929115959
27 0.0302946642795829
28 0.0424065254786044
29 0.0469827359219526
30 0.0316988655945023
31 0.0176998109076125
32 0.00886335379562908
33 0.0343263519163539
34 0.0195949110518514
35 0.0350393701185423
36 0.044817148456394
37 0.0308760900000378
38 0.00456359846948917
39 -0.00617921269609401
40 -0.0120329693872598
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0321681423227753
1 0.0884341459368301
2 0.236463939197271
3 0.265224355079421
4 0.223185841414506
5 0.100024226640191
6 -0.0176413430263667
7 -0.0996734478068531
8 -0.197969825578135
9 -0.245796899930812
10 -0.241889744005092
11 -0.293214243111686
12 -0.277357104338418
13 -0.239255430773306
14 -0.0721572843320599
15 0.0105289176374725
16 0.00725502166412006
17 -0.0037027953233677
18 0.0194086321990579
19 0.0423436641217814
20 0.0514194201093758
21 0.0653704744199697
22 0.0688807120889692
23 0.0961414634919686
24 0.0675689371265067
25 0.0743345441258185
26 0.0872057548947218
27 0.0970996157518753
28 0.115118483106946
29 0.102820033871118
30 0.114171024421752
31 0.0794261347425964
32 0.0660888229593697
33 0.0918433184436083
34 0.0713501893792463
35 0.0680391154128479
36 0.0975543041881526
37 0.0881247046229676
38 0.0747211410072204
39 0.0599708440741447
40 0.0474610820302983
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.046469280626428
1 0.0759773552830687
2 0.223344026279991
3 0.261264242702783
4 0.207437286030483
5 0.0621250457853302
6 -0.0688345463911917
7 -0.175306093207304
8 -0.254189454202124
9 -0.297878989130255
10 -0.263982525728501
11 -0.304803203035285
12 -0.284748607175968
13 -0.226959312903601
14 -0.105489602929805
15 -0.0211297185570904
16 -0.0236135023952313
17 -0.0230095316853625
18 -0.00900400703746929
19 -0.0117742217948011
20 -0.000728717353037034
21 -0.0095408187786381
22 0.000514295844481261
23 -0.00383627998058866
24 -0.0281572980195435
25 -0.0270618465935559
26 -0.0377504352983005
27 -0.0495428919068637
28 -0.0324363146582023
29 -0.0475184660461192
30 -0.0737895353813069
31 -0.123245064303713
32 -0.122407856626117
33 -0.143607991101066
34 -0.169549089448413
35 -0.166921487035822
36 -0.166416529986996
37 -0.183441255383308
38 -0.208081601333837
39 -0.244864624559431
40 -0.234051245203565
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0209970714300178
1 0.102293833111213
2 0.243860468009455
3 0.272415230731605
4 0.209340977581139
5 0.0845205842789598
6 -0.0511720588622726
7 -0.146701804792011
8 -0.250142746016949
9 -0.306872104581223
10 -0.260803189845491
11 -0.278488099879375
12 -0.24182021599371
13 -0.175561922709949
14 -0.0360535534361315
15 0.0321204959379155
16 0.014209428354742
17 0.00913313668035265
18 0.00287454695671485
19 0.00985086622817288
20 0.0104445123522394
21 0.0279428600151217
22 0.0273620597327833
23 0.014047047312479
24 -0.0116895528085665
25 -0.0337933675324189
26 -0.0348916733930151
27 -0.0573315720921643
28 -0.0405441077265687
29 -0.0250987740596447
30 -0.0351942494629629
31 -0.0610227739804046
32 -0.0719606331652924
33 -0.0602736115017466
34 -0.0665979101843117
35 -0.0824801669483213
36 -0.0642329853979584
37 -0.0844507410576911
38 -0.0971676528345853
39 -0.10080995140499
40 -0.0959340861108533
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0098128157207924
1 0.132287304177002
2 0.263559891914474
3 0.303530649495843
4 0.254271388773809
5 0.127153695058569
6 0.0057533271193595
7 -0.073344448771655
8 -0.166292679051804
9 -0.22911322610905
10 -0.221901738905595
11 -0.269789280031473
12 -0.248864693051823
13 -0.200368941543975
14 -0.0700200541924874
15 0.00641047177093501
16 0.0124678687387556
17 0.00715963033764488
18 0.044037521201334
19 0.0650675607884246
20 0.0595528495323014
21 0.0799048003507252
22 0.0695138803349398
23 0.0904869841769465
24 0.0820631461145496
25 0.0893118601882632
26 0.0946685121917517
27 0.0947731636572975
28 0.168364234974876
29 0.162750236701377
30 0.190705415771849
31 0.184031058025797
32 0.184674075766468
33 0.215092760530803
34 0.191108029072192
35 0.200930009121389
36 0.278578908594061
37 0.315118796235911
38 0.373542802941143
39 0.430839663778962
40 0.539575370167714
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0149750227694172
1 0.123836414962073
2 0.27447548982133
3 0.306761584631977
4 0.236309389822043
5 0.0807432484579103
6 -0.0361004845070605
7 -0.118537799273056
8 -0.228203937551802
9 -0.297023652496565
10 -0.308528356694998
11 -0.376214940368907
12 -0.364732314078339
13 -0.325300038977505
14 -0.182370670553064
15 -0.114235772469647
16 -0.100772711524912
17 -0.0993533954677659
18 -0.0776051242747293
19 -0.0627886078316031
20 -0.0656148627570028
21 -0.0498951406440158
22 -0.0578794883858125
23 -0.0547786287642076
24 -0.079967678971256
25 -0.0815792598371905
26 -0.0724908947263438
27 -0.116587510683202
28 -0.076124549367381
29 -0.0820880521318719
30 -0.0829760667674444
31 -0.120601996187952
32 -0.125365155835405
33 -0.10059080249472
34 -0.15544312744173
35 -0.149339332910375
36 -0.124279900371597
37 -0.126270673421472
38 -0.123476880825807
39 -0.176318641444695
40 -0.164189042942168
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0188767656939648
1 0.118283088413852
2 0.267728449312489
3 0.303519326080456
4 0.245206345824266
5 0.131169749121968
6 0.0171983720240361
7 -0.0572460788633453
8 -0.13117854271998
9 -0.180732148637908
10 -0.155028929539278
11 -0.200101573103692
12 -0.177141636628531
13 -0.158753138380378
14 -0.0261299276022831
15 0.0310390322837106
16 0.0107717087143593
17 0.00715177696451086
18 0.0340977397764144
19 0.0579728378366795
20 0.0474199476333288
21 0.0604805704799647
22 0.0617981352716948
23 0.0587767229681386
24 0.047327041050254
25 0.0219377154076641
26 0.0298696627841233
27 0.0276135649900517
28 0.0522382412970019
29 0.0814359594310892
30 0.0860231565702616
31 0.0581469646230399
32 0.0515805566712064
33 0.0762535017913892
34 0.0830752440293319
35 0.0660621030747892
36 0.0876666221289648
37 0.07735485665407
38 0.0663036455725381
39 0.0683842229769454
40 0.0857137474241627
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0108569518406103
1 0.132187494426833
2 0.254640950323669
3 0.277195495009855
4 0.211061752194364
5 0.0660091089786592
6 -0.0543809815180367
7 -0.133296340876569
8 -0.220079176736936
9 -0.28476046879359
10 -0.288345407414574
11 -0.325398153131291
12 -0.308928407995991
13 -0.284358840851739
14 -0.170629196864948
15 -0.0933553373353355
16 -0.0814170281916233
17 -0.104999617046145
18 -0.0902384151360192
19 -0.0701282142094213
20 -0.081761109350877
21 -0.0744420526542688
22 -0.0916216514577295
23 -0.0996918019260065
24 -0.128577510642143
25 -0.140565968593778
26 -0.150646889536059
27 -0.193976552239688
28 -0.145232479772717
29 -0.143046315904526
30 -0.146233823657915
31 -0.17193704640773
32 -0.170776451699601
33 -0.167965908301534
34 -0.220063450018474
35 -0.241489291060492
36 -0.244290600460261
37 -0.266245652162413
38 -0.275776529514565
39 -0.296396032669251
40 -0.299665175065009
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0365626588926515
1 0.107845896406783
2 0.254743770541071
3 0.289773624014312
4 0.219014808677528
5 0.0858430407042929
6 -0.0633295688837654
7 -0.1362330379236
8 -0.223655419906152
9 -0.289961763429701
10 -0.288380248224112
11 -0.34268050201869
12 -0.329438023967382
13 -0.274463104549855
14 -0.143008250575626
15 -0.0822694156515498
16 -0.109197773288037
17 -0.11781661919525
18 -0.128246212494734
19 -0.144987221207549
20 -0.163613967005929
21 -0.184771881524545
22 -0.22352521951557
23 -0.268267264447574
24 -0.328334732882956
25 -0.356799733755155
26 -0.38575215024397
27 -0.415763071010335
28 -0.414384406816698
29 -0.444191079947069
30 -0.480649513061214
31 -0.502547685494207
32 -0.519521228102467
33 -0.535439412186363
34 -0.579533886028855
35 -0.587943827754708
36 -0.593036097456329
37 -0.613843173689887
38 -0.63303273914481
39 -0.656168008689813
40 -0.665286152057652
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.013968464797494
1 0.105846886248711
2 0.24476942022551
3 0.295027832015719
4 0.228716045468285
5 0.0829334767624879
6 -0.0246641042747191
7 -0.103324118867399
8 -0.169599756041436
9 -0.241778726294575
10 -0.212833232349583
11 -0.271260080432789
12 -0.271496843984641
13 -0.257289602599084
14 -0.115924235092199
15 -0.0613042280151745
16 -0.102585402621859
17 -0.119058014569179
18 -0.122264737212294
19 -0.128171846460487
20 -0.132422950517715
21 -0.110764323805739
22 -0.0996915541874008
23 -0.0908864410835157
24 -0.0903551783100403
25 -0.0792756581168179
26 -0.0826189645205542
27 -0.0847126309211959
28 -0.053984378727149
29 -0.0621715223916457
30 -0.0607056957689656
31 -0.0830746471931558
32 -0.0748210741540154
33 -0.0633782031501084
34 -0.076402407012929
35 -0.0616923751925
36 -0.0358261633194044
37 -0.0241674479890124
38 -0.0317792292436403
39 -0.0402385871394255
40 -0.0231878233760971
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0150235552062439
1 0.143884328632777
2 0.288799233357342
3 0.334556497419732
4 0.263474827709976
5 0.136946048136641
6 -0.0172319457039105
7 -0.0906495773561362
8 -0.174965171705484
9 -0.268907615570444
10 -0.260748464408167
11 -0.301386940231277
12 -0.262195628170798
13 -0.219027436530343
14 -0.0930508826787761
15 -0.00340295764257714
16 0.0109900700444756
17 0.0118020286710543
18 0.0335463628574617
19 0.0667037855153723
20 0.0732425746673639
21 0.102524752092578
22 0.0978869395278839
23 0.117979677000996
24 0.100144565843895
25 0.110299353845949
26 0.11988608802805
27 0.133108824656087
28 0.14962490832889
29 0.157430520750427
30 0.188195479981307
31 0.186383119258098
32 0.198879045728575
33 0.192874146860285
34 0.188585777036178
35 0.186995715477023
36 0.230908684449989
37 0.239767956404316
38 0.298911206797461
39 0.378295075412108
40 0.41794967781168
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0698330474281468
1 0.0682970759384505
2 0.24311693013108
3 0.282413020539949
4 0.232833449217467
5 0.0777543138537311
6 -0.0747356117884417
7 -0.159091222960051
8 -0.230083272989178
9 -0.283001249624853
10 -0.273219466815938
11 -0.294370748343487
12 -0.29279141040722
13 -0.253806250922862
14 -0.125743067166904
15 -0.0633698737900668
16 -0.0606754717202866
17 -0.0660488074840266
18 -0.0506818147636681
19 -0.0456604843209982
20 -0.0357479269626948
21 -0.0191352229593749
22 -0.0120888508766903
23 -0.000728672501900895
24 -0.0150495618660837
25 -0.00822895950396951
26 -0.00974857499911419
27 -0.00785588240602308
28 0.00732269090420523
29 0.017024672430038
30 0.0264205760384799
31 0.0126561932117477
32 0.00993837752392857
33 0.0138390718100094
34 -0.0140038360777099
35 -0.00134826906041852
36 0.0195413951080736
37 0.032027276839564
38 0.0479872023666275
39 0.0248904714199281
40 0.0395886400661167
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0799085710392955
1 0.073091691011447
2 0.215674290212807
3 0.225066045402495
4 0.18578147692153
5 0.0671428875648559
6 -0.0698128233879451
7 -0.168606635958218
8 -0.22072497435548
9 -0.283341205589631
10 -0.303863696824633
11 -0.338952094137341
12 -0.331314326069613
13 -0.280694702851324
14 -0.189811033632582
15 -0.154900245718562
16 -0.1275688816169
17 -0.120981366475362
18 -0.0886731600497761
19 -0.0532522595041556
20 -0.0485978150267226
21 -0.017525482503463
22 -0.0142000554017843
23 0.0134012584438956
24 -0.0257354991295857
25 -0.0194196715348749
26 -0.00599720860293917
27 -0.0198915019988899
28 0.0108444774522196
29 0.00633488077902911
30 0.0102986138562384
31 -0.0518800564725908
32 -0.0464577706461125
33 -0.0340496595621573
34 -0.0661140439026706
35 -0.054334285044523
36 -0.0577408012971912
37 -0.0572835322467418
38 -0.0847558460784805
39 -0.097628641048991
40 -0.0973782176506548
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.040678322257504
1 0.0915555230707383
2 0.2414606202274
3 0.270818244338813
4 0.196324480996217
5 0.0329246807101429
6 -0.0961373764762854
7 -0.176457384377067
8 -0.255661762857952
9 -0.302573009329307
10 -0.267082727291122
11 -0.302964804091267
12 -0.275849951861252
13 -0.24019267098697
14 -0.108807453724809
15 -0.0376748714632091
16 -0.0404831596757456
17 -0.0431914895021475
18 -0.0125173062101593
19 0.00378722384084274
20 0.0135197916002436
21 0.0252405521301311
22 0.0506827906179286
23 0.0615496709603205
24 0.0614573082203345
25 0.0872425161050279
26 0.096496587302509
27 0.0948823377086647
28 0.139804562368855
29 0.173169963321299
30 0.179407278759959
31 0.186718535981433
32 0.207653090154833
33 0.205792601293528
34 0.187576349818296
35 0.207818111861925
36 0.211119714951324
37 0.249936512113218
38 0.301202018159114
39 0.35763443794549
40 0.438386965524617
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0344463985820651
1 0.0745468074017781
2 0.224479777373963
3 0.262178391857592
4 0.198924036093244
5 0.054394582985581
6 -0.0757712343945736
7 -0.163887273174873
8 -0.241251837907644
9 -0.308092081930982
10 -0.268582075036556
11 -0.302040730337732
12 -0.276521544368467
13 -0.258199844754186
14 -0.120261749498723
15 -0.00387682541724921
16 0.0085810491009255
17 0.0191071406634187
18 0.0238073999270139
19 0.04430955970503
20 0.0440619149387089
21 0.0642804746265986
22 0.0690093871947957
23 0.110830298422573
24 0.106694437684985
25 0.117145697349758
26 0.139785328821795
27 0.105735870618865
28 0.148638861403406
29 0.165711529407867
30 0.196749779218469
31 0.208988233675591
32 0.232074633856556
33 0.245754492624012
34 0.251592183443941
35 0.266476661921084
36 0.285009212446302
37 0.299601855835085
38 0.313577256576999
39 0.321460561175153
40 0.361834553127336
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0503954282555288
1 0.0855314348595844
2 0.241734215352396
3 0.275335428634553
4 0.21207371620474
5 0.0701448489183365
6 -0.0590739014847514
7 -0.155371068358962
8 -0.223244429973097
9 -0.298288039568189
10 -0.28851486476654
11 -0.345665605330247
12 -0.324823652493254
13 -0.26389638660271
14 -0.134111162950033
15 -0.029901394612323
16 -0.0369619062618982
17 -0.0537950478814153
18 -0.0527395412486413
19 -0.0319583737915359
20 -0.0474707948505015
21 -0.0330523296023921
22 -0.0348010472764306
23 -0.0241156759048726
24 -0.0336896464630572
25 -0.0614212511368661
26 -0.0428541591502727
27 -0.0663413171326317
28 -0.0441644551926768
29 -0.0374481050870648
30 -0.0415286500455148
31 -0.072741561074972
32 -0.0675265518166999
33 -0.0250524947893904
34 -0.0391496722150997
35 -0.043381501519753
36 -0.0302479240267388
37 -0.0269724621959853
38 -0.0438191286576819
39 -0.076579557254993
40 -0.061649651693255
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0858440431593834
1 0.0589308908937296
2 0.206430986813942
3 0.226015021974324
4 0.182093058989919
5 0.0831666885817803
6 -0.0204665057228004
7 -0.102237285128712
8 -0.171075959403081
9 -0.231928336699118
10 -0.242383199523092
11 -0.299832570256853
12 -0.29813387012829
13 -0.298634170249972
14 -0.174415140117796
15 -0.139397207042371
16 -0.14655318175009
17 -0.179633304731331
18 -0.17583643003292
19 -0.181536969744274
20 -0.178617409520916
21 -0.161795937728027
22 -0.158667895203777
23 -0.164034733617083
24 -0.206969838239199
25 -0.225180486133874
26 -0.220079410581436
27 -0.249332441289051
28 -0.217196744862387
29 -0.221265533499913
30 -0.242394639412185
31 -0.299822465452178
32 -0.306580362405087
33 -0.331351312018762
34 -0.385780506705731
35 -0.40445757117392
36 -0.376377799445505
37 -0.412717739313905
38 -0.446687528182997
39 -0.479657544124598
40 -0.485145548256284
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0603838142873503
1 0.0731872750449734
2 0.227477726163048
3 0.277767311044643
4 0.221207800561133
5 0.0821688145775843
6 0.00131369699189943
7 -0.0406895450187159
8 -0.131236617509892
9 -0.195556363431112
10 -0.203370082459633
11 -0.246109059419775
12 -0.253818386793245
13 -0.189834644655673
14 -0.0598753049678162
15 -0.0300754085722188
16 -0.0317239091439214
17 -0.0287955794449859
18 -0.00238010583069581
19 0.0130947875852545
20 0.00058323932453419
21 0.0115828094398696
22 0.00945873061570524
23 0.00995007702914297
24 0.0110915878472335
25 0.0281547920951688
26 0.0564702437088132
27 0.0271565798705415
28 0.0776643458640738
29 0.0876208047553284
30 0.0997155866471591
31 0.10048722277581
32 0.103732185986684
33 0.102764075121303
34 0.109930624381543
35 0.114760043002677
36 0.14724139758482
37 0.157762986739793
38 0.149125729958257
39 0.161240125390842
40 0.185711502881517
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0204428635598344
1 0.13810129763775
2 0.310134051392922
3 0.344027895610705
4 0.27425652799741
5 0.129336036044213
6 -0.00581602329413755
7 -0.107807945882386
8 -0.184879570046484
9 -0.243114970137481
10 -0.225232183097384
11 -0.289822868473168
12 -0.250976245121024
13 -0.197160998697788
14 -0.0659101483599471
15 0.00703270097170083
16 -0.00348664275962651
17 0.0113230080532416
18 0.0260841324594505
19 0.0344492185322123
20 0.0256207350179745
21 0.0438372402132847
22 0.0301400967032066
23 0.047598216725242
24 0.0151919610625928
25 0.00537018002718082
26 0.0276331577282241
27 0.00650395658649305
28 0.016680064448221
29 0.0276006917198615
30 0.042309585894956
31 0.0193184005457452
32 0.0127991907367431
33 0.0295082977575634
34 0.0244299659052487
35 0.020874037639361
36 0.0191193504775322
37 0.0149359102132784
38 0.00463278239058607
39 0.00349782952811761
40 0.0065164420463022
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0518429248688843
1 0.0680548626033914
2 0.213038290703264
3 0.249572498225794
4 0.183684975345599
5 0.0374137477448349
6 -0.0882600457998803
7 -0.169871856332598
8 -0.254825513525367
9 -0.310717174575349
10 -0.269253682888171
11 -0.336212568159964
12 -0.323875937263526
13 -0.272223100596102
14 -0.143442422894934
15 -0.0840013963058768
16 -0.0582587405613317
17 -0.0560907941932891
18 -0.0340484692217107
19 -0.0302572648958641
20 -0.0466852246772955
21 -0.0262515529083238
22 -0.0284055523282776
23 -0.0113500511297593
24 -0.0486608464576186
25 -0.0393259755924493
26 -0.0221854475531975
27 -0.0545103475506217
28 -0.0381170255707728
29 -0.0467582783321312
30 -0.0315213995970787
31 -0.0572909899484895
32 -0.0502741042282038
33 -0.0638066963648818
34 -0.0983706939281506
35 -0.0980066327168361
36 -0.086558904529177
37 -0.0881224118080777
38 -0.097164271436526
39 -0.122971812301634
40 -0.132533928583258
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.034814367591097
1 0.10178381929038
2 0.237681435372937
3 0.25549884269059
4 0.181106791515995
5 0.0394311252565922
6 -0.109339970508306
7 -0.186083477493417
8 -0.252444451197354
9 -0.338595884390167
10 -0.319479190807447
11 -0.365977179931441
12 -0.353787666880274
13 -0.316381910609717
14 -0.19485835099628
15 -0.139220087363614
16 -0.12392070034234
17 -0.120656740691258
18 -0.0941250354564387
19 -0.0639945468352314
20 -0.0568366437953278
21 -0.0499812206112287
22 -0.0831225636535775
23 -0.0831534824193731
24 -0.0959460137688826
25 -0.0828691370131889
26 -0.0782335107200822
27 -0.114753052041125
28 -0.0664899653363271
29 -0.0850982726544292
30 -0.0764679098591108
31 -0.109672888467226
32 -0.112548465072243
33 -0.0989425218281346
34 -0.130841528698112
35 -0.150250523655101
36 -0.144645595367003
37 -0.162605966347192
38 -0.173990146674857
39 -0.189643844787231
40 -0.178297279584791
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0413623399532108
1 0.0718237498491536
2 0.21870756742765
3 0.237034746006262
4 0.167329895340332
5 0.0250882658492335
6 -0.0847409264799586
7 -0.175006733390451
8 -0.247336583237547
9 -0.302805798620042
10 -0.304751614155336
11 -0.319455279122955
12 -0.314323225455751
13 -0.2828427242534
14 -0.190049749372126
15 -0.120966417950406
16 -0.124413775150877
17 -0.12328900603849
18 -0.101148122022519
19 -0.103133658668079
20 -0.115583714879552
21 -0.104602076851594
22 -0.106983380121591
23 -0.1091881851889
24 -0.135173220634347
25 -0.134972095857175
26 -0.123013152466542
27 -0.123413176234122
28 -0.0816634287347098
29 -0.0661841067394162
30 -0.0660186514530716
31 -0.0730440023981327
32 -0.0586395116600773
33 -0.0665820060594866
34 -0.0841374526705634
35 -0.0784808101571279
36 -0.0486311739092811
37 -0.0476184985048693
38 -0.0299015091208537
39 -0.0345899099418139
40 -0.00793601092664709
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0369961723159653
1 0.0729027315970852
2 0.233946138214416
3 0.266607448515781
4 0.203934326520571
5 0.0506585375284452
6 -0.0586924428035349
7 -0.139449660633428
8 -0.231357744237982
9 -0.308551655076687
10 -0.316774842559814
11 -0.375296304993291
12 -0.358820568560454
13 -0.316756095543094
14 -0.169032866428524
15 -0.0979104858726538
16 -0.0985450461012265
17 -0.109064931940527
18 -0.0825152059768737
19 -0.0716331280555478
20 -0.0970087875051719
21 -0.0970875001184526
22 -0.082616255793706
23 -0.0674669582684384
24 -0.0840232829282073
25 -0.0787558363929728
26 -0.0701527282990524
27 -0.0811945306613691
28 -0.0565607244298763
29 -0.0393154788275503
30 -0.0591820764808908
31 -0.102356267045034
32 -0.0941509453611635
33 -0.0949097204434803
34 -0.131309124552883
35 -0.116315945143983
36 -0.104197086680036
37 -0.0943567814401742
38 -0.0875796346755662
39 -0.105758429578898
40 -0.0787458580951848
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0608675911155219
1 0.0497617698174295
2 0.181139719397735
3 0.213041040017354
4 0.134862381786657
5 -0.0197750920427682
6 -0.146903061355998
7 -0.239743507855117
8 -0.30991912324469
9 -0.381523222986297
10 -0.373001559330913
11 -0.395930140877296
12 -0.391143859705675
13 -0.362738185917404
14 -0.242812602754498
15 -0.175601601298511
16 -0.160966427122458
17 -0.174322913038474
18 -0.135784741764778
19 -0.113727203062028
20 -0.106102925458084
21 -0.0952763814840765
22 -0.108167021726028
23 -0.0852532149990148
24 -0.114511040187854
25 -0.128564629205171
26 -0.105927473631207
27 -0.130162505434768
28 -0.117060659190591
29 -0.112865120678913
30 -0.0948783717727366
31 -0.139316210578095
32 -0.142266814163888
33 -0.13939004349248
34 -0.18548041842898
35 -0.199511436747812
36 -0.209608863510652
37 -0.227645284337648
38 -0.276813348671664
39 -0.295399509194279
40 -0.309931293607242
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0193390890784499
1 0.118740653770821
2 0.268607313649586
3 0.310032215226823
4 0.266089780163523
5 0.130624872869362
6 -0.000840340283911445
7 -0.110277385259635
8 -0.203111648102273
9 -0.254412679287867
10 -0.243697559694907
11 -0.270060326541673
12 -0.280290063826905
13 -0.205772149118031
14 -0.0782322065530527
15 -0.00869148067718939
16 -0.00481917482398853
17 -0.0155600274901557
18 -0.0181353912222546
19 0.0239337265016148
20 0.0083437890365623
21 0.028909385776462
22 0.0359813151829238
23 0.0495486941531302
24 0.0346208937522343
25 0.0561295078183974
26 0.0456082184810915
27 -0.0144089479387457
28 0.0146189194801174
29 0.032178761839238
30 0.0299774393339387
31 0.000629678991418636
32 0.0152461928022563
33 0.0207248913029296
34 -0.0167813931782792
35 -0.011114955469302
36 -0.000419840512976499
37 0.0329849012261363
38 0.0450340346043623
39 0.062683801092426
40 0.107068167849836
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0379154875590331
1 0.0940150626626934
2 0.214694064622106
3 0.237777707591928
4 0.175197123102388
5 0.0138787247751813
6 -0.0722082897654861
7 -0.145472168007919
8 -0.228593975661468
9 -0.271528743963045
10 -0.252111308349583
11 -0.308877905906162
12 -0.264571222286416
13 -0.218373212681779
14 -0.102528812271482
15 -0.0676885546827419
16 -0.0600642207854003
17 -0.0764089474339809
18 -0.0590647203307322
19 -0.0404209585865116
20 -0.0456802032431645
21 -0.0209249260828361
22 -0.0341269243909936
23 -0.048249043644641
24 -0.072898874063382
25 -0.0773848905658889
26 -0.0722919074534358
27 -0.0986095648881209
28 -0.084692257113665
29 -0.0995912954943758
30 -0.115289747035723
31 -0.137871314946069
32 -0.147556852076324
33 -0.17074144496502
34 -0.200723311071418
35 -0.203282529535326
36 -0.214535706346584
37 -0.216782425171608
38 -0.22208594450759
39 -0.244760741604594
40 -0.234697638580819
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.00649306074044098
1 0.139534622574858
2 0.292430927955922
3 0.303638393587164
4 0.221705029958322
5 0.0871614363065447
6 -0.0152081577928644
7 -0.0960949927353703
8 -0.212566215566245
9 -0.270909451466466
10 -0.221674983915818
11 -0.272668932674085
12 -0.281917078596056
13 -0.205691297811455
14 -0.072223339569752
15 -0.0201951028772598
16 -0.0278241647738566
17 -0.0483538745206094
18 -0.0381974278740458
19 -0.0530910190549854
20 -0.0848914334351276
21 -0.0967745069940209
22 -0.109752396972629
23 -0.116745172025726
24 -0.151315149753192
25 -0.170605216445163
26 -0.192246423363206
27 -0.191030775175147
28 -0.199805996975929
29 -0.227129116769522
30 -0.249119898691499
31 -0.264605004307498
32 -0.283492233499279
33 -0.297296327178085
34 -0.322043668914944
35 -0.347510808519893
36 -0.35889664181894
37 -0.37466199778256
38 -0.379957490840884
39 -0.412278182939287
40 -0.418667472777503
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0572522936208104
1 0.0878448654069688
2 0.230014657471737
3 0.240240285116763
4 0.176733425563454
5 0.037965152996378
6 -0.0850656279665003
7 -0.166539355409153
8 -0.244607899309927
9 -0.26968581409928
10 -0.228761267599388
11 -0.236943464503252
12 -0.181221264980774
13 -0.121754586423269
14 0.00899467512800367
15 0.0739088372809205
16 0.0960304974808981
17 0.109469358780815
18 0.118517712872878
19 0.143123212876258
20 0.145000027942395
21 0.170438256310399
22 0.189744848279395
23 0.229274735996327
24 0.242026439635167
25 0.242978081112136
26 0.27081489358772
27 0.251780550771647
28 0.299209314567578
29 0.310606072360266
30 0.340637041558396
31 0.352371511354495
32 0.395756175342459
33 0.485881251804926
34 0.53346457907988
35 0.606257785899809
36 0.665546484935924
37 0.760764529798858
38 0.79877383603472
39 0.850769503389887
40 0.877948195701176
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.00682145015341451
1 0.127997698141892
2 0.268890612904571
3 0.308581077212657
4 0.248513941251666
5 0.113259692597661
6 -0.0156156814031787
7 -0.095169303480958
8 -0.179010068153337
9 -0.22248751437705
10 -0.181957532993589
11 -0.251744112304342
12 -0.2517665658677
13 -0.223233931964563
14 -0.122243494151235
15 -0.0369044253479123
16 -0.030725550179997
17 -0.0185324017665227
18 0.00957200697461946
19 0.0270867438946327
20 0.012510732860104
21 0.0419921711140754
22 0.0336611099480981
23 0.029684255691719
24 -0.00558124630561352
25 -0.0146885703398363
26 0.00160721487373561
27 -0.0279115574072621
28 0.019436992927937
29 0.0250525843542757
30 0.00204672745244228
31 -0.0296007754067995
32 -0.0234052983588926
33 -0.0391944671893398
34 -0.0774690936395563
35 -0.0663046347030054
36 -0.0570640412295553
37 -0.0617200070476152
38 -0.0939912889262606
39 -0.134129665033612
40 -0.13082946331313
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0128826517800089
1 0.137309679339298
2 0.283322866739793
3 0.31291630730511
4 0.238992060049695
5 0.0875182036884166
6 -0.0448677982573225
7 -0.140102400951628
8 -0.231886094306447
9 -0.338354574270708
10 -0.340219719604474
11 -0.405547305089702
12 -0.386234950101043
13 -0.332361497888782
14 -0.204190760693387
15 -0.135762690196963
16 -0.129138501066264
17 -0.141168827029102
18 -0.0998373856281161
19 -0.0919234302964931
20 -0.0783337437639178
21 -0.0538987779955491
22 -0.0750188187441383
23 -0.0535333606493973
24 -0.0706128847277627
25 -0.0722821144292141
26 -0.0568962384686058
27 -0.0682762298812749
28 -0.0512993679920752
29 -0.0495213743756224
30 -0.0310250077913876
31 -0.0336939151048332
32 -0.0388919105067771
33 -0.0172270320361871
34 -0.0206715792489911
35 -0.0152993732686291
36 -0.00888499121112485
37 -0.0160612486333038
38 -0.0104411464368441
39 -0.0181931891456841
40 -0.00770527765075091
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0351281122747356
1 0.093281594701085
2 0.251692235944049
3 0.288824683303003
4 0.218855849603962
5 0.0733937645044316
6 -0.0607718024336386
7 -0.150171008315152
8 -0.232649277963547
9 -0.305776202933434
10 -0.314732869217633
11 -0.369065975844635
12 -0.357554893089004
13 -0.324949822895016
14 -0.194244501311402
15 -0.139355806648842
16 -0.134301757363282
17 -0.132333975495258
18 -0.115699724210397
19 -0.116207806919278
20 -0.105685832374849
21 -0.0909924042858581
22 -0.0893277757639064
23 -0.0822505987522719
24 -0.0776316056980999
25 -0.0665141543065237
26 -0.0604679452372769
27 -0.0463934109164699
28 0.030406671349918
29 0.0377313659417817
30 0.0779569824235828
31 0.0645736908607031
32 0.048198956959534
33 0.052993904735839
34 0.135197810244556
35 0.196500045937809
36 0.268831276478535
37 0.324721394278417
38 0.404820693078518
39 0.479835084785977
40 0.578133863575818
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0421227986733692
1 0.0876780775463848
2 0.226446030919714
3 0.255735986655198
4 0.186020051484119
5 0.016246348706602
6 -0.11278576876689
7 -0.197542372357524
8 -0.289628367246839
9 -0.345955153524103
10 -0.320624417660599
11 -0.376979384311109
12 -0.364451083127399
13 -0.325521066724766
14 -0.1856801753484
15 -0.128224126595841
16 -0.124635664873629
17 -0.105279531678038
18 -0.0951311700223458
19 -0.0857638181366758
20 -0.0819394386020873
21 -0.06242598679039
22 -0.065860422347189
23 -0.0688968920845534
24 -0.0773624775900332
25 -0.0775174213217129
26 -0.058278070896618
27 -0.0220080458855421
28 0.0457335739297431
29 0.0461845000759906
30 0.0652605870483951
31 0.0431615372602012
32 0.0290119387851933
33 0.0869778311224501
34 0.100062592426124
35 0.157745844982412
36 0.195627645003416
37 0.227325328438561
38 0.245330763140198
39 0.249007210284302
40 0.236337387505126
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0769255655442587
1 0.045109495726507
2 0.206644538580794
3 0.251769871540551
4 0.212665775481316
5 0.0637488915262265
6 -0.0542509667487563
7 -0.154177926312684
8 -0.233594138627804
9 -0.309194061933733
10 -0.292433893619713
11 -0.313109631833453
12 -0.294623088417834
13 -0.239737910974561
14 -0.128537804334478
15 -0.047849433736106
16 -0.0709353421239722
17 -0.0800739963544777
18 -0.0422926170946427
19 -0.0238651091984154
20 -0.0404701363922326
21 -0.0145442510306726
22 -0.0245624356963923
23 0.00772551472835481
24 -0.0065490768637968
25 -0.018973315712663
26 -0.00202402787051525
27 -0.0171199325637978
28 0.0282620690667894
29 0.0216799787078497
30 0.00898432945930772
31 0.000274471717924385
32 -0.00804191640725893
33 0.00189252370263482
34 -0.0157469133015598
35 -0.0127515656474975
36 0.0182431573919049
37 0.00617126179783511
38 0.000367515251445738
39 -0.00692062106123537
40 0.0114185387007124
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0504971422387843
1 0.093896952271777
2 0.260997948896071
3 0.300548314279576
4 0.218661223040089
5 0.06634816335617
6 -0.0634004527550731
7 -0.158418328121915
8 -0.24882146757921
9 -0.298527962264795
10 -0.270956124685821
11 -0.323782174855551
12 -0.303806329155026
13 -0.246409938564975
14 -0.126233701680982
15 -0.0761461279683031
16 -0.0847631877595019
17 -0.0937383865562058
18 -0.0589799995872191
19 -0.0330712422265007
20 -0.0620195213202148
21 -0.0511681389485501
22 -0.0642220151015298
23 -0.064513798607873
24 -0.092260462202427
25 -0.0945385954487161
26 -0.07349986797459
27 -0.0835481961852231
28 -0.0466469333620259
29 -0.0415370513575013
30 -0.0450099349464503
31 -0.0658541083368789
32 -0.0843391012031898
33 -0.0798959754684612
34 -0.101083964652716
35 -0.0909035036779127
36 -0.0680292722543534
37 -0.0707641679862636
38 -0.084077991550612
39 -0.102892588092783
40 -0.0856034518464499
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0163992373943156
1 0.114748388974462
2 0.264977294246714
3 0.291065692475184
4 0.210980394524746
5 0.081245571791432
6 -0.0530551843340374
7 -0.131312695797098
8 -0.228839273515221
9 -0.320196561803161
10 -0.323358559313393
11 -0.376110393487786
12 -0.352658948097552
13 -0.307381295816246
14 -0.171630675331962
15 -0.0946055786956723
16 -0.0743841673014307
17 -0.0635369220496971
18 -0.0299392658906452
19 0.00756782396373623
20 0.0124413048386076
21 0.0304342469762977
22 0.0304228101764465
23 0.0364056189135891
24 0.0176454443400811
25 0.0350695303310751
26 0.0657636537500927
27 0.0822948009945152
28 0.138661604411504
29 0.148331887047237
30 0.166910906074591
31 0.153974211942046
32 0.183147709938151
33 0.190469554178304
34 0.179811204483979
35 0.206269197839792
36 0.237139830933274
37 0.249289158544644
38 0.247462729834517
39 0.23472741478295
40 0.277508100675093
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0099717659917955
1 0.119583157067673
2 0.25451585298517
3 0.281131324258369
4 0.215069196132723
5 0.0542626051798081
6 -0.0720529419535572
7 -0.163557450756093
8 -0.267123267850283
9 -0.329345453271849
10 -0.309844023818028
11 -0.368510941424129
12 -0.357991782065798
13 -0.316543779665174
14 -0.16719707324452
15 -0.0991941701823169
16 -0.100326922332691
17 -0.123877465918456
18 -0.113534243974986
19 -0.0985959607885123
20 -0.105626899327304
21 -0.0785239503934863
22 -0.0751839969421653
23 -0.0765509082940454
24 -0.123581596597228
25 -0.117697303652461
26 -0.116585633110298
27 -0.123991217071319
28 -0.0980894525920641
29 -0.0687129584808908
30 -0.0576142460785078
31 -0.0961605303415016
32 -0.0750638895595568
33 -0.0802140243590319
34 -0.0749316640300703
35 -0.0503063330388311
36 -0.0401228734366477
37 -0.025123960995967
38 -0.0313749842792177
39 -0.0222265864487206
40 -0.00436323012720319
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0267327618780344
1 0.112523455078297
2 0.270816382660159
3 0.285222003421358
4 0.221329793404784
5 0.0737598046293142
6 -0.0149006064368642
7 -0.0801041417233614
8 -0.187794192020149
9 -0.264852613183757
10 -0.300708944863615
11 -0.29913275748063
12 -0.289510989198592
13 -0.265305146938213
14 -0.137309702005767
15 -0.0937179974217832
16 -0.0842212202920267
17 -0.0863369015931807
18 -0.0605918289350758
19 -0.0687178967043645
20 -0.0747144532908113
21 -0.0580736641424489
22 -0.0754730915277122
23 -0.072860660802597
24 -0.0813023506465171
25 -0.0702921798618101
26 -0.0527205855511914
27 -0.0399100250898279
28 -0.0275522188091459
29 -0.0338234215345636
30 -0.0369081269291502
31 -0.0442775673650146
32 -0.0234268156846946
33 -0.0416386244701679
34 -0.0680968450547388
35 -0.055875642596896
36 -0.0473486938807213
37 -0.0420985595781174
38 -0.0397657699087501
39 -0.0520149456180299
40 -0.0193338540179333
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.00476737873304689
1 0.139791005294267
2 0.280612936837437
3 0.312578105907228
4 0.242477299776209
5 0.113750150722488
6 -0.00938880705167922
7 -0.0777873107252267
8 -0.186084995086422
9 -0.271292738959644
10 -0.258088258748634
11 -0.309844706493673
12 -0.264922070422636
13 -0.230046794274326
14 -0.0996337616440988
15 -0.0323945964650312
16 -0.0307667882578349
17 -0.0347684759252251
18 -0.00916105856520222
19 0.000744069660447266
20 -0.0188446297688731
21 -0.0238113504591695
22 -0.0117552239710275
23 0.00571354165121285
24 -0.0234612713132423
25 -0.000272671537326907
26 0.0074639768360143
27 -0.017375113536958
28 -0.00404529318542401
29 -0.00388595909344769
30 -0.00064092844913155
31 -0.0272871513604542
32 -0.0134883817926097
33 0.00797691246016807
34 -0.0225560011019086
35 0.00337089633716126
36 0.00467716123454931
37 -0.003960388742553
38 -0.0222186617117641
39 -0.0418274020791989
40 -0.00591798522528819
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0307081597325523
1 0.102600348102261
2 0.259537407990994
3 0.279171751288636
4 0.218374048351068
5 0.0830560272396275
6 -0.0357907556083328
7 -0.0921372058160497
8 -0.158029833716504
9 -0.212643223927595
10 -0.214935809941184
11 -0.264620536344047
12 -0.270415606892481
13 -0.232159141177299
14 -0.138787133096089
15 -0.0840570307502988
16 -0.0825580372769128
17 -0.0734648203478168
18 -0.05314039635231
19 -0.0338496632640588
20 -0.0300478339034091
21 0.000686235771843791
22 0.0098562700683491
23 0.0420520573919498
24 0.0201141530901143
25 0.0336266854341947
26 0.0585838621282377
27 0.0256675626707201
28 0.0529726757177897
29 0.0612720049749065
30 0.0825561863767659
31 0.0659163832975524
32 0.0891175826232109
33 0.119483145287388
34 0.105289540781097
35 0.128476728594651
36 0.156208231929224
37 0.182503079260856
38 0.189646155655538
39 0.176292035395976
40 0.185397330720876
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.055304949784075
1 0.0805302981120084
2 0.202435932472707
3 0.226909935986828
4 0.156741191817662
5 -0.012160175074837
6 -0.132889488792373
7 -0.224077673353048
8 -0.304955580394775
9 -0.384183479851636
10 -0.365347736240915
11 -0.402334308313187
12 -0.371150779853861
13 -0.357348183229425
14 -0.243541541369014
15 -0.182257815412828
16 -0.150506730902841
17 -0.148815409027653
18 -0.106410209628551
19 -0.0788695385437732
20 -0.0770131461611001
21 -0.0764406154115393
22 -0.0699300866033301
23 -0.062907841659297
24 -0.0777345938727541
25 -0.0860208916755374
26 -0.0761931044741235
27 -0.0732303129059106
28 0.019520463551145
29 0.0387436357573812
30 0.0440198474858073
31 0.039558537774611
32 0.0522330893451697
33 0.0719930148608077
34 0.0435762478854844
35 0.0545819046570877
36 0.0830774037051771
37 0.0681714471884289
38 0.0735208590472274
39 0.0802499493983237
40 0.0751736884978653
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0170832600979143
1 0.142218493271065
2 0.303286033306023
3 0.327694123181181
4 0.272051723506734
5 0.128413377671983
6 0.00264405143105595
7 -0.0694602612302244
8 -0.14882725634855
9 -0.194678741748011
10 -0.188275389349674
11 -0.229997356682277
12 -0.199424288306215
13 -0.148242508772447
14 -0.0129227060629944
15 0.0827259278945398
16 0.0828685503107733
17 0.0824895474063387
18 0.0817109336504167
19 0.0742462490414191
20 0.0795007791910933
21 0.0568981000839832
22 0.0483228047689712
23 0.040190183644472
24 0.0192654368226028
25 0.0344744151029621
26 0.0377585426144256
27 0.0409924791461371
28 0.0674020097140007
29 0.0532258542184216
30 0.030506545723255
31 0.0144729997952897
32 -0.00101982433609837
33 -0.0170559595558961
34 -0.0355169976246659
35 -0.0257189781053757
36 -0.042445635367887
37 -0.0413012375992494
38 -0.0374446544464462
39 -0.0436403641182288
40 -0.0487024483600846
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0784918435498465
1 0.0413998515018976
2 0.209389487094947
3 0.230549379623159
4 0.174497630076559
5 0.021353276001987
6 -0.119719093148424
7 -0.204264631679288
8 -0.256801776051184
9 -0.329635051041229
10 -0.338246461315825
11 -0.396773890091909
12 -0.392029192022296
13 -0.334879716702315
14 -0.192898245306738
15 -0.116678286632695
16 -0.132790070754318
17 -0.118795322677595
18 -0.0874758549359766
19 -0.0577896792348849
20 -0.0622165891791902
21 -0.0455282289917882
22 -0.0433781148587089
23 -0.0401745620501801
24 -0.065288046398754
25 -0.0653136655506659
26 -0.0630555247843487
27 -0.0807514845384771
28 -0.0563426873978461
29 -0.0254985812087867
30 -0.0240422894082952
31 -0.0433167259355463
32 -0.0441558612126576
33 -0.0336440260220483
34 -0.056355611254812
35 -0.0681600060878624
36 -0.0604154267126082
37 -0.0571221472618033
38 -0.0590368596521866
39 -0.0747366639483067
40 -0.0626778205728966
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0355302374631217
1 0.077293154991108
2 0.22704073574558
3 0.252929412671307
4 0.185808316191909
5 0.0618620793345031
6 -0.072052619137092
7 -0.164335798894255
8 -0.231766776497641
9 -0.29229404468275
10 -0.259754782065445
11 -0.294934801322921
12 -0.274335213111198
13 -0.239938143908703
14 -0.0999192509353639
15 -0.0338617292922105
16 -0.0250870556718796
17 -0.0230626113049555
18 -0.00391342074265388
19 0.00364051193295811
20 -0.025817305457541
21 0.00406749048631028
22 0.036490901593587
23 0.0586647616191236
24 0.0487754405728174
25 0.0358291584003334
26 0.0654281622889439
27 0.0345155453178654
28 0.0869965573478853
29 0.0974816652207968
30 0.138539026348194
31 0.117852673840835
32 0.0953034556763752
33 0.122183202659454
34 0.0822515092659817
35 0.0428032338309201
36 0.0679548656933529
37 0.11069664674781
38 0.150076647410435
39 0.197417836615854
40 0.304713033616939
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.000849350230280876
1 0.123083457565185
2 0.2828481854473
3 0.30281295438163
4 0.237709850365325
5 0.0803987866831086
6 -0.0504606864835813
7 -0.130215395704116
8 -0.209786304061907
9 -0.259700455288326
10 -0.228087133831004
11 -0.275140196101724
12 -0.220739743141851
13 -0.166087403648473
14 -0.0433860657584813
15 0.0201945048530465
16 0.0448138955005559
17 0.0581644604401346
18 0.0701012768332712
19 0.0677979892649283
20 0.0908636077396894
21 0.0893023815791318
22 0.0890045922849865
23 0.0971624172483576
24 0.0923774405210764
25 0.100372376854853
26 0.0961246583152224
27 0.0894134601358543
28 0.11727757859715
29 0.12445258234451
30 0.133833935456698
31 0.106535126250313
32 0.10242635525064
33 0.117322698972702
34 0.0865694177428891
35 0.11119700056546
36 0.128563996376854
37 0.144445698290236
38 0.144566279713445
39 0.159776164321891
40 0.175591457346004
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0366264592459435
1 0.0788411636729149
2 0.223536062922407
3 0.243330960281883
4 0.164198275451469
5 0.0190788045928167
6 -0.122145527301037
7 -0.224927703359068
8 -0.305550453185844
9 -0.338361452522822
10 -0.336426686755405
11 -0.362255185954842
12 -0.3534387695175
13 -0.31938075114062
14 -0.212249754919643
15 -0.114986762548001
16 -0.0986432339034868
17 -0.0728876521769335
18 -0.067037487508923
19 -0.0542267522866364
20 -0.0238805535586479
21 -0.0120146397207579
22 -0.0116569533403634
23 -0.00891226976956538
24 -0.0319068312486719
25 -0.0237235552680355
26 0.00282568864790012
27 0.00724657080469626
28 0.0246595280447472
29 0.0414561416566022
30 0.0221678988361269
31 -0.0178382010252038
32 -0.00584193811030875
33 -0.0111426167987867
34 -0.0342172637023932
35 -0.0280063468387857
36 -0.00039467132393245
37 -0.000468055830278757
38 0.0266942143667706
39 0.0116601501828333
40 0.0301090481581587
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0426105855170213
1 0.0771487138629823
2 0.215297683037322
3 0.269879079075354
4 0.208591104136558
5 0.0715782003405145
6 -0.0527792561726876
7 -0.145557613301157
8 -0.244247951122722
9 -0.298615378494334
10 -0.274317903888066
11 -0.334945989444886
12 -0.335481597031515
13 -0.287015421180243
14 -0.170272626144769
15 -0.0887042051221139
16 -0.0911562137542168
17 -0.0867461596577872
18 -0.0819743842491283
19 -0.066816788298488
20 -0.0698812265033979
21 -0.0565706838438444
22 -0.0537096338253917
23 -0.0395907976430161
24 -0.0570425745875234
25 -0.0520820932670283
26 -0.0509809662175513
27 -0.0821048414535426
28 -0.0626860712936468
29 -0.068223245539774
30 -0.0765032744399416
31 -0.116014378519487
32 -0.118443985375829
33 -0.117374959676694
34 -0.141395388635257
35 -0.147474852041007
36 -0.107291970335292
37 -0.115380528625394
38 -0.13796704328201
39 -0.142708667321953
40 -0.115529120233896
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0174847002674783
1 0.119599351472238
2 0.277371708919866
3 0.312886597885506
4 0.268105000408493
5 0.135517767017855
6 0.0244280762756253
7 -0.0580996989312741
8 -0.123546147420218
9 -0.201435757529013
10 -0.185056931666557
11 -0.226779089871644
12 -0.20419399700754
13 -0.178756287004962
14 -0.0432584137034633
15 0.0255262855453271
16 0.0245776608605839
17 0.025100782886236
18 0.0554155081612411
19 0.082010574465496
20 0.0863659492196733
21 0.109703238276706
22 0.113828897542799
23 0.0998988388914173
24 0.0918330426990623
25 0.0994417755515595
26 0.111452506438297
27 0.0849239938809374
28 0.116616890923763
29 0.125190577958439
30 0.148648157724719
31 0.141259149801827
32 0.164385987871322
33 0.181961105682037
34 0.166888591792786
35 0.190226997843293
36 0.20113245800229
37 0.22784302277091
38 0.246665694699027
39 0.235708916758105
40 0.25284533193984
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.00709334258952765
1 0.142130935262006
2 0.284345740816239
3 0.303803824079935
4 0.243863913512225
5 0.126681890829213
6 0.024384887201526
7 -0.0472973454922139
8 -0.122137408726121
9 -0.157033941721887
10 -0.157761547741384
11 -0.20672217211688
12 -0.159259675156012
13 -0.107006509722246
14 0.0114384872332085
15 0.0996525660574425
16 0.104804068080906
17 0.109102224066069
18 0.142901923209119
19 0.155075063540408
20 0.161502733678122
21 0.183911169888916
22 0.160204794349892
23 0.182089882546542
24 0.169960853679687
25 0.188007519215248
26 0.22068408313705
27 0.240191989649616
28 0.26651688092748
29 0.286105577117518
30 0.308477272853349
31 0.300341620972516
32 0.304227144759296
33 0.320693888953953
34 0.310565839487973
35 0.320853745142029
36 0.360502065007292
37 0.399554000075115
38 0.416507373610504
39 0.458142550371067
40 0.474421245131251
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.00615272554936297
1 0.13072329924187
2 0.283707911099223
3 0.297220054877596
4 0.22241956770064
5 0.0971448998072431
6 -0.00633816473172377
7 -0.0839347541233826
8 -0.160095504138495
9 -0.194064647427582
10 -0.181590305667124
11 -0.263060031412866
12 -0.246010460470303
13 -0.203367579812439
14 -0.0773979443190882
15 0.00534538468297097
16 0.022866962497158
17 0.00616209918199573
18 0.0158605099169922
19 0.00303548251184971
20 0.0187427292360702
21 0.0513598045885812
22 0.0518400648409827
23 0.0584449188993545
24 0.0362038285912032
25 0.05397632550231
26 0.0712050211003952
27 0.0471829856328876
28 0.0861270429396139
29 0.0936690846457688
30 0.0992535889509698
31 0.0844522822346185
32 0.0793963529800061
33 0.0956315490867823
34 0.0487009234760416
35 0.0265274404797378
36 0.0620858974461189
37 0.070130353166153
38 0.103104647144923
39 0.115728870542244
40 0.200832265718261
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0310013615672888
1 0.145904224020037
2 0.290072395315657
3 0.325142530181399
4 0.252225987146555
5 0.106173682909757
6 -0.0370149034141773
7 -0.132856351247143
8 -0.216157174798479
9 -0.268514215960724
10 -0.262328863362039
11 -0.278473155736033
12 -0.262649006179831
13 -0.204215459910269
14 -0.074754761630305
15 -0.00687722699799487
16 -0.00234015584525515
17 -0.00811527176189752
18 0.0181890803712337
19 0.0370916956120366
20 0.0425559834710043
21 0.077407810588749
22 0.0763680466077359
23 0.080014629745822
24 0.0667816328937487
25 0.0800537363755662
26 0.0873185763991939
27 0.0726285325842673
28 0.109085436595534
29 0.108788652346891
30 0.125201334831088
31 0.118703296117721
32 0.11579595947173
33 0.129809797118573
34 0.114565559323775
35 0.14314263039796
36 0.179822985463339
37 0.203453316358455
38 0.246510995108902
39 0.286827122486649
40 0.332011151478525
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0259020245162089
1 0.0999508093447776
2 0.250292161444479
3 0.282600224082889
4 0.225390870474418
5 0.089108679792071
6 -0.0420760195906285
7 -0.132267812535999
8 -0.197718064190015
9 -0.263291649491784
10 -0.263081963011055
11 -0.278978734738712
12 -0.252409390100397
13 -0.22242710478772
14 -0.110157687379708
15 -0.064721194222348
16 -0.0556787042650457
17 -0.057718907906823
18 -0.0513142108421638
19 -0.0326303715449203
20 -0.0196771361662531
21 -0.0221731884886243
22 -0.0122952859412235
23 -0.00660438793412332
24 -0.0128209146441369
25 0.00228496318810301
26 0.00560987865082296
27 0.00830340364741566
28 0.0243134715218689
29 0.0238966825458533
30 0.023024681506195
31 -0.00200922649132274
32 0.00345504220247328
33 -0.00424699975842557
34 -0.037090217419693
35 -0.0324738577385819
36 -0.0103365206098376
37 -0.0261357624557839
38 -0.0264796866621344
39 -0.0193477394429076
40 -0.00825835003443842
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.00839395707343282
1 0.133981803101247
2 0.27020889019059
3 0.320277502184992
4 0.265778406116067
5 0.134340601051409
6 0.0227307197012445
7 -0.0286681146841214
8 -0.11343556282799
9 -0.160511092793088
10 -0.120776550010052
11 -0.152904101631582
12 -0.12474048361236
13 -0.0681209324812118
14 0.0491031933688726
15 0.161440124019377
16 0.151929797970669
17 0.150212457886508
18 0.160600595999941
19 0.1474708066382
20 0.133937694829031
21 0.144788289550164
22 0.129623325017773
23 0.116028808114702
24 0.0852484076680318
25 0.0877915216471994
26 0.107986710280791
27 0.108592284953381
28 0.158561231389156
29 0.159356764349997
30 0.165281277545053
31 0.135724544045089
32 0.14606937338126
33 0.161833519220859
34 0.122932849694039
35 0.11390444974885
36 0.154565578351966
37 0.192225359883346
38 0.212636043565454
39 0.208349798011753
40 0.240015963183761
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0247237234142448
1 0.100055196239856
2 0.249091817580301
3 0.266976991841132
4 0.219066719036362
5 0.0735405195995433
6 -0.0256792607633853
7 -0.0844200490512828
8 -0.132169107549874
9 -0.202208872213945
10 -0.217358280476263
11 -0.231520151216231
12 -0.23944789006998
13 -0.229815022700545
14 -0.112551618065623
15 -0.0465874923958411
16 -0.037518930065481
17 -0.0404572117235018
18 -0.00151243096323395
19 0.0223896846895366
20 0.0314512486787484
21 0.0770052158260306
22 0.0834702386031116
23 0.0962780816733355
24 0.0888880327744976
25 0.0958546325142766
26 0.124123891181852
27 0.0848702424827641
28 0.10501605739033
29 0.11549991997973
30 0.109419147701793
31 0.0903164648716652
32 0.103359568466446
33 0.12310990075674
34 0.111902987638563
35 0.111921472323694
36 0.123157073060716
37 0.141703022010084
38 0.158476854107412
39 0.168603312283008
40 0.186961842910972
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.083116452111728
1 0.0323132257229828
2 0.168877276906882
3 0.195073452800774
4 0.13171438835366
5 0.0148591883847038
6 -0.100021152368427
7 -0.184728676591048
8 -0.28252293515076
9 -0.33152598567948
10 -0.301610030592518
11 -0.322034610659716
12 -0.28228102790285
13 -0.232295168073017
14 -0.0964118141025558
15 -0.0209032102202054
16 -0.036083314755464
17 -0.0355013511626039
18 -0.0566290648080088
19 -0.0826128200332947
20 -0.0963706050689801
21 -0.105171582368075
22 -0.113736662717822
23 -0.124000777930917
24 -0.134693840120288
25 -0.141353678486944
26 -0.164279715377099
27 -0.193133247621212
28 -0.176541265486864
29 -0.207141409129931
30 -0.214839875087163
31 -0.234308112323322
32 -0.244061754755942
33 -0.244313348203981
34 -0.2876998534063
35 -0.313923290441357
36 -0.324733466449763
37 -0.323658777610877
38 -0.371968227253817
39 -0.421968193951302
40 -0.437238680635534
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0324050365983641
1 0.0968604947272382
2 0.250256986256685
3 0.272669667854949
4 0.236710573211358
5 0.11305269035214
6 0.00625988769232411
7 -0.0579645721615849
8 -0.134821412785104
9 -0.203123929500222
10 -0.20996300372808
11 -0.25675763369425
12 -0.237192583978923
13 -0.194763432408654
14 -0.0628844009285761
15 0.0221899793574112
16 -0.00939136932962104
17 -0.0308275792191166
18 -0.00639078583139518
19 -0.00484270186701785
20 -0.0261217679146561
21 -0.00839775830137501
22 -0.0262904304914384
23 -0.0199656675879156
24 -0.0359821561573135
25 -0.0595189984452844
26 -0.0658404791595046
27 -0.0900582247438964
28 -0.0606465804351002
29 -0.0788982033769905
30 -0.0963036806514239
31 -0.135180483064697
32 -0.164018623767319
33 -0.177385174672436
34 -0.207483839209995
35 -0.246773227299617
36 -0.242864423101345
37 -0.265922009349183
38 -0.311308206912707
39 -0.335443161710631
40 -0.333761102334652
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0247391951690474
1 0.103623301011813
2 0.246941459823558
3 0.274453524530839
4 0.217844780771814
5 0.0737836484679466
6 -0.0439949138464346
7 -0.12425862027142
8 -0.21978924559101
9 -0.28976623629417
10 -0.258635104275958
11 -0.304998415122456
12 -0.285148928201825
13 -0.223695622464418
14 -0.113554857893289
15 -0.0448171759881513
16 -0.0665151881371191
17 -0.0752081974894168
18 -0.0765256695948064
19 -0.0531276113007717
20 -0.0614611556112745
21 -0.0662258407926162
22 -0.0799959214922499
23 -0.0677767141420409
24 -0.0922452460194227
25 -0.106777759036862
26 -0.107241464685695
27 -0.122055925208084
28 -0.0921456095013715
29 -0.0850318895330346
30 -0.0886859412653056
31 -0.115213098112839
32 -0.135917328167812
33 -0.137270865743466
34 -0.173379626949083
35 -0.210200549730774
36 -0.215400453772578
37 -0.228832076193061
38 -0.261637374494077
39 -0.306050632594091
40 -0.322701942845764
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0453342787565747
1 0.0940184357583815
2 0.216041512193985
3 0.238910685980696
4 0.198115170468124
5 0.0707501749550348
6 -0.0515977949791031
7 -0.134727330306172
8 -0.218383748358957
9 -0.299184147125072
10 -0.259346105498171
11 -0.30483557342444
12 -0.271135285864535
13 -0.295335639518815
14 -0.159326916923659
15 -0.0819715810887578
16 -0.0978511133672466
17 -0.130721466034674
18 -0.115562519190282
19 -0.114761278501534
20 -0.158550772839765
21 -0.139299672273276
22 -0.134814618244535
23 -0.133420928988691
24 -0.135365709754507
25 -0.151298040740936
26 -0.145402984802712
27 -0.138490023587135
28 -0.113043852112708
29 -0.14226727514901
30 -0.15645295326526
31 -0.158267400287283
32 -0.182712447230856
33 -0.185733214962973
34 -0.207811208682104
35 -0.261171429174206
36 -0.269275988333492
37 -0.296634532019173
38 -0.332458255674327
39 -0.349069771276194
40 -0.352306978926512
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0517356806109825
1 0.0638509908286649
2 0.217881538550391
3 0.236952973602519
4 0.188356943469858
5 0.0650207237112861
6 -0.0564534677270538
7 -0.138905552189891
8 -0.231261840330228
9 -0.301906594586407
10 -0.283023834851147
11 -0.361084303839858
12 -0.320712458515013
13 -0.295522835359839
14 -0.178644069773062
15 -0.0977623909247152
16 -0.108667821719452
17 -0.0946514982689193
18 -0.0707965058953626
19 -0.0565311144479237
20 -0.0647067761371058
21 -0.067609178608647
22 -0.0699083572794859
23 -0.0786587270645702
24 -0.0895694756190322
25 -0.0883302908026868
26 -0.0725514303181685
27 -0.105901063770218
28 -0.0716862546250434
29 -0.0618016663365335
30 -0.0674324872637957
31 -0.0941966380326988
32 -0.0970959477717273
33 -0.101261896541158
34 -0.111632473524854
35 -0.107972088885915
36 -0.087942493704654
37 -0.103005503365367
38 -0.116548014343694
39 -0.118381525810658
40 -0.0860431242230675
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0167328390669219
1 0.147741105052469
2 0.288722344858669
3 0.311188358344176
4 0.223198902837839
5 0.0984529170549537
6 -0.0321150008475355
7 -0.118729493179495
8 -0.216217036102976
9 -0.302760532110248
10 -0.27296416141154
11 -0.307814892229502
12 -0.305792277680454
13 -0.266901675553903
14 -0.143551117462072
15 -0.0811311741713459
16 -0.0988110946105447
17 -0.117630880142749
18 -0.0844193453494988
19 -0.0756141805965864
20 -0.0823798902917874
21 -0.0759499661787482
22 -0.11837903355695
23 -0.13949398179702
24 -0.196089891711531
25 -0.24020156936184
26 -0.246889143635017
27 -0.29294338305965
28 -0.290501393012779
29 -0.315285332974741
30 -0.343447933171956
31 -0.399606269979886
32 -0.442759437825749
33 -0.482396589600849
34 -0.559854804687188
35 -0.623598997394149
36 -0.669359210741583
37 -0.729279176914048
38 -0.774278768669021
39 -0.820285980181216
40 -0.880822586166643
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0832768152240675
1 0.0187620476497408
2 0.157579668066409
3 0.183548877726694
4 0.141100605810182
5 0.025376333777162
6 -0.0774541344422124
7 -0.166793576372911
8 -0.236193122475383
9 -0.27231273707686
10 -0.236143803594011
11 -0.281836634063648
12 -0.250347063746063
13 -0.209553528109947
14 -0.101886502859007
15 -0.00291526509177054
16 -0.00159688045612771
17 -0.0275716475653578
18 -0.00238040529112205
19 0.0230140571855824
20 0.00835378520076979
21 0.0186695995012984
22 0.0225295172005238
23 0.0187427580570265
24 -0.0105817561825861
25 0.0140472037865136
26 0.0286255440021268
27 -0.00592623926985514
28 0.0580863982590385
29 0.0637937943104854
30 0.0527779366298153
31 0.0169029104550145
32 0.00317335508482852
33 0.0178466580070697
34 -0.038439714227585
35 -0.0373149898376024
36 -0.00740242049512041
37 -0.00852103304618446
38 -0.0374809736461863
39 -0.0577386736679522
40 -0.0351962544391267
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0350719005753684
1 0.0777700981116158
2 0.225217636438098
3 0.259536988019255
4 0.170030869222504
5 0.0309081194591814
6 -0.080691133957278
7 -0.135992434262746
8 -0.212632789332202
9 -0.291572523415424
10 -0.27288181178793
11 -0.316595831758653
12 -0.261300856847001
13 -0.208773262016172
14 -0.0620749775904246
15 -0.00816012259016308
16 -0.0109706370559461
17 -0.00631634667832515
18 0.0161176974149155
19 0.0347676443401692
20 0.040498976424292
21 0.0642519631911158
22 0.0680103825861815
23 0.0915257180338447
24 0.0631616399553812
25 0.0729998816096735
26 0.105945796805391
27 0.0946825658509578
28 0.125863600256509
29 0.147331894122958
30 0.136097602388605
31 0.126618336717841
32 0.132627131334321
33 0.159439488978182
34 0.139713691874452
35 0.133873615069247
36 0.152537437370681
37 0.162534098738815
38 0.153059982478891
39 0.145991881719288
40 0.169544202844602
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.00871944955920601
1 0.116219657665166
2 0.252030395733646
3 0.284154161246934
4 0.212517014816594
5 0.067617383641668
6 -0.0531252623800826
7 -0.170137232686276
8 -0.253321344595781
9 -0.30777455956016
10 -0.308214559928333
11 -0.345921830104333
12 -0.326403064056195
13 -0.298283945722372
14 -0.160586790565814
15 -0.0638375632586934
16 -0.0620853586307391
17 -0.0545756072702313
18 -0.0267338120361389
19 -0.00675296090798305
20 0.003395040367554
21 0.00306707851818189
22 -0.00854892569777732
23 0.00330922561706792
24 -0.00682204576135881
25 -0.010375153613027
26 -0.00135932489973989
27 -0.0266579980182815
28 -0.0233959045359997
29 -0.0257391421962927
30 -0.00791327242516093
31 -0.0340062962132315
32 -0.0375029589793696
33 -0.0350858436614674
34 -0.0463378558210774
35 -0.0413647787974156
36 -0.0171200456661023
37 -0.020436488418822
38 -0.0299041792891215
39 -0.0492544280403955
40 -0.0493398422471385
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0459019076016798
1 0.0949839544327631
2 0.241576967364868
3 0.284576590245709
4 0.214595263602532
5 0.0864672966467959
6 -0.0268434661394377
7 -0.107620226425143
8 -0.164535161518129
9 -0.221431201402627
10 -0.234130390024422
11 -0.257864308855665
12 -0.239041422726045
13 -0.171936357322132
14 -0.0507850579634539
15 0.00748371047460061
16 0.00954170305678392
17 0.00728751186833154
18 0.0194971422243011
19 0.0447458708542232
20 0.0502248913906858
21 0.0522487370244633
22 0.0666296647776017
23 0.0814038687729619
24 0.0893545006030481
25 0.104699480254976
26 0.110902877425578
27 0.111079142155791
28 0.167391219431184
29 0.18097091081455
30 0.197085571147108
31 0.17830033308841
32 0.207862974768356
33 0.244169454000972
34 0.270934289409556
35 0.309530987532828
36 0.364992303423938
37 0.410936995936829
38 0.431795350038875
39 0.46676833372193
40 0.522918496750486
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0388377044335577
1 0.0582258814125529
2 0.219734153470552
3 0.262473312324595
4 0.189991775733244
5 0.0481402800927908
6 -0.0773587252342134
7 -0.177732953550803
8 -0.274730323261228
9 -0.346564123705287
10 -0.332767249848255
11 -0.390626401624997
12 -0.394449612515309
13 -0.373278359614384
14 -0.220802148451195
15 -0.146525230473736
16 -0.152045750474167
17 -0.138963461673701
18 -0.115161027832295
19 -0.103153125256869
20 -0.0661151323592639
21 -0.0560576238495951
22 -0.0390291103053837
23 -0.0209518597833203
24 0.0158951703497987
25 0.0325847315813119
26 0.0770494718013461
27 0.143159868831796
28 0.190299792964172
29 0.22095918341833
30 0.232684013555892
31 0.281415537781897
32 0.293543627603321
33 0.279844717684591
34 0.281080416538801
35 0.297796448853977
36 0.322595237441876
37 0.340509925041462
38 0.361735931530727
39 0.340427900295013
40 0.345833043580408
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.00735433339553548
1 0.125441019095872
2 0.264353866085925
3 0.297689061017638
4 0.238228529795607
5 0.0995058971064013
6 -0.0430524935161589
7 -0.141356006991421
8 -0.227810188562506
9 -0.280557459456771
10 -0.26729255947271
11 -0.320816420291732
12 -0.317901953959481
13 -0.285107531705588
14 -0.159080573180932
15 -0.0576808056131961
16 -0.0624608089165726
17 -0.0679835051388151
18 -0.0455332712685683
19 -0.025057209268911
20 -0.0208393996097493
21 0.0100615208048129
22 0.0289271445303392
23 0.0351123341448236
24 0.0244037437164399
25 0.0410119532831219
26 0.0573688955571932
27 0.0561274174762376
28 0.105399182345574
29 0.128295254550492
30 0.142311995759463
31 0.154495147162753
32 0.170332776798516
33 0.200503907137801
34 0.19470006313142
35 0.212536965578402
36 0.221528503589913
37 0.228845957245877
38 0.233956323848281
39 0.259637991013938
40 0.303687030300956
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0504968653621036
1 0.0854697635962589
2 0.199296574156469
3 0.219856709710663
4 0.169163734025215
5 0.0358705402383128
6 -0.0788109069634739
7 -0.142930998377972
8 -0.226739528365938
9 -0.278139078028644
10 -0.272758687746807
11 -0.334986178517965
12 -0.31855590473998
13 -0.259107659749654
14 -0.142800412084066
15 -0.0541290398706344
16 -0.0439819102916905
17 -0.0324104760083452
18 -0.00668560433659682
19 0.0352648398924602
20 0.0518307830259062
21 0.0911751347649226
22 0.105810394646419
23 0.138865687685739
24 0.141806150658546
25 0.153329201731465
26 0.200101047398396
27 0.197017036523198
28 0.253541988005333
29 0.285352021937129
30 0.301997381458028
31 0.305361358921678
32 0.338056692165053
33 0.357480725117552
34 0.362226816131232
35 0.396707944156478
36 0.432624921204328
37 0.462400934598057
38 0.511559588315824
39 0.551576907535695
40 0.578539017080508
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0219086318229529
1 0.0933171064385414
2 0.247670053178759
3 0.267084031981837
4 0.20305912331467
5 0.0756664722403402
6 -0.0560829594589451
7 -0.124799790644659
8 -0.226204346814437
9 -0.274457115444021
10 -0.257513667272505
11 -0.297827228813009
12 -0.257499911032573
13 -0.229940695483688
14 -0.109727357795495
15 -0.0194700251766973
16 -0.0101526619287888
17 0.005250122653222
18 0.0221471205310371
19 0.0272873039393069
20 0.040512235817137
21 0.0645092923121808
22 0.0610403666364814
23 0.0835385229188237
24 0.0845016758102775
25 0.0782479609772926
26 0.107543885347572
27 0.111895100743299
28 0.134485070624026
29 0.154811713613944
30 0.160553245774669
31 0.144982867800789
32 0.173111426933686
33 0.222325040527904
34 0.190091292924737
35 0.206043694184969
36 0.241949054690668
37 0.283983381309213
38 0.300627171447947
39 0.331591169871314
40 0.362372522985019
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0449369159675372
1 0.0855308135867139
2 0.238407839619886
3 0.296680038248358
4 0.221860738410972
5 0.0803054045662162
6 -0.0616280351293899
7 -0.136007839497234
8 -0.232102983642735
9 -0.307442256256274
10 -0.294904417643013
11 -0.316627725245181
12 -0.306054933428547
13 -0.27301197817461
14 -0.112088699627281
15 -0.0706145986902404
16 -0.0689856512623832
17 -0.0945882546248482
18 -0.0712780238109501
19 -0.0623204032545823
20 -0.0658024824462187
21 -0.0586655590062914
22 -0.0633034540979125
23 -0.0479004185137732
24 -0.0685972194484989
25 -0.0723152514315872
26 -0.0350146976643098
27 -0.0601107147061075
28 -0.0525415960817517
29 -0.06059008792176
30 -0.0531896824909284
31 -0.0879807985589718
32 -0.0791320171537464
33 -0.0907939690027275
34 -0.112666181500896
35 -0.112209969095962
36 -0.0929017698817702
37 -0.0862611569587219
38 -0.106363830677267
39 -0.139018613386813
40 -0.117754615837876
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0180154405081572
1 0.111358193314519
2 0.245263776130704
3 0.27567786554376
4 0.19340016731325
5 0.0425970235659729
6 -0.0928667354185926
7 -0.183524793722944
8 -0.262252272050485
9 -0.316811003380234
10 -0.280998762715697
11 -0.338560040916671
12 -0.311436780380626
13 -0.254429246230088
14 -0.122249932905963
15 -0.0303809518515834
16 -0.0329652850665312
17 -0.0209672979695101
18 0.0328625171423544
19 0.0610858051825378
20 0.0637997726987054
21 0.0735943412225737
22 0.0716695354546033
23 0.0670106620301691
24 0.037423836569598
25 0.0140417928724998
26 0.0130884043310759
27 -0.00873803041281107
28 0.00291796657260335
29 0.00235073563705246
30 -0.00825162568036131
31 -0.0333192090967227
32 -0.0439029954653289
33 -0.0416432632324915
34 -0.0859147584838507
35 -0.0848703210411728
36 -0.0720647398031797
37 -0.0767235826578769
38 -0.0809787279064436
39 -0.112557694778052
40 -0.104561720681943
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0481514308335269
1 0.095754966765262
2 0.24301476384808
3 0.280382667838318
4 0.251815554997536
5 0.125735582718844
6 0.00160156580953696
7 -0.093534855363326
8 -0.190445889435312
9 -0.265245230496912
10 -0.239276544336202
11 -0.267179837206729
12 -0.228205094358305
13 -0.195051551780759
14 -0.054969088931907
15 7.62922331514204e-05
16 0.014638174933931
17 0.00257153354615891
18 0.0285449669478153
19 0.0338841058441881
20 0.0432660298713037
21 0.0453111206905943
22 0.0301829263333335
23 0.0617372698907079
24 0.0496440941759442
25 0.0537356590862759
26 0.0719057151812255
27 0.0623123078164243
28 0.0702580102000567
29 0.0733201474163137
30 0.0924337890056499
31 0.101743424128071
32 0.116373187353218
33 0.141142081951993
34 0.134484076003009
35 0.156698975701662
36 0.191540589638868
37 0.214471900722245
38 0.228925461024382
39 0.240702851233292
40 0.258931125405697
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0210683374238023
1 0.080980293927956
2 0.212478896818773
3 0.234414858339569
4 0.18059957562677
5 0.0340159772913298
6 -0.0750861652121682
7 -0.123810839735034
8 -0.208197096834533
9 -0.263275662126835
10 -0.247245114104612
11 -0.289915373856336
12 -0.242156897448569
13 -0.215467933597977
14 -0.0771359141244563
15 -0.0304345395992431
16 -0.0230695408162163
17 -0.0264058121150645
18 -0.00489053501045955
19 0.00510255089362843
20 0.0237482364349386
21 0.0297628404895365
22 0.0311131188311302
23 0.030292274860277
24 0.0249376970971333
25 0.0148859261361443
26 0.0241782324538384
27 -0.00561326318771194
28 -0.00960553425990796
29 0.00278807691580418
30 -0.00174266253289534
31 -0.0192313933318413
32 0.000345277565708457
33 0.0099375212565489
34 -0.0198906869680897
35 -0.0127163501425338
36 -0.00622447237770363
37 0.000494432086108887
38 -0.00397079464137473
39 -0.00355337957064084
40 0.00884513480433924
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0433918059641893
1 0.0936402482732923
2 0.236886069066186
3 0.266342869667878
4 0.221284324510052
5 0.0859265045487021
6 -0.026716242286863
7 -0.0996028349809572
8 -0.179709039021779
9 -0.247554689035423
10 -0.23035101525377
11 -0.239628372558442
12 -0.190598818834576
13 -0.15247227594226
14 -0.0404700858368816
15 0.0222445087736052
16 -0.00072756982342348
17 0.00878582020511498
18 0.0331495926295409
19 0.0527872714578752
20 0.053983498865211
21 0.0729612842869605
22 0.0600744912059596
23 0.0696160714678014
24 0.048379388791175
25 0.0415902062998237
26 0.0552538698588672
27 0.0434105966461171
28 0.0470974476029857
29 0.0412920180624745
30 0.0456849602294467
31 0.0415467810268071
32 0.0350912986228735
33 0.0575286273974589
34 0.045240707276629
35 0.047796381503173
36 0.0617859940869989
37 0.0532478766260152
38 0.0397063770968726
39 0.0227880862975551
40 0.0498237350656101
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.101178630309551
1 0.0561644133141401
2 0.206008025557939
3 0.247222343728104
4 0.200423895284487
5 0.0578299545405709
6 -0.0477860547161804
7 -0.114720258863468
8 -0.211279669437967
9 -0.260805122754068
10 -0.227855976388396
11 -0.266852081557783
12 -0.263457999814512
13 -0.227838387547649
14 -0.0950439642918726
15 0.0154731190346151
16 0.0242670502836004
17 0.0200769410335226
18 0.0482373068346105
19 0.0575245141325764
20 0.0620467840327894
21 0.0820182863460079
22 0.0800690228885514
23 0.0763271933030749
24 0.0254647739790581
25 0.0492696025226351
26 0.0694565556798477
27 0.0536256549632084
28 0.0822747884105004
29 0.0878635448677851
30 0.0794740799275182
31 0.0304700662467425
32 0.0373247142980571
33 0.068637803133246
34 0.0148702440380735
35 0.00583350777053404
36 0.0161360444204739
37 0.019336197003029
38 0.0134928893016824
39 -0.00709113818760709
40 -0.0137562798267767
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0203578514878195
1 0.166498857185421
2 0.298179588254715
3 0.307784476700302
4 0.253192723613624
5 0.112610605499352
6 0.0101414850882433
7 -0.0647733343400407
8 -0.128507527665681
9 -0.195196524837439
10 -0.19464489900113
11 -0.229869085778579
12 -0.213564229671634
13 -0.147401209236231
14 -0.0210685293466302
15 0.0637039005370221
16 0.0595453434003872
17 0.0597182997824079
18 0.0744253545140054
19 0.0975515449855733
20 0.0994174256378564
21 0.111141240462881
22 0.10327311141385
23 0.103006523704553
24 0.0945970124651563
25 0.0856895684373065
26 0.100320117843964
27 0.0894017654349542
28 0.129932233708369
29 0.133892120361729
30 0.127438183139686
31 0.104429751792853
32 0.100781410794589
33 0.126465943312827
34 0.111847955255948
35 0.0996913397838552
36 0.10764845141134
37 0.105222821725016
38 0.111181575193581
39 0.114944562195715
40 0.127704139564069
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0156573951215222
1 0.0767481003675581
2 0.223053457796536
3 0.254430789624053
4 0.204649508302006
5 0.0604349688449872
6 -0.073840880465144
7 -0.156516422697405
8 -0.200878425362161
9 -0.27436507828987
10 -0.260353233603274
11 -0.272941233412113
12 -0.238797595416541
13 -0.223046449383348
14 -0.0989923078712343
15 -0.0153152241967032
16 0.0185542176530813
17 0.0137841289761962
18 0.0510987693797924
19 0.0714854502632667
20 0.0562164666979026
21 0.091389290747391
22 0.101706014529367
23 0.126190778005689
24 0.109511703516567
25 0.128610310063162
26 0.144765164871548
27 0.138809127009808
28 0.174207935460393
29 0.192989413757807
30 0.198452955963814
31 0.17894433723177
32 0.184546490326414
33 0.232921381223919
34 0.201996049431381
35 0.203185911092136
36 0.229970965267187
37 0.241538314066951
38 0.23349316112255
39 0.213260912734036
40 0.20686382383589
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.101817690919086
1 0.0156871038650328
2 0.17130677508015
3 0.187063251517349
4 0.112618175226609
5 -0.0472506190543598
6 -0.159714733675162
7 -0.231492791483079
8 -0.327294184755599
9 -0.382141257530221
10 -0.367292632946828
11 -0.411371671544835
12 -0.440176960540104
13 -0.411762088368018
14 -0.296962051606641
15 -0.257437492620972
16 -0.261031805889258
17 -0.247489076013448
18 -0.202317451107765
19 -0.185264738862711
20 -0.170974843656134
21 -0.17735200991663
22 -0.160285822993996
23 -0.159403817904137
24 -0.172595478946927
25 -0.161016190387635
26 -0.15705818052751
27 -0.169028825331541
28 -0.162145066832371
29 -0.163452068810013
30 -0.141490543622521
31 -0.164478136420579
32 -0.157580136189619
33 -0.145439800433442
34 -0.162357132982264
35 -0.170453840813976
36 -0.161988557898137
37 -0.141470345484107
38 -0.145273577490216
39 -0.165804409259276
40 -0.15186124870711
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0123196028890531
1 0.103740426059785
2 0.26249334479915
3 0.291761424845856
4 0.2231057773124
5 0.069778419375929
6 -0.0513839057372651
7 -0.129447076259631
8 -0.211821347569248
9 -0.283317179341542
10 -0.285953394920641
11 -0.289976278172138
12 -0.281715509504985
13 -0.258162197770003
14 -0.121314801799226
15 -0.0507949328540107
16 -0.0453603733281369
17 -0.0473387202708526
18 -0.0251625347100566
19 -0.0199661102006763
20 -0.00834431550789372
21 -0.00775770075828586
22 -0.00341693885888983
23 -0.00745212504349269
24 -0.0102386248577444
25 -0.0085514776779485
26 -0.0139094692854735
27 -0.0431912238901786
28 0.000126668069617253
29 -0.00565734784334193
30 -0.00375132423835378
31 -0.0234920898629492
32 -0.0241802723745197
33 -0.0226700993809388
34 -0.0451399128308214
35 -0.037597352834279
36 -0.0148811145598069
37 -0.0348408703986571
38 -0.0173629822237329
39 -0.0282818915195469
40 -0.0260762614245689
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0618375151253883
1 0.0828948940140313
2 0.223854350007462
3 0.257044506951875
4 0.204260995774552
5 0.0559773097590917
6 -0.0661987666105563
7 -0.165560767803802
8 -0.251901287086588
9 -0.331206886037261
10 -0.292260430814716
11 -0.325724873959204
12 -0.330481598915926
13 -0.304180212691464
14 -0.177292051750415
15 -0.0832206319188513
16 -0.069062327736364
17 -0.0523398393305481
18 -0.045218077386477
19 -0.0298142132960333
20 -0.0433318028354783
21 -0.0434576093126351
22 -0.0499292666198805
23 -0.0385464935980577
24 -0.0526136691339705
25 -0.0573326664986791
26 -0.0158188872557936
27 -0.0276174903307753
28 0.033125845236345
29 0.0807265845633927
30 0.0907499837703769
31 0.0949779373553135
32 0.171293354657925
33 0.217003502194801
34 0.254431995674585
35 0.29601235641652
36 0.359190616852497
37 0.4105345966426
38 0.498391530822004
39 0.577490897285783
40 0.674648950868422
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0228829074389987
1 0.104980649386097
2 0.247508553692662
3 0.295773350949345
4 0.247551511662047
5 0.106285453127557
6 -0.00941565410132572
7 -0.104132881158515
8 -0.198287074351322
9 -0.256024423217365
10 -0.255806374331804
11 -0.320918213460661
12 -0.303325284134364
13 -0.262330244993477
14 -0.107484538656877
15 -0.0234763056412843
16 -0.00799756334045654
17 -0.00886308802738167
18 0.030173771852672
19 0.0394561185625824
20 0.0550190555492067
21 0.0750585859938964
22 0.0841497473432842
23 0.100875271750863
24 0.119805131725498
25 0.152473702694953
26 0.16966540704099
27 0.153955111010404
28 0.194531791793006
29 0.178499352765519
30 0.178166963465706
31 0.19025148158831
32 0.207787751660657
33 0.256410166030361
34 0.241885282693
35 0.255660317670259
36 0.284035908330146
37 0.299905883364766
38 0.311198181052408
39 0.327500585121676
40 0.366610171593239
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0406226423754177
1 0.0941828852874451
2 0.250027404025347
3 0.296655609033396
4 0.220299822066651
5 0.0720583360620184
6 -0.0676213660220775
7 -0.136190691267182
8 -0.207377778404831
9 -0.26455550632804
10 -0.281090474678777
11 -0.31537260703561
12 -0.302751020418873
13 -0.245853390732034
14 -0.141179743552021
15 -0.0684306411066666
16 -0.0670636435023306
17 -0.0871549080244902
18 -0.0589813075209173
19 -0.0392529716851344
20 -0.0656279898347369
21 -0.0639444896070724
22 -0.0773945331163786
23 -0.0774078426833809
24 -0.100418631465064
25 -0.11119348553228
26 -0.0976263678122669
27 -0.127961501314911
28 -0.103278228038935
29 -0.0976654674330311
30 -0.080237344777343
31 -0.115921904197494
32 -0.106381375746348
33 -0.0800567399569108
34 -0.105530324871353
35 -0.0987533514631318
36 -0.0968024606417552
37 -0.0778392100153651
38 -0.0551692093399243
39 -0.0294239898019191
40 -0.0153689310485001
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0561008075687299
1 0.0831838927833717
2 0.222173402278496
3 0.272479208791193
4 0.19757083349357
5 0.044416444644753
6 -0.0779816080361524
7 -0.166616480552019
8 -0.21726546309054
9 -0.283875223384595
10 -0.224959674713922
11 -0.306022829265739
12 -0.278783053833263
13 -0.239822260781448
14 -0.115889532615426
15 -0.0564098856076205
16 -0.0555619267784495
17 -0.0670322240682522
18 -0.0481371854485166
19 -0.0620795859371652
20 -0.0805492902734875
21 -0.0948730557365609
22 -0.10537346506887
23 -0.147052394686197
24 -0.17044368299448
25 -0.161214608520109
26 -0.176178497461054
27 -0.192324793308329
28 -0.174491344126941
29 -0.177043862426877
30 -0.186325090406612
31 -0.216862286944004
32 -0.238428561588447
33 -0.245688514228602
34 -0.278203787422925
35 -0.291871056611192
36 -0.296464360048275
37 -0.325971542311073
38 -0.347092503721794
39 -0.370079681549468
40 -0.360475042497186
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.019107866301427
1 0.149443265334552
2 0.304468173099995
3 0.324978743925411
4 0.255543413351522
5 0.128214424596331
6 -0.00678417572405987
7 -0.106413121376582
8 -0.195588323481791
9 -0.272058034710062
10 -0.268681917103807
11 -0.312921781385283
12 -0.31140055450803
13 -0.312061557603496
14 -0.166930037550733
15 -0.0742294388312761
16 -0.0595343998244662
17 -0.0576604220043686
18 -0.0287028369838911
19 -0.000983326449243371
20 -0.00652327064394331
21 0.00103589610605148
22 -0.00902464269470737
23 0.00597352745240443
24 0.00675003820247433
25 0.011964780151601
26 0.0272576735677115
27 0.0399455532906243
28 0.0399662046067659
29 0.0197327881421163
30 -0.000119128317598083
31 -0.0205587317754246
32 -0.0347951824881516
33 -0.0281559076205768
34 -0.0212157371114472
35 -0.0216938515048
36 -0.0347690161532643
37 -0.0286233610358151
38 -0.0501592182318014
39 -0.00864344606351608
40 -0.00287646502428984
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0383652797919876
1 0.101056205939483
2 0.241813450030009
3 0.279776906542714
4 0.218628900502849
5 0.0835479273957072
6 -0.0475877469577322
7 -0.136114877118637
8 -0.224053092210728
9 -0.306790926309246
10 -0.282032633831966
11 -0.355277018758616
12 -0.342880127896609
13 -0.287503749296064
14 -0.151863544331897
15 -0.066038609703253
16 -0.0609063413911848
17 -0.0486717704670925
18 -0.038839909253336
19 -0.0325721712503908
20 -0.0424922906877816
21 -0.0335786050363298
22 -0.0264332195679868
23 -0.0243344986303162
24 -0.0547579556969477
25 -0.0382061923607306
26 -0.0322308899659918
27 -0.0519849981218146
28 -0.0137523152186079
29 -0.00625777981973119
30 -0.0238100565684203
31 -0.052184820371715
32 -0.0738827517755167
33 -0.0645450327754036
34 -0.10675819345426
35 -0.10598353646852
36 -0.0928171727986085
37 -0.0802391644142828
38 -0.0934034269796085
39 -0.115147497763786
40 -0.101064894828164
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.00624175552456396
1 0.120987573735825
2 0.273593302611039
3 0.311557408843499
4 0.247101067720629
5 0.104844960431875
6 -0.020955834250584
7 -0.0896048749435794
8 -0.180962513296175
9 -0.247288745076503
10 -0.229818329667992
11 -0.233760593165241
12 -0.201648625694492
13 -0.158690195786911
14 -0.00966123966253551
15 0.051324187064747
16 0.0467828367530023
17 0.0508015049889572
18 0.0634021949731913
19 0.0723526256154639
20 0.0609080695396589
21 0.0567035711565111
22 0.056708906524408
23 0.0377922184032391
24 0.0168101840718844
25 0.0298232272826899
26 0.0343388565845473
27 0.038039388588297
28 0.0354743398181565
29 0.0337963266553327
30 0.0445684559961146
31 0.0471242851170635
32 0.0534436303165773
33 0.0579104638548102
34 0.0562673807952629
35 0.0638508981197532
36 0.065532041450294
37 0.0605585994699247
38 0.0736084604318732
39 0.0829257931157548
40 0.0889444060816293
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0700876383945097
1 0.0437460347681382
2 0.182660991554733
3 0.196462325248807
4 0.102580559318594
5 -0.030673609515218
6 -0.163799575791852
7 -0.231773597661332
8 -0.306159951660828
9 -0.350150490915369
10 -0.339472642066329
11 -0.357011531737347
12 -0.341982190316862
13 -0.323090967706555
14 -0.227886089704906
15 -0.157816969906841
16 -0.161491432917709
17 -0.16898283688074
18 -0.158710331907549
19 -0.145405854053611
20 -0.129487353285711
21 -0.108589626579253
22 -0.119146974922768
23 -0.119244054366668
24 -0.129023045384844
25 -0.131716093875957
26 -0.10562126901823
27 -0.132510306930561
28 -0.138556226868105
29 -0.152276242744899
30 -0.151124386989748
31 -0.172864003856168
32 -0.187784690545826
33 -0.191086586401126
34 -0.1982710480444
35 -0.195822527135567
36 -0.193767104237095
37 -0.204765811496785
38 -0.202671771430039
39 -0.218860906507718
40 -0.226120768074186
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.00547464709896328
1 0.143508495905621
2 0.291365716996077
3 0.321629700904925
4 0.273203744319011
5 0.131419540647437
6 0.00159491033323622
7 -0.0922646486452106
8 -0.170966384794259
9 -0.247683744278087
10 -0.2332687697146
11 -0.265812326411831
12 -0.238573896964887
13 -0.195388745120502
14 -0.0841966256535072
15 -0.0026748070945013
16 0.00435131297384839
17 0.0162523839980144
18 0.0292903088929783
19 0.0167165867292542
20 0.0323755246296402
21 0.0694924364392477
22 0.0891290106866478
23 0.108645451798139
24 0.111385795098344
25 0.117159008389534
26 0.140855285884766
27 0.126970748818882
28 0.163802573650615
29 0.186016120198641
30 0.190594513883054
31 0.188949830660006
32 0.192568343100985
33 0.216170024219446
34 0.196198698913627
35 0.197574830376377
36 0.211529268358923
37 0.216903954342838
38 0.213990053036323
39 0.217810416625949
40 0.218756573493978
};
\addplot [line width=0.01pt, color0, mark=*, mark size=2, mark options={solid, draw=black}]
table {%
1 0.0245940881197116
2 0.226498901996681
3 0.35963173094045
4 0.323192876348203
5 0.111448288247637
6 -0.15695204006051
7 -0.325976982807179
8 -0.334640765706954
9 -0.209549890955135
10 -0.205884173772729
11 -0.395618742668341
12 -0.404592842072073
13 -0.230511879468287
14 -0.055279679833161
15 -0.0210029805809502
16 -0.0164575411401979
17 -0.0161737318314269
18 -0.00358054162625767
19 -0.0104086468728599
20 0.0127963401693988
21 -0.00256627163803121
22 0.00694011005459992
23 -0.0244461075742605
24 -0.0236365740759628
25 -0.0484458903598396
26 -0.0156604557703324
27 0.0128490171223125
28 0.0437716443655508
29 0.03698016897091
30 0.0120928241581541
31 0.0180395493500055
32 -0.00624743566737794
33 -0.00866452893233261
34 -0.00937398036588012
35 -0.00916348210569427
36 -0.0019314931161561
37 -0.00552501045437327
38 -0.0230162558437155
39 0.0125317378882848
40 0.0372569376930346
};
\end{groupplot}

\begin{groupplot}[group style={group size=1 by 3}]
\nextgroupplot[
ylabel={\textcolor{color1}{angle}},
ylabel style={font=\large},
xshift=-8,
xmin=-1.95, xmax=40.95,
%ymin=-1.57659114442869, ymax=10.3791956668369,
ymin=-3.0, ymax=12.0,
width=\figurewidth,
height=\figureheight,
axis y line=right,
tick align=outside,
xtick={},
xticklabels={},
xtick pos=left,
ytick pos=right,
x grid style={lightgray!92.026143790849673!black},
y grid style={lightgray!92.026143790849673!black}
]
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.306461857520244
1 -0.0789248900917179
2 -0.581422402992076
3 -0.833993481823348
4 -0.51153390935989
5 0.348965001301977
6 1.34989891251817
7 2.15975986933723
8 2.8826895384247
9 3.80322486468507
10 4.93725086703725
11 6.52946129845216
12 7.72015279156811
13 8.47764818373024
14 8.90286296461811
15 9.01253071072509
16 9.0242550472872
17 9.09655120508274
18 9.19190458374002
19 9.21626812928691
20 9.28378271463809
21 9.32137873883888
22 9.31757207153977
23 9.29165471362022
24 9.30624937157468
25 9.32314539997073
26 9.34846788109487
27 9.38029356676209
28 9.48192573527974
29 9.44879454972119
30 9.40087197454127
31 9.39589703302776
32 9.37546186593168
33 9.34672175535667
34 9.33761089427467
35 9.36570001151829
36 9.38866149568486
37 9.38456987343778
38 9.36277945044745
39 9.36607464562561
40 9.41645658561275
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.259856511802068
1 -0.173221565794371
2 -0.756131303423697
3 -1.00519367308739
4 -0.744340306666898
5 0.213687030123123
6 1.24106631359121
7 1.99773937547464
8 2.78441620221022
9 3.74744822346124
10 4.86510381500552
11 6.36757176383092
12 7.60355023999704
13 8.3850762277466
14 8.93506607153235
15 9.20767123407224
16 9.20111725191283
17 9.22485713577314
18 9.27911743355157
19 9.28252608673406
20 9.2990743994073
21 9.26431320000578
22 9.25953504183399
23 9.22317166089228
24 9.18372822403344
25 9.18274894707151
26 9.14642458963877
27 9.21520637541327
28 9.29966403529261
29 9.24856388438154
30 9.18614494119094
31 9.0919560276904
32 9.0455955947952
33 9.0638397920673
34 8.99927758713256
35 8.99822674239767
36 9.00553376460496
37 8.97744216404092
38 8.95222941830094
39 8.910369862162
40 8.93932072139184
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.267533688812827
1 -0.0480551779075697
2 -0.59680579862855
3 -0.955852283794091
4 -0.731202048259908
5 0.114156234598758
6 1.07837052421933
7 1.89387348917676
8 2.64122297830968
9 3.58040724427041
10 4.71648988191843
11 6.21780494343163
12 7.45777077626603
13 8.32881609922599
14 8.86257457659096
15 9.10324103738074
16 9.14469258557682
17 9.21540848186507
18 9.29579314962141
19 9.30580338727647
20 9.33679655147935
21 9.34846343330825
22 9.3319060474491
23 9.33496823353565
24 9.28658105483441
25 9.31198626558585
26 9.31996251385133
27 9.38589448697299
28 9.40528304180727
29 9.37139468130852
30 9.35675863024577
31 9.2740521490525
32 9.29046213577545
33 9.2849135314451
34 9.2147455917468
35 9.21718755711013
36 9.25666633630906
37 9.1992723103687
38 9.18989292469848
39 9.19212664496286
40 9.23432410586604
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.294074277617106
1 -0.159135468802149
2 -0.683871850198781
3 -0.924462847425859
4 -0.576057441455108
5 0.343607620981194
6 1.35269957231132
7 2.10278335447072
8 2.88150471922481
9 3.82253904900856
10 5.00135231653157
11 6.55956605690381
12 7.75944058350342
13 8.55889345991841
14 9.01919946005446
15 9.28754272604858
16 9.2907082756978
17 9.31682839991667
18 9.30979808898446
19 9.32740459928887
20 9.35650547769242
21 9.36894061654507
22 9.36883951417443
23 9.34913108059984
24 9.32226109899025
25 9.3376834856316
26 9.32831723656599
27 9.36052801300422
28 9.39137705727659
29 9.37434051080266
30 9.32982228338973
31 9.22167376222799
32 9.23761912013953
33 9.15053793405718
34 9.13201018114596
35 9.16497625454737
36 9.17872225219257
37 9.17619164890644
38 9.15729632465451
39 9.16525264260164
40 9.20841678568274
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.291291453891086
1 -0.0837422991403134
2 -0.612737277917136
3 -0.858432651365196
4 -0.551519235470057
5 0.374309846734194
6 1.35192365805615
7 2.17060220755668
8 2.88544733844227
9 3.82911565149402
10 5.04123465301428
11 6.61511229053349
12 7.75251506672053
13 8.5013874273687
14 9.01112016143692
15 9.26740121785492
16 9.28360948858196
17 9.34231979763991
18 9.42856238055307
19 9.424150019173
20 9.43523953872332
21 9.42367770915667
22 9.43274014407602
23 9.41529986975609
24 9.37102268561564
25 9.39151075603979
26 9.4069590666789
27 9.44282679123627
28 9.50192945627659
29 9.5034606237714
30 9.44693589250597
31 9.38435509343332
32 9.38989213720077
33 9.34026746503267
34 9.27661368513182
35 9.33816134583605
36 9.37355918490174
37 9.35189938484958
38 9.34585668227781
39 9.36278109044066
40 9.42062453264394
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.335247846763737
1 -0.0765216841598892
2 -0.586302780768972
3 -0.797818973020455
4 -0.425676418630283
5 0.501462384498653
6 1.45927744949059
7 2.21722897326395
8 2.96110706785333
9 3.91854780416745
10 5.1605578868667
11 6.75963577631722
12 7.83797246060067
13 8.58981554743896
14 9.11189798058861
15 9.28954163512252
16 9.2674213912606
17 9.33588693429024
18 9.39892276089218
19 9.40880863748226
20 9.4043470342353
21 9.45766382090788
22 9.45408754335521
23 9.44191701609353
24 9.40221069493666
25 9.46030068599963
26 9.47308830725857
27 9.51848488929398
28 9.57398669755842
29 9.54124600455847
30 9.47863421430533
31 9.40514140393715
32 9.37803979574404
33 9.3263497233003
34 9.29336118956532
35 9.33358264083018
36 9.34355765974136
37 9.33278263955407
38 9.28498111703006
39 9.30352940272921
40 9.341066183862
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.277292183587331
1 -0.159588524153253
2 -0.733746319679458
3 -0.927932951297457
4 -0.642111239768197
5 0.295139223985021
6 1.31624031580079
7 2.08627910901849
8 2.85015437486153
9 3.7861371338769
10 4.99924639166691
11 6.50542489236341
12 7.57594190515435
13 8.3478853638502
14 8.86170891725536
15 9.11114634326113
16 9.07564526156791
17 9.19749062691655
18 9.24838170386981
19 9.27790757907574
20 9.29547543890435
21 9.30850449588441
22 9.3052515099881
23 9.33412293917699
24 9.30223771028446
25 9.36637967380666
26 9.38247811611857
27 9.45506216835682
28 9.56854561664788
29 9.60299875608365
30 9.57453147592103
31 9.54946128456706
32 9.55878205223917
33 9.52289594749908
34 9.56233980191849
35 9.6408873882545
36 9.63484337673856
37 9.6516859389558
38 9.61666104244929
39 9.67295564552674
40 9.75903127402322
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.282670757745803
1 -0.12367998989979
2 -0.662886520561288
3 -0.886946329674354
4 -0.533583180202005
5 0.385026402639459
6 1.34331758875761
7 2.09650077367724
8 2.86918123219202
9 3.81680473179284
10 4.94531687281744
11 6.47742391271568
12 7.67426491866848
13 8.47118336210706
14 8.93796943274641
15 9.16654146435927
16 9.14447167200106
17 9.1475748931311
18 9.23621039100805
19 9.26744680350791
20 9.30993945296758
21 9.36837615544726
22 9.38147863047264
23 9.37812162317515
24 9.29960244374509
25 9.30206230642419
26 9.32025443444059
27 9.35866986950888
28 9.40754178891625
29 9.40191177921196
30 9.37411914409386
31 9.32466243365709
32 9.3426409538589
33 9.33861400799212
34 9.32024735450245
35 9.33915677648561
36 9.38189615920281
37 9.36899329258098
38 9.33894105576102
39 9.33907175577026
40 9.43293962985545
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.30778663612148
1 -0.103545037956739
2 -0.664650239908321
3 -0.907604240929771
4 -0.593159344818118
5 0.407265393929183
6 1.37397141222882
7 2.23734216041788
8 3.14821139413718
9 4.19952483080651
10 5.55409204068586
11 7.03146571244964
12 8.0892360357602
13 8.83621721107588
14 9.37360139211413
15 9.62374594383808
16 9.68829411423926
17 9.77301852951187
18 9.86864845420049
19 9.94175052913218
20 10.0062172145861
21 10.0916038654497
22 10.1423656146972
23 10.192610714149
24 10.283614068455
25 10.4026866433871
26 10.5523383473344
27 10.8578356215958
28 11.1608800764189
29 11.5314684215901
30 12.0024683697673
31 12.6908377034046
32 13.5237298094676
33 14.2718389509242
34 15.0563139678569
35 15.79826544623
36 16.4121763786602
37 16.9430652529085
38 17.4662947195553
39 17.8819230361045
40 18.3360305633448
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.289477269598257
1 -0.100307618228403
2 -0.64342487658829
3 -0.933197557905595
4 -0.620542605143569
5 0.317381976961113
6 1.29033896533051
7 2.06410663816707
8 2.81494185942592
9 3.75051764698692
10 4.96963208072013
11 6.51811810544955
12 7.71701446794157
13 8.51118958352134
14 9.01102456143141
15 9.21002240165595
16 9.22415657169427
17 9.30433793735437
18 9.32370790241852
19 9.34220408866725
20 9.34948513818172
21 9.4052813017022
22 9.39156113555353
23 9.40332049695689
24 9.39505717611069
25 9.41286961055026
26 9.43595502111146
27 9.49901452370835
28 9.54588659503758
29 9.58536832281255
30 9.55604318178062
31 9.55148904400924
32 9.55962286107785
33 9.57640961736273
34 9.54450735136128
35 9.64111195807196
36 9.67387803090235
37 9.6450752615336
38 9.66435156532506
39 9.73627964476812
40 9.81678209934754
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.303638303823788
1 -0.073941306132713
2 -0.605495324236116
3 -0.883045407857032
4 -0.602842535550138
5 0.331284562173156
6 1.32871771296567
7 2.167697893049
8 2.94102967588304
9 3.87963197444073
10 5.08587123387598
11 6.63108497780407
12 7.76627542152673
13 8.56042306895541
14 9.0826828186822
15 9.34010904666729
16 9.32442649581629
17 9.39851285781067
18 9.48168155084769
19 9.47079033797843
20 9.51567338193044
21 9.54621205174169
22 9.50053876422546
23 9.49769020456145
24 9.5081162729982
25 9.51329183695119
26 9.51467430834173
27 9.62407358784004
28 9.71864061752105
29 9.70252078226362
30 9.68667562277286
31 9.71039831567529
32 9.74695923261999
33 9.73140296860118
34 9.77623976951253
35 9.89196268013849
36 9.99301258179847
37 10.1371530108628
38 10.3249310091958
39 10.6634605153894
40 11.2107245869564
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.27715195222316
1 -0.133827096472666
2 -0.69088904307962
3 -0.947283705571556
4 -0.680612969939856
5 0.22766026428895
6 1.16459684319255
7 1.90900291315463
8 2.67319921527335
9 3.531481767072
10 4.50575945630608
11 5.95117824096889
12 7.19812250883866
13 8.07386872198669
14 8.5881354428771
15 8.81228179596098
16 8.83300993082567
17 8.88992798158612
18 8.93024685052893
19 8.93515825117248
20 8.97781263498864
21 8.9673803248042
22 8.9570985349334
23 8.96173999263573
24 8.935218478388
25 8.96306908118319
26 9.00730514985063
27 9.14195213073643
28 9.20299385076695
29 9.19152786871203
30 9.12527649369708
31 9.09989595322683
32 9.13576002829717
33 9.09970043043088
34 9.12616336804963
35 9.20155320639902
36 9.25491349318819
37 9.30890907266035
38 9.30899416674714
39 9.32606665725152
40 9.3774370555546
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.316805300616422
1 -0.111937670306141
2 -0.67034513924414
3 -0.8823869714052
4 -0.594400241409544
5 0.314002937944152
6 1.33672658095074
7 2.15574820333333
8 2.90738519170745
9 3.86376342016455
10 5.03615030707591
11 6.59591878218477
12 7.74347259349328
13 8.49713705722553
14 8.97973900479223
15 9.22522505944894
16 9.24558666393484
17 9.30652901759814
18 9.32161503717382
19 9.31381287326703
20 9.2761601766795
21 9.20506745191191
22 9.08264586640527
23 8.97150479889103
24 8.94993572966233
25 8.88248467301073
26 8.78549469606752
27 8.7996795571845
28 8.82192466220105
29 8.746864745961
30 8.67717100002271
31 8.57378813643322
32 8.59980586318015
33 8.54728559711759
34 8.50841057298896
35 8.50880975194561
36 8.51026148173141
37 8.54532966474182
38 8.52677671361216
39 8.52872220720761
40 8.50430475256972
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.269068063090664
1 -0.14945052353132
2 -0.740665640476553
3 -1.00974403317551
4 -0.714439470264864
5 0.184788107877948
6 1.17803322254725
7 1.97271668886349
8 2.74481449856933
9 3.68925368048181
10 4.93931459213137
11 6.54566139393901
12 7.63485651568695
13 8.35814742910721
14 8.85404036258945
15 9.14985974851112
16 9.163944184164
17 9.25091868095309
18 9.35000845466828
19 9.38470652262405
20 9.43146603676577
21 9.4458607637005
22 9.46569907759493
23 9.4838933971581
24 9.47321621006018
25 9.50198830259604
26 9.4889241410844
27 9.57152581716961
28 9.63214211089803
29 9.5920895012469
30 9.56403135318429
31 9.52447285821696
32 9.51312913412671
33 9.53335992969614
34 9.49300240144268
35 9.5390913749588
36 9.50955757473503
37 9.43483532782254
38 9.40938948159097
39 9.41844006767188
40 9.43704535994368
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.318510739213467
1 -0.0919809287922972
2 -0.607541991023397
3 -0.887492003021477
4 -0.566429889641712
5 0.393361229672356
6 1.31058796351704
7 2.0812013981384
8 2.83024377376812
9 3.69203779556322
10 4.85337726920353
11 6.36428210702358
12 7.61011635767082
13 8.39249644535273
14 8.91522655567572
15 9.13338661437698
16 9.17367265867867
17 9.22468432843231
18 9.27274226709137
19 9.30801822264996
20 9.36465194596326
21 9.37562809774132
22 9.35703186427408
23 9.34131198375708
24 9.31372519162391
25 9.36065188085497
26 9.39129507020977
27 9.43102581673478
28 9.47822534261973
29 9.46133803572625
30 9.44557691824264
31 9.42825847487692
32 9.42959456271154
33 9.4023302351868
34 9.37739520889822
35 9.42339871507988
36 9.43024365971513
37 9.42226373905229
38 9.36774847102879
39 9.39961153169797
40 9.40932313047204
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.294916567494147
1 -0.138353393490592
2 -0.64992887323015
3 -0.875686458207836
4 -0.559391335993062
5 0.409284356965331
6 1.38889985262886
7 2.1907807200888
8 2.93029261645811
9 3.81182041159767
10 4.96796897071
11 6.46384856894176
12 7.69187155557683
13 8.47095163422795
14 9.03500669496624
15 9.24467302641513
16 9.30940702136713
17 9.36577206984701
18 9.44664498472421
19 9.45388394884036
20 9.49010422406669
21 9.48944522430609
22 9.43930684470155
23 9.47029602371176
24 9.44883151442632
25 9.45502938057169
26 9.48399523791228
27 9.51498871868313
28 9.58382656857138
29 9.56127201489701
30 9.49891854151286
31 9.48875849731322
32 9.47991832221675
33 9.50978713352236
34 9.48274714060993
35 9.48086636051789
36 9.50017310134394
37 9.49804612878702
38 9.46873725671487
39 9.41772888305513
40 9.42485308288001
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.285384748816589
1 -0.101664283754046
2 -0.634456901875899
3 -0.932597515701145
4 -0.682799459057537
5 0.193646256580806
6 1.10444950595682
7 1.86477953969727
8 2.61686000147781
9 3.45341501789597
10 4.52267888661975
11 5.91116796067521
12 7.20520836181935
13 8.16326766642571
14 8.7146151695407
15 9.04170064379445
16 8.99185045582341
17 9.06501177909447
18 9.14963056139769
19 9.16980365789861
20 9.20888668819909
21 9.23006765918911
22 9.20114365547438
23 9.17807726065914
24 9.1317477894431
25 9.1091200767972
26 9.11247718365474
27 9.16841929160871
28 9.21858591028448
29 9.21098457766896
30 9.19364126928032
31 9.13889853009356
32 9.14512424703163
33 9.1195658723053
34 9.04803879523754
35 9.01662322414592
36 9.02962467638902
37 9.01713283863123
38 8.94966116331131
39 8.9086197785751
40 8.91373372359475
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.302362172167217
1 -0.16396561492034
2 -0.744775028289906
3 -0.95991840652129
4 -0.626641732613892
5 0.299938662237869
6 1.30666524941512
7 2.09777160343674
8 2.83515715887969
9 3.86261302678058
10 5.09335896274133
11 6.72270106189519
12 7.91139866840277
13 8.65739438822483
14 9.21153929303054
15 9.4492555267165
16 9.43575536288846
17 9.45970709312196
18 9.49791256686665
19 9.49157662077204
20 9.52940285932712
21 9.52528665788045
22 9.49290588236615
23 9.43471525579463
24 9.38221272894478
25 9.33039505992943
26 9.28464882422451
27 9.32892235922103
28 9.36935640608409
29 9.31420060312808
30 9.2033434948889
31 9.1411668456277
32 9.15458740886964
33 9.11003443334133
34 9.10547505197311
35 9.12181691716755
36 9.18087404409197
37 9.1576955083995
38 9.10285937622893
39 9.11937193186038
40 9.15301401263844
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.309816564621876
1 -0.0615919178996207
2 -0.573714311484264
3 -0.833702368471334
4 -0.501142476563901
5 0.422066045299745
6 1.38768379526926
7 2.19652421032341
8 2.97948607858161
9 3.92719842026008
10 5.18267668071459
11 6.69648939579938
12 7.83398293422654
13 8.62646082006338
14 9.20114355148645
15 9.41972805595576
16 9.41586992120611
17 9.51361031709506
18 9.5883726675964
19 9.59333849160123
20 9.66574529626096
21 9.69015553947659
22 9.66638311226138
23 9.67218334668188
24 9.72818402316073
25 9.82899299357324
26 9.8527448136013
27 9.99477351909676
28 10.1166590748614
29 10.1222055451545
30 10.1614409254917
31 10.2389296370022
32 10.3056148751101
33 10.420097163846
34 10.5091187176799
35 10.7569533690738
36 11.2570634625056
37 11.8367746224241
38 12.5592400266354
39 13.3838393999477
40 14.2355008281251
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.306375913918502
1 -0.0735677798378305
2 -0.562836075251771
3 -0.800896300003788
4 -0.491856453437032
5 0.422519001881385
6 1.40813921187682
7 2.21777863188577
8 2.9345253766729
9 3.92830617356418
10 5.17830737772993
11 6.64278079873922
12 7.79152709006512
13 8.50450881612533
14 8.97531362471557
15 9.20426627472485
16 9.2196509594725
17 9.25486416348983
18 9.30409670412329
19 9.30612013384257
20 9.32682473573913
21 9.35933413875328
22 9.34344728387575
23 9.26888169694572
24 9.19445885661528
25 9.22443804839011
26 9.23281741912687
27 9.231122789687
28 9.32412826009848
29 9.23935176532596
30 9.17519469131537
31 9.13635233783757
32 9.1150606747805
33 9.07732216055536
34 9.01621766904882
35 9.03333145720272
36 9.00503119621438
37 8.97841390517921
38 8.95886249621772
39 8.92856579701364
40 8.92076022627397
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.303775372248772
1 -0.138222335578946
2 -0.649340270020819
3 -0.81186572259919
4 -0.476530339311992
5 0.4997720197897
6 1.48402071772103
7 2.2565191175788
8 3.04889142933019
9 4.04576345275174
10 5.25946518806244
11 6.79709512591651
12 7.9278489999192
13 8.6560332862052
14 9.16818020011716
15 9.35308573473015
16 9.32545664657713
17 9.34452656399367
18 9.43758973826568
19 9.47708329424772
20 9.48707315194206
21 9.52969115304945
22 9.49922007350112
23 9.456480918289
24 9.4150810306482
25 9.40940614933331
26 9.44304061498996
27 9.53427981560142
28 9.63573041899384
29 9.66306131242433
30 9.6008991443089
31 9.53406519993579
32 9.54099489048557
33 9.53115228499806
34 9.50849898766109
35 9.52212759275759
36 9.57626689720532
37 9.56401349139737
38 9.54581197852542
39 9.52978107391013
40 9.5550834849004
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.323593123684466
1 -0.120390541591671
2 -0.623259107604453
3 -0.869856821800177
4 -0.545358972324349
5 0.359283977631955
6 1.32056897645361
7 2.06559964045856
8 2.77656140942821
9 3.68095903152935
10 4.7844025308216
11 6.29851562060597
12 7.53892306775712
13 8.32175858962925
14 8.8511572035278
15 9.04469664185693
16 9.0543395934391
17 9.07250778420564
18 9.1305123638023
19 9.1103153489063
20 9.11042222899018
21 9.08536629322148
22 9.05813203892924
23 9.03322606568152
24 8.95507332062106
25 8.96253902415537
26 8.9976489121297
27 8.99472572106939
28 9.04658470749508
29 8.98683441354564
30 9.00926972781815
31 8.93305427202472
32 8.93962674911239
33 8.94470002941687
34 8.85935004098628
35 8.82850330423252
36 8.82296342561949
37 8.78893507701804
38 8.69356829433263
39 8.69854002618962
40 8.6694846327674
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.291987588399602
1 -0.119954167390793
2 -0.658796847819547
3 -0.923148978380928
4 -0.668492990448184
5 0.204612597454834
6 1.14463461448776
7 1.9194587637278
8 2.65531233247236
9 3.58106595801408
10 4.71842260938185
11 6.23179768734339
12 7.5067876183253
13 8.35071188553319
14 8.85949207371943
15 9.05506585597315
16 8.97511832531596
17 8.94986231049021
18 8.94580923093258
19 8.93789595405955
20 8.86319374219398
21 8.79382412958839
22 8.71597242683715
23 8.59240063393131
24 8.49046407762132
25 8.41257507676958
26 8.34085171645946
27 8.36762194279184
28 8.36420806304104
29 8.2692172131436
30 8.17545582089011
31 8.15768236495182
32 8.10045314008137
33 8.08790969266584
34 8.059544079774
35 8.03920532410348
36 8.01689086862108
37 7.98017326329873
38 7.96268971839435
39 7.96867632186186
40 7.9703738102394
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.307046792548798
1 -0.0947999692676174
2 -0.60842100390898
3 -0.812811210334375
4 -0.485903519832763
5 0.415288688913388
6 1.34395628155439
7 2.06366739124466
8 2.77641690413557
9 3.64879574496869
10 4.68314498529506
11 6.11633130339882
12 7.36110552375227
13 8.25596706867811
14 8.84317507187719
15 9.1504761767284
16 9.13973472681595
17 9.17434003400248
18 9.26819202937246
19 9.26155622019685
20 9.28440184305892
21 9.29769992666445
22 9.2977605255075
23 9.29861904833755
24 9.30717492209994
25 9.30571805176812
26 9.34226984334763
27 9.41519573510068
28 9.48692881822869
29 9.45722911595334
30 9.40424564211991
31 9.38595001674002
32 9.37406692593858
33 9.40239882066363
34 9.40349215232268
35 9.45852780356235
36 9.53259057483346
37 9.5506136909658
38 9.51923590467668
39 9.53587402501519
40 9.6079250008541
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.326370196875374
1 -0.115417830723606
2 -0.610155672517027
3 -0.834562088015631
4 -0.458086830582455
5 0.456487851288664
6 1.40660299519589
7 2.16454943406674
8 2.90284046631465
9 3.81603093374916
10 4.95945795910713
11 6.55514331073098
12 7.79356806336521
13 8.56368118698581
14 9.11127801968957
15 9.34274348525914
16 9.3778649215382
17 9.43071572712856
18 9.5027712411727
19 9.53676880785947
20 9.60791536666395
21 9.63820241999374
22 9.62574403975923
23 9.66461278796724
24 9.71296539960944
25 9.76292402871412
26 9.79273834478994
27 9.90127813092399
28 10.0122023560114
29 10.0572087735721
30 10.1385455101167
31 10.2504651498278
32 10.372290003363
33 10.4752966508034
34 10.7359538016537
35 11.1135414981427
36 11.6577128531094
37 12.299399899872
38 13.1423904392672
39 13.9602009267345
40 14.7421752029404
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.26981261853925
1 -0.172628641209833
2 -0.681460708787088
3 -0.927038250493952
4 -0.649208817554694
5 0.256385479848459
6 1.20443565928702
7 2.00815656101576
8 2.83152040784804
9 3.83121182957654
10 5.0837451927755
11 6.63140782675664
12 7.80312327412677
13 8.49616335877233
14 9.00657916665472
15 9.239603803183
16 9.3031974936526
17 9.31789466134375
18 9.38162507198766
19 9.40253445941348
20 9.44599107243648
21 9.47142071169884
22 9.45306107026865
23 9.40777635193332
24 9.38601016578704
25 9.39320478829365
26 9.40003735180741
27 9.46241625673801
28 9.49555277359817
29 9.4802370555346
30 9.41521636425717
31 9.40172754216844
32 9.43688036718998
33 9.40499237479311
34 9.38004732467422
35 9.42029456834712
36 9.4333658870398
37 9.44049224678549
38 9.44088774765586
39 9.44583527924873
40 9.53657766704234
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.263097204555847
1 -0.106225288217125
2 -0.688074774375038
3 -0.965215661603204
4 -0.684675177508188
5 0.204143139190168
6 1.15888890263017
7 1.89495722703309
8 2.61629070035242
9 3.50867448791895
10 4.56754469809031
11 6.02524122774566
12 7.3463720605664
13 8.15495758923532
14 8.71398907889415
15 8.96948866054072
16 9.02282998594692
17 9.04654773200408
18 9.16812223154068
19 9.21863414064845
20 9.24143955045381
21 9.26162579416386
22 9.25747091673848
23 9.25110329816031
24 9.16142135365366
25 9.17368660000195
26 9.17593905915639
27 9.23131651300989
28 9.2494080563985
29 9.18702707056646
30 9.14396875299754
31 9.05197435792615
32 9.02192647687624
33 8.97835278660961
34 8.93267099385249
35 8.97860160931831
36 8.96082529321364
37 8.92409334141344
38 8.85059314465048
39 8.80388792639357
40 8.83680591263658
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.289244467111025
1 -0.154138332034353
2 -0.678728815578813
3 -0.926089469956893
4 -0.662213174179092
5 0.295457114440398
6 1.31968295149802
7 2.11971152246733
8 2.93275162182168
9 3.95009592038446
10 5.25865152200793
11 6.72758968803012
12 7.90200549533063
13 8.69871301459318
14 9.21169420692917
15 9.48835465957207
16 9.44473482491635
17 9.50779830911244
18 9.61387983117928
19 9.63966011176509
20 9.64832265374707
21 9.67453392807433
22 9.69408689546377
23 9.70973032525988
24 9.70218868020381
25 9.74339482237004
26 9.78324069424503
27 9.8752906171085
28 10.009862271865
29 10.0692747277289
30 10.0769793011146
31 10.121268156058
32 10.1650577922082
33 10.1661998812134
34 10.2112148475847
35 10.3529852829249
36 10.4580562709367
37 10.6494988837544
38 10.9526382435627
39 11.4184463554265
40 12.0859308155675
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.293398092173967
1 -0.145979533647691
2 -0.650771628271066
3 -0.908202169205525
4 -0.597702187057195
5 0.282687405332044
6 1.25495547686273
7 2.03618545971752
8 2.82706208017529
9 3.71936031531963
10 4.88722240666517
11 6.4607256879306
12 7.68457360842966
13 8.45722147246275
14 8.9854316090013
15 9.23437754900335
16 9.24836968370463
17 9.2842667724508
18 9.31835224897458
19 9.32474808083411
20 9.33246520370822
21 9.36324294202097
22 9.3164750072723
23 9.34959316089751
24 9.33645394692401
25 9.30709027159887
26 9.29390638714572
27 9.29271965470306
28 9.38504088641809
29 9.34126579159673
30 9.30735917308326
31 9.30897683109922
32 9.28953599995697
33 9.31448057803025
34 9.31204715795405
35 9.34412680341236
36 9.34712210476316
37 9.36223519287119
38 9.40975438710423
39 9.45321499661087
40 9.49637833500341
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.282767941223562
1 -0.15998634107311
2 -0.677505588907933
3 -0.93043205885144
4 -0.652905032146918
5 0.296757871240419
6 1.27051911183548
7 2.04322805031739
8 2.78534414010673
9 3.74663720178438
10 4.92666641121554
11 6.42311555347763
12 7.60286326316489
13 8.34855101726538
14 8.86486538685261
15 9.1113773112522
16 9.11129504570939
17 9.15105496428117
18 9.18340716866349
19 9.20347570413875
20 9.20990501035987
21 9.22373220022912
22 9.21481385662492
23 9.21659745313414
24 9.18836331498642
25 9.15766163422473
26 9.1726182380365
27 9.20707193539569
28 9.27729518524283
29 9.24369002520447
30 9.2177601537274
31 9.16796121961929
32 9.16353994256601
33 9.17249627614282
34 9.1388242912613
35 9.16741744522445
36 9.20648434325703
37 9.2046284057629
38 9.1566814846241
39 9.12218318602944
40 9.12252175079221
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.259141166734723
1 -0.136188292794054
2 -0.742168384464596
3 -1.01733029103311
4 -0.724430235387467
5 0.228005718375445
6 1.17856153834054
7 1.93451926570768
8 2.6823855834413
9 3.53010976825954
10 4.54456074213107
11 5.98824675311652
12 7.27385415981665
13 8.19851929060702
14 8.75697854561539
15 8.96684930725083
16 8.97990325728756
17 9.04100091418848
18 9.07970885714924
19 9.0801538206004
20 9.04477679517773
21 9.05283432354542
22 9.00802387409853
23 8.95611051297687
24 8.85598456805938
25 8.84952326786035
26 8.85938594174235
27 8.88378363893472
28 8.87170792159376
29 8.86599256621424
30 8.78373731243827
31 8.69843222859222
32 8.62906230481808
33 8.63346139897693
34 8.54568458067562
35 8.52318246802975
36 8.59419024011454
37 8.54932590266561
38 8.44934654714116
39 8.37509893747939
40 8.39199822518932
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.276110605107006
1 -0.185410503301544
2 -0.715146497713326
3 -0.995979476779589
4 -0.746787850217594
5 0.0882320689031433
6 1.12452299877755
7 2.01023667043886
8 2.72398637727058
9 3.60761691573971
10 4.72155278223273
11 6.19312109669575
12 7.44902354736756
13 8.34004580148524
14 8.86116737994343
15 9.1181140510439
16 9.16336308988143
17 9.23590445817197
18 9.36212212309034
19 9.42536769884915
20 9.4376480888487
21 9.46304212898129
22 9.50453265865311
23 9.47719130567564
24 9.46301880993057
25 9.5196783763914
26 9.55378510130704
27 9.62793091789739
28 9.73452565471259
29 9.7765083722471
30 9.74811830431786
31 9.70268548587069
32 9.77787793437748
33 9.82021746286948
34 9.84348098590165
35 9.94163486978439
36 10.0321197680835
37 10.1315575582112
38 10.1694194127282
39 10.3075734275498
40 10.5179357049678
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.329982207576019
1 -0.0909732759030377
2 -0.604544699657822
3 -0.85994508463763
4 -0.563064217791923
5 0.326114509834408
6 1.30468748634426
7 2.10734387373124
8 2.93514444698741
9 3.87926140230039
10 5.0800955813507
11 6.58347799712702
12 7.78555453880385
13 8.52408189368711
14 9.03128664986784
15 9.24527793758925
16 9.1976549294344
17 9.28352888677251
18 9.3456166721828
19 9.39538832898895
20 9.42697578139469
21 9.43931729592145
22 9.41030895596388
23 9.39498330840181
24 9.3902472595019
25 9.37055746646874
26 9.39626865168304
27 9.45327375011283
28 9.50307695494135
29 9.49365272925302
30 9.47961568014658
31 9.4314819146855
32 9.41177780113623
33 9.44744658538854
34 9.44589220835378
35 9.4973556966314
36 9.51613115922668
37 9.53108424914782
38 9.4998385377564
39 9.48776355753059
40 9.53510599678761
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.281803173597244
1 -0.122901224255362
2 -0.64753370548896
3 -0.903422100886355
4 -0.651278572589025
5 0.254944250522804
6 1.24572577249995
7 2.05780678141905
8 2.84340070063669
9 3.79425650930454
10 5.00391550196251
11 6.56808009973988
12 7.734561015677
13 8.51632226233882
14 9.03389190718448
15 9.24649888273146
16 9.268205973825
17 9.28729848949744
18 9.31841252719575
19 9.32169586155542
20 9.31165054387738
21 9.35338255662337
22 9.33839526169513
23 9.3090437402383
24 9.29279989317994
25 9.31548887855294
26 9.33720154369971
27 9.3284952946203
28 9.38094718128623
29 9.34801623209736
30 9.28704560533764
31 9.24057388782602
32 9.2494241887037
33 9.2179954809364
34 9.16234467504108
35 9.15880292472529
36 9.16965996770563
37 9.10536215628937
38 9.08049699707082
39 9.07677999587716
40 9.0348062742201
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.293152837999189
1 -0.0996208228570858
2 -0.620286295868404
3 -0.861818715497512
4 -0.552077635995341
5 0.377905534686275
6 1.32277648854087
7 2.09731494751981
8 2.8608303676147
9 3.75082914659868
10 4.95738988943766
11 6.45048972375591
12 7.65815877408149
13 8.43742483852768
14 8.99785353929866
15 9.22752299743938
16 9.20678122012271
17 9.26078492868754
18 9.27194020051208
19 9.25951594194109
20 9.29475666766651
21 9.30385450185293
22 9.26764283933446
23 9.22806264335471
24 9.1930329104133
25 9.22394166909444
26 9.21828251523021
27 9.23923599076147
28 9.31445316305019
29 9.24772938048465
30 9.14228555788156
31 9.10510099621126
32 9.10003765996792
33 9.03831355164517
34 9.01227777710397
35 8.97990497812402
36 8.90929932399067
37 8.79542941783314
38 8.69192785857364
39 8.68333854897145
40 8.65509660351414
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.288788564055668
1 -0.154947455045335
2 -0.666432415757507
3 -0.928748944267907
4 -0.596151766011406
5 0.283874461604244
6 1.23554440717461
7 1.9913195849982
8 2.77460173506205
9 3.68209442536544
10 4.78583380651371
11 6.31060821770096
12 7.48428777900879
13 8.30495466557366
14 8.76638775391635
15 9.00276514417801
16 9.036085752415
17 9.08707069034145
18 9.16555421242759
19 9.16142343948395
20 9.17829467615768
21 9.20250897642886
22 9.22322158591481
23 9.21311108193326
24 9.18447126648902
25 9.23429715742359
26 9.22024544944764
27 9.32444193030059
28 9.37947469230995
29 9.3671713611921
30 9.34003339348316
31 9.28599700635556
32 9.30569173628082
33 9.27506220392614
34 9.24040407629823
35 9.27910576832322
36 9.29183264239844
37 9.28780604518133
38 9.30377187403795
39 9.31189749183091
40 9.36766575223567
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.291698648368566
1 -0.160650774244112
2 -0.707636973496115
3 -0.965545130660894
4 -0.807592536710914
5 0.127114879329419
6 1.11332149486422
7 1.93977637490111
8 2.71557240464813
9 3.6439985262426
10 4.70796843619205
11 6.2654506975915
12 7.52544420729996
13 8.36208612872615
14 8.91890594802288
15 9.18923361507002
16 9.19447330717919
17 9.23899657744273
18 9.29368470151259
19 9.29384783003185
20 9.2830612294126
21 9.29237702614419
22 9.29580235433438
23 9.27388555493173
24 9.24639954535953
25 9.27425221931016
26 9.27699778263074
27 9.30705517142832
28 9.36210765211537
29 9.35389625050989
30 9.31252507857609
31 9.25926370594121
32 9.2868929625112
33 9.27732084816095
34 9.26026999593509
35 9.26209539744011
36 9.27289098741407
37 9.25985529980943
38 9.24363883164742
39 9.27373293382921
40 9.31834062829778
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.275788164130027
1 -0.178321791536475
2 -0.731393623160371
3 -0.963606745457273
4 -0.77812540728625
5 0.130206239376587
6 1.06845840236009
7 1.81163732940517
8 2.5628974365261
9 3.41698315208056
10 4.42501045221074
11 5.91457281626329
12 7.13739745374016
13 7.91867149914177
14 8.50905748092134
15 8.79571934281686
16 8.8462370372756
17 8.81872707125906
18 8.94917626515526
19 9.02115508573258
20 9.00697355195402
21 9.03310280424984
22 8.96889053365844
23 8.97636994986363
24 8.9187856932981
25 8.88348688823661
26 8.92060172573768
27 8.95232047532964
28 8.99334592812742
29 8.96096826045228
30 8.93231231309136
31 8.84454110487605
32 8.80241444811789
33 8.71918307274221
34 8.65442260601916
35 8.60242331904598
36 8.63065024772965
37 8.55351840272078
38 8.43861754688735
39 8.39277876743253
40 8.36464084864522
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.303467230157021
1 -0.0672868435505651
2 -0.62903782944716
3 -0.873440979379257
4 -0.587407532682382
5 0.37969098481824
6 1.41300013791447
7 2.16808625070922
8 2.9502381937724
9 3.90992077844765
10 5.12999872345181
11 6.68538030364817
12 7.76784276846818
13 8.53664874885587
14 9.05640681679227
15 9.29737634897356
16 9.30671446153497
17 9.32771326687743
18 9.33908803061649
19 9.38939099733444
20 9.41668588611262
21 9.46960511985263
22 9.47659091038472
23 9.49626023647502
24 9.49977672741684
25 9.55887486166023
26 9.5397782019839
27 9.58263838357684
28 9.65946301634188
29 9.6631291487022
30 9.68821191282338
31 9.70265388013105
32 9.73800322207201
33 9.76754123098168
34 9.82976127381623
35 9.89691582781681
36 10.0417627068193
37 10.1979488502192
38 10.3739340706533
39 10.6625066253779
40 11.13854616851
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.291085917688085
1 -0.130931623296303
2 -0.655749477863072
3 -0.86989574611278
4 -0.505408399041248
5 0.358655527514175
6 1.32392020056028
7 2.12034934635426
8 2.85787943865393
9 3.76166635105614
10 4.91031657031248
11 6.43147303462227
12 7.6622688391287
13 8.45792027348539
14 8.96486507451267
15 9.19712827183161
16 9.18535608365978
17 9.18014567054309
18 9.24069241256289
19 9.25083562494573
20 9.23771856948303
21 9.22971509038395
22 9.17695828967541
23 9.1482250715822
24 9.05885243296608
25 9.0968963579984
26 9.06601528252875
27 9.0700656716612
28 9.10712370333827
29 9.03109803690078
30 8.99109976721485
31 8.93211767753786
32 8.93250276542647
33 8.93114685893319
34 8.85992910596236
35 8.86074809394582
36 8.87871133726576
37 8.84656942540667
38 8.83283465015159
39 8.77352555179943
40 8.80428109499629
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.32068455670104
1 -0.10751418117863
2 -0.61916216245915
3 -0.835434406996868
4 -0.452440088188432
5 0.439386620848163
6 1.39746661967791
7 2.19678465321981
8 2.87951820135437
9 3.80131294508962
10 4.98968998636056
11 6.50645961340076
12 7.68173332655529
13 8.49383023672359
14 8.99512472651232
15 9.10884661342192
16 9.08967619202769
17 9.09174484923131
18 9.11542721713828
19 9.10439326767679
20 9.07125377041289
21 9.04330768331269
22 8.96335444657393
23 8.94590782555326
24 8.87559592857128
25 8.82679024408272
26 8.78470835818247
27 8.82962305242565
28 8.83657737126213
29 8.78950487828241
30 8.71366506932012
31 8.655536634082
32 8.6319617334755
33 8.58702140530445
34 8.54467467894465
35 8.50779326078539
36 8.49335224917151
37 8.45184377323591
38 8.38860932171598
39 8.40467676701662
40 8.47568200557313
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.278197787717559
1 -0.101282463385031
2 -0.627075189555773
3 -0.905785644761877
4 -0.641179719258482
5 0.326404360708367
6 1.34070967004796
7 2.17695278662492
8 3.02644735719074
9 4.13843087970654
10 5.41482215006878
11 6.90503976191832
12 8.07997202844412
13 8.85227638188032
14 9.38403770405014
15 9.54202754577263
16 9.56737753396132
17 9.65795655888532
18 9.73698915898341
19 9.8035429276505
20 9.87130051832918
21 9.94761327200897
22 10.0283030866186
23 10.113349973924
24 10.1892209093936
25 10.3142344553568
26 10.5243777420185
27 10.8455309764846
28 11.2637357311137
29 11.7702060278693
30 12.4458420988844
31 13.2629313384152
32 14.0490847732513
33 14.8383292027779
34 15.4377775811499
35 16.0248306576325
36 16.5714819491889
37 17.1270946043185
38 17.6066366433331
39 18.1122112382372
40 18.5328964434632
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.320903430770616
1 -0.0918435607120207
2 -0.585693553375888
3 -0.801039008788999
4 -0.486712671029141
5 0.477547094522428
6 1.42506143051623
7 2.17489889223646
8 2.90824928239729
9 3.79729111675661
10 4.89934836574112
11 6.42642613177473
12 7.63302643732025
13 8.50926307807873
14 8.97695387605332
15 9.23286863617809
16 9.28047568134208
17 9.363399934056
18 9.41412289637759
19 9.41770656067121
20 9.4218969207412
21 9.45341540701999
22 9.41572632346858
23 9.36323778157786
24 9.32993934394097
25 9.34606010232505
26 9.34289299196417
27 9.34488284903986
28 9.39670131923729
29 9.36514129577266
30 9.29427025762701
31 9.2752846861144
32 9.31568415469097
33 9.24120805999802
34 9.20112874611268
35 9.24720599959338
36 9.26826927967683
37 9.22885406448195
38 9.15922370044367
39 9.12694425670231
40 9.17235721070359
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.324943268274885
1 -0.13975646620354
2 -0.625705085267994
3 -0.879009573365928
4 -0.602351437054757
5 0.328172270252921
6 1.32906875598
7 2.11331317040146
8 2.90723462921532
9 3.89357696182343
10 5.13551826503678
11 6.66178085078387
12 7.77113582106065
13 8.60769152514603
14 9.10533614900604
15 9.26882536306636
16 9.24410331844229
17 9.27744979984304
18 9.33337866790862
19 9.36921706624111
20 9.39813370618286
21 9.40868824739267
22 9.37502175172185
23 9.35148512276514
24 9.30556974213331
25 9.34320558006271
26 9.32815148453831
27 9.40884637760405
28 9.46815522521996
29 9.47520121220111
30 9.44606728882707
31 9.40403366892088
32 9.42780124956123
33 9.40044232989164
34 9.39789925116023
35 9.42887188261295
36 9.4173268394904
37 9.37148558518965
38 9.36476596612379
39 9.39049712722118
40 9.47486836681255
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.292943724754355
1 -0.119902257986614
2 -0.633051337261356
3 -0.867281552119722
4 -0.586810620863788
5 0.371570912894325
6 1.36433545906264
7 2.11489890369691
8 2.85426614004824
9 3.86159027033348
10 5.13669463455903
11 6.64488862807959
12 7.70214588291339
13 8.4134898490683
14 8.97260807580476
15 9.20282043343308
16 9.27353537574456
17 9.35367415737252
18 9.4196565805524
19 9.44298269652518
20 9.55021617751231
21 9.58455676448107
22 9.63401615397633
23 9.61698381947718
24 9.64708102427074
25 9.75343080732468
26 9.81926030233979
27 9.99628950171838
28 10.2454915568431
29 10.3908024025242
30 10.6004163734243
31 10.8976451642373
32 11.3865242482481
33 12.0949236627375
34 12.978601210806
35 13.7896749203605
36 14.593151636252
37 15.2495198586892
38 15.8553687248531
39 16.4921983418362
40 17.1342407263277
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.288281712469563
1 -0.116319897195992
2 -0.672566501219416
3 -0.964035922359245
4 -0.676603224990846
5 0.150431465207955
6 1.12795889123552
7 1.96546498416775
8 2.78449248424687
9 3.76305699256068
10 4.94966121362138
11 6.51418552908797
12 7.63927514143082
13 8.41173684286268
14 8.96768670478385
15 9.26579856061383
16 9.28376892287833
17 9.38595393695301
18 9.45819595994447
19 9.51099681053608
20 9.5592698290818
21 9.58497868493253
22 9.59200667535634
23 9.55777348860462
24 9.63450910595032
25 9.69462912260037
26 9.75433803766443
27 9.91348427414115
28 10.1476621061599
29 10.283205926595
30 10.4126933485673
31 10.6441451337485
32 11.0056170828085
33 11.500677426502
34 12.0912167886595
35 12.9404630033099
36 13.7739810424852
37 14.5283703333008
38 15.2371078826108
39 15.8779859703957
40 16.407038110213
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.265085400662277
1 -0.184666607402022
2 -0.705859641260708
3 -0.92180536554498
4 -0.608265288403416
5 0.318261912364198
6 1.30246398177024
7 2.06124359356751
8 2.84085171435209
9 3.76439911198905
10 4.94802820076408
11 6.52009059206945
12 7.77010616909151
13 8.56109858886853
14 9.02661396596903
15 9.20444068221082
16 9.20507041172828
17 9.22729347667771
18 9.2945140238296
19 9.33046723549921
20 9.33339632481768
21 9.35640691319049
22 9.29139748779693
23 9.26559491760799
24 9.22647087159466
25 9.21590097993824
26 9.24589636619865
27 9.29370601966118
28 9.35697608524862
29 9.3291536039459
30 9.28312098787099
31 9.2978968585985
32 9.30620527083998
33 9.25301340913732
34 9.24555035044512
35 9.26598997883204
36 9.29954820998047
37 9.26615856787093
38 9.23435664488823
39 9.23974211152377
40 9.33477088033217
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.282700148071383
1 -0.178899092603716
2 -0.739123412636887
3 -0.936297150742279
4 -0.619852861921807
5 0.311226823281427
6 1.25715111598048
7 1.98641222978874
8 2.76904280577176
9 3.72028964365083
10 4.90277396470861
11 6.39189353295076
12 7.61034364860217
13 8.40951736465117
14 8.92468879715224
15 9.19411784325718
16 9.21243632714353
17 9.23363168067214
18 9.31083531551264
19 9.31048592216925
20 9.30383078605019
21 9.34163921370697
22 9.33684210688485
23 9.29722225582976
24 9.26145030560112
25 9.25467479611466
26 9.28696277467144
27 9.36403201785557
28 9.41021934455132
29 9.36842390392202
30 9.3060567366392
31 9.29969061964255
32 9.2849035672271
33 9.25545462013852
34 9.25321150323677
35 9.31458804735112
36 9.33110653100915
37 9.32063014692463
38 9.26857561662572
39 9.23725351048705
40 9.24996971425071
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.305426663916564
1 -0.135070572829134
2 -0.636905366219494
3 -0.87214849346747
4 -0.51609120052637
5 0.450401544927669
6 1.42315482675039
7 2.23282283217274
8 2.95750522499781
9 3.88147289085945
10 5.14186201673077
11 6.67926664894181
12 7.81720878788081
13 8.57726396098173
14 9.12476119037789
15 9.39956763698619
16 9.42887838324016
17 9.51886525242537
18 9.56413447140075
19 9.5826133324546
20 9.63020781986656
21 9.66530073304789
22 9.67523815816266
23 9.66100624330619
24 9.66413043511726
25 9.70966325930253
26 9.77746781166252
27 9.88959252270317
28 9.96418570998539
29 9.9904024917969
30 9.99542881006348
31 10.0694532132237
32 10.1771068868553
33 10.2725807080191
34 10.4823461107694
35 10.7796937165211
36 11.2100694972042
37 11.7223171266721
38 12.4493370856439
39 13.2802393182451
40 14.1208471543849
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.309710623043675
1 -0.0749789340577438
2 -0.597658962096691
3 -0.883789847172906
4 -0.58009015505475
5 0.346893674885164
6 1.34657409480421
7 2.11075455047135
8 2.86911614695299
9 3.81027653482306
10 4.9769077484155
11 6.52707904348232
12 7.68446834507119
13 8.47367288627809
14 9.00804959391785
15 9.19357046056782
16 9.19312152702025
17 9.19021072030234
18 9.22444340682715
19 9.26161104734391
20 9.267285624912
21 9.31409196822171
22 9.30307464476749
23 9.30392228039243
24 9.27085083910244
25 9.31470088735856
26 9.34861988242272
27 9.43887381127959
28 9.50385508713402
29 9.5106059346713
30 9.47394823428041
31 9.43080250004267
32 9.46134868765569
33 9.41157625504505
34 9.40028645856228
35 9.45873319740713
36 9.51236638872427
37 9.49771904114118
38 9.50358777101204
39 9.51249813661398
40 9.59151698296221
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.298539290367163
1 -0.092370863299704
2 -0.629351682630606
3 -0.856584291200774
4 -0.506531310222152
5 0.359777203255376
6 1.33459316479416
7 2.13600611128872
8 2.8389134616572
9 3.69957142976522
10 4.75964691968428
11 6.32589627053342
12 7.54771679259683
13 8.37574834323915
14 8.95523282756844
15 9.227594184845
16 9.26376878890901
17 9.32214588084683
18 9.37425692925018
19 9.38158089257187
20 9.42211309569623
21 9.45472107973342
22 9.41190778473886
23 9.41313605770089
24 9.42009372042668
25 9.42242257383431
26 9.47189979248421
27 9.55500739772204
28 9.62247369036568
29 9.58298253038489
30 9.53292880076148
31 9.53152021134047
32 9.5719891088338
33 9.51935180489272
34 9.5104728309406
35 9.58449385739623
36 9.59889775219117
37 9.59553104541278
38 9.55197808430438
39 9.60700839118046
40 9.69736709303827
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.319534376369913
1 -0.114329010419369
2 -0.616047423482674
3 -0.846748459327954
4 -0.480303131443496
5 0.458597690094051
6 1.40588564634515
7 2.1946286739053
8 2.94571703365131
9 3.84865406909419
10 5.02191001551835
11 6.5604505287028
12 7.73784381287747
13 8.47383378449571
14 9.02499962518499
15 9.24102429826524
16 9.26482076079733
17 9.33411487651104
18 9.38698698692286
19 9.43772343854994
20 9.42728928557667
21 9.42728923889309
22 9.44292590046613
23 9.45126657977613
24 9.42333659652713
25 9.49892873532108
26 9.51409080517076
27 9.558349160824
28 9.6553459944662
29 9.63509256014969
30 9.57219199658196
31 9.53120466708292
32 9.53422659674496
33 9.51426769516489
34 9.50281630671103
35 9.59133286914468
36 9.56589702687697
37 9.52931793097769
38 9.47940408665694
39 9.47341021874709
40 9.53068421465801
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.295889657120085
1 -0.155913017000689
2 -0.63742718561509
3 -0.818259123194195
4 -0.468747879084003
5 0.445303628638481
6 1.39515750627616
7 2.18218615568546
8 2.93628274513139
9 3.85117766774221
10 5.07959136332816
11 6.56582520868999
12 7.69699188064268
13 8.46588639321242
14 8.93197725521579
15 9.11376128896851
16 9.11942225258776
17 9.19468072851187
18 9.22090667962527
19 9.21068733413786
20 9.16983299159386
21 9.24231717477114
22 9.24415609690871
23 9.22734652618467
24 9.19776821622537
25 9.23977470113712
26 9.30947576432945
27 9.37568304684022
28 9.43559891516791
29 9.40685914123181
30 9.38152791623417
31 9.36363962062101
32 9.36636464278289
33 9.36223482834476
34 9.32558835415209
35 9.36606842073307
36 9.4144545453187
37 9.37526677157315
38 9.36888329622317
39 9.42838560580657
40 9.43938711659644
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.279495707362869
1 -0.124005642515305
2 -0.699343258924151
3 -0.92437977439968
4 -0.674413782793051
5 0.189033652668936
6 1.18967486488345
7 1.96022361264237
8 2.7220693405634
9 3.67910028599588
10 4.91736901833889
11 6.41948611512471
12 7.63525607695695
13 8.39800407900329
14 8.91342172179521
15 9.14848641850312
16 9.14868206208802
17 9.21216591253588
18 9.29511194172684
19 9.33443605885052
20 9.3669220185769
21 9.41716595833369
22 9.44792810014504
23 9.47265569836994
24 9.50357172368818
25 9.52283043285383
26 9.57069718913005
27 9.70364941805469
28 9.8774673546065
29 9.90060955625452
30 9.89203864431549
31 9.84751579493735
32 9.87056082695081
33 9.86425625322037
34 9.81658186241081
35 9.85079861684942
36 9.88282078583521
37 9.86935751166968
38 9.84741159840584
39 9.89883752615831
40 9.96721605039749
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.327743006028031
1 -0.0763362334363795
2 -0.596127823174935
3 -0.784326413851418
4 -0.454165596295356
5 0.429934537588356
6 1.38315324640991
7 2.15778597513332
8 2.89382164475837
9 3.85830662820619
10 5.01955464748786
11 6.5435584241954
12 7.72917620938684
13 8.47910356723241
14 9.01473130689316
15 9.23042207620997
16 9.23857966626616
17 9.30287767538483
18 9.29473365278741
19 9.2979617057404
20 9.30316555928083
21 9.2694519774836
22 9.27403767844335
23 9.26245738567185
24 9.27775647612833
25 9.30683437941866
26 9.31266998114296
27 9.39645099041296
28 9.4058684236488
29 9.33424406354843
30 9.24092953217515
31 9.19616290754247
32 9.15917652906958
33 9.07219478587731
34 9.03541878467998
35 9.05427606127387
36 9.0583519178478
37 9.01313935219016
38 8.98721797029491
39 8.98111046800784
40 8.97703646071276
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.26404146432442
1 -0.171668378922071
2 -0.701467875370122
3 -0.926215150810378
4 -0.649584793636124
5 0.303613281350982
6 1.25008945122637
7 2.07229232803219
8 2.86689176144914
9 3.8582356269421
10 5.10201670981043
11 6.59027810113844
12 7.69767134602229
13 8.49100149942
14 9.00209462867023
15 9.20463328853293
16 9.23201219118275
17 9.286489914885
18 9.34745645454603
19 9.36349164999123
20 9.399381512259
21 9.41699710118312
22 9.38578362897209
23 9.35075393188995
24 9.34667061034983
25 9.35341300744229
26 9.34942806747095
27 9.39292971757031
28 9.41646920147845
29 9.40839128279296
30 9.33005084567935
31 9.26309493031032
32 9.27996297815436
33 9.24169728137434
34 9.23239091365473
35 9.27645443929039
36 9.29862258725201
37 9.2794650826586
38 9.20824278645331
39 9.19909646578514
40 9.21938144166312
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.292675705223323
1 -0.16176475888558
2 -0.699347547176402
3 -0.946340772652202
4 -0.615138443639395
5 0.324319909109485
6 1.31293638670147
7 2.0865988767539
8 2.86879324482354
9 3.87645715440444
10 5.09073654640957
11 6.66327136010294
12 7.8507769787202
13 8.65650296866921
14 9.15181235610584
15 9.35171679561659
16 9.37281537604259
17 9.4587447661626
18 9.5697866719113
19 9.59937136404953
20 9.56978974893687
21 9.62717472278807
22 9.68838540337383
23 9.71356908859969
24 9.71197686100295
25 9.75035696030245
26 9.77971964883135
27 9.87959056728454
28 10.0144083400182
29 10.0406178457288
30 10.0977214683527
31 10.1172792117206
32 10.1576762199718
33 10.24107860221
34 10.2662793892631
35 10.3941341038519
36 10.6350139358968
37 11.0519307779207
38 11.6672713335776
39 12.4654420820115
40 13.3524473815103
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.315790783314403
1 -0.124576381652901
2 -0.619780279042376
3 -0.830725593474963
4 -0.520841590561108
5 0.403460067049619
6 1.41683837959117
7 2.20101784742814
8 3.0174189886255
9 4.0207584736165
10 5.35243583667856
11 6.84187441328883
12 8.02345441378701
13 8.74987220694871
14 9.29336428261288
15 9.55093754895018
16 9.53438782200958
17 9.61541743032781
18 9.65430623735967
19 9.65293474216552
20 9.68450262944048
21 9.66815905873896
22 9.60073051805537
23 9.55602278403782
24 9.58313725831523
25 9.62192473529467
26 9.62668935751591
27 9.71618891778749
28 9.76962619282149
29 9.75860213720754
30 9.73096780792268
31 9.73088618910861
32 9.72998429543617
33 9.71691670629061
34 9.73511300800599
35 9.77423896260109
36 9.78990946678569
37 9.78393307490715
38 9.74565825426324
39 9.8157828284714
40 9.82638897678234
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.291945064973409
1 -0.157190589154787
2 -0.67334523851102
3 -0.94841026454794
4 -0.721357776575218
5 0.189622923741908
6 1.1637697343296
7 1.98679408985484
8 2.79411771898388
9 3.75982585574468
10 4.97842093107718
11 6.50755693991049
12 7.68799503941974
13 8.45743327519761
14 8.94536004684557
15 9.24717418287175
16 9.28015903449663
17 9.36195584543857
18 9.40613388382259
19 9.4301432643894
20 9.49144244130705
21 9.48191007689663
22 9.47155115131149
23 9.42049504597856
24 9.41176932662633
25 9.46904210036069
26 9.46569117112736
27 9.565541521821
28 9.65025599676886
29 9.63036373821018
30 9.58111563932857
31 9.55268142865371
32 9.55190909716287
33 9.51398163098874
34 9.53094563857979
35 9.59118999085415
36 9.65869896056673
37 9.63926799286439
38 9.65838269120981
39 9.66883206772533
40 9.77051172392748
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.287956598786423
1 -0.144992327606211
2 -0.679405516101288
3 -0.949008418555534
4 -0.669766117581958
5 0.227767321753038
6 1.23099373323246
7 2.01055058168143
8 2.74930904981507
9 3.71063422524851
10 4.94199027635375
11 6.47160359319947
12 7.65161831546522
13 8.38358650514958
14 8.94938751857669
15 9.19436826890492
16 9.12448521928566
17 9.17887985506209
18 9.25203847156579
19 9.29139636095176
20 9.31381305917
21 9.32462970194962
22 9.31491140239057
23 9.29153154251389
24 9.25974929395948
25 9.24963659321598
26 9.22493294897425
27 9.24768596345098
28 9.29308032055285
29 9.20939206818295
30 9.14863704465713
31 9.05118411775541
32 9.01447636483246
33 8.96713020080315
34 8.89203748336463
35 8.88329213412699
36 8.95388974194631
37 8.90660547113022
38 8.82435488368159
39 8.77079911189982
40 8.80231534817576
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.304703194562689
1 -0.080405954010295
2 -0.622086603467504
3 -0.843082996353471
4 -0.481635013458926
5 0.458814686255331
6 1.42373764332034
7 2.2080786973221
8 3.010601605134
9 3.95901352675496
10 5.19831481941008
11 6.73900450814461
12 7.88491139560609
13 8.64662446400708
14 9.17585052798958
15 9.38590220371832
16 9.36806072743152
17 9.38582539794705
18 9.44014934867861
19 9.48797530587946
20 9.53267087796584
21 9.57624274888325
22 9.56633978262536
23 9.54102804998972
24 9.50406606222142
25 9.54648038057717
26 9.58499093045664
27 9.69963604962044
28 9.7789692176527
29 9.74318117814379
30 9.71833309840217
31 9.72005191804445
32 9.75169745115748
33 9.71801341338502
34 9.72960829613905
35 9.78505096610418
36 9.83356603359274
37 9.85010691757806
38 9.83089146443284
39 9.87971090738424
40 9.97193029652235
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.321084649170565
1 -0.130376762652518
2 -0.642148083789047
3 -0.833946952067597
4 -0.462561899573902
5 0.507682609754044
6 1.50019769220811
7 2.33124836852971
8 3.13235165741835
9 4.11198512872255
10 5.31289705439502
11 6.84466657110501
12 7.99680413765783
13 8.68393426788491
14 9.19009150764554
15 9.39343902101223
16 9.42560163962994
17 9.46753831052357
18 9.60543360623178
19 9.67193904605229
20 9.67943124594271
21 9.70841148437727
22 9.72516032652609
23 9.74938633591501
24 9.69638423246006
25 9.74045040426594
26 9.81184023779118
27 9.91832392105315
28 10.0369432073708
29 10.0818435405875
30 10.0857533672649
31 10.1094045952294
32 10.143345709147
33 10.2153820078789
34 10.3141520184061
35 10.4789885536903
36 10.6695850260346
37 10.9360305726699
38 11.2964652083772
39 11.9308549463079
40 12.6357520924787
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.320457720678476
1 -0.117495840253633
2 -0.645441863310632
3 -0.890351929500993
4 -0.565416095240928
5 0.370068390538059
6 1.33326357084957
7 2.12846738573764
8 2.86017644622225
9 3.79021753268561
10 4.9742589775522
11 6.49242704132006
12 7.69795835146689
13 8.5249514256814
14 9.01568002328132
15 9.23436759063979
16 9.25736059465878
17 9.29982974110455
18 9.36692332616238
19 9.36391781820863
20 9.45233043481867
21 9.51150096840485
22 9.53030155114986
23 9.55489287393586
24 9.55977415737889
25 9.5906425377531
26 9.6427085718539
27 9.72240870702499
28 9.82230296304224
29 9.85859070818567
30 9.8533480335817
31 9.93094106161563
32 9.99638874364602
33 10.0830011192551
34 10.1272754866952
35 10.3177573424048
36 10.6555612957624
37 11.0613387399033
38 11.6887949029837
39 12.5247418596636
40 13.4434434418156
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.337019527709389
1 -0.0962598586016115
2 -0.595281851650704
3 -0.839840564133004
4 -0.521933614214254
5 0.404272310655761
6 1.39186015962025
7 2.19008855539123
8 3.01096789958938
9 4.00076221652444
10 5.32405386426157
11 6.88254273914107
12 8.00140165921348
13 8.77697308231144
14 9.27323732903251
15 9.51587731270818
16 9.51589532171162
17 9.56175907296043
18 9.6537990606941
19 9.70591440624768
20 9.6875012483223
21 9.74292591590842
22 9.76763400912859
23 9.7362661831967
24 9.73452000138128
25 9.80124320348061
26 9.82685098734164
27 9.87973682838724
28 9.98651685856706
29 9.99291347942458
30 10.0525502597294
31 10.0623635290331
32 10.1230330302393
33 10.1959376092548
34 10.2327004809708
35 10.3812461548067
36 10.6596453290051
37 11.0022465997903
38 11.526946315986
39 12.2401982774909
40 13.0767305944594
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.299092983208492
1 -0.10976804542163
2 -0.630945063028957
3 -0.893155556652325
4 -0.597938679717795
5 0.328565920748527
6 1.31927390183386
7 2.11846644876039
8 2.92848167472988
9 3.91861678365945
10 5.17951963801349
11 6.73735398146709
12 7.92171136498052
13 8.70690109259026
14 9.17546725792503
15 9.31231468316887
16 9.3004444742587
17 9.34859595031904
18 9.38817800207922
19 9.4174839105622
20 9.43738664827317
21 9.43119364221134
22 9.41601243913805
23 9.40646951203846
24 9.38688924885737
25 9.39420550357452
26 9.3848170455161
27 9.45290246057092
28 9.48323411366531
29 9.44869535170736
30 9.42688312976517
31 9.39328159468619
32 9.39520916418212
33 9.36552315705149
34 9.35702214088423
35 9.39745172033009
36 9.43214101809351
37 9.42052862365635
38 9.41221064498402
39 9.45854621148751
40 9.49724622084068
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.310762244823588
1 -0.118531350107986
2 -0.672735851243384
3 -0.88765619506497
4 -0.578199933941931
5 0.360251931998985
6 1.30302421294508
7 2.18497565134509
8 2.99507447674171
9 3.97264825818849
10 5.20425677112537
11 6.79404971457515
12 7.9570925747423
13 8.7217261520868
14 9.24455037153665
15 9.51281628161724
16 9.52993458343038
17 9.60636189058152
18 9.67257302112541
19 9.69403950337694
20 9.73525211279016
21 9.7634306223932
22 9.7905583052108
23 9.76355811869905
24 9.77462005143761
25 9.79856072620346
26 9.83875938042359
27 9.94285416420524
28 10.0060787165147
29 10.0050292348888
30 10.0037840883229
31 9.95681939474714
32 10.0080522924874
33 10.0111552716623
34 10.0311237939447
35 10.1009635765002
36 10.1935384971769
37 10.2968557014108
38 10.4300692421471
39 10.658052639172
40 11.0341225181994
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.299878329955934
1 -0.0892029645679755
2 -0.653561875682821
3 -0.934941900436539
4 -0.714100421482275
5 0.113249076401095
6 1.05956030692965
7 1.82825237967268
8 2.56117516118917
9 3.31719506364404
10 4.16054999002571
11 5.50613930534006
12 6.7462284251415
13 7.71947298036941
14 8.40376550850837
15 8.76018592544061
16 8.87429482015657
17 9.02048949349707
18 9.112948087819
19 9.21355215504581
20 9.27006117271942
21 9.33867888406608
22 9.33347199832151
23 9.30847292436491
24 9.31482158176823
25 9.31312550365776
26 9.34143241464616
27 9.33090743303178
28 9.38982183464634
29 9.31252644603648
30 9.27073762817959
31 9.24354801565939
32 9.27222361712482
33 9.28224042154373
34 9.27088621102887
35 9.29602272259791
36 9.32245643225004
37 9.30005857257405
38 9.29938395230289
39 9.32617213095676
40 9.36226605956013
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.260959127147436
1 -0.153779291208023
2 -0.650483614217419
3 -0.971365857721241
4 -0.667539015364913
5 0.286245423828784
6 1.27364278621319
7 2.08991208611257
8 2.8340333676746
9 3.80421377459092
10 5.06458812005986
11 6.63375500283297
12 7.77057683964115
13 8.50858082812271
14 8.99942067277017
15 9.1773439458376
16 9.10903247645415
17 9.16021879046341
18 9.15362555310249
19 9.13115518077823
20 9.09619139666056
21 9.12463696242143
22 9.06962610874485
23 9.06092776890542
24 9.03166422785906
25 9.03266900230093
26 9.00230502267181
27 9.01288921472394
28 9.05635457632996
29 8.9880450920602
30 8.92382153607147
31 8.8386100324269
32 8.76819349019677
33 8.71326416779835
34 8.64365483749221
35 8.59487220315477
36 8.57341804401648
37 8.50160794535513
38 8.41358914878854
39 8.3385814414455
40 8.35050525472447
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.294758675637378
1 -0.155580141887118
2 -0.675652783892759
3 -0.950753947849636
4 -0.60021078919649
5 0.33879551049034
6 1.33563390268073
7 2.16201549942176
8 2.89976655211253
9 3.803629071798
10 4.97113783294224
11 6.50473719259852
12 7.72517862450288
13 8.52449753148648
14 9.01665803597442
15 9.19381187298539
16 9.16481032672974
17 9.21385352771813
18 9.2714823683036
19 9.26412614616855
20 9.26960198854204
21 9.28236775366233
22 9.25026649323771
23 9.1911749407476
24 9.15958287345959
25 9.17029883059806
26 9.13280762288726
27 9.14886047350798
28 9.21594265673681
29 9.15007139475993
30 9.06450300351552
31 9.00194629981799
32 8.93855873380212
33 8.85156792469075
34 8.78458111632537
35 8.81011033363846
36 8.78545868382682
37 8.71794140112654
38 8.64982218560871
39 8.63224702276312
40 8.63807260679373
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.299868017912356
1 -0.114016322171083
2 -0.611450416241822
3 -0.851135850438491
4 -0.50168461802793
5 0.43143507051556
6 1.31904941265688
7 2.06953976169133
8 2.79886689399884
9 3.72758999287137
10 4.8980731936674
11 6.38843848748104
12 7.57035036339304
13 8.43288175979291
14 8.88347698074568
15 9.12747285384745
16 9.11762624813493
17 9.12226890596016
18 9.17753023233271
19 9.22020425117775
20 9.24825341345219
21 9.22270765953059
22 9.18574404061975
23 9.19762390548779
24 9.2015523606567
25 9.17378569470062
26 9.16433734557563
27 9.14875477158676
28 9.21323342905744
29 9.19478661754671
30 9.16029838251243
31 9.113136792968
32 9.05825122200857
33 9.0191851596108
34 8.9828876502508
35 8.95222253424768
36 8.94525335339203
37 8.92274443681818
38 8.83323774192094
39 8.75933522715632
40 8.74224943224281
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.28614123629279
1 -0.119441525692289
2 -0.631997558178476
3 -0.903382302747097
4 -0.60485139420566
5 0.309961662390285
6 1.27560733946194
7 2.04210627764172
8 2.79178731240512
9 3.6937063595537
10 4.89698904710388
11 6.40872102654572
12 7.57225356546695
13 8.31721563050004
14 8.83144721092118
15 9.06776667599412
16 9.05467190650879
17 9.04231667372492
18 9.07442871660686
19 9.0630009727479
20 9.02165283057211
21 9.02133341630356
22 8.99384853181915
23 8.9769442352998
24 8.90458005967604
25 8.88888981884502
26 8.87748374818847
27 8.91025143630772
28 8.95392926039723
29 8.91532449593362
30 8.89422051355225
31 8.85324444793397
32 8.7889046834105
33 8.74989188943654
34 8.66715776896777
35 8.61686665584887
36 8.621214168638
37 8.54453863309581
38 8.51998230834183
39 8.5115310079216
40 8.5005895209424
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.281874652720011
1 -0.148970054779046
2 -0.692322827350788
3 -0.933522519010297
4 -0.648974063809262
5 0.297565882161328
6 1.31581705126912
7 2.10013376926921
8 2.8482668147626
9 3.77343840896855
10 4.96287184417638
11 6.45029105483355
12 7.69275933529672
13 8.43965587341864
14 8.95897573910623
15 9.22399045015817
16 9.21134807705808
17 9.27124672368529
18 9.31768139529261
19 9.31074731772942
20 9.30330294124227
21 9.32092841960501
22 9.32417033406949
23 9.2687581992308
24 9.27626695991168
25 9.31930661970045
26 9.31830691890802
27 9.39021933185393
28 9.48002639633736
29 9.46219251553926
30 9.38827933855623
31 9.38671735278458
32 9.37043202611257
33 9.33105491057752
34 9.31209968934475
35 9.34414275839809
36 9.34778277736688
37 9.31009449117543
38 9.27827493831591
39 9.29029162528215
40 9.33562976550927
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.327509447715588
1 -0.0416511664180939
2 -0.554969311910812
3 -0.837176453885264
4 -0.577106783893626
5 0.310000238182745
6 1.28995268517071
7 2.09150208383176
8 2.82833456199285
9 3.80246271458946
10 4.96110090291097
11 6.52717240148446
12 7.67876688541918
13 8.46190646758945
14 8.98310949469763
15 9.12072150480067
16 9.06269904865548
17 9.02000491066945
18 9.04379872779537
19 9.01439169538223
20 9.03239104126297
21 9.01791613258235
22 8.92475698542998
23 8.8607135294167
24 8.78056363374567
25 8.71091850197653
26 8.66279172178798
27 8.64329949596278
28 8.6380443301928
29 8.54413414101912
30 8.40557866672473
31 8.30254477193582
32 8.19873867808304
33 8.07793220261004
34 7.96673718899185
35 7.85234000019105
36 7.77191603855686
37 7.60645309114415
38 7.52469135876581
39 7.43885679112274
40 7.35387888638599
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.260852243899618
1 -0.197016166833355
2 -0.72726766147785
3 -0.930131605147081
4 -0.638327557956999
5 0.257198639073548
6 1.23134022162881
7 1.98935952367247
8 2.71459856066401
9 3.62466657945317
10 4.79764146155715
11 6.30584053803327
12 7.54297422468116
13 8.42101879627685
14 8.93042297241405
15 9.26176569907721
16 9.29113508018477
17 9.32833334299354
18 9.41055527648829
19 9.45634379261744
20 9.44028431290807
21 9.42593022102981
22 9.39349108694319
23 9.36446137125952
24 9.34327041995037
25 9.36677545669849
26 9.38162538865635
27 9.42400576058888
28 9.50073684510699
29 9.46115934759358
30 9.40577007008684
31 9.31908252104885
32 9.32539861213411
33 9.33138356620432
34 9.24928569013042
35 9.26993862688781
36 9.31430264824341
37 9.34117471294165
38 9.26958294318783
39 9.25402951542451
40 9.30098961634254
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.29298119028434
1 -0.151071207680164
2 -0.646532113907263
3 -0.907921117666218
4 -0.610124439713774
5 0.35126854307432
6 1.34060444063035
7 2.15969949947723
8 2.86932135634024
9 3.77937091056558
10 4.97869383937287
11 6.48280690631657
12 7.72262845083646
13 8.52062835467469
14 9.11247485795653
15 9.34539231561453
16 9.36756867127395
17 9.398198696998
18 9.47634101970202
19 9.51790854292748
20 9.55275558188866
21 9.59963038423975
22 9.59594599528069
23 9.59523317462016
24 9.56444793392463
25 9.602686580117
26 9.65116054124638
27 9.77364134464564
28 9.777777164237
29 9.74424776372449
30 9.73692150796923
31 9.74354591870934
32 9.72828756209571
33 9.72137149726137
34 9.74962543225786
35 9.76908008367414
36 9.75623029006442
37 9.6878198908511
38 9.68449676867577
39 9.72593954711114
40 9.78220083591884
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.310545301578272
1 -0.0941885553718609
2 -0.612432600727193
3 -0.875336892956265
4 -0.577300365985305
5 0.316818567021449
6 1.30249822023742
7 2.08392389256461
8 2.7936200959924
9 3.71084596122014
10 4.92465060902402
11 6.53450244226988
12 7.75432116173215
13 8.42468390881663
14 8.93980331380823
15 9.21266818624149
16 9.21889959635662
17 9.32696413371822
18 9.40409500738745
19 9.44409372202599
20 9.47262282243278
21 9.48285768959763
22 9.44635235357614
23 9.44458881265872
24 9.43800403168667
25 9.44393187701678
26 9.45161758866058
27 9.4142225817399
28 9.41510942175356
29 9.41749995031011
30 9.39565261971097
31 9.33104763057154
32 9.31526766028465
33 9.29222635857733
34 9.28309056446357
35 9.31374807522394
36 9.32707573402287
37 9.25912080757588
38 9.2135753860173
39 9.24069241518032
40 9.24326183197934
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.285762907301572
1 -0.133102341006684
2 -0.625078178544305
3 -0.846720385898074
4 -0.556346030387481
5 0.399995263316697
6 1.37334442656745
7 2.17133491626247
8 2.92706087172983
9 3.89436651399357
10 5.06997792179214
11 6.6505590273812
12 7.83395988229377
13 8.71391346897408
14 9.22478051300083
15 9.41285094641211
16 9.42507063339663
17 9.52821872627452
18 9.58833063851446
19 9.66869156401851
20 9.6975433785557
21 9.75093421713196
22 9.73068404413911
23 9.73802232399358
24 9.70975968348134
25 9.81227963000643
26 9.90127948839858
27 9.9507442328407
28 10.1215086479647
29 10.1737668712002
30 10.2286456085693
31 10.2206242913617
32 10.3716637303193
33 10.6086027773191
34 10.8139829819095
35 11.2237849120676
36 11.8032029695389
37 12.4596993478992
38 13.198132605093
39 13.961757234429
40 14.6809444854312
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.290471253047921
1 -0.134139740008982
2 -0.629312289513952
3 -0.918380021358519
4 -0.642629046505096
5 0.245241799670091
6 1.2181258556838
7 1.983161595976
8 2.80187209212617
9 3.68666938402025
10 4.78993553903321
11 6.32661715141218
12 7.56442556884175
13 8.33839374838481
14 8.900027496835
15 9.23478695273428
16 9.25715427270302
17 9.43287513506906
18 9.54710331633524
19 9.65812240054953
20 9.80644646706667
21 9.93651725778034
22 10.1025794770234
23 10.2541809195032
24 10.567689956141
25 11.0224276981178
26 11.5890171402599
27 12.367715670021
28 13.1844999248182
29 13.9901652301748
30 14.6635415702085
31 15.3150599646821
32 15.7683365422176
33 16.2964997007683
34 16.7383343497236
35 17.1372172153199
36 17.5353788619118
37 17.8950825234196
38 18.2480985258373
39 18.6018419095622
40 18.9659088346797
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.311455162001243
1 -0.0833692033997635
2 -0.615423071940215
3 -0.858572324917959
4 -0.55363730260886
5 0.348954699580147
6 1.33959165102895
7 2.11752820208373
8 2.87495671523269
9 3.87294467543229
10 5.08442932411231
11 6.58178140835274
12 7.72622535626506
13 8.47420095901101
14 9.00105890219391
15 9.25313604336998
16 9.30507520674704
17 9.41803176922091
18 9.43826972581589
19 9.46301881225268
20 9.49563200630948
21 9.53929760465323
22 9.54388166234829
23 9.51412374991541
24 9.54089661432774
25 9.56436505032828
26 9.53778140639417
27 9.70773201768827
28 9.80746531058286
29 9.77005152475058
30 9.71316231868291
31 9.7476109729905
32 9.7339048763156
33 9.75401914531988
34 9.75197374615135
35 9.8148801918356
36 9.82132021208711
37 9.79768165180328
38 9.79679353482282
39 9.88050268473779
40 9.93373654436222
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.28270033261182
1 -0.131800534547438
2 -0.709931551431457
3 -1.00876464349013
4 -0.706281117092037
5 0.199297677406432
6 1.1577554563429
7 1.98499049998731
8 2.73404531797148
9 3.63763401453801
10 4.82104572856646
11 6.3235581362955
12 7.59196304789766
13 8.3787970085202
14 8.90950797840397
15 9.24087376870076
16 9.28551550401954
17 9.35037258746457
18 9.45007128614535
19 9.51083457969018
20 9.56115086871376
21 9.58615824856519
22 9.62308066307201
23 9.61039660819501
24 9.63032158898492
25 9.71853371831872
26 9.78151544522097
27 9.89869099842789
28 10.01401691002
29 10.065854779643
30 10.1061135675169
31 10.1431499037716
32 10.2369775203648
33 10.3194748832429
34 10.4085991940937
35 10.617085440185
36 10.8709021131448
37 11.1958315696597
38 11.6891995521726
39 12.313806849472
40 13.0241511205028
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.301754610153997
1 -0.12949031566306
2 -0.638260511900011
3 -0.912688203289753
4 -0.600124978922297
5 0.355532931370824
6 1.31297900762415
7 2.10305751938326
8 2.84156129666072
9 3.72265067202575
10 4.85843621929473
11 6.41836154524106
12 7.62262426986384
13 8.38624790657129
14 8.91463741891666
15 9.10641533145877
16 9.10025235230793
17 9.17218672953067
18 9.20488475555254
19 9.22931198594713
20 9.32572588897714
21 9.38818628841507
22 9.41765282330469
23 9.46114035079662
24 9.47435331124995
25 9.56527968634584
26 9.62112922053109
27 9.7226605401774
28 9.84552636147949
29 9.84688430834084
30 9.83960364773344
31 9.82208712369215
32 9.89995488567259
33 9.95364739969741
34 9.94906722903039
35 10.110294950518
36 10.261537447703
37 10.3942247848284
38 10.5195352985365
39 10.7373307807034
40 10.9962319566781
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.286406081648026
1 -0.134897490147933
2 -0.644804276110532
3 -0.856191249475857
4 -0.54820609764029
5 0.394894931286946
6 1.34747596387175
7 2.13950021353918
8 2.90550260314461
9 3.83924427275251
10 5.01866872967433
11 6.57233138000217
12 7.67966193898294
13 8.4206582196407
14 8.9081689942242
15 9.14411742502144
16 9.15510600481213
17 9.15107636657125
18 9.20012944153162
19 9.18545721480774
20 9.18443835785861
21 9.20033126471898
22 9.16195157215242
23 9.15923298914102
24 9.12038823033779
25 9.10863568541928
26 9.10986074723396
27 9.16919924386465
28 9.1913612836957
29 9.13420481300848
30 9.08159646945906
31 8.98577297266805
32 8.97239455879884
33 8.9380779937516
34 8.91110066419554
35 8.90153126781876
36 8.92376220735961
37 8.89152218589799
38 8.83042030402022
39 8.81538574615194
40 8.87804430343601
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.304349452110053
1 -0.128568248142951
2 -0.676648147900675
3 -0.914623101503693
4 -0.596405532829596
5 0.344702088786611
6 1.31502881714138
7 2.10164338933599
8 2.90969269511034
9 3.88803303208927
10 5.14129797379496
11 6.66335964233785
12 7.77065073253284
13 8.56368549862087
14 9.05590602384953
15 9.2556080763788
16 9.22210482362076
17 9.25388959112546
18 9.32397630988704
19 9.32386015503544
20 9.33808795511388
21 9.31626913545754
22 9.28276799538703
23 9.21491855965814
24 9.16018892010459
25 9.1729149414893
26 9.12997998902484
27 9.1561642029359
28 9.10655449916599
29 9.05120779411873
30 9.00575610120193
31 8.94532748938028
32 8.92446240366293
33 8.91633445168242
34 8.85898544943326
35 8.85308543977379
36 8.87485310005006
37 8.81662765030232
38 8.78016234835832
39 8.72763667905976
40 8.73374712388347
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.284263582765185
1 -0.145720747973014
2 -0.712626188097632
3 -0.98720060412432
4 -0.761482830788734
5 0.0511364186619501
6 1.03466335222203
7 1.85555045789884
8 2.61671868637053
9 3.57944260179168
10 4.69581822892294
11 6.27089202673126
12 7.57204476594537
13 8.47320689031287
14 9.00974517793044
15 9.27208037787058
16 9.3208003969366
17 9.37430531331663
18 9.42666753641355
19 9.44059458896777
20 9.46546182158402
21 9.46060159715966
22 9.46493746520503
23 9.44995728664851
24 9.45162227775171
25 9.5180703922571
26 9.55091470399403
27 9.66210051908269
28 9.73734671450534
29 9.75469708403797
30 9.70901838823711
31 9.74287924840662
32 9.77154251201256
33 9.81887349558565
34 9.87993639790622
35 10.0173218306023
36 10.1250601387119
37 10.2532192829021
38 10.4183112431179
39 10.6531043333849
40 11.0517486679197
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.302314672834213
1 -0.172277791222662
2 -0.699603580559373
3 -0.973568875691458
4 -0.706579417463517
5 0.234420155785708
6 1.25349620227073
7 2.14624430018339
8 2.94110548543776
9 3.87746227994207
10 5.10587106533008
11 6.65528779683935
12 7.78356607895802
13 8.50588521446632
14 8.99838340947315
15 9.1602630356582
16 9.18014991199796
17 9.2374743232119
18 9.25572634471985
19 9.28061385827304
20 9.29570130568491
21 9.31154635804477
22 9.27240854973175
23 9.24156531866258
24 9.20843725421726
25 9.2270422144554
26 9.26224597575648
27 9.28088194459207
28 9.30664538581925
29 9.31057926450967
30 9.24659544351544
31 9.19885118571387
32 9.17287717985667
33 9.16139909451429
34 9.09786927778418
35 9.15475672024053
36 9.15881108074468
37 9.13017834177902
38 9.07581186746511
39 9.08854247852095
40 9.14579299242715
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.287435909349576
1 -0.108247335026927
2 -0.638324967925233
3 -0.900068969791565
4 -0.588508311100889
5 0.365174431700452
6 1.32332912671171
7 2.13507098837515
8 2.89925310850609
9 3.78651922876023
10 4.95598287121446
11 6.48241796151386
12 7.73531302769476
13 8.51448338820637
14 9.0308408008871
15 9.22200624586775
16 9.20318396590246
17 9.2983904836412
18 9.37375448592582
19 9.37878334062862
20 9.40965865991629
21 9.45722526507182
22 9.43223445396016
23 9.37447143101152
24 9.3637761657456
25 9.36961288563281
26 9.38761338559934
27 9.45126112976988
28 9.49528134708654
29 9.44901359345194
30 9.4268793284605
31 9.38898446268687
32 9.36712070623139
33 9.35582905259204
34 9.33801954809149
35 9.39062590867865
36 9.39988457620521
37 9.35636519501016
38 9.33430768985249
39 9.34495546865729
40 9.41480339301094
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.24892054645212
1 -0.15856665321955
2 -0.681835491327341
3 -0.94800840935891
4 -0.667933660004629
5 0.218882269496878
6 1.26677242539574
7 2.11883507732672
8 2.88012275152038
9 3.84744735103079
10 5.08911228800347
11 6.57813983719482
12 7.7147504341705
13 8.46142025017398
14 8.99243032835295
15 9.28184828214663
16 9.31397941717583
17 9.37593857683342
18 9.44243879612783
19 9.4634617287399
20 9.50592388621164
21 9.53744623270389
22 9.57466776547082
23 9.52994016782348
24 9.44751460049401
25 9.51372332004966
26 9.54145178285772
27 9.62536487975319
28 9.66682083423164
29 9.67516246287581
30 9.62247766282228
31 9.58886745324476
32 9.62241567756049
33 9.6069290084851
34 9.59985977498546
35 9.67034923847915
36 9.6760450978383
37 9.64067117912356
38 9.63264009041512
39 9.66453119646486
40 9.66283188269826
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.329925546376144
1 -0.0264780406152032
2 -0.548018478655493
3 -0.806646764723098
4 -0.493314550608705
5 0.450523359360661
6 1.465488590903
7 2.26120408146455
8 3.03814665273127
9 3.95425808280492
10 5.16099528372182
11 6.66170436680872
12 7.77863860037719
13 8.53489573082443
14 9.0573893175998
15 9.30385089976791
16 9.29068657539306
17 9.33247762697781
18 9.38955774177684
19 9.37148156387856
20 9.3617535937464
21 9.37464873879347
22 9.34973940231776
23 9.27781218515316
24 9.27723475767954
25 9.25391469297459
26 9.28550033969824
27 9.31982000595721
28 9.378697745554
29 9.31880387524769
30 9.26189576520171
31 9.21581142420032
32 9.19731611816259
33 9.19495362149073
34 9.16567114433544
35 9.16336058921844
36 9.16981495482089
37 9.16340463686019
38 9.105515263903
39 9.06319110973822
40 9.05855858463828
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.305921107497311
1 -0.126699737331141
2 -0.655300308266818
3 -0.920196071593804
4 -0.596917428347004
5 0.373222839969361
6 1.38635794790894
7 2.1549691750619
8 3.01908533456603
9 3.9420549169306
10 5.21465418834032
11 6.77218887258456
12 7.94179582609864
13 8.66654265703937
14 9.17771915502416
15 9.34273633516436
16 9.3961102134845
17 9.47571070044492
18 9.55870968276049
19 9.59145480837023
20 9.62608000403058
21 9.64250527067952
22 9.66530307388801
23 9.64287321562179
24 9.62883049689973
25 9.65578205966117
26 9.68070818315433
27 9.75087087164225
28 9.79546758869394
29 9.81902622770718
30 9.76970319975495
31 9.69521157534679
32 9.69738084568584
33 9.67823242337986
34 9.59046675387347
35 9.57482795729031
36 9.59914121355985
37 9.55465099244329
38 9.52324321034953
39 9.48207180951601
40 9.50614805518415
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.248494607640488
1 -0.224940871120961
2 -0.773514414557663
3 -1.07338927936982
4 -0.889717337685819
5 -0.08779902113069
6 0.8294412551328
7 1.6036971241888
8 2.32894502125423
9 3.1183412616278
10 4.06468946574882
11 5.39089025225073
12 6.68729629172689
13 7.69284003424437
14 8.37316476225949
15 8.74726182213616
16 8.86147473936114
17 9.00728821522209
18 9.11418184956976
19 9.1605061446878
20 9.1806411270646
21 9.15337091630319
22 9.16284707648359
23 9.16708655106396
24 9.13330569812842
25 9.16829829481452
26 9.1665353706809
27 9.17180008632816
28 9.20751372318942
29 9.17856769190306
30 9.14435572334304
31 9.05951854216842
32 9.10271257011835
33 9.03724135499676
34 8.92790628574052
35 8.91602448137023
36 8.90656542665745
37 8.83002950261074
38 8.74815347792666
39 8.66736082576536
40 8.71312829836728
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.308145771693107
1 -0.124327667448227
2 -0.603861138635782
3 -0.854863715772877
4 -0.558361978607783
5 0.378165086593211
6 1.35786306651294
7 2.16189659548534
8 2.95912763803404
9 3.90872349617977
10 5.19211342100052
11 6.83411313315985
12 7.92026951038186
13 8.61411166770954
14 9.14148624420603
15 9.37150281248494
16 9.35689373817123
17 9.4100653031997
18 9.47103166352798
19 9.50277354093506
20 9.53080103542041
21 9.52345149772071
22 9.53966193297039
23 9.54320391909487
24 9.47743903762687
25 9.50605312902752
26 9.53851766907266
27 9.63492530476267
28 9.69286122625153
29 9.66257849664803
30 9.63778337215692
31 9.5850804410623
32 9.56996762212417
33 9.5805572747898
34 9.53003232643477
35 9.55306120488946
36 9.59171249254553
37 9.60379125947593
38 9.59071885278102
39 9.6259208829703
40 9.6650911132534
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.275141702317216
1 -0.163694477668555
2 -0.684798506839791
3 -0.917795783225084
4 -0.575823458622892
5 0.365383936679947
6 1.33167823236411
7 2.0833924893436
8 2.86900630971907
9 3.789604173673
10 5.04181707087868
11 6.60711610795921
12 7.77280279487855
13 8.57053471542274
14 9.1190815081996
15 9.35335689124211
16 9.36849238574136
17 9.47950771281538
18 9.54636245668274
19 9.59420116728621
20 9.61351559025992
21 9.68274481548121
22 9.70294482594972
23 9.70005232871435
24 9.68708634016936
25 9.78927585892857
26 9.86503178945578
27 10.0303460985321
28 10.2825600859862
29 10.4966482533734
30 10.7202806609444
31 11.1070032183097
32 11.761197637057
33 12.5357721396686
34 13.3815856453269
35 14.191942055528
36 15.0118188884801
37 15.7419335666297
38 16.4219663167468
39 17.0160092999006
40 17.5884852809899
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.301105247962196
1 -0.109966364229772
2 -0.647862460898681
3 -0.869344344609304
4 -0.546675552485484
5 0.35748012285714
6 1.3376706020462
7 2.08870878536072
8 2.80418531040937
9 3.76828921208207
10 4.94322712858369
11 6.5330199830871
12 7.70778507749876
13 8.55821314597981
14 9.07822617048993
15 9.37583684407218
16 9.41483903678817
17 9.49553036748718
18 9.58879013535875
19 9.59937602105329
20 9.66624146669568
21 9.71092165828875
22 9.74686080332783
23 9.7321752957841
24 9.76502293767361
25 9.87916548686955
26 9.90285765478064
27 9.97508313392624
28 10.1114932387295
29 10.1227329725431
30 10.2061344877768
31 10.3429258028123
32 10.5523063075808
33 10.8566432457174
34 11.2759899371134
35 11.883942690496
36 12.610416925802
37 13.3413730270947
38 14.0509556435164
39 14.719229436859
40 15.3450836407156
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.289281578180701
1 -0.129812626186868
2 -0.655646908975643
3 -0.940730999228324
4 -0.67532852045014
5 0.235608447752051
6 1.18021210672025
7 1.9881494269468
8 2.78992550859949
9 3.72994928295289
10 4.8859492542818
11 6.50684128891844
12 7.70702678484642
13 8.54448605420196
14 9.06867267767741
15 9.30294243096493
16 9.32647172769014
17 9.38144457539677
18 9.44228472499948
19 9.47888945525685
20 9.47901485962371
21 9.49779217138356
22 9.47302451340744
23 9.43648436103074
24 9.44818790086092
25 9.43395591321678
26 9.46387115299171
27 9.52351610611313
28 9.66558252627221
29 9.68047647742072
30 9.66284641499596
31 9.63387754634635
32 9.65937730439742
33 9.71061197828518
34 9.71968132139122
35 9.85655038673191
36 10.0102417806613
37 10.172888392671
38 10.4240243977887
39 10.9127438127331
40 11.5193516080033
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.278965262028003
1 -0.0837284093448489
2 -0.617841573460833
3 -0.891505667865921
4 -0.701325238298477
5 0.181766621284591
6 1.13025421922177
7 1.94768097159977
8 2.69890572575004
9 3.57569819302507
10 4.69991486936868
11 6.11704478002662
12 7.38447609591446
13 8.1762839369811
14 8.66675669304159
15 8.93857604758112
16 9.02597972977775
17 9.06036536896495
18 9.13603392134512
19 9.12127876674673
20 9.14104170627278
21 9.14170587229468
22 9.17333860408392
23 9.09745302447066
24 9.03496558006093
25 9.11469056022928
26 9.07670988733862
27 9.05614825272789
28 9.13128437747744
29 9.07569116730616
30 9.02340460173525
31 8.9382110039645
32 8.94550749165503
33 8.88868696857699
34 8.80751250345922
35 8.81820401240824
36 8.81427474189117
37 8.79137786319403
38 8.77433227100547
39 8.72326068782754
40 8.73460146544152
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.329092421635068
1 -0.0523140536405493
2 -0.548607395757708
3 -0.778637929263459
4 -0.424667263784702
5 0.48567759916359
6 1.45566901316386
7 2.26035221806972
8 3.03271615810776
9 4.08478444388608
10 5.38490420410198
11 6.84329856481659
12 7.96570978849471
13 8.7058982523432
14 9.20471427942696
15 9.3741624139359
16 9.41821588959891
17 9.44511842903179
18 9.52489969277508
19 9.57208346915185
20 9.56576755374873
21 9.59697041631704
22 9.58279713702572
23 9.59604275861526
24 9.58995182659507
25 9.61287118920114
26 9.6659022975848
27 9.7543716880875
28 9.82342438681792
29 9.79648718503142
30 9.73506489844702
31 9.68881552232419
32 9.70476293659886
33 9.68119605763836
34 9.67043014658318
35 9.76621866299911
36 9.83107491514389
37 9.84740655931455
38 9.88994618727642
39 10.0100259941079
40 10.2545494047575
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.290786127705215
1 -0.110123523895876
2 -0.65212067234628
3 -0.881597662134826
4 -0.535312681747254
5 0.403890841536708
6 1.36704767506947
7 2.11124246168448
8 2.80177286621167
9 3.74531130307551
10 4.97057548236696
11 6.42927768918548
12 7.64514862842094
13 8.45022270211751
14 9.01886997050054
15 9.23406724692727
16 9.27387794321342
17 9.32530895969395
18 9.34647595392099
19 9.3658226291557
20 9.35819633152381
21 9.33634236459346
22 9.31559408924587
23 9.2353817641894
24 9.18410246117335
25 9.16424078975048
26 9.17686910652889
27 9.16957337562237
28 9.2240847125521
29 9.1822060697281
30 9.14828704007083
31 9.10287742549018
32 9.03945549374815
33 9.01209043104583
34 8.93880063765961
35 8.92841559881837
36 8.92983754230869
37 8.89683121261475
38 8.83426108170172
39 8.84068900377951
40 8.8543053636957
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.320517059841727
1 -0.123695615882811
2 -0.6409764737499
3 -0.910880775690813
4 -0.620949555749378
5 0.292786839719921
6 1.27049754003992
7 2.08509466549833
8 2.87046782981172
9 3.81433405547371
10 5.06776263632919
11 6.68551715957368
12 7.80909378315879
13 8.5771361270547
14 9.10639928988333
15 9.38862114879744
16 9.39718008010204
17 9.43307267876054
18 9.49631800229775
19 9.50969481083033
20 9.52174847421609
21 9.52397764231641
22 9.57691158490672
23 9.53792525033372
24 9.47752921195632
25 9.5615374486773
26 9.55852685996403
27 9.59391314789901
28 9.69150143885975
29 9.67351823824994
30 9.61322632025067
31 9.59779566527269
32 9.62714027980818
33 9.55744608089696
34 9.56288514710441
35 9.59309822196496
36 9.58400179819866
37 9.60503950341418
38 9.62263240590347
39 9.65408238936946
40 9.67874451623763
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.269642931701965
1 -0.21176026646337
2 -0.744766987816518
3 -1.01377594097764
4 -0.740279520243225
5 0.175106123106215
6 1.14157347501071
7 1.95686043762785
8 2.76466327358
9 3.69364121067874
10 4.8642499455314
11 6.41492015457183
12 7.61631397367854
13 8.41113037875832
14 8.86892224305776
15 9.08672312419706
16 9.08350364581139
17 9.12674718038641
18 9.16648464855644
19 9.19744056865333
20 9.24283736327653
21 9.26435810604789
22 9.22900465377483
23 9.24200122399961
24 9.19786297618282
25 9.26029267562371
26 9.29572929220545
27 9.35804883580555
28 9.35749874086812
29 9.33744580349589
30 9.32029486587015
31 9.29512719306837
32 9.25889252036262
33 9.22729321696941
34 9.22688763711358
35 9.25595510700681
36 9.24473677983352
37 9.19284005657486
38 9.15895086902023
39 9.17255549611873
40 9.16270453331583
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.320005776175798
1 -0.111919450010358
2 -0.671609119840602
3 -0.858247877743805
4 -0.514605387603887
5 0.428484660589397
6 1.42900589155137
7 2.13807213717756
8 2.93652134054903
9 3.88829763816495
10 5.10158611712447
11 6.62420876649535
12 7.81178770050212
13 8.66023570723798
14 9.13306778117788
15 9.37683250349276
16 9.41145084914047
17 9.48850032009974
18 9.53906782174627
19 9.58188289718046
20 9.61728565603672
21 9.66545889228425
22 9.67118873388651
23 9.66711142609272
24 9.63783186298823
25 9.69287430054077
26 9.76761880580814
27 9.80575395211086
28 9.94020207188788
29 9.95272943278192
30 9.9089318148818
31 9.84727513713334
32 9.87086751708748
33 9.81675893682448
34 9.77221601330023
35 9.81763674556174
36 9.84684513906084
37 9.85029919449095
38 9.82715327968824
39 9.83395181546696
40 9.8705246475784
};
\addplot [line width=0.01pt, color1, mark=*, mark size=2, mark options={solid, draw=black}]
table {%
1 -0.216971117452557
2 -0.698311813338088
3 -0.845437931574839
4 -0.510347906996663
5 0.417785295755321
6 1.45063997856431
7 2.18000698194071
8 2.91511410045934
9 3.99138570661581
10 5.18010069663342
11 6.78065117660923
12 7.92074360825274
13 8.74285795470332
14 9.32370003511269
15 9.44974184549204
16 9.39728065453565
17 9.39942446694502
18 9.45875925073886
19 9.41596191419465
20 9.44604175500281
21 9.43595937363876
22 9.4563381291001
23 9.4069938263042
24 9.38363158073475
25 9.40550089098364
26 9.38007003255305
27 9.42642504798656
28 9.50602660780519
29 9.50516219108816
30 9.43584948844373
31 9.4053013696456
32 9.43579387299814
33 9.39838716046376
34 9.37035636536838
35 9.40687083255091
36 9.4411863522549
37 9.44827707366167
38 9.39444475031715
39 9.40444975096704
40 9.47548755380175
};
\end{groupplot}



==> experiments/figs/cart_pole/tikz_samples_ep-2-all.tex <==
\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}

\begin{groupplot}[group style={group size=1 by 3}]
\nextgroupplot[
xshift=-8,
title={2 episodes (80 time steps in total)},
title style={font=\large},
ylabel={\textcolor{color0}{cart position}},
ylabel style={font=\large},
xmin=-1.95, xmax=40.95,
%ymin=-2.42067264251211, ymax=0.974406515869978,
ymin=-0.45, ymax=0.45,
width=\figurewidth,
height=\figureheight,
xtick={},
xticklabels={},
tick align=outside,
tick pos=left,
x grid style={lightgray!92.026143790849673!black},
y grid style={lightgray!92.026143790849673!black}
]
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.076550700862454
1 0.210573927455759
2 0.319383814620569
3 0.236673119892683
4 0.16163202688982
5 0.0628509877292398
6 -0.0791942910795385
7 0.0148080258349168
8 0.152776535172408
9 0.228026719755102
10 0.178738841757177
11 0.325910439629499
12 0.49873183909129
13 0.628856572787753
14 0.534288408997006
15 0.431076437730984
16 0.429875386753652
17 0.444905907587634
18 0.365178363860436
19 0.293865266790057
20 0.246484924054903
21 0.14995975561893
22 0.0870098878221892
23 0.0115979073343726
24 -0.0196853209646224
25 -0.0782243380798699
26 -0.196765439657808
27 -0.208028726982095
28 -0.280912083789304
29 -0.366860453453481
30 -0.427447626502214
31 -0.429461826031629
32 -0.40650789649498
33 -0.419871343564499
34 -0.363440785637975
35 -0.278953283049385
36 -0.263027061701919
37 -0.219409374286565
38 -0.182825222008649
39 -0.166734396140079
40 -0.193390131357039
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0751122514773908
1 0.204649465719531
2 0.313955915650942
3 0.261619819776983
4 0.192243124724185
5 0.055248355606762
6 -0.117860770678965
7 -0.0607383772208561
8 0.00351948940669766
9 0.119652214802248
10 0.172530004753444
11 0.179404250629961
12 0.27045279874071
13 0.387900022667769
14 0.26564373860444
15 0.112525169155363
16 0.118614805565748
17 0.123449819644015
18 0.00534602239303839
19 -0.0724486627546548
20 -0.135487067795705
21 -0.230220222093636
22 -0.304958404577335
23 -0.391806345994073
24 -0.396533142272763
25 -0.398588681014601
26 -0.462556292092671
27 -0.452994120775752
28 -0.623892434806923
29 -0.667466599292112
30 -0.771989445705942
31 -0.797682970044823
32 -0.85818954133546
33 -0.975679965514129
34 -1.0324423957188
35 -1.10079797848557
36 -1.17124624993914
37 -1.26774942523259
38 -1.36755920812206
39 -1.4403354464864
40 -1.53647809641671
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0794996284282283
1 0.245655741453681
2 0.387763936079379
3 0.324429051476324
4 0.303793836980612
5 0.216975916310132
6 0.0953507296881293
7 0.155610633412202
8 0.27730647839228
9 0.446501987417787
10 0.450731122049283
11 0.54498225203982
12 0.695396546500787
13 0.823709583723606
14 0.786336826959496
15 0.6374752910199
16 0.644308050438251
17 0.66550915430815
18 0.599986756792237
19 0.541193869045204
20 0.53456107869141
21 0.462071519524812
22 0.4499479989356
23 0.405838899315178
24 0.486601550563929
25 0.483815151985904
26 0.377951709785789
27 0.404455794891005
28 0.308295629789438
29 0.233186019558327
30 0.126289925569066
31 -0.0213900682655033
32 -0.161167779638937
33 -0.346722735438675
34 -0.476342873340256
35 -0.644646461819161
36 -0.806804772554467
37 -0.935387666873637
38 -1.05611428768321
39 -1.22469811465693
40 -1.3287001345583
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.061888316010005
1 0.123425202482086
2 0.214309885760103
3 0.167447799053351
4 0.123096266271769
5 0.0558632227771261
6 -0.106339172787804
7 -0.151831646727011
8 -0.125766729805658
9 -0.0723335612005815
10 -0.113737159919697
11 -0.105312206123537
12 -0.0820364113075067
13 -0.0244696619150351
14 -0.023997991203577
15 -0.0593907794911117
16 -0.0449605975504306
17 -0.0745551240989584
18 -0.0885230818915064
19 -0.126036289402377
20 -0.113261618502559
21 -0.103929267172217
22 -0.119614426476756
23 -0.144486022059751
24 -0.18155070915511
25 -0.20642383367974
26 -0.2503861070771
27 -0.263747557833904
28 -0.367904331772818
29 -0.4895187740052
30 -0.648647111951608
31 -0.701777659464482
32 -0.81429158761229
33 -0.996512346488114
34 -1.1015239070967
35 -1.2786216197888
36 -1.47617570092811
37 -1.68798840057775
38 -1.86347276377693
39 -1.98078801220949
40 -2.16967296460132
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0812133880999584
1 0.147787946069977
2 0.217289643882026
3 0.239400289752536
4 0.241574393812328
5 0.178774392736721
6 0.0742419178442844
7 0.143364426763704
8 0.212031180541752
9 0.266572676813852
10 0.238425925736128
11 0.3360465232134
12 0.358965819153553
13 0.415122866329702
14 0.383417433517148
15 0.386318024789222
16 0.427628783311351
17 0.46926376827683
18 0.438274844534166
19 0.392276485944487
20 0.377943806664408
21 0.379157123114954
22 0.39564344998084
23 0.387316433781351
24 0.448331601161575
25 0.494956959618067
26 0.437909246996722
27 0.450439176848956
28 0.356674514822498
29 0.284436079037947
30 0.222765193198078
31 0.18235855439158
32 0.100812390608218
33 0.0144818936823214
34 -0.0135424407795628
35 -0.0577733988895495
36 -0.0963481306674367
37 -0.136791767176025
38 -0.246121887870689
39 -0.304148950865555
40 -0.382943490735841
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.117214992271315
1 0.168872003591541
2 0.243111750099483
3 0.218918408666229
4 0.180207993319593
5 0.10129874186626
6 0.00144065813045691
7 0.102572014317307
8 0.130476616556477
9 0.210752110901983
10 0.229633245856689
11 0.231885812776295
12 0.294834429509369
13 0.289425483773402
14 0.269896816773755
15 0.239512113093147
16 0.173618536261062
17 0.159996456104631
18 0.0905323148959103
19 0.0566594998542587
20 0.113824952880655
21 0.0931606984750855
22 0.0894049004611861
23 0.0563784311244611
24 0.0792748801217948
25 0.0805376292363831
26 0.121909907291406
27 0.143425271373133
28 0.034093288325229
29 0.017619451846735
30 -0.0469266472679148
31 -0.0952139551234468
32 -0.129083133290857
33 -0.155268713480579
34 -0.232791877098805
35 -0.294103960913715
36 -0.290771013577639
37 -0.339608824707727
38 -0.406930512779047
39 -0.427761009792854
40 -0.514952819024452
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0827250931605503
1 0.114345260512255
2 0.148715026514433
3 0.136243058707076
4 0.111707778951788
5 0.0436267833417174
6 -0.0726898295587159
7 -0.161264489776481
8 -0.175783683441743
9 -0.134759587230873
10 -0.105961208336693
11 -0.0864681300225141
12 -0.142385093409711
13 -0.15508235161409
14 -0.155996150474966
15 -0.262359247337744
16 -0.274374042032572
17 -0.21895836724012
18 -0.207621117187845
19 -0.254574898557482
20 -0.307402601078371
21 -0.391496200174136
22 -0.415182502675768
23 -0.504768539631361
24 -0.466138579129811
25 -0.495853905572905
26 -0.516229427385465
27 -0.430972576375976
28 -0.510146629939446
29 -0.491222287018475
30 -0.482914417994038
31 -0.482928024336114
32 -0.495896802262823
33 -0.519881971142108
34 -0.606072135219715
35 -0.737084643310952
36 -0.893668636694458
37 -1.09111377583531
38 -1.20836312489301
39 -1.32811782050522
40 -1.4567860949248
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0501864644613383
1 0.188413899400204
2 0.29788724783734
3 0.265149966691487
4 0.219308116572851
5 0.175002052764647
6 0.0224453670535358
7 0.140286031021828
8 0.28642506895664
9 0.373321097651104
10 0.35987452666589
11 0.480033136406945
12 0.580690753055187
13 0.675654245532142
14 0.603327325167589
15 0.60596933562568
16 0.563721063478855
17 0.547400822883874
18 0.453666691032155
19 0.433901738569156
20 0.476324451465414
21 0.461868807596903
22 0.500996205783418
23 0.388434320523435
24 0.4359114834193
25 0.414874852014372
26 0.430893896434069
27 0.506732542185859
28 0.482031834239972
29 0.490845352153405
30 0.46504250604191
31 0.455918738323679
32 0.434132015239084
33 0.323432023731324
34 0.244699845984423
35 0.167475713227121
36 0.0227154333373463
37 -0.105482553616275
38 -0.21520598499712
39 -0.339617260838213
40 -0.519362473285356
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0941882310590012
1 0.183543060530124
2 0.349264107546889
3 0.304249589889686
4 0.264688701365632
5 0.1418558794114
6 0.0561227334463217
7 0.119685917828895
8 0.171356809956641
9 0.250824815922078
10 0.249164166038721
11 0.319593882333428
12 0.452108147353476
13 0.5712524025495
14 0.511653266827991
15 0.406937525862358
16 0.468449976343893
17 0.565581185560978
18 0.598170192296709
19 0.578113418308042
20 0.618678371876024
21 0.566325608800999
22 0.535593777169292
23 0.433830193258681
24 0.478207270876859
25 0.510324496382592
26 0.492990412511304
27 0.546433176233377
28 0.478984081085138
29 0.469160594990781
30 0.378627825088382
31 0.406027842647669
32 0.356207974811743
33 0.408863823741698
34 0.50438010401017
35 0.550591575206191
36 0.5879357471836
37 0.621452699097276
38 0.656351405804344
39 0.706046053294178
40 0.693844831113852
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0907927103884667
1 0.206578482448717
2 0.286080040102421
3 0.245703569703739
4 0.164938688206464
5 0.0455443415442462
6 -0.0920044101955491
7 -0.00956618028755463
8 0.0193500151547807
9 0.147300500251433
10 0.147624540990666
11 0.222514758433096
12 0.299035782666436
13 0.37626034134505
14 0.372455599108531
15 0.335102765285961
16 0.266224501531658
17 0.197730242832197
18 0.124524463628449
19 0.0626719177179385
20 0.0586100771954725
21 0.0642578874959647
22 0.123793126959244
23 0.149878661451192
24 0.229779153294775
25 0.286202810340171
26 0.318871350356149
27 0.36027149316295
28 0.238580542221898
29 0.222426038139016
30 0.192025074081315
31 0.231525923983171
32 0.205282491512397
33 0.131048395888361
34 0.206762644199769
35 0.255315133823333
36 0.250642568620089
37 0.254923983479776
38 0.257923885054092
39 0.231672705689888
40 0.180808775717188
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0607384488020264
1 0.19654341688996
2 0.294155548627454
3 0.278468918034909
4 0.259381748202842
5 0.166370866360662
6 -0.0294507491764824
7 0.0136038007166097
8 0.131231280189851
9 0.199093277369095
10 0.201569290405597
11 0.211638293142706
12 0.172394206009949
13 0.182124337234747
14 0.0934360774536795
15 0.072911014429045
16 0.040418649184621
17 0.0353175995142072
18 -0.0322387697523197
19 -0.157513906508434
20 -0.248365205795361
21 -0.328019049435561
22 -0.354376815939341
23 -0.337533919719964
24 -0.350649456543193
25 -0.466729999903496
26 -0.538075521730339
27 -0.535867648673939
28 -0.644291257041559
29 -0.669735625051908
30 -0.689177626615063
31 -0.683767928574846
32 -0.754868890340681
33 -0.847105670057989
34 -0.917190379122856
35 -0.979047813442619
36 -1.05616282309316
37 -1.09388276895424
38 -1.11987485116381
39 -1.15246170185662
40 -1.15242150544469
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.11086890601695
1 0.152169094307942
2 0.319960015781513
3 0.24014420478827
4 0.157570710865703
5 0.0645340306278746
6 -0.0368952936044691
7 0.0122712648525671
8 0.0744242026381805
9 0.188113186880981
10 0.182988387202354
11 0.269173286348711
12 0.380142072959021
13 0.471488618441701
14 0.427474669057952
15 0.348470028817907
16 0.289910945369931
17 0.323711630098698
18 0.233377410919723
19 0.230018786698666
20 0.170925172814659
21 0.102471021329398
22 0.0994163085112203
23 0.056580282963802
24 0.0972765474808379
25 0.1257940188457
26 0.0992034161755471
27 0.147300548405813
28 0.0306482931242749
29 0.0306309150887336
30 -0.0354655039598852
31 -0.0390370174243304
32 -0.0811648814321018
33 -0.154571561204373
34 -0.209902973112718
35 -0.347196556776618
36 -0.503915765500001
37 -0.631905964733341
38 -0.850914674755832
39 -1.05794764049059
40 -1.21576974447186
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0710382474576488
1 0.214405775653805
2 0.377308232824966
3 0.34751462945602
4 0.258022333424129
5 0.155176151954514
6 0.0387815041069453
7 0.110759405740336
8 0.191801109287352
9 0.299548558286546
10 0.201904536580483
11 0.291096860582823
12 0.496474402659108
13 0.632037348330997
14 0.600512359289525
15 0.589784558756336
16 0.537034635292533
17 0.507013600657281
18 0.493876128396173
19 0.419032358182566
20 0.478985121651883
21 0.405396404684035
22 0.349179478325337
23 0.284196986660122
24 0.303349289278983
25 0.321800566851442
26 0.296472703499815
27 0.415363357355168
28 0.356763269682184
29 0.298072854323399
30 0.193982589415644
31 0.132366101764411
32 0.0539139090917997
33 0.100001465616814
34 0.125737448208075
35 0.138974871765456
36 0.255706812329151
37 0.37656829151241
38 0.468195184939312
39 0.626732370076214
40 0.72515088974502
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0711346173366154
1 0.144406293967217
2 0.27543101605993
3 0.334327829156783
4 0.346742297871348
5 0.338057994218599
6 0.270070146409398
7 0.318743079553002
8 0.445955716111897
9 0.566788667032867
10 0.705450300524223
11 0.829671730653413
12 1.0016727628995
13 1.150947905907
14 1.07844308214884
15 1.00766156914028
16 1.02870139787364
17 1.08027494693932
18 1.04845462646495
19 0.907296400492849
20 0.788808396715698
21 0.620852168421012
22 0.522064292450461
23 0.409347910417504
24 0.401220813439543
25 0.320173616827606
26 0.260115099448022
27 0.240325360407642
28 0.189599736259017
29 0.208847172368845
30 0.22692923869168
31 0.167562214393419
32 0.105528090221528
33 -0.0350228882645611
34 -0.111512468556215
35 -0.269675848881371
36 -0.456543793932797
37 -0.68461480748213
38 -0.850541753303464
39 -1.02768007916949
40 -1.20409051688884
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.104891099566314
1 0.216335484474873
2 0.382786801979338
3 0.373964084652179
4 0.373364843388995
5 0.310250443052802
6 0.235706531455223
7 0.254371696033038
8 0.337203235338249
9 0.439052984411311
10 0.389280849994555
11 0.450256269822173
12 0.555709435835388
13 0.685258228449218
14 0.754803333244038
15 0.769659062118982
16 0.767882526797687
17 0.710915489378375
18 0.617238205593329
19 0.524679431009082
20 0.548444674848872
21 0.441303446101906
22 0.456566975438038
23 0.401074044201243
24 0.432461390248458
25 0.410041338951434
26 0.334899212272948
27 0.378200007963006
28 0.225184143017215
29 0.0855300818950084
30 -0.0266435092024033
31 -0.0166149326248894
32 -0.102772047896721
33 -0.23142758515205
34 -0.189416408434117
35 -0.202916982360291
36 -0.272742557407562
37 -0.338532868227885
38 -0.417245074227357
39 -0.509669820416665
40 -0.585949254279579
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.088462259157013
1 0.152487308055316
2 0.219473483842374
3 0.217138782204606
4 0.157199270463952
5 0.0331368801525143
6 -0.0632795417008327
7 -0.0136353717825832
8 0.0497246624522463
9 0.163226428634189
10 0.170086274921554
11 0.204018853599597
12 0.308869595227378
13 0.45831307263445
14 0.5116258066954
15 0.524503368087929
16 0.523538256565185
17 0.569323323403951
18 0.520070544173695
19 0.517641347118279
20 0.540156010720546
21 0.534939464575569
22 0.579473859558489
23 0.594353641140644
24 0.58479267787596
25 0.553666489476496
26 0.49966251206917
27 0.497422701150843
28 0.356214072815727
29 0.261081557822888
30 0.131523112262158
31 0.0765944789311401
32 -0.00357350049306238
33 -0.0894373057403768
34 -0.139140560560897
35 -0.191558685327064
36 -0.251902714639449
37 -0.300407491726778
38 -0.396526972918406
39 -0.600378053575396
40 -0.763286896041486
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0694850663600044
1 0.178723306309833
2 0.267869126447976
3 0.238549967353392
4 0.239900457484797
5 0.223401379746892
6 0.173562454994293
7 0.284088435465685
8 0.347591976817461
9 0.455018653834852
10 0.48441200879286
11 0.520346127754331
12 0.572995885502015
13 0.616239121790434
14 0.571200422398247
15 0.526919639176952
16 0.564117294912553
17 0.565592327668571
18 0.524332217716375
19 0.463118867656673
20 0.42832113189159
21 0.34815571412914
22 0.248973642680142
23 0.156074518166245
24 0.0933282122344985
25 -0.0492919014921047
26 -0.11026862199584
27 -0.113639157752038
28 -0.204680770861182
29 -0.293295295360509
30 -0.307085290216253
31 -0.412475742980886
32 -0.499232862095455
33 -0.571573232489645
34 -0.679595550613114
35 -0.793458740572241
36 -0.841227669184667
37 -0.936006877100703
38 -0.998147132600622
39 -1.06424802922813
40 -1.10188296447275
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.12362607924061
1 0.143567065905034
2 0.238378358456699
3 0.187261286765436
4 0.14347005387489
5 0.0774601167908839
6 -0.0730856969277878
7 -0.0333331308026028
8 -0.0213079297757677
9 0.0618599242653119
10 -0.0109896168037524
11 0.0565893232149222
12 0.168550093625298
13 0.303434579692501
14 0.220074041529308
15 0.0961191480444357
16 0.0774648587733209
17 0.12139529577211
18 0.0678665480766045
19 0.0294374827449269
20 0.0708194380997789
21 0.0388766446833033
22 0.0132999487999568
23 0.0118420405710449
24 0.0831652528523668
25 0.125340946591902
26 0.132683501584554
27 0.177129555622202
28 0.152598597102728
29 0.0687516223909745
30 -0.0265508739319049
31 -0.0782927326119194
32 -0.152757016879445
33 -0.307728973961115
34 -0.357710168829657
35 -0.402326290852407
36 -0.466765522569215
37 -0.492096305229597
38 -0.487449219136074
39 -0.445314767790863
40 -0.456242207026292
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0867575976608825
1 0.171743117305099
2 0.296348174675406
3 0.323837463235052
4 0.317059188322224
5 0.233957040317188
6 0.0978461802491304
7 0.200182112238101
8 0.245024964083715
9 0.346472500919205
10 0.348684079347708
11 0.435921748700138
12 0.498716201300992
13 0.568855943111096
14 0.530627931992907
15 0.458163025527131
16 0.404448733278261
17 0.396022244092334
18 0.415397149119533
19 0.335276099240062
20 0.268581808131375
21 0.183826675693782
22 0.140177130112493
23 0.0714589202526961
24 0.0796262960378438
25 0.056817153784376
26 0.047970232323149
27 0.0633758730602003
28 -0.00659710575507111
29 0.0334397871367527
30 0.0588842823601676
31 -0.00225700037446819
32 -0.0857017365952966
33 -0.125903590049799
34 -0.224164558081572
35 -0.323817422154963
36 -0.448028734252933
37 -0.540894290771576
38 -0.589510751006626
39 -0.605767753791971
40 -0.625362355874711
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0846457397723581
1 0.114504166399843
2 0.178444588690208
3 0.0579894151639455
4 -0.0378916469250941
5 -0.125313425688811
6 -0.26258172165237
7 -0.240692733437267
8 -0.144425208903257
9 -0.0130074236678537
10 -0.0519723302326005
11 -0.00966075049498194
12 -0.00114395866963468
13 0.0168681058458784
14 -0.0659436278305883
15 -0.071713778526878
16 -0.120858447385556
17 -0.143812890970009
18 -0.232237004251934
19 -0.283000667874173
20 -0.299269365452526
21 -0.314850291748994
22 -0.320524857390678
23 -0.369321318920498
24 -0.39865108817715
25 -0.388359286145059
26 -0.406923586857972
27 -0.352668001406885
28 -0.442836021698028
29 -0.457800628972113
30 -0.502333051971886
31 -0.502800347913129
32 -0.450759634651172
33 -0.411974188952126
34 -0.274867984887251
35 -0.111804644244821
36 -0.015285041531611
37 0.17185035089223
38 0.358694518657476
39 0.473831239864062
40 0.602925401704272
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.135589950475548
1 0.240319767501691
2 0.368356934751444
3 0.278350554858755
4 0.228096626492277
5 0.114881148313702
6 -0.0409042377540327
7 -0.00172816685214672
8 0.0545227956107479
9 0.087333766443463
10 0.062170641752024
11 0.188229897707924
12 0.262164540208334
13 0.344510588871592
14 0.283055450881154
15 0.253908857825431
16 0.186583113586267
17 0.105943524460425
18 0.0675192246237395
19 -0.0381344989218597
20 -0.0585197125957437
21 -0.191912761976853
22 -0.241299043505816
23 -0.346702225742182
24 -0.343481169627559
25 -0.350287712964184
26 -0.368888806215508
27 -0.377133810811816
28 -0.419341504541047
29 -0.464482542110663
30 -0.536064051298929
31 -0.604403396542304
32 -0.664562412206426
33 -0.735185399552671
34 -0.775734736563808
35 -0.836533515917776
36 -0.897919115993694
37 -0.970690465830836
38 -1.03241790762782
39 -1.07246403272112
40 -1.10271115004392
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0824207521003193
1 0.235966466931654
2 0.35806910632872
3 0.395878757249427
4 0.356651052816645
5 0.260638592739022
6 0.109840117090422
7 0.201478961391715
8 0.349638874472606
9 0.408609420376562
10 0.429621215070906
11 0.557211058314485
12 0.700160241946644
13 0.931283646901624
14 0.930240601125259
15 0.907829182611499
16 0.997504280979736
17 1.03357328268782
18 0.964407836512012
19 0.939812012430071
20 0.964363764811203
21 0.90730356153269
22 0.884829943054774
23 0.798794521541681
24 0.788947676392752
25 0.730484960362825
26 0.672486940762518
27 0.681951260072973
28 0.610029374468894
29 0.590120942255171
30 0.515955215510336
31 0.514673242500523
32 0.473853317263927
33 0.415275026816692
34 0.413282327707606
35 0.408732951568043
36 0.422735532602613
37 0.428415468259571
38 0.453531598974614
39 0.554885193618157
40 0.669986133192302
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0810485648226953
1 0.159285798371523
2 0.286270577881866
3 0.2582443575577
4 0.220509184754133
5 0.171111689980692
6 0.0726858116582911
7 0.0794123381068057
8 0.173775862804064
9 0.289818557952187
10 0.27274061357886
11 0.383339903336867
12 0.417690183348746
13 0.4519493079669
14 0.408042031396039
15 0.297161910892331
16 0.354777854708717
17 0.436302727007135
18 0.400510770892574
19 0.322353745333047
20 0.315887411657446
21 0.251260920134591
22 0.266004027566139
23 0.220962538372035
24 0.264292652204359
25 0.237772151290602
26 0.265476047476182
27 0.360477157278927
28 0.311219603536657
29 0.347686990953729
30 0.393434151866316
31 0.438820739215958
32 0.503486332221609
33 0.477487451201201
34 0.530659893464189
35 0.584108687062039
36 0.667382845733918
37 0.700002383773052
38 0.762014857145492
39 0.866974192053559
40 0.997447186878886
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0965735188003518
1 0.0912415055532483
2 0.212668294037135
3 0.161159540356267
4 0.124146857212814
5 0.0377271862063977
6 -0.11285981870577
7 -0.0998537741622376
8 -0.0717176218843694
9 0.0207622297758743
10 -0.00417204270121152
11 0.0591148441991098
12 0.139678289832776
13 0.217428214317251
14 0.172967768798233
15 0.10074140502833
16 0.127529793975711
17 0.124149163588528
18 0.0956960100418387
19 0.0395885093135924
20 0.0611580811628039
21 0.0187735695711089
22 -0.00110542899153643
23 0.0142399544689393
24 0.0114637986676338
25 0.0154128585828013
26 -0.0206049312335566
27 0.0610398916051795
28 -0.0249303565907537
29 -0.0728015074628274
30 -0.0981580524680159
31 -0.0783621474902572
32 -0.106969298568903
33 -0.195657661756947
34 -0.197854317399215
35 -0.303779542756687
36 -0.468176389501372
37 -0.621182030931288
38 -0.772618241521404
39 -0.85703786839599
40 -0.961617439929525
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0869829323071971
1 0.207429651003287
2 0.241539175530837
3 0.231242154088831
4 0.178869220613703
5 0.101462035550302
6 0.0108112330447723
7 0.0235940536187518
8 0.0614601753539064
9 0.121982351857246
10 0.0924933696053598
11 0.115834693273362
12 0.158265506885187
13 0.152649703596403
14 0.158535801759148
15 0.114472090304471
16 0.163599953986206
17 0.170475489344973
18 0.0976619250801716
19 0.077491099481545
20 0.170063755182883
21 0.157728857685764
22 0.0892654940103204
23 0.0782287237579591
24 0.0378155622129706
25 -0.0113523701713172
26 -0.0619778354757057
27 -0.0986730204204269
28 -0.247829792271907
29 -0.347381356260119
30 -0.501250867443833
31 -0.605407635569487
32 -0.809070064792569
33 -0.819092865061708
34 -0.85875056979496
35 -0.907456252365894
36 -0.967426246683232
37 -0.96306655961365
38 -0.931254396012836
39 -0.955656290484943
40 -0.985578945399752
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.082842017856958
1 0.186873665915035
2 0.302363063078223
3 0.261251904336398
4 0.229181112948479
5 0.141117883602724
6 0.0383255292947053
7 0.102934091388007
8 0.146565653584781
9 0.236164804525432
10 0.223297426253355
11 0.276995487767887
12 0.287793915028447
13 0.315213032554161
14 0.306974339865648
15 0.269353451002895
16 0.292144964838617
17 0.315707889519083
18 0.264224620107167
19 0.194299036824417
20 0.181154170302921
21 0.118898775700524
22 0.036876452558225
23 -0.0612899346614082
24 -0.140404630566102
25 -0.196091030010009
26 -0.346490355173033
27 -0.336929115362618
28 -0.467722329069684
29 -0.584030788697904
30 -0.710472246592926
31 -0.661995130968933
32 -0.758167229582867
33 -0.916358922821995
34 -0.940922165798231
35 -1.05220535701122
36 -1.14229550609851
37 -1.20263998447974
38 -1.2125669851477
39 -1.23830484170662
40 -1.26516567359427
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0718584013569115
1 0.118434618255611
2 0.25023262066627
3 0.189006847858011
4 0.109981331411738
5 0.0229401636049693
6 -0.0798700680836801
7 -0.128037719969233
8 -0.0587109009369779
9 0.0235913920074804
10 0.0445648788261739
11 0.158236407249067
12 0.244949532620198
13 0.365787980101268
14 0.315102199046442
15 0.292708501604829
16 0.300649820002109
17 0.325593202618207
18 0.264942405824605
19 0.224445380370493
20 0.182895971623089
21 0.0810416272699777
22 0.0321197719319706
23 -0.0433429249366544
24 -0.057111491022968
25 -0.0424711767975419
26 -0.158872875386632
27 -0.129112671791783
28 -0.292302792338462
29 -0.374687464654827
30 -0.529915324808933
31 -0.536852942556296
32 -0.594630395862386
33 -0.709149438646198
34 -0.693880040021553
35 -0.680825822173861
36 -0.735157900144897
37 -0.801671961903946
38 -0.860176409556302
39 -0.873525769472285
40 -0.904048951268336
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0513891536602706
1 0.140643661337
2 0.185326543842512
3 0.135572572811332
4 0.123240754455474
5 0.0895301678418883
6 -0.0146180430009171
7 0.0186077452350548
8 0.102948464948559
9 0.169299619011039
10 0.160010614237926
11 0.17215401062477
12 0.221613847058963
13 0.262801405155422
14 0.206126085860881
15 0.137753395035364
16 0.138524371210063
17 0.097011500258037
18 0.147248911034806
19 0.146230059112511
20 0.178494608793898
21 0.0881288758505732
22 0.0359191655023361
23 0.00253463656060759
24 0.0510872272984133
25 0.0743033400147115
26 0.0325624104184152
27 0.120062753510942
28 0.093247188138728
29 0.070169296165163
30 -0.0516221696486028
31 -0.0166598581417565
32 -0.0721475295333089
33 -0.220948796365021
34 -0.30594636493617
35 -0.404035547422022
36 -0.481309509455054
37 -0.497619900665497
38 -0.490622178374734
39 -0.476491996330342
40 -0.433830107973442
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0841335898689439
1 0.153367047114585
2 0.217490825555
3 0.119567022729114
4 -0.00345382978804976
5 -0.131738114380216
6 -0.280355282733696
7 -0.25119639220834
8 -0.174679577432325
9 -0.0856388118377196
10 -0.186486259115334
11 -0.125917243228242
12 -0.0384094199392044
13 -0.0390135766575295
14 -0.213411888221921
15 -0.369838557087306
16 -0.453475682511066
17 -0.465014124175835
18 -0.484352068570129
19 -0.567181289449513
20 -0.660284071315204
21 -0.760980874674149
22 -0.929667794496922
23 -1.04005345372741
24 -1.13371405113159
25 -1.23981475580746
26 -1.44703830257392
27 -1.57161948805238
28 -1.80304751755776
29 -1.98695219902621
30 -2.18059182911325
31 -2.36833511624149
32 -2.52405395364716
33 -2.75237669534244
34 -2.87138770967981
35 -3.00925580662777
36 -3.18766886349552
37 -3.3556049799489
38 -3.47914881683092
39 -3.57722340127159
40 -3.69924080763327
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0962897531977958
1 0.104626782653122
2 0.153647135369858
3 0.129784718024112
4 0.0607432062053799
5 -0.0226196745234675
6 -0.103176121029122
7 -0.0892345762312079
8 -0.0543232655733372
9 -0.00804027678502228
10 0.0161097147177474
11 0.0814924010260847
12 0.15298912563086
13 0.206656728841225
14 0.060946639994917
15 -0.117053275328788
16 -0.141921507442113
17 -0.175148826145573
18 -0.19782093929025
19 -0.210772409250601
20 -0.179847970869631
21 -0.237615234098795
22 -0.279824569622597
23 -0.337852173396125
24 -0.294096804436325
25 -0.23599438040384
26 -0.284013011781929
27 -0.181194550413187
28 -0.137351881744189
29 -0.138239433920373
30 -0.0884116774088968
31 -0.0643553651168332
32 -0.0453403098489429
33 -0.0534433477097425
34 -0.0752247374709554
35 -0.052185792593535
36 -0.0748889051860413
37 -0.115655663851071
38 -0.118192443654042
39 -0.109977194884491
40 -0.0653286704552074
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.108849337058667
1 0.246328638102126
2 0.413458761115691
3 0.480246750900004
4 0.488108488232343
5 0.424414247600695
6 0.378396577288601
7 0.405431418786794
8 0.492521638934665
9 0.619112839990856
10 0.537664200143691
11 0.573817912929013
12 0.701056616991076
13 0.842365580444593
14 0.837019196053277
15 0.775118412422207
16 0.815547215269966
17 0.789817029072754
18 0.711285062254679
19 0.651653409616708
20 0.628213548621567
21 0.671228645149169
22 0.664614787087604
23 0.691217113603662
24 0.697906862343593
25 0.741441188696346
26 0.720908369032865
27 0.728033792172085
28 0.706851710213771
29 0.660901010304877
30 0.662061426201428
31 0.735971770254353
32 0.730756504803936
33 0.695731892726962
34 0.765724140389155
35 0.77499935931012
36 0.769350655900576
37 0.823000465899858
38 0.842703023993328
39 0.899455414932145
40 0.904572264583961
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0670029844140374
1 0.241949800580211
2 0.389207988272581
3 0.375335651061099
4 0.326774538711622
5 0.22804977255956
6 0.100133024949833
7 0.15537540321737
8 0.263256312409057
9 0.359928611800539
10 0.360403408829788
11 0.410393583148148
12 0.460469946143108
13 0.576299993220051
14 0.555580715291133
15 0.526481595084008
16 0.488177548650583
17 0.482304772497739
18 0.455418320490518
19 0.443099156649501
20 0.458725256703205
21 0.380128784502269
22 0.371872619729281
23 0.356804477665596
24 0.375969877274138
25 0.352263087060425
26 0.271892127790959
27 0.329441741440184
28 0.255270964963886
29 0.126906605981637
30 0.010941711283019
31 -0.0153966211507672
32 -0.147092189499662
33 -0.271076983876442
34 -0.45074136939855
35 -0.668864811108973
36 -0.844838969780991
37 -1.06433187985485
38 -1.25856578700361
39 -1.42748634144834
40 -1.58191959354928
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.154275648150222
1 0.263054909818782
2 0.337484219759086
3 0.239130952574491
4 0.160899798378868
5 0.0824461250630804
6 -0.00227080118516731
7 0.024164533200481
8 0.0757506128611531
9 0.19551535678116
10 0.127711390155983
11 0.199562924400173
12 0.355738154964107
13 0.453919553274886
14 0.267437977335695
15 0.0928018857903536
16 0.0853361273349633
17 0.0858904208183882
18 0.00687201708812779
19 -0.00875390734787329
20 0.000226326668734789
21 -0.0112546163805236
22 -0.00025868699858389
23 -0.065719148908141
24 -0.0285586763089096
25 -0.0600380967000937
26 -0.0745375161903197
27 0.0676165859052418
28 0.0570053145161276
29 0.0299784792842623
30 -0.0363842605595788
31 -0.0116076813449184
32 -0.0168553442773711
33 -0.0531780639290025
34 -0.046603476763496
35 -0.0940744801944446
36 -0.19892946106915
37 -0.327158973082657
38 -0.393528705070544
39 -0.384054022923318
40 -0.465478494781564
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0682635847583413
1 0.155307792713274
2 0.248889427387979
3 0.179137592716903
4 0.083170451594254
5 -0.0418284049421196
6 -0.204181429531975
7 -0.176557240882282
8 -0.112100888413836
9 -0.0101234450730883
10 -0.0647365994583877
11 0.0256765198105717
12 0.10709748612279
13 0.202397021886976
14 0.109041588929858
15 -0.0164817567448323
16 0.0123179369046005
17 0.0565041513106812
18 0.0411169767434711
19 0.0019886576612449
20 -0.0172482946794776
21 -0.0910001122556019
22 -0.202012939937579
23 -0.321080359866567
24 -0.352276202326317
25 -0.406571619418223
26 -0.41015717386267
27 -0.444903778817833
28 -0.462104226260315
29 -0.547998990931001
30 -0.640359063810346
31 -0.708699062617484
32 -0.817717114455151
33 -0.854514094051302
34 -0.953024853885353
35 -1.02945742623604
36 -1.10588691595453
37 -1.16715797249394
38 -1.20722658309226
39 -1.25827022025801
40 -1.29895538978594
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0850996201839576
1 0.229987458778826
2 0.326204682180698
3 0.258474175212965
4 0.146879143029204
5 0.0319575702687542
6 -0.153805065506383
7 -0.0736995740369757
8 0.0138245389830587
9 0.100013968843578
10 0.0641354283201103
11 0.0970326858149315
12 0.19749691427145
13 0.335337587921099
14 0.307046997210712
15 0.281469748838882
16 0.328346718393227
17 0.362134583367169
18 0.291517119481863
19 0.207696734771344
20 0.13560776069198
21 0.00451512677951849
22 -0.0674196164775895
23 -0.0670283721235125
24 -0.0511659544627934
25 -0.0387090666771313
26 -0.0110244365904717
27 0.0350763819201174
28 -0.0325664605807066
29 -0.0232394644992739
30 -0.026771621839508
31 0.0213480811419657
32 0.0361530633801763
33 -0.0268815181262316
34 -0.0784871168982049
35 -0.107053097397616
36 -0.234897208349563
37 -0.302175573562648
38 -0.394032136742317
39 -0.430842794733974
40 -0.477460006096874
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0659493491486041
1 0.109389280383283
2 0.259550279058135
3 0.242144720772327
4 0.220517251210155
5 0.135647655006057
6 0.0332428847942219
7 0.0475518758874305
8 0.0941906735773559
9 0.173378270642092
10 0.154721187346714
11 0.274064977698867
12 0.374248369509803
13 0.524491229666688
14 0.526164008740351
15 0.462674710058744
16 0.465694371299564
17 0.435976834036293
18 0.365956084566603
19 0.294425048539741
20 0.317415840511136
21 0.259660895199774
22 0.334928798766652
23 0.332352513296805
24 0.359251846235614
25 0.317531419344086
26 0.230907337019131
27 0.291263553951072
28 0.197664231060682
29 0.110021407780909
30 -0.0212732953607464
31 -0.0866268308486768
32 -0.183204149507459
33 -0.271964033504261
34 -0.31683185156484
35 -0.40278615465286
36 -0.49719851906553
37 -0.583161082427597
38 -0.678019429134121
39 -0.705085271804796
40 -0.770783502938657
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0506431617170211
1 0.0547864457772405
2 0.152488047539872
3 0.134354486808011
4 0.140681908034082
5 0.114801995443639
6 0.0729695993054169
7 0.0932581940509523
8 0.146967336859711
9 0.199344717169202
10 0.180157291020973
11 0.208899784058497
12 0.273878558843913
13 0.296617027689179
14 0.141320104550526
15 -0.0460328826017071
16 -0.128677149359488
17 -0.0953421877608993
18 -0.0591784570458751
19 -0.0887912435496259
20 -0.0221736666621184
21 -0.0113583071076104
22 -0.0162105728452033
23 -0.047260216898791
24 -0.0966251562831764
25 -0.1030132434624
26 -0.234652203844675
27 -0.237132141153133
28 -0.291115499911962
29 -0.259681081290863
30 -0.30236707923929
31 -0.291706187320795
32 -0.335472407141111
33 -0.369130983973859
34 -0.349520174879772
35 -0.338752052469547
36 -0.349052299559752
37 -0.332089179978127
38 -0.33867021884123
39 -0.341177889350873
40 -0.350467767312834
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0903104268461528
1 0.108078440624032
2 0.151838008610489
3 0.161536950629389
4 0.137230758000866
5 0.0876094201537314
6 -0.045902842363835
7 -0.0465747928757514
8 -0.0365138670516187
9 0.0473155113655901
10 0.0973511256751136
11 0.149937778986134
12 0.183268904513611
13 0.185360185544741
14 0.17587363065903
15 0.11616247311302
16 0.0909401742128115
17 0.0561938897575711
18 0.0153988221782484
19 0.0146251437878275
20 0.0158546439229887
21 -0.0245573501515053
22 -0.0214983007814453
23 -0.0689402515768798
24 -0.0602497808897202
25 -0.0579858273295262
26 -0.0802653132439053
27 0.00325629844677744
28 -0.0384721620025661
29 -0.0726840359155756
30 -0.0941504356410401
31 -0.0168930431433121
32 -0.034518034769162
33 -0.133226606230072
34 -0.0835519573578405
35 -0.0637222174486287
36 -0.163325437330738
37 -0.233754679210939
38 -0.277536742327527
39 -0.277076251695359
40 -0.276791608216136
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.124775602911534
1 0.188328709960564
2 0.188660253571382
3 0.097776973614434
4 0.00979550112994776
5 -0.10363415856172
6 -0.228917762492211
7 -0.223461560063884
8 -0.107944235148217
9 0.0341226515913529
10 -0.0402844706409788
11 -0.0331726911063477
12 0.0850552854649393
13 0.189931195095804
14 0.135706853082342
15 0.099832833414939
16 0.115279853031653
17 0.1901124139425
18 0.139758009940198
19 0.0727186172199059
20 0.0560976843267667
21 0.0131798395552294
22 -0.0997624218479374
23 -0.155302766916522
24 -0.160214157751138
25 -0.204544771713774
26 -0.245013091555356
27 -0.268377532489574
28 -0.34881019570559
29 -0.436512630569722
30 -0.475877086689433
31 -0.45239083123168
32 -0.487658836423613
33 -0.487642438805542
34 -0.361016613250226
35 -0.281519095705827
36 -0.180715082763622
37 -0.0197823808398416
38 0.121775743133693
39 0.249795915352096
40 0.429744861531095
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0918713412971042
1 0.159751733573898
2 0.263729290369191
3 0.298943991578789
4 0.292201121609282
5 0.246568013720876
6 0.0462904735011462
7 0.0372511794493251
8 0.0591776618349718
9 0.0760185942725604
10 0.0857391880509804
11 0.114776081035322
12 0.158083773905074
13 0.249881790196352
14 0.320656048617655
15 0.300183124052512
16 0.289959918048722
17 0.259965871192741
18 0.212243875573217
19 0.184470372856143
20 0.196128458219705
21 0.205702592071161
22 0.21230251551961
23 0.175096209093439
24 0.179183284818896
25 0.162278842598036
26 0.10988858626471
27 0.166226835827429
28 0.0400113852311899
29 -0.0662457539633663
30 -0.199216385032661
31 -0.245775195990898
32 -0.344667309439742
33 -0.462742767814308
34 -0.542987503885638
35 -0.611758379672897
36 -0.673554522318079
37 -0.794754150747375
38 -0.93629157314406
39 -1.07788769887403
40 -1.19102761604769
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.117250961715724
1 0.19683687164664
2 0.354059239228426
3 0.361086997855107
4 0.4315242527081
5 0.454678573070246
6 0.437062848598623
7 0.488354793064387
8 0.573337923762623
9 0.740036892696354
10 0.756163382191668
11 0.871026683970291
12 0.996363688156142
13 1.10496474153512
14 1.15731766388287
15 1.16508429204941
16 1.18865291125452
17 1.23073105697342
18 1.2523779152327
19 1.2528617316477
20 1.31972784208042
21 1.36962232267987
22 1.41760953931493
23 1.40908158139377
24 1.53308546024948
25 1.62707551697452
26 1.58624200869504
27 1.6163087963926
28 1.48330192765901
29 1.39282686226095
30 1.34425697376358
31 1.36619903984203
32 1.37945281984065
33 1.4279942704075
34 1.43090554473796
35 1.46240382803636
36 1.50452882198119
37 1.55306968196047
38 1.59196178322578
39 1.59472411933451
40 1.58009859706028
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0846340406829902
1 0.175383082784746
2 0.298711861196944
3 0.21786774785306
4 0.157015787046471
5 0.0124609803986115
6 -0.125870584789521
7 -0.0657435921727512
8 0.00149028607691815
9 0.0835803775963089
10 0.0689481421235629
11 0.146915115527252
12 0.251544187220738
13 0.314029495562425
14 0.279252253572493
15 0.190243190078808
16 0.188867978005097
17 0.156823683336795
18 0.00907750499845461
19 -0.1075073616058
20 -0.199687963115109
21 -0.317402099430594
22 -0.322548882994212
23 -0.421859854978756
24 -0.42123273725765
25 -0.456135649883395
26 -0.512989161955275
27 -0.459583065974976
28 -0.576231488488062
29 -0.614543783380522
30 -0.685081323633136
31 -0.706708551901648
32 -0.769903923977299
33 -0.897564653574652
34 -0.903341022858923
35 -0.89824661321218
36 -0.91214832186809
37 -0.911113622391575
38 -0.904071423261016
39 -0.804656179524488
40 -0.789579937522236
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.135904851022227
1 0.219626358581515
2 0.306115594538559
3 0.301614012868006
4 0.258137158025579
5 0.172407985378018
6 0.0241112686445675
7 0.00335762889563496
8 0.050734514408969
9 0.092700545196609
10 0.112256165968535
11 0.0835330321615579
12 0.036368401638244
13 0.0703638401436697
14 0.0691908460099286
15 0.0423557982086278
16 0.0324401623860715
17 0.046236782332302
18 -0.0184454629472559
19 -0.106889320416137
20 -0.0567451913075052
21 -0.148803100547633
22 -0.242805288308731
23 -0.355096458999147
24 -0.334329720277979
25 -0.344721985143868
26 -0.386281067092598
27 -0.321677194421273
28 -0.430005269640421
29 -0.567018825989623
30 -0.677181682466404
31 -0.692412096465276
32 -0.760926770664862
33 -0.836120095189478
34 -0.772066622979443
35 -0.720794483350589
36 -0.771260746256978
37 -0.796578285351706
38 -0.813069878317089
39 -0.843885818963365
40 -0.842263138169503
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0713357831304089
1 0.142565097635448
2 0.215533453175218
3 0.238299205360905
4 0.222777515511718
5 0.158020486197612
6 0.0899310852900794
7 0.0813324832376994
8 0.172268353509274
9 0.260084290713555
10 0.277751880892434
11 0.347948715752209
12 0.406672969783075
13 0.435341014996399
14 0.378395044790588
15 0.251163706603908
16 0.21229582834777
17 0.161069650046938
18 0.162370036244061
19 0.0942795008185211
20 0.153465368207142
21 0.144142954085617
22 0.153268710916734
23 0.144188016623645
24 0.201391441298391
25 0.152769188515919
26 0.126930688196916
27 0.163563664955343
28 0.152042870981603
29 0.138785966732829
30 0.10664596886753
31 0.0885185586290769
32 0.134264258063011
33 0.113920744827394
34 0.0559519193853202
35 0.0150234383335208
36 -0.064712138000742
37 -0.107701640914061
38 -0.125646409516957
39 -0.172815348123073
40 -0.237237484445669
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0728755341528116
1 0.247403808538127
2 0.367689052954061
3 0.254686726944873
4 0.137293098801029
5 -0.00311768967328518
6 -0.15562262262497
7 -0.143431350215003
8 -0.028808050284006
9 0.0382973330097656
10 -0.120239314274564
11 -0.0626438315807234
12 0.05068717717347
13 0.177024893994187
14 0.162222856858159
15 0.152745453453794
16 0.115049609375795
17 0.112635935652508
18 0.0364818303575394
19 -0.0195663988624974
20 0.0391439205997819
21 0.0855187742452075
22 0.175883097763477
23 0.147011562746214
24 0.135721885999464
25 0.156137713128691
26 0.151575128190759
27 0.168002164693292
28 0.168435612161474
29 0.22581071251125
30 0.232815405966896
31 0.29226669898069
32 0.358837305917721
33 0.283656295397529
34 0.289294742186966
35 0.185723511267336
36 0.0584539016970664
37 -0.0159037724527944
38 -0.0411798538900414
39 -0.0722646819534143
40 -0.129583365018762
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0944691476976875
1 0.177225391435013
2 0.343358365915455
3 0.328798847335347
4 0.323980006172193
5 0.250686259677625
6 0.132182870755388
7 0.118923554876033
8 0.130734263765502
9 0.216768658236878
10 0.144108419345336
11 0.217662340613115
12 0.241720515863126
13 0.307326834615286
14 0.327887568301249
15 0.383518800481067
16 0.359158913069431
17 0.405504719002316
18 0.352409105568428
19 0.329863932132629
20 0.342883070857211
21 0.339026280385107
22 0.375044613741224
23 0.297664299373175
24 0.297446027972649
25 0.234444306935841
26 0.193274974566733
27 0.238746786271615
28 0.163674276422825
29 0.113520607837883
30 0.0660061967563079
31 0.00530309137642737
32 -0.0702217822783546
33 -0.177693204007808
34 -0.257403889675413
35 -0.412882448734456
36 -0.601828165506649
37 -0.714027053193317
38 -0.833190821779206
39 -0.941541604244015
40 -0.991262451085035
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0345234099582168
1 0.17764505486993
2 0.343717620088648
3 0.332966240637921
4 0.317008828713963
5 0.272255144070672
6 0.1986238237954
7 0.32875745861652
8 0.474727624448535
9 0.572466780608701
10 0.565463475847659
11 0.700988637097776
12 0.75619385818363
13 0.83393969996433
14 0.733383370374958
15 0.659378840381529
16 0.627778716932199
17 0.641358924407327
18 0.537306015799865
19 0.45541487527029
20 0.445239112505122
21 0.384544126488283
22 0.365099059935728
23 0.347492253914258
24 0.293730599828093
25 0.222086009706198
26 0.202262560260871
27 0.222100607016408
28 0.189316092974691
29 0.11557241852878
30 0.00646196701534274
31 -0.00595276453637306
32 -0.00501833707964883
33 -0.0521129275793806
34 -0.0381044896338469
35 -0.0336346748642655
36 -0.0346898498347716
37 -0.0183479918475737
38 0.0207979757150527
39 0.0928965578810526
40 0.106060817638148
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0784817719798521
1 0.147117616990986
2 0.193292037427232
3 0.220073034443852
4 0.150562683931429
5 0.0441865405860464
6 -0.0953801655818869
7 -0.13154661702405
8 -0.143641986410191
9 -0.129284788273818
10 -0.16594357548956
11 -0.180736445679445
12 -0.140983976733084
13 -0.119663382107592
14 -0.150889606575146
15 -0.258042275716869
16 -0.306284129311702
17 -0.331146445920124
18 -0.349374898087365
19 -0.375667802320206
20 -0.414868164884534
21 -0.423446208384686
22 -0.411229391863052
23 -0.496764114038612
24 -0.495352100484883
25 -0.52709599277014
26 -0.590424795497597
27 -0.579245503853385
28 -0.616450261808371
29 -0.605438216552022
30 -0.626849875346401
31 -0.577576906639947
32 -0.512535777056662
33 -0.550370706477658
34 -0.548480827997719
35 -0.545447011310013
36 -0.582255568347879
37 -0.638219122992043
38 -0.705505726714637
39 -0.753944551426875
40 -0.878945740271433
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.107800855363262
1 0.172848351741577
2 0.332870738129196
3 0.358971781962977
4 0.346669387427641
5 0.262419551317126
6 0.139725273947011
7 0.259785333420403
8 0.313219139031839
9 0.438648323829045
10 0.434016567526754
11 0.551758717170995
12 0.649754396761121
13 0.790803507307234
14 0.732864510726576
15 0.724891885692176
16 0.726019474080876
17 0.790233730992111
18 0.808534886623459
19 0.763829450968475
20 0.737442180362935
21 0.68155230509732
22 0.687669119919649
23 0.686584833673299
24 0.694017689767011
25 0.694736221969012
26 0.653084009535665
27 0.697533246655603
28 0.683621784742626
29 0.664577656677428
30 0.61587671027524
31 0.582969256931387
32 0.477813918317895
33 0.336050562240845
34 0.174909633989246
35 0.0440163755007337
36 -0.109995417782415
37 -0.250433617266577
38 -0.398003145046184
39 -0.495590356708032
40 -0.617321128221315
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0689925549168326
1 0.134841636807302
2 0.220981442936243
3 0.176402774183548
4 0.0861126035179298
5 0.00187583585442708
6 -0.0709858222003401
7 -0.0883560002198109
8 -0.0362637533173307
9 0.0287622440181328
10 -0.0822653178888508
11 -0.0158304141255825
12 0.0987142952102547
13 0.177720442344492
14 0.139693554763867
15 0.0811881183810046
16 0.0172713831859768
17 0.0149382018775954
18 -0.0722532847819752
19 -0.17221084350133
20 -0.209196162210372
21 -0.325361885925326
22 -0.293996728522983
23 -0.318158478083506
24 -0.265644200366554
25 -0.240989967561625
26 -0.275131689991667
27 -0.246962771330756
28 -0.318651984692219
29 -0.332962620010342
30 -0.346164794940994
31 -0.300981608807998
32 -0.301918510753063
33 -0.303872659321989
34 -0.248220689164075
35 -0.289819581649865
36 -0.322194810256942
37 -0.36808683364496
38 -0.409053417172814
39 -0.371073995345388
40 -0.345256566617391
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0294651636039589
1 0.157401604837797
2 0.264187958604529
3 0.217204487460772
4 0.148430504396312
5 0.00173208483884357
6 -0.138318662431523
7 -0.0102488500527764
8 0.095069619167202
9 0.214978929981754
10 0.154986668285872
11 0.205115049473502
12 0.231012624372439
13 0.285847012068169
14 0.187619313718317
15 0.0869822827185742
16 0.125706579958165
17 0.149226527974679
18 0.169009972240739
19 0.140699383945358
20 0.239642372938174
21 0.230534811213699
22 0.198921874878327
23 0.116077610032906
24 0.141027493582822
25 0.098916703285937
26 0.027616893224415
27 0.0715466127442865
28 -0.015860702619849
29 -0.0131246648712513
30 0.00773039773882944
31 0.0572931650305013
32 -0.0221356840417122
33 -0.170489334827445
34 -0.228609698358277
35 -0.365933892075088
36 -0.527626813462489
37 -0.639713366930341
38 -0.758858789802028
39 -0.848122473146847
40 -0.90535431989799
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.116914373644741
1 0.22140075576745
2 0.307432241623396
3 0.261393020570175
4 0.212680640318145
5 0.142145331438934
6 0.0675664849980384
7 0.195672453769703
8 0.295974184297649
9 0.406536498847875
10 0.349617303153631
11 0.437706377400945
12 0.487435382637049
13 0.546575254836326
14 0.576092494251879
15 0.532288023387967
16 0.533716477918982
17 0.492517061333241
18 0.432614290311842
19 0.404483839979104
20 0.370942494171852
21 0.307735809593885
22 0.296079898264255
23 0.250842340133191
24 0.272346950569929
25 0.237938315896606
26 0.12819383396124
27 0.0995553049692233
28 0.000392202882479875
29 -0.0373556244312496
30 -0.0455403077210557
31 -0.0448728322694927
32 -0.0148259149338306
33 0.0049262255561433
34 0.016679829293615
35 0.0164849425109712
36 0.0466684155445236
37 0.0119095994773262
38 0.0378051603863687
39 0.0388990101939926
40 0.00600223800009303
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.108747917276613
1 0.174452099942603
2 0.308562387945352
3 0.293539125426926
4 0.235277905439357
5 0.142600936169397
6 0.0191203934629347
7 -0.0219354883351119
8 -0.00436062720709351
9 -0.000810487993663678
10 -0.0134051699036699
11 -0.064502126226706
12 0.0139284061005482
13 0.0922533728890036
14 0.0775560704499885
15 0.0119557716205554
16 -0.0174033149787354
17 -0.0870166820336045
18 -0.150285860837177
19 -0.203930785058283
20 -0.263006008102349
21 -0.35016017934882
22 -0.414851498590778
23 -0.479814802336923
24 -0.529995221809151
25 -0.545091759008891
26 -0.575798083801377
27 -0.57941323995544
28 -0.673953447049669
29 -0.607099639098995
30 -0.593054296100243
31 -0.543630264372517
32 -0.517251762661183
33 -0.507278849842413
34 -0.356518147332094
35 -0.237058505567256
36 -0.11041403921012
37 0.0406117681208005
38 0.223273363865962
39 0.309165287667401
40 0.398355755639853
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0752435261083662
1 0.173543049922222
2 0.195444313864223
3 0.153289690136535
4 0.142455169236842
5 0.0886498383548111
6 -0.0114026015056945
7 0.00501943062293631
8 0.11213163640696
9 0.237318397520719
10 0.171177747434103
11 0.271825814125354
12 0.342711398725887
13 0.414463513633103
14 0.410821400174085
15 0.375715494210528
16 0.428780102292543
17 0.497067408757927
18 0.485802576950632
19 0.548717970879766
20 0.560941104974033
21 0.56468330768971
22 0.643609406441755
23 0.63530831224082
24 0.722065848081442
25 0.765396093371941
26 0.701679441181153
27 0.787364096111172
28 0.759945589437569
29 0.795922112368602
30 0.794477368766901
31 0.799672320178846
32 0.801926783314537
33 0.740329048867644
34 0.655283967388232
35 0.586318103433531
36 0.517421518577579
37 0.469321015676969
38 0.452975429064671
39 0.46427277749907
40 0.482572693223768
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.124474781913566
1 0.10115706177452
2 0.133273503421925
3 0.136584216197685
4 0.0828691897171572
5 -0.0244245843577184
6 -0.177630890834072
7 -0.175756471178391
8 -0.183500618996367
9 -0.139479196016775
10 -0.116378675160897
11 -0.0252609380384508
12 -0.041542614325615
13 0.000701331497085178
14 -0.0695685259006149
15 -0.146849937096825
16 -0.0974841315902424
17 -0.0940563187820183
18 -0.226046648195907
19 -0.323647425107769
20 -0.410391368720981
21 -0.511819135290893
22 -0.522248415832077
23 -0.562029818745296
24 -0.511325161487329
25 -0.508112620141012
26 -0.539226319201597
27 -0.458565170275608
28 -0.569493709008343
29 -0.571726100094415
30 -0.568287901499235
31 -0.590843872363024
32 -0.581537066315873
33 -0.62516196846269
34 -0.563974806131684
35 -0.512671093930447
36 -0.539132559355847
37 -0.495157111704662
38 -0.45641883280316
39 -0.403562964943098
40 -0.375181238865814
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0675695528966558
1 0.224704009457893
2 0.296600084585031
3 0.258139009900569
4 0.214754476562903
5 0.152500512476616
6 0.0965421394391823
7 0.216211797572503
8 0.351856116948487
9 0.457626079235032
10 0.470507957556429
11 0.549809381223036
12 0.637932234424459
13 0.773702538619212
14 0.829188100953708
15 0.846440134856192
16 0.829872032042887
17 0.805295300010762
18 0.703243063416398
19 0.650841830735053
20 0.594559349767122
21 0.516082293055061
22 0.464722395404119
23 0.440581967556256
24 0.410884966565237
25 0.39871130097504
26 0.397980122722023
27 0.29042566398884
28 0.146370980631109
29 0.129146891512321
30 0.0830757201259456
31 0.0340142805153381
32 -0.00468394780363646
33 -0.0714412803346409
34 -0.104429746676041
35 -0.0844618338756589
36 -0.132325067082839
37 -0.12474377319405
38 -0.126319442822221
39 -0.10222772194776
40 -0.083961671567387
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0967736882594199
1 0.139960784567413
2 0.198357148774928
3 0.240874105685576
4 0.288301301577148
5 0.273584627557882
6 0.167232280933135
7 0.189455040442149
8 0.19599281004473
9 0.239194001450485
10 0.194096327147284
11 0.202978440205264
12 0.24961671188419
13 0.296007705514694
14 0.276798587676563
15 0.223662328679768
16 0.213450701477409
17 0.152121148475435
18 0.00818056758888064
19 -0.0937181393918933
20 -0.13202870006264
21 -0.2752000920831
22 -0.358129848516685
23 -0.419480743004807
24 -0.424252361798772
25 -0.469425987150368
26 -0.555264014168069
27 -0.502542157379071
28 -0.61676072723453
29 -0.698533080388054
30 -0.740215514758798
31 -0.777677083620008
32 -0.836774208991539
33 -0.855191926585159
34 -0.762060816767946
35 -0.717017529494659
36 -0.74119129577358
37 -0.734573903700049
38 -0.662846988189933
39 -0.558582276894329
40 -0.44655598506068
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0771863768678966
1 0.134253480240958
2 0.274882015422175
3 0.3151147524605
4 0.346561553128344
5 0.351882538152553
6 0.297481929949505
7 0.305368610799704
8 0.326698855960325
9 0.401490438094318
10 0.362044276206534
11 0.453081552864281
12 0.501317439848425
13 0.595552836788316
14 0.605638423465325
15 0.605367581028122
16 0.642322592993909
17 0.63122571308315
18 0.571004019646027
19 0.502281497687187
20 0.436644143644977
21 0.389251867857036
22 0.338192293627111
23 0.207327838130427
24 0.132688012622995
25 0.00818007714911584
26 -0.0216036254869798
27 0.0351845384296912
28 -0.0811885947803699
29 -0.135219733749978
30 -0.213122062216424
31 -0.280820516972414
32 -0.391103318746642
33 -0.522244574638765
34 -0.663617239381077
35 -0.82948858960854
36 -0.997052587608819
37 -1.14788135808772
38 -1.30580009906402
39 -1.5627220069261
40 -1.70706046610028
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0686605574203276
1 0.196463302583168
2 0.22640342610215
3 0.171788573914872
4 0.0587642718058992
5 -0.0713054777333295
6 -0.205569714075545
7 -0.169524353773252
8 -0.095326700763587
9 -0.055124681490021
10 -0.0302962397377322
11 -0.0285030448297898
12 0.0617470100158268
13 0.20627570963758
14 0.151063627808599
15 0.116660770029549
16 0.132839548630738
17 0.181728139264616
18 0.178864534572376
19 0.169356255886046
20 0.136477625373681
21 0.181055361760442
22 0.1829841731176
23 0.154148562199112
24 0.134134601405789
25 0.13005034682535
26 0.129380193761786
27 0.146211594596046
28 0.18453946134533
29 0.208841057571447
30 0.126804117556003
31 0.0609300410758888
32 0.0085332995808165
33 -0.107247809903319
34 -0.135363618702202
35 -0.186443195713548
36 -0.243441791938507
37 -0.281713238294744
38 -0.292874942832842
39 -0.335911312283582
40 -0.428150909566768
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.115937592415646
1 0.226413905794828
2 0.274949845786634
3 0.297989969344978
4 0.325460984645556
5 0.325665815998142
6 0.236663313123917
7 0.266046513338568
8 0.314327619187299
9 0.404562941928134
10 0.357405069307829
11 0.467661646479809
12 0.547557129778852
13 0.627337629354251
14 0.544013355905957
15 0.406438747405893
16 0.499805584486303
17 0.509233208095102
18 0.479118050880863
19 0.45787508898304
20 0.408049750055302
21 0.278238956971693
22 0.213821411991188
23 0.0673064341887888
24 0.111447175374709
25 0.115348401793514
26 0.103813943994655
27 0.109744337030026
28 -0.0307800271449201
29 -0.113877929915946
30 -0.22547891849991
31 -0.28611553763239
32 -0.360418408874063
33 -0.490207168767786
34 -0.52521661514868
35 -0.592061913002219
36 -0.685309922414146
37 -0.777325765431873
38 -0.895783062761865
39 -1.01581562326809
40 -1.1166985671091
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.1158897577108
1 0.195477816188354
2 0.345972500961695
3 0.366917627391031
4 0.322205229595585
5 0.272224246514536
6 0.152631937897695
7 0.192563927866064
8 0.302333758666544
9 0.379278766901239
10 0.404444886602128
11 0.458142637923844
12 0.577846008724329
13 0.64258335259572
14 0.679265740859541
15 0.704990790487147
16 0.751169901505019
17 0.787048409080672
18 0.753844034593408
19 0.827781360912338
20 0.94663552664853
21 0.950157519584371
22 0.997216921336515
23 0.98276803656473
24 0.997808285782745
25 1.05307243655513
26 1.00028655097768
27 1.06176197006886
28 0.931609657919993
29 0.907834115203958
30 0.840273504836845
31 0.786770745844897
32 0.751435722756481
33 0.705990859094165
34 0.750644430389564
35 0.762772318110284
36 0.668672750062411
37 0.552046146294531
38 0.499636547740044
39 0.485306499660385
40 0.483316587571535
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0938974033547928
1 0.208648848771031
2 0.342948829410798
3 0.329244920462152
4 0.381385046403275
5 0.39123533912087
6 0.361437228409482
7 0.431147838154984
8 0.488843614427323
9 0.651125221030522
10 0.682929683620943
11 0.808621188096591
12 0.973573647350067
13 1.10912168360582
14 1.10542819671705
15 1.08318186281305
16 1.06273310059923
17 1.11874141663132
18 1.05448057349663
19 1.05104757785574
20 1.02240348737786
21 1.01111927542315
22 0.893283670932428
23 0.790320931074167
24 0.818324896770028
25 0.761327041865963
26 0.765953126289293
27 0.775140220923402
28 0.718589162276257
29 0.65071915078326
30 0.605626339971386
31 0.627084477225664
32 0.627528443073863
33 0.636855721147849
34 0.645932599358571
35 0.671563168819682
36 0.622529316530687
37 0.584776500319109
38 0.616267448916645
39 0.705544689931386
40 0.754151742373737
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.11771227742557
1 0.0944276705586535
2 0.174687950916004
3 0.126147287668375
4 0.0349012325293172
5 -0.0298535420118755
6 -0.137399542356886
7 -0.216181494156804
8 -0.243245940279906
9 -0.222386146166576
10 -0.258322471731208
11 -0.269609808334857
12 -0.258447354579398
13 -0.195103916163597
14 -0.227077972730366
15 -0.304121491587598
16 -0.29604890505895
17 -0.294380214964774
18 -0.351934087837905
19 -0.431069018383644
20 -0.473252348048754
21 -0.500150422818147
22 -0.567020273986048
23 -0.614639738849482
24 -0.5918270802699
25 -0.576172381005621
26 -0.662792604173656
27 -0.64235189079764
28 -0.76848341992718
29 -0.806645261347559
30 -0.889466406038185
31 -0.915834863025968
32 -1.01582160844565
33 -1.14286482117404
34 -1.28958077157378
35 -1.37434359378501
36 -1.44252283696824
37 -1.46401892781409
38 -1.50136633650188
39 -1.60274754796525
40 -1.60691079144828
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0970613528690598
1 0.17610946165211
2 0.322706135965289
3 0.320968421501986
4 0.258459610950035
5 0.150849145940393
6 0.0601704989598675
7 0.133301418108817
8 0.21441801401432
9 0.266390165339855
10 0.199670366483527
11 0.256331045293943
12 0.303575496779165
13 0.33709097892648
14 0.255915252064446
15 0.20355500101033
16 0.176324489927611
17 0.163990841022564
18 0.113140823193629
19 0.0235804409199853
20 -0.0140174000480306
21 -0.033051232433023
22 -0.000755644544110368
23 -0.0105229796793886
24 0.00761583987782899
25 -0.016662708454616
26 -0.075519018539147
27 -0.00350059880988862
28 -0.107340468057336
29 -0.0803624367196023
30 -0.130654616693006
31 -0.120305669245481
32 -0.091337300993994
33 -0.203074678363473
34 -0.178924761665458
35 -0.148047234396769
36 -0.130627382685209
37 -0.125929863393859
38 -0.10805684613121
39 -0.0524171046047979
40 0.0217017394237708
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0976283525932224
1 0.203828621913762
2 0.333920877885998
3 0.31161657093844
4 0.268914013881489
5 0.202324505206588
6 0.128893298718438
7 0.146987220310197
8 0.258205716817686
9 0.354532563341263
10 0.365840480641909
11 0.446158704303462
12 0.568191990001344
13 0.678227845687169
14 0.622976234624744
15 0.527952909052472
16 0.567740877215523
17 0.645065862504775
18 0.612581153767107
19 0.60548882429919
20 0.647907005398762
21 0.632468996650406
22 0.63381886147016
23 0.572567762722672
24 0.609599541235804
25 0.632382701142471
26 0.584561778545077
27 0.606356109693913
28 0.56715968560607
29 0.498240738223886
30 0.442955853241234
31 0.433174364782968
32 0.404773995436274
33 0.287425312010018
34 0.374734770921354
35 0.485716706519699
36 0.418581460288094
37 0.456075949067281
38 0.498987138781533
39 0.572656443028505
40 0.592017723950012
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0698474308313974
1 0.224614123515928
2 0.400214782048941
3 0.391124861412601
4 0.409263637322054
5 0.36937596606841
6 0.28850109943036
7 0.405939923644187
8 0.561546787608126
9 0.687523407856786
10 0.715089471124197
11 0.870842508638615
12 0.967428654557945
13 1.1194687222068
14 1.12933044210031
15 1.08983532428319
16 1.10273463101007
17 1.07738039237021
18 0.993773484322849
19 0.910298840914733
20 0.876023204486323
21 0.785976905585987
22 0.763041530874852
23 0.656304798025669
24 0.717084609863293
25 0.644423875230126
26 0.586428122176897
27 0.647972529221808
28 0.622796175178077
29 0.638384848869769
30 0.563836334774745
31 0.417837283489918
32 0.292058991927375
33 0.219086715684166
34 0.113845852446086
35 0.0489666323092286
36 -0.0019463832223372
37 -0.0771174241124255
38 -0.148518904346497
39 -0.214384920714286
40 -0.34284664345597
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0842695611353856
1 0.198523297699181
2 0.293465584473327
3 0.211283941481344
4 0.112853180701385
5 0.0560544708539732
6 -0.0123413229503049
7 0.0241298754850749
8 0.0869453016488664
9 0.176998953305115
10 0.130452982012716
11 0.148865766007988
12 0.194800111592081
13 0.239507210413265
14 0.226299620499591
15 0.197775547766316
16 0.131148468817252
17 0.115964490488683
18 0.0664042112015206
19 -0.0075451309289285
20 0.0333102904329219
21 -0.00916342898215872
22 0.00779969654850365
23 -0.00123913464465009
24 0.0112983762744165
25 -0.0458222194679956
26 -0.18634715720411
27 -0.145506010169201
28 -0.359322065463729
29 -0.445949657458128
30 -0.529795621741454
31 -0.523422176704016
32 -0.53700089316622
33 -0.626184646654965
34 -0.536506702636308
35 -0.483225424161181
36 -0.54266079411072
37 -0.539344953405619
38 -0.444933528769131
39 -0.368230787830841
40 -0.27811487251619
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0492914355176444
1 0.204055243382902
2 0.268658538706688
3 0.292634378405166
4 0.334834706884336
5 0.358226703092774
6 0.290332121471907
7 0.359783797360304
8 0.466059687263909
9 0.545423186501385
10 0.59429673931429
11 0.666449106702418
12 0.761889290797757
13 0.811151142994417
14 0.769224753544549
15 0.679247959426944
16 0.643510873051178
17 0.611885422713486
18 0.581932699612921
19 0.542073403969483
20 0.527851923658426
21 0.497488167580648
22 0.456593018659723
23 0.410061137755341
24 0.495938193246063
25 0.568205146702879
26 0.582368928092631
27 0.652698003431953
28 0.643382902806543
29 0.665263648880546
30 0.714332493093188
31 0.738444310860429
32 0.742793114107049
33 0.70613993641306
34 0.667099225434514
35 0.576480526260193
36 0.572418982034919
37 0.548842778591976
38 0.600149293558964
39 0.666742741131237
40 0.673834445733912
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.108230137090253
1 0.171319343188463
2 0.234606447092915
3 0.137187488902755
4 0.0864483704729291
5 0.0120896478026933
6 -0.048782978113143
7 -0.0383247324589333
8 0.0167208952210904
9 0.0742440421920447
10 0.0317942046663608
11 0.0460853605770626
12 0.0770080618371649
13 0.125651489860454
14 0.144466142431479
15 0.200235721498202
16 0.158017504133862
17 0.172384542072468
18 0.0890599751582042
19 -0.0416536367759681
20 -0.0660655905747918
21 -0.101490207594519
22 -0.115842417411312
23 -0.256829212499817
24 -0.326171803715728
25 -0.472787077314984
26 -0.622162176260239
27 -0.605786071485387
28 -0.729217495737457
29 -0.857519668983061
30 -1.00026867468325
31 -1.04170798170635
32 -1.10395989002842
33 -1.22244590777643
34 -1.22419908533354
35 -1.27889854891109
36 -1.4271097309525
37 -1.52270934461966
38 -1.66563334752993
39 -1.81392330204643
40 -1.94540873944693
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.111741754834008
1 0.180648705086563
2 0.225495265945375
3 0.21774777028497
4 0.175087230552901
5 0.103706886910768
6 0.000985902121811488
7 -0.0325861972203669
8 -0.0145653321764621
9 0.0617838420477277
10 0.0150514998276394
11 0.048737013658934
12 0.154144532134729
13 0.287127201733031
14 0.203369065643338
15 0.0550895146848296
16 0.0402967582145553
17 0.0194608972813883
18 -0.0731023333144529
19 -0.0928279653786901
20 -0.134711693054331
21 -0.141419201243607
22 -0.176709905382323
23 -0.19627704631897
24 -0.222248291715188
25 -0.290398899200068
26 -0.414233140623822
27 -0.46136344563953
28 -0.62662965142487
29 -0.765594730152355
30 -0.901721614385405
31 -1.03009530732509
32 -1.12987482194028
33 -1.22849207217436
34 -1.31457652019368
35 -1.38459989305613
36 -1.49693227402752
37 -1.58473167348369
38 -1.69248938563788
39 -1.76371491820439
40 -1.93692433028094
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0776209399345111
1 0.181812312080782
2 0.241347478941351
3 0.222786251690962
4 0.171680011574929
5 0.0989932607994706
6 -0.0552571429683613
7 -0.0604853419618143
8 -0.0852079038867064
9 0.0244014997123245
10 0.0172451304701502
11 0.116007726137981
12 0.150588361246587
13 0.129160922811387
14 0.0893752714371292
15 0.00839243621096664
16 0.0429293134533233
17 0.107886823897399
18 0.138788565740855
19 0.116268038783405
20 0.105419346563751
21 0.0529788725563307
22 0.00249758657733512
23 -0.0153621753868793
24 0.00754066358487204
25 0.00230483921927238
26 -0.0199028870490947
27 0.0321419043115898
28 0.00766556031608401
29 -0.000576936843089015
30 -0.00344517708857817
31 -0.024321281051396
32 -0.0523479181149957
33 -0.0212892191796268
34 -0.0918482377324832
35 -0.0655192575707355
36 -0.0481764979491985
37 0.00340761491089969
38 0.0524639829223617
39 0.0981138285146215
40 0.175195747214382
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.100037306422804
1 0.192207099941059
2 0.365927499366248
3 0.364976029283994
4 0.331852921345226
5 0.269740224840761
6 0.15342909446151
7 0.18312243144798
8 0.217866238979593
9 0.22418586504196
10 0.159101555938472
11 0.200196020622302
12 0.274710950413809
13 0.395011237196544
14 0.433475673819633
15 0.392953447070038
16 0.407631905720519
17 0.404231799219076
18 0.390739196458035
19 0.39590182439332
20 0.37901734237384
21 0.304159616410054
22 0.277545254732519
23 0.174366044251544
24 0.102955478485559
25 0.0505854828479118
26 -0.0465538746823868
27 -0.0453782545716779
28 -0.206782701501157
29 -0.315719376840665
30 -0.454233071256327
31 -0.484688793056927
32 -0.556382852184242
33 -0.661108647770838
34 -0.831749273324571
35 -1.0166564426927
36 -1.10403958288053
37 -1.2439262490649
38 -1.41491933111183
39 -1.62721348223428
40 -1.84154098617153
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.104856256033059
1 0.200953964987781
2 0.292728774979426
3 0.222271461002772
4 0.0511266725316255
5 -0.0667733253375764
6 -0.266986548904532
7 -0.152728310903439
8 -0.0383272544819504
9 0.0821019751711813
10 0.101195943451977
11 0.126443244118567
12 0.181374240539624
13 0.248432560945348
14 0.22112726924686
15 0.147755006189596
16 0.12298486184657
17 0.029079879921297
18 -0.0360090726948177
19 -0.0811091753962474
20 -0.108960664890778
21 -0.164399564475503
22 -0.114648728660858
23 -0.0421038800171818
24 0.02892721734802
25 0.0985072598264787
26 0.108548996354448
27 0.253019292745024
28 0.167497484837159
29 0.113704941390541
30 0.0199021838721989
31 -0.0430031528361532
32 -0.0895456302585016
33 -0.136142130828432
34 -0.186259195362871
35 -0.263330466932792
36 -0.354043885356183
37 -0.494674184555332
38 -0.597105374901857
39 -0.721002487708075
40 -0.785998496628962
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0984199595054998
1 0.178325529550329
2 0.276856710988024
3 0.313067854723153
4 0.346142956362539
5 0.340820836091366
6 0.273386066940918
7 0.296715441575391
8 0.329700099428201
9 0.462277728400608
10 0.50580864091513
11 0.539382707245738
12 0.65405778155085
13 0.759362698100956
14 0.683715285135734
15 0.579147007986194
16 0.547551411997617
17 0.519787667439081
18 0.418905605778674
19 0.324091746778016
20 0.312155449873298
21 0.313405718591576
22 0.294267437104719
23 0.287364676105744
24 0.343539517362757
25 0.343623202094355
26 0.323982528924466
27 0.344730709336928
28 0.255320927254219
29 0.183360167030261
30 0.0477432776192823
31 0.00511345350729853
32 -0.115813190636325
33 -0.278681309452153
34 -0.416643974153406
35 -0.60239262021193
36 -0.777606714568146
37 -0.871990408748326
38 -0.958380933833223
39 -0.981825664260338
40 -1.08150681637001
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.13192987248698
1 0.232383909860847
2 0.337583209201084
3 0.277951393402121
4 0.187890649523987
5 0.0675145672525685
6 -0.10883710752384
7 -0.0922216074811431
8 0.0443408544622854
9 0.125795704566436
10 0.0796862346815539
11 0.134268442661849
12 0.20721406273401
13 0.226765714312778
14 0.155754096314419
15 0.0415634595908307
16 0.0167644195300665
17 -0.0047838786553478
18 -0.0527765003708671
19 -0.127157708028204
20 -0.133580800484786
21 -0.166263802128047
22 -0.12557216269053
23 -0.162348818571451
24 -0.186042160993072
25 -0.178832933416643
26 -0.245216429902781
27 -0.177350111331859
28 -0.274351851729942
29 -0.326525378850864
30 -0.404040243005792
31 -0.395362801079366
32 -0.546941503981822
33 -0.705176310495015
34 -0.614718259701099
35 -0.65660893366521
36 -0.730200672954822
37 -0.779868660950397
38 -0.825067192287053
39 -0.828577491656401
40 -0.814405839477554
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.066023547726378
1 0.179327736792499
2 0.284661121912937
3 0.214455599886896
4 0.135770888754822
5 0.0408996457724164
6 -0.0290566351188737
7 0.0163403091170551
8 -0.000899207009382952
9 0.0246897049461232
10 -0.037058689550062
11 -0.0374859620156713
12 0.076724852575174
13 0.205225498980642
14 0.110268211776681
15 0.0429855648716484
16 0.0530972957298887
17 0.12659555074093
18 0.120480992151145
19 0.152358081800829
20 0.181224269711845
21 0.171181947814419
22 0.147715119837012
23 0.146625985964325
24 0.192807538758254
25 0.20792715812449
26 0.159008114643017
27 0.225996889423959
28 0.167999410454412
29 0.100889984554913
30 -0.0247621076769513
31 -0.110271044863229
32 -0.259565001931719
33 -0.423827519786042
34 -0.570575203088826
35 -0.766301737555578
36 -1.02667150588166
37 -1.2767113756233
38 -1.56900924519274
39 -1.87088770509931
40 -2.18280032274398
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0821826715518297
1 0.145564112652808
2 0.258327244889116
3 0.288678199070305
4 0.27025718889996
5 0.163773854064806
6 0.0140332388990183
7 0.0286123639425138
8 0.14190726098119
9 0.219187086290688
10 0.230014255825839
11 0.270002008443471
12 0.361848283057092
13 0.488623151833802
14 0.425508688614655
15 0.355416254310148
16 0.330699488434773
17 0.319701402327698
18 0.253599171661012
19 0.10567965703931
20 0.0923933437073594
21 -0.0496300746966232
22 -0.140582935914404
23 -0.23159792053595
24 -0.298114668453119
25 -0.338969696177842
26 -0.351683034467367
27 -0.296486642370799
28 -0.33183239929648
29 -0.303806434812067
30 -0.309987402969735
31 -0.265451790458514
32 -0.255821311205481
33 -0.349445504749206
34 -0.271031351465335
35 -0.224384334384478
36 -0.177500821552053
37 -0.166876219719066
38 -0.132497253616778
39 0.0247501882013954
40 0.0748788775363125
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.102324366885278
1 0.123867258076566
2 0.220548679108135
3 0.125258442966424
4 0.0102454240319152
5 -0.119795382491193
6 -0.299008236743444
7 -0.257239080933162
8 -0.196416280986299
9 -0.0998667376228892
10 -0.152797671857408
11 -0.0974837304682696
12 -0.0446178487105455
13 0.0644732047183245
14 -0.0136326263951032
15 -0.0676670406336579
16 -0.030947450501368
17 0.0189697849030379
18 0.00651189826784915
19 0.031444470802779
20 0.0441053362277639
21 -0.048202261785097
22 -0.0821645037750236
23 -0.11266043734862
24 -0.0728468543651601
25 -0.111997532119674
26 -0.153906257538414
27 -0.0870011349380588
28 -0.141201450101519
29 -0.190104878938115
30 -0.326062739342303
31 -0.360807770824487
32 -0.402659237846973
33 -0.499897714834484
34 -0.473826666471116
35 -0.379276745219367
36 -0.333520128888771
37 -0.308642707462859
38 -0.22770809885009
39 -0.135081227449848
40 -0.0146295419590317
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0665545860203762
1 0.155854353214944
2 0.2738719015831
3 0.241794892558768
4 0.143096304818553
5 -0.00204598215419383
6 -0.165159865783361
7 -0.0894030428116928
8 -0.0345856375761278
9 0.0579244747138832
10 0.00452830700553264
11 0.0282240385017736
12 0.102751723020537
13 0.158290141223821
14 0.0808879696532294
15 0.0334229659506331
16 0.00956049316677499
17 0.0188320179024499
18 0.0228323301094253
19 0.0215426405897996
20 0.0143402706310165
21 -0.0316017257112322
22 0.0484542342012668
23 -0.028752213591515
24 -0.0346798660756633
25 -0.0765737366459764
26 -0.145286194683156
27 -0.0509076788108858
28 -0.101968055887513
29 -0.117903445910738
30 -0.143633127376053
31 -0.188067899070984
32 -0.280309982744295
33 -0.417249131252272
34 -0.498408802796211
35 -0.571465623345048
36 -0.684078232283647
37 -0.762277199209169
38 -0.765732625715132
39 -0.775863628729413
40 -0.891150959245661
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0829208224959368
1 0.195537894904355
2 0.25367702963324
3 0.158613949026375
4 0.124648842915032
5 0.0516814143038622
6 -0.067009827415311
7 0.0464663097397313
8 0.168599587252272
9 0.234791932017003
10 0.240534913381
11 0.265614831759064
12 0.262834591799515
13 0.303646352180997
14 0.365615199957575
15 0.420232363717391
16 0.474917076609887
17 0.443796801670937
18 0.400776314355442
19 0.325727358264639
20 0.30487359352492
21 0.266356546217207
22 0.335777713183525
23 0.346084506896651
24 0.447884557702876
25 0.496107451913457
26 0.471057620276222
27 0.482766829473418
28 0.388515543309195
29 0.304340772961905
30 0.2310170396856
31 0.237104578215351
32 0.22180199910179
33 0.157240328150419
34 0.212398770893349
35 0.314353918226578
36 0.361541780982654
37 0.411236163547497
38 0.497758668040303
39 0.615300152354764
40 0.714680054913725
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0440515037634537
1 0.106895292922031
2 0.166789998934297
3 0.107796473468996
4 0.0399235863475864
5 -0.0293185398222358
6 -0.145644076224604
7 -0.111422319886809
8 -0.0297966341413614
9 0.0702145995877155
10 0.0250502366197218
11 0.115674804971866
12 0.191075010424717
13 0.197338621129237
14 0.184225414464704
15 0.207508655096422
16 0.259292643208179
17 0.200986357298167
18 0.19942452053486
19 0.215662126577034
20 0.237338804573489
21 0.303143243166728
22 0.305677078363285
23 0.267142662652255
24 0.266404512593342
25 0.249754528075965
26 0.273584891667331
27 0.30057521261961
28 0.193374613949257
29 0.181461688297152
30 0.0709046808730815
31 0.0227995193619099
32 -0.0586484536962435
33 -0.103919721442865
34 -0.197480745393336
35 -0.24128584464727
36 -0.251194893145423
37 -0.280327143630904
38 -0.290183305616297
39 -0.335476508453319
40 -0.36651050336235
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0903023434643959
1 0.154601815400824
2 0.250049853522186
3 0.247631832856543
4 0.1889729398453
5 0.109165007625628
6 0.0357186079715834
7 0.0450816857413772
8 0.100092442712585
9 0.208863235546968
10 0.194394668726284
11 0.21579635495133
12 0.292767953840979
13 0.382697855019897
14 0.249708427269947
15 0.171824658307464
16 0.103730703447196
17 0.0530084989384645
18 -0.0795072521833138
19 -0.191793312526725
20 -0.165197616827131
21 -0.213817476751009
22 -0.281187497656286
23 -0.425991698012566
24 -0.461827206544159
25 -0.525339852576932
26 -0.5667988117222
27 -0.563798954105861
28 -0.626441320412606
29 -0.673641956397908
30 -0.734004450635311
31 -0.822290882587508
32 -0.925023059965055
33 -1.0225655346347
34 -1.11556691898161
35 -1.28551870808794
36 -1.40672842961498
37 -1.58468556212912
38 -1.71399373807491
39 -1.79886811013585
40 -1.9840761249043
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.086771739219806
1 0.163716631059212
2 0.256111305934044
3 0.182209738776248
4 0.043305814889786
5 -0.0916971783648863
6 -0.259679798328323
7 -0.277885371163987
8 -0.193594641953543
9 -0.127740902735787
10 -0.19530923761568
11 -0.0834145795722172
12 -0.0209524771034881
13 0.0325458323550691
14 -0.0978679940940244
15 -0.242753760639403
16 -0.288203739843322
17 -0.250433625482732
18 -0.361570298648685
19 -0.473791642369374
20 -0.614834814156168
21 -0.715973905711205
22 -0.783841933303935
23 -0.881523484491961
24 -0.865246914478315
25 -0.891466073095952
26 -0.922656789064485
27 -0.98051528033177
28 -1.04011596852397
29 -1.13788337813945
30 -1.25463508608564
31 -1.34957858873148
32 -1.44486509276863
33 -1.52292223161419
34 -1.6485181491571
35 -1.72644641154292
36 -1.80103715044773
37 -1.87708114742684
38 -1.95722015982556
39 -2.05964679299307
40 -2.13896832809532
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0705959138953824
1 0.0870282437394749
2 0.184998069945998
3 0.143624449014089
4 0.0818700115165298
5 -0.0458604746524105
6 -0.146196427703642
7 -0.133793994684739
8 -0.0543351644096672
9 0.0462841395092046
10 0.0261854313102576
11 0.10400293945349
12 0.16755441771297
13 0.301576889416086
14 0.228745635018011
15 0.194277384838165
16 0.199034599003019
17 0.21054630001963
18 0.193120727985586
19 0.153375463405125
20 0.15318401839781
21 0.0674151507562675
22 0.022961565481316
23 -0.0862890273142267
24 -0.113078729329641
25 -0.153200666136275
26 -0.235147973372742
27 -0.168821105847361
28 -0.217424736624642
29 -0.202084571824591
30 -0.186837067167471
31 -0.235502158736515
32 -0.240953517280234
33 -0.272576425110475
34 -0.292287599735972
35 -0.343212592877167
36 -0.371298589024466
37 -0.432517853758794
38 -0.4663875676088
39 -0.465432745065966
40 -0.519657633664078
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0555434565123609
1 0.172586527586095
2 0.317742104035459
3 0.269278745849539
4 0.214014120750592
5 0.15353195881144
6 0.0674732265433211
7 0.148285027324626
8 0.255766586131648
9 0.363499783291778
10 0.347735570211139
11 0.392372246238977
12 0.504624683944225
13 0.620276269344411
14 0.572685908010622
15 0.468947909296584
16 0.386143290161197
17 0.377305270795179
18 0.335496763968511
19 0.341959359618439
20 0.450700174860408
21 0.508436620538757
22 0.570597765444217
23 0.557453295694896
24 0.621568388436086
25 0.630262795056866
26 0.604209135984045
27 0.679813210083721
28 0.588158083463838
29 0.586949122863554
30 0.544229999148352
31 0.519554798063152
32 0.49222647987531
33 0.363010698798532
34 0.256630630872564
35 0.206228955254725
36 0.0977206123600465
37 0.0090921754939699
38 -0.0254744989795852
39 -0.0806622702225162
40 -0.109072821121348
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.105555625050499
1 0.157219779688831
2 0.24399312752562
3 0.182991097920904
4 0.11583671297722
5 0.0749955822506752
6 -0.0222518941449699
7 0.0305251342612869
8 0.0909366027573308
9 0.143867249807094
10 0.101948578917101
11 0.179142146038569
12 0.245538176711555
13 0.392619489197913
14 0.29327118391057
15 0.252602559193023
16 0.270446975296793
17 0.29071369463307
18 0.309498536416867
19 0.331810609740608
20 0.291056527398737
21 0.268352945445163
22 0.245143656022893
23 0.218485995220645
24 0.289572743419429
25 0.371850807815008
26 0.324528259919756
27 0.345690950714285
28 0.350826694420286
29 0.286356750130381
30 0.238331314434123
31 0.245393558536995
32 0.187378898058302
33 0.0924901652454388
34 0.114819453947128
35 0.0356152881641805
36 0.0199035965761492
37 0.0246876262510325
38 0.04591866413837
39 0.084540182373487
40 0.0586909742221522
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0814847051548786
1 0.140731135963391
2 0.273819543864301
3 0.183442913206804
4 0.0912646420777694
5 -0.0221489920765587
6 -0.143395867251536
7 -0.0707768535246234
8 0.063396254888568
9 0.205419888583638
10 0.226115026239404
11 0.26619997792629
12 0.350910959015823
13 0.461324136484145
14 0.36613080830378
15 0.254934255903469
16 0.284373443253203
17 0.262606740688091
18 0.22256093972956
19 0.160497055785326
20 0.192245588552355
21 0.19590915653438
22 0.227924807629313
23 0.145030964499546
24 0.204398650109604
25 0.232775668760199
26 0.21584459637595
27 0.257845036950254
28 0.218368054655118
29 0.108100522259698
30 0.0111837851050987
31 -0.0149657239228174
32 -0.0633068534511363
33 -0.113072058277752
34 -0.189638063702329
35 -0.241940856442604
36 -0.334799724638121
37 -0.486613909646656
38 -0.593564720699377
39 -0.69092740591491
40 -0.761064982423857
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0843063606670222
1 0.143074510331589
2 0.239520112972122
3 0.176490586298233
4 0.149547825480471
5 0.120671895593319
6 -0.0132400606139753
7 0.0372562856054772
8 0.138140958103336
9 0.241541775465045
10 0.21391754994391
11 0.325527182812763
12 0.391001166727651
13 0.423210725854761
14 0.406687717290763
15 0.314124367847519
16 0.372909110149089
17 0.358012877095041
18 0.228483493427468
19 0.172592737377864
20 0.206969287561719
21 0.144151895658997
22 0.219830960515337
23 0.185700782257294
24 0.305885319767851
25 0.420018718523113
26 0.374342514212177
27 0.427337570851584
28 0.387560259157146
29 0.329630619778801
30 0.263553436406485
31 0.204572306900628
32 0.163114067898631
33 0.0618728554835819
34 -0.00998592563473855
35 -0.118457607878282
36 -0.212538051111306
37 -0.37050999418413
38 -0.551113878481001
39 -0.707326128144484
40 -0.896335181503413
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.112678862250304
1 0.200910662521478
2 0.317845972753462
3 0.30318197292294
4 0.258369590069463
5 0.162249151081777
6 0.0579914788508051
7 0.105213254188238
8 0.153703802272862
9 0.246786098849188
10 0.260649235208239
11 0.286723526001482
12 0.340203066990004
13 0.416656855059257
14 0.381392707936838
15 0.304052039779486
16 0.267955843401203
17 0.258226090542961
18 0.240568492891927
19 0.190425932145615
20 0.188180202535729
21 0.149827204158081
22 0.198405770752164
23 0.177505110035016
24 0.19045611297246
25 0.147006903138577
26 0.111672435478686
27 0.154792712082429
28 0.0281154288817644
29 -0.0560373088682105
30 -0.100914727781138
31 -0.12199191324799
32 -0.119371078487098
33 -0.17821380052733
34 -0.15589864918843
35 -0.162485640693913
36 -0.190790042132883
37 -0.192009424612508
38 -0.163722982517791
39 -0.12328693863337
40 -0.0349757651730518
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0673104751997329
1 0.104334096181004
2 0.15557931926457
3 0.19549799622715
4 0.180611190999118
5 0.167493696444518
6 0.0863782726782496
7 0.141648621590036
8 0.13514443510662
9 0.146388609172045
10 0.166554347796633
11 0.25313023376162
12 0.299615014903357
13 0.338634860174177
14 0.289747203835118
15 0.207163321382494
16 0.20122510880987
17 0.181291036316913
18 0.182515570594983
19 0.146361829843047
20 0.13954406495366
21 0.136627753163747
22 0.141675872310959
23 0.0688876672938381
24 0.0542356978943879
25 0.0136697209715915
26 -0.0455556237575681
27 -0.0781858523193342
28 -0.2252478576854
29 -0.316491256952381
30 -0.437685568762794
31 -0.515923499447043
32 -0.63486372256828
33 -0.716370870464067
34 -0.754986808474719
35 -0.827607667914141
36 -0.89609426927811
37 -0.981012948843948
38 -1.08655384303548
39 -1.18745308324742
40 -1.24947317274942
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.124233929301444
1 0.229464955934264
2 0.368602532152134
3 0.316075595893532
4 0.242580669510589
5 0.162847400081735
6 0.0285302989207552
7 0.0490882292832659
8 0.152105790222711
9 0.27215254188128
10 0.22529242748828
11 0.370293729740624
12 0.4429686000841
13 0.455242560320749
14 0.436521766080273
15 0.364763273414448
16 0.316713048772209
17 0.323401586620011
18 0.295091334626703
19 0.253692623156842
20 0.175113438964363
21 0.0905058308356521
22 -0.0275950675622121
23 -0.206409909763634
24 -0.184485788395108
25 -0.246602295421259
26 -0.346459340908017
27 -0.361979356961502
28 -0.427540602872804
29 -0.454726774063525
30 -0.475760320416411
31 -0.507744179495692
32 -0.598282039391344
33 -0.736908455171435
34 -0.73529103420702
35 -0.769937634543735
36 -0.827500384202019
37 -0.897043957223311
38 -0.954929850190373
39 -0.999169566487415
40 -1.09044053342514
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0895069419788372
1 0.188775051837202
2 0.264438475696134
3 0.248856604296803
4 0.183385379904172
5 0.0838943754416399
6 -0.0351523935003537
7 0.05828814709652
8 0.123743432092319
9 0.258058421343099
10 0.221089335006415
11 0.339828530764002
12 0.468998154709266
13 0.59339268209791
14 0.540488084333318
15 0.507865203818189
16 0.487406546752239
17 0.502625796379694
18 0.469730128008032
19 0.403489929808888
20 0.33331236735354
21 0.244261862446323
22 0.165800916476932
23 0.119611588766576
24 0.19120227074879
25 0.246028644598077
26 0.277557005693446
27 0.292542721458908
28 0.167366783613612
29 0.096459099299274
30 0.0590984518427415
31 0.0290817779626096
32 0.0601791222612138
33 0.0954289561216037
34 0.0646187246953764
35 0.070739501432425
36 0.067507328414417
37 0.00889684942761226
38 0.012807261550571
39 0.00887780188079912
40 0.0363444932580714
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0876642046043483
1 0.225851785578684
2 0.256243632346756
3 0.21101932482145
4 0.0898936385741966
5 -0.0784634066652696
6 -0.290031318545296
7 -0.219323587181105
8 -0.0513107557128385
9 0.0860615615441507
10 0.0459300391235864
11 0.0836747701796825
12 0.177797910310497
13 0.270573843331721
14 0.286643258107302
15 0.347790885158302
16 0.329168048788674
17 0.275279392075925
18 0.170642018240959
19 0.114146107878219
20 0.016867093460724
21 -0.0407365924837069
22 -0.158986403527651
23 -0.313271993840188
24 -0.412824362380889
25 -0.528236550572766
26 -0.615490435070189
27 -0.65868935992315
28 -0.738443808027065
29 -0.699727496320697
30 -0.693065113654046
31 -0.628556891814734
32 -0.582435466200264
33 -0.550638767933728
34 -0.575295909695333
35 -0.557322322927971
36 -0.472851206359442
37 -0.436438932858724
38 -0.426646304294574
39 -0.463989166737931
40 -0.509783895311683
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0687970092074361
1 0.105162102762519
2 0.145125815007081
3 0.154845621923969
4 0.116434086282248
5 0.0195946300314329
6 -0.131592005316909
7 -0.0609466545624815
8 -0.0155218946212665
9 0.0457109451965065
10 0.0299279062006343
11 0.0743752110071347
12 0.0461806288514546
13 0.0433737800626086
14 0.0595068347174714
15 0.0841194188889212
16 0.124509049223128
17 0.217894913110116
18 0.111256355865327
19 0.0177920380615539
20 -0.0545343962973934
21 -0.159512850641862
22 -0.164358261732805
23 -0.207744352770703
24 -0.205057980205936
25 -0.173632729371279
26 -0.129088614602567
27 -0.0907594488879551
28 -0.158184460730884
29 -0.273766542069787
30 -0.413610189934666
31 -0.478321164739777
32 -0.619902507444416
33 -0.847133264063616
34 -0.878239056417622
35 -0.955001094336858
36 -1.07611690552021
37 -1.1954843295151
38 -1.30811642627271
39 -1.37137999623191
40 -1.48135079723699
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0726191560976148
1 0.283789156185145
2 0.461871183396643
3 0.406805074622817
4 0.316509655335391
5 0.247482561171256
6 0.170507803680898
7 0.293420522419615
8 0.434245662736467
9 0.530455177191128
10 0.52550450074156
11 0.580746218120017
12 0.669319098879619
13 0.799219902550808
14 0.815049748987165
15 0.764179533203396
16 0.770398283957633
17 0.757136749965333
18 0.677686700831308
19 0.587350624187475
20 0.492712940036542
21 0.393921210801994
22 0.400150453701416
23 0.386682584343077
24 0.414635177653204
25 0.422086218202861
26 0.35633862298504
27 0.4285207629244
28 0.359388766711593
29 0.372013680791662
30 0.302552248201458
31 0.337826897883203
32 0.3653032250136
33 0.306669132826832
34 0.425242254142622
35 0.436078558053532
36 0.463821404847734
37 0.470508205536313
38 0.465379447272537
39 0.491855915525247
40 0.51598340310534
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0707119178995135
1 0.13301891379254
2 0.167441783304385
3 0.215892089977844
4 0.242093775356892
5 0.21289440511533
6 0.154392157929883
7 0.190497595584298
8 0.325667136834292
9 0.45307928216961
10 0.548503921766262
11 0.626257237637498
12 0.692945268624373
13 0.771136182181375
14 0.763911984171664
15 0.759733264561811
16 0.744581045383751
17 0.792974843043023
18 0.707946937862591
19 0.647987396182157
20 0.689708031211338
21 0.733478301669492
22 0.750796533598153
23 0.776197625806283
24 0.748777084000862
25 0.782498205271058
26 0.765297089468289
27 0.699500714795917
28 0.714333615948477
29 0.693173556995831
30 0.628655714971403
31 0.608933663600516
32 0.518176705309832
33 0.527209480120932
34 0.40645070206244
35 0.329523998372909
36 0.273041526963517
37 0.216257727697568
38 0.163460101331065
39 0.145116036024944
40 0.192611031991677
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0985760145520498
1 0.253210102307473
2 0.324990143227165
3 0.366766767776645
4 0.321665609950065
5 0.198942981577759
6 0.0380521188020291
7 0.111894742907839
8 0.23839430634925
9 0.344325941327341
10 0.346057542537187
11 0.403957449144833
12 0.536909861964037
13 0.699686647876673
14 0.640682559147824
15 0.608651398100916
16 0.654350763891749
17 0.700187931100903
18 0.64410177031816
19 0.543313971330798
20 0.486869916713738
21 0.384224852852868
22 0.274468455271031
23 0.22258755822845
24 0.224583426353522
25 0.255550855350349
26 0.287899458958544
27 0.387271721005542
28 0.355962426889959
29 0.360068239086529
30 0.362883330993449
31 0.335977390624753
32 0.264381257904736
33 0.217563595723202
34 0.240578905171444
35 0.215986437343251
36 0.189333535404901
37 0.208953033082855
38 0.242892570865142
39 0.296832572195614
40 0.340832278308155
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.125466579260818
1 0.162270961925941
2 0.236567798373978
3 0.220927398684275
4 0.144022330712337
5 0.0646371412522639
6 -0.0488783334699456
7 0.0127305600283005
8 0.0581602536643384
9 0.109750565493806
10 0.0467635786943199
11 0.147999541200666
12 0.237811334085865
13 0.287775286176949
14 0.257667135390623
15 0.197709754848936
16 0.146351498381957
17 0.137409754951964
18 0.0682518482080967
19 -0.0101509045994805
20 0.0534694416771306
21 -0.0191085039868382
22 -0.105137827456198
23 -0.276986706494589
24 -0.311163462009544
25 -0.452963339722245
26 -0.55792177084876
27 -0.526063721147029
28 -0.671980233924282
29 -0.746737468539891
30 -0.768198695774143
31 -0.709900704316695
32 -0.684386748754897
33 -0.626575568455664
34 -0.55315367913897
35 -0.487693395720436
36 -0.476221476124095
37 -0.440299722621966
38 -0.401009304319963
39 -0.418884204930057
40 -0.343470381754941
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.0767407431837586
1 0.144760618628763
2 0.213812569452136
3 0.182499789800225
4 0.0918980860855729
5 -0.0156476944493567
6 -0.143390975143261
7 -0.112549230109472
8 -0.0363109774657455
9 0.0462380251451089
10 0.00180174364278862
11 0.038688730273746
12 0.0471504599009065
13 0.0538344421173815
14 0.0143685696526106
15 -0.0307029815350957
16 -0.0120775146505263
17 0.037429042450642
18 0.0440587041554372
19 0.0637073845838541
20 0.0594667742543824
21 0.0179435064135758
22 -0.00713002197550994
23 -0.104613412807789
24 -0.128182947682607
25 -0.213034980236965
26 -0.304066937700085
27 -0.366787078505748
28 -0.505163272278088
29 -0.636070956657017
30 -0.77678447924259
31 -0.810291186042243
32 -0.879642666869428
33 -0.953947940246206
34 -1.0832329691817
35 -1.23348631502711
36 -1.37158352807904
37 -1.51014966319195
38 -1.59108021660304
39 -1.61661425766354
40 -1.76289495293726
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 0.100064102405172
1 0.0844514801446525
2 0.176638193853986
3 0.16802359966549
4 0.140620387899664
5 0.0749204953029614
6 -0.0377171847405249
7 -0.0151937539369831
8 0.0176250984727342
9 0.0660226053012654
10 0.0687744253723217
11 0.14059832650278
12 0.220304013210649
13 0.300563018986593
14 0.276615240918415
15 0.226494392244544
16 0.269496332667795
17 0.278372329850279
18 0.300771976455707
19 0.288223596831293
20 0.306296793777164
21 0.225251843156384
22 0.221558162566062
23 0.204258259719855
24 0.266699030095511
25 0.264158111258897
26 0.149877578430395
27 0.0935940397847417
28 0.00523135405058905
29 -0.0717602631944771
30 -0.156978592839243
31 -0.252275074601562
32 -0.259828952334225
33 -0.262929157094975
34 -0.242846745146491
35 -0.236577184769849
36 -0.260720443820594
37 -0.248668520735869
38 -0.298716785977409
39 -0.320551282135739
40 -0.402144914436664
};
\addplot [line width=.01pt, color0, mark=*, mark size=2, mark options={solid, draw=black}]
table {%
1 0.0245940881197116
2 0.226498901996681
3 0.35963173094045
4 0.323192876348203
5 0.111448288247637
6 -0.15695204006051
7 -0.325976982807179
8 -0.334640765706954
9 -0.209549890955135
10 -0.205884173772729
11 -0.395618742668341
12 -0.404592842072073
13 -0.230511879468287
14 -0.055279679833161
15 -0.0210029805809502
16 -0.0164575411401979
17 -0.0161737318314269
18 -0.00358054162625767
19 -0.0104086468728599
20 0.0127963401693988
21 -0.00256627163803121
22 0.00694011005459992
23 -0.0244461075742605
24 -0.0236365740759628
25 -0.0484458903598396
26 -0.0156604557703324
27 0.0128490171223125
28 0.0437716443655508
29 0.03698016897091
30 0.0120928241581541
31 0.0180395493500055
32 -0.00624743566737794
33 -0.00866452893233261
34 -0.00937398036588012
35 -0.00916348210569427
36 -0.0019314931161561
37 -0.00552501045437327
38 -0.0230162558437155
39 0.0125317378882848
40 0.0372569376930346
};
\end{groupplot}

\begin{groupplot}[group style={group size=1 by 3}]
\nextgroupplot[
xshift=-8,
xmin=-1.95, xmax=40.95,
%ymin=-6.67801912353941, ymax=25.9865734086558,
ymin=-3.0, ymax=12.0,
width=\figurewidth,
height=\figureheight,
axis y line=right,
tick align=outside,
xtick pos=left,
ytick pos=right,
xtick={},
xticklabels={},
yticklabels={},
x grid style={lightgray!92.026143790849673!black},
y grid style={lightgray!92.026143790849673!black}
]
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0375830523940754
1 -0.175452906471659
2 -0.399722803486828
3 -0.411062512947472
4 -0.482156596174985
5 -0.442109850745522
6 -0.460628854337077
7 -0.776507021145477
8 -1.17108793304054
9 -1.62846790691629
10 -1.72413592206594
11 -1.7317450796912
12 -1.69731683921897
13 -1.34814552804864
14 -0.919401762035825
15 -0.34524486430088
16 0.588781754937982
17 1.67274709313093
18 2.79702065706981
19 4.11247832110552
20 5.33559494035729
21 6.63845885839307
22 7.80770365512498
23 9.0170480945251
24 10.0751340283893
25 11.1198673897336
26 12.1590174050187
27 13.1951966302943
28 14.0650033251572
29 14.7684038510633
30 15.4930769850247
31 16.017458965133
32 16.5153898949857
33 17.0256843246427
34 17.4286996331545
35 17.8516173865179
36 18.2833775941932
37 18.562660256967
38 18.9074980878948
39 19.0094118927974
40 19.0372841436363
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0406611765441744
1 -0.150574600773195
2 -0.278049044506838
3 -0.393812430861038
4 -0.40848185184922
5 -0.429342365251118
6 -0.514092276525598
7 -0.83911244918382
8 -1.31175017301868
9 -1.77190054094758
10 -1.88180422316886
11 -1.85495497340151
12 -1.6898239315395
13 -1.27963649514673
14 -0.886692335770115
15 -0.318285866727577
16 0.367937080361454
17 1.15786608661944
18 2.10710568393784
19 3.16535740735039
20 4.28999364762905
21 5.44453891635575
22 6.45851267182095
23 7.51770703343136
24 8.65130044790427
25 9.63749230550675
26 10.5000153597152
27 11.3547961575409
28 12.2108575241747
29 12.94886084566
30 13.7473611913679
31 14.2820658402386
32 14.7526651419057
33 15.4037673322965
34 15.7849945171316
35 16.2095236262303
36 16.6270301238617
37 16.7830074505321
38 16.9474765927768
39 17.1220514540454
40 17.300729143924
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0312726703595358
1 -0.222495662278114
2 -0.518105175732691
3 -0.526624100386198
4 -0.534557341326102
5 -0.442374434721371
6 -0.329072509531479
7 -0.578916207605503
8 -0.995076822596552
9 -1.25831905651212
10 -1.29070715401157
11 -1.14349747872316
12 -1.18091549487696
13 -0.982761541098639
14 -0.640664594624329
15 -0.206671298838031
16 0.662223989860503
17 1.7457782082199
18 2.9228747629415
19 4.03442677783698
20 5.20067912806371
21 6.28302590615897
22 7.35863437710808
23 8.35540126201555
24 9.36430420818706
25 10.2691321055089
26 11.1845981481551
27 12.2607481843715
28 13.2023746686815
29 14.1830646999451
30 15.0787437945406
31 16.0094171003664
32 16.8677808833943
33 17.6097913282845
34 18.3936928433484
35 19.0621504883679
36 19.6242915883488
37 20.1388206050235
38 20.688443557838
39 21.1911825091496
40 21.696710314512
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0689589502052925
1 -0.0331450134432689
2 -0.318883792824807
3 -0.417914453563441
4 -0.418712898798907
5 -0.383520673138256
6 -0.389958401371132
7 -0.746423685934953
8 -1.20885194430937
9 -1.63569566703089
10 -2.0362468046705
11 -2.07769370158893
12 -1.91757102403899
13 -1.51873461916641
14 -0.993115408246222
15 -0.452759730708085
16 0.546060857189845
17 1.65332584182116
18 2.76439772588405
19 3.78641426091535
20 4.86185361815146
21 5.96547509174808
22 6.93139563358937
23 7.84209518673198
24 8.81641053902057
25 9.77462567932596
26 10.8795532716006
27 11.8805907468234
28 12.959487177558
29 13.91173609346
30 14.7866349554405
31 15.223053169101
32 15.7104773716241
33 16.3305514078953
34 16.6705541911824
35 17.1252810308159
36 17.4672355289347
37 17.7319541212621
38 17.9989602335401
39 18.2949432621178
40 18.4081614530012
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0276054123469898
1 -0.196096062572249
2 -0.529432391311538
3 -0.757337135843913
4 -0.842518811740518
5 -0.904464337486956
6 -0.966310806264943
7 -1.18202430663277
8 -1.42123339856163
9 -1.55273733445132
10 -1.4666188572818
11 -1.21423712253228
12 -0.744914831603636
13 -0.0621116166067512
14 0.416764431045307
15 0.975660188505088
16 1.92439808487194
17 3.0481967180935
18 4.28020889938334
19 5.49422962368031
20 6.61813272784746
21 7.77062329993665
22 8.73232845156528
23 9.67263557592409
24 10.7049851316376
25 11.8411963394634
26 12.8174856640043
27 13.9140814334868
28 14.8930851530954
29 15.9303275088986
30 16.7705265407216
31 17.3707615788981
32 18.0956452036599
33 18.767737751531
34 19.4530048979605
35 20.0365943899894
36 20.5379276378264
37 21.0043992589103
38 21.3566498686826
39 21.6849570478848
40 21.9444181286814
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 -0.049434077810143
1 -0.326846474661949
2 -0.636818409459095
3 -0.764334058667657
4 -0.79201660029066
5 -0.787533005529394
6 -0.79520044912467
7 -1.18118284494409
8 -1.60509741363083
9 -1.87930499402753
10 -1.95598291631981
11 -1.7292735580652
12 -1.44410160277853
13 -0.952164837550152
14 -0.334115110569546
15 0.235814411925613
16 1.04454994491852
17 2.13219410211544
18 3.001001687679
19 3.89907291687675
20 5.00869345005125
21 5.95086755187162
22 6.87326959504224
23 7.78759853580924
24 8.6236716624499
25 9.47507424729922
26 10.5620052498144
27 11.5819545336773
28 12.6256450300682
29 13.6918442290742
30 14.5950592633774
31 15.3580677607932
32 16.1349046220999
33 16.8131433009078
34 17.3328573119483
35 17.8253513576236
36 18.298806261005
37 18.7048590910003
38 19.0004109977753
39 19.2221065104383
40 19.4955554438329
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0243705290739653
1 -0.282230068623943
2 -0.551493573152379
3 -0.728212266076694
4 -0.854107554880195
5 -0.941372973819691
6 -0.991772839263484
7 -1.66629524504503
8 -2.26336818350671
9 -2.73211486672686
10 -3.11707517832082
11 -3.20850954003404
12 -3.15816517136476
13 -2.79737229950639
14 -2.39727831539149
15 -1.93915153427961
16 -1.07213094223038
17 -0.22228654515071
18 0.906767739663972
19 2.01852500702689
20 3.0681896961791
21 4.10238742144884
22 5.15080932391131
23 6.06734516740255
24 6.83768417497463
25 7.6724270051394
26 8.54761264964146
27 9.25538948555539
28 10.0846827737708
29 10.9121659543919
30 11.6974898001889
31 12.4275469425585
32 13.2088478940227
33 14.0347148132535
34 14.7500790359057
35 15.5202144682778
36 16.351483959869
37 17.0727619125968
38 17.8262778405212
39 18.5510697085526
40 19.2644727153468
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0939996309736499
1 -0.262102852496075
2 -0.493324980222476
3 -0.514071758370588
4 -0.395507773488273
5 -0.302952637004976
6 -0.295974748790917
7 -0.726082453458372
8 -1.22895563134453
9 -1.7240285703123
10 -1.90110466345791
11 -1.88178347735376
12 -1.77766067018251
13 -1.31175750889199
14 -0.524330544738127
15 0.378994684545911
16 1.19694360262529
17 2.20922737486663
18 3.37851498963478
19 4.55321821994124
20 5.91871727243925
21 7.04525317017023
22 8.19632472194705
23 9.18385951755748
24 10.2628351468859
25 11.4299891052309
26 12.5634360363333
27 13.5186040481204
28 14.6426042788476
29 15.6730113723079
30 16.6108954842793
31 17.4666139749356
32 18.2869754495774
33 19.039581585012
34 19.7157642279462
35 20.3767627599287
36 21.1864023559995
37 21.8569271056383
38 22.4648723865568
39 23.0244813452867
40 23.600792174211
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 -0.000159330626015031
1 -0.268930873094111
2 -0.479489418630632
3 -0.585661426888656
4 -0.611389597112346
5 -0.606844815663221
6 -0.617671709495672
7 -0.844437377258333
8 -1.19896784709046
9 -1.46304352762302
10 -1.60800270667418
11 -1.48808915572218
12 -1.40962811710869
13 -1.19675938487135
14 -0.92921771642487
15 -0.520625515876479
16 0.44689183275787
17 1.64924370850035
18 2.84078967378724
19 3.85478135321495
20 5.08696692552069
21 6.19008973816324
22 7.23206684825279
23 8.24309231110193
24 9.21110150647267
25 10.2519082607739
26 11.2691770602657
27 12.1942303292046
28 13.1658601711518
29 14.1919844890902
30 15.1868157621206
31 16.0984486776786
32 16.9133978584985
33 17.5379006582049
34 18.0864416918056
35 18.5918033836846
36 19.07325335224
37 19.4308738422914
38 19.9169118147301
39 20.3719906328266
40 20.9476816772026
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.00710671174339961
1 -0.0903661091586687
2 -0.223811624554009
3 -0.323475227785596
4 -0.250545911316681
5 -0.161304117054315
6 -0.0627258555815118
7 -0.250530620522864
8 -0.755123264744239
9 -1.39413076092291
10 -1.71584662174541
11 -1.83479878236144
12 -1.7027504157412
13 -1.15291524081566
14 -1.06207532004315
15 -0.756440657603914
16 0.109351708207416
17 1.2051467441475
18 2.32862944873853
19 3.34604670259268
20 4.51206163217208
21 5.68560387735622
22 6.76433851780256
23 7.75154902342017
24 8.64334961224821
25 9.56601334219291
26 10.3658721539084
27 11.2776023292032
28 12.2753412426221
29 13.2246890372488
30 14.0755037273019
31 14.8505279267295
32 15.502922870715
33 16.2017265567484
34 16.7420748743006
35 17.2153435223251
36 17.7071937710228
37 18.2536770344582
38 18.6859255447227
39 19.0344224501405
40 19.4903138424644
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0714195401009379
1 -0.136380256950501
2 -0.514575508703832
3 -0.672842157380731
4 -0.698058279907412
5 -0.739743264024996
6 -0.664480090708336
7 -0.89634061063207
8 -1.29128342333494
9 -1.73184458262137
10 -1.82785715101914
11 -1.76596214791224
12 -1.67430251896974
13 -1.37377116479584
14 -0.654069461428845
15 0.0873196150709155
16 1.00082726223102
17 2.10373136901498
18 3.01919701662411
19 4.04126933428933
20 5.05610701720852
21 6.07090239941053
22 6.96933253207202
23 7.85500971566815
24 8.67242518301345
25 9.48736866332506
26 10.3246535748613
27 11.2904246148196
28 12.1600867706058
29 13.2573402204899
30 14.3054363809053
31 15.0923592804654
32 15.8613066666995
33 16.519690987508
34 17.1538437659268
35 17.6990779985117
36 18.2407540670941
37 18.6166453065221
38 18.9004607107992
39 19.1109585456887
40 19.3832493147098
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 -0.0358541482269388
1 -0.194961787551114
2 -0.396622667467286
3 -0.519821690378991
4 -0.490816027237538
5 -0.428453631993781
6 -0.484679724566998
7 -0.545044788931655
8 -0.856565745188393
9 -1.29707870629749
10 -1.68233470387797
11 -1.53055592325141
12 -1.45187182507084
13 -1.25778560025566
14 -0.943172463199839
15 -0.466063618415957
16 0.357533118110893
17 1.4555270188407
18 2.46741690083531
19 3.52128556403732
20 4.80354974753308
21 5.9167864312633
22 7.00212610418884
23 7.97657852853624
24 8.96096524632916
25 9.90488853659865
26 10.92724274849
27 11.9120177273771
28 12.9616019087198
29 13.9097448005138
30 14.891770204754
31 15.7628374222957
32 16.6379300527796
33 17.4012605629288
34 18.0928348163966
35 18.7662620825258
36 19.3340058434854
37 20.0121500520322
38 20.6819364757495
39 21.2607093333409
40 21.8241754115404
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0493790989757734
1 -0.250151488238382
2 -0.461715683937456
3 -0.61985858447932
4 -0.845990360969397
5 -0.908523724471941
6 -1.02367517906145
7 -1.41667992761411
8 -1.87110859397741
9 -2.2124292869906
10 -2.38339754035218
11 -2.2418597275022
12 -2.06905350004424
13 -1.64655874592227
14 -1.39718199548683
15 -0.96415350693197
16 -0.0529867944845859
17 1.10297910834725
18 2.20844241298453
19 3.32680416725981
20 4.64069410239438
21 5.72561307823161
22 6.89155560698888
23 8.02736584509614
24 9.02515228340684
25 10.046039817769
26 11.087296900764
27 12.0723845864893
28 13.1595243252151
29 14.2491949625806
30 15.3423724043208
31 16.1245253475974
32 17.0539629736686
33 18.0362576990541
34 18.7702908204169
35 19.5456198863658
36 20.2555147133478
37 20.9149052133499
38 21.459655812348
39 22.0105800091735
40 22.5531311060986
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0491728779888754
1 -0.0809214340152664
2 -0.242516640774141
3 -0.186941134972805
4 -0.026984759718367
5 0.0972440082187607
6 0.205277649297187
7 0.17505344802088
8 -0.155862320071751
9 -0.368327026987166
10 -0.370642146828486
11 -0.328784597510273
12 -0.0838277063247421
13 0.447692712560053
14 1.02043911942021
15 1.78256615110315
16 2.74958707186071
17 3.89574261398494
18 5.05005432942247
19 6.18091325413658
20 7.32247283654567
21 8.3182427347567
22 9.36639151056744
23 10.3647629141262
24 11.3010073809563
25 12.2727669169856
26 13.2759037331152
27 14.1317270514674
28 15.0636097570145
29 15.9016352510609
30 16.648178472053
31 17.4638132849323
32 18.0850685992695
33 18.8106383763909
34 19.4316045118088
35 20.1441697519514
36 20.7506552951638
37 21.3609312866911
38 21.8964692428251
39 22.4647557134214
40 22.9832358339791
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 -0.0230622970909993
1 -0.193200928461716
2 -0.325703464442865
3 -0.334499962085129
4 -0.203537129675467
5 -0.116786267973452
6 0.0441084413538375
7 -0.146515874164433
8 -0.671720788944062
9 -1.2188224403641
10 -1.53869108490036
11 -1.77789852300662
12 -1.87051284071363
13 -1.64784638164171
14 -1.30434138541474
15 -0.849538224085029
16 0.014977602601995
17 0.954809991453617
18 2.06702268584321
19 3.16508450456816
20 4.33274605868518
21 5.56870677325457
22 6.65265832442627
23 7.7511301295288
24 8.60747645736716
25 9.45885959121888
26 10.300338122545
27 11.3407363520892
28 12.1883092324117
29 13.0360263098347
30 13.8936000659855
31 14.670383572641
32 15.5305352930544
33 16.3407585408666
34 17.0666567941873
35 17.7147791852825
36 18.2601420338225
37 18.6737786508623
38 18.9790525656241
39 19.3088295146554
40 19.6043337590541
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0120936221558567
1 -0.217314653213718
2 -0.446207699750051
3 -0.520416592438468
4 -0.52825146156834
5 -0.464397244478699
6 -0.355746722373892
7 -0.694232388231173
8 -1.27410372156768
9 -1.76037423153887
10 -1.81407934957585
11 -1.8204719930239
12 -1.73964408268751
13 -1.34419001339081
14 -0.810236487194031
15 -0.184988933056642
16 0.915936600851082
17 2.04000954289637
18 3.11082551497852
19 4.26487706270735
20 5.34378970749234
21 6.32757423099068
22 7.32641480649838
23 8.37584841035121
24 9.30010686515937
25 10.2994514869116
26 11.2827912951614
27 12.2897158902676
28 13.3494632439959
29 14.4313744835624
30 15.400640515109
31 16.1689282157072
32 16.8345595927313
33 17.6210372470148
34 18.1303473088642
35 18.6454560103732
36 19.1134270799981
37 19.5933798820155
38 20.0065310173879
39 20.3389397576463
40 20.6557343574462
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0527027364257795
1 -0.139375307987454
2 -0.331849956269669
3 -0.370242658647455
4 -0.426473791898102
5 -0.425910082680831
6 -0.290096108028787
7 -0.566868316096668
8 -0.940442235308874
9 -1.34918850489201
10 -1.31800186440057
11 -1.21206568061778
12 -0.998516939885202
13 -0.471676740772545
14 0.152591543548604
15 0.789228883238701
16 1.70444205655978
17 2.9044919295314
18 4.15337469113842
19 5.36398246633729
20 6.38786142607757
21 7.34128958553434
22 8.34815420226201
23 9.31777567958683
24 10.3344425931286
25 11.3379006778393
26 12.4024655580415
27 13.2407335962289
28 14.2298545068168
29 15.0626704898172
30 15.7278921185422
31 16.1593820234572
32 16.6413806219919
33 17.0802590861519
34 17.2718147901282
35 17.5184896310784
36 17.8099084562083
37 17.9507580384333
38 18.1286474329219
39 18.1900969560778
40 18.2102756363855
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 -0.0631531018046494
1 -0.421196263033543
2 -0.644076172630448
3 -0.716590079729845
4 -0.701267492785731
5 -0.63763699985605
6 -0.509640852401525
7 -0.794154327188959
8 -1.18271417156221
9 -1.56392376047337
10 -1.68055807947844
11 -1.40554611396496
12 -1.02315245553897
13 -0.378335088786856
14 0.259200054281228
15 0.9572758592536
16 1.80788674761141
17 2.8472966462248
18 3.85055716694585
19 4.87366757262599
20 5.75987913957172
21 6.54226973769229
22 7.37220154252464
23 8.22080113467635
24 9.071450689801
25 10.0408904764105
26 11.1282230508406
27 12.1816967438596
28 13.0799708864315
29 14.0519833997715
30 15.0438999978393
31 15.815038198215
32 16.5530345084716
33 17.1965300925936
34 17.7913093108497
35 18.2647808466852
36 18.7111275359581
37 19.1838646092161
38 19.5818012112846
39 20.039345255619
40 20.4157253760599
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0157414110690204
1 -0.129555139198524
2 -0.330790373483739
3 -0.402929561463492
4 -0.405406881733162
5 -0.470527729616701
6 -0.472997656385532
7 -0.653000082467762
8 -1.00552105796004
9 -1.27966521282781
10 -1.41719886727514
11 -1.42545136046323
12 -1.29914975921121
13 -0.979610569495028
14 -0.504869434232973
15 0.0844590126326423
16 1.01747056588193
17 2.21277576052146
18 3.50267554497545
19 4.74280282817296
20 5.94961912415336
21 7.18951581571951
22 8.31261467326562
23 9.3434838952527
24 10.2239562378921
25 11.163597910785
26 12.1395713789947
27 13.0597559959987
28 14.0516352240225
29 15.0870113109433
30 16.1645161600603
31 16.8207604619194
32 17.4956146162036
33 18.1037144550675
34 18.4859852165692
35 18.900587988194
36 19.378868145146
37 19.8199744125241
38 20.224143609431
39 20.4914025891131
40 20.8044632301901
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0202605556671851
1 -0.114416161904958
2 -0.227111662794135
3 -0.251282371141048
4 -0.242974555640252
5 -0.188859706954703
6 -0.161014538998431
7 -0.378778645284539
8 -0.893266489593892
9 -1.47573767074047
10 -1.73613785955168
11 -1.70570121438442
12 -1.49387432683679
13 -1.05256258338708
14 -0.797196990861252
15 -0.498048415514284
16 0.190527362814529
17 1.17965997929105
18 2.18818297294304
19 3.2773742153856
20 4.59282896983431
21 5.76866802997897
22 6.91806845657979
23 7.80661616974706
24 8.7531767037763
25 9.59240419251561
26 10.3790980946039
27 11.4332726041965
28 12.3011592982031
29 13.323154901463
30 14.2306112761022
31 15.0328409102088
32 15.8738618642764
33 16.7524671266428
34 17.4196826401842
35 17.9241340670587
36 18.514653519988
37 19.0076642514156
38 19.4534571661361
39 19.7900387851799
40 20.0659479806491
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 -0.0887544760061494
1 -0.326542473616375
2 -0.511671740758648
3 -0.534501708004449
4 -0.438604767952356
5 -0.234854407890544
6 -0.0399388895677948
7 -0.269060084370732
8 -0.790351823185433
9 -1.39713947326909
10 -1.77783399640991
11 -1.94179473287995
12 -2.08100931381856
13 -1.90032174364233
14 -1.61266258910862
15 -1.14073487613647
16 -0.35548234120845
17 0.545944371962888
18 1.57089114190306
19 2.72125179595683
20 3.95030125489913
21 4.9977751849709
22 6.09296611271706
23 7.02467628985406
24 7.90158460035716
25 8.82870434578289
26 9.71062292425951
27 10.5867938819069
28 11.5697069255283
29 12.4342656220354
30 13.2299166002418
31 13.9736027018213
32 14.7041980068282
33 15.4059099158255
34 15.9456698928255
35 16.6302479983487
36 17.3389776246286
37 17.9719888314021
38 18.6054283501952
39 19.1148318561082
40 19.7450942675317
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0250217856124926
1 -0.0656842576025651
2 -0.287649354475426
3 -0.235587332933472
4 0.019135444758636
5 0.241869996031232
6 0.437132103886247
7 0.253068177613189
8 -0.343403627173318
9 -1.07428761193811
10 -1.40417586203575
11 -1.60438221957871
12 -1.62320369126164
13 -1.42711799068343
14 -1.14508343153442
15 -0.57196704422799
16 0.299845421102516
17 1.60345116862736
18 2.87320796289567
19 4.10085047565603
20 5.45386369951752
21 6.54344520479335
22 7.67286090668685
23 8.68714618968853
24 9.62027488687546
25 10.5670962798658
26 11.524207069009
27 12.4719478786452
28 13.5230588491609
29 14.5030499671286
30 15.5817062774681
31 16.479186811277
32 17.4676240767158
33 18.3976986220973
34 18.9305782872016
35 19.5291853564579
36 20.1790452907243
37 20.6864590234759
38 21.2024839748742
39 21.7022134336062
40 22.2829110786901
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0279581161094642
1 -0.201992801390531
2 -0.528623529102459
3 -0.657594161793928
4 -0.755440621372836
5 -0.676290741529773
6 -0.529761524948495
7 -0.656729144504919
8 -0.939473418566602
9 -1.17097184101766
10 -1.07202479659989
11 -0.804833102805859
12 -0.442454860293736
13 0.307728876372852
14 0.867632277923464
15 1.44925472821204
16 2.31202736630658
17 3.44842014650087
18 4.48174857198944
19 5.68509612699392
20 6.76230497163007
21 7.89855180194118
22 8.83427061358043
23 9.70261314173344
24 10.6542584972451
25 11.6956951495896
26 12.7509003873142
27 13.6767277431137
28 14.7638676271182
29 15.7412227501311
30 16.6839432823754
31 17.4579618217167
32 18.2858812976751
33 19.004502073338
34 19.628455757469
35 20.1427229009252
36 20.5700335480126
37 20.9038587784788
38 21.3354306356472
39 21.7281769830276
40 22.0942888525713
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 -0.00526358516414804
1 -0.228861827001709
2 -0.428978188212826
3 -0.515736128122536
4 -0.504584695757255
5 -0.589712188445648
6 -0.64814977212629
7 -0.97702007808966
8 -1.40849810552773
9 -1.6719960978653
10 -1.68179458026971
11 -1.454260461461
12 -1.09203158833023
13 -0.436020973430971
14 0.26987484138986
15 0.971739050173655
16 1.90063729324239
17 2.97834683190905
18 4.03901947441272
19 5.13747771276083
20 6.25532034409814
21 7.24766616702773
22 8.16428403244978
23 9.17092882788094
24 10.1707458125976
25 11.1275761971175
26 12.1815962960114
27 13.3295898673913
28 14.315245955047
29 15.0287307327061
30 15.7055176512939
31 16.3646707732885
32 16.9656157063867
33 17.5282801683869
34 17.8445129250369
35 18.1389265934591
36 18.4137118352304
37 18.5800343607659
38 18.6589969080689
39 18.7938366376489
40 18.8419635083606
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.015259219603768
1 -0.234665990326819
2 -0.399811772608264
3 -0.447074745656639
4 -0.412651265279219
5 -0.335001825940041
6 -0.244562299925975
7 -0.537553263495772
8 -0.993384313926784
9 -1.62076524790879
10 -1.83804817569737
11 -1.93397109431876
12 -2.01307485559798
13 -1.75257497179016
14 -1.23507234897343
15 -0.546746904899301
16 0.436557120084647
17 1.5186976527443
18 2.683499218749
19 3.9197819819013
20 5.16799588186502
21 6.26243348827241
22 7.33734566346496
23 8.45166012224106
24 9.4777067045354
25 10.6063087281181
26 11.6468146961422
27 12.6266168664491
28 13.5744382328694
29 14.5568894374543
30 15.3903685294274
31 16.1653225343174
32 16.7828151705061
33 17.2828957761887
34 17.7841607406053
35 18.2192433782547
36 18.5892868238984
37 19.0616524635358
38 19.471118860361
39 19.9087096778802
40 20.2943869610089
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0241203230288356
1 -0.263231922051897
2 -0.53977042265478
3 -0.606084569106522
4 -0.579599625396167
5 -0.502410729219358
6 -0.388789524779374
7 -0.570315465581693
8 -1.1052357136189
9 -1.57127406208265
10 -1.82137221920596
11 -1.78466108651745
12 -1.78679019494257
13 -1.5257788308123
14 -1.2309149380149
15 -0.808916604569448
16 0.0113965229765904
17 1.0844339387928
18 2.26076319398309
19 3.46308300022261
20 4.83774566775428
21 5.93951069673567
22 6.98628682219621
23 7.87649824267292
24 8.81761586874062
25 9.64426976811849
26 10.3477932380307
27 11.3544835102475
28 12.3560885712416
29 13.3067714072722
30 14.2207626104616
31 14.9798007922345
32 15.7590037068718
33 16.5597374731929
34 17.016028527696
35 17.6426047329987
36 18.3430823787527
37 18.923390454707
38 19.4789357603605
39 19.8730934977149
40 20.1859842502251
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0476240594517336
1 -0.0328303129638039
2 -0.145554288266122
3 -0.131782299236757
4 -0.0874348739048192
5 -0.030681821725282
6 0.0176353016101709
7 -0.0953033375388017
8 -0.263412634154942
9 -0.384742644721492
10 -0.426660471208879
11 -0.184575414705388
12 0.232861636150866
13 0.777495812735528
14 1.18482691083509
15 1.81047064797793
16 2.66349866606696
17 3.80381397988081
18 4.966386296715
19 6.05682341253952
20 7.16221105153466
21 8.09886165388087
22 9.13944160364723
23 10.0106067008799
24 10.9885607890181
25 12.0108353031004
26 12.926037464988
27 13.8045748459137
28 14.693583130827
29 15.4780715904754
30 16.1413230346712
31 16.7162565206919
32 17.1838738765467
33 17.7084530873175
34 18.1102929455033
35 18.6498779676621
36 19.1357468538467
37 19.6029977442519
38 20.0099675786812
39 20.1769397290178
40 20.4015059415329
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0914260078022426
1 -0.144891409545678
2 -0.460842271248316
3 -0.580061592827469
4 -0.590137422426664
5 -0.504358606041022
6 -0.54378942107167
7 -1.00539501540832
8 -1.57612327461432
9 -1.93450207545069
10 -2.12345056858192
11 -2.12177351828976
12 -2.06992019833249
13 -1.68610898930124
14 -1.21259670636696
15 -0.539012684191305
16 0.375404774925058
17 1.39132070077132
18 2.34746316239086
19 3.33819488026207
20 4.49994834009117
21 5.69071198106386
22 6.81277265675804
23 7.73914529826733
24 8.7346062917854
25 9.63540036319691
26 10.5534752025182
27 11.5879959649771
28 12.6283472619526
29 13.665232933818
30 14.5883604981923
31 15.4740009856598
32 16.2869261809412
33 17.0762244090366
34 17.730271222316
35 18.3522419118255
36 18.980232654688
37 19.5326109566404
38 20.044881497866
39 20.5639672656964
40 20.9513282339368
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0213565003716276
1 -0.222408463786064
2 -0.30881410691963
3 -0.41097569984639
4 -0.387296732087206
5 -0.205060223757902
6 -0.103306234425486
7 -0.456185040531173
8 -1.06478087320454
9 -1.49727045908126
10 -1.8000762795645
11 -1.8633567673195
12 -1.9411696864878
13 -1.8243634023181
14 -1.63280012730075
15 -1.16060569362087
16 -0.477207843505231
17 0.297856412220828
18 1.28954550519072
19 2.22126982260509
20 3.21037522722364
21 4.12124460230737
22 4.96242698269256
23 5.74946909746978
24 6.61754440855537
25 7.45930220453456
26 8.17687748078226
27 9.03712631073411
28 9.66708801905055
29 10.311861947658
30 10.9402573553848
31 11.5864438254876
32 12.2778426254386
33 12.7663725204502
34 13.4488938731019
35 14.0184950479489
36 14.5446820107735
37 15.1532765922718
38 15.7290182991813
39 16.1922394542233
40 16.8311548190299
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 -0.00465635785169161
1 -0.189088763929349
2 -0.485083954043134
3 -0.536673993263014
4 -0.448844814480412
5 -0.35704216411227
6 -0.330456247627629
7 -0.532915960750687
8 -1.04613149987906
9 -1.63172389971966
10 -1.78816314570168
11 -1.7678220712054
12 -1.52161789820469
13 -1.07329779641202
14 -0.586934753910942
15 -0.0121370238701641
16 0.797522996309382
17 1.77454489710109
18 2.77970062699886
19 3.83395852441074
20 4.89035133698553
21 5.81132995587376
22 6.76910498281911
23 7.6329551111122
24 8.55463127445997
25 9.47316154342177
26 10.2726474462327
27 11.1544596851079
28 12.0833326897959
29 12.9301024554181
30 13.879644985819
31 14.6143596067544
32 15.5304950604802
33 16.4383458714007
34 17.0681746947138
35 17.747333044768
36 18.3397930629116
37 18.9554189290169
38 19.5063178489857
39 20.1582691190427
40 20.7201165425442
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 -0.0315324918323316
1 -0.303191361855547
2 -0.58340549345625
3 -0.682054398773043
4 -0.681839502135837
5 -0.606699316165599
6 -0.596802127504239
7 -0.90265891654102
8 -1.36058726370426
9 -1.72850780024939
10 -1.89201373805622
11 -1.92394277201117
12 -1.86068665999443
13 -1.56035237516495
14 -1.34619007138267
15 -1.00547867169215
16 -0.176392627615123
17 0.612169707462272
18 1.63618042467383
19 2.73264966227364
20 3.72980319852995
21 4.67898613235762
22 5.35402944688186
23 6.05444293892159
24 6.70872374414619
25 7.36278295607029
26 7.92528016448987
27 8.52894648312611
28 9.03953794891279
29 9.42617906444377
30 9.76266105645628
31 9.94323557261147
32 10.2033542852278
33 10.4372481694194
34 10.6169094987343
35 10.8682188485555
36 11.0907930910408
37 11.2252532524293
38 11.3603954854052
39 11.5532644432973
40 11.6470714014378
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0580141199612285
1 -0.0701542529462
2 -0.402548814396992
3 -0.496797417508719
4 -0.496798240655492
5 -0.426105431089009
6 -0.505634036053972
7 -0.920755020895768
8 -1.45581166586101
9 -1.97520895683307
10 -2.29733541695338
11 -2.12368053279241
12 -1.89412370940603
13 -1.25271409173029
14 -0.84157159571252
15 -0.229052680878521
16 0.724091191607422
17 1.86734743220364
18 2.9992758686405
19 4.15453649003828
20 5.40375370714153
21 6.66245286035922
22 7.67596186004353
23 8.63339919529529
24 9.48523712420101
25 10.3365324899072
26 11.2606650494006
27 12.2591349192603
28 13.3011544134279
29 14.2527637382671
30 15.0905676774375
31 15.7417588701775
32 16.2547224868227
33 16.7653019494717
34 16.9960154500661
35 17.2206413406532
36 17.5941103839341
37 17.7589228612979
38 17.9242805983533
39 17.8380221663694
40 17.7653361677297
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 -0.128739822637801
1 -0.283336565531089
2 -0.496146816022186
3 -0.549482141115084
4 -0.597361402603521
5 -0.622879653787956
6 -0.636428436255497
7 -0.744939442574007
8 -0.924965276127527
9 -1.22229889069792
10 -1.2489770611993
11 -1.10312112128989
12 -0.893692790805226
13 -0.462027623469235
14 -0.0903633930017635
15 0.36102669823105
16 1.29647004302607
17 2.30769534518595
18 3.39472545697082
19 4.39076545305444
20 5.39762442355729
21 6.28489876821504
22 7.2445653466627
23 8.24442873879665
24 9.21400393139416
25 10.1425404348869
26 11.0064941849252
27 11.9289785350487
28 12.971126808178
29 13.8372367428031
30 14.7130550319333
31 15.4507217546931
32 16.1788491916296
33 16.8838498262278
34 17.463743836351
35 17.8721971136146
36 18.2932331306924
37 18.6040983309752
38 18.8375500101607
39 19.0939194225715
40 19.2326203956401
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0553165732809524
1 -0.18961289483137
2 -0.460147284568636
3 -0.667052534776817
4 -0.76666827969776
5 -0.742790080221738
6 -0.715754127468593
7 -0.839223980886533
8 -1.10218527430966
9 -1.23490953104581
10 -1.21421076076782
11 -0.864358390725986
12 -0.497744028407748
13 0.0840584837058911
14 0.680025143455461
15 1.29205868472297
16 2.08619987515481
17 3.12409101414573
18 4.12811562072439
19 5.21577759832811
20 6.27288651211332
21 7.33007146586906
22 8.39727649690146
23 9.48793214837604
24 10.5575704062639
25 11.6303592994615
26 12.7142998123366
27 13.6262585295428
28 14.5590204421492
29 15.2795889240627
30 16.0045610926997
31 16.6523643426199
32 17.2145168762374
33 17.8392162453604
34 18.4538031504288
35 18.9372212783396
36 19.3373177327451
37 19.776516584192
38 20.2191608214786
39 20.599826614901
40 20.9649952476727
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0192893012937536
1 -0.155865118729972
2 -0.343520881042779
3 -0.293339536250651
4 -0.252418167819088
5 0.00197799744181282
6 0.13195134865492
7 -0.389861574263194
8 -1.07704572942164
9 -1.67694596190947
10 -2.12593982689642
11 -2.27787807505123
12 -2.43195371071609
13 -2.16676540800182
14 -1.84658782167297
15 -1.35984730671598
16 -0.51786092331301
17 0.502924090510893
18 1.55875662556795
19 2.78595497472766
20 3.92314793289978
21 5.17721995091093
22 6.27851710996911
23 7.27167111325841
24 8.13921662674606
25 8.93817794322979
26 9.74057844055366
27 10.5701975774771
28 11.6188183468992
29 12.6951401921796
30 13.703339423726
31 14.5624325569533
32 15.3731430513734
33 16.2387599542262
34 17.1061021999325
35 17.7799629073871
36 18.5649244526215
37 19.2834314076698
38 19.8938824657022
39 20.3308772210463
40 20.8412561996515
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0602687840388119
1 -0.0751302425352653
2 -0.225471757617862
3 -0.418156647817718
4 -0.527268000211989
5 -0.461533596985379
6 -0.48581541659142
7 -0.724316172676717
8 -1.14716098507428
9 -1.63478893782029
10 -1.95090102457775
11 -2.10659260728425
12 -2.16075142721024
13 -2.14961651951267
14 -1.96705957073974
15 -1.71138251000137
16 -0.904034335253529
17 -0.044708745742851
18 0.958058414737136
19 2.04232812834411
20 3.09697173976988
21 4.16166490371168
22 5.26399992862141
23 6.21347462194211
24 7.1191352277102
25 7.88014453282123
26 8.65685948781699
27 9.44085948300647
28 10.3305530010425
29 11.1858703062468
30 12.0993315034257
31 12.9319674408468
32 13.7048959033874
33 14.364151055721
34 14.8766682071315
35 15.371094772396
36 15.7810979803609
37 16.1602350888628
38 16.4501946908171
39 16.9243970047767
40 17.160912761123
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0930223488623727
1 -0.160524504147077
2 -0.280449985636871
3 -0.478004353457063
4 -0.443338828374608
5 -0.493629697397179
6 -0.541663459649047
7 -1.07305785686554
8 -1.75230995658888
9 -2.17896705196448
10 -2.25423224931524
11 -2.10699353272094
12 -2.02162345768457
13 -1.66068908920049
14 -0.988125000731702
15 -0.230005234080373
16 0.752615318873363
17 1.88570481374022
18 2.95454214337229
19 4.2301575356939
20 5.55036901947842
21 6.96980197577489
22 8.16071285924822
23 9.34902152671774
24 10.355987987369
25 11.4264459073982
26 12.4572866755229
27 13.4327862913771
28 14.5184315676386
29 15.4159926954785
30 16.3838488442222
31 17.1154170078402
32 17.68039494781
33 18.2060161901539
34 18.5755940024665
35 18.9630380112786
36 19.376351921341
37 19.7441772365268
38 20.0423325642466
39 20.318525355423
40 20.5330039376613
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.00813874570594741
1 -0.303746834148767
2 -0.530190623062652
3 -0.523297336895863
4 -0.559850601997184
5 -0.473892194083794
6 -0.448996343353951
7 -0.884128220646618
8 -1.52129452731322
9 -2.05844843621002
10 -2.33305130609961
11 -2.42812680691058
12 -2.34077517328023
13 -2.06982236863384
14 -1.68960228507295
15 -1.16250542042953
16 -0.264206321396433
17 0.855612121408833
18 1.89315962958569
19 2.83838538139073
20 3.80929163694302
21 4.70914782229031
22 5.60511514880573
23 6.38105552294886
24 7.11335395326266
25 7.89709867162278
26 8.69255744397685
27 9.46423210572653
28 10.2806427682782
29 11.0705272483015
30 11.7986118050262
31 12.7267033137157
32 13.5904007553102
33 14.4095493457715
34 15.3421900401425
35 16.152966236509
36 17.0229511156891
37 17.7954750855056
38 18.5199521372705
39 19.1239921271047
40 19.828891436231
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 -0.0656129565686201
1 -0.306939152432071
2 -0.488112472790134
3 -0.381754030036235
4 -0.262769538850545
5 -0.213988148029054
6 -0.159299297804047
7 -0.495196744236151
8 -0.932738969261543
9 -1.34494086729667
10 -1.40618189227783
11 -1.26426917243553
12 -1.14703960115177
13 -0.66501577966773
14 -0.339714608979328
15 0.148244986066066
16 1.03247173625455
17 2.04442799248215
18 2.95401896540646
19 4.02914255161121
20 5.22059876386504
21 6.22983609523936
22 7.26412447825629
23 8.20499694086751
24 9.10219693078136
25 10.0869213256756
26 11.1415299282275
27 12.0700233308084
28 12.9820945969481
29 13.925055374774
30 14.9041969347274
31 15.51432077794
32 16.2726501640945
33 16.9951804714688
34 17.6151842270162
35 18.1455168726257
36 18.7289785145882
37 19.1823760054006
38 19.5487952980827
39 19.904343442014
40 20.4012736172705
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.00479855972679388
1 -0.231329878986346
2 -0.305926782459203
3 -0.428119509072935
4 -0.480461824660885
5 -0.601429063675975
6 -0.663784561229791
7 -0.961473324040521
8 -1.55441548100677
9 -1.93719729886538
10 -2.19947594769285
11 -2.1055915621691
12 -1.97124435745373
13 -1.58925991005025
14 -1.24907954967687
15 -0.844305348005495
16 0.0796493343147846
17 0.99196027853208
18 1.96433843153803
19 2.91054050528309
20 3.92608502801089
21 5.00202519610595
22 5.99579032178304
23 7.00071790869356
24 7.95160797833522
25 9.06547113648007
26 10.0668331875387
27 11.1719432364363
28 12.0715706167368
29 13.1118706989516
30 13.9965614385749
31 14.8958911779456
32 15.6393406614745
33 16.4261892743117
34 17.0849868994661
35 17.6160404604191
36 17.9263745466346
37 18.1943257788322
38 18.4304266093745
39 18.6860182317247
40 18.8095868961017
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 -0.0495110484819312
1 -0.131289241417336
2 -0.370168025466877
3 -0.41080792640948
4 -0.342398020032407
5 -0.287983000779899
6 -0.345018175044554
7 -0.634971127803339
8 -0.923486006563853
9 -1.14591338150435
10 -1.11560382615613
11 -0.971901003267016
12 -0.691362351660788
13 -0.25007195020301
14 0.172516865302607
15 0.705021296043268
16 1.58501755215198
17 2.65000486528346
18 3.76408569335119
19 4.92009943558779
20 6.17635484674799
21 7.37539125801305
22 8.39966383770212
23 9.42265270058736
24 10.3640701345659
25 11.3730240642778
26 12.447259317585
27 13.3893837787083
28 14.6085310827818
29 15.5364656420196
30 16.3345694197994
31 17.1051182585816
32 17.9387034888782
33 18.6523410128729
34 19.206003468884
35 19.6469012330299
36 20.1170898500834
37 20.6065991012125
38 21.1043397292582
39 21.5361658144585
40 21.996663733346
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0202855904371879
1 -0.145029343986733
2 -0.379432194967363
3 -0.50342393311381
4 -0.498345421678844
5 -0.529901515879537
6 -0.557026709567852
7 -0.803476364311809
8 -1.28503615237708
9 -1.98789214357302
10 -2.36213622285609
11 -2.41193912061951
12 -2.17970812254558
13 -1.88628902135819
14 -1.46554788932207
15 -0.874901344826182
16 0.00464934914180493
17 0.893119336395241
18 1.99116336367085
19 3.07991173670876
20 4.25424316687346
21 5.37495678443933
22 6.48918079694397
23 7.44005017991332
24 8.49731807508708
25 9.39080101546165
26 10.1888501121907
27 11.1071348476621
28 11.9670669778183
29 12.9127314665585
30 13.7590640659693
31 14.3938852144288
32 15.1453879390143
33 15.8008632721162
34 16.3114374822487
35 16.8738359622894
36 17.3934135585921
37 17.8614567741134
38 18.2612177685306
39 18.6186016762566
40 18.9566801625463
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 -0.0894283286892392
1 -0.360335019864611
2 -0.617757396041396
3 -0.630960869980375
4 -0.499869308562717
5 -0.419268655703898
6 -0.482789140194744
7 -0.821421643613797
8 -1.38509693074632
9 -1.96923401850662
10 -2.31928204259727
11 -2.47024928542581
12 -2.58395426406574
13 -2.45081495037656
14 -2.28902325831964
15 -1.95025987575822
16 -1.19622210757069
17 -0.332554135276062
18 0.690819764360224
19 1.72918325872525
20 2.86408008822313
21 3.80056404918376
22 4.85489652151117
23 5.81973052743673
24 6.75589598327054
25 7.58511230490339
26 8.37377930511317
27 9.0717994743831
28 9.88735036436448
29 10.5837751118638
30 11.3790947731439
31 12.0667573707879
32 12.8277684888105
33 13.6505713558159
34 14.336721488997
35 15.04860118917
36 15.5967089124412
37 16.1298869897915
38 16.6001606145694
39 17.088323019777
40 17.4214367874107
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0487424052211307
1 -0.104325155429886
2 -0.403193880603526
3 -0.453566205389687
4 -0.464436352788505
5 -0.356723630052455
6 -0.301214498410292
7 -0.283668882190224
8 -0.576758311727494
9 -0.73822171196651
10 -0.710208509949814
11 -0.546807348748833
12 -0.148642047189877
13 0.416247032026654
14 0.899058960669431
15 1.52110248765269
16 2.39026284380685
17 3.52404572232729
18 4.80108770219772
19 5.91697850691771
20 6.96144866630153
21 7.99561275815813
22 9.00309901566132
23 9.99421336507252
24 11.1235383041507
25 12.270296426265
26 13.3379258363063
27 14.2923235560318
28 15.3077405088127
29 16.2564215462363
30 17.0789120500333
31 17.6036000435332
32 18.1763172963742
33 18.6165815391354
34 18.9978538809224
35 19.3727576074113
36 19.5795119408505
37 19.7613339341084
38 19.8690317079489
39 20.0454921934926
40 20.0268177567924
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0454475066613274
1 -0.301225804843841
2 -0.410654152877011
3 -0.447765129484256
4 -0.338613293476117
5 -0.295915349991712
6 -0.280805494678157
7 -0.72725567581659
8 -1.31163032131855
9 -1.94284154467465
10 -2.31285917104431
11 -2.57962852398606
12 -2.48941459390831
13 -2.37035263218987
14 -1.98916576418118
15 -1.41651732129811
16 -0.60592987225498
17 0.413785306850349
18 1.49934882174001
19 2.56648711696996
20 3.65812106903695
21 4.69542607351367
22 5.58386012047873
23 6.54175841673023
24 7.33615856148307
25 8.0503508210744
26 8.65802092136283
27 9.42115797101388
28 10.1477493433755
29 10.9223677429986
30 11.7815147624759
31 12.6204976139503
32 13.6121979848516
33 14.4598570024677
34 15.2953053064113
35 16.0597649114256
36 16.7788710820659
37 17.4221591147912
38 18.0058860679465
39 18.4864490758236
40 18.9784321876111
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 -0.000760461467796958
1 -0.167481649041651
2 -0.403292226987923
3 -0.509427807089644
4 -0.528038541960436
5 -0.550191879011518
6 -0.535507269823996
7 -0.881653814949813
8 -1.44173456252782
9 -1.94885750884144
10 -2.23932930886873
11 -2.40942105098041
12 -2.39928235726141
13 -2.12939346385512
14 -1.87265461583107
15 -1.48012258135276
16 -0.675355337314477
17 0.370881128902829
18 1.58623644599006
19 2.79424449828952
20 3.99183213972921
21 4.95499115682689
22 5.94350633641046
23 6.84918637481189
24 7.76515458462833
25 8.67651716766295
26 9.44687191601809
27 10.2592482175458
28 11.0220240040875
29 11.9945529679692
30 12.9290867233946
31 13.72306616655
32 14.566560013202
33 15.1882341201692
34 15.8882066819838
35 16.6055079131628
36 17.2998454988669
37 17.954178785153
38 18.5779538123136
39 19.1103019729465
40 19.6376482197134
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.127516852247471
1 -0.162598852196097
2 -0.365412966744494
3 -0.320903629615849
4 -0.243948463534341
5 -0.0897004088377771
6 0.133934790736558
7 -0.220303271743919
8 -0.766975708665418
9 -1.13146319590528
10 -1.24756922384772
11 -1.12811103680938
12 -0.924235525942005
13 -0.517957557513312
14 -0.190734751979937
15 0.382285144194894
16 1.48317787203743
17 2.88538827899582
18 4.20312979554812
19 5.49404213901081
20 6.8668717679834
21 8.01586577705127
22 9.2867095734418
23 10.5309640917862
24 11.5691892969939
25 12.6715764503304
26 13.7082817877645
27 14.6227313165816
28 15.4673509214846
29 16.3907871116566
30 17.2792317371302
31 18.0389900785311
32 18.6816448099076
33 19.393745015219
34 19.956466659893
35 20.5512920498228
36 21.092944207021
37 21.6589995769222
38 22.059715742296
39 22.4762300815609
40 22.7401713650245
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0334507716869878
1 -0.0680702932877519
2 -0.352012566942617
3 -0.37322033161295
4 -0.413144864810898
5 -0.366811939590928
6 -0.397438617563483
7 -0.571045146530322
8 -1.17705714406621
9 -1.90308443547479
10 -2.30884345331119
11 -2.61535463860451
12 -2.81641966558845
13 -2.72430713818027
14 -2.55568144242299
15 -2.36069945784903
16 -1.52110953152693
17 -0.439056120836841
18 0.565189762198717
19 1.52419315605432
20 2.66405359161856
21 3.64280918940435
22 4.53574558211654
23 5.2363581383864
24 5.99174956643816
25 6.74552384228553
26 7.29315979059353
27 8.02167298415536
28 8.5508557780999
29 9.06526474737609
30 9.57457706240783
31 10.2873656041115
32 10.9114517446256
33 11.5689009132578
34 12.5364036320113
35 13.5345530210849
36 14.4693193002641
37 15.2816210848123
38 16.0396931619223
39 16.6201764460665
40 17.2095178942578
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 -0.029288855830206
1 -0.283506674278094
2 -0.592322374003969
3 -0.681510936631919
4 -0.632078238697049
5 -0.59400815105821
6 -0.524379836294111
7 -0.716143997910039
8 -1.16515456600594
9 -1.63421019851849
10 -1.7801706097432
11 -1.79443989991284
12 -1.62125035281289
13 -1.22682521416497
14 -0.821926710459408
15 -0.273388653951196
16 0.465938776936496
17 1.5005434978166
18 2.57861262820097
19 3.68441207765894
20 4.83559970087791
21 6.05672082221308
22 7.04539120448892
23 7.9958297906194
24 8.96006342151092
25 9.86358321399954
26 10.7899057423369
27 11.7232551274904
28 12.7217020369423
29 13.6726945902269
30 14.5740814429387
31 15.5293841363485
32 16.4309793128626
33 17.2261916824601
34 17.9730150760805
35 18.6778529319124
36 19.3724022323178
37 20.1053073087484
38 20.7967035136973
39 21.425018533695
40 21.9333394978276
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0537566569760384
1 -0.130165496135204
2 -0.467895018480454
3 -0.467137354629763
4 -0.452694039001471
5 -0.437486672570884
6 -0.36918643114603
7 -0.689615781653092
8 -1.26885661955746
9 -1.67697955896947
10 -1.91028355323037
11 -1.93998164662297
12 -1.81530257162927
13 -1.36593564767951
14 -1.08903458983426
15 -0.621810431524617
16 0.0863115212324268
17 0.998014876470747
18 2.00973117902729
19 3.02638801691171
20 4.22727970198651
21 5.3273534346926
22 6.34625085772933
23 7.18468736671057
24 8.03819928033752
25 8.85797287625543
26 9.48357494745286
27 10.5507647778003
28 11.2350501441322
29 11.9889916282191
30 12.8361910296188
31 13.6320071922062
32 14.4523588941755
33 15.2447289472193
34 15.8829784763184
35 16.4485679450374
36 16.7031041894898
37 16.9819519026218
38 17.253629096166
39 17.6069853805317
40 17.8220455240687
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.138340945484162
1 -0.222142780459007
2 -0.418036423620061
3 -0.341941319605437
4 -0.242143171021441
5 -0.0730348806209364
6 0.0947941242889114
7 -0.0781714128851423
8 -0.619905259202181
9 -1.10740352585378
10 -1.16730879414939
11 -1.12235148105284
12 -0.970914079427217
13 -0.633685868476423
14 -0.264334599667122
15 0.3010310148579
16 1.15656975420392
17 2.14498763401311
18 3.13512099455822
19 4.08372490264516
20 5.05493090857436
21 6.04561144521968
22 6.96829099584974
23 7.94390159915493
24 8.89846983200669
25 9.9126331640021
26 10.8762457275971
27 11.8916825877088
28 12.8454001992622
29 13.7707628865995
30 14.6846965844249
31 15.4249196032592
32 16.2900251464408
33 16.9270809658064
34 17.3371137947597
35 17.8535110204905
36 18.2879438056634
37 18.6917694835592
38 18.9902899480122
39 19.345941136454
40 19.5695525526689
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 -0.0487907868719768
1 -0.171846297500737
2 -0.277795954463835
3 -0.252238650432392
4 -0.117937476142969
5 0.081596534533428
6 0.0628684580105978
7 -0.296522285268083
8 -1.02760357171251
9 -1.56898173385963
10 -1.6775241765369
11 -1.77569023178755
12 -1.84627175134323
13 -1.53338415516435
14 -1.22011543431707
15 -0.778076660094282
16 0.116080624461266
17 1.09924748880705
18 2.19348718708388
19 3.30475104562738
20 4.56000433923842
21 5.76814625597004
22 6.87785252935453
23 7.96697386313203
24 9.01721548493242
25 9.93950874053236
26 10.8526802118896
27 11.9311399598913
28 12.8786487690109
29 13.9315409751941
30 14.8744092355398
31 15.68045487732
32 16.5600627397969
33 17.3952005665164
34 18.0582300292802
35 18.5847003974037
36 19.2168742547865
37 19.714431075556
38 20.0837022212392
39 20.4281905237418
40 20.8026729376639
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 -0.0313154646058731
1 -0.182585747868389
2 -0.492583013400292
3 -0.568816421238005
4 -0.552063719771169
5 -0.518601057530272
6 -0.543446532101585
7 -0.587850877841201
8 -0.920701567053356
9 -1.21451992974407
10 -1.39234226844353
11 -1.48345160301993
12 -1.41929587630813
13 -1.05789873110714
14 -0.882572532840651
15 -0.517587663011412
16 0.232450206342406
17 1.08841547548248
18 2.07549057466006
19 2.98747202707828
20 4.07687728218212
21 5.00044026767959
22 5.95157068918629
23 6.75989481683916
24 7.50093432078472
25 8.25001641743693
26 8.98065128851067
27 9.73846872321237
28 10.508077825415
29 11.3190965080633
30 12.1277645689386
31 12.9106353946306
32 13.7161668706452
33 14.6519044134709
34 15.2760339991457
35 15.7499996283987
36 16.3741466447907
37 16.9315268710654
38 17.4778453744571
39 17.8688159730947
40 18.3422630164312
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0403802632106243
1 -0.116661618348709
2 -0.283548706244655
3 -0.351262211397426
4 -0.352089718505999
5 -0.284616818029461
6 -0.319275644523874
7 -0.326655683203132
8 -0.61949978380278
9 -0.936334061468781
10 -0.998707824590017
11 -0.764281303816611
12 -0.364466769221627
13 0.193027870686372
14 0.70141756299593
15 1.29508327766706
16 2.08296222298658
17 3.16543550344662
18 4.24566002075026
19 5.4431545213856
20 6.58115855391506
21 7.70325018739528
22 8.81209981991367
23 9.91393997037174
24 10.9232115870623
25 11.8584193491044
26 12.7994786558827
27 13.7385554249937
28 14.8836726691996
29 15.8747280026708
30 16.8059489980974
31 17.6942965630184
32 18.5583243283551
33 19.2435040647361
34 20.0558931648907
35 20.7119215153184
36 21.3266590422289
37 21.8803995689802
38 22.4600485044186
39 23.14479005072
40 23.7564787212486
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 -0.0649692325778322
1 -0.200531819000418
2 -0.33272738869808
3 -0.328603735409656
4 -0.169880886656315
5 -0.0267962604178971
6 0.179519172025448
7 0.0821511872893224
8 -0.161773765446374
9 -0.313901293755473
10 -0.32804810085845
11 -0.119441925897381
12 0.141739476436287
13 0.58256907240852
14 1.09504488531395
15 1.6829079538241
16 2.37313573534466
17 3.28624555370259
18 4.33343460355695
19 5.20244878435949
20 6.16734247543533
21 7.02565519925954
22 8.04795147678576
23 8.89635045256632
24 9.73130359054622
25 10.7294168903744
26 11.6682153430856
27 12.5696841402113
28 13.4985966450143
29 14.3406700434703
30 15.1035008594021
31 15.610841117917
32 16.3080439217082
33 17.0169494393583
34 17.5440894829019
35 18.0782714196359
36 18.6958899108459
37 19.2646529375187
38 19.7426863285303
39 20.2675457818332
40 20.7513684043166
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0568017254570212
1 -0.0831460967429822
2 -0.327085199263223
3 -0.229725517038437
4 -0.0767475990895785
5 0.0969743517078405
6 0.271395958129853
7 0.0684420034361293
8 -0.253690227127144
9 -0.626332800312221
10 -0.656951172982716
11 -0.544648863338694
12 -0.263802346382903
13 0.2113930253968
14 0.7766627167164
15 1.47852026714663
16 2.20096577238253
17 3.17919147904173
18 4.52202334257797
19 5.88405769255512
20 7.21925119085971
21 8.44763475865792
22 9.52346365115834
23 10.5893995849202
24 11.6635583758728
25 12.5900247866625
26 13.522655298424
27 14.5480423939869
28 15.584547615684
29 16.6001220662144
30 17.4842061795764
31 18.1937423056124
32 19.020226390075
33 19.6726336374888
34 20.3024996390353
35 20.8884681046812
36 21.4441518501059
37 21.9943545748731
38 22.5130018367344
39 22.9562039194663
40 23.4685011781726
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 -0.00569192588469525
1 -0.319208855642044
2 -0.475982477213101
3 -0.553204052232257
4 -0.585196368119225
5 -0.528111744344296
6 -0.492194528740221
7 -0.893850900156723
8 -1.43704875570817
9 -1.96792918345121
10 -2.14257798420583
11 -2.38877100535117
12 -2.51429296701575
13 -2.32680450580955
14 -2.13004247235087
15 -1.7581057624255
16 -0.982500483999343
17 -0.0129899572358045
18 1.08619884732294
19 2.20409956207636
20 3.50838032397538
21 4.53469029381852
22 5.5053569814287
23 6.51567330666988
24 7.4046555466996
25 8.31804934605089
26 9.06724928739245
27 9.85964166758747
28 10.6780286666633
29 11.5019234624467
30 12.290430475851
31 13.0915332378705
32 13.9743475356818
33 14.8608963959878
34 15.6378966898642
35 16.412114948311
36 17.0106176229845
37 17.7320504719511
38 18.3163305690293
39 18.8512520704193
40 19.3538152096896
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.036222775359438
1 -0.274257428457292
2 -0.531724766262537
3 -0.4933206978279
4 -0.460847499671898
5 -0.420798484573029
6 -0.391757377573543
7 -0.69178939770376
8 -1.20167391907466
9 -1.61023931648824
10 -1.77193424574877
11 -1.79833854253019
12 -1.7303564857941
13 -1.50957210816041
14 -1.22418258416874
15 -0.741753566705058
16 0.20402636128378
17 1.22803586289117
18 2.45423538675451
19 3.77752062118751
20 4.95595058778126
21 6.26093089258845
22 7.33420949134024
23 8.41344360541939
24 9.31032925508658
25 10.3475360332595
26 11.2896704024332
27 12.2411403232214
28 13.3024734887867
29 14.3469304621279
30 15.4294195260895
31 16.1958273756109
32 17.047545112881
33 17.9619843306779
34 18.4531594150031
35 18.9662261481083
36 19.5801798877583
37 20.1905253644322
38 20.8170090800634
39 21.3540274169145
40 21.863504997559
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0544670952593567
1 -0.214619424290012
2 -0.525818468673987
3 -0.638031061328934
4 -0.67176647793478
5 -0.600004097487403
6 -0.460552992498469
7 -0.558953940306429
8 -0.8889965276685
9 -1.41794798480464
10 -1.61460876620849
11 -1.54438829148272
12 -1.55659555738979
13 -1.14396797369493
14 -0.622830218884785
15 -0.122272336292971
16 0.660443272645715
17 1.62991817900251
18 2.67361475107195
19 3.79098601899826
20 5.06054010658745
21 6.11023128019491
22 7.19341608375348
23 8.18163772246973
24 9.10302666785648
25 10.0117518233188
26 11.0163833370821
27 12.1028160326172
28 13.2014645880967
29 14.0468274957903
30 15.0047284639275
31 15.8638534832882
32 16.6746115694855
33 17.3379411539658
34 17.8465115142143
35 18.1609131013013
36 18.6555723198637
37 19.0165992470097
38 19.2383414407019
39 19.4017204895586
40 19.5134654710735
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 -0.0467005820153696
1 -0.263967549119384
2 -0.492015361992824
3 -0.621696318050051
4 -0.65598325868774
5 -0.702197285570231
6 -0.695083743007661
7 -0.881580903186609
8 -1.33733738616331
9 -1.74169259965465
10 -1.91736309703968
11 -1.81544627190315
12 -1.69620824406197
13 -1.33601852568649
14 -0.842355085165865
15 -0.191840187140197
16 0.700928522673836
17 1.82510171333499
18 3.04820638600788
19 4.22541319048829
20 5.42162838022788
21 6.51293855275807
22 7.68335985378574
23 8.68098057508677
24 9.68658516197
25 10.7925273864916
26 11.7755157524325
27 12.7694382444338
28 13.8776746114922
29 14.8063557129471
30 15.6858948689923
31 16.3307607408337
32 16.9411306593627
33 17.5012651145147
34 18.0106715499236
35 18.5525261975643
36 19.031717078189
37 19.5209958898285
38 19.9098369636045
39 20.1586728144781
40 20.5614824262942
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 -0.0465982209856883
1 -0.401002305844894
2 -0.631387924312771
3 -0.548058000691666
4 -0.367522081433664
5 0.0205663339923841
6 0.352586041296362
7 0.0582477218487796
8 -0.563011950277695
9 -1.19782443650366
10 -1.46708189583478
11 -1.55060010492134
12 -1.63722606918919
13 -1.35608011135798
14 -0.906842749709053
15 -0.347363892466458
16 0.511104743300194
17 1.58809195128104
18 2.64789006283904
19 3.93109230868915
20 5.33688226800894
21 6.39122100892884
22 7.51232202138415
23 8.54156992305177
24 9.87770102423932
25 11.044905917075
26 12.1561410872089
27 13.3246133812523
28 14.4412950171925
29 15.4133171374418
30 16.3320453673796
31 17.2342079561194
32 18.1098721878349
33 18.7684402352299
34 19.4970497788729
35 20.206955326368
36 20.9402195010846
37 21.6109693339964
38 22.2598851624835
39 22.9532520831261
40 23.6263956186656
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.000463008810560162
1 -0.280461044668726
2 -0.478160252130588
3 -0.622422022216748
4 -0.56468366598668
5 -0.485107072406562
6 -0.494512548277038
7 -0.757570079779437
8 -1.02548291346114
9 -1.17292996333361
10 -1.20643654778784
11 -0.960745310000175
12 -0.641336980472709
13 -0.26656159916046
14 0.143411921654947
15 0.750718183910946
16 1.74409089100222
17 2.95876837435971
18 4.17393244214062
19 5.359513540322
20 6.49174301526112
21 7.7112272810913
22 8.91759735556553
23 10.1253339965481
24 11.4323504229592
25 12.6324352461339
26 13.8433448666188
27 14.7831512043832
28 15.8049043284337
29 16.7076251588447
30 17.5563480664694
31 18.297165032057
32 19.1107403343379
33 19.8620137158884
34 20.4992113738683
35 21.0938393537884
36 21.5405197427087
37 21.956031443767
38 22.4029032044521
39 22.838686162708
40 23.2907367509481
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 -0.0504982135793206
1 -0.303239337815911
2 -0.543145834837835
3 -0.611805514963906
4 -0.642582253154378
5 -0.642164453385
6 -0.660461047603849
7 -1.00948494689822
8 -1.41346150972859
9 -1.83654957367691
10 -1.88358154815674
11 -1.91970735856437
12 -1.86565588147537
13 -1.54364945850279
14 -1.11640465861662
15 -0.520192755475219
16 0.36851888721819
17 1.4746897962509
18 2.50693467093837
19 3.48388946113833
20 4.55910624765862
21 5.39383090866721
22 6.16184959455024
23 6.95451520372122
24 7.77907038890943
25 8.62684874017223
26 9.39590281100389
27 10.1323209265984
28 10.9072974252825
29 11.7340209980071
30 12.5486343168437
31 13.3893850803617
32 14.2085165568109
33 15.0193028043562
34 15.8382682382848
35 16.6488199485701
36 17.3824158132696
37 18.0625387434827
38 18.6558107531541
39 19.1791606634875
40 19.7738643807903
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 -0.0063074966453045
1 -0.129829298107721
2 -0.301129551445666
3 -0.542037213801951
4 -0.668194294116127
5 -0.638611949720936
6 -0.646590952036273
7 -0.842098648612942
8 -1.29071360081417
9 -1.63402184275805
10 -1.84092578767578
11 -1.87570258832365
12 -1.90677123878758
13 -1.78181481713121
14 -1.61230622724274
15 -1.22588759143036
16 -0.452393749129179
17 0.549597385337338
18 1.58755635125846
19 2.49757169871624
20 3.53466375169653
21 4.64813272268239
22 5.75854462484515
23 6.87473863171594
24 7.87045605300511
25 8.88561921041384
26 9.81924937899289
27 10.7498686889759
28 11.8496887206
29 12.8532378650843
30 13.7269828248659
31 14.5004960716966
32 15.2819613251127
33 16.0337761985623
34 16.6816104370037
35 17.1707519126239
36 17.6463591861201
37 18.0357986558657
38 18.3681483945702
39 18.6539031237869
40 19.0058571129583
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 -0.00752081395918847
1 -0.249983691020137
2 -0.549447460862701
3 -0.594951899357496
4 -0.452511974764745
5 -0.307635271723606
6 -0.132870176648612
7 -0.191411359436461
8 -0.37524436277223
9 -0.458974218334091
10 -0.385958732078984
11 -0.0697387541571008
12 0.312965757052321
13 0.920111610657138
14 1.68150200783519
15 2.4482205097948
16 3.65448899363159
17 4.81935997048484
18 5.97524989752272
19 7.09895471711849
20 8.18474631332386
21 9.21702757702919
22 10.2551345628736
23 11.2398149003305
24 12.2607159183775
25 13.2183223650823
26 14.2651030249382
27 15.137104643282
28 16.0428385862389
29 16.8992781312604
30 17.6645466732679
31 18.3831338567631
32 19.0870500626986
33 19.7892533033122
34 20.4535701646598
35 21.1278722172909
36 21.6942884715695
37 22.1550302844694
38 22.5800249953968
39 23.004450964084
40 23.3607693394473
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0519273161418852
1 -0.270020875905633
2 -0.623142655151968
3 -0.728154533440963
4 -0.725421881303606
5 -0.664067692536806
6 -0.651014169419626
7 -0.730102219086126
8 -0.844515966286737
9 -0.855933227205577
10 -0.734305305546552
11 -0.381623797415349
12 -0.0769923508487107
13 0.571439652140032
14 1.24020335982123
15 1.90392476389553
16 2.8676919887755
17 3.96072650645434
18 5.06584024217588
19 5.93642278933226
20 6.87641958946593
21 7.67258735519654
22 8.43277105881972
23 9.06473829316718
24 9.77246344352572
25 10.4814916863022
26 11.3893883415875
27 12.5010944740242
28 13.5593048776806
29 14.6779066985699
30 15.6991431507565
31 16.5695762408538
32 17.3624160825029
33 18.0712602227489
34 18.6756719654608
35 19.2307545771884
36 19.769194409643
37 20.2066925806152
38 20.563108505593
39 20.883412856075
40 21.1510773207563
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0210655367525394
1 -0.208354140449843
2 -0.495096962700733
3 -0.648948170835558
4 -0.851413027765694
5 -1.00858625456401
6 -1.0936115449658
7 -1.46437741043798
8 -1.86178572551617
9 -2.19114768011283
10 -2.48801940847741
11 -2.30678194436619
12 -2.16885524632761
13 -1.6683713525642
14 -1.28281438817747
15 -0.823936455994313
16 0.0112010688611792
17 1.08059810762404
18 2.24027320131544
19 3.29490666812858
20 4.3520339082712
21 5.32307627848419
22 6.23121528042784
23 7.07801351379717
24 7.84196823476833
25 8.73307937555844
26 9.67002487949826
27 10.4900944012031
28 11.4465978337343
29 12.3050946329009
30 13.2143387238873
31 13.9969874470206
32 14.7622677525882
33 15.3956902906345
34 16.0724992086614
35 16.5947590149482
36 17.0803939295711
37 17.4149293921012
38 17.7130048731164
39 18.0024671627301
40 18.3112954702559
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0959148948927209
1 -0.111353073306211
2 -0.329493146792301
3 -0.499876950362212
4 -0.505781374995123
5 -0.496623150208842
6 -0.378139126197405
7 -0.659158784219261
8 -1.15000641178508
9 -1.50067742951447
10 -1.56583621975245
11 -1.40330081494933
12 -1.20545104629401
13 -0.893823845101128
14 -0.482015463087216
15 0.0595540672322707
16 0.977453630570606
17 2.01813645922616
18 3.03068359143002
19 4.1670457004544
20 5.27617708396121
21 6.15632344863384
22 7.09452080795892
23 8.00725150749098
24 8.93370813631909
25 9.93250907581758
26 10.8860625428231
27 11.8036449363348
28 12.7969594536774
29 13.8520324208668
30 14.7448926871565
31 15.5442779615659
32 16.3063751283339
33 17.0765006524833
34 17.728040416296
35 18.2931636786421
36 18.8591686016627
37 19.3912975314709
38 19.8286192368383
39 20.2305565690885
40 20.6513834592025
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 -0.0302074717125356
1 -0.151139681431237
2 -0.22757276124733
3 -0.286534996999793
4 -0.354168721559428
5 -0.307465905704598
6 -0.169385469680807
7 -0.42096499678695
8 -1.16480618350385
9 -2.03946032645404
10 -2.42188395440442
11 -2.77708803143181
12 -3.07503797246179
13 -3.06113040110145
14 -2.92321660526605
15 -2.70512797774136
16 -2.12648871047449
17 -1.29107271510221
18 -0.199651054402393
19 0.826770472832561
20 1.89353279165023
21 2.9369290069104
22 4.07707737274413
23 4.9422422939716
24 5.8809523009379
25 6.73777994626622
26 7.5113491732197
27 8.18241769794945
28 8.99555236013287
29 9.62406278496054
30 10.3503382902337
31 11.0551719624265
32 11.8612412664624
33 12.6036154579612
34 13.0817595888708
35 13.6151900712522
36 14.2057218727931
37 14.7023310811974
38 15.1221073569404
39 15.4842090765999
40 15.7788004178295
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 -0.0377219491040965
1 -0.25592566619424
2 -0.456857448897776
3 -0.451280890811232
4 -0.430588967004736
5 -0.297158458775751
6 -0.216355707764493
7 -0.597679766528306
8 -1.09224329762332
9 -1.48777593570689
10 -1.72005110432791
11 -1.65225090620433
12 -1.61824589628337
13 -1.26561570190441
14 -0.656939050707082
15 0.0372987768738891
16 0.794940422082612
17 1.71656939876331
18 2.73172869220844
19 3.8129623598782
20 4.9438972528392
21 6.00638881166049
22 7.1766347764981
23 8.28647671251313
24 9.40159274294543
25 10.4614937998546
26 11.3968923692432
27 12.4233884843252
28 13.3566592476604
29 14.2472578589754
30 15.1735312976049
31 15.8847631105339
32 16.6529295938206
33 17.3400600772867
34 17.8029032899434
35 18.2194435429824
36 18.60559793915
37 18.8971221490139
38 19.1880683572373
39 19.5626832555685
40 19.8486187432842
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0352928579887077
1 -0.0382444633813726
2 -0.227142059742844
3 -0.379829739309371
4 -0.591685110542211
5 -0.707748024518234
6 -0.777518481487442
7 -1.02931786640182
8 -1.42486522109562
9 -1.85449823318668
10 -1.95827866230435
11 -1.861720061142
12 -1.70445036821294
13 -1.30931120682004
14 -1.00663167829031
15 -0.648524834853023
16 0.244184301861011
17 1.36764755852608
18 2.3974842287785
19 3.46795927527421
20 4.5043766260341
21 5.51693647173107
22 6.43632365889948
23 7.37534920509074
24 8.30818093837537
25 9.22783209819527
26 10.1707731258028
27 11.2850894990307
28 12.2964392236519
29 13.2211524909391
30 14.1521612386871
31 15.1041380666415
32 15.9981891650406
33 16.8056652375889
34 17.5736437462495
35 18.1906072481583
36 18.793828850943
37 19.2297043469406
38 19.665767800921
39 20.0702874803462
40 20.4495276814498
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 -0.0126757113343072
1 -0.204189270459962
2 -0.403704260230663
3 -0.507905531853537
4 -0.432182636222415
5 -0.214212493131769
6 -0.0355926806419915
7 -0.412749961637682
8 -1.01234613283198
9 -1.57839235098635
10 -2.0639039205505
11 -2.35488038649808
12 -2.39078271542777
13 -2.22043684827234
14 -1.96373915321777
15 -1.64781273116673
16 -0.940110421124154
17 0.00193255849476559
18 1.01410069742865
19 2.12992545122383
20 3.10240832923646
21 4.294814083818
22 5.37360797138195
23 6.44538588278778
24 7.4751721337913
25 8.44531331272691
26 9.45481033212031
27 10.3620946340746
28 11.3738257115572
29 12.356130526128
30 13.1783120522847
31 13.8035318950437
32 14.4649768777663
33 15.0703731636709
34 15.606623880864
35 16.0845468120411
36 16.3654201015622
37 16.7391338045469
38 17.0163763549975
39 17.1939228707612
40 17.4385819678801
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 -0.0229877357457751
1 -0.212774703104669
2 -0.492701498318201
3 -0.304083906349351
4 -0.109471546344325
5 0.189124969201036
6 0.419720258930507
7 0.17970170820211
8 -0.412990307059272
9 -1.18346930066794
10 -1.50896000923914
11 -1.73737756541111
12 -1.74132339671601
13 -1.56436102275584
14 -1.24897439162649
15 -0.796910387002959
16 -0.103671851750454
17 0.794250191900327
18 1.60504952795606
19 2.57751818025912
20 3.87508356160243
21 4.97919501006233
22 6.12647191548396
23 7.20358979372163
24 8.15680263572645
25 9.17878623624139
26 10.0372500173213
27 10.9630625558457
28 11.7278157706746
29 12.6042560581623
30 13.5276908005313
31 14.3257003075178
32 15.1673245034183
33 15.8322724676626
34 16.5407881450446
35 17.1611597803072
36 17.6533888010481
37 18.088753791031
38 18.4680495280734
39 18.8624339453546
40 19.2184167515765
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 -0.00921476605744731
1 -0.0872550128576912
2 -0.398961518361352
3 -0.556215265526637
4 -0.707193440762082
5 -0.765067274137104
6 -0.848917892170147
7 -1.04480897594057
8 -1.32836576396878
9 -1.63940958802691
10 -1.6968841431087
11 -1.5245384495345
12 -1.32884614665213
13 -0.892816103825488
14 -0.32781430395448
15 0.282344732070307
16 1.23365842418678
17 2.30017358874563
18 3.41481067571967
19 4.56894294276445
20 5.65119367515583
21 6.74240764581396
22 7.85128859021935
23 9.04113003134482
24 10.1169539445712
25 11.0556153783377
26 12.2033209352695
27 13.2118725467542
28 14.2514292783294
29 15.2122798810451
30 16.0355952510331
31 16.7463168644104
32 17.4864093516084
33 18.1425433693222
34 18.7707147913264
35 19.3874182576368
36 19.8610198221435
37 20.2472599908874
38 20.6249071661991
39 21.0870020987899
40 21.4775309899914
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 -0.0809223099495338
1 -0.22886194711154
2 -0.535554695778663
3 -0.59415496119437
4 -0.419103980512841
5 -0.303657891751458
6 -0.288154338884939
7 -0.564717452484008
8 -1.26634915873629
9 -1.95987610191376
10 -2.31994817623695
11 -2.5333417498425
12 -2.56956012476236
13 -2.46700916192742
14 -2.17210296112665
15 -1.7656410038956
16 -1.04017880691891
17 -0.0329971925685908
18 1.0069440102154
19 2.09512555418007
20 3.23733320364545
21 4.32805684813225
22 5.42834996790338
23 6.50087236207516
24 7.35085833149467
25 8.30164333020913
26 9.16556244712244
27 10.1371848415808
28 11.017336046418
29 11.9271402399387
30 12.8508367054446
31 13.6556126231089
32 14.5225381360717
33 15.4552862455748
34 16.3595524887832
35 17.1499632195507
36 17.8405727283558
37 18.5122361220472
38 18.9932141800288
39 19.49417436569
40 20.0010191773306
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0601100072083445
1 -0.168621822792135
2 -0.498963237905417
3 -0.53831462819938
4 -0.525976941636348
5 -0.420274413759282
6 -0.334716053845343
7 -0.770401443552716
8 -1.31003621937799
9 -1.94183628350004
10 -2.16974137737528
11 -2.17890739543623
12 -2.13940669146568
13 -1.77879122371194
14 -1.49640304230695
15 -0.920454451919765
16 -0.119558930775603
17 1.01570200481138
18 2.06400748365315
19 3.15944687976655
20 4.32167926131245
21 5.49059676582975
22 6.65201826232442
23 7.80239961257558
24 8.84290329353099
25 9.99116487456957
26 11.1979223398288
27 12.2281492445654
28 13.4460969488379
29 14.3851684508872
30 15.1870054592893
31 15.9124420916277
32 16.6509744995417
33 17.3746137718933
34 17.9468171228696
35 18.5740191998526
36 19.08955522385
37 19.5661628564769
38 19.9721438090756
39 20.2745897667235
40 20.5712399466132
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0255312519125126
1 -0.188176244388042
2 -0.456737860832917
3 -0.582282048886749
4 -0.62438963613977
5 -0.525278249361145
6 -0.402090833841064
7 -0.63706044083052
8 -1.06346230708822
9 -1.6361551281342
10 -1.8783517601272
11 -1.96446310771289
12 -1.93672215242686
13 -1.65421281533967
14 -1.26171143514003
15 -0.759749901255601
16 -0.0141223032181381
17 0.968206332971476
18 2.02042632900932
19 3.06842707583272
20 4.16326275193553
21 5.21735350922806
22 6.1643651328947
23 7.0127843483834
24 7.79353733301694
25 8.61393098268071
26 9.34375059587257
27 10.0597446849639
28 10.7302550920651
29 11.4513747260671
30 12.1336533034073
31 12.7475993247104
32 13.4983119245284
33 14.2685314243844
34 14.971289905764
35 15.6374221916839
36 16.1231364972125
37 16.5918580191756
38 17.1438795119979
39 17.7767408112257
40 18.3441500718519
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 -0.0175697702531541
1 -0.237172960685619
2 -0.414259706584739
3 -0.561104829985352
4 -0.584267448927416
5 -0.613366487595821
6 -0.793393516147857
7 -1.06428844434729
8 -1.48525088301299
9 -1.78357972933506
10 -1.90623802104454
11 -1.69817788583302
12 -1.5300883742011
13 -1.11846484548764
14 -0.759873878036562
15 -0.257274555284896
16 0.574026642966165
17 1.55808447179033
18 2.55050377967604
19 3.57799412472601
20 4.67405749978081
21 5.70527888037646
22 6.65305877021109
23 7.51316146804469
24 8.43269495409091
25 9.33386760483247
26 10.2821218417984
27 11.2435586563742
28 12.2075609371158
29 13.1199637284737
30 13.8939469048143
31 14.5563584704138
32 15.3200462512246
33 15.9122897267081
34 16.3686269880554
35 16.8401477765858
36 17.2618711655393
37 17.6135443681688
38 17.9527998048023
39 18.2588791043684
40 18.6135412850693
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0589736434166421
1 -0.142622019372274
2 -0.505174453468113
3 -0.555432218706854
4 -0.479747589736752
5 -0.371643386443604
6 -0.350499758109812
7 -0.729711414874072
8 -1.33209884504983
9 -1.90671877316708
10 -2.28550432977784
11 -2.22492674900632
12 -2.27414133148763
13 -2.05943333575954
14 -1.82504964526846
15 -1.39470134431549
16 -0.673881208105205
17 0.165408721514483
18 1.03612350271757
19 1.92638614993509
20 3.07554453390574
21 4.2708243896388
22 5.28701766047101
23 6.24550453861871
24 7.24861779281615
25 8.0269979315989
26 8.75371008353419
27 9.57775633183947
28 10.4145286304578
29 11.2267284324464
30 12.0951985486463
31 12.9777258341078
32 13.8173886801454
33 14.6540831452532
34 15.2982676367154
35 15.886929350562
36 16.4766145417006
37 17.0358948431722
38 17.5928842281022
39 18.1256528492131
40 18.610085797596
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0239516897318284
1 -0.289847798441595
2 -0.571718620272021
3 -0.560043229683105
4 -0.500847284744349
5 -0.413446783318719
6 -0.415555855589905
7 -0.690177749934387
8 -1.11866038016003
9 -1.40060514469695
10 -1.38847541381065
11 -1.22297396851381
12 -1.12256105901459
13 -0.814527223526346
14 -0.315909566356879
15 0.23195225623339
16 0.948859284368875
17 2.05298268190446
18 3.1159396897554
19 4.2826780762942
20 5.72721598514148
21 6.95725996909616
22 8.23112728239094
23 9.3039705493672
24 10.5435818727549
25 11.6166880661396
26 12.5938144143171
27 13.4557140750785
28 14.524056583849
29 15.3914240905529
30 16.2141629457845
31 16.8071697857508
32 17.4529852799394
33 18.2417013390247
34 18.6930142762113
35 19.2694047493603
36 19.8601566889478
37 20.2581881851967
38 20.6534624022098
39 20.9997266658518
40 21.3432906103018
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.107127774987719
1 -0.211322153626541
2 -0.412593219942324
3 -0.577692751312697
4 -0.694816011254051
5 -0.695117694951608
6 -0.652274779615222
7 -0.904685166105141
8 -1.43903796507103
9 -1.96322404773709
10 -2.21077878537623
11 -2.32989235850963
12 -2.39144988557857
13 -2.34035615883325
14 -2.12856635927041
15 -1.60427358425417
16 -0.767024870248135
17 0.286236098974725
18 1.3993745927252
19 2.51251730999011
20 3.76244241896396
21 4.94566867614204
22 6.16120458714174
23 7.31325700785226
24 8.25120137663481
25 9.31052706939488
26 10.4116431349749
27 11.4659224264962
28 12.6262253819963
29 13.6523729871231
30 14.6442820272583
31 15.6450551122043
32 16.4785792447484
33 17.3754379484451
34 18.207789734496
35 18.9130836026323
36 19.5206961518303
37 20.168396718409
38 20.7809913802998
39 21.27150490739
40 21.7668913079944
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.00815604325764374
1 -0.164570241415788
2 -0.391344958741918
3 -0.503763085347323
4 -0.431629496014486
5 -0.363667935857201
6 -0.270510879438262
7 -0.44483871762147
8 -0.803744926068719
9 -1.12426604041478
10 -1.33482010708914
11 -1.29815778600782
12 -0.937017173373722
13 -0.408565711197487
14 0.232826241421091
15 0.93785202507582
16 1.80133469521764
17 2.91341203467853
18 3.89085924678117
19 4.79391885944393
20 5.74259543266279
21 6.71535604044871
22 7.67935027064661
23 8.4560544976063
24 9.24309978077248
25 10.1934386796784
26 10.9458312615785
27 11.9072851680576
28 13.033173339136
29 13.9725620022452
30 14.946972491016
31 15.9358788342822
32 16.7280649225183
33 17.4473740134532
34 18.1850989395813
35 18.7412524073007
36 19.3528572410148
37 19.8522319327246
38 20.2265561638504
39 20.6133874618409
40 20.9466189322699
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0157111496816582
1 -0.163281760789787
2 -0.296983525488961
3 -0.419183520804963
4 -0.546943585113073
5 -0.60738493735668
6 -0.742732521130264
7 -0.927276919984022
8 -1.31537042988207
9 -1.5898282738386
10 -1.62100690010221
11 -1.46946008510595
12 -1.23136372897504
13 -0.663526127873593
14 -0.0563315818011727
15 0.655912693600449
16 1.52809869791826
17 2.59479723126755
18 3.65860097924874
19 4.66982384320718
20 5.73419030975459
21 6.70488274092579
22 7.4827253432676
23 8.17944253578292
24 8.98876476233663
25 9.73519634897325
26 10.5029408136229
27 11.3168339726352
28 12.2962496928962
29 13.1360013949463
30 13.9106898465176
31 14.760744079983
32 15.5140216946803
33 16.1302436260003
34 16.6504615935427
35 17.1699092787145
36 17.7506413246805
37 18.3572670081331
38 18.8870703022219
39 19.1225757900621
40 19.4280331368782
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0503256443562017
1 -0.0294632468240752
2 -0.189073179896804
3 -0.258773215692924
4 -0.302649436912075
5 -0.400491552319525
6 -0.572789634572529
7 -0.743027941214394
8 -1.27094884987717
9 -1.66848417445025
10 -1.86293476881435
11 -1.78129560312175
12 -1.63108293620366
13 -1.24552440242662
14 -0.866927384140668
15 -0.31707809115911
16 0.627232568527275
17 1.7325776828497
18 2.83899010745522
19 3.87633823237559
20 5.12984983525656
21 6.20350639645246
22 7.25362532991013
23 8.30611191272844
24 9.42043551946355
25 10.3924172451826
26 11.3759136327803
27 12.3924747587127
28 13.4600287557382
29 14.3612334851415
30 15.2058671926527
31 15.8205687482815
32 16.5462753925203
33 17.3857920252652
34 17.9868798554318
35 18.5624935126184
36 19.1092378707398
37 19.6909687446674
38 20.2698139039294
39 20.7840468626578
40 21.340707710243
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0825362546634651
1 -0.214151005162174
2 -0.541919376191375
3 -0.641843352992209
4 -0.781669866138029
5 -0.834526251226287
6 -0.898005758391119
7 -1.05448573745813
8 -1.45564864495298
9 -1.75688786523186
10 -1.86359339344226
11 -1.76244805792359
12 -1.62670399673474
13 -1.16842689505675
14 -0.762687951760946
15 -0.194097470773743
16 0.762584338833919
17 1.64219497696494
18 2.71600882824573
19 3.82233828627039
20 5.0279763410141
21 6.15677628873167
22 7.15351141431903
23 8.03860839649346
24 9.00636917210971
25 9.93641697430637
26 10.8338985996786
27 11.8312582744286
28 12.8329159907171
29 13.8047856702146
30 14.6939819189068
31 15.296715632241
32 15.9744213058638
33 16.6942997707934
34 17.2977767112464
35 17.8508789721853
36 18.6080055731887
37 19.1693525029198
38 19.6898645523165
39 20.2059423914548
40 20.6799111303176
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 -0.0244843088506519
1 -0.276008377822787
2 -0.444262820895684
3 -0.536604381043622
4 -0.57135597619525
5 -0.554196127485504
6 -0.443884639507096
7 -0.432394180332647
8 -0.5091131826666
9 -0.708197361485832
10 -0.686192294076965
11 -0.433847457036925
12 -0.0692107721702984
13 0.739493417626905
14 1.32690649249863
15 1.83797131749545
16 2.74553592383888
17 3.74562979401362
18 4.85096140054038
19 5.8435261705824
20 6.8076405153449
21 7.62013177094523
22 8.51024131949801
23 9.32981031090477
24 10.2371971264351
25 11.1398262964533
26 12.1526692253135
27 13.1122977548788
28 14.2231162562402
29 15.3958929157786
30 16.3968557597468
31 17.1252262633895
32 17.8786737950421
33 18.4610368141861
34 18.8904556578136
35 19.3444286614048
36 19.8031026993276
37 20.0998886258196
38 20.3338938884908
39 20.4576396455901
40 20.6978548070431
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0270248235631527
1 -0.17953807144952
2 -0.441361411238437
3 -0.553721082812789
4 -0.666790548962705
5 -0.686697570800356
6 -0.754823801902972
7 -0.947702055706242
8 -1.27952061381166
9 -1.52196676704519
10 -1.54572090008289
11 -1.42716374023059
12 -1.10725475295346
13 -0.394000150888863
14 0.214307971036244
15 0.950826810378748
16 1.98765421245306
17 3.18164077294913
18 4.35108392868533
19 5.47050583987502
20 6.4205016393222
21 7.36074557808875
22 8.21292955465573
23 9.10034076714852
24 10.1095050287564
25 11.1346103401977
26 12.120561812705
27 13.3226758954544
28 14.4292784427879
29 15.464122710833
30 16.5101189893218
31 17.2070463897971
32 17.9405121327935
33 18.7152737767652
34 19.2756900812701
35 19.8021883638133
36 20.1816856881425
37 20.5838590694974
38 20.9802248689216
39 21.4360957120643
40 21.9136990804559
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0209867897849931
1 -0.182457935298026
2 -0.360543838001756
3 -0.59559540793211
4 -0.725593340996772
5 -0.844172533398709
6 -1.00248362203817
7 -1.06655634346056
8 -1.29607584397285
9 -1.5128637081822
10 -1.70505127257507
11 -1.56353879824331
12 -1.46521536463209
13 -1.21029149642795
14 -0.745207641865481
15 -0.188973448996177
16 0.743016115429897
17 1.72249656374755
18 2.7589096364269
19 3.78950623234974
20 4.89704716219767
21 5.90842894718328
22 6.91972457363299
23 7.77908066996627
24 8.76996672607313
25 9.64482069593954
26 10.388568781257
27 11.3631291319472
28 12.3348753166527
29 13.258684702206
30 14.1565653709522
31 14.9812415441047
32 15.7584849186714
33 16.4709660117041
34 17.1260061092886
35 17.6306482316127
36 18.0671219564163
37 18.424439317769
38 18.7189307849752
39 18.974779016441
40 19.2591669610129
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 -0.039727256346251
1 -0.263264867480253
2 -0.453701530634908
3 -0.60629682810428
4 -0.507274051359561
5 -0.36542596326964
6 -0.104022928646407
7 -0.358385743100115
8 -0.855398592341642
9 -1.34999796840228
10 -1.67319622625425
11 -1.76995282163717
12 -1.64402316055933
13 -1.28548491635693
14 -1.12935675306169
15 -0.850894737847536
16 -0.157006973400315
17 0.896087966468055
18 1.97544433591677
19 3.11601160367608
20 4.33496639688963
21 5.58055864332538
22 6.60264943362417
23 7.53179927492099
24 8.42296169323954
25 9.36303795349276
26 10.2091331183488
27 11.1537956650405
28 12.0572005488556
29 13.1016937885771
30 14.1781932276232
31 15.194550788702
32 16.1289721649282
33 16.8666805051731
34 17.5423449146684
35 18.1807969199451
36 18.8299065122905
37 19.3998888333131
38 20.0365062582384
39 20.7548427339174
40 21.5344800797334
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0573561233551549
1 -0.219989171947609
2 -0.314022467533679
3 -0.294667096752642
4 -0.236646906315493
5 -0.153344659790967
6 -0.155503876674742
7 -0.386123652083193
8 -0.884446831036445
9 -1.32452097967494
10 -1.43739270133029
11 -1.25798518289922
12 -0.844405089256417
13 -0.193424360366774
14 0.456593423524382
15 1.21419806110437
16 2.09019195086517
17 3.22319093099795
18 4.38583358833351
19 5.43118450094216
20 6.54638399058887
21 7.53082879681293
22 8.59825212300113
23 9.51220657269477
24 10.5134507779024
25 11.684981230254
26 12.7681142902187
27 13.7751179494904
28 14.7671358921584
29 15.6858358222495
30 16.5398134953852
31 17.1229565562624
32 17.7558306192705
33 18.3446931186055
34 18.7281811532738
35 19.1290133566865
36 19.5999612570272
37 20.1067522751024
38 20.5527769470068
39 20.9167985204021
40 21.209566589347
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 -0.0644538343652257
1 -0.240940751108885
2 -0.426783437155934
3 -0.536319417776314
4 -0.571093713467506
5 -0.394904956871152
6 -0.33491164833752
7 -0.233446031050446
8 -0.503464630467434
9 -0.804864867291398
10 -1.01830291800737
11 -0.915255758103268
12 -0.541460732279246
13 0.0897860954334533
14 0.429128179889207
15 0.923898477194231
16 1.79521378441604
17 2.96466267079579
18 4.05080478562934
19 5.1642558087918
20 6.17463553991016
21 7.17328966360212
22 8.15875714743108
23 9.14688764239742
24 9.99938856322387
25 10.898350802448
26 11.7487483341636
27 12.7265402962592
28 13.6008082060196
29 14.4468411427577
30 15.3673152554097
31 16.1164998476743
32 16.9342443291267
33 17.6206578657529
34 18.2969898275423
35 18.9402140189246
36 19.575373502453
37 20.1450453889465
38 20.5848216989614
39 20.8503628098813
40 21.2636290454288
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.00985811532715442
1 -0.138136252708666
2 -0.305801787553805
3 -0.385942846532334
4 -0.409360046482747
5 -0.385032548575038
6 -0.341060716499626
7 -0.404755765914147
8 -0.838442246891951
9 -1.36269249685351
10 -1.52396083041381
11 -1.42288961367866
12 -1.27631651896584
13 -0.939806849609454
14 -0.558061499882201
15 -0.0687861578114575
16 0.576853654482659
17 1.40634337180516
18 2.50083258056954
19 3.78195333492623
20 4.95670748662219
21 6.07089006213456
22 7.24217227586723
23 8.18731443414689
24 9.20521433163949
25 10.2146299512228
26 11.2034359759145
27 12.2514132886891
28 13.1764467503504
29 14.1237476237497
30 14.9241545468532
31 15.6977438029144
32 16.3997842499324
33 17.2397919998808
34 17.7165083210179
35 18.2078740191828
36 18.6579248095236
37 18.984682653666
38 19.1707121527536
39 19.343038365303
40 19.5088650588756
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0138013714984195
1 -0.305294825141111
2 -0.546658352290097
3 -0.498633498744814
4 -0.471149945712066
5 -0.383766720558705
6 -0.369516390616593
7 -0.701938335060724
8 -1.20797124910158
9 -1.66339299450737
10 -1.85641149803053
11 -1.76328259251398
12 -1.62023088990424
13 -1.28716145199278
14 -0.777929242056925
15 -0.0681896961663782
16 0.772092874251551
17 1.64668460407002
18 2.79229231572284
19 3.97536447773155
20 5.05717993295162
21 6.02764307034144
22 7.10500877687267
23 8.07861727699005
24 9.12515080960195
25 10.1170900139973
26 11.1038055305302
27 12.1385122739936
28 13.2577305340697
29 14.3398092701551
30 15.4022899037445
31 16.4645623336452
32 17.4857292467522
33 18.4372363961993
34 19.4152336378745
35 20.2333655729024
36 20.9882330623674
37 21.7806612629443
38 22.6152826989894
39 23.2888257044638
40 24.0174024786831
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0541751033786664
1 -0.253714218772545
2 -0.354214527671236
3 -0.405325871185049
4 -0.358661963585021
5 -0.365645203682444
6 -0.473892140508161
7 -0.800791082414336
8 -1.29523456221153
9 -1.65561860806381
10 -1.82711653907354
11 -1.73545737035308
12 -1.59589630488917
13 -1.17880962717589
14 -0.78489030408882
15 -0.375946833130651
16 0.5549799337415
17 1.57780249163769
18 2.59748485806627
19 3.65562879118845
20 4.77632024296275
21 5.91525595811113
22 6.94425953732658
23 7.89113205278863
24 8.83620941932807
25 9.80730705031831
26 10.8478854373393
27 11.6082594977917
28 12.5894635216761
29 13.4927139258387
30 14.2908672737204
31 14.9590074011965
32 15.6228482704655
33 16.2073181158677
34 16.6535923435269
35 17.1259987121245
36 17.7193590370339
37 18.2322100568073
38 18.6304528849545
39 18.869528495059
40 19.2849142155902
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0459961276218217
1 -0.257391446801473
2 -0.56557723075691
3 -0.664240884997464
4 -0.708813441551968
5 -0.747430891025642
6 -0.794365885153665
7 -1.12958694998559
8 -1.50781582473139
9 -1.7663830136642
10 -1.73872338702868
11 -1.52253922548612
12 -1.20961561463605
13 -0.794929199862453
14 -0.267651904260488
15 0.342143197914595
16 1.28259052255513
17 2.3974980593789
18 3.4501960432356
19 4.37718885108
20 5.35741804834113
21 6.29881663152232
22 7.24328600864358
23 8.1618590416551
24 9.02092877957152
25 9.98130778721709
26 10.8677413811415
27 11.8429615047364
28 12.8989778977154
29 13.9624256389139
30 15.0004891475962
31 15.8414398060367
32 16.5667058377125
33 17.2093182494121
34 17.7794516034159
35 18.2009041742861
36 18.7074463200191
37 18.9905611286838
38 19.2185019436535
39 19.3603900616033
40 19.4310346437518
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0500774084917119
1 -0.0562784181584477
2 -0.186153003079445
3 -0.146644894748381
4 -0.133216740860384
5 -0.0326859738537633
6 0.0818934053506317
7 0.0813150447588598
8 -0.17261895102945
9 -0.507478625175525
10 -0.686916724516886
11 -0.544527155937045
12 -0.258418663896474
13 0.180284114133379
14 0.540686735077646
15 1.10678219091475
16 1.95698969604791
17 2.96501627650759
18 3.97856363202514
19 5.05941929703291
20 6.21363114381514
21 7.30832679126403
22 8.42465788555597
23 9.39690812567442
24 10.4898778327969
25 11.3835175243383
26 12.3277856388131
27 13.3335411944503
28 14.3118477274213
29 15.3237082872956
30 16.2312541496226
31 17.0169949385119
32 17.8116799501154
33 18.4397754907471
34 19.0353701205276
35 19.6458367865384
36 20.2569829987762
37 20.8027080359225
38 21.3088286405682
39 21.6841093246712
40 22.2061252478664
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 -0.00954870676646102
1 -0.241182054359237
2 -0.537964920865489
3 -0.536503371735546
4 -0.389580043449551
5 -0.36650830391726
6 -0.255436296094591
7 -0.504253210457768
8 -0.843453477671152
9 -1.23585008526117
10 -1.39645541365901
11 -1.36585032212674
12 -1.30099324574672
13 -0.970428024541584
14 -0.644821168820488
15 -0.205374394748689
16 0.692893417737867
17 1.71078290415443
18 2.92103565019704
19 4.28077024888336
20 5.62661495023
21 6.9518341339143
22 8.11688835719573
23 9.22442908018099
24 10.2587466016993
25 11.380257351845
26 12.4520150075791
27 13.5408469894061
28 14.637850664389
29 15.5181346714881
30 16.372462501974
31 17.1978499292228
32 17.9447623678522
33 18.6504917595364
34 19.3832659196338
35 19.974271339839
36 20.5113082031959
37 21.0576209030876
38 21.6353114151881
39 21.9673910683796
40 22.5290344781014
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 -0.067091570282781
1 -0.274305417735517
2 -0.389156080379537
3 -0.309491747152745
4 -0.265413724415438
5 -0.203920562932693
6 -0.242296097870023
7 -0.669009784697728
8 -1.44879460661804
9 -2.20743149419885
10 -2.56580780209955
11 -2.58424838706199
12 -2.48788285207716
13 -2.23094550830276
14 -1.7626879977834
15 -1.25271136684164
16 -0.494767672320541
17 0.57929407404845
18 1.64785175415383
19 2.87819178890936
20 3.99492414515654
21 5.07779585821472
22 6.15324838181886
23 7.06181054267626
24 7.89552536480306
25 8.75934638433458
26 9.66735492465565
27 10.6099128950437
28 11.465514516477
29 12.2687541096764
30 13.0897097422461
31 13.6843598561172
32 14.390949900352
33 15.0737898736975
34 15.4929121897459
35 15.9315559502259
36 16.4126837653985
37 16.8718030631752
38 17.3364688250783
39 17.7063405735226
40 18.1784292455842
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.0371763826392537
1 -0.236059263856653
2 -0.444128634012008
3 -0.522930201103215
4 -0.602402380157381
5 -0.641341183749333
6 -0.580027995126728
7 -0.656109471909656
8 -0.713550322972941
9 -0.671094557481994
10 -0.621919029284989
11 -0.231891000696495
12 0.409898458606056
13 1.27518941495317
14 2.0035961615484
15 2.77919524886654
16 3.68346284077811
17 4.83710211211393
18 5.7395920650651
19 6.59112703860366
20 7.44563323788501
21 8.48333909283972
22 9.41138162121645
23 10.3463710650663
24 11.3334198487289
25 12.250633341085
26 13.2321516343634
27 14.2456415370409
28 15.0878774872436
29 16.0477196731206
30 16.8826138458869
31 17.5381987145188
32 18.1829078381602
33 18.6821949798489
34 19.079945889926
35 19.5050853610619
36 19.927589479604
37 20.3113964833813
38 20.6420606985943
39 20.9754173818054
40 21.3166995877722
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 -0.0127330518019755
1 -0.23970454185632
2 -0.495225496389658
3 -0.664408553891489
4 -0.703676939720578
5 -0.711191176231192
6 -0.714256607167072
7 -0.83427660569942
8 -1.12131980510328
9 -1.43778383141627
10 -1.67152787003577
11 -1.61144947069184
12 -1.37718657946444
13 -0.848144447812623
14 -0.341173638599886
15 0.296084173355296
16 1.46963999007042
17 2.68028810087061
18 3.85648005131003
19 5.03375238967165
20 6.24368277785412
21 7.33841237818291
22 8.45710613652401
23 9.6625001751346
24 10.7843994670461
25 11.8699463561402
26 12.8422929014537
27 13.7179906864181
28 14.656563293424
29 15.5337749843562
30 16.2612826100546
31 16.8200139628593
32 17.2595188567166
33 17.7306652217294
34 18.0534878159723
35 18.3325068346539
36 18.5580347793825
37 18.8418152963343
38 19.1677805452215
39 19.4789216822497
40 19.7696563273532
};
\addplot [line width=.01pt, color1, mark=*, mark size=2, mark options={solid, draw=black}]
table {%
1 -0.216971117452557
2 -0.698311813338088
3 -0.845437931574839
4 -0.510347906996663
5 0.417785295755321
6 1.45063997856431
7 2.18000698194071
8 2.91511410045934
9 3.99138570661581
10 5.18010069663342
11 6.78065117660923
12 7.92074360825274
13 8.74285795470332
14 9.32370003511269
15 9.44974184549204
16 9.39728065453565
17 9.39942446694502
18 9.45875925073886
19 9.41596191419465
20 9.44604175500281
21 9.43595937363876
22 9.4563381291001
23 9.4069938263042
24 9.38363158073475
25 9.40550089098364
26 9.38007003255305
27 9.42642504798656
28 9.50602660780519
29 9.50516219108816
30 9.43584948844373
31 9.4053013696456
32 9.43579387299814
33 9.39838716046376
34 9.37035636536838
35 9.40687083255091
36 9.4411863522549
37 9.44827707366167
38 9.39444475031715
39 9.40444975096704
40 9.47548755380175
};
\end{groupplot}


==> experiments/figs/cart_pole/tikz_samples_ep-8-all.tex <==
\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}

\begin{groupplot}[group style={group size=1 by 3}]
\nextgroupplot[
xshift=-8,
title={8 episodes (320 time steps in total)},
title style={font=\large},
xmin=-1.95, xmax=40.95,
%ymin=-0.625995024727565, ymax=1.63552063628766,
ymin=-0.45, ymax=0.45,
width=\figurewidth,
height=\figureheight,
xtick={},
xticklabels={},
yticklabels={},
tick align=outside,
tick pos=left,
x grid style={lightgray!92.026143790849673!black},
y grid style={lightgray!92.026143790849673!black}
]
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0237535315866602
1 0.0798579537471182
2 0.206293156205604
3 0.231528364813398
4 0.174940079913299
5 0.0656132347151663
6 -0.023821142511161
7 -0.0545619234131696
8 -0.109429362267362
9 -0.171503473590674
10 -0.240854750458467
11 -0.298003658955224
12 -0.226332015341541
13 -0.142227261310583
14 -0.115100087543555
15 -0.0901554278603998
16 -0.053130475153865
17 -0.0371958259211906
18 -0.0011228166407582
19 0.0164557751340553
20 -0.00477689708107665
21 0.0294825931872778
22 0.0154017153864334
23 0.0400362735900535
24 0.0649662753528384
25 0.123077097192207
26 0.154317870021898
27 0.204580048754517
28 0.249282875089391
29 0.302561017410419
30 0.356782919518281
31 0.430503654305233
32 0.529820147628956
33 0.667657014859438
34 0.773971891491812
35 0.876071907672553
36 1.00623013066472
37 1.15055245915884
38 1.28175888316729
39 1.42267611037323
40 1.58159065258265
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0364767269387274
1 0.0763115509928944
2 0.178936868406556
3 0.184300205612809
4 0.148539310839356
5 0.023533690109045
6 -0.0918431737452927
7 -0.204052592654766
8 -0.25223792582141
9 -0.304668160332676
10 -0.339105093163526
11 -0.370623626533438
12 -0.272879901638835
13 -0.199849642222818
14 -0.143831019956792
15 -0.12419811379768
16 -0.0952394285373082
17 -0.0887392650451666
18 -0.0561508076289812
19 -0.043582347657801
20 -0.0602974901075575
21 -0.0589294455084381
22 -0.0376135557586865
23 -0.0018353515954459
24 0.0607531493539231
25 0.156148638361773
26 0.28954813678927
27 0.391580352759525
28 0.469971307686211
29 0.548111700836402
30 0.618821965966432
31 0.687136407268421
32 0.73831837607598
33 0.766283022905026
34 0.803470487517153
35 0.814097580123631
36 0.836226416065676
37 0.862693561183932
38 0.890950000623252
39 0.90398835578385
40 0.940841825434891
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0328548541873239
1 0.0713421221410799
2 0.178893476041573
3 0.187393065862135
4 0.14883457738412
5 0.02448565922281
6 -0.109835522381654
7 -0.201738586536367
8 -0.272117120050251
9 -0.351248279279211
10 -0.374789461154688
11 -0.374341117123962
12 -0.283754203245776
13 -0.208943375988228
14 -0.17010058958987
15 -0.129507204977112
16 -0.0919029780706655
17 -0.0940424281212566
18 -0.0727633102576375
19 -0.0579498449986904
20 -0.059379285604769
21 -0.0838181550578332
22 -0.0997132901935975
23 -0.153754753532322
24 -0.182973176562605
25 -0.208325821096775
26 -0.215446371865341
27 -0.237996349650844
28 -0.215719227845461
29 -0.153545438057102
30 -0.0556667386842955
31 0.000132092694316022
32 0.101164799907663
33 0.192477412355268
34 0.210616335624248
35 0.257503392281785
36 0.296255888600464
37 0.290319510533496
38 0.301977357576637
39 0.283155286767725
40 0.220173364167275
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0263982479137796
1 0.072931577995873
2 0.18469804326719
3 0.184549547896231
4 0.164819276023321
5 0.0112030173605211
6 -0.128060282826567
7 -0.217579306449556
8 -0.297545143520333
9 -0.352644837381746
10 -0.497177363087539
11 -0.535424455932419
12 -0.469547543556303
13 -0.385287139880336
14 -0.33572444744415
15 -0.289851058641315
16 -0.278573861045555
17 -0.249021973069401
18 -0.256809976878489
19 -0.264861178166246
20 -0.255826439691183
21 -0.236660063210264
22 -0.232843035088671
23 -0.22637135617282
24 -0.201152431168385
25 -0.193883871951391
26 -0.17495706214679
27 -0.174397902010735
28 -0.170613481498271
29 -0.169436493068649
30 -0.174698079952156
31 -0.14963007321937
32 -0.146666655363616
33 -0.143349888731471
34 -0.145211517242168
35 -0.124298939032427
36 -0.108740798718618
37 -0.113818189650713
38 -0.102295831941094
39 -0.0976929936369917
40 -0.0968087757887961
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0282823829193806
1 0.0863295544106348
2 0.224824107936088
3 0.218561844025333
4 0.183921497554064
5 0.0361858672664175
6 -0.104334159449514
7 -0.175279744559358
8 -0.268298799405972
9 -0.297511777209682
10 -0.398715833648121
11 -0.418283788257081
12 -0.339667029492969
13 -0.268403118985916
14 -0.194827124755075
15 -0.108812097827012
16 -0.071249099170136
17 -0.0453225003655477
18 -0.00694372021924305
19 -0.00651379861798507
20 0.0108848135477118
21 0.00187052839921975
22 0.00330469143957046
23 0.0230191133036364
24 0.079516364391516
25 0.172780462495887
26 0.326601257821015
27 0.423911300703408
28 0.550056571390931
29 0.649399584302595
30 0.727851480597492
31 0.805710725505246
32 0.882267704902598
33 0.951746518353612
34 1.05300228998663
35 1.10834776313744
36 1.20302626226585
37 1.30063558845282
38 1.39017721546181
39 1.48231149523009
40 1.6053128251182
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0164232447776289
1 0.0881692442484248
2 0.198613509387486
3 0.193005676046487
4 0.132543131545419
5 0.0284562509873965
6 -0.097767834807553
7 -0.220623135529507
8 -0.293894539784122
9 -0.360458207636071
10 -0.412970587662388
11 -0.474613728337658
12 -0.448394058532024
13 -0.378514747926859
14 -0.319970486176918
15 -0.273859270134949
16 -0.251919192812629
17 -0.237765384835916
18 -0.237615222223098
19 -0.223984432867945
20 -0.238352785753178
21 -0.218061590874871
22 -0.188681235198857
23 -0.144603993504858
24 -0.142170303297259
25 -0.0667987110234476
26 0.0488453749737126
27 0.112657726754192
28 0.228434302899946
29 0.353706675484836
30 0.454390740314978
31 0.493168303697075
32 0.524884855876041
33 0.585258572982863
34 0.574341476048165
35 0.562658623074657
36 0.562472005999574
37 0.560211381260254
38 0.598795926983844
39 0.635291832309271
40 0.725775080456484
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0296009047148829
1 0.0588586294833986
2 0.18650721579153
3 0.214396594768671
4 0.179869572177425
5 0.0999149549908456
6 -0.0292760599357438
7 -0.101111595749702
8 -0.162257150807092
9 -0.190281166787376
10 -0.268676979076989
11 -0.31467918993395
12 -0.224301065475735
13 -0.133417540163054
14 -0.0764876082024371
15 0.00262661190751778
16 0.0162456658733596
17 0.0237456092104402
18 0.0209812817228778
19 0.026710544862687
20 0.0167097461724905
21 0.0208922598812213
22 0.0360888904165977
23 0.0377457852241614
24 0.0275205277882895
25 0.0385034485509674
26 0.0584063189948987
27 0.0532254567674704
28 0.0656142186190465
29 0.0629962795244872
30 0.0402097680741056
31 0.0461871689219002
32 0.0712216788562667
33 0.0643816834887163
34 0.075850481340459
35 0.102868242722503
36 0.117299287008557
37 0.119425182758569
38 0.119414905363564
39 0.132991385215689
40 0.129667363468706
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0292471845990629
1 0.0627932726628204
2 0.168503086869078
3 0.168195236238082
4 0.118051257055793
5 -0.0100700977199599
6 -0.0954659807751925
7 -0.147979742248713
8 -0.177999294013159
9 -0.186815882905903
10 -0.181245202537052
11 -0.219260707933
12 -0.177706208901401
13 -0.105107163439869
14 -0.110835283284024
15 -0.0779866556670843
16 -0.055811055357017
17 -0.0211570594423574
18 0.0260599667915722
19 0.0510494029955471
20 0.0591925821988086
21 0.0944637745237369
22 0.079592486912853
23 0.0937915425864988
24 0.0796548141357096
25 0.0712408479740363
26 0.0907103076387079
27 0.0680793215901998
28 0.101135628083621
29 0.0876173896065611
30 0.0722083808314427
31 0.0665877058954667
32 0.0465309524187996
33 0.0450143982824889
34 -0.00695716385618006
35 -0.0133263034320148
36 -0.00372524314710621
37 -0.0335267545023923
38 -0.0536295756313701
39 -0.0894818873315515
40 -0.0851192771326792
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0242409196379061
1 0.0524753900295334
2 0.176170660910052
3 0.200055898318263
4 0.162947981762204
5 0.0170886062201587
6 -0.090617112665103
7 -0.15802590112044
8 -0.208561384764447
9 -0.246158014240721
10 -0.38075207290712
11 -0.438110714916878
12 -0.386747874102453
13 -0.315006329552091
14 -0.232524486561396
15 -0.174615387102445
16 -0.181669398113751
17 -0.16209752683383
18 -0.142983616693106
19 -0.125327196032835
20 -0.106857817647095
21 -0.102187944003491
22 -0.117191458210081
23 -0.0975957575844744
24 -0.0892486213112837
25 -0.0726382183571195
26 -0.069131301178631
27 -0.0576111961993249
28 0.00561630040944916
29 0.101217464385173
30 0.23244271592571
31 0.391635437929478
32 0.541876651070203
33 0.657668928107126
34 0.778591990222753
35 0.876292799285659
36 0.932967169461789
37 1.00144788222071
38 1.08924401131294
39 1.14845292272276
40 1.19527258622517
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.029067484502395
1 0.0804956536612389
2 0.203368453423881
3 0.212152211535795
4 0.181377295514406
5 0.0748191497819173
6 -0.0600925234092662
7 -0.132980120858216
8 -0.198789362954449
9 -0.268777371644103
10 -0.291268357729789
11 -0.343959403460538
12 -0.333092711574638
13 -0.275029351573705
14 -0.252818685575865
15 -0.235712624778268
16 -0.240421299358524
17 -0.237837803499316
18 -0.218265558155444
19 -0.221131007287395
20 -0.208797799024942
21 -0.210032758571032
22 -0.24411576072557
23 -0.220590539685816
24 -0.236332827654898
25 -0.247156691302766
26 -0.243716209644976
27 -0.221885201562323
28 -0.223534447841171
29 -0.241258841325624
30 -0.232127845543538
31 -0.223896638942492
32 -0.215992936770482
33 -0.236588909369054
34 -0.219304288786252
35 -0.223550529736574
36 -0.224001384153771
37 -0.227559718647806
38 -0.243304647093186
39 -0.259146437238431
40 -0.26775789536882
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0234216171399462
1 0.0750594315941866
2 0.202896335304224
3 0.201305437299433
4 0.193079302205359
5 0.100182815105201
6 -0.00826112635051324
7 -0.0867478122407332
8 -0.142175102861515
9 -0.185976584338176
10 -0.203479547272775
11 -0.212359106572347
12 -0.152215893883496
13 -0.0576188250259753
14 -0.0525712832194252
15 0.00926069269658125
16 0.0315786725268072
17 0.0201929866632575
18 0.0496625445389487
19 0.0802945518093603
20 0.0718857139111959
21 0.0692092939782487
22 0.11181766355501
23 0.179327663557545
24 0.321409375560955
25 0.441958691177662
26 0.531588015780778
27 0.579757676610246
28 0.606018946524725
29 0.624745435273146
30 0.648685746739461
31 0.713694020700999
32 0.765138191231471
33 0.79976964005835
34 0.81749087982588
35 0.789573500934431
36 0.773587338677045
37 0.766582179274992
38 0.756127314640966
39 0.763092635235579
40 0.738986431092965
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0302615175036598
1 0.0645830707730894
2 0.232044205121432
3 0.237769978287838
4 0.202518846076324
5 0.0664262813095604
6 -0.0710063626621515
7 -0.15603172824708
8 -0.223929111104325
9 -0.275136562101246
10 -0.349584443400778
11 -0.357900012064646
12 -0.293221371157283
13 -0.203886027624153
14 -0.130422041017182
15 -0.0903414184909197
16 -0.0797976622973149
17 -0.0343020730834791
18 -0.0282859826532844
19 -0.0274407015402423
20 -0.00439957152155479
21 0.0993304824821299
22 0.151134980594581
23 0.228136314079173
24 0.317110364998095
25 0.39939289364319
26 0.457043380223611
27 0.58756648614452
28 0.666174672689652
29 0.76970910844313
30 0.869037806195067
31 0.945995483001116
32 1.01944722557062
33 1.08505680133375
34 1.20965691778021
35 1.27182510019316
36 1.35280400084517
37 1.42750581857059
38 1.50246626378592
39 1.54791139812037
40 1.62077283562639
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0210791774364409
1 0.0833112409468288
2 0.191972779945881
3 0.231877299524395
4 0.189826706258395
5 0.0564641962425352
6 -0.0686817431053743
7 -0.149055153459336
8 -0.231064776831663
9 -0.25488299818804
10 -0.293937298693948
11 -0.332378595584486
12 -0.279430119805895
13 -0.196077475843271
14 -0.165094544286592
15 -0.118274335525383
16 -0.107934357557721
17 -0.0961864824834375
18 -0.0773266937021138
19 -0.0635676598929678
20 -0.0488291093145214
21 -0.0231609592516842
22 -0.0377064070169917
23 -0.0521119125418377
24 -0.0610424605278688
25 -0.0742298088957085
26 -0.0379897049612463
27 -0.016062567415065
28 0.00649105473672051
29 0.00426453166816732
30 0.0517646466863555
31 0.123425185245949
32 0.223012666864188
33 0.336165135502881
34 0.385041058435793
35 0.468835296858316
36 0.5766746942598
37 0.657641179227193
38 0.744831311269075
39 0.804452677349057
40 0.840054430975189
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0340484637768865
1 0.0706674420521303
2 0.198461718486694
3 0.218173205262086
4 0.132941809409564
5 -0.00817234855669913
6 -0.112564566633984
7 -0.1827156577224
8 -0.243846031530114
9 -0.274094110081651
10 -0.377730991129089
11 -0.340275987455403
12 -0.247661610901901
13 -0.171180071377106
14 -0.14756795694489
15 -0.112877394554632
16 -0.070989923821517
17 -0.0374899724463287
18 0.00573846967731217
19 0.0139191525804341
20 0.0278227592371465
21 0.0364134099808133
22 0.0938228921626045
23 0.147222633151607
24 0.192511323999169
25 0.246575565173242
26 0.339897713304381
27 0.378416315484342
28 0.402078835295121
29 0.395902183308675
30 0.459906850220621
31 0.452037686344295
32 0.492805152718386
33 0.54787670184427
34 0.575304119513525
35 0.567847921165237
36 0.597860232529828
37 0.632150854460573
38 0.662843959289111
39 0.697845619725303
40 0.732533166764481
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0202100400955887
1 0.0709919778999533
2 0.214816612263603
3 0.210043426602769
4 0.171021450168165
5 0.0506284404371335
6 -0.0933065578676819
7 -0.156760389282629
8 -0.212808025671444
9 -0.26127225585633
10 -0.311571163374921
11 -0.371956973497285
12 -0.305317075866671
13 -0.263346253853675
14 -0.229028405410367
15 -0.174058143250673
16 -0.162273426747291
17 -0.155789799689972
18 -0.14320957229732
19 -0.131731900048641
20 -0.145146895116897
21 -0.134876839628732
22 -0.131547641058566
23 -0.138378971063293
24 -0.146727181354827
25 -0.152207989969159
26 -0.150134181132942
27 -0.167221653290778
28 -0.182663145983604
29 -0.182336306076566
30 -0.167963548969808
31 -0.16364142784243
32 -0.134327918859699
33 -0.127369610060708
34 -0.148124954821362
35 -0.151535627430482
36 -0.132689268078328
37 -0.108701186600136
38 -0.086581392798105
39 -0.074619684360905
40 -0.047597223738161
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0259367209217238
1 0.0537376246590133
2 0.17254537361806
3 0.200748729172338
4 0.164336247409565
5 0.015094976280924
6 -0.0887491759541916
7 -0.16936303359869
8 -0.238635713891985
9 -0.292574957254681
10 -0.348177426381912
11 -0.381277632421189
12 -0.337279411529817
13 -0.22109692677668
14 -0.160321619891303
15 -0.130233597436328
16 -0.1165051943744
17 -0.113484665136911
18 -0.0822786645480598
19 -0.0803925919412114
20 -0.0791342091002152
21 -0.100666057400451
22 -0.104179301998208
23 -0.123153993208569
24 -0.124315714950193
25 -0.118658662760418
26 -0.130887811796593
27 -0.122931695171216
28 -0.125523754676748
29 -0.121707993060792
30 -0.11299332159838
31 -0.0998918690006416
32 -0.0979963591203701
33 -0.110547674679175
34 -0.0988018498600347
35 -0.0924709313084682
36 -0.0862944988784147
37 -0.106851481210335
38 -0.105427268960871
39 -0.0751412235175035
40 -0.0871910494664929
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0282903090820241
1 0.0677092887049584
2 0.19280163074042
3 0.206486210763448
4 0.165377151339601
5 0.0411161111989573
6 -0.0794105196617707
7 -0.181793618796853
8 -0.259761144540431
9 -0.335474013498891
10 -0.40119114522114
11 -0.467758960263795
12 -0.391830780001936
13 -0.338336555143572
14 -0.294907399062737
15 -0.297465640321946
16 -0.252939509105344
17 -0.244842109442579
18 -0.206786687685346
19 -0.204012732603479
20 -0.233161738137308
21 -0.236643215067972
22 -0.255005626985041
23 -0.263929437144534
24 -0.265248661048147
25 -0.246135518932741
26 -0.235137677957352
27 -0.198333046599572
28 -0.137631180533345
29 -0.100049696094178
30 -0.0374424790931149
31 0.0054017238803441
32 0.0362199597392427
33 0.117386314345752
34 0.195768827873736
35 0.281447717542402
36 0.362833147947494
37 0.427859758397327
38 0.549083191267512
39 0.664787020111832
40 0.729913270798571
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0258779984602269
1 0.078662463315414
2 0.184067621409106
3 0.186983138162199
4 0.135265804134992
5 0.00547043498742195
6 -0.0895742214923185
7 -0.146447135598341
8 -0.20834258843015
9 -0.232043062409942
10 -0.270103046622033
11 -0.305702663091843
12 -0.256397412795158
13 -0.196322882239803
14 -0.175397972434033
15 -0.129118472927175
16 -0.0914627848040226
17 -0.0860303872950272
18 -0.0690993497975221
19 -0.0567160198208612
20 -0.057188167325358
21 -0.0708024458268728
22 -0.0780232591679466
23 -0.0900522052002346
24 -0.0609663975358954
25 0.0177128010822516
26 0.133876657038139
27 0.25363593794198
28 0.361615282990135
29 0.464679881671131
30 0.549775078432971
31 0.590542369230529
32 0.625312521959226
33 0.624553857090095
34 0.661195028454356
35 0.684907145033542
36 0.689046973817584
37 0.683897896964004
38 0.6917919387249
39 0.719998413648728
40 0.728644077726573
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0251527769937594
1 0.0827938189820001
2 0.212529075577494
3 0.223776718157284
4 0.197128655622581
5 0.0628779363478129
6 -0.0171090655677384
7 -0.0991300929970365
8 -0.176437489233133
9 -0.241055018517137
10 -0.217366120327315
11 -0.204268317456293
12 -0.122433144359179
13 -0.0632796469457979
14 0.00359371261124686
15 0.0619798004014847
16 0.0834895587926727
17 0.103632273684616
18 0.125247874188593
19 0.143971837574188
20 0.10744662429548
21 0.133813084824967
22 0.126101870921842
23 0.200843957352311
24 0.259013909389059
25 0.355020904728538
26 0.481519068736841
27 0.605863868430232
28 0.659830015299198
29 0.736160638516787
30 0.810644355540763
31 0.904534519624576
32 0.978244723116293
33 1.03818614032644
34 1.03696101219998
35 1.01623244879351
36 1.02412579634004
37 0.985007194785467
38 0.935432451001449
39 0.884205673568256
40 0.80753522338436
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0240263649938699
1 0.0749184608864226
2 0.161504137706419
3 0.174304520645148
4 0.155021806599083
5 0.0227771853928314
6 -0.081815855385071
7 -0.134932860739352
8 -0.1730238441177
9 -0.21702019242
10 -0.288327162836459
11 -0.39281855762241
12 -0.309193906980002
13 -0.220235789446041
14 -0.167588761482341
15 -0.156919954565172
16 -0.145291201419556
17 -0.132508606856898
18 -0.114784669965021
19 -0.111300406856161
20 -0.121564104471256
21 -0.0877685666666776
22 -0.0723648432452348
23 -0.0401707717872393
24 0.0303789914621202
25 0.127524070869269
26 0.209068438720243
27 0.28539746077973
28 0.40084076890563
29 0.556125406467594
30 0.710715707139632
31 0.881587405968242
32 1.07222735016465
33 1.28050593438788
34 1.46040191870661
35 1.65727739295247
36 1.83695027536582
37 1.98117479449905
38 2.12929410086048
39 2.25398734953732
40 2.38713433518639
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0240698554996914
1 0.0701049112111862
2 0.186720774766829
3 0.249946851908496
4 0.198448668561548
5 0.0928431059417445
6 -0.0410310818418953
7 -0.110866544684463
8 -0.181863836366704
9 -0.185361513211782
10 -0.255435810669413
11 -0.27735850594311
12 -0.239652110726916
13 -0.162656390392886
14 -0.127220529566727
15 -0.0821458492036422
16 -0.0813644822138011
17 -0.0644799652208361
18 -0.0272067011173789
19 -0.0281651158839047
20 -0.0304189227244436
21 -0.0155010726587292
22 -0.0139457649656745
23 0.031406425584267
24 0.0270296906974057
25 0.0476146342240193
26 0.0755680036741593
27 0.104259559465523
28 0.205449038414087
29 0.300772503323546
30 0.357164242978733
31 0.448058975220326
32 0.52051473400727
33 0.583782968962594
34 0.659127997411658
35 0.735189914860072
36 0.787623070716288
37 0.849097342478408
38 0.893503774371768
39 0.922992405786203
40 0.989022744549175
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0215043129679469
1 0.0744262271041309
2 0.181314830890349
3 0.187047269587596
4 0.140529465146496
5 0.0458160535889229
6 -0.0716442853704109
7 -0.153436374422608
8 -0.231952415667633
9 -0.277207085400591
10 -0.292016103605314
11 -0.331588103930229
12 -0.259218846512858
13 -0.183643155426141
14 -0.135520628717281
15 -0.122439671575725
16 -0.104901822466636
17 -0.108165009307431
18 -0.0913154061189134
19 -0.090994448935894
20 -0.0980303336844424
21 -0.100601639620887
22 -0.106488855123032
23 -0.118309866554909
24 -0.128882786498014
25 -0.100825157327654
26 -0.0159172435120398
27 0.0575962718292642
28 0.17448127024976
29 0.284959634983001
30 0.378078936567972
31 0.442357913784314
32 0.466121961296125
33 0.511401619130474
34 0.495470218104768
35 0.533502348260837
36 0.559678336601596
37 0.578221637345013
38 0.594112275516398
39 0.587951740967892
40 0.572126382207923
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0265804215213432
1 0.068254650967762
2 0.183758073128458
3 0.168844833768902
4 0.125054601262167
5 0.0229820825972107
6 -0.103557184405023
7 -0.166080748915758
8 -0.25104171799039
9 -0.330757398187313
10 -0.375729355565873
11 -0.430278585394358
12 -0.359332454824414
13 -0.266295267376597
14 -0.208286119365234
15 -0.168356180537562
16 -0.155082264778622
17 -0.120457756355478
18 -0.106054415757463
19 -0.10484705908466
20 -0.117550498813349
21 -0.119423308006972
22 -0.109906602122217
23 -0.104298025817386
24 -0.103682210967439
25 -0.0985932993830385
26 -0.101606757564736
27 -0.112144343489338
28 -0.0777431702209475
29 -0.0695300982330451
30 -0.0609504403458869
31 -0.0723452968958433
32 -0.0619256554593042
33 -0.050984133202773
34 -0.0678816554762589
35 -0.0713926009935948
36 -0.0769324761489907
37 -0.0729458915444985
38 -0.0694501917007893
39 -0.0723868198617668
40 -0.0653550602854223
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0235224376008913
1 0.0834503429791011
2 0.192361002281996
3 0.187603467047555
4 0.159272788522026
5 0.0341433767908752
6 -0.0817758162862026
7 -0.162301273691788
8 -0.226651907354708
9 -0.279729082999833
10 -0.30301732296858
11 -0.388503004759278
12 -0.343920360862132
13 -0.284514919813516
14 -0.264227669604922
15 -0.213387053405167
16 -0.201916893047662
17 -0.179874887053816
18 -0.171671844188016
19 -0.16767621963916
20 -0.174436888023132
21 -0.156067115340415
22 -0.132241559682774
23 -0.114125408178348
24 -0.101135167579045
25 -0.0725860008524268
26 -0.0396416417197472
27 0.0130047076765925
28 0.0952408262706435
29 0.186687076726031
30 0.272569942201788
31 0.312870354336352
32 0.340082458068375
33 0.378187513701794
34 0.426538836653982
35 0.494868197232817
36 0.584266889901989
37 0.707079118144375
38 0.805726829555541
39 0.905284824480142
40 0.990189738890861
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.020915807678362
1 0.0608822109421645
2 0.19232279299437
3 0.182220390623792
4 0.122489156980312
5 -0.0234392469650633
6 -0.143759356896608
7 -0.198509441981263
8 -0.23382697227486
9 -0.28130896163617
10 -0.333896695890488
11 -0.388600331599651
12 -0.322857744064458
13 -0.264585792830082
14 -0.219461116373794
15 -0.200266965375418
16 -0.1788481348256
17 -0.178609688511193
18 -0.163053558250853
19 -0.164175781634953
20 -0.152362474427432
21 -0.163714025279134
22 -0.163699911717385
23 -0.153887067795734
24 -0.146380602545864
25 -0.144183211333153
26 -0.15122606802394
27 -0.152640355126572
28 -0.110200379868092
29 -0.112031020390554
30 -0.0937792982118468
31 -0.0927565234699568
32 -0.0839635067794138
33 -0.067712130551719
34 -0.0569730258462258
35 -0.0703980218567359
36 -0.0523206710607065
37 -0.0467000575103098
38 -0.0414774417885662
39 -0.0375902548041216
40 -0.0253058814791913
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0339211306119154
1 0.0803056473576031
2 0.234831021999834
3 0.235817015707034
4 0.180553305760486
5 0.07254967954949
6 -0.0470255391333696
7 -0.132194595009357
8 -0.236388799531746
9 -0.29996144701146
10 -0.299822481243018
11 -0.336652093854438
12 -0.233265743394726
13 -0.138206295503713
14 -0.0405817559689297
15 0.0440655086128512
16 0.0473584468541537
17 0.0389993040326946
18 0.0608466206729519
19 0.112587385961908
20 0.122094165494957
21 0.143810814661361
22 0.164099791387065
23 0.302972930486547
24 0.337238784797437
25 0.411676465077621
26 0.452932184188186
27 0.511923576231393
28 0.563790479950844
29 0.618018860405757
30 0.676591912097349
31 0.750242493472472
32 0.814198070406679
33 0.912257570512285
34 0.992705141417431
35 1.08706330435967
36 1.1886216430521
37 1.26549433050617
38 1.37216101991617
39 1.46720197900754
40 1.55197500284079
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0346004859056546
1 0.0757167562987462
2 0.204387816815679
3 0.198465293369321
4 0.158364613529801
5 0.0101248930031668
6 -0.114666878761368
7 -0.157598931468922
8 -0.217621316580411
9 -0.249678263006114
10 -0.31899258977217
11 -0.337037913327349
12 -0.281933632569154
13 -0.21833368604759
14 -0.161552011712284
15 -0.113825396330115
16 -0.108024577032425
17 -0.111544736732036
18 -0.0870672473459777
19 -0.0711308852901453
20 -0.0563506431069838
21 -0.0374336516596703
22 0.0147014552049969
23 0.0462676777682525
24 0.0842405089258298
25 0.10094441262159
26 0.140084840869311
27 0.166154936223222
28 0.251447960390943
29 0.311477425796828
30 0.39156025000442
31 0.428104406140828
32 0.457623791421741
33 0.509444501582308
34 0.52589141542998
35 0.558993633091655
36 0.5557779012379
37 0.566853830434079
38 0.577349974745156
39 0.569362218267599
40 0.550857199265866
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0270088846889758
1 0.072600764257948
2 0.193509887406931
3 0.185706137821851
4 0.161152246325802
5 0.0491875781003595
6 -0.0702498591169123
7 -0.161223471789542
8 -0.22907367620108
9 -0.263423582285034
10 -0.332123482961401
11 -0.357410161987814
12 -0.29622383710297
13 -0.217168838302441
14 -0.224844460540993
15 -0.185063463634211
16 -0.171878321256818
17 -0.171707093985861
18 -0.181326636130841
19 -0.181678725473321
20 -0.205449308817593
21 -0.206070091327192
22 -0.245366537575237
23 -0.262845647009557
24 -0.267590056071368
25 -0.277151142154818
26 -0.284338705369272
27 -0.292742651950405
28 -0.272553369222183
29 -0.284672102545718
30 -0.30488236399157
31 -0.306478576977204
32 -0.322112157081555
33 -0.352863053219048
34 -0.346302530152851
35 -0.365404406752091
36 -0.417127458673785
37 -0.429239515462334
38 -0.444031729499182
39 -0.475137452738607
40 -0.492481887814093
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0272238418426491
1 0.0868586388137098
2 0.225399619834947
3 0.238122216478473
4 0.207100941089345
5 0.0973542214765937
6 -0.061268104807052
7 -0.100262844959949
8 -0.152977941148666
9 -0.200484582722475
10 -0.240899978747475
11 -0.284168292256312
12 -0.191779449236241
13 -0.11589482455568
14 -0.0972486995389703
15 -0.0857009176084427
16 -0.0511435384913126
17 -0.0143371278172086
18 0.0129587429793476
19 0.0424082955350551
20 0.0700321913817303
21 0.0714413904414464
22 0.104211019028592
23 0.18210575274265
24 0.331746791373811
25 0.461810077804837
26 0.559630225893876
27 0.675503974014017
28 0.780135463781743
29 0.856267526768355
30 0.926638662059812
31 1.01177122139716
32 1.07966410056285
33 1.15987179259347
34 1.25376551249233
35 1.35468704510009
36 1.46667024384396
37 1.60605375155151
38 1.7338350769126
39 1.86181076366897
40 1.98699516050616
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.030375983595909
1 0.0639025016692587
2 0.170513534987617
3 0.157511889226751
4 0.118228210588389
5 0.0220799173135422
6 -0.0969218499596538
7 -0.206307888680754
8 -0.252288243257871
9 -0.277128318019823
10 -0.353145079294897
11 -0.32218177740853
12 -0.270835430202442
13 -0.215364694035003
14 -0.15631727343376
15 -0.0983068600265318
16 -0.086851777973397
17 -0.05090131044168
18 -0.0461560256818245
19 -0.0270122354695399
20 -0.0216961847300645
21 -0.0316436720610929
22 -0.0251087394616007
23 -0.0139221909932914
24 0.0244418440254623
25 0.0790835652629145
26 0.141009840790115
27 0.167464640293227
28 0.262161526487183
29 0.307606512526534
30 0.374973837921808
31 0.443742982957464
32 0.518710253072242
33 0.602783545543184
34 0.646181855701174
35 0.696554843078323
36 0.775304432719573
37 0.82795276123678
38 0.826614331850048
39 0.842783957353912
40 0.834580565675943
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0358692669558263
1 0.0601476079855017
2 0.189715234374394
3 0.238796802226245
4 0.197390512756031
5 0.056009866599136
6 -0.0520954787913679
7 -0.127313192516432
8 -0.210233907575471
9 -0.28868755487601
10 -0.362634216923138
11 -0.407088904231545
12 -0.345694775932379
13 -0.256528146200583
14 -0.197416899881409
15 -0.167646672061755
16 -0.131090894526475
17 -0.127252365201443
18 -0.10039935231461
19 -0.0756265873535611
20 -0.0544542074593819
21 -0.0171872462390077
22 -0.000177568115611315
23 0.0362294058877728
24 0.0500890880056701
25 0.0213511608402737
26 0.0553421928444227
27 0.11011992900512
28 0.173432836917373
29 0.242245414784254
30 0.287494215957901
31 0.314983899333677
32 0.341898963710791
33 0.354081327056584
34 0.386130226126975
35 0.414476208786943
36 0.406009133122303
37 0.423686863027962
38 0.450094968520403
39 0.458560155307459
40 0.48033254479134
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0316009580019889
1 0.0879142855958346
2 0.194549951511458
3 0.195183284833357
4 0.174832731788238
5 0.0335876638432158
6 -0.0930825222056297
7 -0.161227771148836
8 -0.176297875277308
9 -0.209282908550953
10 -0.239210218135737
11 -0.262659665949346
12 -0.205591634120098
13 -0.137528751582653
14 -0.105351397461067
15 -0.0685972675908788
16 -0.0481130964164205
17 -0.0224457129040658
18 0.00985501293187419
19 0.0160195287990144
20 0.0613065491505651
21 0.089490514284515
22 0.186231991177681
23 0.306235533691638
24 0.446143608337088
25 0.613489160177637
26 0.742673874094587
27 0.883942809010119
28 0.992962543466449
29 1.09082457388452
30 1.19264063522635
31 1.2900838822989
32 1.39100912034433
33 1.45909236880151
34 1.4859049858915
35 1.54099396841254
36 1.59223511124593
37 1.62390681217804
38 1.67976378710157
39 1.69980989630248
40 1.73069883797409
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0215244025243191
1 0.0776310055543181
2 0.198118287698585
3 0.202825108314406
4 0.16066245671516
5 0.054824973421681
6 -0.0773904993855323
7 -0.143043318948247
8 -0.212057118166538
9 -0.199853943311128
10 -0.250452181680322
11 -0.304531389647249
12 -0.213525284539042
13 -0.145742247532289
14 -0.0990758257557562
15 -0.102004977468427
16 -0.107187465593744
17 -0.0950144093988881
18 -0.0647572293969869
19 -0.0179936466520605
20 -0.00367483001585889
21 0.0351112488879117
22 0.0526697670603502
23 0.0975530894312309
24 0.0994340707992638
25 0.101414906302373
26 0.100669088945961
27 0.105221043357303
28 0.165079167442657
29 0.296433400189489
30 0.402186475367219
31 0.434908108286611
32 0.491742742922217
33 0.540311958153421
34 0.540649012727133
35 0.553701994038132
36 0.529772863681468
37 0.570849270745829
38 0.6205526654449
39 0.643337028126076
40 0.650234801149585
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0294633730244396
1 0.0756411174282237
2 0.207832931888126
3 0.241478534399301
4 0.193316139856065
5 0.0676291342615309
6 -0.0642074066401506
7 -0.140787883074956
8 -0.208130995581808
9 -0.254126084747571
10 -0.372179835099604
11 -0.37122851592545
12 -0.292095955077042
13 -0.201471387424741
14 -0.180402883159551
15 -0.155049795038872
16 -0.131535881719234
17 -0.133646557003195
18 -0.12987437345619
19 -0.122318518804867
20 -0.119288689218168
21 -0.103392000584314
22 -0.0667445617760922
23 -0.0492823967283744
24 -0.0334148675641179
25 0.0583971919749855
26 0.148018043314335
27 0.206943177442636
28 0.283976204190392
29 0.363974230038738
30 0.395910776464082
31 0.492870872361327
32 0.564598456104307
33 0.600473598111593
34 0.657558880311649
35 0.704456044967598
36 0.736447012037599
37 0.779926469347237
38 0.847489710306224
39 0.884375523371264
40 0.915930755088493
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0251272773755833
1 0.0872811791617005
2 0.194795502441929
3 0.22913685945884
4 0.177696245583766
5 0.0601597013902548
6 -0.0599552052942256
7 -0.173184262440037
8 -0.238178854963387
9 -0.260580436230096
10 -0.287975159452714
11 -0.357146683958321
12 -0.331217528977624
13 -0.225364295020481
14 -0.183557362679077
15 -0.0917565317810896
16 -0.0867869255458924
17 -0.105448468699878
18 -0.10016157523221
19 -0.0836189605474091
20 -0.0956159050226271
21 -0.0772817519510234
22 -0.0707764810263027
23 -0.0604353801950266
24 -0.0649199393489157
25 -0.0531248380916614
26 -0.0334904519382988
27 -0.0463117055366853
28 -0.0270987005411341
29 -0.00268808433879286
30 0.00687243838673623
31 0.0115925678763134
32 0.0381773406021084
33 0.0341304444521899
34 0.0358720207356651
35 0.0322455475944237
36 0.0533749550031253
37 0.0591464093908911
38 0.088508013326706
39 0.0885007266577293
40 0.106920753250224
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0272167858594772
1 0.0493950288108325
2 0.158433100483923
3 0.184140454594364
4 0.133274191706918
5 0.000519633567837907
6 -0.137330098729531
7 -0.216063442531333
8 -0.258372462905712
9 -0.285410265677751
10 -0.406509136167925
11 -0.405256530947539
12 -0.3211630611303
13 -0.245356873875058
14 -0.184805710253451
15 -0.146126839420751
16 -0.135257484580288
17 -0.118942195450606
18 -0.103291092280907
19 -0.0685277337582475
20 -0.0604508492546776
21 -0.0380981446913511
22 -0.0112605776906607
23 0.0313240783836282
24 0.0798521893291211
25 0.150904048435691
26 0.256730046138643
27 0.374709912599135
28 0.445475039117922
29 0.529200097349095
30 0.614888126719062
31 0.705870243560387
32 0.779729760113498
33 0.804863371847789
34 0.880626273573878
35 0.953024156614761
36 1.03565734017247
37 1.10986107940579
38 1.16067036918564
39 1.23820834277554
40 1.30111901691417
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0263444230373633
1 0.0608023883630553
2 0.185803637458203
3 0.181518509675997
4 0.12060711217659
5 0.00929306795185614
6 -0.0902201937415406
7 -0.183155780421227
8 -0.24150995185579
9 -0.267350144090156
10 -0.358263125636877
11 -0.372286375833622
12 -0.279792500363047
13 -0.178795052624818
14 -0.122679648241595
15 -0.032120771766297
16 -0.0155733497833941
17 -0.0155761234785698
18 -0.0115671657395406
19 0.00142068077094937
20 0.0308185221012609
21 0.0328717753011825
22 0.0301882987824831
23 0.0162905269107059
24 0.021430276407771
25 0.0617078764538332
26 0.184712963597728
27 0.316629778280995
28 0.455672053267907
29 0.591601921129872
30 0.726314080922722
31 0.810310801258612
32 0.931730126376522
33 1.04737133094422
34 1.13974853167928
35 1.21815472180606
36 1.28077434881766
37 1.32920675623487
38 1.38398098943142
39 1.4323493564392
40 1.46753497898482
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0314213261697684
1 0.0623450255181401
2 0.16340550485488
3 0.145816622627227
4 0.128124588538483
5 0.00557578704473727
6 -0.110921817890841
7 -0.18706042761715
8 -0.242173776968461
9 -0.30490483562481
10 -0.369742819856749
11 -0.429022778275476
12 -0.416447931960345
13 -0.37342996245978
14 -0.352888659868724
15 -0.29918709950844
16 -0.298188681054442
17 -0.271712268635706
18 -0.266455017030729
19 -0.255658977557705
20 -0.261127334369574
21 -0.259088092465596
22 -0.270978881659456
23 -0.262586220965591
24 -0.275134018390694
25 -0.283695880520407
26 -0.255398025169773
27 -0.268973823761383
28 -0.226081281323836
29 -0.206486711429331
30 -0.171616468014623
31 -0.166031523179327
32 -0.152755011185747
33 -0.131742140651935
34 -0.0928305489679264
35 -0.0149279901701105
36 0.126464448804469
37 0.222809541564635
38 0.350849760029737
39 0.422974083141513
40 0.446810426354481
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0240340247119422
1 0.0693260230079256
2 0.187344970167413
3 0.206242781038399
4 0.167413788206197
5 0.0335266165015371
6 -0.114339851308976
7 -0.166506929332058
8 -0.230060988069003
9 -0.244475547416172
10 -0.287060730027509
11 -0.357455885055721
12 -0.285364177539654
13 -0.195380864029105
14 -0.141604367895051
15 -0.0828666216181988
16 -0.0695583541924831
17 -0.067137153787777
18 -0.0402656584697096
19 -0.0133361575132973
20 -0.0178749711058783
21 -0.00856824384670407
22 -0.0117353724734857
23 -0.0288445233090027
24 -0.0432731660079213
25 -0.0533029606785478
26 -0.057265724911697
27 -0.0797811068249814
28 -0.100727021099614
29 -0.113516343448104
30 -0.117444709120255
31 -0.128202471784983
32 -0.0838639202762916
33 -0.0424811972193631
34 0.0623793357510936
35 0.114585459504973
36 0.187850937513373
37 0.257392865996684
38 0.344896477470805
39 0.40400930956393
40 0.485639438683143
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0281942261604513
1 0.102856701114801
2 0.226046530612483
3 0.2564450001225
4 0.223504843370878
5 0.0978872491718583
6 -0.036946757524416
7 -0.126760167409167
8 -0.175238193586244
9 -0.202930678683094
10 -0.301863980308087
11 -0.324014029032027
12 -0.237384578934906
13 -0.118676654650399
14 -0.0856892472559716
15 -0.00555713784450518
16 -0.000549750401584781
17 -0.0139094960015687
18 0.00872842137126373
19 0.0168777987979922
20 0.00892209133833965
21 0.0144437172773895
22 0.00444366573606914
23 0.000225670871031092
24 0.0408275959638766
25 0.0770348941120718
26 0.146404621072323
27 0.255609528630989
28 0.417586510228174
29 0.554938532196557
30 0.697233907718683
31 0.820062770043759
32 0.998694733728614
33 1.16401904847886
34 1.30860757459695
35 1.4775136160944
36 1.63536787831477
37 1.82363851987643
38 2.00152986829013
39 2.16630078305106
40 2.34124545131278
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0195748822890049
1 0.0973027406437499
2 0.201422360897632
3 0.214902571039471
4 0.173762460959872
5 0.0440509090144836
6 -0.0792539834858381
7 -0.160975230672503
8 -0.223020240779491
9 -0.30093616261537
10 -0.320629461320348
11 -0.371427467195219
12 -0.327407830017672
13 -0.277204339285947
14 -0.227162716492969
15 -0.187914835161695
16 -0.167189075536747
17 -0.162003996732476
18 -0.125946605213784
19 -0.0963265802466724
20 -0.11368129519911
21 -0.110841184590377
22 -0.147137179764838
23 -0.14692676118744
24 -0.175880374175858
25 -0.178072704925628
26 -0.189562021489608
27 -0.242542080123032
28 -0.223035191330458
29 -0.257218855953981
30 -0.300837734974368
31 -0.317232214355189
32 -0.352190000988691
33 -0.382711492711021
34 -0.428274927259107
35 -0.45966293349414
36 -0.497879351750901
37 -0.527666078559605
38 -0.573265595757367
39 -0.631119620679665
40 -0.684062630576924
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0317625856488677
1 0.0578704412498636
2 0.163767950590043
3 0.17426361557709
4 0.136489815801236
5 -0.00889655827466473
6 -0.121009717917092
7 -0.249326733267565
8 -0.322511553482723
9 -0.371641124265619
10 -0.422100772629832
11 -0.466603696534616
12 -0.368113372705436
13 -0.277156778799034
14 -0.251757617249791
15 -0.247223123604606
16 -0.220377723728467
17 -0.189846203795049
18 -0.15575083526103
19 -0.137708619973663
20 -0.125152778754063
21 -0.110476655873769
22 -0.0995066892426921
23 -0.0971221441506698
24 -0.108528114034349
25 -0.0786853342797977
26 -0.0672827448273896
27 -0.0277624515131292
28 0.00801957078436022
29 0.0329413500516944
30 0.088990607800099
31 0.146092301711135
32 0.242815936383138
33 0.347409470532687
34 0.481220639713957
35 0.607140759087836
36 0.763758405056896
37 0.906705154946333
38 1.02625236418781
39 1.13479465546374
40 1.19889697278491
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0199176265703782
1 0.0655320790743401
2 0.176282374713059
3 0.166085804733409
4 0.0986887934829639
5 -0.0301329623028108
6 -0.16604562052526
7 -0.228337780162423
8 -0.310089478910329
9 -0.310893325129708
10 -0.380496364642217
11 -0.464322865275647
12 -0.485169822410218
13 -0.418656469622936
14 -0.394470281784282
15 -0.346041308257414
16 -0.307578687293962
17 -0.289083754802927
18 -0.262432793336258
19 -0.247365372764471
20 -0.251990941730632
21 -0.218681878535392
22 -0.221505522395954
23 -0.199059731848238
24 -0.218060677134124
25 -0.238308106659831
26 -0.22637560324496
27 -0.268128562553966
28 -0.263017861410363
29 -0.26362228321294
30 -0.271340666887275
31 -0.313757824090016
32 -0.322720111229541
33 -0.313597327469354
34 -0.360853831478787
35 -0.378940831036656
36 -0.355060327093031
37 -0.366988418255118
38 -0.381247566087646
39 -0.41013298038672
40 -0.393264261792109
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0191560600961855
1 0.0830193988735477
2 0.19557607927962
3 0.217589361697786
4 0.164684138057248
5 0.014278522615327
6 -0.102870012666721
7 -0.196364187083004
8 -0.250453690233178
9 -0.286771302714035
10 -0.367294189600949
11 -0.404705015542324
12 -0.305818785952743
13 -0.222293244478189
14 -0.174499094147772
15 -0.135154458702834
16 -0.146271950251474
17 -0.154894985218267
18 -0.145279948910102
19 -0.136906535048195
20 -0.132500555014546
21 -0.0912085485709664
22 -0.0968681480417093
23 -0.0697435471125081
24 -0.0816337808231298
25 -0.0830254511292798
26 -0.069410890150218
27 -0.0886093761979989
28 -0.0564228837785254
29 -0.0739691993685021
30 -0.0744527262364461
31 -0.0830714866104829
32 -0.0875400526351919
33 -0.0802945946691249
34 -0.100551062455456
35 -0.120263345440016
36 -0.109817752265236
37 -0.13350566285901
38 -0.135440759904675
39 -0.156059339351174
40 -0.151251538401389
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0274870178034838
1 0.077041975318787
2 0.194613224889745
3 0.198351892750058
4 0.161298234773399
5 0.0589679371348355
6 -0.0682417106546822
7 -0.152702873910813
8 -0.225336406277456
9 -0.275702134250489
10 -0.361891497977896
11 -0.398869867472777
12 -0.344616450571907
13 -0.262016649060406
14 -0.222378107798878
15 -0.180736165766078
16 -0.153941146387171
17 -0.165283849187701
18 -0.139776594135985
19 -0.135921607009774
20 -0.174395820245543
21 -0.170920125668212
22 -0.153859874188686
23 -0.134616961668203
24 -0.120170036229948
25 -0.0776986923337146
26 0.0258893251462853
27 0.143825652058547
28 0.260999478462291
29 0.364525419985462
30 0.467623051455546
31 0.554200350742318
32 0.637765548204927
33 0.683845332560896
34 0.745632596002419
35 0.782520119357536
36 0.808592151403401
37 0.825169777381023
38 0.868978032139131
39 0.890519907286009
40 0.918841328709862
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0297077407691919
1 0.0695986610112787
2 0.194477156922465
3 0.215261640852692
4 0.182025297926397
5 0.0732343973387479
6 -0.0642818032574608
7 -0.137930776522558
8 -0.193135155739784
9 -0.289849940678187
10 -0.380949098256609
11 -0.436234235050713
12 -0.380362801531233
13 -0.321765420080279
14 -0.279239767143988
15 -0.243233877717732
16 -0.242108860302542
17 -0.242905233074163
18 -0.232722559280929
19 -0.229994966374124
20 -0.218065968188253
21 -0.200837892265933
22 -0.210547806371272
23 -0.212931630493383
24 -0.22415577096483
25 -0.220538212315574
26 -0.222758193476083
27 -0.224846639642453
28 -0.207379889034675
29 -0.201288447413722
30 -0.201388129940391
31 -0.23673073929495
32 -0.223538269660198
33 -0.218154812724554
34 -0.247787212932488
35 -0.251581608118471
36 -0.235792243029587
37 -0.241957665030248
38 -0.250735808071197
39 -0.261145699321074
40 -0.275597516293742
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0332471027061603
1 0.0708137139343439
2 0.201555320664488
3 0.215063961409924
4 0.175535882284474
5 0.0163841713422039
6 -0.0890539996442801
7 -0.136562426344478
8 -0.168954341099699
9 -0.175534855199587
10 -0.153808148347674
11 -0.191028456017269
12 -0.0899262256369919
13 -0.0165947354678542
14 0.0254752049558968
15 0.0571026188411698
16 0.0932345762804827
17 0.104088482255192
18 0.136258975568282
19 0.142760151031707
20 0.178733602392358
21 0.204187983642401
22 0.278932077475551
23 0.406759457885228
24 0.476083074217942
25 0.539915963459621
26 0.608710407822518
27 0.744687016812827
28 0.823201523687707
29 0.871490468668204
30 0.928475065307045
31 1.04240851864272
32 1.14518144051824
33 1.20239244341795
34 1.3397694275739
35 1.44311946250859
36 1.50568091990005
37 1.5634007417843
38 1.65998119553749
39 1.72154848585435
40 1.78712010968577
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0295095526280935
1 0.0850060715223044
2 0.231816279459165
3 0.24015603315472
4 0.183300295805995
5 0.0669515808283778
6 -0.0599704198591056
7 -0.160400458220644
8 -0.203227492575272
9 -0.222745361833701
10 -0.217151657263773
11 -0.233936240556779
12 -0.183123094105876
13 -0.121062160593628
14 -0.0871888237443503
15 -0.03101476989979
16 0.0105793176189062
17 0.0317758308020641
18 0.057031911326308
19 0.0805170703751426
20 0.09947815586718
21 0.115187533167281
22 0.138641939777478
23 0.153430716244276
24 0.204388113100391
25 0.419360064017128
26 0.626882739118892
27 0.825118553219324
28 0.959099736127184
29 1.12404548998361
30 1.23143972981779
31 1.33037326430502
32 1.43823573582664
33 1.55039120477406
34 1.64140828718775
35 1.72526463508598
36 1.7908506041087
37 1.85669405978576
38 1.9454543882703
39 2.04860899389563
40 2.12201846320634
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0252034430664283
1 0.0579629537083655
2 0.17055610286992
3 0.245121362218958
4 0.205647699569429
5 0.102247843635298
6 -0.0115722364470674
7 -0.0853746532148758
8 -0.145387948112169
9 -0.221627363595374
10 -0.306405074608438
11 -0.392162258848503
12 -0.360829617414661
13 -0.305469998047644
14 -0.270898415020507
15 -0.259272320376084
16 -0.276350853263358
17 -0.289770856398459
18 -0.27212097691547
19 -0.244312420021839
20 -0.234032573472591
21 -0.179847239179024
22 -0.190178453058848
23 -0.139948290741512
24 -0.159428608389504
25 -0.140436393220869
26 -0.11053461954544
27 -0.0646217815887269
28 -0.0205352491418642
29 0.102504489797756
30 0.215187431408643
31 0.320736973788724
32 0.444934086470718
33 0.548634557013183
34 0.686709192579213
35 0.822000869171616
36 0.896844799226247
37 0.985123934824919
38 1.08570816628611
39 1.17496271630065
40 1.2382382125279
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0235157135852448
1 0.0717545165453997
2 0.203221512363271
3 0.236444280736209
4 0.183121988291007
5 0.0459418875375102
6 -0.0842794765090673
7 -0.190847551552612
8 -0.250944070072082
9 -0.247212650709496
10 -0.279153604348187
11 -0.314014511355628
12 -0.329602203179874
13 -0.259784481642832
14 -0.195506598766885
15 -0.156882841850731
16 -0.160887377259443
17 -0.161470454139986
18 -0.157546870634947
19 -0.164886302534952
20 -0.147881221350598
21 -0.140426813833519
22 -0.144542374276807
23 -0.12388386406325
24 -0.148991718028062
25 -0.147470290643732
26 -0.148935872077021
27 -0.16278174809092
28 -0.149004419675415
29 -0.150970423696589
30 -0.153176517123992
31 -0.15038297342979
32 -0.160515086510131
33 -0.146872877627029
34 -0.161068531917693
35 -0.176196799339104
36 -0.160641169198041
37 -0.171562143399264
38 -0.174778076712114
39 -0.177488294490064
40 -0.191540797413738
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0239622030608775
1 0.065761432635262
2 0.177689160884456
3 0.217049381163565
4 0.187617099088764
5 0.100510524619459
6 -0.00385582935452256
7 -0.0327259631199226
8 -0.0912775548010654
9 -0.167457654482794
10 -0.202891325877493
11 -0.218730968257995
12 -0.133656235936503
13 -0.0783984703963565
14 -0.0426666887675902
15 -0.0240722056085687
16 0.00731667564874527
17 0.0134942879162461
18 0.00302220357821081
19 -0.0102257102705163
20 0.00187327957535466
21 0.0168019859566764
22 0.0109389860167859
23 0.0219999052434252
24 0.116463257544939
25 0.194964012524851
26 0.283405914731564
27 0.325211304902719
28 0.458625382496673
29 0.561963285747095
30 0.646056238022226
31 0.762878213808297
32 0.824866186808408
33 0.839498024235603
34 0.87289962906102
35 0.915468956937251
36 0.89671995692634
37 0.902693381621193
38 0.898500217400934
39 0.911397190222703
40 0.91176092829052
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0227158076685328
1 0.0988356315543513
2 0.218841825947442
3 0.22239776569327
4 0.168366599586515
5 0.0413348770938509
6 -0.0651326162107679
7 -0.120902953829673
8 -0.192788796311214
9 -0.260082194116959
10 -0.316648335247746
11 -0.40061781434492
12 -0.37915468321891
13 -0.279017243691424
14 -0.226267176463223
15 -0.209924876058104
16 -0.143164581759704
17 -0.0925705457018422
18 -0.053761269697481
19 -0.0562257316677721
20 -0.0598216846177921
21 -0.0428851806211572
22 -0.0508857498029158
23 -0.0653421668842151
24 -0.0745715350471743
25 -0.0887824327615521
26 -0.0839113413057735
27 -0.0922025159463491
28 -0.0939289511822459
29 -0.115838628899455
30 -0.16133015841001
31 -0.160226707901379
32 -0.179242469584021
33 -0.224076828172746
34 -0.235211589885012
35 -0.238302821556619
36 -0.288387350419473
37 -0.308527844306708
38 -0.336327347674573
39 -0.356692552154402
40 -0.379622274282235
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0254259582198149
1 0.0767195091617054
2 0.18985548909066
3 0.23356163161071
4 0.204049251216635
5 0.0940094519110568
6 -0.0216062563584734
7 -0.0959859342679197
8 -0.155204395983915
9 -0.184823839570015
10 -0.214680920825
11 -0.205651060950348
12 -0.0955256792174906
13 -0.0109058707977265
14 0.025244388181993
15 0.0356710007754701
16 0.0788801037144511
17 0.10356715941436
18 0.138669921852819
19 0.171246979772084
20 0.182208300029993
21 0.21221029947333
22 0.230602979021382
23 0.243837920952112
24 0.256613946820146
25 0.269177643367489
26 0.287039058498874
27 0.292098161569145
28 0.329231273276469
29 0.412721345701312
30 0.508810890514726
31 0.63276158886817
32 0.806483305733982
33 0.964016644595216
34 1.11724613773964
35 1.25603587639831
36 1.41131215479199
37 1.57849925804389
38 1.74037241167065
39 1.89785849051337
40 2.03166938123993
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0288361373397672
1 0.062429668231494
2 0.192712207415959
3 0.200192684761547
4 0.161510663194054
5 0.0425387555568486
6 -0.105895492781326
7 -0.220703057150216
8 -0.271737298110766
9 -0.315002422630673
10 -0.318017305966706
11 -0.326202278939592
12 -0.257589914601423
13 -0.17787050970801
14 -0.125585245741363
15 -0.0747364910296815
16 -0.0581352475991066
17 -0.0372180016011772
18 -0.0434917732699835
19 -0.0344871107215079
20 -0.00695990986574646
21 0.00923740267444817
22 0.0378281359135428
23 0.090026130845045
24 0.131052428357313
25 0.223362697374518
26 0.361011211642467
27 0.394761184360044
28 0.473240992898154
29 0.508869525337731
30 0.532791475177267
31 0.529182931047325
32 0.560804838136405
33 0.583742303935581
34 0.606848224707345
35 0.664125528558151
36 0.699514146568362
37 0.712045853553291
38 0.736059567237746
39 0.733606213925259
40 0.716984512168725
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0202697745827507
1 0.0870311619464612
2 0.179489229506931
3 0.149567950337135
4 0.105018211069253
5 -0.00916171186696246
6 -0.115773731238889
7 -0.206715403965389
8 -0.262673475194576
9 -0.296387601158908
10 -0.311491973103534
11 -0.375667556832987
12 -0.301177324651503
13 -0.211363043598848
14 -0.210466929630929
15 -0.203305816894471
16 -0.193507087727448
17 -0.212677057663094
18 -0.204576003467042
19 -0.190409736070518
20 -0.193344783729594
21 -0.200074166114552
22 -0.201624531318148
23 -0.180348451540314
24 -0.211143952881807
25 -0.228057842016668
26 -0.215985394272081
27 -0.199165733684728
28 -0.177795385624287
29 -0.180715209605484
30 -0.148659792150394
31 -0.127538376648926
32 -0.0500697058828461
33 0.038526422381187
34 0.173033202285326
35 0.314868329006482
36 0.44351708630609
37 0.531796928788586
38 0.599675163337018
39 0.698469527920722
40 0.787056871095592
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0335410912574696
1 0.0486595424212464
2 0.164090651138593
3 0.192197716082027
4 0.171395756375308
5 0.0370594109329598
6 -0.0815195452617354
7 -0.158840476456821
8 -0.20552261819207
9 -0.238276811189174
10 -0.301544522401741
11 -0.367431266547112
12 -0.313928818526828
13 -0.272440573776547
14 -0.234923572324981
15 -0.193052017048351
16 -0.15354642656261
17 -0.127918870137075
18 -0.0954089456353762
19 -0.0838551136491326
20 -0.050216952867685
21 0.0084350027839859
22 0.0769276906998995
23 0.172013787726583
24 0.264167028094882
25 0.332073160221769
26 0.452428380530944
27 0.510433379065231
28 0.660466626697453
29 0.738453827830657
30 0.808486788740789
31 0.851368832344427
32 0.906851403130487
33 0.990645300503292
34 1.03364153434319
35 1.07340772040531
36 1.08780249762355
37 1.06667952028682
38 1.07350740959848
39 1.09024560600507
40 1.1211254920932
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0274064477897316
1 0.0762405142573384
2 0.190252559649687
3 0.205095082203748
4 0.164010280725252
5 0.0727875324545577
6 -0.057261843682598
7 -0.157998189786444
8 -0.185149198913959
9 -0.211631299113494
10 -0.276465030426519
11 -0.324846089391085
12 -0.272897721007032
13 -0.202330783492056
14 -0.176425116186588
15 -0.135015225867851
16 -0.13704379054391
17 -0.100199538552563
18 -0.0725879368444549
19 -0.0378287009587837
20 -0.0321806172528563
21 0.0216677839022719
22 0.0493494373813288
23 0.0767024120112767
24 0.107338549227768
25 0.104912105025261
26 0.116923764440776
27 0.146550793767826
28 0.257180072398459
29 0.354281512826703
30 0.438990224078583
31 0.517228472786046
32 0.603739443528795
33 0.731756989527273
34 0.847714419593515
35 0.970930675332381
36 1.06659877475778
37 1.17267012899031
38 1.33385153490308
39 1.45060795517784
40 1.60855017371274
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.022920541275397
1 0.0797897215474306
2 0.20724321445403
3 0.152182587694434
4 0.0801911220712865
5 -0.0477292580195892
6 -0.164392968934977
7 -0.236087471887761
8 -0.276351043416641
9 -0.337809641729288
10 -0.405437562631178
11 -0.463709262618152
12 -0.391506712654203
13 -0.323903825080579
14 -0.273306576630659
15 -0.21242738822121
16 -0.18515824872322
17 -0.162687825139709
18 -0.154238772153057
19 -0.167374456973437
20 -0.163791933445236
21 -0.15827431930761
22 -0.157758938918087
23 -0.167271230933543
24 -0.163135891580356
25 -0.175432516120747
26 -0.156564900192081
27 -0.0821926434520934
28 -0.0394898187869819
29 0.0420005394410499
30 0.118105998108008
31 0.19072420125211
32 0.254583793533455
33 0.308711510324288
34 0.313717002531891
35 0.319633433779249
36 0.377283595566193
37 0.421143218342471
38 0.48153869107293
39 0.512701067353569
40 0.572099245551931
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0260517131503377
1 0.0744295190937878
2 0.182121237048591
3 0.239529702186112
4 0.224184161066406
5 0.108237284957908
6 -0.0127139036334984
7 -0.0604054575743769
8 -0.108247050451233
9 -0.140694465713698
10 -0.140737379504985
11 -0.201834610608362
12 -0.0921503338093288
13 -0.0055370784160047
14 0.0702117107804261
15 0.106859163728501
16 0.123023076060019
17 0.133248373893077
18 0.1612066278997
19 0.208423337780608
20 0.269529527794156
21 0.379283206434494
22 0.478510336963208
23 0.541714308367952
24 0.544498375746425
25 0.58116535162449
26 0.616563016634812
27 0.645904158070181
28 0.658426383058091
29 0.660078483326337
30 0.648172922339334
31 0.670953444288931
32 0.691033350020968
33 0.697219552726339
34 0.724287949177475
35 0.762692544351835
36 0.789953948299264
37 0.783939225151331
38 0.766515030412356
39 0.748851753616609
40 0.736829455249611
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0285270737279237
1 0.102487157247513
2 0.234428178632862
3 0.271284738970803
4 0.231176636284356
5 0.0804653971270621
6 -0.0422914854048351
7 -0.146623561955087
8 -0.242369018985959
9 -0.318676802593382
10 -0.321155884211771
11 -0.323484941590272
12 -0.223727865567892
13 -0.174549445244518
14 -0.113544735811899
15 -0.065844324102823
16 -0.0662704897864614
17 -0.0556880565728655
18 -0.0470518903244947
19 -0.0325429405151825
20 -0.0293597614493839
21 -0.00493304452377075
22 -0.0033136471584827
23 0.00994928617497592
24 0.0161580662221343
25 0.0184926833451273
26 0.0229494089984472
27 -0.00715829469639218
28 0.0259790174165628
29 0.0151209780775918
30 0.0906506490977224
31 0.134751728740587
32 0.197637356342981
33 0.253094349419023
34 0.300250263627274
35 0.330403442127663
36 0.359694819232192
37 0.380923280263994
38 0.379325616697718
39 0.410713324437727
40 0.439807424767452
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0264753735970045
1 0.0725877532097314
2 0.184945696573834
3 0.178224141829895
4 0.151975509534339
5 0.0287343258011106
6 -0.0887468313074278
7 -0.178967327237414
8 -0.260240584206409
9 -0.324812294041434
10 -0.340270712661147
11 -0.370849218933669
12 -0.296106586632938
13 -0.259604668623818
14 -0.204386408819376
15 -0.145285266087422
16 -0.142599687504378
17 -0.124829689886622
18 -0.117029686304377
19 -0.0985572726110755
20 -0.0789205526377934
21 -0.0537234443489778
22 -0.0479586711501314
23 -0.0377162386593008
24 -0.0308638700184094
25 -0.0154807607876508
26 0.00529432450885281
27 -0.00446892551242062
28 0.0193263487390931
29 0.0490822842498577
30 0.0861640694539423
31 0.0883488637515111
32 0.106043171980646
33 0.101657188976033
34 0.0963037939847569
35 0.125986721776274
36 0.142413629677137
37 0.169332357413541
38 0.18789007129882
39 0.208268046182377
40 0.22731734931729
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0196340044424934
1 0.0999627015495186
2 0.2120967513815
3 0.260048868568001
4 0.221453499143341
5 0.110017125228342
6 -0.0239040229384999
7 -0.0962277857686047
8 -0.172890792317975
9 -0.233348556241065
10 -0.262904589620907
11 -0.30148283178635
12 -0.285372834106589
13 -0.218713324488322
14 -0.163073289751233
15 -0.141714326578472
16 -0.153797736543685
17 -0.122872634019841
18 -0.103597641849114
19 -0.104816490310373
20 -0.0895485267346237
21 -0.10129217794766
22 -0.0913129322899922
23 -0.101089601817635
24 -0.0902313795186496
25 -0.064394094437084
26 -0.0597693118382834
27 -0.0401452544663741
28 -0.0176867327499588
29 -0.0378450683612463
30 -0.0676514226361089
31 -0.0173560977228178
32 -0.00544303199300611
33 0.025769254383909
34 0.032166859403616
35 0.067412806207555
36 0.164549222497981
37 0.230068262618834
38 0.261279201207626
39 0.288540923466761
40 0.315851896218205
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0213478686528275
1 0.0849827652411337
2 0.178820281056972
3 0.146257531182926
4 0.110540880701536
5 0.00367287523996662
6 -0.146619598706841
7 -0.258667869281731
8 -0.314015843758779
9 -0.326896427565989
10 -0.343811027885745
11 -0.441917804766597
12 -0.391537968680434
13 -0.335810863047576
14 -0.260865358204906
15 -0.224471368894385
16 -0.200003644658775
17 -0.15744385770606
18 -0.137862845238106
19 -0.126126139110528
20 -0.114216044695412
21 -0.0848542007219191
22 -0.0619276169744207
23 -0.050386275900463
24 -0.0384884533329615
25 -0.0428903018267892
26 -0.0251288036804507
27 -0.0314579128050765
28 -0.00514480562889208
29 -0.0167852347779043
30 -0.0198326588538862
31 -0.0081945129154386
32 0.000623565479391353
33 0.0230383205853713
34 0.0263474684518314
35 0.028729494950003
36 0.0449227006254977
37 0.0474569727953131
38 0.0284227043640373
39 0.0295722917216601
40 0.0167579349294051
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0173745015063345
1 0.0844205230020503
2 0.1959002809352
3 0.241415325597159
4 0.196211363092861
5 0.051379142794465
6 -0.0555996488142343
7 -0.104463012835518
8 -0.1649128568106
9 -0.236443632467224
10 -0.307714769773226
11 -0.335594601322047
12 -0.288969241903576
13 -0.192373148279652
14 -0.158498082225007
15 -0.099082549823053
16 -0.0964234898691609
17 -0.0805431711521347
18 -0.0784069847783098
19 -0.0846319790520882
20 -0.0926500696436943
21 -0.0858549266693505
22 -0.0982354952296305
23 -0.093039599776386
24 -0.113242000384068
25 -0.111095737389126
26 -0.114079116704876
27 -0.0971050945066922
28 -0.0924510543154042
29 -0.0819316420158014
30 -0.0937675805504128
31 -0.0807746610418247
32 -0.100987425553422
33 -0.0893015171604548
34 -0.0920185951744585
35 -0.0928938178675596
36 -0.0818970519192206
37 -0.0879209588249701
38 -0.0990606532557416
39 -0.119416433093263
40 -0.0987861643042667
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0266699211936539
1 0.0719279264267714
2 0.202395792133277
3 0.238716055222719
4 0.207194057442713
5 0.0951681413495624
6 -0.0272718343190057
7 -0.137273297182054
8 -0.227919527769458
9 -0.283241471294511
10 -0.35708160010538
11 -0.378075480554869
12 -0.284931766703665
13 -0.181825104996195
14 -0.116958786115703
15 -0.0453664706069068
16 -0.0242701617009873
17 -0.0357183298727755
18 -0.0185343270985321
19 0.000703684052227871
20 0.019058479825838
21 0.0511192654913168
22 0.0750202145249332
23 0.079936148758101
24 0.0836562674789141
25 0.153133984758726
26 0.179063832216335
27 0.197378069395527
28 0.294405060378931
29 0.412394814868972
30 0.564269419335051
31 0.720118106151084
32 0.867518363002833
33 0.989816539009042
34 1.08008374150678
35 1.14759874873137
36 1.22394013106539
37 1.28179327165001
38 1.32712955721023
39 1.3775989033675
40 1.40467538054631
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0221618071228544
1 0.0935731297725617
2 0.227526957945866
3 0.24866460668076
4 0.195942607775278
5 0.0573204150570676
6 -0.0779141169147115
7 -0.208391495055423
8 -0.293318922185322
9 -0.28481076695544
10 -0.276651149634022
11 -0.308938395913286
12 -0.252105209274332
13 -0.157718993087455
14 -0.134775364090951
15 -0.105654815995004
16 -0.0914685165614477
17 -0.0794463550542979
18 -0.0559853139504147
19 -0.0379283589034483
20 -0.0124482720046766
21 0.0240428782443214
22 0.0460983693525101
23 0.0644020175136131
24 0.0815224649984643
25 0.176001983551807
26 0.242270237155427
27 0.305261139136001
28 0.40912158000329
29 0.481933708859089
30 0.619003356742731
31 0.704815258554053
32 0.823984484639674
33 0.936247426439998
34 1.02031718757898
35 1.13371049344028
36 1.2015033311178
37 1.27358179443562
38 1.31063481867725
39 1.34844630491074
40 1.3868083183633
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0243940016217019
1 0.0731551641045067
2 0.208402526115235
3 0.188200662124661
4 0.170091408264391
5 0.0466554666163015
6 -0.0867420971170647
7 -0.177463471172224
8 -0.253175604928583
9 -0.309473562288393
10 -0.346249511444814
11 -0.399151107076424
12 -0.301114718416138
13 -0.22065936000858
14 -0.18429156702424
15 -0.143889329801755
16 -0.151248511248967
17 -0.181427811353494
18 -0.187207394708692
19 -0.184787630137472
20 -0.163488364183986
21 -0.153925097083137
22 -0.151353259964112
23 -0.148943915277192
24 -0.119756362699648
25 -0.0955624614339827
26 -0.0652189032683284
27 -0.028376232291806
28 0.0736989174444549
29 0.174664366117763
30 0.331621321689346
31 0.459122435476623
32 0.587010052995553
33 0.705196677353589
34 0.819329226217289
35 0.883761351342332
36 0.976403782769019
37 1.07089342641405
38 1.17381779816866
39 1.27051800202538
40 1.37964158634971
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0333761916754831
1 0.0824879138670056
2 0.201482101455197
3 0.217711606943348
4 0.170589266970381
5 0.0626659439148556
6 -0.0885185624426663
7 -0.116526482542438
8 -0.167579534794395
9 -0.181715589611587
10 -0.154184094521194
11 -0.204683395221463
12 -0.142080994751119
13 -0.0105939317416217
14 0.0415517190168861
15 0.0611031416287924
16 0.0914821543001967
17 0.119754504181064
18 0.123892859706513
19 0.14605557342863
20 0.137396498451997
21 0.167307621029163
22 0.149950242458508
23 0.16215477484686
24 0.169359105884171
25 0.151519872165937
26 0.169080935327636
27 0.186807759556153
28 0.215177482170245
29 0.211458612103982
30 0.220487525527133
31 0.210195658712303
32 0.190913080852827
33 0.22421803561013
34 0.207002035023048
35 0.213840836327439
36 0.244855543718251
37 0.27049242785844
38 0.268235785187554
39 0.236632849105668
40 0.227784640289683
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0279118348345513
1 0.0643556973722736
2 0.178139701620292
3 0.170095779873863
4 0.135754736879654
5 0.00569006092324464
6 -0.0813756057048174
7 -0.173707210063228
8 -0.236348351201287
9 -0.271776950143784
10 -0.316032841083896
11 -0.306125063067868
12 -0.222089671151943
13 -0.130230810309432
14 -0.0305144082020883
15 0.0550437031221476
16 0.0872573630824194
17 0.0795131411859193
18 0.111363994566343
19 0.112087579548353
20 0.132052879482837
21 0.180626505862064
22 0.22287576179821
23 0.286112733759774
24 0.340647635236268
25 0.453296939090655
26 0.520307219743558
27 0.597310281110086
28 0.654599659248682
29 0.725741688417192
30 0.801883410121816
31 0.841182033187176
32 0.853074289486684
33 0.835384469022331
34 0.808782340335243
35 0.802746239331879
36 0.7846248542959
37 0.806224545307344
38 0.819130633089211
39 0.831418500570117
40 0.845692896284668
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0265037990171209
1 0.0719131755639673
2 0.189510913705214
3 0.189989949321467
4 0.152614342272076
5 -0.00226654250786051
6 -0.138771219981416
7 -0.174659760835794
8 -0.22583202680033
9 -0.269510316940309
10 -0.348444992630044
11 -0.359075768489746
12 -0.292604015868242
13 -0.210213361925746
14 -0.160971924862461
15 -0.126857214360024
16 -0.110342108044219
17 -0.103103413101034
18 -0.0754525723427797
19 -0.0642168192966786
20 -0.0413376498480567
21 -0.0412284412126862
22 -0.0132515908393023
23 0.0140596181396191
24 0.0321030115416621
25 0.0696721175454993
26 0.0895227307730817
27 0.122792484134915
28 0.192519059303362
29 0.225228661626715
30 0.327213748940464
31 0.438038617003429
32 0.518600394692201
33 0.581981460668319
34 0.609859802245019
35 0.689286662392799
36 0.745371727343572
37 0.77341440533311
38 0.79102695650488
39 0.830575271781187
40 0.888281633226073
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0293652764774341
1 0.0695887398541721
2 0.196902900040937
3 0.219275659375239
4 0.186233088921002
5 0.0687830772020588
6 -0.0511075535143251
7 -0.152353786540425
8 -0.256623493504261
9 -0.30326928128898
10 -0.341489704231256
11 -0.291382100873048
12 -0.203091505855489
13 -0.10828415345074
14 -0.0476946099757045
15 0.0593385912643223
16 0.0831929270870946
17 0.0963628246136032
18 0.143035702255583
19 0.143452382034536
20 0.164140527884924
21 0.188778297362295
22 0.173283321527826
23 0.24686765371346
24 0.298152112589579
25 0.320745024199341
26 0.388399652279796
27 0.465857278870933
28 0.567177665345147
29 0.657029123814629
30 0.738766502229243
31 0.803130244077193
32 0.853049938104109
33 0.857005594419726
34 0.868947161749793
35 0.856861597032231
36 0.852257685983806
37 0.825373784756065
38 0.834633512119345
39 0.817486786393319
40 0.789315070068475
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0305416290710543
1 0.0732549936670628
2 0.200108816249974
3 0.233865179096273
4 0.208951953102539
5 0.0702636216822246
6 -0.0666649945426316
7 -0.152187390796143
8 -0.165286023374829
9 -0.198806566113892
10 -0.266407301407336
11 -0.247088895616863
12 -0.171689783580174
13 -0.111577779606563
14 -0.0421676899927457
15 0.00313838962155533
16 0.00261043142739492
17 0.0310721387995576
18 0.032206954677843
19 0.0393849550368435
20 0.0404840453818078
21 0.0512866648378125
22 0.0548749238267279
23 0.0874233842927303
24 0.0759973321589476
25 0.102108129198232
26 0.147060480660978
27 0.228705679947982
28 0.331150395307968
29 0.412158374506975
30 0.526205512495366
31 0.691729300153638
32 0.794231802061408
33 0.93399404950107
34 1.04433469880787
35 1.14106036250994
36 1.24008333316677
37 1.35682912869827
38 1.45050853770314
39 1.55507784555428
40 1.67757514807284
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0181371215893886
1 0.0728384602654835
2 0.195503838092177
3 0.204478717631663
4 0.170272327117587
5 0.0461555054057046
6 -0.0991646603480545
7 -0.17846342530626
8 -0.223130414246759
9 -0.2578138521243
10 -0.315544250060678
11 -0.358367407244036
12 -0.322580315559541
13 -0.247216751534754
14 -0.184100511598184
15 -0.136680913896122
16 -0.121867486140577
17 -0.0907248177577085
18 -0.0832779959370926
19 -0.087829400893324
20 -0.0916213947192031
21 -0.0873892747130558
22 -0.10760297264324
23 -0.123690509915826
24 -0.13274295447795
25 -0.13335649340481
26 -0.146155430599649
27 -0.183756281666284
28 -0.180534864781095
29 -0.166783825896921
30 -0.159773249216587
31 -0.173779119685097
32 -0.210027831249731
33 -0.194210395488515
34 -0.218083464711494
35 -0.230293847130607
36 -0.236516196489895
37 -0.249614553624085
38 -0.266945725587277
39 -0.252043858133382
40 -0.270709385418661
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0360468359290733
1 0.0728858385016631
2 0.204644267490158
3 0.243255793969922
4 0.187951711699783
5 0.0290764411580327
6 -0.108664421579004
7 -0.188570352997237
8 -0.260280146862852
9 -0.344003386966455
10 -0.388742994503311
11 -0.398474534020157
12 -0.343008271424535
13 -0.278176082125952
14 -0.27519403218062
15 -0.272529679694347
16 -0.251447237071772
17 -0.23346317622022
18 -0.194959153088246
19 -0.177599496403703
20 -0.196329148164664
21 -0.189122046976886
22 -0.177768149838291
23 -0.126886286180015
24 -0.0378580389521757
25 0.0694123720537734
26 0.154297948021631
27 0.194121262756685
28 0.262614326210961
29 0.354182607164192
30 0.403202502340509
31 0.467264775074363
32 0.461433262036949
33 0.485542735146886
34 0.501363190722901
35 0.459589378993345
36 0.423143780265551
37 0.381715253291218
38 0.352594436832902
39 0.327331924912721
40 0.342160534944278
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0284441463083125
1 0.0742709412581348
2 0.158737352411867
3 0.1445250324805
4 0.0960166358316616
5 -0.00233912464433317
6 -0.124424169273568
7 -0.235479414668984
8 -0.323073442390398
9 -0.385879000172452
10 -0.401484899359692
11 -0.453323444585291
12 -0.39130022673235
13 -0.328836094388969
14 -0.263031366106916
15 -0.219115160857101
16 -0.207151098817731
17 -0.195313756783241
18 -0.178164820803753
19 -0.161307443532878
20 -0.156086923581295
21 -0.142073227892106
22 -0.126209429550304
23 -0.101759732291775
24 -0.09262541897834
25 -0.0842973142014909
26 -0.0661519914890496
27 -0.0445446367473137
28 0.0782705988977934
29 0.174053860226495
30 0.256644614479146
31 0.315289910996674
32 0.371544418145899
33 0.440210667441439
34 0.494501745452327
35 0.559188122654082
36 0.634961977618948
37 0.700259279782405
38 0.775492358823894
39 0.850269864626144
40 0.907873060102717
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0233834065336502
1 0.0729925048057272
2 0.207362521640968
3 0.227583461186533
4 0.181947757961029
5 0.0503789175135916
6 -0.0731496179948365
7 -0.131861518114713
8 -0.171172450125672
9 -0.199759758273286
10 -0.2246431728053
11 -0.25880565139239
12 -0.295254482573584
13 -0.233691027373961
14 -0.220595220571837
15 -0.195209244417646
16 -0.151048385349545
17 -0.120925940979485
18 -0.104427661517034
19 -0.0814852200552698
20 -0.081757106244007
21 -0.0672674145926422
22 -0.0484081940617997
23 -0.0434882946693165
24 -0.0327638640073404
25 -0.0154608068228317
26 3.69932746302482e-06
27 0.0209695232242826
28 0.0202019622016012
29 0.0366879186790516
30 0.0481754046487524
31 0.0570213958924697
32 0.0544313710488353
33 0.0474725445770581
34 0.0742887377991606
35 0.0745447802872379
36 0.085545285970559
37 0.127937679899051
38 0.156313514221176
39 0.164125770227989
40 0.189204723146916
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0295925697148123
1 0.072107184159532
2 0.175311613407121
3 0.19329247199493
4 0.179158481338621
5 0.0436151712266613
6 -0.0767894934324467
7 -0.196070918407303
8 -0.275180915918841
9 -0.29192579235453
10 -0.337504234837993
11 -0.378855769065878
12 -0.321471659427021
13 -0.267009634495933
14 -0.204135283419182
15 -0.176843275707533
16 -0.164036056820685
17 -0.150425503333631
18 -0.131151325693613
19 -0.119565377207769
20 -0.116894896086934
21 -0.138204636173476
22 -0.135127708725045
23 -0.121180269314531
24 -0.0815929834975098
25 -0.0348227302958541
26 0.0665143672155537
27 0.177802446947571
28 0.256143565461246
29 0.3729351630615
30 0.453659463507056
31 0.537564746971315
32 0.629127594472253
33 0.723087309206752
34 0.793662288602178
35 0.88041645701924
36 0.931268965348295
37 0.960733107333517
38 0.973109389147127
39 0.985144699033392
40 1.00984219408063
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0292544693040062
1 0.0718092160659323
2 0.178333655404885
3 0.196511551637508
4 0.181347305323925
5 0.0263309194067007
6 -0.0772252733815995
7 -0.163900159940805
8 -0.227890455556849
9 -0.28188379836225
10 -0.338150097107844
11 -0.372045744187925
12 -0.309354404988734
13 -0.237339439271167
14 -0.219781670895618
15 -0.159900361701308
16 -0.169843192085454
17 -0.176272507249939
18 -0.162772434084462
19 -0.1546279518433
20 -0.154437090066001
21 -0.143483190241089
22 -0.111327941990004
23 -0.0837651702550675
24 -0.0701412736574873
25 -0.0411428779452176
26 -0.00186192968912646
27 0.101172027762423
28 0.221891461743795
29 0.363424921713339
30 0.455025582297234
31 0.577807561916188
32 0.662930837773687
33 0.730947670962373
34 0.856465398356618
35 0.977418988360625
36 1.12304312982037
37 1.26816908152786
38 1.4203406474342
39 1.55948983664138
40 1.687759704985
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0231104661428976
1 0.0975308015647913
2 0.237005646991283
3 0.224377828417722
4 0.195948280541286
5 0.0838239897050883
6 -0.045148680597455
7 -0.119696362285926
8 -0.202678310698597
9 -0.262598872443743
10 -0.269124611182763
11 -0.244655677042147
12 -0.168351679881637
13 -0.0709636912257894
14 0.0122549704451131
15 0.0551285482703046
16 0.0710270336007595
17 0.102999748783633
18 0.144669057748238
19 0.174714030693504
20 0.182234739218788
21 0.239372256470322
22 0.250081504082847
23 0.289947902003839
24 0.342386274853516
25 0.405345552491611
26 0.504210397966072
27 0.552820622142755
28 0.680399433456834
29 0.80169115795215
30 0.870580125288294
31 0.892074016226596
32 0.946396229540512
33 1.00707400991323
34 1.06385772979772
35 1.12605657317717
36 1.1796544887304
37 1.2378280310559
38 1.294254563719
39 1.34704952875709
40 1.41478193854776
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0297783055672101
1 0.0771127813250212
2 0.161613283660777
3 0.159050057635356
4 0.0912106086806421
5 -0.0310020568458587
6 -0.135347214711515
7 -0.170520656920197
8 -0.235079807616268
9 -0.273780111273814
10 -0.281102517941057
11 -0.296945666302787
12 -0.201941837002174
13 -0.134587422672719
14 -0.0989212356220479
15 -0.0432396274933549
16 0.000899142107559037
17 0.0368973433237043
18 0.0888355429456427
19 0.133766199490235
20 0.154467945299758
21 0.17703719517022
22 0.252754140277236
23 0.321324348407481
24 0.365105298337077
25 0.462230825423219
26 0.495605882073179
27 0.498848579574931
28 0.550984950785364
29 0.601377889586719
30 0.635538569855946
31 0.693659054908382
32 0.736255600979674
33 0.7880421716535
34 0.852881038057059
35 0.905229473129478
36 0.935270062218486
37 0.991142400761017
38 1.04682207743507
39 1.09490514011269
40 1.14558064209496
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0252174219888737
1 0.0931210526238653
2 0.219297532948674
3 0.20163307972613
4 0.173075686319328
5 0.0520187222279986
6 -0.0730435010619939
7 -0.178230733145103
8 -0.215684366378969
9 -0.233803040713521
10 -0.266466729375789
11 -0.361899834661272
12 -0.260372139026046
13 -0.16704121530198
14 -0.109359548858048
15 -0.0615026743195273
16 -0.0397993889707369
17 -0.0136817777215397
18 -0.00681279118433586
19 0.00649440268403279
20 0.016866717372511
21 0.0364535188473871
22 0.084551945511361
23 0.130137229087026
24 0.170740462338385
25 0.275825840933706
26 0.362843745774057
27 0.430724290921538
28 0.482757581930981
29 0.474608471165169
30 0.482185090477826
31 0.485789102983348
32 0.464046241704222
33 0.423007868999653
34 0.357538885889419
35 0.304285469609
36 0.232945786808298
37 0.155307072657576
38 0.0621107287702127
39 -0.00358238028766245
40 -0.0766486403432785
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0289776524155956
1 0.0724634079749995
2 0.230947006495338
3 0.224396464969121
4 0.17014047202257
5 0.0490839153036111
6 -0.0513704194812146
7 -0.118718296021409
8 -0.193509600112693
9 -0.20856762223073
10 -0.236157496153453
11 -0.302691343987694
12 -0.229648854025364
13 -0.158924651959856
14 -0.115048196358103
15 -0.0788503217415144
16 -0.0420584839289724
17 -0.0194184175628846
18 0.00874593989068817
19 0.0235887171988569
20 0.0248214666137558
21 0.0280383001665827
22 0.0529911394334661
23 0.0890832796300369
24 0.090995003027122
25 0.0826140884515647
26 0.082359072093432
27 0.068902473161093
28 0.126714923292664
29 0.173308297634194
30 0.217721604782583
31 0.303362077260743
32 0.335496656010347
33 0.395213823799651
34 0.5127101591828
35 0.675833936628069
36 0.816368628735048
37 0.918203663651248
38 1.0141476851993
39 1.10192162364491
40 1.1669387025892
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.024940720272296
1 0.0587665022662209
2 0.187732385840872
3 0.183202437956358
4 0.153129033066493
5 -0.00820846397364683
6 -0.116230638842523
7 -0.202383480366286
8 -0.258988715670819
9 -0.283369270502496
10 -0.32578221644693
11 -0.294959932601834
12 -0.250588948093051
13 -0.155837492569084
14 -0.110737964890347
15 -0.0290391850248861
16 -0.0351963806619553
17 -0.0320690235905792
18 -0.0174197737219988
19 -0.00664372437868099
20 -0.0335388682070468
21 -0.0495548630247669
22 -0.0386680780854194
23 -0.0244114054285847
24 -0.0705789508866363
25 -0.081233487185834
26 -0.0517260383389342
27 -0.0725539150064476
28 -0.0210889132418153
29 0.0167053506454069
30 0.0603361035178187
31 0.0558698383285092
32 0.0641480209530405
33 0.105987461134583
34 0.0950412920245016
35 0.0865057821962916
36 0.0998504056548741
37 0.105632126351582
38 0.113686974665708
39 0.0833421399988623
40 0.0791414384195104
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0312812331708461
1 0.0812591080839669
2 0.189818029996003
3 0.199813381421401
4 0.175491963321095
5 0.0704832828261592
6 -0.0431126745957222
7 -0.115758777562252
8 -0.187731411533625
9 -0.222404058724051
10 -0.23254865412042
11 -0.256513942300849
12 -0.190877788980741
13 -0.144736612349198
14 -0.122346525098207
15 -0.0899895649936662
16 -0.0620037987675346
17 -0.0268878784339792
18 -0.0257325007201805
19 0.00650246990995296
20 0.00825053146116339
21 0.0422818918026993
22 0.0335285942457837
23 0.0446396874175949
24 0.0333287488013525
25 0.0343316297875251
26 0.0537864785958782
27 0.0430616935884878
28 0.0712831559156584
29 0.0772296635869152
30 0.079603463556845
31 0.0504152635074453
32 0.0331214215927318
33 0.0485894607111828
34 0.031278397869297
35 0.0106027340550803
36 0.0285845420590229
37 0.0383562844039576
38 0.0200464809320371
39 0.000140165750099008
40 0.0130566324821775
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0235139809302822
1 0.0633085613891708
2 0.178604731225999
3 0.159807471648136
4 0.112077517135122
5 -0.0192880522166874
6 -0.124489846819835
7 -0.221962617610433
8 -0.295289956182313
9 -0.35619018529032
10 -0.416738302486904
11 -0.502648704112927
12 -0.467807850718969
13 -0.414609516595708
14 -0.369768564207122
15 -0.314471808999898
16 -0.301651017640213
17 -0.301253144759211
18 -0.288066521527297
19 -0.292380793045761
20 -0.272918308936239
21 -0.276677372824567
22 -0.256282104104423
23 -0.263098225037595
24 -0.219167048732118
25 -0.217576320302788
26 -0.216986948800112
27 -0.181720763374378
28 -0.190560837758
29 -0.153700990498703
30 -0.147421514284698
31 -0.107357982309668
32 -0.0105971965306741
33 0.114640572044452
34 0.198215722368687
35 0.275748953272259
36 0.373988864147762
37 0.469282138323064
38 0.549824340842539
39 0.624157566624182
40 0.690242667369341
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0306743126530034
1 0.0956060803892136
2 0.217526919839647
3 0.273425106902045
4 0.235091615045548
5 0.101698644332652
6 -0.0430868916177136
7 -0.1419799259317
8 -0.194677497377806
9 -0.230633965421625
10 -0.22752338672362
11 -0.275954075463666
12 -0.17918530909472
13 -0.0971599258781142
14 -0.0437826513439745
15 0.00380478970590126
16 0.0192252836873168
17 0.0199164912515197
18 0.0458829089959112
19 0.0595187537657917
20 0.0624019092703199
21 0.0777938494682688
22 0.0873937283499169
23 0.0851736503867917
24 0.104568230152645
25 0.133885773994998
26 0.136937508669891
27 0.192833934492
28 0.261968866510368
29 0.36392070587498
30 0.511305582688604
31 0.70224401793554
32 0.842115141467785
33 0.945475754763862
34 1.11209486612514
35 1.2216576594608
36 1.31731171027203
37 1.40467217050167
38 1.48382896387025
39 1.53662006243832
40 1.57430387696038
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0375324278255755
1 0.0581658909551566
2 0.146473754145563
3 0.147778089137196
4 0.0985292590363755
5 0.0120612273843737
6 -0.0913408654800802
7 -0.164521006492073
8 -0.229741673657945
9 -0.292447412070035
10 -0.353040067905782
11 -0.410264936466755
12 -0.346868355853183
13 -0.257759177518097
14 -0.233454936258951
15 -0.183010620173041
16 -0.131390402577131
17 -0.0667903607794429
18 -0.0486137681887087
19 -0.0390715678448643
20 -0.0223533232869206
21 -0.00808227491803759
22 -0.00215273628728774
23 0.0318572710879126
24 0.0144001882940774
25 0.041757072596881
26 0.0943020282169815
27 0.177342158243254
28 0.291501480257866
29 0.458633958743916
30 0.615849521827465
31 0.770053029251843
32 0.930355127768856
33 1.07877335101387
34 1.21328996685389
35 1.36251067379243
36 1.54539151917112
37 1.71444551385657
38 1.87038672053419
39 2.06019535550786
40 2.23782505513367
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0191188184677165
1 0.0624559881694271
2 0.167997157283629
3 0.183762123626697
4 0.119166229689649
5 -0.0108941531412432
6 -0.123161468398338
7 -0.166030107162113
8 -0.233147722082178
9 -0.264809902349139
10 -0.344060827587129
11 -0.363278832064427
12 -0.377448685770273
13 -0.302681558073198
14 -0.280729635144993
15 -0.261846257215616
16 -0.264241124925873
17 -0.279429764473106
18 -0.24680934596727
19 -0.229314884638287
20 -0.237822250468487
21 -0.224909004307435
22 -0.240282442570576
23 -0.254082843293194
24 -0.273032919755671
25 -0.308519508735153
26 -0.354354383501758
27 -0.377925721596032
28 -0.386131478942089
29 -0.412092441737995
30 -0.449998993470068
31 -0.47666675497044
32 -0.497993149482295
33 -0.516685197415653
34 -0.522670161372057
35 -0.50330403863015
36 -0.501206663849163
37 -0.48401862905007
38 -0.466821561749978
39 -0.460925869977335
40 -0.44872244708828
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0238235238292033
1 0.0828080284208204
2 0.189679569445845
3 0.163388890479369
4 0.152903325982337
5 0.0150518647115527
6 -0.098357213496401
7 -0.191636219456795
8 -0.225758386989181
9 -0.275967497508905
10 -0.327261245994132
11 -0.365347026626052
12 -0.254465817286021
13 -0.160125661636714
14 -0.14701968294088
15 -0.13423346878731
16 -0.137254702682796
17 -0.167988234036622
18 -0.157028896156688
19 -0.151377748903836
20 -0.10685639969987
21 -0.0279243598507808
22 0.0741970429271079
23 0.182412596344413
24 0.311727840114292
25 0.4180207557024
26 0.542743274842892
27 0.655236341184882
28 0.798236400866166
29 0.936723104370173
30 1.11649993602771
31 1.26370868640653
32 1.41488663171214
33 1.57490848103791
34 1.74703343921962
35 1.94699389565944
36 2.14552734501602
37 2.33826968410941
38 2.52555160781941
39 2.71015276913358
40 2.88366190047837
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0371202969903708
1 0.0643801921104705
2 0.187736975309017
3 0.209180882276258
4 0.190069948602177
5 0.0585622993611388
6 -0.0657803861019
7 -0.136841417760592
8 -0.190111802189908
9 -0.259149988219145
10 -0.317657020903887
11 -0.357185189503205
12 -0.26902921203207
13 -0.213942539153765
14 -0.181117625565815
15 -0.131508907418568
16 -0.0883649506670441
17 -0.0842550707553853
18 -0.021995326952152
19 0.016309612034223
20 0.0276344036701159
21 0.101802413193133
22 0.139375971054442
23 0.22649402786901
24 0.303877145106831
25 0.435024846217481
26 0.555825366634152
27 0.62671665528711
28 0.725029567449801
29 0.846513117182916
30 0.923391680040515
31 1.02715682132714
32 1.11436796482514
33 1.16045420967699
34 1.24925459275259
35 1.30908731379235
36 1.33723631195291
37 1.38868042129911
38 1.42803682948209
39 1.45342631668473
40 1.46524658455566
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0243165145280662
1 0.0611981522981111
2 0.163806600555231
3 0.166973348350138
4 0.0990312875085495
5 -0.0184683281440856
6 -0.122111553226714
7 -0.211605317677544
8 -0.247041126989248
9 -0.296163323603857
10 -0.294439695998771
11 -0.329312130300007
12 -0.283916197410241
13 -0.235112547776498
14 -0.197909466712449
15 -0.169573653184989
16 -0.135608392880214
17 -0.125581449004616
18 -0.0878968260047932
19 -0.0608507160035696
20 -0.0351098036283224
21 -0.0227180977998342
22 -0.0246429670545272
23 0.034924389141703
24 0.0929079960454811
25 0.205118107029893
26 0.321401913784758
27 0.392890734347698
28 0.516727054804147
29 0.604398766181828
30 0.686555909124849
31 0.766701698957613
32 0.81080957129824
33 0.852040634770534
34 0.928866492825843
35 0.972106465510552
36 1.02133368541095
37 1.05555312612267
38 1.08732260833058
39 1.14650302432582
40 1.16671934051528
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0305955005157665
1 0.064575331992156
2 0.197151455287153
3 0.196014082871298
4 0.166235414817734
5 0.0939730516324291
6 -0.0271373845868563
7 -0.118753001896608
8 -0.200480299653134
9 -0.220526326475368
10 -0.296290938856885
11 -0.360412568566881
12 -0.284122401892424
13 -0.232389243631018
14 -0.223173484834033
15 -0.153527442592745
16 -0.139495175813654
17 -0.128468086118249
18 -0.124757673861381
19 -0.121365131784565
20 -0.109997569434871
21 -0.0793086852212932
22 -0.0528097923114865
23 -0.0444151197845946
24 -0.0300594706336659
25 -0.0232183931640693
26 0.00445826449935804
27 0.0634797431246232
28 0.127767960217457
29 0.217982645571026
30 0.273653204186658
31 0.331157232830207
32 0.399900628491981
33 0.455487915630125
34 0.532900841758396
35 0.604132210581648
36 0.66424945887302
37 0.754633087939924
38 0.835426307334767
39 0.919326508129677
40 0.992574784232147
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.025127830962143
1 0.0673102322606853
2 0.180114090493843
3 0.183698004320937
4 0.159566468734357
5 0.010043661144028
6 -0.125401466388378
7 -0.200622557726692
8 -0.283781776673326
9 -0.347744780183939
10 -0.400340725588152
11 -0.40293032204455
12 -0.351183956371196
13 -0.278690358485344
14 -0.296630145311176
15 -0.293109541150968
16 -0.283777565583389
17 -0.268701573768017
18 -0.236488340161058
19 -0.227286931035234
20 -0.219036585357511
21 -0.187124680117498
22 -0.160096935425998
23 -0.142668462062103
24 -0.11853631156932
25 -0.0869694907089071
26 -0.060465481851927
27 -0.0114683596651339
28 -0.0225207254105086
29 0.0394688883850129
30 0.131590194596684
31 0.254263730660314
32 0.344960613858067
33 0.437417676804135
34 0.586683845722908
35 0.715708769556564
36 0.836012464238166
37 0.956412364352225
38 1.06092289825189
39 1.14291338872441
40 1.27922163218985
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0265674694707947
1 0.0778763859903417
2 0.166461301142648
3 0.195508177757021
4 0.17042723784783
5 0.0685547264645328
6 -0.062351573121024
7 -0.102866587480124
8 -0.180306876608237
9 -0.25005134643724
10 -0.287215124205225
11 -0.308566657298379
12 -0.228900164009073
13 -0.16056712266959
14 -0.140528698845697
15 -0.12322018560025
16 -0.0777725755614078
17 -0.0794566718183418
18 -0.0595190794474547
19 -0.0698465781934567
20 -0.0514351308534886
21 -0.0289135671185266
22 0.0388710144414341
23 0.13464573151302
24 0.253919790920699
25 0.373043308536944
26 0.437953316831563
27 0.522556545318968
28 0.567509284679114
29 0.57451696899142
30 0.611148862593473
31 0.607982658471175
32 0.620293020557149
33 0.664683961744559
34 0.661982807917918
35 0.665193124297343
36 0.705843432856438
37 0.714200309472106
38 0.704959364867622
39 0.684627560156605
40 0.677093753730911
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0299200013553858
1 0.0541767768034997
2 0.174580211253095
3 0.18032891280501
4 0.10086292041237
5 -0.0373063106219327
6 -0.14955633584074
7 -0.20678659646599
8 -0.260889568393329
9 -0.309323075245232
10 -0.359546736269768
11 -0.407533422949624
12 -0.318585428865394
13 -0.23480499740559
14 -0.2183041682138
15 -0.162963671686623
16 -0.147209297489144
17 -0.136815662724628
18 -0.104404724003542
19 -0.0813959485939479
20 -0.104835105106943
21 -0.0959942474334365
22 -0.0908638711628145
23 -0.0735386155767985
24 -0.0768046328562519
25 -0.0896200614561717
26 -0.0812906736481649
27 -0.0856968452141302
28 -0.0970960421492286
29 -0.0904714832102043
30 -0.0795417484023506
31 -0.0732167508538284
32 -0.062341160816378
33 -0.0608657130942074
34 -0.0424267203858859
35 -0.0387520002684241
36 -0.0432343207886801
37 -0.0479237288160643
38 -0.0382113297275657
39 -0.0366149618811917
40 -0.0336025590177371
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0183245873389346
1 0.0719666860670358
2 0.188613666209605
3 0.213135870903585
4 0.173867152430459
5 0.0747748941816049
6 -0.044463978043372
7 -0.114461501198801
8 -0.178522158569596
9 -0.212069679453431
10 -0.234082267015184
11 -0.273949486324654
12 -0.246238800484734
13 -0.188049607073258
14 -0.121174182956704
15 -0.0604187248056425
16 -0.0387645970774475
17 -0.0334642154035798
18 -0.0301481382797064
19 -0.0518796828983437
20 -0.0509241627692738
21 -0.0428712048885638
22 -0.045614586955895
23 -0.0464146028190919
24 -0.0666666528699915
25 -0.0695311004345482
26 -0.0674326769481057
27 -0.0740655360928493
28 -0.0516468667940391
29 -0.0411063822743296
30 -0.0346247989389239
31 -0.0719282376895789
32 -0.0587200633394449
33 -0.0524371844310707
34 -0.0655298420119239
35 -0.078969802040322
36 -0.0564101817936669
37 -0.0381829985135678
38 -0.0418561480471347
39 -0.0525477045847058
40 -0.0494289212168537
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0283804183820955
1 0.0607616223475294
2 0.188639205904806
3 0.189674490449671
4 0.138943368920096
5 0.0048548564443216
6 -0.116512663922591
7 -0.193205684059972
8 -0.24566497836554
9 -0.29742955854996
10 -0.363542524512458
11 -0.396302171985975
12 -0.313819964479931
13 -0.255450480690454
14 -0.247125247982399
15 -0.218822582625737
16 -0.179506637169069
17 -0.181600448399861
18 -0.156033447019689
19 -0.146353607489435
20 -0.134099385850011
21 -0.108903393618101
22 -0.105701449829447
23 -0.0964612809682519
24 -0.0971763358750408
25 -0.0832759342174869
26 -0.0777209600102884
27 -0.0633352517968477
28 -0.0695188659197168
29 -0.0540121095139385
30 -0.0584936389362696
31 -0.0757610387038712
32 -0.046595066204496
33 -0.0540902706738668
34 -0.0668841664666315
35 -0.051263441026979
36 -0.0211599027594938
37 -0.0121019302466401
38 0.0541172267524468
39 0.130250995795987
40 0.253806460431977
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0218221581998552
1 0.0709637372324812
2 0.175454236921126
3 0.12786731444271
4 0.0659456602113515
5 -0.0608925606828974
6 -0.184260155476174
7 -0.29981958621689
8 -0.374671414336035
9 -0.419554297690779
10 -0.450386699634806
11 -0.512399038927823
12 -0.453820092253546
13 -0.329081481625626
14 -0.317250815346536
15 -0.271123899411457
16 -0.270223666582941
17 -0.277317544134002
18 -0.239160554975276
19 -0.209928901345871
20 -0.209198798957535
21 -0.185907503216532
22 -0.183347807580538
23 -0.160333078193266
24 -0.141264689093886
25 -0.143580726574764
26 -0.131244854401385
27 -0.132893324604674
28 -0.0971074652341199
29 -0.10950766121594
30 -0.0602105562599533
31 -0.0264656852753378
32 0.0826383784025007
33 0.206815866546033
34 0.289494248546756
35 0.356257492263355
36 0.426984532098329
37 0.495129314070748
38 0.576897904428075
39 0.659996180194694
40 0.657780362641961
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.0337898232506255
1 0.0531562577804756
2 0.151742005210957
3 0.16632810521342
4 0.124074663981212
5 0.0077005188703243
6 -0.0918745731584441
7 -0.170638316342092
8 -0.219340517630594
9 -0.271572842888294
10 -0.269371684128043
11 -0.280313036738899
12 -0.185806435038379
13 -0.136070895059343
14 -0.0842354083478227
15 -0.0337381762430269
16 -0.0304451507621266
17 -0.00964765826759084
18 0.00601040843845624
19 0.0291270366602108
20 0.0198718268787719
21 0.0310310153672182
22 0.0479755934828612
23 0.134616053468046
24 0.23136334269302
25 0.337022153074622
26 0.487678393658556
27 0.579600582289691
28 0.713677347644684
29 0.810295070172975
30 0.91375129821534
31 0.99423296536173
32 1.05966451086859
33 1.15261536891646
34 1.19269639183983
35 1.25468030686386
36 1.3373827286679
37 1.37622121223065
38 1.42578690024121
39 1.47972441188378
40 1.49672549603876
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 -0.020796980169477
1 0.0594181887779079
2 0.16185784784373
3 0.175420507946209
4 0.126226017792606
5 0.00128163358790445
6 -0.111270259094127
7 -0.18071308365131
8 -0.23949425726974
9 -0.265364976696466
10 -0.318002223592566
11 -0.376870359929548
12 -0.298913770365318
13 -0.248492308907752
14 -0.208807135686788
15 -0.204414224273551
16 -0.186851367163144
17 -0.173470036861612
18 -0.152266408785956
19 -0.125716647208544
20 -0.145198157251906
21 -0.143575322968519
22 -0.164621363611214
23 -0.173145494683791
24 -0.184219523040851
25 -0.183335416477219
26 -0.195710738075986
27 -0.192035008146587
28 -0.164483616204326
29 -0.182236376070205
30 -0.173866385900372
31 -0.194225486064263
32 -0.202682952689066
33 -0.19181272079654
34 -0.19817786925364
35 -0.217950422213775
36 -0.219605139971639
37 -0.241615576402771
38 -0.256320160586539
39 -0.248120913139629
40 -0.262444034770305
};
\addplot [line width=0.01pt, color0, mark=*, mark size=2, mark options={solid, draw=black}]
table {%
1 0.0245940881197116
2 0.226498901996681
3 0.35963173094045
4 0.323192876348203
5 0.111448288247637
6 -0.15695204006051
7 -0.325976982807179
8 -0.334640765706954
9 -0.209549890955135
10 -0.205884173772729
11 -0.395618742668341
12 -0.404592842072073
13 -0.230511879468287
14 -0.055279679833161
15 -0.0210029805809502
16 -0.0164575411401979
17 -0.0161737318314269
18 -0.00358054162625767
19 -0.0104086468728599
20 0.0127963401693988
21 -0.00256627163803121
22 0.00694011005459992
23 -0.0244461075742605
24 -0.0236365740759628
25 -0.0484458903598396
26 -0.0156604557703324
27 0.0128490171223125
28 0.0437716443655508
29 0.03698016897091
30 0.0120928241581541
31 0.0180395493500055
32 -0.00624743566737794
33 -0.00866452893233261
34 -0.00937398036588012
35 -0.00916348210569427
36 -0.0019314931161561
37 -0.00552501045437327
38 -0.0230162558437155
39 0.0125317378882848
40 0.0372569376930346
};
\end{groupplot}

\begin{groupplot}[group style={group size=1 by 3}]
\nextgroupplot[
xshift=-8,
xmin=-1.95, xmax=40.95,
%ymin=-1.94544759152227, ymax=19.7889081638297,
ymin=-3.0, ymax=12.0,
width=\figurewidth,
height=\figureheight,
axis y line=right,
tick align=outside,
xtick pos=left,
ytick pos=right,
xtick={},
xticklabels={},
yticklabels={},
x grid style={lightgray!92.026143790849673!black},
y grid style={lightgray!92.026143790849673!black}
]
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.214353511237433
1 -0.106120958679399
2 -0.514886666446013
3 -0.784494422076315
4 -0.458568900625465
5 0.418987603775546
6 1.29425580016446
7 2.15266214860292
8 2.83749335775784
9 3.58950649504455
10 4.33172421434039
11 5.56484676738897
12 6.87251460206219
13 7.96207074582617
14 8.53281520833922
15 8.94355154612134
16 9.16326385098619
17 9.43704542285295
18 9.51399959608953
19 9.59917116336894
20 9.65794794279697
21 9.73160081362204
22 9.80589694741104
23 9.88333491752959
24 10.0504838709296
25 10.3806292559312
26 10.8121504266936
27 11.3912324023762
28 12.1961878500797
29 13.1496851781482
30 13.982159226331
31 14.6900880771247
32 15.3571225390803
33 15.9952074307237
34 16.5418728724477
35 17.0447206403823
36 17.4753311134475
37 17.9516955919955
38 18.38862828948
39 18.9009597328713
40 19.405533848429
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.179694738204016
1 -0.159811833207564
2 -0.626146637430736
3 -0.871845838177253
4 -0.565741199534712
5 0.318941556181334
6 1.26207369506822
7 2.1043875734365
8 2.91403189841685
9 3.95188829614418
10 4.99514458768816
11 6.50661379403488
12 7.60012586340457
13 8.50744338013964
14 8.92855718342585
15 9.22919787445356
16 9.42587848891101
17 9.57096823370509
18 9.8082619406941
19 10.0179381852087
20 10.290280326523
21 10.6219320439239
22 11.0403485587435
23 11.6418055147648
24 12.5141357066281
25 13.472148525893
26 14.4295321900207
27 15.2064088605786
28 15.9562990958531
29 16.6095613319064
30 17.2165250208649
31 17.898038392216
32 18.4012581321522
33 18.7858157723186
34 19.2946671227411
35 19.6862939986421
36 20.0378391593825
37 20.2733802179854
38 20.5280940449616
39 20.8089033083634
40 21.1181968176249
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.189560944150969
1 -0.109570913996144
2 -0.623671293853481
3 -0.872769345756064
4 -0.654718785328962
5 0.284991504199509
6 1.23149810805132
7 2.11629087348507
8 2.97861566222528
9 3.90334060875016
10 4.95969891225655
11 6.4219243301679
12 7.48135353148851
13 8.22238236776296
14 8.70826158019635
15 9.00795893534085
16 9.1552961834717
17 9.28350317289343
18 9.38306798456754
19 9.47244213685584
20 9.56339330588897
21 9.59846683261577
22 9.66533111473256
23 9.68450262233929
24 9.83266239952738
25 10.0711431230719
26 10.4125573152816
27 10.8941513577496
28 11.5673777099416
29 12.3941612338733
30 13.320350187884
31 14.1058396302248
32 14.8278142031582
33 15.5695032610732
34 16.0299029712487
35 16.5186442902611
36 16.8772875700227
37 17.0956585879808
38 17.3534125464686
39 17.6998585668438
40 17.9063253810408
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.207149139978249
1 -0.101860776363146
2 -0.574648851114327
3 -0.821327833586073
4 -0.50786614609583
5 0.282198476528142
6 1.1426568016751
7 1.95850971226141
8 2.70807243853783
9 3.54202368667761
10 4.40191376801562
11 5.83061421794754
12 7.02419033851473
13 7.9007330626685
14 8.4659562665759
15 8.7266041400506
16 8.84699184264332
17 8.99141514777294
18 9.03569194928757
19 9.06910708879801
20 9.12503849918548
21 9.15043963302563
22 9.17577553049077
23 9.14285084036781
24 9.17065499904154
25 9.25615208742209
26 9.24305814196917
27 9.33634748228397
28 9.35781997270826
29 9.30163554484934
30 9.24215169006138
31 9.29477137164483
32 9.27463604730942
33 9.22628128389811
34 9.22460063983272
35 9.29833770222027
36 9.29139572959872
37 9.27692036656174
38 9.22925681274818
39 9.26354991723157
40 9.35773780055502
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.202016639398289
1 -0.0867743265978973
2 -0.555615617816782
3 -0.888267524176522
4 -0.623343125278604
5 0.310375841559678
6 1.2823299602201
7 2.11524610478532
8 2.9320712552437
9 3.89359173032266
10 4.91361379080934
11 6.33732340983476
12 7.50246052033918
13 8.37847523488313
14 8.79616673041666
15 9.08676343911306
16 9.26450761595677
17 9.43555180997522
18 9.62635204940361
19 9.7706866187158
20 9.93166679839918
21 10.1621336094094
22 10.5190155665195
23 10.965294632222
24 11.6898716056939
25 12.6090788933652
26 13.5675139538339
27 14.3660185729917
28 15.0980340508179
29 15.7027519899079
30 16.3562004991521
31 16.9274461285258
32 17.4602666747103
33 17.9845607905854
34 18.432395133466
35 18.8432544727786
36 19.274522728942
37 19.6360431532522
38 19.9238383803532
39 20.2282562952715
40 20.4582971571021
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.234321667015435
1 -0.00311888577776287
2 -0.500160059600963
3 -0.824315891147323
4 -0.528336283553982
5 0.319872147897387
6 1.19037821197493
7 1.89527406304944
8 2.56172699670759
9 3.31972365769428
10 4.23301293258913
11 5.61915510588595
12 6.82809585585884
13 7.8267872007311
14 8.44426807645508
15 8.75862287127624
16 9.05798785460466
17 9.23987145491366
18 9.42641247479808
19 9.54184966117885
20 9.69432034386898
21 9.87301263894954
22 10.2696140542053
23 10.7139889781675
24 11.3086301213186
25 12.1727523235686
26 13.1096706535996
27 13.9331535296534
28 14.7357914419866
29 15.4517080130519
30 16.0123409101328
31 16.4093860327397
32 16.8054248128916
33 17.2392945102221
34 17.5637108881496
35 17.9286409025655
36 18.2744318557244
37 18.6783729770314
38 19.0587557286894
39 19.3774165073518
40 19.7607058020382
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.198424904273157
1 -0.0922941611829781
2 -0.513735875628107
3 -0.735271927352967
4 -0.436558219418445
5 0.505682536477218
6 1.31963788199619
7 2.11153060744045
8 2.9092903830344
9 3.81261639307951
10 4.7460141080914
11 6.08539355383017
12 7.16587723166719
13 8.06353977774892
14 8.59193017406098
15 8.90464899791076
16 9.02368272719464
17 9.25156276960359
18 9.31443695312028
19 9.33303803191565
20 9.28792924820968
21 9.31275490189205
22 9.29678177437423
23 9.28840078658099
24 9.23681232574217
25 9.19554094202329
26 9.19481151741759
27 9.2423341117416
28 9.20299996029695
29 9.20032977317584
30 9.06454866891326
31 8.97894680967272
32 8.9197047356992
33 8.92608363670155
34 8.90033313501122
35 8.81197100942379
36 8.82797907773306
37 8.76355606402885
38 8.69866950810274
39 8.66438180781749
40 8.62949283705863
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.199388459800863
1 -0.119240897881483
2 -0.553127037236566
3 -0.756541325274978
4 -0.463337966291131
5 0.478261419918628
6 1.35441085210931
7 2.15015722410467
8 2.85455949899654
9 3.7215508401118
10 4.65974518878301
11 6.08068825437416
12 7.19296930267955
13 8.07140721535045
14 8.58268105276845
15 8.87981661533777
16 9.02584521023947
17 9.1863170269531
18 9.27265299061252
19 9.33612851844313
20 9.36795773672386
21 9.38398848891494
22 9.31305834912381
23 9.22678929583438
24 9.14889787465654
25 9.09674458412394
26 9.02461952417716
27 9.0965018898009
28 9.04064419150074
29 8.89797690912311
30 8.67186927852631
31 8.62858941188541
32 8.51310679483702
33 8.39989118648832
34 8.29731128347405
35 8.24688523298211
36 8.10777829138902
37 7.97129890149656
38 7.82886371346509
39 7.72520440160272
40 7.67174973650349
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.213025835965624
1 -0.0919323655054965
2 -0.523049983386545
3 -0.760631215216043
4 -0.497979108637275
5 0.348434215995447
6 1.27464112487426
7 1.94662343923374
8 2.6309909570204
9 3.43437073507927
10 4.31745063150633
11 5.65528065220912
12 6.90086383373658
13 7.89569045102025
14 8.55298096820063
15 8.92826614502533
16 9.08440044637947
17 9.2721995218438
18 9.36414041786299
19 9.44832218141505
20 9.5474996394814
21 9.62154420001262
22 9.67443289149563
23 9.75705027923301
24 9.90393703794733
25 10.1875822824305
26 10.5678556771706
27 11.1418717251447
28 11.8574520246711
29 12.7292587393995
30 13.6906879134519
31 14.6587687399933
32 15.3863026968234
33 16.0601124417204
34 16.7587730867085
35 17.2606969524246
36 17.6275339732911
37 18.0108223185419
38 18.3715202244998
39 18.6384954296431
40 18.9296663847616
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.199877974006386
1 -0.103694694454984
2 -0.536700517143406
3 -0.796687778864242
4 -0.37005907639728
5 0.533796227326863
6 1.30537954019262
7 2.03705698967317
8 2.69731916368665
9 3.44467945918939
10 4.30650630319588
11 5.68539327028923
12 6.87721227518
13 7.83261972330941
14 8.31965229022727
15 8.58824124019665
16 8.84445686326787
17 8.959646095653
18 9.04807303396824
19 9.07889125179724
20 9.14375575822691
21 9.11854118474668
22 9.09268991385893
23 9.06785875826831
24 9.07406938753242
25 9.12212263225471
26 9.08079609085266
27 9.0815730768724
28 9.03833798042223
29 8.94195441847378
30 8.85792737314958
31 8.89040720464796
32 8.79139761602867
33 8.63365774258005
34 8.69116933390943
35 8.75457603750472
36 8.62292052617705
37 8.51347321180311
38 8.44172148860981
39 8.45469872212934
40 8.40840806521446
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.215257666770445
1 -0.100631753274087
2 -0.502022249187171
3 -0.885214157871777
4 -0.62519745681917
5 0.372061117056169
6 1.35537860064815
7 2.189134006181
8 2.99593419985951
9 3.8987382683873
10 5.02470514606339
11 6.55709278045493
12 7.66352518630547
13 8.55512712269567
14 9.06811835296721
15 9.39035555672072
16 9.61473326663005
17 9.78964798904943
18 10.0896331678213
19 10.4702089641494
20 10.9068862863195
21 11.5166215800446
22 12.3239295747592
23 13.2661011095615
24 14.3258755555657
25 15.2324673591701
26 16.0392675691687
27 16.7885860775922
28 17.1865957412027
29 17.7009634572845
30 18.1082267458858
31 18.6266875766317
32 19.0297780656036
33 19.361056204114
34 19.830258776188
35 20.1290576910005
36 20.4026493823884
37 20.6420078343557
38 20.9094950840287
39 21.1516022215496
40 21.3513332278118
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.196625354075614
1 -0.136473797573996
2 -0.625869328803194
3 -0.929380924266206
4 -0.680556508909015
5 0.233774305307775
6 1.19897992688942
7 2.15036039611016
8 3.04398193921376
9 4.11662447307462
10 5.04348559371716
11 6.52606514550481
12 7.70995543151929
13 8.60575587228887
14 9.08726984419814
15 9.34604481666788
16 9.60292948898809
17 10.0053765889295
18 10.4544223930826
19 10.9184721736692
20 11.6536283470588
21 12.5314481422797
22 13.4554607239966
23 14.3495142209308
24 15.1467044812826
25 15.9168758851195
26 16.6559784110877
27 17.4210646975797
28 18.022598056811
29 18.6168691906753
30 19.1760269581914
31 19.6379104615082
32 20.0924243711925
33 20.5066082248633
34 20.912610592923
35 21.276533290672
36 21.6124577806148
37 21.9001051058412
38 22.1439773340833
39 22.3729010821972
40 22.5501705873593
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.221638617764416
1 -0.0126470209533318
2 -0.497983991231298
3 -0.85551361254898
4 -0.608997173555514
5 0.355973752009137
6 1.28809982168632
7 2.06411042689967
8 2.88219270947868
9 3.81854883251563
10 4.75649486639209
11 6.17478582587204
12 7.2732140475077
13 8.17727824965168
14 8.67341275088846
15 8.96843630818616
16 9.12945229393161
17 9.28581929284009
18 9.39461569957441
19 9.46164711203077
20 9.52820712336739
21 9.56650494308156
22 9.67505508677209
23 9.70458798729406
24 9.7825933691345
25 9.96081413863955
26 10.1849241135391
27 10.5911098171178
28 11.0103611210356
29 11.5838345354766
30 12.4180232644812
31 13.3278832173555
32 14.1833229526564
33 15.0203599031345
34 15.7365336011373
35 16.3876732200634
36 16.9976659470025
37 17.5161085711166
38 17.9986671746834
39 18.4302252560264
40 18.7072286058139
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.186309477619926
1 -0.124012503569834
2 -0.581899616824023
3 -0.967522696077479
4 -0.708595823977477
5 0.238614780221162
6 1.18193934653929
7 2.06786544921625
8 2.90356809037254
9 4.00139945671618
10 5.01263336500941
11 6.50496927273212
12 7.56841553964534
13 8.33032048906012
14 8.88543006117492
15 9.30431972739279
16 9.48972203036427
17 9.75205123847632
18 10.0596598788831
19 10.3946605735661
20 10.8683429360643
21 11.4587192833618
22 12.3231017969295
23 13.2079781027469
24 13.9816140616095
25 14.6966078181585
26 15.4638404030384
27 16.048640312125
28 16.5574762247598
29 16.9790094928888
30 17.4083140129233
31 17.8848345664991
32 18.4278837871227
33 18.9558107103531
34 19.5548092900345
35 20.1752796980386
36 20.7194597846617
37 21.263118222571
38 21.6896072167193
39 22.1118498232825
40 22.4718349224246
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.224006201771257
1 -0.095135584368829
2 -0.538584381003037
3 -0.774600047741661
4 -0.555532523638402
5 0.319768404708469
6 1.18312777579827
7 1.94171928084301
8 2.68849156784264
9 3.54763652659104
10 4.41767820033727
11 5.79506636669459
12 6.94244419563311
13 7.8676302219664
14 8.45289495566234
15 8.65653808195181
16 8.84109209718974
17 9.0404469498739
18 9.14340724303397
19 9.16642964866026
20 9.22951051080595
21 9.20853891066236
22 9.22110921722376
23 9.14748613678843
24 9.1310355922746
25 9.17939911837057
26 9.13888887244502
27 9.2338198582483
28 9.18103993757102
29 9.10782906385786
30 8.99118180256704
31 8.95120015871801
32 9.02145672856686
33 8.99303310396679
34 8.99060569151719
35 9.00976959831689
36 9.01713017183947
37 8.99058602704973
38 8.96163976965688
39 8.99778193841605
40 9.0720081734409
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.208406368121323
1 -0.103392875522712
2 -0.578730826396183
3 -0.855312306489371
4 -0.675431231420994
5 0.297063059006437
6 1.26081132909488
7 2.03478627386624
8 2.83462148810157
9 3.65572247079161
10 4.57327258075249
11 6.00044743571208
12 7.17692709864137
13 8.14180658900728
14 8.64995427464933
15 8.88976513314894
16 9.0211658387617
17 9.10393958591029
18 9.22611402419691
19 9.32472930495604
20 9.38677905806771
21 9.38726683430471
22 9.39757174531059
23 9.36991729765823
24 9.38850793172553
25 9.40819573258941
26 9.3876519171618
27 9.52249125009443
28 9.55292121350067
29 9.54882997542607
30 9.48037293471316
31 9.58213795903914
32 9.63922761537867
33 9.61478086809328
34 9.73147518460864
35 9.9445767558676
36 10.1887367954401
37 10.5621730581819
38 11.1016954860516
39 11.9768319118653
40 12.7941838631681
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.20199504803979
1 -0.101262005051601
2 -0.561600167647283
3 -0.798741247743446
4 -0.583391974122818
5 0.324181338026472
6 1.27613553830381
7 2.03872852894815
8 2.80299839252646
9 3.64004729287596
10 4.66949451942085
11 6.10840227087916
12 7.22295812658531
13 8.0856755414855
14 8.54858286681388
15 8.79003020762358
16 8.91666505367585
17 9.10128951503015
18 9.2928660123656
19 9.36266956095029
20 9.37881774798841
21 9.41665206928709
22 9.42989216382574
23 9.43622980332077
24 9.55142156277288
25 9.80715642330793
26 10.1120145159721
27 10.6835804878437
28 11.4429507120212
29 12.2805883076951
30 13.0261403947325
31 13.822179888463
32 14.5207107889121
33 15.2047050745996
34 15.7024426563384
35 16.2226425074975
36 16.7040505234953
37 17.1004049196007
38 17.5544531914259
39 18.0082944216043
40 18.4021247787381
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.208566331747493
1 -0.0929776870004291
2 -0.560816949751825
3 -0.882551975383914
4 -0.675462619143165
5 0.264837685877113
6 1.28693699371523
7 2.15730555342732
8 3.00443996581136
9 3.93600996912772
10 5.06042218038884
11 6.48416840424188
12 7.54449047775749
13 8.46967261146981
14 8.90085977505974
15 9.2178423581728
16 9.34203848721452
17 9.54980204614012
18 9.68058089118753
19 9.75165558556039
20 9.93491774727273
21 10.1316447821095
22 10.4894830180575
23 11.0086659684752
24 11.764594212016
25 12.6729248953671
26 13.7003363580927
27 14.6516734691062
28 15.4674046490615
29 16.2174416341695
30 16.8500431874184
31 17.4275026390515
32 18.0510467977796
33 18.4845381680205
34 19.012936991384
35 19.3687101946515
36 19.6967420379893
37 19.9869009652144
38 20.3761476273644
39 20.7337841990127
40 21.0732349895756
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.210541879989089
1 -0.126437943273876
2 -0.528615852749088
3 -0.854272672207038
4 -0.59737787959286
5 0.39272380286412
6 1.35917617551568
7 2.20555230427871
8 3.00696664240608
9 3.88004465217946
10 5.08948842803591
11 6.52349159127688
12 7.64261389137071
13 8.47718600741905
14 8.98249663486527
15 9.30416435772884
16 9.50605343529568
17 9.73837487448791
18 9.9201472361602
19 10.1254229613463
20 10.3165292632653
21 10.6446890883098
22 11.1271850400936
23 11.7794092044795
24 12.657868349096
25 13.5012536831001
26 14.3478166259754
27 15.0996192530176
28 15.805948291009
29 16.4454724009789
30 16.980332855462
31 17.4980480149024
32 17.9363849969125
33 18.3477611877177
34 18.5449042365003
35 18.7452911779403
36 18.8911117179608
37 19.023836085547
38 19.1722118705411
39 19.3104767633801
40 19.4500743984579
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.213610296119315
1 -0.0879258998772763
2 -0.497837365507346
3 -0.711990805051869
4 -0.420291731682617
5 0.462435547800118
6 1.34916900836129
7 2.15056003547462
8 2.84409926103534
9 3.63680637885696
10 4.56687541653878
11 5.90586297025309
12 7.1893041943115
13 8.13839803494209
14 8.68545329638799
15 8.95814415648115
16 9.13458613671073
17 9.35318845312313
18 9.5254547575207
19 9.66623796811271
20 9.92609199996463
21 10.219843669213
22 10.6812309014769
23 11.2680315774751
24 12.0716690525471
25 13.177964207572
26 14.0796136906491
27 14.8377131232845
28 15.6189883848617
29 16.3549584956195
30 16.9896663054879
31 17.6123935086368
32 18.2756404519524
33 18.9335946068724
34 19.5595839881603
35 20.2106519492248
36 20.84014289943
37 21.4646747134492
38 21.9888173382349
39 22.5050110856181
40 23.0023152672244
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.213491825284854
1 -0.0850664180814542
2 -0.532476856978764
3 -0.858512993946958
4 -0.59995242823462
5 0.406191300766432
6 1.28166794291778
7 1.98922818035764
8 2.73877808127254
9 3.59068604211496
10 4.45390780974118
11 5.85293027694538
12 7.07437113579777
13 8.00768259928515
14 8.61997091559483
15 9.00501463959755
16 9.21772970403432
17 9.41075266754989
18 9.53688380293089
19 9.63925521772601
20 9.68997959067084
21 9.78123213988589
22 9.93907360392644
23 10.1645632108376
24 10.5228611647293
25 11.0057870298184
26 11.6418640347077
27 12.5105197455738
28 13.3336456017543
29 14.1339291332501
30 14.8467849327856
31 15.3972137233985
32 15.9855687210201
33 16.4597720343139
34 16.9727858085475
35 17.490471422235
36 17.927398036224
37 18.2417826177359
38 18.6071416423163
39 18.9286953420873
40 19.2426858602315
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.220480522216308
1 -0.0369299492630439
2 -0.55008770218931
3 -0.896400521940527
4 -0.720931981130308
5 0.262032129218857
6 1.17318782484071
7 1.95739588332067
8 2.69292083335337
9 3.53642944386038
10 4.43705841401285
11 5.7577216111915
12 7.01354493401042
13 7.93226334301131
14 8.49342385177507
15 8.8463948599416
16 9.09339640165964
17 9.31713347347392
18 9.47403670866928
19 9.57438897802116
20 9.65784901441072
21 9.77926645981644
22 9.93483135892098
23 10.2161891915633
24 10.5815217842127
25 11.1554934583561
26 11.9741469346514
27 12.8141334393747
28 13.7331075675429
29 14.4985231439735
30 15.1748482887732
31 15.8017621318523
32 16.4157941145847
33 16.9371592057258
34 17.3214287953308
35 17.7707897610037
36 18.1674245410584
37 18.6226738481487
38 18.9809326707189
39 19.2956742291043
40 19.5718080904509
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.206652887775676
1 -0.0758930210062796
2 -0.556345129101107
3 -0.766866551937445
4 -0.473235334848699
5 0.438603492096238
6 1.31039558113443
7 2.01345432678025
8 2.70787766453648
9 3.5672118255893
10 4.44781343914695
11 5.79795835086109
12 7.02907889252604
13 7.92966703100879
14 8.47612352398707
15 8.77652569691886
16 8.94553636297323
17 9.08629286166284
18 9.16276326946598
19 9.22565951162932
20 9.29083258369468
21 9.30185677557505
22 9.31381334525586
23 9.26540824414063
24 9.31050352655963
25 9.33629009925762
26 9.3115760281204
27 9.48853394300567
28 9.50805412367091
29 9.43743465193651
30 9.38181341180039
31 9.3771373859534
32 9.37679559025403
33 9.33664767929525
34 9.33162796031212
35 9.39007713118035
36 9.37436604590121
37 9.31677708912742
38 9.29114335394529
39 9.32463036082957
40 9.3486988154345
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.214983025583516
1 -0.0879661879651768
2 -0.544151617459278
3 -0.861464679996355
4 -0.551155443420116
5 0.285209746116112
6 1.23250218898453
7 2.01171198226324
8 2.65468012250198
9 3.50540053642465
10 4.42324586639693
11 5.76610447139794
12 6.96990012223362
13 7.88785351288137
14 8.49716294860562
15 8.87495581768434
16 9.05579943763603
17 9.28689417250485
18 9.38648337983624
19 9.44554073903725
20 9.55507830314559
21 9.62493478217883
22 9.76623059936344
23 9.94531291249592
24 10.2677113185557
25 10.8270058203291
26 11.4536185098461
27 12.3036143801626
28 13.160405370289
29 14.0460761152641
30 14.750821157506
31 15.3011977296518
32 15.7378411303185
33 16.2077924909889
34 16.6091162622236
35 17.076263106918
36 17.4794797281054
37 17.8862969772289
38 18.2357382809656
39 18.5873546612942
40 18.9828440645706
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.222083647115069
1 -0.13059998290482
2 -0.465696635205679
3 -0.809480043972409
4 -0.649128551752637
5 0.23696585181135
6 1.16361640534591
7 2.02453302353782
8 2.79625919378386
9 3.71700423920932
10 4.82816691256706
11 6.22725887005027
12 7.29084040665219
13 8.13703759384789
14 8.60914145225052
15 8.80459486403147
16 8.95871043011097
17 9.08777224673702
18 9.16196466934896
19 9.15067968118029
20 9.22880899321748
21 9.2005297662534
22 9.23859636867774
23 9.18796690263021
24 9.24322955357833
25 9.30423240665901
26 9.27360809760276
27 9.35283768476582
28 9.34753424414103
29 9.31671990999091
30 9.26476309392559
31 9.27316752829029
32 9.24951526918649
33 9.22478117237555
34 9.23138360313203
35 9.23392178967341
36 9.23684312419525
37 9.19365426053978
38 9.1355737116718
39 9.17082111771087
40 9.14066670373126
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.186656341056527
1 -0.0983036060699043
2 -0.53280433784997
3 -0.892038626962834
4 -0.74113626121242
5 0.199728886509256
6 1.22842782546643
7 2.10253661127556
8 2.8657091642407
9 3.8262531666728
10 4.93110158830966
11 6.44252409816182
12 7.58083948891457
13 8.46675594381784
14 9.10426300599051
15 9.44979454321918
16 9.67301889277002
17 9.96086414152601
18 10.3219482611744
19 10.9122313227765
20 11.4700913736547
21 12.2124088753589
22 13.0593841697091
23 14.0424585598548
24 14.7993120129846
25 15.5117409049463
26 16.2038141496938
27 16.7821878764173
28 17.2400498710846
29 17.6802046594541
30 18.1034899077908
31 18.6069373929583
32 19.0673341278996
33 19.4910818090715
34 19.8370760955764
35 20.1201692013777
36 20.4280244097657
37 20.6715954555173
38 20.9236705012584
39 21.1278309183512
40 21.312530902501
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.184805735113348
1 -0.157074113593528
2 -0.585678679872658
3 -0.951948873081079
4 -0.698125255860052
5 0.303314226494928
6 1.21935162138201
7 2.06269365319609
8 2.93275698265267
9 3.79582062390331
10 4.7265129811909
11 6.1564430191457
12 7.33752467014466
13 8.19687447629045
14 8.70215809254127
15 9.08448366590608
16 9.28722261309415
17 9.47237040476794
18 9.61721188280613
19 9.71051414869727
20 9.84751695111105
21 10.0301818264501
22 10.3956638750493
23 10.844653995825
24 11.4983464496432
25 12.3827957289833
26 13.2825944033198
27 13.9955377909213
28 14.7313767491536
29 15.3973945920557
30 16.0153997541545
31 16.6225827357937
32 17.1239626717897
33 17.5933318371779
34 18.0314850575015
35 18.5103233107682
36 18.8773588810782
37 19.2408804413616
38 19.4931751246663
39 19.7021019719568
40 19.9383911875933
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.205485727540434
1 -0.0703523087235224
2 -0.594367928231661
3 -0.824901511679331
4 -0.552448310182371
5 0.405062551032752
6 1.30243499564646
7 2.07437584157705
8 2.87611866720365
9 3.79014297624384
10 4.79791489025675
11 6.2564774418905
12 7.35113096329626
13 8.19839775936135
14 8.66411797076919
15 8.92580571753943
16 9.02503468273608
17 9.1626933529666
18 9.20019300464847
19 9.1943074926445
20 9.15704182779634
21 9.10452585480939
22 9.02989893771215
23 8.94890153097887
24 8.89761724505164
25 8.83117243320503
26 8.76932243267036
27 8.83227216577883
28 8.77384322738577
29 8.69637457308976
30 8.59773434091255
31 8.55479008231984
32 8.48219096783927
33 8.42672644124135
34 8.41946349685766
35 8.36524800562102
36 8.25792207224776
37 8.19556853887081
38 8.14263718323684
39 8.10102203826273
40 8.01476967166077
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.204900170925532
1 -0.0645500140194931
2 -0.507806876682419
3 -0.873789897382385
4 -0.661941725136383
5 0.284883806328627
6 1.27915602967432
7 2.21630649024728
8 3.0572613373859
9 3.96874494513024
10 4.99883092747388
11 6.44977306247189
12 7.61832154174488
13 8.50993828483757
14 9.11343316278976
15 9.39242001549794
16 9.49740891417401
17 9.78754379669924
18 10.0653514112714
19 10.3909331798347
20 10.9737683708904
21 11.5794899433702
22 12.3873631844174
23 13.305601487773
24 14.2716993328804
25 15.1009031956666
26 15.7791491582518
27 16.4494363259055
28 17.0790258401801
29 17.6834589268004
30 18.1154446709299
31 18.5060886797895
32 18.8699796903948
33 19.1875536752257
34 19.584996610366
35 19.9144920232604
36 20.1879623959679
37 20.4704728044038
38 20.7339189813762
39 21.0177320944959
40 21.2823908057246
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.196313541342923
1 -0.112782464673449
2 -0.648514562334105
3 -0.992789132264479
4 -0.715120025841472
5 0.235000774280324
6 1.2524520797012
7 2.06999489749052
8 2.91594128068893
9 3.93656382252555
10 5.01768818644989
11 6.47459758069719
12 7.49612430685372
13 8.3440159417349
14 8.82983793898183
15 9.15155952884853
16 9.31716435693229
17 9.50123277108133
18 9.6568866399196
19 9.80388058180827
20 9.99562035257145
21 10.2885039866364
22 10.6746764111087
23 11.1886075706772
24 11.887763542721
25 12.6605253390296
26 13.4479830458075
27 14.1407530495821
28 14.7905306709616
29 15.3842403042364
30 16.058398887321
31 16.545806021909
32 17.0265474401157
33 17.4459808686193
34 17.8533723672311
35 18.1811737730689
36 18.5123959901263
37 18.7359313957364
38 18.8599660663893
39 19.043795985518
40 19.1267183244052
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.181349496862645
1 -0.185256726248675
2 -0.647605459512823
3 -0.826419284457665
4 -0.596942954088174
5 0.290464586606464
6 1.29242911849149
7 2.0815260634057
8 2.82189956272641
9 3.72991782782623
10 4.67830369987297
11 6.0995009907181
12 7.24575749730596
13 8.15754444251126
14 8.7170218817599
15 9.04858257160018
16 9.22706488342222
17 9.38250911107465
18 9.53823308972324
19 9.62557018215431
20 9.78131417819451
21 9.93610368743918
22 10.1501461625603
23 10.449707818554
24 10.9293779181359
25 11.5173770320366
26 12.3150686198612
27 13.2063839781617
28 13.9425364355361
29 14.6526487577385
30 15.3715034686882
31 15.9435383733187
32 16.4725067276102
33 16.9114130828624
34 17.3355098290886
35 17.7880428347169
36 18.1390449672416
37 18.5769924308027
38 19.0070891439779
39 19.3412639534475
40 19.6894105015642
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.19297663510693
1 -0.0686804920361293
2 -0.50114395785057
3 -0.845459908855271
4 -0.606001567981291
5 0.273084937329608
6 1.26101581327413
7 2.15707109068306
8 2.99213048510029
9 3.99927679808001
10 5.05385606241656
11 6.50670505156489
12 7.62532161347038
13 8.52649936159725
14 9.01755052209119
15 9.30074378684855
16 9.48161057748974
17 9.71122930464336
18 9.9615680321838
19 10.2142080742436
20 10.7062238042775
21 11.1857261560563
22 11.9148595623035
23 12.7987683779904
24 13.5858532336066
25 14.3674296797018
26 15.0845816427835
27 15.6700904923567
28 16.2934453140734
29 16.8567388465843
30 17.4438665377301
31 17.8466041137734
32 18.2983083836019
33 18.6573139419801
34 18.9196689803408
35 19.1584724479112
36 19.3673373760733
37 19.5767419554391
38 19.6658145671883
39 19.8047120240611
40 19.8958940056025
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.22042579701911
1 -0.088403237338865
2 -0.584704723871136
3 -0.862891634129553
4 -0.640046310633519
5 0.227456254608169
6 1.22838132648293
7 2.07589530861394
8 2.82487742252039
9 3.71741423180373
10 4.66028867863111
11 6.04443994918015
12 7.25871572040202
13 8.17374473890957
14 8.83275736712202
15 9.08702238277176
16 9.24533097920888
17 9.36299984144153
18 9.5276472196666
19 9.6412524374315
20 9.74342973594902
21 9.86724680095837
22 10.0050964231568
23 10.1729254687195
24 10.4019122384462
25 10.7792728829313
26 11.4261578087638
27 12.1192255579446
28 12.9714616476466
29 13.7494630137125
30 14.5301677585096
31 15.1472177707163
32 15.7244266620639
33 16.2599179265388
34 16.6318072333714
35 17.0862762404932
36 17.5199896747218
37 17.9524752075765
38 18.4139413889112
39 18.8015177324422
40 19.0518189990369
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.198799549125499
1 -0.0694578124081029
2 -0.534855645421635
3 -0.798978922114094
4 -0.539552225761819
5 0.465072947824682
6 1.35173297929872
7 2.15060946869269
8 2.92695403844839
9 3.87294649880459
10 4.8917567673074
11 6.27488700924166
12 7.49372878883509
13 8.35109633789518
14 8.84631991561967
15 9.07787450491664
16 9.23874556330873
17 9.41091593317118
18 9.54354612380469
19 9.68872654497823
20 9.88166031455947
21 10.1528754025289
22 10.5570652357324
23 11.0422679581418
24 11.745629982099
25 12.6480192996995
26 13.5731960036585
27 14.3759291106182
28 15.1262332875483
29 15.9016945586972
30 16.5401892595483
31 17.3069367190533
32 17.9164158229865
33 18.4136087421845
34 18.9757859485317
35 19.4135176288673
36 19.78294424732
37 20.1598523708036
38 20.561995213368
39 20.8903429054767
40 21.1464103278913
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.21061134253009
1 -0.0848265856271576
2 -0.551122377688936
3 -0.838743830987131
4 -0.600907350781869
5 0.294858770554887
6 1.22175365998925
7 1.95466288244814
8 2.73381551634282
9 3.60637363383617
10 4.5754151105465
11 5.9358844218571
12 7.1154378751849
13 8.04709452013523
14 8.59478007559554
15 8.95623610963352
16 9.0712845847826
17 9.16348307934242
18 9.29914024646252
19 9.33258522135942
20 9.39144112676022
21 9.43428093065526
22 9.42172916505503
23 9.40286603623485
24 9.44071047161995
25 9.50160062508018
26 9.56778707535003
27 9.6836981527781
28 9.73584117283978
29 9.7922496517849
30 9.74324257282134
31 9.79080378541298
32 9.91042369934623
33 9.94345289325706
34 10.1275926623382
35 10.3763089755564
36 10.7934181069307
37 11.409623733354
38 12.2220316420446
39 13.0209085054094
40 13.7207244860343
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.204919391861194
1 -0.141965635713837
2 -0.57599715832305
3 -0.805291612242886
4 -0.522916066771744
5 0.38985994123707
6 1.30205333837772
7 2.10544163592427
8 2.87352775407331
9 3.72102546129006
10 4.62002852465207
11 6.08808930178085
12 7.28275720263625
13 8.10606500625189
14 8.73310217360849
15 9.07721961382411
16 9.24868660126454
17 9.44711743943287
18 9.63333692509926
19 9.81068655300745
20 10.0681166747148
21 10.3922249966568
22 10.8425306259225
23 11.441419849275
24 12.1989932298317
25 13.2287360706735
26 14.1105141113807
27 14.8236941186732
28 15.4916887402084
29 16.1225475909372
30 16.6664786850961
31 17.128076343887
32 17.6084496822617
33 17.9528454898671
34 18.2561794109504
35 18.6023170220319
36 18.9498662487307
37 19.2597250732703
38 19.4431507724308
39 19.7426730117632
40 20.0253048144731
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.207295762278988
1 -0.118866140811634
2 -0.589329720073498
3 -0.831075667825667
4 -0.510961567569788
5 0.427884525482828
6 1.32659137210654
7 2.16477440265489
8 2.9168443725438
9 3.80219982964429
10 4.80319512465002
11 6.29694526648578
12 7.43007840644858
13 8.30798252357471
14 8.89620195592832
15 9.30540065039676
16 9.38498890994379
17 9.53456502786305
18 9.69208559630481
19 9.7943848803336
20 9.97091243419185
21 10.1467227511097
22 10.3279425199028
23 10.6884510665244
24 11.3309947270774
25 12.1526773876643
26 13.0119527930179
27 13.8054440767237
28 14.6386917823764
29 15.4580727587956
30 16.2462741832344
31 16.9794659640419
32 17.6673582269009
33 18.2249648283061
34 18.731008286335
35 19.2633332183946
36 19.7765553756958
37 20.3218883415897
38 20.8178472397006
39 21.2609309548776
40 21.6980138223985
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.193465963355867
1 -0.0899865954826371
2 -0.557287054155283
3 -0.753920330734818
4 -0.404414473870694
5 0.380562445146704
6 1.24314705286609
7 1.96619026217729
8 2.64307138329507
9 3.32636087803022
10 4.06528093452392
11 5.22304221383286
12 6.56932031599043
13 7.54790441200893
14 8.19532117332612
15 8.61115163740038
16 8.7306934922574
17 8.88249122448467
18 9.01552154031805
19 9.10175426399659
20 9.16245697126917
21 9.20580491108002
22 9.24326176250247
23 9.25774598316683
24 9.239816828121
25 9.29227604185632
26 9.34270364495723
27 9.48966979976682
28 9.62050612056481
29 9.70135886894993
30 9.81361612167048
31 10.0426504443734
32 10.4421861941685
33 10.9039341332749
34 11.5617422334429
35 12.5024730485817
36 13.3349270520765
37 14.1053929224935
38 14.9757519763661
39 15.6987597533783
40 16.3267609825427
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.213589430572349
1 -0.09321454813582
2 -0.639858179036686
3 -0.910721282398776
4 -0.593957620822188
5 0.320555106520351
6 1.22652499044507
7 2.12432729067009
8 2.87486221776625
9 3.76862480595889
10 4.75490941042193
11 6.09358340802464
12 7.36598294078415
13 8.31458069981381
14 8.80288806228465
15 9.03179197417598
16 9.17925585039503
17 9.29916955167764
18 9.38295398142142
19 9.43796401226478
20 9.51418381766776
21 9.5206262510742
22 9.54206670090766
23 9.49455873565023
24 9.50437697885422
25 9.57845272857377
26 9.52561744011674
27 9.67497081785471
28 9.82567591650288
29 9.93723140870483
30 10.0834817330854
31 10.4027432507067
32 10.8863625413273
33 11.4951973260499
34 12.2707552776552
35 13.0531679320079
36 13.8707515478157
37 14.5545867720434
38 15.200084308275
39 15.8767120504745
40 16.4704661322508
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.20225678387572
1 -0.0866044005940121
2 -0.541396084753837
3 -0.784397579294906
4 -0.44122480218785
5 0.481219648334077
6 1.40314604403065
7 2.22519167191474
8 2.94398426740821
9 3.84841561546693
10 4.83196019679458
11 6.3297197166882
12 7.40522925388586
13 8.37727999143441
14 8.93089355060093
15 9.26829566809446
16 9.42734993712153
17 9.56495475637444
18 9.74175000269422
19 9.86253953762086
20 10.0353764006051
21 10.2331385058368
22 10.5974928652436
23 11.0089190611219
24 11.6885514493368
25 12.6118078159903
26 13.455613134768
27 14.2704426988949
28 15.0824639655493
29 15.9129662911423
30 16.675953795437
31 17.279979198407
32 17.840555332422
33 18.3351469297454
34 18.7966753370187
35 19.1755606001466
36 19.5001799812228
37 19.8575522465275
38 20.0748778860297
39 20.3456269799367
40 20.5562961183682
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.225736411018984
1 -0.0594022709194979
2 -0.527362348453074
3 -0.828052257977146
4 -0.619991184638784
5 0.266380867452493
6 1.18595921339263
7 1.906357325105
8 2.62283557269628
9 3.37166153825932
10 4.21418411340405
11 5.55669157231735
12 6.86235456395449
13 7.77806039929438
14 8.36199461541294
15 8.67425639482025
16 8.88461349508372
17 9.04490352372658
18 9.13212380804107
19 9.14701896307392
20 9.13960346288577
21 9.06910580778155
22 8.98904103410736
23 8.88564778294682
24 8.90258918908052
25 8.85991672230166
26 8.74493007648503
27 8.83574293640709
28 8.75562530251015
29 8.64256145971597
30 8.52809254312254
31 8.54470364873021
32 8.47962343921054
33 8.3698125799261
34 8.37905534155971
35 8.33132318203972
36 8.26446997657592
37 8.17070281158004
38 8.05853954735388
39 8.06696893501018
40 7.96396579415608
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.192536351375204
1 -0.147203214849604
2 -0.552887601214613
3 -0.860614723767288
4 -0.571327611849859
5 0.330491433558356
6 1.25291214200934
7 2.01902071952927
8 2.75772946099057
9 3.62568511236682
10 4.69675358854973
11 6.11482114497953
12 7.29539545486713
13 8.10873229953689
14 8.5813358370818
15 8.78266669334441
16 8.97834079867898
17 9.14085423029016
18 9.27242247439557
19 9.37049713440343
20 9.38758262189713
21 9.46284104665412
22 9.51345984047844
23 9.5053604467576
24 9.57481443725401
25 9.68381176211599
26 9.7995112790313
27 10.1314097716479
28 10.4960431423341
29 10.9353001219502
30 11.5615249081156
31 12.3328395434711
32 13.2542729803822
33 14.0665996751696
34 14.8329205935963
35 15.4985367991252
36 16.1991708640665
37 16.7603950304489
38 17.1599629301865
39 17.5867167321015
40 17.9750797557087
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.22480275434486
1 -0.0771552272275945
2 -0.546484771515604
3 -0.881894386004433
4 -0.639499667492516
5 0.218417385548006
6 1.04583745380081
7 1.86330145533802
8 2.44399039492756
9 3.12381101931479
10 3.68943700308011
11 4.71124633562159
12 6.06461683085845
13 7.16558752734286
14 7.93060334137581
15 8.31986633585192
16 8.59397211943176
17 8.80190878982419
18 8.97773558733659
19 9.02611831017767
20 9.07884591688185
21 9.10051829274826
22 9.07140291600699
23 9.06005328396509
24 9.077243851123
25 9.10716686583767
26 9.12238859310589
27 9.16604718723361
28 9.17085383710346
29 9.10300210006992
30 8.99768813448322
31 8.9855885533472
32 8.9675995233461
33 8.93203123883721
34 8.95102978619182
35 8.95500776549248
36 8.89824702715638
37 8.86172863170962
38 8.80002002027103
39 8.82517176434194
40 8.86806387889914
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.22687730864105
1 -0.0723228639765403
2 -0.521191914859001
3 -0.86964822614893
4 -0.643862686186842
5 0.253330803397889
6 1.19450106655993
7 2.00789619388434
8 2.75182132505179
9 3.69770847628237
10 4.53285775474895
11 6.03478221443245
12 7.17503132877367
13 8.06920429216302
14 8.51801647319329
15 8.81019745452833
16 8.9025830851932
17 8.99991054368077
18 9.05999424097678
19 9.0773930651642
20 9.12139126566626
21 9.18099364852072
22 9.20262342132944
23 9.22161454333324
24 9.24990690179998
25 9.29064800539513
26 9.27229427143385
27 9.28690755503077
28 9.30538043583835
29 9.21075300978739
30 9.14249456738965
31 9.13708152877948
32 9.13273750388432
33 9.09491301070803
34 9.08661402167674
35 9.11780041378872
36 9.12313483483787
37 9.07700561756758
38 9.04922278578067
39 9.06729229114543
40 9.10735342167255
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.204183263290146
1 -0.10671041060642
2 -0.586411043306318
3 -0.864846010425139
4 -0.55797428392434
5 0.314755374865312
6 1.20198237006104
7 2.05166463094997
8 2.79196092953182
9 3.6836464241174
10 4.54156104544518
11 5.98634787822678
12 7.1258230062313
13 8.11151281227034
14 8.66952588399299
15 8.96096612779126
16 9.20222918896151
17 9.32783018753737
18 9.51309773514568
19 9.59005952064994
20 9.77195450012153
21 10.0617083597992
22 10.469201597165
23 11.0003130762315
24 11.7615197358399
25 12.7020569306315
26 13.5591035309946
27 14.324053425597
28 15.0333285596842
29 15.6027561760724
30 16.1262590265385
31 16.5167668979791
32 16.8916449507965
33 17.22483818177
34 17.5814879944333
35 17.801642108198
36 17.9392499471166
37 18.1140498175843
38 18.287156190764
39 18.4421328197384
40 18.5584926132732
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.198133876236911
1 -0.124722649808843
2 -0.545920203524835
3 -0.883437842134225
4 -0.585260611157486
5 0.366078013553175
6 1.33391765384294
7 2.05002456698067
8 2.82603167436967
9 3.57652521322143
10 4.45845123960532
11 5.86657266888367
12 6.9996004370339
13 7.88635944261419
14 8.44145981077319
15 8.80814157755665
16 8.96313741469809
17 9.08999587276782
18 9.19164797868201
19 9.24387225103136
20 9.27157737684649
21 9.27302845741325
22 9.24851474819676
23 9.24821390894363
24 9.22537999041068
25 9.23501607024804
26 9.22010996848726
27 9.31885643372142
28 9.37125345610958
29 9.31273832114651
30 9.25312982505992
31 9.1863585643716
32 9.16113829552379
33 9.15372751493322
34 9.08482912017806
35 9.08165013613448
36 9.09630108653564
37 9.11108445503309
38 9.08043042025352
39 9.08234565196997
40 9.09465970064684
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.188492434864516
1 -0.210434128409263
2 -0.668288811204744
3 -0.884775277792478
4 -0.587905724774593
5 0.369538878026911
6 1.28773153405898
7 2.20933559530555
8 3.06374781500399
9 4.17249108090287
10 5.34482220986083
11 6.67297272447542
12 7.82763056559913
13 8.72890338390401
14 9.15737127514859
15 9.5075926530676
16 9.74953570696449
17 9.97281724393979
18 10.2627992140193
19 10.5686767159505
20 10.9805603643925
21 11.4711511063744
22 12.1813630183058
23 12.9979919823342
24 13.9287785139566
25 14.7242178792553
26 15.4742094471318
27 16.1068355978204
28 16.6874534841686
29 17.1571901801273
30 17.637732398063
31 18.0815295799212
32 18.5975259141328
33 18.8924997850663
34 19.3604838172036
35 19.7559019112738
36 20.0497615449663
37 20.300123016222
38 20.5503458662885
39 20.7523247415702
40 20.8918872541301
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.198673753021805
1 -0.0749939523515782
2 -0.513670583297038
3 -0.690950673691179
4 -0.420451994416353
5 0.538779449178036
6 1.45128066110003
7 2.25088022532434
8 3.03330540646915
9 3.98788910538806
10 5.17875746426619
11 6.58613587908463
12 7.64889503559184
13 8.45999601887661
14 8.98310520571894
15 9.32954749953444
16 9.49626152236764
17 9.70246546267097
18 9.89580655842458
19 10.0909281390973
20 10.3458702125842
21 10.666975149208
22 11.1761792169663
23 11.7476822876769
24 12.6884943810745
25 13.7787947423741
26 14.7784240487688
27 15.6526086103803
28 16.4190648659997
29 17.1703928260258
30 17.7680354057637
31 18.299545137
32 18.7977510092822
33 19.2517009801994
34 19.6758332289571
35 19.9726347472293
36 20.2696317521999
37 20.609371140106
38 21.0236744584511
39 21.4241206269246
40 21.6635355322433
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.21040386246562
1 -0.0838537572079721
2 -0.531343915740736
3 -0.748314677132473
4 -0.48793078554463
5 0.385338191343828
6 1.28281286305236
7 2.00732107020998
8 2.75775763148185
9 3.58573115286148
10 4.31601564665945
11 5.71919200439804
12 6.97490391809138
13 7.91843687766826
14 8.47453066658668
15 8.84868223263119
16 8.97407188822251
17 9.08187376750385
18 9.25977716679803
19 9.32051882424834
20 9.45429037793477
21 9.50408186208766
22 9.65225122885296
23 9.8053823063491
24 10.1009610481969
25 10.5541332667438
26 11.0969227228159
27 11.8113079628806
28 12.6248222231716
29 13.4802388800837
30 14.2615198926247
31 14.9231059957864
32 15.5962601340952
33 16.2231604766443
34 16.7693220696835
35 17.3054094441742
36 17.7564239198387
37 18.2175995505594
38 18.6979679075185
39 19.116580654422
40 19.4925665695244
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.215001342219053
1 -0.133045018196046
2 -0.600392368662761
3 -0.849273950446737
4 -0.617086710527081
5 0.302510096288078
6 1.1628545640299
7 1.98326570344912
8 2.75008520825926
9 3.59866872304938
10 4.40260086295193
11 5.7355872347148
12 7.0051847204129
13 7.95295326915451
14 8.50936043069729
15 8.8232797654718
16 8.9686643549144
17 9.10187373176827
18 9.20043894072633
19 9.23486091623862
20 9.2944750144047
21 9.27244596705559
22 9.2772895395496
23 9.2545863494139
24 9.25077137728526
25 9.24401206640148
26 9.18972952085381
27 9.30149122472981
28 9.34272710874662
29 9.2680296778305
30 9.22191760429497
31 9.19276817804822
32 9.14029793753666
33 9.11630610014013
34 9.11711677312271
35 9.16580028021683
36 9.18160384686715
37 9.14526659978058
38 9.1190133473923
39 9.08835723671808
40 9.15317319113976
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.21378507720311
1 -0.077796022727949
2 -0.486974352886808
3 -0.782904686835806
4 -0.504294879634683
5 0.489375532812599
6 1.41751052681288
7 2.16534242772401
8 2.8803305914547
9 3.68021956467165
10 4.6761275243983
11 6.10846934526813
12 7.3904672321768
13 8.33058160265287
14 8.87428706517306
15 9.2300705033127
16 9.43361626721912
17 9.64944424442383
18 9.78506044080827
19 9.92188453203312
20 10.1715986520725
21 10.4873235399677
22 10.910887373096
23 11.5230771278948
24 12.4213653649512
25 13.3048678006121
26 14.0978307243629
27 14.853117672212
28 15.6106972969508
29 16.3829779584347
30 17.1127664012718
31 17.6761183083603
32 18.2394729656335
33 18.7892841343405
34 19.2392954845161
35 19.5988279994916
36 19.9232230667184
37 20.3773783624054
38 20.7003099771022
39 21.0525876129939
40 21.3816042569335
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.217180335533884
1 -0.0793217928423581
2 -0.530193140136512
3 -0.769888325651731
4 -0.450158747494054
5 0.323309027055248
6 1.21621615973258
7 2.01043144010448
8 2.6764473928709
9 3.42803153167706
10 4.06627437731136
11 5.31344420937284
12 6.58835744665496
13 7.63896711498945
14 8.15811508902879
15 8.45268483634523
16 8.68227715241173
17 8.88046320535585
18 9.035678316014
19 9.12152661281336
20 9.1303721777711
21 9.20321161103745
22 9.24469032655041
23 9.21522520218122
24 9.21716526667898
25 9.24067822494255
26 9.21818131930093
27 9.26242848133182
28 9.21959814588101
29 9.13704098245745
30 9.00406413301023
31 9.03311092194292
32 8.99601132066273
33 8.92073858408037
34 8.96693561046902
35 8.97919766686906
36 8.90133438608289
37 8.86736263045961
38 8.82675955799808
39 8.83382035210711
40 8.76427106701016
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.209797717390871
1 -0.14331186865247
2 -0.607208926333515
3 -0.846144271755295
4 -0.525416059226253
5 0.443937833105328
6 1.3870172776235
7 2.18659998743416
8 2.97479683630781
9 3.95995816969906
10 4.97061477416426
11 6.43202015222564
12 7.57687398361387
13 8.30400011876061
14 8.9228131208602
15 9.21664810741172
16 9.38048941075336
17 9.54978725765825
18 9.69807636148354
19 9.73472732371718
20 9.87122583067129
21 9.96989377516969
22 10.1533338265398
23 10.2637298182228
24 10.6092777604027
25 11.0776410065764
26 11.578314264434
27 12.4172272553539
28 13.2005676538045
29 14.0140862663995
30 14.7475821102744
31 15.4980750370978
32 16.140872153304
33 16.7764098002153
34 17.2960605674731
35 17.7444646137124
36 18.2449921160339
37 18.7328661008978
38 19.3000625202425
39 19.811269746313
40 20.2457455038473
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.200508178021932
1 -0.124047886547848
2 -0.610937453723662
3 -0.984017543330828
4 -0.703406754106962
5 0.191201734837618
6 1.19285526624662
7 1.99915806587121
8 2.84462619940384
9 3.90847186183974
10 4.93158949376833
11 6.42066971180734
12 7.44906097915817
13 8.27635942767036
14 8.87090402111813
15 9.14499464039942
16 9.29842820024993
17 9.55157775340524
18 9.74329529757577
19 9.89399759611307
20 10.1613430314521
21 10.5018805409333
22 10.9385694009341
23 11.4944017189251
24 12.2968909258179
25 13.1442823778524
26 13.9206226356571
27 14.4783175204351
28 15.0173476451221
29 15.4553253821938
30 15.8758829639789
31 16.2590312594547
32 16.6205205949443
33 17.0113837934878
34 17.399334806381
35 17.7674358665869
36 18.0852054419015
37 18.3339212165664
38 18.6029164450505
39 18.9611630281661
40 19.1768180182175
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.223843481324425
1 -0.0641758154036846
2 -0.513307810350376
3 -0.941648218352757
4 -0.649355186743863
5 0.298995709588793
6 1.22254896094642
7 1.97336263010462
8 2.70085585042571
9 3.482737952579
10 4.37601875651459
11 5.76494881271373
12 6.9648368771487
13 7.83597117376442
14 8.25597983847105
15 8.57352649175231
16 8.79589265067619
17 8.99260794690563
18 9.08864493418727
19 9.14260385343058
20 9.24177149341477
21 9.24822494435623
22 9.30777386347521
23 9.30956072750563
24 9.32228385196327
25 9.42978159360238
26 9.49470471645134
27 9.67395829921374
28 9.88569051192379
29 10.1393177853553
30 10.4323244058245
31 10.9629052723426
32 11.6725000176689
33 12.498656979987
34 13.3152905260125
35 14.0839480554994
36 14.7750340861759
37 15.4142635421071
38 15.9707709498805
39 16.4362606800997
40 16.9970841608697
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.187691591822159
1 -0.137749800681628
2 -0.622830315823228
3 -0.968727844677302
4 -0.702941362542933
5 0.237146167097535
6 1.17579633863837
7 2.01031417797578
8 2.82777908875052
9 3.7978667348507
10 4.6915030845554
11 6.13739149898536
12 7.31535260912574
13 8.23927315702822
14 8.80044361232591
15 9.19079310555422
16 9.41503777436954
17 9.71189538037836
18 10.0217583639271
19 10.432361654447
20 11.0487042213007
21 11.7583287276664
22 12.6102039965374
23 13.4322520448972
24 14.2698670749146
25 15.1151431682775
26 15.915295548331
27 16.504316849736
28 17.1152369683363
29 17.7210679704547
30 18.2834206769153
31 18.7780713085005
32 19.2872269237574
33 19.7121763317408
34 20.0972824735268
35 20.4888924622436
36 20.7020046032046
37 21.0132502568865
38 21.2947785985835
39 21.6694339809386
40 21.9105476726571
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.204402741003306
1 -0.12409291585852
2 -0.537739390650841
3 -0.82459755064384
4 -0.582126695285782
5 0.396607623197719
6 1.26447648386691
7 2.01795268768425
8 2.72013918527812
9 3.49929818388708
10 4.27820673594429
11 5.60585377477801
12 6.91431852518221
13 7.89073806274484
14 8.52654045396326
15 8.85143345862143
16 9.05826187963442
17 9.29185675061025
18 9.40662245416995
19 9.54725442822841
20 9.67102094277583
21 9.83582964101714
22 10.0017080466005
23 10.1229818107758
24 10.3968614603265
25 10.900545712724
26 11.5879654515032
27 12.3977541899116
28 13.2811544189484
29 14.1052710664575
30 14.7918681502295
31 15.4068135131811
32 15.9522751627217
33 16.5497083004814
34 17.0295941944045
35 17.4647378004097
36 18.0166610932511
37 18.5536271723322
38 19.0652253122835
39 19.466605918275
40 19.9046484631062
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.216622628494397
1 -0.0569905902582787
2 -0.488994217261346
3 -0.809033062141317
4 -0.503730466137193
5 0.500914178661569
6 1.31938544889454
7 1.99608197008706
8 2.61309388032123
9 3.36355965307102
10 4.24813187363424
11 5.53988737464432
12 6.82354194141406
13 7.81399592122838
14 8.42403173829345
15 8.80751604740882
16 8.99001745845485
17 9.16678053983537
18 9.27508262160083
19 9.32505139596573
20 9.45984887396407
21 9.55750267458058
22 9.68992016245212
23 9.805969333866
24 10.1142057956453
25 10.5496200356604
26 11.1127805212106
27 11.9772724268874
28 12.7764651627616
29 13.672740107387
30 14.4047883516536
31 15.043872184062
32 15.5852967908015
33 16.0390240509643
34 16.4332391313112
35 16.8077959681308
36 17.2555185434767
37 17.565117549907
38 17.7856820567937
39 18.0861140391394
40 18.488475106108
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.208093122160552
1 -0.133785109758379
2 -0.571996740648676
3 -0.810413845435033
4 -0.578793588951147
5 0.343114335231736
6 1.35538824885755
7 2.28082748746477
8 3.11063360688741
9 4.22632615817137
10 5.21990107507562
11 6.61005158495232
12 7.7895982365409
13 8.63936478879663
14 9.39540453766798
15 9.82369997459903
16 10.1087564349104
17 10.469903120891
18 10.895430521158
19 11.4429755770645
20 12.2535116324074
21 13.2073349114829
22 14.179911877588
23 14.998085441811
24 15.7773811901363
25 16.5246432413964
26 17.1678887974471
27 17.817367369328
28 18.3864070532701
29 18.8692268393169
30 19.3169127967474
31 19.7394299516754
32 20.2551442502913
33 20.6306984668145
34 20.9120745958391
35 21.250183729359
36 21.6704821220416
37 22.0135309583296
38 22.3207044282744
39 22.5860511294738
40 22.8436621246834
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.201350086463906
1 -0.0756947325445319
2 -0.521593713747153
3 -0.721027002028473
4 -0.381480933247458
5 0.534404005052798
6 1.48763905243985
7 2.28924977552278
8 3.04133467723351
9 3.9732580126339
10 5.15282096276397
11 6.52670310326545
12 7.54459812571111
13 8.31487799814438
14 8.81443523397959
15 9.08536734300556
16 9.20825529683569
17 9.32352866762668
18 9.41273216493883
19 9.47788173054145
20 9.55577592103486
21 9.59216207086853
22 9.66241662465709
23 9.6687820510193
24 9.71731608171142
25 9.83147235509858
26 10.0168487731575
27 10.3252014341644
28 10.7263388349509
29 11.1476364621499
30 11.7740325533282
31 12.6335357654577
32 13.4232661505225
33 14.1491703211501
34 14.8683956571975
35 15.5395776041481
36 16.0858695497233
37 16.6113691896111
38 17.1368389325635
39 17.6849705765986
40 18.0510624121166
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.206939044835011
1 -0.0822050417492422
2 -0.521710677523448
3 -0.972288689693428
4 -0.727758874533131
5 0.230204774910692
6 1.17881301162984
7 2.05568954753004
8 2.93834506817032
9 3.95496470983224
10 5.20506458906601
11 6.6197961430385
12 7.65235814271659
13 8.39594458708188
14 8.7960474183677
15 9.01974160914348
16 9.11106261343731
17 9.20453792466443
18 9.29358992781837
19 9.33626096949707
20 9.40866317096856
21 9.40105120043759
22 9.41214963166229
23 9.41419449208701
24 9.41232696759901
25 9.47144230635866
26 9.51832277481155
27 9.65329566341151
28 9.68671757104681
29 9.71914051549892
30 9.66879024409037
31 9.68343926355326
32 9.70553288704697
33 9.65500666679702
34 9.72671255984893
35 9.82577715413831
36 9.87884650860022
37 9.88335735623151
38 9.87592701240623
39 9.96764599451025
40 10.0291574294243
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.225575358607046
1 -0.0292611519536333
2 -0.502902412944105
3 -0.721717301060305
4 -0.518582247194848
5 0.364796551482321
6 1.20689177470532
7 1.97504437918793
8 2.64555849507585
9 3.3489694450947
10 4.19496312465408
11 5.44332683583561
12 6.65685196955647
13 7.6670259594768
14 8.33297279688666
15 8.71645511831155
16 8.9102533983171
17 9.14578214764962
18 9.30165281462554
19 9.35454014996375
20 9.42936337949337
21 9.4689512555595
22 9.53570251788369
23 9.4891287531879
24 9.57566103081036
25 9.60888360545184
26 9.61627682517376
27 9.78527629378406
28 9.99172880621873
29 10.1793689304669
30 10.4112863869047
31 10.8436261192864
32 11.4128997398577
33 12.1280052425648
34 12.7895840367612
35 13.4945618994189
36 14.3196731790414
37 15.0798800823815
38 15.7760670007848
39 16.3169733278426
40 16.9312935211069
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.220906686230935
1 -0.0811316131791002
2 -0.561375402455489
3 -0.900213193032722
4 -0.609173818753648
5 0.296792661800034
6 1.18988903844459
7 1.99092514922393
8 2.72544236391791
9 3.6965113936698
10 4.66170471643535
11 6.02531236972709
12 7.14919412962193
13 7.94849464946118
14 8.4602665874839
15 8.65688934400532
16 8.83632226216648
17 9.00247674738448
18 9.1102272828643
19 9.15685304466942
20 9.19564181096015
21 9.29483177533018
22 9.28645122369787
23 9.27315643237375
24 9.26317687513124
25 9.28452117854543
26 9.25726439693802
27 9.37248844016368
28 9.35046348568231
29 9.24682963965332
30 9.19329115491713
31 9.17678194194703
32 9.14748957779156
33 9.13155102628751
34 9.19655439354405
35 9.21069859949642
36 9.2116205520079
37 9.19578801535004
38 9.16457996818456
39 9.21030327664628
40 9.24961959531516
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.231730384704318
1 -0.0910619175044876
2 -0.563404033807703
3 -0.81501617164043
4 -0.569459890356991
5 0.401174572132407
6 1.29979262017825
7 2.10632462485604
8 2.82171602247958
9 3.6199221878007
10 4.50710477056843
11 5.86917010788749
12 7.00212904166708
13 7.9437264855122
14 8.5183940407599
15 8.8605587429978
16 8.94236829187717
17 9.12141571842979
18 9.2096843909742
19 9.20547775588304
20 9.27858851711188
21 9.29681740503554
22 9.29974734194669
23 9.28027661294812
24 9.30878288904459
25 9.39299412043108
26 9.35844068116288
27 9.48753212332756
28 9.50450317893273
29 9.49385543019426
30 9.41972721725911
31 9.45061531514459
32 9.43167958178871
33 9.39843760967564
34 9.4305500493178
35 9.4340834526095
36 9.43547400101769
37 9.37962964528502
38 9.33105965315821
39 9.4048584040573
40 9.47654689232074
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.206409085118926
1 -0.128039016324634
2 -0.632458769640806
3 -1.01618237443551
4 -0.770437880152809
5 0.173838629123292
6 1.2024339388422
7 2.12179103976848
8 2.93390461909616
9 3.90907650797879
10 5.10495198538028
11 6.48773852526775
12 7.58258069916253
13 8.46309338905392
14 8.85516191067796
15 9.12675537647014
16 9.25620135599243
17 9.44716760443208
18 9.58177846499618
19 9.69393888276927
20 9.77565497679882
21 9.84821826189599
22 9.97217220081313
23 10.1229228312699
24 10.386903349159
25 10.8619040754708
26 11.4582538194083
27 12.3443950826339
28 13.1631121686171
29 13.9791236787692
30 14.7945858762284
31 15.5335682194904
32 16.0814229887772
33 16.6213315243587
34 17.1712018472662
35 17.6506988084865
36 18.1822865983502
37 18.6399930834895
38 19.0531262153757
39 19.5518052671306
40 20.0132937946484
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.218689467370794
1 -0.094611956488955
2 -0.602882719076793
3 -0.938780906463596
4 -0.771812253944944
5 0.139194760869283
6 1.09847817015175
7 1.89610802735603
8 2.60783087150697
9 3.63662360089149
10 4.7069234858312
11 6.23282976647983
12 7.37955003890231
13 8.31354190665722
14 8.92195597520433
15 9.18560199743568
16 9.3262864996295
17 9.55427183060343
18 9.71357641259484
19 9.86329658988097
20 10.1459201041303
21 10.4325629421773
22 10.9148831295956
23 11.4771803880781
24 12.2366836707737
25 13.1599287600866
26 13.8991669776151
27 14.6610628413621
28 15.3446598370118
29 15.9267535763853
30 16.4802872472012
31 16.8967101687025
32 17.4490414794835
33 17.839222889584
34 18.154465697273
35 18.5305936909302
36 18.7490721251156
37 18.9668411371343
38 19.2301135559371
39 19.5125973232161
40 19.681436311997
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.212608831150003
1 -0.0749872609107812
2 -0.512606749799871
3 -0.821322424266933
4 -0.56760528362577
5 0.356423908124578
6 1.27037846778443
7 2.13552103070804
8 2.96147415574127
9 3.79393766281387
10 4.70406894657051
11 6.12664988898748
12 7.24577736478428
13 8.17398683851155
14 8.66669927322442
15 8.90575053530958
16 9.01472265518212
17 9.18014188854358
18 9.30577497117734
19 9.3789765562887
20 9.48879559252476
21 9.63701572512206
22 9.7267136834763
23 9.92964858657048
24 10.0966844015836
25 10.5291789413977
26 11.0099105836224
27 11.8162380911549
28 12.5919117375669
29 13.4278970371006
30 14.2952686981073
31 15.0880576410677
32 15.9424058534462
33 16.6630678518522
34 17.3017904147083
35 17.8829779565614
36 18.3276965039664
37 18.8110740554507
38 19.2566531495594
39 19.7454393949709
40 20.216576665429
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.188140788507994
1 -0.122248443557352
2 -0.549753806812448
3 -0.760354794321258
4 -0.556423394682516
5 0.3854719818816
6 1.27925234713649
7 2.10244122734624
8 2.85072663684887
9 3.8084901798736
10 4.72703126448536
11 6.13722690498397
12 7.31437232924285
13 8.30821433880774
14 8.85951510730201
15 9.11447181959335
16 9.28309282014837
17 9.44241045775835
18 9.53881663296009
19 9.57662631126667
20 9.62587097411926
21 9.65017373117506
22 9.65091605603622
23 9.61361504061071
24 9.63529638354121
25 9.67782547340501
26 9.67012013277681
27 9.78412031316206
28 9.82512784182977
29 9.77373240467683
30 9.67986105557559
31 9.66127380332133
32 9.59670572220009
33 9.56257948151196
34 9.563512479017
35 9.60414890384295
36 9.62749401892243
37 9.5407603856884
38 9.44018436675475
39 9.38194150673093
40 9.32800746002253
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.203026035356984
1 -0.145698338719584
2 -0.602611108814167
3 -0.857814437282346
4 -0.598063772933841
5 0.310454637303128
6 1.29928951356498
7 2.15452333362511
8 3.00586872907811
9 4.0293060143534
10 4.99548994029543
11 6.50541012857732
12 7.59162746982652
13 8.42351426321801
14 8.93156185612203
15 9.27594544825144
16 9.53682702421584
17 9.75201514982962
18 10.0052146147394
19 10.2536391177791
20 10.7746915489059
21 11.3226135713035
22 11.9892305039569
23 12.8628472424951
24 13.7612575852412
25 14.6335548387204
26 15.3867131435746
27 16.1369027025989
28 16.719259522784
29 17.3045772127671
30 17.8498130077669
31 18.2862751107619
32 18.6924589180976
33 19.0809300233754
34 19.3997465293249
35 19.7079901399104
36 19.9631255552327
37 20.2354084553308
38 20.5086102700702
39 20.7578174119032
40 20.9507617529749
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.206861612228111
1 -0.0492429606544382
2 -0.532433872680987
3 -0.931377359639184
4 -0.683700623082743
5 0.284113137020973
6 1.25298241754108
7 2.12203032822757
8 2.95761523348091
9 3.89108628446263
10 4.8462268228422
11 6.30963004829567
12 7.42769102790658
13 8.3186633301899
14 8.82462297193437
15 9.0585269065324
16 9.22638705299191
17 9.37592360569957
18 9.53169621319101
19 9.5494917103201
20 9.66462726101038
21 9.70118736551341
22 9.82875793421194
23 9.89861556486041
24 10.0534748816356
25 10.3769154244833
26 10.5995438491461
27 11.02054507282
28 11.6475987085157
29 12.3199897072512
30 13.1473281032187
31 14.0959742267575
32 14.9608774999663
33 15.7750163118489
34 16.4409439172174
35 16.9636749833187
36 17.437871210923
37 17.7559767126584
38 18.1747434803252
39 18.5758736483006
40 18.9695739184477
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.19906677020196
1 -0.122229398663299
2 -0.578363582904995
3 -0.881451730235807
4 -0.636422505571585
5 0.348455271229043
6 1.34336778870225
7 2.18274876438377
8 3.03604464340182
9 4.08297617813307
10 5.31066335038579
11 6.69911905819643
12 7.78480219497021
13 8.60576135986001
14 9.14471052933574
15 9.42755757845943
16 9.53522092888934
17 9.70386112660832
18 9.92828954847393
19 10.0430041666002
20 10.2780735627415
21 10.6196982730135
22 11.0175331835862
23 11.5806566111048
24 12.3534214559275
25 13.1782196124406
26 14.022874612205
27 14.848704137289
28 15.7093313182056
29 16.487291535725
30 17.2436348883144
31 17.7864041175785
32 18.4064224757169
33 18.9905697128633
34 19.4469815877448
35 19.9040820526381
36 20.4237266213909
37 20.8289797576318
38 21.251899808278
39 21.5596456103845
40 21.8798398400785
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.195862312797875
1 -0.0982304284893811
2 -0.614824955840891
3 -0.974535249013124
4 -0.672098144459671
5 0.325468218950002
6 1.32858163025971
7 2.24799777629363
8 3.30527502509797
9 4.44254062489379
10 5.55957515607662
11 6.84601076916562
12 7.76850929711788
13 8.57914423968299
14 9.0739504998027
15 9.40196196244916
16 9.47251137753909
17 9.61586699184205
18 9.68302051871908
19 9.74697386906042
20 9.85819938747731
21 9.97376617871961
22 10.1593244152156
23 10.3903294652369
24 10.6988482652126
25 11.2428306176681
26 11.9198394291315
27 12.8784850176135
28 13.7491529624809
29 14.5770712357766
30 15.280802591965
31 16.0581498898286
32 16.7734021760404
33 17.4060031494915
34 18.1229579111868
35 18.7400892716196
36 19.3318886290339
37 19.8162854670797
38 20.3808069868655
39 20.9208109143611
40 21.4480700479197
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.22965296031226
1 -0.0559478677348691
2 -0.558567532252906
3 -0.858320142045412
4 -0.566495683132417
5 0.398223058164344
6 1.285551983413
7 2.0888666773611
8 2.90909981767718
9 3.86691136463034
10 4.83161861417053
11 6.19626180216475
12 7.25042625857027
13 8.06282132165945
14 8.48546269681145
15 8.65762640615951
16 8.74023340401493
17 8.80949745995197
18 8.81780981308778
19 8.81571879387991
20 8.81648709224353
21 8.8113769794166
22 8.72683715583447
23 8.72064810195247
24 8.72468966278834
25 8.64370374200242
26 8.5861826465125
27 8.63027056389819
28 8.6084551801519
29 8.52361823210541
30 8.40069763644897
31 8.39573903505925
32 8.32832901049824
33 8.27730074587615
34 8.20636857899432
35 8.12686957791814
36 8.03141074198695
37 7.92345320853673
38 7.8858426075888
39 7.81791474127434
40 7.79649181245395
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.180865787969458
1 -0.161921829993891
2 -0.606827146699607
3 -0.856827582587307
4 -0.567883473099581
5 0.377169233075654
6 1.34387829030372
7 2.14299880350351
8 2.92520673101552
9 3.88927546362318
10 4.94229740113279
11 6.28962246334028
12 7.45480596465148
13 8.34606708325478
14 8.70248232456948
15 8.92978082416035
16 9.17783305408247
17 9.3656024358598
18 9.57715391229529
19 9.85950988256733
20 10.2035508728135
21 10.6193775795252
22 11.199129814094
23 11.8992091961225
24 12.8888862865871
25 13.7150504146018
26 14.5235656408558
27 15.3027221359294
28 16.0413738545742
29 16.7402405868893
30 17.4032775644194
31 18.0217534250973
32 18.5194676415023
33 18.9957249498789
34 19.3916188905059
35 19.661877408584
36 19.926003781539
37 20.153707804316
38 20.4270193150403
39 20.6284186135579
40 20.8720150007114
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.201575985896791
1 -0.112484869073636
2 -0.595049344285081
3 -0.921257967657817
4 -0.580249440729413
5 0.370105130748534
6 1.26852823942986
7 2.04153613316558
8 2.83475286177868
9 3.70107898686656
10 4.82512753477304
11 6.20073641347557
12 7.27768426166046
13 8.1307874766354
14 8.62867374460656
15 8.84344001452753
16 9.07150333101904
17 9.2590068078663
18 9.38516182567476
19 9.43267129333398
20 9.54794685038825
21 9.69120742611767
22 9.81834839797373
23 10.0471914867329
24 10.3668173982249
25 10.8505329119568
26 11.4338345400005
27 12.2216646369996
28 13.0257462215448
29 13.8063582707699
30 14.5785287911995
31 15.2736226616828
32 15.9108247447447
33 16.4886961714365
34 17.1106064549342
35 17.5717799165618
36 18.0667978321361
37 18.4941716708898
38 18.9602410407245
39 19.4469447156887
40 19.868802441877
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.215361754831222
1 -0.0508415890871985
2 -0.530165702418364
3 -0.835349538750308
4 -0.489311034921804
5 0.387992636631447
6 1.28982497505668
7 2.03697667397199
8 2.68668521781109
9 3.37301978673126
10 4.1184707174478
11 5.29850952543901
12 6.63614790106404
13 7.63252914293427
14 8.24104454634535
15 8.49033112391206
16 8.69676086058323
17 8.87356642066753
18 8.95245939752129
19 8.98261918160187
20 9.00739074636295
21 8.99095589407139
22 8.98423746817881
23 8.97769002214771
24 8.94403745250109
25 8.94652287006667
26 8.9231046818473
27 9.06778517782617
28 9.05094465684225
29 9.03221646595819
30 8.99528448178802
31 8.99211343703576
32 8.92151307769126
33 8.83535965991356
34 8.89713491530964
35 8.85470636799395
36 8.75056134576355
37 8.63062271326984
38 8.5747260443843
39 8.54822703914934
40 8.45233194162812
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.198447609330155
1 -0.107882047978498
2 -0.588814649525625
3 -0.814337168961648
4 -0.529380963837434
5 0.428769565131314
6 1.27880639090046
7 2.06081950746669
8 2.83293967969034
9 3.75558055223608
10 4.75004764564769
11 6.23606638491419
12 7.42400865694554
13 8.2517928342462
14 8.78349862913315
15 9.03401702967793
16 9.22228356136911
17 9.40103689033141
18 9.63168400799926
19 9.8446118960954
20 10.1834332213254
21 10.5179206901518
22 10.949901179915
23 11.7453913400248
24 12.7023210656031
25 13.5752617047969
26 14.4742907087275
27 15.2200358841764
28 15.9457401531764
29 16.5895349588845
30 17.1024726804782
31 17.6805481082115
32 18.1483925965724
33 18.6607257038159
34 19.1547242346032
35 19.6304808043698
36 20.0827259588326
37 20.4891449780887
38 20.812077778237
39 21.1184573505395
40 21.4193849358183
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.199368615812913
1 -0.115412923435555
2 -0.524364162158441
3 -0.756418190655089
4 -0.474198104597059
5 0.404566399030441
6 1.34486599775136
7 2.0886581231235
8 2.86398699453043
9 3.80610175407322
10 4.76861761913494
11 6.16158717063334
12 7.21768968216684
13 8.07612695141953
14 8.65671871728453
15 8.99414014236886
16 9.14047393859598
17 9.31696910308248
18 9.42170074126226
19 9.4789665054253
20 9.59112494763835
21 9.72711470835393
22 9.93622946605079
23 10.2420151805109
24 10.67637450927
25 11.32693747165
26 12.1263730960683
27 13.0801412168106
28 13.9305511947744
29 14.721797840195
30 15.3863458866131
31 16.0154797183973
32 16.6491916319621
33 17.1135328093894
34 17.5950037588429
35 18.0409254299241
36 18.455101272392
37 18.8296554795879
38 19.2063737434839
39 19.5535323325448
40 19.8677344001034
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.216105261379143
1 -0.0907782772221425
2 -0.546861980180952
3 -0.886920437703326
4 -0.60939122190826
5 0.352970893032631
6 1.29990307146093
7 2.21926006733053
8 3.02351769948811
9 4.01963399795901
10 5.2033790711827
11 6.52833402308378
12 7.63016657902338
13 8.45902145841876
14 9.05471937622565
15 9.33468125902674
16 9.54139642885098
17 9.74683543762257
18 9.9458241379576
19 10.0933281443108
20 10.303571236544
21 10.6059075042612
22 10.9601323380519
23 11.4401451819513
24 12.061247941187
25 12.780171031558
26 13.7285072214696
27 14.4905661968779
28 15.3630172952493
29 16.1167629304249
30 16.6735549566654
31 17.1114473039276
32 17.5495161770679
33 17.9271264929526
34 18.2441430794403
35 18.5772213072196
36 18.8635019836894
37 19.1036020685658
38 19.4217089322256
39 19.7598876009171
40 20.1070149245556
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.197941653351781
1 -0.13364849433382
2 -0.637030483055222
3 -0.850220600488488
4 -0.60271107488463
5 0.351966324481189
6 1.27368006340503
7 2.07126299085085
8 2.84262542947425
9 3.77547338805702
10 4.9115162152777
11 6.43637290924974
12 7.55404288568161
13 8.52839277292341
14 9.03029250621534
15 9.28811743029432
16 9.50060862491702
17 9.722432909098
18 9.93646562978873
19 10.1608580012043
20 10.4472927464885
21 10.8539670827555
22 11.4398168506229
23 12.198141954683
24 13.0581898421111
25 14.0108351065372
26 14.8214017981285
27 15.3770521323767
28 15.9976063653653
29 16.5797136777221
30 17.0981839184909
31 17.4927011316489
32 17.8074109022893
33 18.1556083686937
34 18.4236023181691
35 18.6272893781551
36 18.7127150481604
37 18.8177989438916
38 18.9114825946122
39 19.0314099936761
40 19.1257257793297
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.210365783014124
1 -0.0698760708525055
2 -0.534022101066382
3 -0.894533696358548
4 -0.74467985604819
5 0.228406774456138
6 1.216603143077
7 2.07131364755416
8 2.88574864870996
9 3.84190334900525
10 4.83381392403728
11 6.25804313594204
12 7.4937267941095
13 8.35088571284846
14 8.93896539874855
15 9.20876949303743
16 9.3656311751538
17 9.5818713298997
18 9.73988676356513
19 9.88579570125398
20 10.1598932023014
21 10.5320445070206
22 11.1055253947128
23 11.7979162258697
24 12.676017332173
25 13.513851213734
26 14.1699773808159
27 14.8366489727907
28 15.4131419837188
29 15.8591777398838
30 16.2461755449173
31 16.586104268983
32 16.8938675356104
33 17.175351623767
34 17.3360026332996
35 17.5919830016919
36 17.8030051644796
37 18.0531702468854
38 18.2145154359554
39 18.4716279214771
40 18.8202563448989
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.200122682180815
1 -0.142073163548132
2 -0.580872002594197
3 -0.884631405982935
4 -0.549748269288734
5 0.410187466911052
6 1.27388965449344
7 2.05022759961522
8 2.81613538888396
9 3.73868876410473
10 4.63820185078972
11 6.03073363169948
12 7.19730317703434
13 8.08024899472014
14 8.62846136610441
15 8.9133023577767
16 9.07359729738431
17 9.26959579336632
18 9.4347707317123
19 9.55050181610626
20 9.62552408639441
21 9.67518026854687
22 9.77124665249188
23 9.85580041423087
24 9.9119855880735
25 10.0557301323551
26 10.3095435786862
27 10.6680850453184
28 11.0890165722589
29 11.6306191932638
30 12.2714717421375
31 13.1529367928582
32 13.9168930373748
33 14.7804481464719
34 15.5520002402018
35 16.2989629529542
36 17.0072989750277
37 17.6199627575573
38 18.2329580122236
39 18.8868461781799
40 19.5340785633045
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.211119535646813
1 -0.107896097958633
2 -0.57133983766649
3 -0.917587997803803
4 -0.676947729343393
5 0.24502658962213
6 1.24887511775667
7 2.06028546722624
8 2.92549111646753
9 3.9741005174248
10 5.11683248780457
11 6.47734265808975
12 7.55676762934148
13 8.31313255491579
14 8.67849606438703
15 8.94841759273319
16 9.028598518821
17 9.14009688828175
18 9.23440313547528
19 9.25683288771438
20 9.28885547141974
21 9.26622478122818
22 9.26844979423471
23 9.20678506529519
24 9.18551838225591
25 9.20349053059029
26 9.13133411795631
27 9.12454737050913
28 9.15698557494182
29 9.13436443364297
30 9.11021441532617
31 9.14496504080637
32 9.12511509218241
33 9.13197496652625
34 9.20047296676906
35 9.24711920376853
36 9.16704369823447
37 9.14638202751498
38 9.17284404461101
39 9.22644582529644
40 9.16480830876063
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.193847585371317
1 -0.115753755083002
2 -0.557008306090333
3 -0.806474154678557
4 -0.483836779364014
5 0.530695309238839
6 1.46962466952628
7 2.27665312536967
8 3.04277863997071
9 4.02099641102528
10 5.07446203350808
11 6.51376457044698
12 7.61614977309356
13 8.36446651831779
14 8.79743146127184
15 8.97604295465453
16 9.12005341031579
17 9.22640284152431
18 9.30003523573648
19 9.36493745835646
20 9.40323459660689
21 9.42553767576335
22 9.42791710079183
23 9.4519496526395
24 9.41860685240701
25 9.41829974188421
26 9.45020638890679
27 9.49604401654969
28 9.53548263157879
29 9.48918647684891
30 9.43719078437969
31 9.38920024647145
32 9.33820599494534
33 9.37446887429697
34 9.31781521814084
35 9.32812819611612
36 9.34270956981831
37 9.33462973000756
38 9.31963368084294
39 9.28366957616965
40 9.30985575050362
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.215006062078605
1 -0.103112556101572
2 -0.576053218055604
3 -0.897569086076366
4 -0.620158543291792
5 0.313028896648291
6 1.26250699568025
7 2.05963179706648
8 2.82844586543563
9 3.6091072784602
10 4.5638106218446
11 5.93482868600431
12 7.00826740068339
13 7.93693104951842
14 8.42647487242766
15 8.71364976519894
16 8.87501001632144
17 8.9910423401243
18 9.08338542505556
19 9.12569319244879
20 9.22085584316517
21 9.22513465251753
22 9.29678679203078
23 9.3210004913736
24 9.40883415049852
25 9.52406251900272
26 9.63967875046162
27 9.93367467016324
28 10.328412861878
29 10.7675309907198
30 11.3066291631129
31 12.1363061533026
32 12.9171620042403
33 13.7079413518142
34 14.2353213551884
35 14.7842499905089
36 15.2927805359196
37 15.7719297518826
38 16.3635414467243
39 16.9118354494096
40 17.3959399810903
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.195500874493677
1 -0.0830094141953178
2 -0.481813291608472
3 -0.772285184058562
4 -0.507054968818929
5 0.440411066514808
6 1.38590771955828
7 2.1108850887745
8 2.87207543859223
9 3.86081554711863
10 4.84846720658365
11 6.29389456028184
12 7.45730184238274
13 8.33092909735799
14 8.87929903526929
15 9.18346020522474
16 9.33210080532321
17 9.48511077557855
18 9.62091914995312
19 9.68466079524082
20 9.76522553624606
21 9.89951634795096
22 10.0127961868305
23 10.1975833627796
24 10.5283296309795
25 10.9145138927462
26 11.4421877942233
27 12.2329640329808
28 13.180495164746
29 13.9986889653392
30 14.8699646411319
31 15.665769575738
32 16.2493921025046
33 16.7038293225229
34 17.2809747639971
35 17.7165125329723
36 18.2489125660526
37 18.7086398734281
38 19.2492154879375
39 19.7138899028819
40 20.1840176228774
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.176818943530117
1 -0.162764082423096
2 -0.595789480150504
3 -0.715255491883628
4 -0.371143965787101
5 0.407075042808232
6 1.2736513421961
7 1.96708652039811
8 2.62541314559192
9 3.32084187393313
10 4.20323350422524
11 5.48382985321345
12 6.83139267482831
13 7.91089069325956
14 8.57192406890475
15 8.8959076738545
16 9.10823485509309
17 9.33541275687717
18 9.53765218966704
19 9.58961262053977
20 9.75318661520327
21 9.88844074741895
22 10.1058026554976
23 10.3793159634373
24 10.7979443796114
25 11.3661768753044
26 12.0119351426659
27 12.9046378028862
28 13.6756658215266
29 14.485784560068
30 15.1255489331062
31 15.7728996468474
32 16.3483614871917
33 16.8895082110591
34 17.391266577655
35 17.900072707637
36 18.393143026612
37 18.8294328957747
38 19.2224446216949
39 19.5972570350881
40 19.8788160353692
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.226978757146148
1 -0.049811054440164
2 -0.501865372184509
3 -0.834552793668839
4 -0.572877595721358
5 0.251064323843502
6 1.01101830077499
7 1.78099821931371
8 2.39622935042944
9 3.01187275459952
10 3.60927454729574
11 4.55895653595807
12 5.86074942784502
13 7.06843145383098
14 7.81696051056717
15 8.22434173764418
16 8.48807694137447
17 8.69999296233863
18 8.81690194484602
19 8.84838870823922
20 8.84314271253512
21 8.8125611737781
22 8.76686439466677
23 8.70974265847481
24 8.71146508258439
25 8.66881588993127
26 8.5278481273905
27 8.55866457871182
28 8.48252718663715
29 8.38983366061963
30 8.29749291347335
31 8.29739371804621
32 8.23428408753881
33 8.12310501531537
34 8.08526087049925
35 8.06251286042966
36 7.96753939271688
37 7.91496941455694
38 7.85394753574153
39 7.81771890112093
40 7.7191889822797
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.214162848028917
1 -0.116242845788976
2 -0.614707689803164
3 -0.879079805869294
4 -0.54927193460644
5 0.341994754752425
6 1.25802495186751
7 2.09885828769908
8 2.95151541777545
9 3.90975653729422
10 5.04781986597764
11 6.54092142347566
12 7.63266500946584
13 8.49916310556009
14 9.12117190056513
15 9.46731154608317
16 9.73360419027711
17 10.0396223520669
18 10.4753371526195
19 11.0235627174704
20 11.6878175284813
21 12.4891595872125
22 13.3683237276936
23 14.1077554367375
24 14.9036702524262
25 15.4909824712753
26 16.0370367379075
27 16.6292962792736
28 17.1430391404252
29 17.6596698561021
30 18.0602999550098
31 18.4436924762989
32 18.7675491688013
33 19.111993106729
34 19.5029226480761
35 19.8586910403093
36 20.2363109675096
37 20.6326801572145
38 21.0017494988125
39 21.3947588119797
40 21.7446264867583
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.17794161347915
1 -0.147597117581172
2 -0.531622500023813
3 -0.727869072067752
4 -0.479421259557464
5 0.342017486993787
6 1.28274873660463
7 2.11177917787477
8 2.85914277287721
9 3.68058385642414
10 4.61589529273578
11 6.15315358856029
12 7.38740269259985
13 8.18908218440002
14 8.8131688514335
15 9.14098488325557
16 9.33021994085327
17 9.52887624561144
18 9.79351725050654
19 10.0478506132949
20 10.4421076328057
21 10.9718918222238
22 11.5966699671899
23 12.3944784054692
24 13.26161135648
25 14.1029205387706
26 14.8929394816381
27 15.5658885978543
28 16.1773040581727
29 16.723465080585
30 17.2410267061934
31 17.8125037596382
32 18.2347062219211
33 18.6722725660918
34 19.0936652920782
35 19.471776488596
36 19.8100222687634
37 20.1070869618312
38 20.4328333295763
39 20.7505401859729
40 21.0073071238474
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.21281991079761
1 -0.156757713306959
2 -0.626999764329143
3 -0.870441593822614
4 -0.554876673226129
5 0.380764158517039
6 1.22852605772593
7 2.03147802093798
8 2.72974070229413
9 3.56552543800377
10 4.525867031929
11 5.97307966181678
12 7.14540035680699
13 8.10726125612818
14 8.68829379415194
15 9.0083391609925
16 9.23752035118032
17 9.49796549175874
18 9.68605494250528
19 9.90309188126935
20 10.2485174158731
21 10.6527955503109
22 11.1350465735257
23 11.9370464707261
24 12.8281774016792
25 13.7226450045116
26 14.4586753203512
27 15.1969844082489
28 15.9427700086828
29 16.5761611426895
30 17.1544524447703
31 17.6567532993821
32 18.0568866156859
33 18.4448188637305
34 18.8523040981416
35 19.1131291401444
36 19.3831384536805
37 19.6440806574101
38 19.9851778511525
39 20.3223565700587
40 20.6535401756181
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.195715563642212
1 -0.0843223260033334
2 -0.488401503471572
3 -0.689573889022864
4 -0.381287285216238
5 0.519890285731967
6 1.42270025738265
7 2.19245704857095
8 2.89595994251257
9 3.70702631366597
10 4.60537731852058
11 5.93890990868009
12 7.14749209808847
13 8.05147836631494
14 8.59759845893319
15 8.9371261404039
16 9.1012618583129
17 9.24904460132666
18 9.3925939650267
19 9.5339815226815
20 9.71221733353102
21 9.93044558944679
22 10.1430714567617
23 10.4765536700994
24 10.9281627718521
25 11.5523685950763
26 12.3287149957985
27 13.1623824497297
28 13.8999824667972
29 14.6224089994071
30 15.2034050043765
31 15.9154064354266
32 16.5206860757466
33 16.9665256595444
34 17.3440514788011
35 17.6659874965305
36 17.9909339185775
37 18.2927643462603
38 18.5696080128589
39 18.8983457034052
40 19.1133321377277
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.210609834525976
1 -0.0548452726693998
2 -0.501006361993717
3 -0.865964293884071
4 -0.557236326714043
5 0.318928498915017
6 1.25455675734611
7 2.12417998576444
8 2.93535882086318
9 3.8795009391562
10 4.88208994907258
11 6.29343144404447
12 7.34339383213529
13 8.17828174683116
14 8.6111879277953
15 8.86320188215069
16 8.99729112213666
17 9.14074959336086
18 9.27051625804866
19 9.282964271548
20 9.36485500212462
21 9.46510955689939
22 9.57434622705003
23 9.68598937074274
24 9.87867475577078
25 10.2330847173922
26 10.6645738704032
27 11.402874595897
28 12.1591506683196
29 13.0638606577893
30 13.9097016013106
31 14.8819338868834
32 15.7674910232919
33 16.4194605579865
34 17.0718378113044
35 17.7407146760089
36 18.4018956929336
37 19.0061966049736
38 19.5395618567848
39 19.9803036876643
40 20.4755571746001
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.206688169964455
1 -0.12415168915222
2 -0.594942184548476
3 -0.8357784166313
4 -0.575313117203288
5 0.45178301517525
6 1.31745939521333
7 2.19133807520004
8 2.88075018959821
9 3.7294154964112
10 4.86646636270796
11 6.24934020193959
12 7.4268604996482
13 8.33403430117361
14 8.93818040504176
15 9.27254603839015
16 9.55614490893739
17 9.73009689091895
18 10.044715814682
19 10.4253214058222
20 11.0375269969334
21 11.8042606703276
22 12.6508732544565
23 13.4003846189471
24 14.1429669659144
25 14.8590542308442
26 15.5294241024761
27 16.2123433507257
28 16.7860085318563
29 17.3371761224982
30 17.8250807263902
31 18.2716667604291
32 18.6687461355009
33 18.9794591665397
34 19.3839054317364
35 19.6683583698687
36 20.0045340237223
37 20.1818807035305
38 20.3907673902474
39 20.705584627138
40 20.8977664504164
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.197555665239024
1 -0.147160105814202
2 -0.573019687281531
3 -0.810391725667475
4 -0.607847770181036
5 0.32467183818329
6 1.25731224593022
7 2.03299560724507
8 2.78112068951517
9 3.60813121034543
10 4.61272627326792
11 6.0503728837623
12 7.20961041632037
13 8.12537944489035
14 8.59551494080829
15 8.83632529447883
16 8.98106728519907
17 9.08562255868692
18 9.16588588987018
19 9.20487384698112
20 9.17807356272795
21 9.16379346066191
22 9.13646190446555
23 9.11564257357606
24 9.10191693131456
25 9.10464221481364
26 9.14468852681235
27 9.22485384627711
28 9.21556444985535
29 9.17565103722822
30 9.16533292508477
31 9.11206431629641
32 9.0545536127908
33 9.05131220558506
34 9.10507493420079
35 9.08875885879898
36 9.13069396674218
37 9.11875400822505
38 9.07188897600387
39 9.09748222549214
40 9.10514447927238
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.229142291986792
1 -0.0819575297171815
2 -0.551843811699478
3 -0.783355061119182
4 -0.552689093092992
5 0.360717774270045
6 1.28892247820838
7 1.91685103757301
8 2.54089266480297
9 3.23972015307465
10 3.93149097429365
11 4.96929183902674
12 6.24363549045706
13 7.47526324080955
14 8.18027333489842
15 8.67835628637624
16 8.94861643466903
17 9.17294563748797
18 9.30093566886031
19 9.3237305446774
20 9.34490206840532
21 9.34759265940308
22 9.37050494819568
23 9.31654939508886
24 9.28684214915728
25 9.30904900472332
26 9.28673134817285
27 9.4765445312352
28 9.46279851161331
29 9.45998473784183
30 9.4087023215063
31 9.35172483292445
32 9.37796193899095
33 9.35279759235413
34 9.3689538610127
35 9.40484805181559
36 9.42779924157586
37 9.40783657838063
38 9.38998728156633
39 9.44706315168652
40 9.51050481545572
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.20174958471922
1 -0.113623996039725
2 -0.564302871306513
3 -0.896043983772964
4 -0.68671920979753
5 0.269687328798743
6 1.25569788696689
7 2.09077459540428
8 2.85957363509625
9 3.79597281391784
10 4.81998396367795
11 6.18550844840076
12 7.24099827625742
13 8.03956100078041
14 8.56360365828129
15 8.85412684388003
16 8.95096073645919
17 9.09895593312902
18 9.2301076158489
19 9.25357499255628
20 9.35210779405043
21 9.37591991355766
22 9.40425340262896
23 9.36298687285776
24 9.37373289680782
25 9.46189007086046
26 9.45568827177153
27 9.57271910590759
28 9.6199492229213
29 9.57928395982881
30 9.55100363386964
31 9.60267620413214
32 9.70510774237811
33 9.80213104928584
34 9.96847397028745
35 10.2806632970992
36 10.7093345800014
37 11.2438517566028
38 12.124664732389
39 13.023078779221
40 13.8904589918702
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.219614692096781
1 -0.0806275200246311
2 -0.517003541639502
3 -0.89397950037962
4 -0.676791065966834
5 0.251770912732555
6 1.16322337419436
7 1.8700277442795
8 2.56530661968304
9 3.45905857810567
10 4.41731263468985
11 5.8536715667119
12 7.00694722505765
13 7.98563208551192
14 8.44343048238569
15 8.76789885301997
16 8.87757243774904
17 9.00204580647225
18 9.15332728026532
19 9.20045462270092
20 9.30176020014765
21 9.3316747765261
22 9.39374305938129
23 9.44252571967584
24 9.54851864247609
25 9.64123572458841
26 9.79669786935234
27 10.1179836877001
28 10.5067326157957
29 10.9199392696363
30 11.5243452873099
31 12.3375751641512
32 13.2522357442586
33 14.0555765943771
34 14.8601052950323
35 15.5849968415514
36 16.1814075385824
37 16.7223109221381
38 17.272609126917
39 17.7514497130564
40 18.1973601357911
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.187014030450317
1 -0.14348971674017
2 -0.581228673251697
3 -0.745076113063801
4 -0.511276969304656
5 0.392666539199218
6 1.3452596425237
7 2.12458764908006
8 3.02250886382324
9 4.04176083974614
10 5.18043044626338
11 6.59860808210612
12 7.70367768553801
13 8.52835576539296
14 9.00852927290526
15 9.36591719814344
16 9.55393352084707
17 9.74793645127327
18 10.0004365600866
19 10.331178940551
20 10.7286742637148
21 11.2736462011614
22 12.0113865976932
23 12.8566668730497
24 13.7077789422132
25 14.5462192328953
26 15.2668941279055
27 15.8509592772504
28 16.4716813493012
29 16.930930236479
30 17.4582864810312
31 17.8663469123139
32 18.3803251822189
33 18.8919610905629
34 19.3541683208959
35 19.75774785619
36 20.1108760670684
37 20.4577820442242
38 20.7444842257188
39 20.9656551560951
40 21.1656348655941
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 0.222407340617103
1 -0.0792220179893691
2 -0.579478888488021
3 -0.909053204178205
4 -0.748421735046829
5 0.152901248562975
6 1.07041625393552
7 1.91751970657731
8 2.64508227288895
9 3.55512160741288
10 4.45597743663127
11 5.81614339816672
12 7.01837649757049
13 8.03621367840269
14 8.53352030631864
15 8.73890669336135
16 8.81967097873415
17 8.9167255611024
18 9.04018309680306
19 9.10619211345221
20 9.1255873913857
21 9.11135700444086
22 9.12070403727878
23 9.08562888492644
24 9.14979851180747
25 9.19787766299194
26 9.16400241557427
27 9.28094570773125
28 9.27444661415584
29 9.28407570419259
30 9.21925629655787
31 9.17190394879811
32 9.19256992668156
33 9.13571401178798
34 9.13595700916808
35 9.14978893471957
36 9.1797089694238
37 9.16433897259163
38 9.13162355609867
39 9.22207432462185
40 9.26008450111955
};
\addplot [line width=0.01pt, color1, mark=*, mark size=2, mark options={solid, draw=black}]
table {%
1 -0.216971117452557
2 -0.698311813338088
3 -0.845437931574839
4 -0.510347906996663
5 0.417785295755321
6 1.45063997856431
7 2.18000698194071
8 2.91511410045934
9 3.99138570661581
10 5.18010069663342
11 6.78065117660923
12 7.92074360825274
13 8.74285795470332
14 9.32370003511269
15 9.44974184549204
16 9.39728065453565
17 9.39942446694502
18 9.45875925073886
19 9.41596191419465
20 9.44604175500281
21 9.43595937363876
22 9.4563381291001
23 9.4069938263042
24 9.38363158073475
25 9.40550089098364
26 9.38007003255305
27 9.42642504798656
28 9.50602660780519
29 9.50516219108816
30 9.43584948844373
31 9.4053013696456
32 9.43579387299814
33 9.39838716046376
34 9.37035636536838
35 9.40687083255091
36 9.4411863522549
37 9.44827707366167
38 9.39444475031715
39 9.40444975096704
40 9.47548755380175
};
\end{groupplot}



==> experiments/figs/double_pendulum/tikz_samples_ep-14-all.tex <==
\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}

\begin{groupplot}[group style={group size=1 by 3}]
\nextgroupplot[
xshift=-8,
title={14 episodes},
title style={font=\large},
xmin=-1.45, xmax=30.45,
%ymin=1.15124371169553, ymax=6.91115994797861,
ymin=2.7, ymax=6.7,
width=\figurewidth,
height=\figureheight,
xtick={},
xticklabels={},
yticklabels={},
tick align=outside,
tick pos=left,
x grid style={white!69.019607843137251!black},
y grid style={white!69.019607843137251!black}
]
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07458395821178
1 3.43842695271583
2 3.50824142215418
3 3.30848082221099
4 2.91507354422
5 2.68900302009432
6 2.71631303282751
7 3.10319292423733
8 3.69148840572748
9 4.20579280514528
10 4.61139641036265
11 5.00726243937489
12 5.3929815996214
13 5.6397457399846
14 5.49233735764289
15 5.30770531222288
16 4.98575090528061
17 4.54983802341745
18 3.89206702116767
19 3.13512086096961
20 2.45167980383282
21 1.92708336230029
22 1.43393682120338
23 1.32621631663338
24 1.70174827297958
25 2.44327851086336
26 3.00065338135446
27 3.36962685469317
28 3.5892694521513
29 3.72303246219819
30 3.82648382587514
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07455298401178
1 3.26367600782676
2 3.36908750852189
3 3.14785318776715
4 2.83141106993159
5 2.95055051517117
6 3.45172464427015
7 3.95704245009974
8 4.47492530892288
9 4.86180225041448
10 5.17067691757135
11 5.39209703612826
12 5.55754250966347
13 5.54280109203447
14 5.49454768818805
15 5.33956616074009
16 5.11144751653717
17 4.7809390367991
18 4.49639266744979
19 4.19435389296793
20 4.06111191386178
21 3.86039720003697
22 3.58487394510438
23 3.33753343358464
24 2.7964250427176
25 2.13782116240175
26 1.40684476669072
27 0.664251595929878
28 -0.0924687730859635
29 -0.670314692055921
30 -1.20740584301595
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07386109981346
1 3.34055116498378
2 3.33471036688858
3 3.17942795637245
4 2.93986079123799
5 2.99910929774386
6 3.42735551120463
7 4.07918486085861
8 4.8190456613909
9 5.46499503133639
10 5.78904464945566
11 6.01491154611865
12 6.15451368746854
13 6.14754847009266
14 5.97831463857243
15 5.67765942313536
16 5.31284210015071
17 4.94854128238834
18 4.46361874027393
19 3.82839077356466
20 3.27444114011334
21 3.05458976097517
22 3.1932842179212
23 3.05850022447328
24 2.8813166539928
25 2.44088349985716
26 2.02190914956391
27 1.50496012455681
28 0.907376269140743
29 0.250913774525385
30 -0.293791648237187
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07456957606211
1 3.29305873983767
2 3.37532864091998
3 3.29760888420072
4 2.87644970074059
5 2.76667183124701
6 2.98581372924909
7 3.46632854307838
8 4.01631666618676
9 4.62063688536867
10 4.84334252154104
11 5.1404170766056
12 5.3854850014537
13 5.55774036356691
14 5.73422309663923
15 5.73485898839098
16 5.78874278586331
17 5.72238819154272
18 5.79307315622553
19 5.95333586373675
20 6.09061599803979
21 6.25280365439852
22 6.3864670671615
23 6.46417188444326
24 6.64257644903667
25 6.89287784588951
26 7.1009481789328
27 7.25704090256401
28 7.40443480062132
29 7.59259172395142
30 7.75733964887807
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07429772027816
1 3.40491456255525
2 3.45967500809535
3 3.42881213474405
4 3.23270851442213
5 3.21128192286495
6 3.50280081724801
7 3.80684105354063
8 4.26541602554476
9 4.62522756273881
10 4.89138057871795
11 5.10185719338553
12 5.23482626923126
13 5.36233683277246
14 5.36733178383719
15 5.34693396554094
16 5.18041957488181
17 4.93392090800666
18 4.68907290935547
19 4.43091372877413
20 4.42431642581996
21 4.40976487071988
22 4.12632446595038
23 3.65047008371128
24 3.03355073120882
25 2.42326626075899
26 1.78188490217271
27 1.23202774826545
28 0.828963903215879
29 0.405492992000037
30 -0.158651103341304
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07401902655931
1 3.42559096456657
2 3.41996796010118
3 3.20523361377886
4 2.78528524891485
5 2.65687992533902
6 3.15200262756202
7 3.7781861490483
8 4.37979583899524
9 4.79068730783528
10 5.03788272316766
11 5.16441225264777
12 5.25965268985027
13 5.26158006010343
14 5.06263780822247
15 4.7091079303981
16 4.21360665506391
17 3.52529512420985
18 2.69605494205769
19 1.90168386042635
20 1.33980116715972
21 1.31827454247259
22 1.73369180019991
23 2.40265192490682
24 3.1185331103188
25 3.78393411384843
26 4.4253351359935
27 4.90346935956686
28 5.24460266668091
29 5.40328424749348
30 5.44863877282009
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07423575535287
1 3.29482751503847
2 3.40847578953075
3 3.32492470843729
4 3.10723296689788
5 3.14226091870268
6 3.56614997474335
7 4.07261844747418
8 4.65993734393126
9 5.11249992233424
10 5.49128956484312
11 5.76059453956663
12 5.9110868835932
13 6.0209929822113
14 6.03473465406588
15 5.95313493414325
16 5.82444210152172
17 5.56615067141063
18 5.13766429950781
19 4.47109174004586
20 3.90242182431789
21 3.30818324701662
22 2.78382962173559
23 2.37497888087196
24 2.09439800764271
25 2.05193168834697
26 2.13203456565801
27 2.33767525374538
28 2.72416091768768
29 3.13492509708387
30 3.41426303407792
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07450693536193
1 3.2056325193568
2 3.27487604322982
3 3.21754854971471
4 2.89241468567263
5 2.83190042624
6 3.23539165148647
7 3.65751845520081
8 4.19875890062988
9 4.64504635472302
10 4.89862224421973
11 5.07391275327008
12 5.25691775310589
13 5.27976585395211
14 5.25784942452472
15 5.08726625849837
16 4.87425036297176
17 4.5526433906023
18 4.33255398744684
19 4.27236751184008
20 4.28560887851737
21 4.11931923159156
22 3.91340405704324
23 3.50154652351439
24 2.83640751750679
25 1.93822564855944
26 0.991290948198357
27 0.215599063948902
28 -0.364852355043892
29 -0.894728004317768
30 -1.38131425864603
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07482344080747
1 3.39657446400282
2 3.50571854502644
3 3.443794252333
4 3.10893842261865
5 3.00011031587906
6 3.05767963915362
7 3.23757831532121
8 3.66809563606713
9 4.06667456599835
10 4.26405991482723
11 4.44250315653924
12 4.5668506319037
13 4.6699924219642
14 4.61952739213427
15 4.39073883763509
16 4.01122214348751
17 3.48898862479143
18 3.1411348384913
19 2.68079210592149
20 2.26108730753169
21 1.91308516045961
22 1.52117314562289
23 1.32813906464851
24 1.27097889538584
25 1.61217021368593
26 2.20576678222575
27 2.72511166892339
28 3.2749234476405
29 3.73651967372853
30 4.13450871397661
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07478989287772
1 3.48808708143672
2 3.67753731598265
3 3.52558153617536
4 3.19199672672739
5 3.23569824123604
6 3.54238997651279
7 3.94955397114678
8 4.49725687872899
9 4.953752718977
10 5.19811529595094
11 5.40377283049455
12 5.4876920402518
13 5.63127896889811
14 5.61021285298928
15 5.40788667609604
16 5.14954947123258
17 4.80482554460412
18 4.48483334605178
19 4.23421199291344
20 4.17440124934018
21 3.98264026532783
22 3.73532560964436
23 3.37158892570077
24 2.8695116002503
25 2.33397999180804
26 1.7720438786391
27 1.23840636710234
28 0.697985460266597
29 0.222759385641258
30 -0.204406766491102
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07481615183636
1 3.40411821948077
2 3.51993791932291
3 3.42014464789618
4 3.00612405045605
5 2.87786280928826
6 3.09651143863678
7 3.405136290552
8 3.8018419987578
9 4.19147752577273
10 4.47901814243229
11 4.61183373512559
12 4.73608108608263
13 4.64650443305049
14 4.41477832413375
15 4.03494628618816
16 3.59825213270248
17 3.13781951796908
18 2.62977156392614
19 2.33219829221419
20 1.967414102792
21 1.78739473956013
22 1.67100136917086
23 1.89947370414425
24 2.19978131313116
25 2.83788063299925
26 3.36202822277101
27 3.71528390339776
28 4.05577520601588
29 4.34982272582945
30 4.58081555535001
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07462476368603
1 3.39518125337717
2 3.57619133114872
3 3.54932864648278
4 3.23881096999438
5 3.0890427936515
6 3.13603531552866
7 3.39416386341583
8 3.66502649011734
9 4.05798951607157
10 4.31087060946072
11 4.54547380247308
12 4.7700375303399
13 4.85499708454617
14 4.82806493001008
15 4.58060953720556
16 4.20290570724465
17 3.81656955458935
18 3.41900830502563
19 3.02144557471399
20 2.6425700955716
21 2.29005131068352
22 1.98150505955598
23 1.7828131410786
24 1.62195885993457
25 1.82950236812429
26 2.37821248792783
27 2.75818725518658
28 3.06386263541666
29 3.46175045741974
30 3.91042440506617
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07436307322093
1 3.34829157623408
2 3.47593178949846
3 3.41633328566854
4 3.10269166448981
5 2.96779199621327
6 3.21358880675977
7 3.50966342060384
8 3.99156489530647
9 4.49255165605567
10 4.8707174019632
11 5.23589920481206
12 5.37355025236619
13 5.45087202388936
14 5.33285290215608
15 4.93282107581179
16 4.475625886941
17 3.84838093626998
18 3.35096254289833
19 2.90753323756122
20 2.55023171678788
21 2.29003862980815
22 2.22352307610187
23 2.13324374407368
24 2.12922297732348
25 2.24644502013912
26 2.46309316501024
27 2.77019077670237
28 2.99047541003363
29 3.24617191671077
30 3.38861130403494
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07456166004161
1 3.33815665935963
2 3.44156133095998
3 3.3685178937514
4 3.06104318595551
5 2.95867075867364
6 3.21094753939126
7 3.60885329121918
8 4.17424603463153
9 4.64887118485095
10 4.91493689953004
11 5.09884523240832
12 5.31162797519131
13 5.42297379685117
14 5.45145340853213
15 5.44136219059541
16 5.37282471232029
17 5.2708720054904
18 5.1371530011419
19 4.98279248567208
20 4.70081367892655
21 4.28205637443423
22 3.79948803231836
23 3.21347460009641
24 2.57171134276546
25 2.14455734016839
26 1.94259651748226
27 1.90633805452295
28 2.17635035776249
29 2.62520666948377
30 3.25936654993082
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07356542169157
1 3.3457524083584
2 3.36344381933875
3 3.19127637836635
4 2.76035882425687
5 2.69907856882685
6 3.00658323224787
7 3.36935025213909
8 3.93395901919977
9 4.37363957651749
10 4.67990786073704
11 5.1251719929132
12 5.50475431382176
13 5.6218884583183
14 5.68659834891346
15 5.62729082727412
16 5.49685914829613
17 5.33136355856695
18 5.03177900639756
19 4.62913177005536
20 4.12781536423773
21 3.37817063671893
22 2.55288791080662
23 1.70178378830292
24 0.891312499491228
25 0.082831638956625
26 -0.505764738904624
27 -1.05065071636466
28 -1.54248768022303
29 -1.98025567633894
30 -2.34850855202562
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07446582204502
1 3.43141367811621
2 3.43421756596755
3 3.24925252597667
4 2.85763025431603
5 2.57673576982496
6 2.63636134763327
7 3.07748454433755
8 3.64183943338354
9 4.18946751331473
10 4.72953937768654
11 5.10295838718207
12 5.39845560070089
13 5.64843036087595
14 5.66354100465389
15 5.54833982035989
16 5.32936264693848
17 5.00273198207886
18 4.44188929800936
19 3.76260598730785
20 3.17956693011769
21 2.5539690843963
22 2.10442791401815
23 1.68850771988043
24 1.38739650357872
25 1.40601430040133
26 1.6687405882199
27 2.27948968126642
28 2.92305887310977
29 3.47190712213203
30 3.76912206435569
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07433053593028
1 3.49950132800515
2 3.43963843860192
3 3.18573009585806
4 2.74015952764092
5 2.61460608794589
6 2.82976652501179
7 3.38983422504613
8 4.07664451483886
9 4.65581952657939
10 5.03069880006137
11 5.27551577298001
12 5.40370706571348
13 5.46526019813959
14 5.40365271920667
15 5.26761627448781
16 4.9511175533765
17 4.51513406429888
18 3.92312077369407
19 3.38953158562133
20 2.81941333169381
21 2.45739075368279
22 2.19520734554976
23 2.06529666108689
24 2.05610245149271
25 2.22669545246626
26 2.58832333456182
27 2.89966983223716
28 3.07882375931979
29 3.25003613170012
30 3.36348912090918
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.0750999819131
1 3.37197378734939
2 3.42039653983463
3 3.34177066901436
4 3.02361791806342
5 2.88321433981889
6 3.06619850978699
7 3.25770925363888
8 3.50774958662065
9 3.87218401729675
10 4.12168994646696
11 4.27826040363688
12 4.42938866139701
13 4.33948407441433
14 4.14353500222869
15 3.86040137307727
16 3.48161697721904
17 2.99347206154617
18 2.47336013103197
19 2.14840517630223
20 2.03178667288765
21 2.11619992235875
22 2.34297873141016
23 2.75294083307695
24 3.17116781047461
25 3.54058187826255
26 3.74082833320811
27 3.82725525397518
28 3.75039676844834
29 3.57142529544899
30 3.34850641419662
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07505747038572
1 3.28721382905708
2 3.37376327347181
3 3.2838458565562
4 2.964630495063
5 2.78744099289045
6 2.98624697515709
7 3.4490979785656
8 3.96399811201016
9 4.3852319519935
10 4.65855471738808
11 4.8463546046438
12 5.04707910012849
13 5.02607209602778
14 4.76948497930669
15 4.37804819144886
16 3.85861137535652
17 3.42396078243853
18 3.07308731511939
19 2.68397798664491
20 2.37777052631128
21 2.15361028474055
22 2.19540088222112
23 2.37540642712135
24 2.63785633720964
25 3.03890354469155
26 3.41407787065817
27 3.69518123648492
28 3.87005525017066
29 3.88569790709414
30 3.90954047117578
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.0745141445467
1 3.5035463020937
2 3.73244171566712
3 3.73081141405967
4 3.39243416436891
5 3.37958689511853
6 3.59306982191286
7 3.82668591290794
8 4.17465858345615
9 4.44259490322783
10 4.70531202795061
11 4.84314541213135
12 4.89043979492022
13 4.72888484550513
14 4.40211736481132
15 3.98557682386717
16 3.61312203953024
17 3.14400775881892
18 2.48628203553104
19 2.08174874611518
20 1.69565618427103
21 1.49858230678015
22 1.4832579711175
23 1.59163918329365
24 1.86789966341185
25 2.27585671366428
26 2.7614955302851
27 3.09278502137025
28 3.32177301524252
29 3.48233587880997
30 3.57417144956052
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07410687945947
1 3.26113506822159
2 3.29468788088766
3 3.22278661486438
4 2.93269715891249
5 3.02137498990805
6 3.39969326706787
7 3.87185228078308
8 4.40828012719137
9 4.99333195311755
10 5.30173719871365
11 5.64043003260297
12 5.79150539754801
13 5.82647585219325
14 5.71135075468871
15 5.43045084719664
16 5.15265494108895
17 4.83467799523917
18 4.64207430628945
19 4.25575656774206
20 3.88213352419381
21 3.34024083043017
22 2.61915157904024
23 1.86040596876554
24 1.1057203398209
25 0.311116725683773
26 -0.492891931138127
27 -1.17174884636857
28 -1.86926369789315
29 -2.48138983472782
30 -2.95800912451198
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.0742782088235
1 3.35593095380117
2 3.41199688887888
3 3.28223601951455
4 3.02797607773059
5 2.91511135849108
6 3.15139859134721
7 3.5290262186838
8 4.00517814942662
9 4.44154685876827
10 4.73764369135405
11 4.99964869878844
12 5.17486444736008
13 5.25642081210765
14 5.20408803889694
15 5.10684000486889
16 5.0999744503944
17 5.09908889727489
18 5.00272152472915
19 4.82228335868304
20 4.56302149636426
21 4.0890205677094
22 3.49422418774755
23 2.97481994725142
24 2.4446640555828
25 1.71049588663914
26 0.958240372209293
27 0.156084818627733
28 -0.439473568786797
29 -0.96325744755525
30 -1.35877756047479
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07431976457507
1 3.45172113200398
2 3.5666404652803
3 3.51923958332917
4 3.32869989698566
5 3.27448087284439
6 3.73303489409911
7 4.2229408613347
8 4.62103772689017
9 5.01624029447717
10 5.25755518010048
11 5.58951391457891
12 5.88920407460072
13 6.08964517826191
14 6.1960797120902
15 6.21706183402904
16 6.1888993165438
17 6.20084256686018
18 6.16332945646095
19 6.22686030472115
20 6.41182052691097
21 6.5623120097506
22 6.72904112036922
23 6.82992117731986
24 6.95217399593152
25 6.97314272459263
26 6.96220256762019
27 6.98454241696179
28 6.96585458240685
29 6.99347569652307
30 6.99411938621002
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07474478280855
1 3.48272872240097
2 3.55820205542315
3 3.29155510232255
4 2.80085059213529
5 2.6419309993004
6 2.92882178109453
7 3.530572671616
8 4.40726735416724
9 5.02371105742526
10 5.47714073618496
11 5.77300166539868
12 6.02512061731678
13 6.15167995661462
14 6.13441971229768
15 6.10340979577496
16 6.03224974313715
17 5.88594649717892
18 5.5213754006034
19 5.08060355712202
20 4.52632915933232
21 3.92212323969121
22 3.21710407873204
23 2.46178867700301
24 1.87583079463206
25 1.62359025386462
26 1.57040319810602
27 1.72526035116909
28 2.21312936933321
29 2.82148138255895
30 3.43064747608609
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07360796648904
1 3.47583504556008
2 3.57920135558315
3 3.44210910992122
4 3.19634356013108
5 3.28172422400821
6 3.79778411466344
7 4.59272027844753
8 5.24451130741805
9 5.5803542075216
10 5.75332355974234
11 5.8420690621407
12 5.74059393668898
13 5.57545657485719
14 5.27685136781518
15 4.89072358810955
16 4.51672261056949
17 4.23555634764412
18 3.96420714522583
19 3.4163182626651
20 2.67661566030561
21 1.95177726371054
22 1.21317945978291
23 0.541739619725806
24 -0.0608382756896173
25 -0.687949872469471
26 -1.1367240981981
27 -1.5728329027538
28 -1.87855716016626
29 -2.26468762055889
30 -2.65291375421318
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07478025156005
1 3.37247676908155
2 3.47282273198264
3 3.32920506098485
4 2.99248223134938
5 2.85343186386402
6 2.81992639048991
7 3.01633306327766
8 3.45605003711777
9 3.91215908220462
10 4.36738099305296
11 4.7482934304189
12 5.08842086796597
13 5.09306787030293
14 4.92829788584977
15 4.57271580933449
16 4.00615634079892
17 3.35523979428385
18 2.76493848100426
19 2.31160728543613
20 1.98629199083193
21 1.8455003597127
22 1.96857026538666
23 2.24109975342328
24 2.52494973098445
25 2.7653876221335
26 2.96513230667994
27 3.15355120811969
28 3.42459046702156
29 3.84993281601827
30 4.28528954205979
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07428167731135
1 3.33765120160318
2 3.39392748432742
3 3.19962503678144
4 2.92031656685781
5 3.06265875419193
6 3.55670814306263
7 4.14395119127482
8 4.79982898381014
9 5.24379855222101
10 5.63782950606935
11 5.92967818809766
12 6.07438726627055
13 6.10061689065718
14 6.0665643105176
15 5.86232303195357
16 5.51812045055007
17 5.26893593356569
18 5.0235616706205
19 4.86671489823584
20 4.74068550098334
21 4.4743495605491
22 4.01681580057286
23 3.41072420032041
24 2.58836467185148
25 1.86356252540301
26 1.16113243663089
27 0.47263626300413
28 -0.102507919721424
29 -0.567039160673827
30 -0.986708660943581
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07430139392598
1 3.3279951270322
2 3.41462483114947
3 3.39582028249731
4 3.05772885496191
5 2.91523295733648
6 3.19216803431779
7 3.57187011683705
8 3.95052095911065
9 4.28417529318744
10 4.5932114736417
11 4.91540635495386
12 5.21446211049937
13 5.13457272852023
14 4.92722261834072
15 4.6543865512152
16 4.32860147928836
17 4.02013259755715
18 3.68516612890073
19 3.32974451892208
20 2.91991972414013
21 2.55068680902525
22 2.14582519937043
23 1.6978552904371
24 1.39665880563472
25 1.56714771173792
26 2.04313503494014
27 2.64017950573083
28 3.28955780902192
29 3.87308805119438
30 4.25843792267929
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07541341047704
1 3.37143179457058
2 3.44554374375319
3 3.3426815534291
4 3.00688506074656
5 2.95846270468749
6 3.27738163348602
7 3.61750668124643
8 4.10621298678739
9 4.57260358127212
10 4.83246022201747
11 5.09851512817782
12 5.22804166507571
13 5.31129143194475
14 5.3139860349089
15 5.23036759935415
16 5.04508420488503
17 4.93396806126614
18 4.76110626387127
19 4.66596008918908
20 4.7353910643107
21 4.56796082715607
22 4.16238394900652
23 3.56769856516177
24 2.86868552352914
25 2.07076930880679
26 1.19868796416452
27 0.491275903092463
28 -0.0250342317084566
29 -0.559404952657458
30 -1.02756999660197
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07463513400303
1 3.35796282255327
2 3.44468616669271
3 3.30488442499199
4 2.89347084820779
5 2.74157261472043
6 2.9554399450356
7 3.35516151222904
8 3.96383382905845
9 4.55207342212688
10 4.95972065225678
11 5.37624427666605
12 5.58242129348526
13 5.56197147153838
14 5.4371027410268
15 5.20333551242183
16 4.95453205373391
17 4.78582311627796
18 4.76978328254346
19 4.80099790392162
20 4.70525677101994
21 4.46295190567962
22 4.01447415640571
23 3.51187388970721
24 2.76113843214392
25 1.79057356277869
26 0.822732461186506
27 -0.152614958557576
28 -0.939390551783353
29 -1.75785647244728
30 -2.4596682484199
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07397257763869
1 3.28877828383039
2 3.26669786678994
3 3.00829565624052
4 2.60061719384517
5 2.6429668010936
6 3.04076168166287
7 3.78385339638383
8 4.60872463594757
9 5.05733935031467
10 5.39343367533234
11 5.67168760472367
12 5.97955207044884
13 6.11945125419346
14 6.1368798710315
15 6.02494458699433
16 5.67828416322147
17 5.25321133973244
18 4.75136997200059
19 4.0936776389482
20 3.36459880003405
21 2.67209815619246
22 2.01620105990314
23 1.49461710670199
24 1.35880866852753
25 1.41149925439462
26 1.79492398626817
27 2.44762951104023
28 3.10449096053115
29 3.80196204475084
30 4.44862032811366
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.0746896535713
1 3.37002068960759
2 3.46010874990343
3 3.42334957676631
4 3.11090154678212
5 3.11230431904036
6 3.34450030424497
7 3.72945593728149
8 4.23850860546644
9 4.57825076048046
10 4.90289582420895
11 5.2968851037079
12 5.49405413246081
13 5.6550055821704
14 5.73956979139028
15 5.52866706494258
16 5.075555731825
17 4.53964788467709
18 3.78272805044524
19 2.95236156562088
20 2.15272040300613
21 1.51959861446882
22 0.831384560578787
23 0.176269898489616
24 -0.402781803161549
25 -0.863433066515004
26 -1.37553521484929
27 -1.72523388596158
28 -2.00598877570389
29 -2.24522547463539
30 -2.35635163148877
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07486851648212
1 3.31092989762893
2 3.36908653887218
3 3.30917801476561
4 2.98366481366291
5 2.94398971840718
6 3.20164995413065
7 3.57460017851969
8 4.14938021028324
9 4.56836093445132
10 4.88562637971217
11 5.2046431273788
12 5.45593931044847
13 5.40357928118618
14 5.36419956012341
15 5.19763448677578
16 5.03559724482108
17 4.74883039213399
18 4.32755862240783
19 3.81722083245776
20 3.22944545174269
21 2.69824372575768
22 2.57730876747266
23 2.63870366902946
24 2.65655819231339
25 2.49108415415461
26 2.00549088046277
27 1.3918263527968
28 0.772333506471975
29 0.181195593624821
30 -0.377472399055263
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07427548421694
1 3.44211530682883
2 3.57523393892121
3 3.44266918951083
4 3.17826646673825
5 3.16704629548209
6 3.4893696632025
7 3.89271231351289
8 4.4324668684597
9 4.85434936854845
10 5.1654525746689
11 5.38188138443068
12 5.49769797101611
13 5.35993331545059
14 5.22209105933546
15 4.98729319435731
16 4.71454584120234
17 4.40864989768752
18 4.18959761969877
19 4.00471588008765
20 3.87794445901994
21 3.78687617321219
22 3.5467951213618
23 3.14968305633161
24 2.54769628699081
25 1.69145778592698
26 0.770249042904156
27 0.0622966687920705
28 -0.624876072631041
29 -1.18772888499638
30 -1.70506362355198
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07412383241666
1 3.31476059824481
2 3.38433062412464
3 3.13820200526544
4 2.81470298062402
5 2.75479324763785
6 3.06059964668865
7 3.47322677249409
8 4.1438485751185
9 4.69330281283276
10 5.04910208372276
11 5.32854853723809
12 5.50033683673559
13 5.57903013053026
14 5.61703198235715
15 5.58527110608057
16 5.37818775298801
17 5.2813036207482
18 5.19000289600136
19 5.0506974951465
20 4.76111392675677
21 4.40446606916666
22 3.82583372810567
23 3.16176382709587
24 2.47400281850023
25 1.72503845967468
26 1.04569563642247
27 0.496629018526367
28 -0.131784894131407
29 -0.698838534165446
30 -1.18032330362436
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.0748776992302
1 3.28229093008656
2 3.27759906966079
3 3.12765991213953
4 2.78133819140458
5 2.70429777658533
6 3.11762272908182
7 3.69795333019183
8 4.32244784262699
9 4.846120660956
10 5.16984143771364
11 5.48589190416605
12 5.7609083498122
13 5.77966269552053
14 5.86549431268907
15 5.88723474479428
16 5.93886315809079
17 5.96761637209387
18 6.02792426749822
19 6.11383419635909
20 6.13685438764973
21 6.25390275631856
22 6.29782902583703
23 6.40073372113111
24 6.52343368351237
25 6.55080125801379
26 6.62577621066867
27 6.70030450745383
28 6.82469956154714
29 6.94797522573258
30 7.07161699727619
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07399436226576
1 3.41980236496188
2 3.51397993436953
3 3.38312423686296
4 2.94045765657137
5 2.84220332254838
6 3.11963093062519
7 3.78585903303646
8 4.61274358280828
9 5.12787241545267
10 5.44084634245768
11 5.69092801681874
12 5.86438291762693
13 6.04723219588199
14 6.05319221569835
15 6.11681372070935
16 6.132361938448
17 6.2092857808435
18 6.32359525317843
19 6.49402990698783
20 6.63293007188893
21 6.74961320735823
22 6.85778475035741
23 7.00825160757248
24 7.26574047808574
25 7.5345475507695
26 7.78965177423994
27 8.07618389843468
28 8.33323515671856
29 8.49832427591681
30 8.73636542703618
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.0748446854687
1 3.32050985618717
2 3.46163428450238
3 3.34813262297948
4 3.07564732317847
5 3.09611030157971
6 3.45303185384128
7 3.87483398994195
8 4.36939973778366
9 4.79451516033147
10 5.07892646025517
11 5.33988484333837
12 5.53369866204792
13 5.66153433937542
14 5.59340928854328
15 5.58227698408312
16 5.40552849679456
17 5.34470389078711
18 5.19014231937326
19 5.04860270781234
20 4.94494787959363
21 4.88834967357067
22 4.85329696358845
23 4.77776604172463
24 4.71381934987212
25 4.43164951771297
26 3.96744034548705
27 3.35560629541231
28 2.75047990581617
29 1.93959551681047
30 1.14238705237606
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07515714900649
1 3.47482129277008
2 3.52598586285353
3 3.29826176015917
4 3.01146587172312
5 2.95790597679976
6 3.12197529565923
7 3.35404349542945
8 3.79393292702496
9 4.26045943605601
10 4.68684290652835
11 5.01737938612209
12 5.31469988796184
13 5.44125135754056
14 5.37988226489533
15 5.18700527815842
16 4.92365812954322
17 4.63082521582677
18 4.03170583858523
19 3.33796827150322
20 2.62490909436766
21 2.0743586567059
22 1.74882231504917
23 1.78995911289999
24 2.06001743426675
25 2.60168069327928
26 3.17416649423563
27 3.60500050975342
28 3.93759751427037
29 4.16873199357639
30 4.50033286819049
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07441908487466
1 3.39237576761714
2 3.49511552840808
3 3.35556146404251
4 3.05845018970799
5 2.95230108417928
6 3.12051423214904
7 3.51055526659829
8 3.91733881667577
9 4.20043550657893
10 4.43843471369365
11 4.66044379522195
12 4.81649305952834
13 4.7508415789709
14 4.59248562929406
15 4.36373532450529
16 4.0590619845026
17 3.75141277678872
18 3.41331946592607
19 3.09248271675645
20 2.6119621515424
21 2.16640712489188
22 1.84646215404744
23 1.5352354980472
24 1.62984014868582
25 1.84828076468453
26 2.33350342239719
27 2.91217359996258
28 3.35286876627358
29 3.8767199607171
30 4.51793202237482
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07446890994927
1 3.38264526186443
2 3.43033114009669
3 3.35582118891624
4 3.02256151758702
5 2.97388017167097
6 3.30826233040717
7 3.7915108874427
8 4.48378580830377
9 4.93090994853127
10 5.21133536597778
11 5.37604117196448
12 5.57529803203664
13 5.60689304590035
14 5.47300224334503
15 5.17054536654264
16 4.76298158291374
17 4.37996125039097
18 4.01248653023896
19 3.94826153374325
20 4.08710954373014
21 4.02680901668591
22 3.92173012709079
23 3.50483983305087
24 2.93480170307171
25 2.30318789621191
26 1.59801359473868
27 0.869474978299303
28 0.378453826347187
29 -0.196812537472017
30 -0.72186738980208
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07440564977715
1 3.55440777431523
2 3.53550658187788
3 3.29572799894708
4 2.97518729712725
5 2.96467310887765
6 3.17267625478677
7 3.5086235253074
8 4.04645907742637
9 4.58883928636719
10 4.86547612140454
11 5.20489221950006
12 5.358403780748
13 5.37526602940784
14 5.16680081318579
15 4.92350413280248
16 4.654143620815
17 4.40717129779764
18 3.99280183142087
19 3.56211600758637
20 3.14877047412191
21 2.74724834998984
22 2.3362026000599
23 1.83889805730134
24 1.59089633557334
25 1.45556174352975
26 1.34646169336365
27 1.43992587401362
28 1.76361917094696
29 2.26316362544424
30 2.86213526529713
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07428957199559
1 3.32374239484348
2 3.51610354606739
3 3.42315625201908
4 3.10270692018809
5 3.31999278376565
6 3.72007105817528
7 4.54187225855219
8 5.35539520801593
9 5.68388027518602
10 5.89230692779786
11 6.14039562596581
12 6.32281340557061
13 6.4650847961074
14 6.38137307801866
15 6.31306121185055
16 6.28163245637542
17 6.33892618814602
18 6.37955697858618
19 6.50995203687498
20 6.74797031751983
21 6.97250807555665
22 7.1154064005943
23 7.33833100767761
24 7.53039668501685
25 7.75419472641891
26 7.97049961677819
27 8.15058150659128
28 8.36502656470956
29 8.59841159901186
30 8.81953030023574
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07453868258244
1 3.37703220210587
2 3.50341164489175
3 3.29773477086986
4 3.05572502307679
5 2.85289405131265
6 3.13842628024151
7 3.81371559213941
8 4.55601391778556
9 4.95691016146037
10 5.17079189605777
11 5.4677336578787
12 5.63877796630543
13 5.6610484477668
14 5.64686140003562
15 5.55410318866581
16 5.4560829773303
17 5.32924318266669
18 5.23203274248979
19 5.0529471703259
20 4.87626980166666
21 4.74211994647214
22 4.62216061906583
23 4.60603393926976
24 4.64857487400149
25 4.58797308339053
26 4.34461668631799
27 3.94434359002818
28 3.36480405089431
29 2.66449676844497
30 1.9006561870086
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.0739160511541
1 3.48794067986512
2 3.52148541438604
3 3.31917796778852
4 2.88054538154032
5 2.88049971774508
6 3.16550921255681
7 3.56770751809345
8 4.25244482054901
9 4.69067753285052
10 5.01756171926475
11 5.33283883757267
12 5.64333208694738
13 5.79981752366227
14 5.86880963780854
15 5.84310500892518
16 5.77175162485278
17 5.68802029077101
18 5.63311497789594
19 5.59538141483364
20 5.6859226630195
21 5.78404839027728
22 5.79508530707104
23 5.86408884849731
24 5.89899780232932
25 5.91058549852334
26 5.99634575047457
27 6.00675614969367
28 6.05700576712279
29 6.12374798053983
30 6.21701263285882
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07412237643855
1 3.49855047865673
2 3.65199580602005
3 3.53691101224455
4 3.20527633781191
5 3.07712103835024
6 3.28874248715811
7 3.45227409476144
8 3.70630429577836
9 4.09835046706032
10 4.23554479278365
11 4.25591048754395
12 4.12098941452726
13 3.83470197725156
14 3.51458619662995
15 3.24706471708165
16 3.01305049631886
17 2.76072729477087
18 2.51699105248108
19 2.39814555839672
20 2.40015491318065
21 2.3488791808291
22 2.44176842522002
23 2.48583740588988
24 2.57132095775722
25 2.72566105846368
26 2.89052590902663
27 2.88452275353795
28 2.88942345827153
29 2.92647991549285
30 2.96036250694346
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07445012531701
1 3.43111319649481
2 3.54980822258948
3 3.48914620505119
4 3.13710068511375
5 3.08480371152096
6 3.14598160844731
7 3.28262174178063
8 3.61627073423719
9 3.96164629643577
10 4.30369864611146
11 4.67061443503282
12 4.94619865018876
13 4.93464223554776
14 4.78097518219877
15 4.4623981411095
16 4.02988728689787
17 3.49971145351394
18 3.07746397156283
19 2.84028368168604
20 2.71951880688633
21 2.58477119963683
22 2.4471412365999
23 2.30625125948508
24 2.27819370218397
25 2.36341629323241
26 2.61328996275603
27 2.89285392894715
28 3.19381118572997
29 3.48966376432787
30 3.60096536905577
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07444807063363
1 3.34811022584986
2 3.51855805363059
3 3.3543032234612
4 3.05147456715712
5 3.03740432898931
6 3.39028787207682
7 3.72294805839152
8 4.17378303996808
9 4.57019862032865
10 4.79942970466099
11 5.1429870716209
12 5.31788387540676
13 5.43804049888805
14 5.40672568766889
15 5.35301156896099
16 5.3088934134468
17 5.32603632362991
18 5.43166306317924
19 5.40469161522228
20 5.23800504528799
21 4.8993846918639
22 4.52008039987424
23 4.0923781716082
24 3.4569838869397
25 2.69908609187427
26 1.91702219333271
27 1.19488520745905
28 0.417441695304182
29 -0.351779757000672
30 -1.01566297829915
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07443486162751
1 3.36360632130748
2 3.44418922790644
3 3.3495412156806
4 3.09071866948624
5 3.14967800387812
6 3.45497611204412
7 3.98003047687078
8 4.56846553465083
9 5.21527956822939
10 5.71974402196027
11 6.14154409600884
12 6.42028437468953
13 6.5479432185948
14 6.54836836663152
15 6.51111560742793
16 6.44624357111461
17 6.40427655245436
18 6.36430275766538
19 6.30608719962474
20 6.29531952136386
21 6.16108010833057
22 6.11859018713123
23 6.14324196362232
24 6.17262763566874
25 6.20632585887911
26 6.1961421559473
27 6.17956049151933
28 6.15688400067982
29 6.07949553072963
30 6.05991882076034
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07488144955929
1 3.37402090976931
2 3.45989912821021
3 3.40655724486662
4 3.10979983545375
5 3.08021325674419
6 3.44087799110654
7 3.96856969340507
8 4.57582570258191
9 5.03979252410004
10 5.25632715281098
11 5.53857640649675
12 5.75649969216431
13 5.7618615545369
14 5.79453425052317
15 5.68518388767864
16 5.48623509972083
17 5.36735387881566
18 5.29497635260106
19 5.19928453787494
20 4.99916862483413
21 4.64244355986819
22 3.91779987792457
23 3.11432497277295
24 2.2417116058085
25 1.31009485926108
26 0.421922994154423
27 -0.164483231701361
28 -0.807294388496826
29 -1.48374696487322
30 -2.13441220252512
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07430869876728
1 3.40082927128079
2 3.47431386444148
3 3.29801360418307
4 2.91008842244329
5 2.89130046678561
6 3.08207431763836
7 3.5349578702083
8 4.10013391274559
9 4.66777304162109
10 5.0557923765852
11 5.40898109542094
12 5.69131245271052
13 5.7524019393059
14 5.76261561827946
15 5.67419561679041
16 5.53455699823842
17 5.29275127395045
18 5.10686252896293
19 5.00260409385507
20 4.91521587580917
21 4.72923403590357
22 4.417682083171
23 3.87516746965454
24 3.36996204459011
25 2.68207997806618
26 1.96039889079256
27 1.451004837478
28 0.958313537258281
29 0.415685035327606
30 -0.20518441631236
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07395575662968
1 3.38522459986585
2 3.49583092663155
3 3.39423408316598
4 3.03379776259032
5 3.03589374464171
6 3.30905833646205
7 3.79884226742303
8 4.41176773195858
9 4.78647268562339
10 5.02473013539865
11 5.20672599135187
12 5.46946712837003
13 5.72839304438635
14 5.78892661243452
15 5.79034840209839
16 5.7769395104771
17 5.67788299298969
18 5.37984552143728
19 4.92930516450937
20 4.30973187406722
21 3.63636502736628
22 2.91547562250882
23 2.10745595726064
24 1.2519722379627
25 0.267408214367117
26 -0.584229227783887
27 -1.4301717912076
28 -2.1894479540962
29 -2.90825851174302
30 -3.62401765663162
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07441381946416
1 3.49365006137801
2 3.64545358020171
3 3.40710924735795
4 3.06459842857348
5 3.11194170907519
6 3.5139803977384
7 4.10169443549705
8 4.64662516456517
9 5.03752692335105
10 5.31614224684777
11 5.60036883653584
12 5.8177049770084
13 5.84119691821065
14 5.66588060800222
15 5.40702482441344
16 5.15257025364319
17 4.8031756689141
18 4.38740212088707
19 3.71726142090484
20 3.08959927190844
21 2.27298064430365
22 1.40770295185869
23 0.708188247236547
24 -0.0529243897274103
25 -0.93487433716103
26 -1.75047424556168
27 -2.48950751125079
28 -3.23058480867773
29 -3.76138211463074
30 -4.31362810856929
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07409328116475
1 3.31770757173792
2 3.3887832901278
3 3.32431255259151
4 2.95919004894839
5 2.86639990583029
6 3.22551362781337
7 3.59398101929259
8 4.17435665901372
9 4.7046745125853
10 5.03507753004539
11 5.27264036356583
12 5.48109266417981
13 5.68271864888999
14 5.81753723743885
15 5.87071691837425
16 5.87433090211698
17 5.77484481690973
18 5.64493085557857
19 5.59983752329568
20 5.47717861190041
21 5.38553367460992
22 5.18131093252235
23 4.88425059949995
24 4.65215633481853
25 4.47975631964013
26 4.19265737061265
27 3.98470112888234
28 3.56161153147546
29 2.99830581868369
30 2.22054664383168
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07411913053342
1 3.4787302189176
2 3.63535890612891
3 3.45174600339202
4 3.05609956559353
5 2.98352345215625
6 3.17001018956335
7 3.44642621460962
8 4.00257327139305
9 4.53210301641238
10 4.90701579888526
11 5.20566853687516
12 5.59756962000408
13 5.79173914016951
14 5.90896160515837
15 5.95362560933787
16 5.93875553276531
17 5.90833361883993
18 5.83277952742021
19 5.78795140764246
20 5.71320950996077
21 5.54564664007713
22 5.45551389456102
23 5.31785584727681
24 5.21368632509438
25 4.86902930628013
26 4.52875391571622
27 3.96482033844068
28 3.24772329604588
29 2.34099057459732
30 1.27544939464967
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07442550436322
1 3.34363475842286
2 3.24323509376294
3 2.9468694888662
4 2.54681889026077
5 2.47211998503988
6 2.89141465042869
7 3.38967253642919
8 4.29228189374839
9 5.04539384300465
10 5.51250612929933
11 5.88656789386421
12 6.2082521727601
13 6.38647708458126
14 6.43356375854185
15 6.46917617215913
16 6.41657970885108
17 6.27988232406913
18 6.20036881725482
19 6.20819151340867
20 6.26452064146759
21 6.31191940078816
22 6.37353970309606
23 6.44574723641359
24 6.64663616290231
25 6.75710986672419
26 6.85913651656276
27 6.96255831585379
28 6.95725272538771
29 7.03205152139446
30 7.02812027528687
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07390930715097
1 3.27633189855561
2 3.20064261162379
3 3.03682033526118
4 2.6745590820254
5 2.51725926339638
6 2.89863484894666
7 3.52075213177028
8 4.39146376442704
9 5.01094649736238
10 5.44675200506464
11 5.77834944639354
12 6.02527010366943
13 6.0554264219508
14 6.04204430160914
15 5.85973975771546
16 5.6725060493243
17 5.44641934176084
18 5.12263409185941
19 4.6591006557831
20 4.12585639708954
21 3.52123853257187
22 3.04377688596833
23 2.62022573992197
24 2.32127235523367
25 1.91254622440101
26 1.60599741271558
27 1.4637553613745
28 1.62537821352796
29 1.95325554264197
30 2.40044092131695
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07520095065168
1 3.33570605863621
2 3.39823168206817
3 3.3026841452434
4 3.0159796773558
5 2.9162380381582
6 3.18162784476752
7 3.65991421074387
8 4.25523882111411
9 4.5880596091448
10 4.8421429774749
11 4.93950382312524
12 5.01422186833245
13 5.06442746401813
14 4.91721236370008
15 4.69325243271091
16 4.25972354746393
17 3.82405647017464
18 3.27389843278565
19 2.7647749733422
20 2.30992560552383
21 2.04499589454204
22 1.95637448399762
23 2.05791675483644
24 2.34434904214316
25 2.78560364378709
26 3.13627133441151
27 3.40377409168921
28 3.68412078081045
29 3.99653867741613
30 4.31140945831411
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07461915832465
1 3.35164719850738
2 3.38760497959038
3 3.24521479887849
4 2.92340717799657
5 2.74391011990155
6 2.89966500121683
7 3.26858235925441
8 3.77756843472039
9 4.34758098902332
10 4.85125582503993
11 5.21646101436086
12 5.50578385782567
13 5.68927482707859
14 5.70252660664437
15 5.63964135430101
16 5.48166514923325
17 5.27719976718037
18 5.03569465984678
19 4.70095658452645
20 4.24100029286547
21 3.82865867448972
22 3.55051149989436
23 3.56715448830164
24 3.6610943545918
25 3.55180008731219
26 3.15150762145569
27 2.60302288271755
28 2.07519295750211
29 1.47708230586815
30 0.915235401660228
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07427742874544
1 3.42235888910301
2 3.52947576214839
3 3.33221468715742
4 2.95844210852862
5 2.91845280732225
6 3.17092249614277
7 3.59430002248945
8 4.17177836469006
9 4.59535537104826
10 4.93354987112232
11 5.25790228135535
12 5.50234366582184
13 5.57873962404816
14 5.48852742499932
15 5.3473450687233
16 5.074502753375
17 4.79658534931084
18 4.6781283784158
19 4.6076501943112
20 4.43266650750917
21 4.187266919018
22 3.76678880293999
23 3.29554653592224
24 2.81467832862339
25 2.3003222795956
26 1.66818759264818
27 0.904237894888581
28 -0.0615971410975575
29 -0.979317349899713
30 -1.79403314799782
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07459613900966
1 3.41542845464903
2 3.48675868334819
3 3.30924155283423
4 2.91326758199284
5 2.85745500347261
6 3.12349796057989
7 3.64938726603402
8 4.25748325495559
9 4.79355961213772
10 5.0765190397203
11 5.4765719393389
12 5.74409597159116
13 5.84386724947542
14 6.02004905003783
15 6.04723552414779
16 6.05856302349957
17 5.9295320307243
18 5.84621688158452
19 5.60461932174703
20 5.26724247062344
21 4.74388983902497
22 4.09233893309133
23 3.33123452433498
24 2.50996862728568
25 1.86242810804722
26 1.39848503433541
27 1.26213627274558
28 1.44292793867506
29 2.07423842692245
30 2.72720889745005
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07424080804703
1 3.48363731696564
2 3.33153812174487
3 3.071765542146
4 2.71293660536634
5 2.71455357976201
6 3.1266943058323
7 3.78172224512963
8 4.5963761628066
9 5.21726381772548
10 5.63303079174878
11 6.04789258434094
12 6.26339866313119
13 6.46221842157186
14 6.38507545112661
15 6.31513181289239
16 6.19466836953645
17 6.07195913348522
18 5.96654562244996
19 5.76897265568507
20 5.33992250221058
21 4.84163048320332
22 4.30544612118115
23 3.76051858579661
24 3.20943228314264
25 2.72631295088586
26 2.23184390883046
27 1.87618886537306
28 1.66251666256292
29 1.67548673448616
30 2.04580142857654
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07494287355682
1 3.3920675955872
2 3.52826432888655
3 3.49152253229783
4 3.2318221721353
5 3.22092285435808
6 3.41623637409973
7 3.64993701603411
8 4.10538544179607
9 4.53045999121242
10 4.89122487213626
11 5.19905207655255
12 5.41698485883255
13 5.54823567663672
14 5.60806774183014
15 5.59706275022494
16 5.53691770626627
17 5.37502273445701
18 5.06474975282867
19 4.62353233633107
20 4.10945751292897
21 3.54239785494891
22 3.2029710780398
23 3.00309278124656
24 3.21315076732566
25 3.20699620663101
26 3.01231772016148
27 2.756610264997
28 2.20902685346465
29 1.48849866909709
30 0.931341180332391
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07450305023761
1 3.46970393636011
2 3.51603723984989
3 3.45460402689076
4 3.23658872909956
5 3.31688878167349
6 3.7360158873466
7 4.27092946411306
8 4.91137709211757
9 5.28777403203298
10 5.47344324617784
11 5.77345387265164
12 5.92978713850831
13 5.98517073073878
14 5.90242044823655
15 5.82585909684879
16 5.63798945836293
17 5.60087785240666
18 5.56643847726336
19 5.56211780467056
20 5.53092176735579
21 5.48635345777229
22 5.41865664427088
23 5.34682243660264
24 5.32065297248355
25 5.31295942866329
26 5.1603367484787
27 4.96893959988643
28 4.56094391792597
29 4.01452054101704
30 3.39796724074193
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07468043422452
1 3.34106716882065
2 3.55828450990806
3 3.60621769530258
4 3.51408025911961
5 3.56505888920961
6 4.02716333051242
7 4.55929135495405
8 4.99575505575431
9 5.06202040640844
10 5.17055227500596
11 5.17865318743859
12 5.01270408742802
13 4.82197666191316
14 4.349850369928
15 3.66588155101243
16 2.92892854770317
17 2.02290589027614
18 1.16928436332629
19 0.192651827881681
20 -0.682977897227465
21 -1.28332071890043
22 -1.88532995160063
23 -2.40245126990133
24 -2.85610623172922
25 -3.17960116566989
26 -3.37725412097649
27 -3.52052198795921
28 -3.60744108547927
29 -3.60810231049609
30 -3.51157239706893
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07452869519567
1 3.36377952843297
2 3.47354523547966
3 3.39632404337646
4 3.09762381816302
5 3.03130726977261
6 3.3539108288343
7 3.65884348156156
8 4.05118298990003
9 4.48642041874498
10 4.69236141076502
11 4.99796040384896
12 5.15345362017534
13 5.20026154135682
14 4.97912500037186
15 4.6193270270715
16 4.03517103501201
17 3.44825120580564
18 2.87658854897414
19 2.34515017640937
20 1.92667754640073
21 1.636117334235
22 1.66171935564473
23 2.15255697085429
24 2.68678260465305
25 3.04889285534859
26 3.30034336902385
27 3.5047306553637
28 3.66640696254239
29 3.88417212310576
30 4.09526994194199
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07516382983076
1 3.35615505814889
2 3.47592162878598
3 3.40392131212284
4 3.07478648243585
5 3.03344260338249
6 3.32993224616485
7 3.92164191105126
8 4.62032925208488
9 5.15672940444164
10 5.58221501216323
11 5.9401276439394
12 6.14461244267113
13 6.29231690959527
14 6.38957708466433
15 6.44455035769634
16 6.45757293072772
17 6.46652761288302
18 6.47036285058627
19 6.57074082364034
20 6.59449059329639
21 6.69620930810232
22 6.8475127582674
23 6.91885921731603
24 6.94372795692659
25 7.00357094895128
26 7.12960802427957
27 7.31550474664185
28 7.46885960117956
29 7.595973730136
30 7.71007909305788
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07399698626967
1 3.34607956436482
2 3.31552041054036
3 3.13264827272908
4 2.80268297830221
5 2.6700940412796
6 2.75758206580696
7 3.06856630650734
8 3.42634406681858
9 3.83648748199022
10 4.19959279671169
11 4.46961553880353
12 4.63535328268849
13 4.66510053826459
14 4.75292450237867
15 4.55028802488821
16 4.19734449134478
17 3.7468340017339
18 3.19469785278507
19 2.65792486915834
20 2.23573004168575
21 1.81579216333281
22 1.52338875796908
23 1.42031105393222
24 1.64338986855488
25 2.1790258153758
26 2.63670954731888
27 3.09126288442221
28 3.38994924972217
29 3.69120277152295
30 3.85177444366881
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07472825120125
1 3.40052924955956
2 3.49024231242911
3 3.39722214123756
4 3.0098774599021
5 2.88130168974429
6 3.05496237710166
7 3.35929918605842
8 3.86345084137134
9 4.26766707463198
10 4.5329034772958
11 4.73838538326181
12 4.89216312513081
13 4.91132284171334
14 4.80451816629441
15 4.51535181474935
16 4.1348255002376
17 3.57686215547118
18 2.93071034882238
19 2.41157809536779
20 2.11613820648085
21 1.82490618781633
22 1.85803620154138
23 1.98619064740049
24 2.25760234315965
25 2.85634202389593
26 3.34709105773901
27 3.79268539169302
28 4.04105507890865
29 4.22537564594096
30 4.43636816109268
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07480728139423
1 3.36216937043041
2 3.43713560025156
3 3.25533109096263
4 2.90447231608107
5 2.66815672711394
6 2.98294353621034
7 3.52411794097606
8 4.23037642609292
9 4.74706733523776
10 5.07954084363925
11 5.52265316590037
12 5.72599877004122
13 5.8018745601614
14 5.82450537636043
15 5.83919470942617
16 5.76356960449043
17 5.72469312324208
18 5.64009498051413
19 5.59598058273451
20 5.59576274493103
21 5.60625519110499
22 5.69127890975563
23 5.73860620316757
24 5.77144704736973
25 5.83302319599676
26 5.86048374124452
27 5.78465840900202
28 5.76732226803059
29 5.71821213831531
30 5.58689256576342
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07415638601071
1 3.39398377890652
2 3.5086692769126
3 3.39219491490302
4 2.9321629892049
5 2.82376809679267
6 3.08890919821548
7 3.58823137249688
8 4.35493234275497
9 4.83758171714042
10 5.13552538233443
11 5.33915754807269
12 5.63615437311081
13 5.71247812970342
14 5.62959490480031
15 5.45478126176043
16 5.26849265442814
17 4.9727792526249
18 4.79656336989564
19 4.68058784261509
20 4.49579711214702
21 4.23087447899751
22 3.73555664759068
23 3.18084620154327
24 2.50678509584508
25 1.88747398864574
26 1.39199066273805
27 0.810193608334879
28 0.398811294494195
29 -0.0584941409998034
30 -0.518512854628895
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07480778073586
1 3.41278107844661
2 3.48613366624223
3 3.41685702645249
4 3.09415841554414
5 3.12120016895965
6 3.3140722313252
7 3.62539299408717
8 4.04441368527446
9 4.3577570473447
10 4.56434479952136
11 4.716152923323
12 4.64946290021394
13 4.45481493429122
14 4.01321681490878
15 3.52966393318359
16 3.09020676558217
17 2.74995981171903
18 2.34263466293249
19 2.060152704806
20 1.93227369056636
21 1.88460814527024
22 2.09518931189561
23 2.51098773101613
24 2.80702205911208
25 3.06030223822339
26 3.1965065756303
27 3.42473666520544
28 3.81954593524634
29 3.93592846530017
30 3.92320875866656
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07406825896482
1 3.38230723688738
2 3.4276894023365
3 3.27692795650426
4 2.87296194087059
5 2.75639546403789
6 3.07033704291416
7 3.5171939948161
8 4.17657038858308
9 4.65077044493167
10 5.1635694702885
11 5.40697778392956
12 5.71228415196477
13 5.79217860563238
14 5.75584772447456
15 5.45505087973602
16 5.11170873235549
17 4.62044699689297
18 4.09845407313866
19 3.62532476249538
20 3.12222112421365
21 2.6177971994214
22 2.4395116874596
23 2.54339183748862
24 2.67043605306491
25 2.58919961734081
26 2.4878980105892
27 2.18923415339579
28 1.77434415729294
29 1.20841811432859
30 0.588398599292173
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07459176854488
1 3.36732221837021
2 3.41856380803778
3 3.18020725515107
4 2.77453121468531
5 2.69077945257795
6 2.9957687562969
7 3.52235945902292
8 4.38336020168158
9 5.08969603707339
10 5.62897559624987
11 5.95608036011343
12 6.16029417396458
13 6.29484626254369
14 6.4617413239768
15 6.47437092566136
16 6.35456102195616
17 6.10938201485168
18 5.93847514421975
19 5.88675126370577
20 5.68272563045671
21 5.5673568843511
22 5.43700081139083
23 5.34434780223444
24 5.26354695862983
25 5.21353276061894
26 5.2689911208148
27 5.23939668574659
28 5.17701147310974
29 5.22791583360441
30 5.08252047921396
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07444995163342
1 3.41567395513909
2 3.50469418944464
3 3.40418775388718
4 3.08155418314971
5 3.03903253087238
6 3.46724313799465
7 4.02287631080333
8 4.64711231987514
9 5.22048024934468
10 5.5888074015779
11 5.89749333924359
12 6.2035490139641
13 6.40312208999194
14 6.67963683312957
15 6.82890260711655
16 7.09801654369399
17 7.28963612595558
18 7.42684065121379
19 7.62178345235882
20 7.81689749363047
21 7.90403489509442
22 8.00125259236078
23 8.04902523178585
24 8.14768141893208
25 8.11495563142932
26 8.12062226985695
27 8.11963392885595
28 8.15823564292438
29 8.11410599582425
30 8.07672887074919
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07448725502131
1 3.43566849502264
2 3.62684363776203
3 3.60003235995525
4 3.3191338999341
5 3.27531386600893
6 3.51414464875415
7 3.78945521082738
8 4.15784085158106
9 4.50335909138912
10 4.80372313121859
11 5.13157096056659
12 5.30050692903058
13 5.32383791324115
14 5.25327713257822
15 4.99543624788097
16 4.80290441864447
17 4.32883385189739
18 3.90428541369079
19 3.532597851683
20 3.27395368918524
21 3.31086450166414
22 3.19936916148469
23 3.15179939801463
24 2.85003559337613
25 2.45266271663789
26 1.77965810265425
27 1.0308453970888
28 0.278572165820755
29 -0.283391637392876
30 -0.77158150684614
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07446830986616
1 3.33502625629069
2 3.31665615088119
3 3.17889862268316
4 2.76672025007526
5 2.60234227181402
6 2.83870779694058
7 3.11169618847677
8 3.51888199536353
9 4.10366095179218
10 4.52728983010575
11 4.98833294946538
12 5.27925246117785
13 5.44560656938085
14 5.45532629001046
15 5.33360786101217
16 5.02936233789593
17 4.58562842960961
18 4.04028328955196
19 3.4064689593616
20 2.70836222821867
21 1.99967460407084
22 1.49315671840602
23 1.28374776698813
24 1.22415760847792
25 1.41212911066033
26 1.78791660591891
27 2.47895151417763
28 3.1674372213706
29 3.88833166868869
30 4.52059521978644
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07465971517175
1 3.30770171936167
2 3.40009122902017
3 3.30413207855005
4 2.98161635624224
5 2.83534910123886
6 3.08859675361521
7 3.41889156658023
8 3.75079942535136
9 4.19621131542299
10 4.44548293376263
11 4.60363898122256
12 4.73823069839768
13 4.74823283814584
14 4.56661244332731
15 4.16489496161753
16 3.54337241929971
17 2.93826610152235
18 2.46898650313183
19 2.12884855063884
20 1.87420974384197
21 1.9195204230587
22 2.2544199150448
23 2.67093706081608
24 2.9421202076683
25 3.21431488686979
26 3.29326882604643
27 3.30746113014092
28 3.28210081446547
29 3.28507099018389
30 3.5277174778908
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07447372616273
1 3.33206132617012
2 3.3327091164494
3 3.17661183278021
4 2.76560869993428
5 2.73680876111603
6 3.11480578739474
7 3.89974570220305
8 4.8034992170148
9 5.10456724268951
10 5.30933762909277
11 5.42609300764205
12 5.43702286151257
13 5.2023920204307
14 4.89561720240674
15 4.59038026597946
16 4.38939701780211
17 4.30289447349406
18 4.10114139900082
19 3.73015831713173
20 3.20954061997938
21 2.49681275993241
22 1.64670374266655
23 0.739234209660035
24 -0.0945496799468071
25 -0.829727660642819
26 -1.46126784194865
27 -2.01716898925387
28 -2.32168492604084
29 -2.57174178140883
30 -2.81722589679153
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07392628875675
1 3.42397151005056
2 3.41735993076576
3 3.29991363798563
4 2.98309314241056
5 2.92216622227762
6 3.20038491044372
7 3.65649744661082
8 4.34254811180265
9 4.76105304745083
10 5.00815397091201
11 5.27235092565206
12 5.40928135858864
13 5.50055326508107
14 5.45997563640001
15 5.35689820143262
16 5.27517446101113
17 5.06895394120173
18 4.67405934932753
19 4.28245587770333
20 4.08316601018607
21 4.13819448186801
22 4.18261352414773
23 4.06518680244735
24 3.78174546979328
25 3.37569047891267
26 2.64171963029464
27 1.79792603773499
28 0.980224299940094
29 0.2352184716996
30 -0.444380157584236
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.0744304975052
1 3.39268270374047
2 3.53555940673948
3 3.3763824907892
4 3.01556208613258
5 2.86934638844586
6 3.14222284439641
7 3.56540438989371
8 4.11139152427415
9 4.55200408400253
10 4.79167364055787
11 5.07296200709115
12 5.24096824671753
13 5.2868480707296
14 5.2308645757782
15 5.10313571252306
16 4.78414965298239
17 4.31997506915497
18 3.82741871418373
19 3.16842225960521
20 2.63248717871325
21 2.17775820647638
22 1.87053650570202
23 1.76799168222561
24 1.74763816131439
25 1.94824263730112
26 2.13453792144603
27 2.37863942861759
28 2.6166380999527
29 2.98841529732937
30 3.34558448482096
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07443247824106
1 3.38920576183096
2 3.54003613405876
3 3.51344873219043
4 3.23789165206996
5 3.27226481840112
6 3.64255227115589
7 4.12958034065718
8 4.45928932873883
9 4.61667432320001
10 4.81307871610916
11 4.9110341202884
12 5.01434500242
13 4.9858725760957
14 4.78577485657573
15 4.45231827957106
16 3.93352850213645
17 3.2335600214396
18 2.39712101572926
19 1.80780344973545
20 1.35882481120225
21 1.2290320515229
22 1.49176489038534
23 2.0878148208639
24 2.78457713771786
25 3.3820293189791
26 3.71998093211759
27 3.93019650794579
28 4.10228529332584
29 4.10320988313678
30 3.82554792767127
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07447339359056
1 3.40824524502073
2 3.42104179656115
3 3.26826261356134
4 2.86220819102351
5 2.76353741589059
6 2.8647413019512
7 3.16058034827856
8 3.78463133664585
9 4.49809510123683
10 4.87199148716941
11 5.1606607393726
12 5.33522612818
13 5.41213394949793
14 5.30319499952759
15 5.02482805644223
16 4.46759497640819
17 3.86402189264271
18 3.28085689164743
19 2.7061283740496
20 2.10111033547807
21 1.51698388182207
22 1.00778570771577
23 0.667476522877751
24 0.775994460334562
25 1.2773889572861
26 1.96808825507532
27 2.56938991143059
28 3.16568443881034
29 3.48498276661906
30 3.60533598249176
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07454802684622
1 3.25500133585202
2 3.44217565004949
3 3.47966719442879
4 3.12458858090517
5 3.08937057826939
6 3.46690767386733
7 3.78788231296349
8 4.20337963975147
9 4.72831654058238
10 4.96375887820388
11 5.13589518910307
12 5.34687523761891
13 5.33628599115322
14 5.14930073754501
15 4.73307948481531
16 4.18298720595587
17 3.60052716962018
18 3.06475353979577
19 2.38538778582382
20 1.98351507929012
21 1.95337157457618
22 2.24813989110246
23 2.81375823212331
24 3.06190823657747
25 3.100417824033
26 2.97246004738073
27 2.82931309050288
28 2.67122387971713
29 2.3024384634401
30 1.77560852415293
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07492861408513
1 3.36700550868438
2 3.52106796907772
3 3.42105910472236
4 3.09773444761504
5 2.99971183726947
6 3.19264925763748
7 3.58713034111662
8 4.0777215036564
9 4.62050264431491
10 4.97157279886839
11 5.02675975263562
12 5.08005753675366
13 4.76197601708029
14 4.37469901578898
15 3.99398099730696
16 3.66747864715604
17 3.23581086609864
18 2.7913569396692
19 2.38003272768438
20 2.01743208023471
21 1.70863901823819
22 1.58306512268527
23 1.82971619527515
24 2.26683844332843
25 2.8470251434987
26 3.46058666193217
27 4.15829032216838
28 4.62752169301525
29 4.93639466004187
30 5.07510321810914
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07458906931394
1 3.35572502811929
2 3.47335273741787
3 3.38772649927341
4 3.07856033576502
5 3.00626255126521
6 3.27635644357571
7 3.5831612745363
8 4.08359665926988
9 4.53811096959691
10 4.79979453475646
11 5.09192303092655
12 5.31751470158328
13 5.41802196748558
14 5.49494609765135
15 5.48622960057829
16 5.39582090561732
17 5.28350680277353
18 5.01574298850199
19 4.67389302450104
20 4.3392184131086
21 4.24813695809859
22 4.18501173221278
23 3.98713983199609
24 3.75459284076214
25 3.31846784519703
26 2.71077418045945
27 1.90460542602025
28 1.10803625518294
29 0.296019676892239
30 -0.445850638228059
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07429720237256
1 3.33731736429407
2 3.42919361394143
3 3.30314951659677
4 2.94575429110322
5 2.90071427436878
6 3.32807031000174
7 3.79040227942811
8 4.36315382113428
9 4.68736276587668
10 4.90118789344464
11 5.02940152323406
12 5.10560716036018
13 5.12547314602783
14 5.02721597839977
15 4.73932707940311
16 4.32134095084285
17 3.96795679616042
18 3.77646659136737
19 3.80664463041579
20 3.84359051809088
21 3.75162363196251
22 3.54190173530878
23 3.06446966373085
24 2.49113856224552
25 1.82734468181108
26 1.06863675213537
27 0.233755605147648
28 -0.518057439814566
29 -1.24426358551572
30 -1.92638415989937
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07425735181823
1 3.31288928975507
2 3.39239272378046
3 3.46077945841232
4 3.31551634588355
5 3.43441741628987
6 3.88093118723522
7 4.53365021204032
8 5.01311431878401
9 5.21800673459907
10 5.43364405939554
11 5.45571471395637
12 5.36799367045796
13 5.16090905345616
14 4.85515072891728
15 4.68065109256066
16 4.22225568002848
17 3.55509317830103
18 2.90677415139386
19 2.15330464481214
20 1.32919498855367
21 0.630132381254935
22 0.0324925882434606
23 -0.507218445881005
24 -0.842243307387987
25 -1.08719696985601
26 -1.15946166862886
27 -1.32023005563584
28 -1.32516565489479
29 -1.28124918022562
30 -1.18819691607886
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07453410253838
1 3.31470346413145
2 3.44883422275251
3 3.38295245827682
4 3.17766264382793
5 3.16428184435911
6 3.36627283682343
7 3.62998476849583
8 3.99171064358397
9 4.40449994077055
10 4.63712011104658
11 4.82435273719303
12 5.00424920352111
13 5.08419591819774
14 5.07226788376293
15 4.88741983021897
16 4.56519731472115
17 4.20337784224044
18 3.74179676058206
19 3.5007183860045
20 3.64601405489432
21 3.63702140067639
22 3.4501148028375
23 3.15200141748562
24 2.72580784299113
25 1.97803537187957
26 1.34249281414973
27 0.589027979311973
28 -0.15614028839012
29 -0.822358312956252
30 -1.33882939390285
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07477845569546
1 3.37515039240992
2 3.43671787950476
3 3.31624524917318
4 2.96044567629676
5 2.87932840861617
6 3.18341665564392
7 3.68282109171331
8 4.26870309217819
9 4.70736275608187
10 4.96527594600893
11 5.18669419204862
12 5.44586978675783
13 5.76958292307006
14 5.94149434148349
15 6.04300304737744
16 6.05662141846489
17 5.91300308388848
18 5.61658651405384
19 5.18436463788612
20 4.73902299929807
21 4.19549629776614
22 3.58102292962027
23 2.88338247002685
24 2.16292770650667
25 1.66745651752075
26 1.39600550418282
27 1.52475997707
28 2.01246005736293
29 2.75585841318846
30 3.62445124643064
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07403219169243
1 3.42747001599379
2 3.5055260512784
3 3.30865971793696
4 2.91334258869701
5 2.91472559613582
6 3.3395259391063
7 4.00496332443632
8 4.79991048170652
9 5.2317375368236
10 5.70390665720051
11 6.10908861228323
12 6.30928071166161
13 6.50672177191823
14 6.6126757935528
15 6.64441179481599
16 6.54946912588872
17 6.45105020122209
18 6.36416234460757
19 6.20988342811481
20 6.16796891063631
21 6.13495345336752
22 6.09538575839303
23 6.16129114585185
24 6.21753129969574
25 6.2406920407283
26 6.27811534328777
27 6.2610714611881
28 6.36678995639777
29 6.46804497811658
30 6.51943856319897
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07449720892435
1 3.34858812473851
2 3.37428159493692
3 3.30509706998815
4 2.92349189844549
5 2.86503024120398
6 3.04758831448023
7 3.57924973794237
8 4.27764936728152
9 4.78769863466723
10 5.21611426340307
11 5.49931693080063
12 5.65008417966012
13 5.73970239188557
14 5.66101230688997
15 5.55067700094222
16 5.26159857078958
17 4.75196713120744
18 4.06984117023128
19 3.3880026818228
20 2.85321375511692
21 2.33829232317177
22 1.91871420141147
23 1.44109204545063
24 1.11006037930626
25 1.25816531516904
26 1.64132539592561
27 2.21842055731316
28 2.85273907885409
29 3.47143937463653
30 4.15013262956773
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07436984319872
1 3.36760552853686
2 3.52440128099097
3 3.49745708702079
4 3.16833216078422
5 3.04582689230517
6 3.22626744846824
7 3.53361354840352
8 4.01540104105018
9 4.39059679383598
10 4.72983993617442
11 4.97655248051475
12 5.25144907225445
13 5.40903830285513
14 5.31959319875418
15 4.99059450318618
16 4.5917387248413
17 3.99821859687221
18 3.41976513672716
19 2.81702968387501
20 2.40628816161464
21 2.19293710551143
22 2.14395552814998
23 2.14598209005935
24 2.20262437649901
25 2.38427228461639
26 2.52481938203613
27 2.69467777254829
28 2.9447991470346
29 3.09864843886016
30 3.25578887690045
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07420091947022
1 3.3896227713146
2 3.48972826840123
3 3.38473114086418
4 3.14619566815243
5 3.18094085961297
6 3.56478165254555
7 4.22401439495612
8 4.94449074188822
9 5.27058834520023
10 5.65545620635069
11 5.89177504802404
12 6.10925658823176
13 6.20045087491143
14 6.18988786529571
15 6.11848775481558
16 6.0986656803221
17 6.09660536015853
18 6.11858952867256
19 6.21210218701131
20 6.27376883982876
21 6.2545528110437
22 6.19799077427798
23 6.15311768779558
24 5.93515750919352
25 5.64397958026994
26 5.33236184812401
27 4.85593075813279
28 4.33354668379876
29 3.62336712162053
30 2.80761317277944
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07466951232855
1 3.30352296678253
2 3.36329148069194
3 3.24934881512094
4 2.82413309416114
5 2.72770437630277
6 3.01467375775532
7 3.5645722202273
8 4.42749535659347
9 5.02864746939105
10 5.46439964485683
11 5.78495927604134
12 6.02712340786222
13 6.11044921133439
14 6.17479519991339
15 6.14469499867015
16 6.14579917091047
17 6.05307968562844
18 6.01133759588565
19 6.0914591441661
20 6.10563553824883
21 6.21985704569938
22 6.32532799010066
23 6.39884202409245
24 6.51316133713177
25 6.69425323518147
26 6.85469254243106
27 7.03281143652145
28 7.25405393746581
29 7.38446489663508
30 7.50548221804982
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07482555221873
1 3.32415923879918
2 3.33201711724802
3 3.16420744909216
4 2.80845862390087
5 2.77496781952971
6 3.18182394230967
7 3.79002161537842
8 4.54135838960678
9 5.05784896527737
10 5.49315493774369
11 5.7861946040249
12 5.99326116626758
13 6.11053556226307
14 6.10369171226341
15 6.11861242674511
16 6.18021676294168
17 6.27501393547405
18 6.37580105648321
19 6.61034993705284
20 6.68067489944433
21 6.80629835832788
22 6.89000051738305
23 6.92396482401257
24 6.93934670093981
25 6.91168416221405
26 6.89098048994633
27 6.83044371057726
28 6.85226424014246
29 6.85355553115321
30 6.91168099301677
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07409993410763
1 3.34623066407553
2 3.44715262566938
3 3.293126785673
4 2.92733958777978
5 2.81283940114382
6 3.10869238517219
7 3.41506514398095
8 3.89625545487489
9 4.36137668337214
10 4.74421113984713
11 4.99353521465188
12 5.07348691554835
13 5.09909795888208
14 5.04331135755571
15 4.91414932475209
16 4.73873895335989
17 4.56385277272763
18 4.3236600035152
19 3.98007954889221
20 3.52098478259534
21 2.93518560407712
22 2.24523985834767
23 1.46786541580878
24 0.599005010788462
25 -0.304175656055451
26 -1.07828189816907
27 -1.78766854128663
28 -2.31203072049456
29 -2.86425767761743
30 -3.34099060345143
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.0742969122237
1 3.28851114909115
2 3.38939337153271
3 3.3530008647752
4 3.04827415482139
5 2.90924069544209
6 3.04288971729051
7 3.31045774705836
8 3.73683137035146
9 4.21426282994022
10 4.55120025854358
11 4.94105810113657
12 5.10577367232113
13 5.07277570357934
14 4.94270340616629
15 4.6784179627219
16 4.10742185533463
17 3.5567397718545
18 3.0445788168385
19 2.58223956791634
20 2.17739072860386
21 1.90057293700463
22 1.66965963710601
23 1.56830682030873
24 1.77524950299327
25 2.08859221437573
26 2.65722907236875
27 3.25094532856167
28 3.8278236576931
29 4.33394709162599
30 4.77833928416369
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07495496324139
1 3.43891262931791
2 3.58642466395719
3 3.54162880875891
4 3.18346741138542
5 2.99683938389182
6 3.13542045161858
7 3.55192519386816
8 4.1334173910599
9 4.57087669062651
10 4.96679096924629
11 5.30577893844995
12 5.63545102820606
13 5.75981892473867
14 5.80201671334632
15 5.76807181410681
16 5.69332085226715
17 5.67747026454312
18 5.71560398677484
19 5.76453486020912
20 5.63578520868472
21 5.34615215295165
22 4.8859508364878
23 4.53864527148858
24 3.96384985328408
25 3.24143104085274
26 2.44417277481093
27 1.54239187952289
28 0.658471817494657
29 -0.129561767454739
30 -0.831115475529737
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.07481021661487
1 3.32936124580229
2 3.3155900269382
3 3.12525184818878
4 2.78575216558774
5 2.75311385518541
6 3.02693300623931
7 3.48910971800885
8 4.06775763821488
9 4.60439515729352
10 5.02649730653832
11 5.26115058806891
12 5.46002553547905
13 5.72441098111785
14 5.76541581876651
15 5.70837448692291
16 5.36257791051361
17 4.89739943730431
18 4.43872169950222
19 3.85301483005068
20 3.26910440893269
21 2.61773446651863
22 2.10116693515142
23 1.74357728527897
24 1.71014726405951
25 1.87368818788343
26 2.22089174586412
27 2.56042015881794
28 2.90919429258869
29 3.28113761314323
30 3.48374493366364
};
\addplot [line width=0.01pt, color0, mark=*, mark size=2, mark options={solid, draw=black}]
table {%
1 3.31996634253658
2 3.45443899460193
3 3.38784218387077
4 3.01931286439371
5 2.82906626173755
6 3.09427938765557
7 3.60416870184349
8 4.24596487007442
9 4.84338888587772
10 5.27994908427636
11 5.61004074039071
12 5.90268352537916
13 6.05852129333431
14 6.16858387553312
15 6.19509636026208
16 6.21485180933973
17 6.20378189365436
18 6.1468591562609
19 6.14787992255152
20 6.14579317317396
21 6.15283082950704
22 6.15412613868876
23 6.14366281427887
24 6.16587792193215
25 6.18223254289368
26 6.18638821201769
27 6.14794417270148
28 6.14179954980725
29 6.15812095860932
30 6.16746194810668
};
\end{groupplot}

\begin{groupplot}[group style={group size=1 by 3}]
\nextgroupplot[
xshift=-8,
ylabel={\textcolor{color1}{outer angle}},
ylabel style={font=\large},
xmin=-1.45, xmax=30.45,
%ymin=-9.72718755361779, ymax=3.33959760594388,
ymin=-0.85, ymax=5.85,
width=\figurewidth,
height=\figureheight,
xtick={},
xticklabels={},
axis y line=right,
tick align=outside,
xtick pos=left,
ytick pos=right,
x grid style={white!69.019607843137251!black},
y grid style={white!69.019607843137251!black}
]
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.48334285848053
1 2.90944389175027
2 2.29939633205269
3 1.53389603352793
4 0.680782393439429
5 0.186545955982867
6 0.242680962855699
7 0.571383143286502
8 1.04505067834569
9 1.52162499956425
10 1.58103338293563
11 1.66643789546777
12 1.66624668257114
13 2.02495308019187
14 2.17360020972302
15 2.23895072046117
16 2.22635367058472
17 2.03229776119944
18 2.03234757537478
19 2.08771189400888
20 2.00283138761746
21 1.91736225591453
22 1.77365785783345
23 1.45872504008842
24 1.07836072993102
25 0.77407605974126
26 0.505400466785034
27 0.23151324550584
28 -0.131272685434384
29 -0.633561023223308
30 -1.29310600942124
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.48529456944789
1 2.68702422463723
2 1.73621377980908
3 0.623995254404457
4 -0.418744198971949
5 -1.04393491767625
6 -0.963709928357396
7 -0.680900826150727
8 -0.196181134036575
9 0.193902863216672
10 0.211746278060547
11 0.187973166591646
12 0.222473698210765
13 0.118640752387815
14 0.0748165674383283
15 -0.0603382017595422
16 -0.463337994078412
17 -1.03857869140706
18 -1.87869084382071
19 -3.20716902459746
20 -5.0209750812536
21 -6.95486258865395
22 -8.84564378369414
23 -10.5129287842855
24 -12.1731677814377
25 -14.015192249151
26 -15.3664382479556
27 -16.6344525231225
28 -17.8275844521447
29 -18.6387551941656
30 -19.2156787490779
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.52889078753411
1 2.62836027557055
2 1.73024960057138
3 0.744903307370752
4 -0.224123011394103
5 -0.854346491167853
6 -1.15301249251946
7 -1.18026834585741
8 -1.14681083695501
9 -0.681822717252957
10 -0.426922548771575
11 -0.159701843846995
12 0.169784652023664
13 0.425103398718363
14 0.676917216803659
15 0.80844506057941
16 0.734804018757548
17 0.577620035664322
18 0.143549382075033
19 -0.48558109348669
20 -1.69324514451423
21 -2.94429178635252
22 -4.72280984253002
23 -6.51670840502947
24 -8.28575748699403
25 -10.1996539601389
26 -12.1645376527258
27 -14.0549569106579
28 -15.747971097576
29 -17.366408296182
30 -18.7405161355458
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.484249090094
1 2.74552025189927
2 2.00896170768854
3 1.12894129007528
4 0.236023487054973
5 -0.240071700157138
6 -0.0125289447843795
7 0.454205014431485
8 1.02786684134241
9 1.51424548007564
10 1.58625070500789
11 1.64700332718069
12 1.68269360035259
13 1.83063956371996
14 2.00361834707399
15 2.09039588080172
16 2.09276781888849
17 2.01448985115706
18 1.82545260997068
19 1.61829512798709
20 1.45891505066746
21 1.42328298473632
22 1.59937544733169
23 1.7757449351661
24 2.05402919383603
25 2.23207766508286
26 2.44935216107939
27 2.56688528755024
28 2.58372102354085
29 2.65853050727989
30 2.81404504264297
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.50137895673017
1 2.63137241516037
2 1.77416126423389
3 0.841563129045592
4 -0.079313672521474
5 -0.714621159440327
6 -0.76531251994476
7 -0.556055028796317
8 -0.240764114179902
9 0.0786466859012136
10 0.162384576789818
11 0.333234930440726
12 0.297673945827754
13 0.277829619547615
14 0.13896611786302
15 -0.156041315471856
16 -0.604174143670798
17 -1.32136095776301
18 -2.19175266473378
19 -3.70024842575842
20 -5.73610800643833
21 -7.45118077993401
22 -9.17222756043543
23 -10.992558053684
24 -12.7904149903149
25 -14.5597097573964
26 -16.1407534101245
27 -17.3451842054836
28 -18.2451339636279
29 -18.7625066650925
30 -19.1356196146214
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.51893968752228
1 2.63307658496052
2 1.73912067118508
3 0.692177191580898
4 -0.421526393691857
5 -1.09386648088968
6 -1.05218799623647
7 -0.809721069636835
8 -0.308844474685649
9 0.179472046943562
10 0.444886556936089
11 0.626082674988905
12 0.906988093148563
13 1.2548124176525
14 1.56715366339464
15 1.57813918725068
16 1.34645703082067
17 1.04187805782277
18 0.667968775792815
19 0.247275445003419
20 -0.0379419801450109
21 -0.156206096175258
22 -0.38440753113784
23 -0.665581520581071
24 -1.17817485034233
25 -1.98286847818683
26 -3.04356010557291
27 -4.09211063047977
28 -5.25117481270936
29 -6.56608228990424
30 -7.91213133561517
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.50528341993881
1 2.57179337913129
2 1.73049159436745
3 0.789922476966123
4 -0.176113200674454
5 -0.727296835703343
6 -0.952172655639794
7 -0.895486962347172
8 -0.446425327141509
9 -0.249174460378919
10 -0.110368983046151
11 -0.0538937357954496
12 0.315312482797363
13 0.538113383221143
14 0.992667437846063
15 1.46507613196211
16 1.79753860125882
17 2.11296450479658
18 2.32751623542875
19 2.48680799582068
20 2.55428794685764
21 2.72840999337892
22 2.87527065029023
23 2.75718141270054
24 2.36793921957404
25 1.89121800125878
26 1.45683774076865
27 0.970142422577322
28 0.483335091262286
29 0.102088019652451
30 -0.33606049137981
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.48819613445912
1 2.75915891124006
2 1.80330028918601
3 0.915590594830125
4 -0.146579706315803
5 -0.664136460181354
6 -0.630165741459547
7 -0.365130179395783
8 -0.00128690538696219
9 0.381927079750412
10 0.402612680133763
11 0.410426512670716
12 0.200112208054985
13 0.239328929950127
14 0.135026270130497
15 -0.137427167799143
16 -0.574917852416368
17 -1.46868049610455
18 -2.77858816200902
19 -4.39906810291685
20 -6.1775355334626
21 -7.84200842278014
22 -9.78913295435603
23 -11.741480100604
24 -13.6600531889503
25 -15.3443975014343
26 -16.7151086671511
27 -17.8358555365602
28 -18.8399561400893
29 -19.5412459528786
30 -20.2261612371566
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.46825285426485
1 2.7000021151317
2 1.84160700220778
3 1.07274166771081
4 0.208576898716205
5 -0.209000242500343
6 0.312545539774716
7 1.00386304874673
8 1.92583775053467
9 2.57352852130465
10 2.94196649208249
11 3.26842240602582
12 3.72429580947345
13 4.29410550944024
14 4.73748810056017
15 4.98527235012557
16 5.09095670933091
17 4.96936793896466
18 4.42079391470192
19 3.78306492720783
20 3.53602097354205
21 3.02606812573833
22 2.46171048091531
23 1.94731072751888
24 1.47868531496596
25 0.841724737687284
26 0.165440947786122
27 -0.499932725526157
28 -1.04858151096255
29 -1.9541701925992
30 -3.01288081871449
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.4703667381564
1 2.68017869462059
2 1.84489576545631
3 0.685595857032408
4 -0.424498209747461
5 -0.96140264646941
6 -1.15073773239772
7 -1.11382779715599
8 -0.901461283869092
9 -0.693952458559403
10 -0.598440132896989
11 -0.700377239750245
12 -0.752300920170553
13 -0.832896825671996
14 -0.923577325712676
15 -1.26188835227024
16 -1.7125390095962
17 -2.37257184384876
18 -3.45316020241942
19 -5.0350549090477
20 -6.89313197585747
21 -8.66691174913206
22 -10.5552304148447
23 -12.2723022105978
24 -13.9266552384916
25 -15.4536153174888
26 -16.8521926404262
27 -17.9625755649016
28 -18.8249317903694
29 -19.3474250188865
30 -19.6871058556916
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.46871213859979
1 2.75167955771052
2 1.97648762422618
3 1.20258685200084
4 0.451554003839024
5 -0.0446875207821757
6 0.0519143932219479
7 0.555701900174834
8 1.26808043616713
9 1.85287875810739
10 2.37890486921698
11 2.71880789768353
12 3.12237239341986
13 3.66576526011138
14 4.41408482134373
15 4.8770931109611
16 5.10443032559014
17 5.25568191959546
18 5.19080387808435
19 4.53674061290648
20 3.71431796621551
21 3.16435151416135
22 2.39214011438815
23 1.80350804940079
24 1.28847878484445
25 0.972226868078381
26 0.627461742229319
27 0.238784484951014
28 -0.231057205411012
29 -0.804770165623024
30 -1.74817373467639
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.4807716704713
1 2.62454278914952
2 1.83987756260222
3 1.03579344333313
4 0.338501487064789
5 -0.0957625102557651
6 0.221824717345829
7 0.814041397374833
8 1.69616110769127
9 2.54067312408241
10 3.09169172152601
11 3.48307886566027
12 3.86491752887677
13 4.28498563511137
14 4.6976114097437
15 5.07085958255081
16 5.11428512524105
17 4.93953282281702
18 4.61314335505939
19 4.2957397012701
20 3.82786280539348
21 3.31549518309691
22 2.76980599738345
23 2.09609285708043
24 1.42640783638188
25 0.811363031938857
26 0.33222864255331
27 -0.203464993315023
28 -0.698436854712377
29 -1.32006354305133
30 -2.30118824422931
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.49726101162845
1 2.71957271521408
2 1.76382491206046
3 0.784613219368423
4 -0.185535264560154
5 -0.590013071437034
6 -0.412085888650143
7 0.0777743962367197
8 0.640017137836114
9 1.21952231741111
10 1.47408460986345
11 1.58015676451267
12 1.81673300651479
13 2.24803798278496
14 2.66222781177017
15 2.87651481201074
16 3.10682465973872
17 3.3534539063645
18 3.5608741263728
19 3.68800438514115
20 3.62249611209543
21 3.44691324741359
22 3.05991120221456
23 2.60125021340729
24 2.41484290584604
25 1.78894075447603
26 1.17570552572723
27 0.63098800872707
28 0.243956837910239
29 -0.175406795801882
30 -0.703836371583802
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.4847478853502
1 2.64896339154966
2 1.83087302119413
3 0.931192094258865
4 0.128893717326409
5 -0.335862496396915
6 -0.114507400549488
7 0.230307379212987
8 0.828193967436581
9 1.17208755783191
10 1.42167704401712
11 1.55182872414494
12 1.84070095828154
13 2.17524214752805
14 2.57607044106862
15 2.85120489500542
16 2.83028636075646
17 2.91626581567518
18 2.80168316411568
19 2.65472763813798
20 2.66160664090772
21 2.39940897234275
22 2.24977081580432
23 2.05710565127111
24 1.84731786875094
25 1.43139547487492
26 1.23203945893044
27 1.18951072399153
28 1.18983692448426
29 0.820261093920894
30 0.314912754267736
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.54752172016153
1 2.57332324601612
2 1.59193251558502
3 0.732412864122037
4 -0.291082807314992
5 -0.796709675809739
6 -0.606961524852872
7 -0.253971530705658
8 0.053843941439879
9 0.38114506175503
10 0.161749501313808
11 -0.142817766520377
12 -0.490103373278025
13 -1.00258579862832
14 -1.63402629132855
15 -2.3111736152706
16 -3.08286932500135
17 -4.16625276729348
18 -5.50113101855449
19 -7.08629633246562
20 -8.95179379630879
21 -10.849910025791
22 -12.9846382476777
23 -14.8745377607607
24 -16.3299885093214
25 -17.9040316061929
26 -19.1818098979674
27 -20.1779841150409
28 -21.0166220738572
29 -21.6224670351097
30 -21.8156997966642
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.4907867198985
1 2.66973979419233
2 1.92327094449391
3 1.06749033222273
4 0.302654027446718
5 -0.0423823175958062
6 0.312076644325623
7 0.98228960406024
8 1.69310157436064
9 2.21526069749174
10 2.49031493611184
11 2.5698515544347
12 2.75888253693205
13 3.2234795721016
14 3.60049033443196
15 3.87209929255249
16 3.9132024644138
17 3.70165229827734
18 3.50808797014124
19 2.86390092653213
20 2.18036545364415
21 1.26080418669158
22 0.436492908311194
23 -0.286086529413892
24 -1.04406641614982
25 -1.58358625668193
26 -2.16876320301751
27 -2.9278336650523
28 -4.06985411094509
29 -5.3688189452547
30 -7.01836814103168
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.49931121428154
1 2.81614237611319
2 1.9076869907268
3 1.0990096448779
4 0.196922888628949
5 -0.117422898416444
6 0.0896336537281743
7 0.739841819122282
8 1.29347347435163
9 1.64633881113983
10 1.83207927275715
11 1.92087226609083
12 2.06846882742232
13 2.44938831654743
14 2.61031250407802
15 2.69656415075796
16 2.6159647263561
17 2.60690749908794
18 2.70706747378495
19 2.75056069091248
20 2.73215706265288
21 2.88431430663102
22 2.71541891025612
23 2.54834271870679
24 2.29457049069762
25 1.73326995191653
26 1.2243950268411
27 0.90138708101021
28 0.566436981490508
29 0.327469777076165
30 -0.00358567862068537
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.45082776148169
1 2.77151455986681
2 1.95449354062475
3 1.24003404080269
4 0.483749250604625
5 0.0112903897678496
6 0.618164671952693
7 1.51886289814751
8 2.62839191974652
9 3.82921563000418
10 4.53563750912862
11 4.91332465697905
12 5.33835095235627
13 5.62091184900928
14 5.52826263489459
15 5.23734232904058
16 4.76623492700572
17 4.53734310826153
18 3.95642875144018
19 3.08548301720153
20 2.61103021745008
21 2.30615676243999
22 1.61325800169278
23 1.16029934416843
24 0.948905876451119
25 0.671751723368579
26 0.393933273785269
27 0.169376880031804
28 -0.210226911505114
29 -0.587268912764082
30 -1.2295286998019
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.45350644936503
1 2.88811414615297
2 1.96436473000663
3 1.2455309188436
4 0.245948687364984
5 -0.213200560920543
6 -0.0860807961163044
7 0.378017252133763
8 1.06888918833713
9 1.65410183577702
10 1.93919985188532
11 1.96538736074631
12 2.29310649819508
13 2.70099062842603
14 3.06099959112389
15 3.37296296323037
16 3.60291817278364
17 3.63261526422308
18 3.49340459687557
19 3.21448789476516
20 2.86062000460364
21 2.55166269623847
22 2.0455537500801
23 1.60335661387341
24 1.15590775915886
25 0.767327867759242
26 0.333981776125862
27 0.00304211193193438
28 -0.37770486585693
29 -1.08978950037825
30 -1.88222961477739
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.48774187752923
1 2.84347356313602
2 2.00283194044587
3 1.1662200137617
4 0.255776458130489
5 -0.269409283526243
6 -0.202441430077279
7 0.164014044500332
8 0.917983801706959
9 1.7198223321904
10 2.35684737954021
11 2.86107796125538
12 3.31192690950598
13 3.75915396949817
14 4.2130567005975
15 4.45231346255393
16 4.56405953432057
17 4.46044781529507
18 4.26625259334346
19 3.940901969615
20 3.34683514699266
21 2.80926440291917
22 2.20527292143203
23 1.67200361446853
24 1.23057318726711
25 0.826201192724833
26 0.56588314387767
27 0.396295408392957
28 0.2819706526439
29 0.165805071022657
30 -0.127439203124885
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.51340400076415
1 2.57622563496233
2 1.60644294434434
3 0.677428928600638
4 -0.311058739764755
5 -1.14862764514465
6 -1.44913138744947
7 -1.63188000651535
8 -1.54963772517354
9 -1.27575471912842
10 -1.43390902900442
11 -1.80629877849187
12 -2.19252331294214
13 -2.39232835302657
14 -2.56405120223839
15 -2.76357330401454
16 -3.30393941021156
17 -4.42890793675626
18 -6.1582633904712
19 -8.06773296952048
20 -9.97807611335991
21 -11.941508636193
22 -14.0806854714421
23 -15.9059168913153
24 -17.5036850040367
25 -18.7599338374672
26 -19.9554536903949
27 -20.6893878920243
28 -20.8185295379697
29 -20.7929636673499
30 -20.5273801789986
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.50260839026096
1 2.68181621129634
2 1.82513588465471
3 0.895168856464113
4 -0.0796345032977877
5 -0.76384314100506
6 -0.755110214418111
7 -0.491710588268024
8 -0.230624403719695
9 5.32273563054186e-05
10 -0.0746835139132653
11 -0.243328656525206
12 -0.43389077435821
13 -0.721490818159817
14 -1.17144257598052
15 -1.84864635113999
16 -2.72135399532008
17 -3.95373768641609
18 -5.27268327196274
19 -6.7379893502747
20 -8.26236131278083
21 -10.0710819499501
22 -12.0532328633496
23 -13.9507974893126
24 -15.7590000523601
25 -17.4294097844347
26 -19.0593011632566
27 -20.2536452710269
28 -21.0933536115357
29 -21.9000824752829
30 -22.5229564401428
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.49998992663268
1 2.82976203480671
2 1.86784040299687
3 0.873176290710198
4 -0.262963440076531
5 -1.07936208093817
6 -1.69072415287512
7 -2.20269815919682
8 -2.05998831019628
9 -1.78030750096833
10 -1.87356898813449
11 -1.93064538151782
12 -2.04455698386295
13 -1.83347094117045
14 -1.47037813572054
15 -1.22314863623338
16 -1.1412034265883
17 -0.971723208362088
18 -0.930830191809715
19 -0.922119457424089
20 -0.70266229131335
21 -0.504434949630334
22 -0.237734861022748
23 0.0474893252148074
24 0.213765102868697
25 0.466905328287534
26 0.674545781802617
27 0.630357276954913
28 0.397288021605117
29 0.544858038215062
30 0.73524607491672
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.47320916239165
1 2.73155793607409
2 1.80475807186093
3 0.880981811330854
4 -0.079953223494432
5 -0.846007581780916
6 -0.863680603634178
7 -0.590180201782945
8 -0.161229963544848
9 0.0925252144125475
10 0.324115201579395
11 0.607150198961641
12 0.910804142474977
13 1.3508205190606
14 1.78401077142313
15 2.13767163112677
16 2.43088033868345
17 2.43723270565948
18 2.28072533030061
19 2.05204313067466
20 1.55607988623853
21 1.09244185188098
22 0.609696644803218
23 0.142093897425349
24 -0.190925231698927
25 -0.419649899048704
26 -0.671765147268748
27 -0.97375017546985
28 -1.17043143676755
29 -1.46703705529954
30 -2.0913613040129
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.54484093590129
1 2.71558088008665
2 1.69449792132209
3 0.579935381779951
4 -0.743807988644366
5 -1.76422425833838
6 -2.73337600399357
7 -3.28792955987403
8 -3.41215700111833
9 -3.218775001012
10 -3.46564221289249
11 -3.59263969519783
12 -3.6057441764443
13 -3.66248320134851
14 -3.96485693565695
15 -4.75044227189627
16 -6.28078542607681
17 -8.47731666415592
18 -10.5897780999142
19 -12.7816541737157
20 -14.8368341556963
21 -16.7668664864072
22 -18.5470098050892
23 -19.9862060700496
24 -21.1487110798838
25 -21.8811970774437
26 -22.1561924308016
27 -22.1893537837904
28 -21.8960993153121
29 -21.3129810657982
30 -20.7753469153108
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.47097424587015
1 2.70855510614291
2 1.90151948495531
3 1.27124026118501
4 0.49003857745558
5 0.167936439145265
6 0.306237390986178
7 0.729912033960143
8 1.40095260042917
9 2.0966184519716
10 2.44961237976318
11 2.81966464157889
12 3.18975216420995
13 3.56022614882374
14 3.79604426701723
15 3.78226014178179
16 3.63278098838541
17 3.30497491362195
18 3.02855298507472
19 2.57465297942006
20 2.19684748255703
21 1.92027167519318
22 1.5036968758263
23 0.987264919755016
24 0.619992471172055
25 0.117456034945851
26 -0.520524091101815
27 -1.07898094578485
28 -1.88440107814159
29 -3.29777932760398
30 -4.81553975427614
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.50238983785959
1 2.7034762060607
2 1.75906623287659
3 0.724538638040137
4 -0.522279870967854
5 -1.42546373503242
6 -2.11144147316075
7 -2.55160068575035
8 -2.65603713454224
9 -2.40817170963983
10 -2.30905172443808
11 -2.15419007226816
12 -2.1182037704474
13 -2.14386525088004
14 -2.08058504632992
15 -2.0191626520058
16 -2.12850829266911
17 -2.54252846123619
18 -3.25851099195709
19 -4.51067101382906
20 -6.04466747440686
21 -7.60155445734758
22 -9.40050389988219
23 -11.2567343913619
24 -13.2380718545521
25 -15.2512660067834
26 -16.9355495933061
27 -18.3947650640587
28 -19.5516574768242
29 -20.6562902897148
30 -21.4441052598753
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.50114747702359
1 2.70990408318629
2 1.93863008911456
3 1.07329967011796
4 0.165845355655162
5 -0.358867144048255
6 -0.0646599906695087
7 0.571799960488822
8 1.2599896479225
9 2.01013218128869
10 2.44830382091081
11 2.88455688434192
12 3.29467984805699
13 3.53860398585546
14 3.85037722228343
15 4.09065557083638
16 4.24677840051221
17 4.22246399308406
18 4.01478915587417
19 3.62963276627059
20 3.20203065382185
21 2.77888190807006
22 2.33340465145831
23 1.84566869922738
24 1.20796190773789
25 0.469659880265188
26 0.0268728588765297
27 -0.251126739630168
28 -0.566612096604343
29 -1.00805011763304
30 -1.81268221808463
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.43107835824164
1 2.71559675159377
2 1.80433088734085
3 0.812918140821111
4 -0.0460386382088398
5 -0.515560136508422
6 -0.528177169508996
7 -0.191331212866586
8 0.190878783207626
9 0.475990984518593
10 0.292148733245917
11 0.158175224170862
12 -0.298161664005753
13 -0.62152987015445
14 -0.963726769055087
15 -1.24316656813113
16 -1.64683504734103
17 -2.30702238734842
18 -3.21584520672004
19 -4.61654202784557
20 -6.27529005816202
21 -8.05751004934544
22 -9.9605270245786
23 -11.8281409671182
24 -13.7274417986822
25 -15.6218425734118
26 -17.081056430856
27 -18.1428562166195
28 -18.8734694619613
29 -19.3875822948708
30 -19.5466082703391
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.48011822788259
1 2.65734692855711
2 1.97187146394758
3 1.10889957409835
4 0.00662411388899997
5 -0.570447844109413
6 -0.412297202744279
7 -0.0553744409631034
8 0.230074107492273
9 0.376188693397237
10 0.21423191590736
11 0.0979227826115294
12 -0.00684296756540581
13 0.00253913807500084
14 -0.212186347440802
15 -0.359263658311515
16 -0.825034586459274
17 -1.73640350542666
18 -2.81170315421519
19 -4.30880772292752
20 -6.06609553357803
21 -7.76559797917085
22 -9.62848686168721
23 -11.7765834266616
24 -13.990193878089
25 -16.2544398174672
26 -18.1669135690679
27 -19.5317602182025
28 -20.4956405733725
29 -21.3218498498872
30 -21.7758317066039
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.52186647393886
1 2.60274164708945
2 1.65935807279166
3 0.69157918823403
4 -0.333496514130209
5 -0.928676800203316
6 -1.00098715963843
7 -0.583763150088424
8 0.0181663770171454
9 0.362155477099027
10 0.664412842966629
11 0.756726058937256
12 1.08349584552489
13 1.53362475385073
14 2.12125085196109
15 2.6550026853162
16 2.98432574932409
17 2.94669945348625
18 2.50809325249606
19 1.98478226243966
20 1.35925842958168
21 0.810533734494331
22 0.27907820724777
23 -0.170093461309479
24 -0.488822030684468
25 -0.601844489717202
26 -0.821059562197975
27 -1.15701861030869
28 -1.54078296361572
29 -2.10726995764143
30 -2.93887934138437
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.47668290302015
1 2.6108507293186
2 1.64050303562556
3 0.696537772987788
4 -0.340199411111829
5 -1.00190989886533
6 -1.37515328799545
7 -1.57864145495946
8 -1.37883752830391
9 -1.41667865411016
10 -1.85468192899691
11 -2.33508586448454
12 -2.99097402358962
13 -3.87203477283776
14 -5.08554650347724
15 -6.659954594986
16 -8.7525436881336
17 -10.7553156491252
18 -12.8289346083615
19 -14.7268713936349
20 -16.7371612538121
21 -18.4595357099923
22 -19.9113668509665
23 -21.275375752251
24 -22.3111606892725
25 -23.0373250061942
26 -23.4511755763485
27 -23.6960180543979
28 -23.9303442151245
29 -24.085814252157
30 -24.2347776398983
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.46541259725728
1 2.65834787895682
2 1.73998918771074
3 0.957098600260789
4 0.0833996432156161
5 -0.535931685566231
6 -0.327020583608001
7 -0.0751249727040484
8 0.432971556017156
9 0.854984014681606
10 1.01229701390983
11 0.954522950491598
12 1.00020297065467
13 1.04004801891072
14 0.96414621790412
15 0.844824243673542
16 0.731634775720167
17 0.668232295323406
18 0.323903324001745
19 -0.301068438670926
20 -1.23462874854908
21 -2.55974206844875
22 -4.11114030028083
23 -5.71666452259127
24 -7.32836972552667
25 -9.17002026371166
26 -10.9285075419447
27 -12.4025970497898
28 -13.7357041850398
29 -14.8265649571357
30 -15.897700121297
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.50278007006192
1 2.59571609524477
2 1.67403194462354
3 0.647281500337388
4 -0.354548920984854
5 -0.899980789838058
6 -1.00699457112739
7 -0.936355186995329
8 -0.637568353602397
9 -0.383818323663923
10 -0.212786950775155
11 -0.0594483551969702
12 0.112770694342354
13 0.156687519414281
14 0.0820609748418362
15 -0.0300310019775223
16 -0.316996851771123
17 -1.06160614065712
18 -2.01001322436091
19 -3.23415155613321
20 -4.93420971011737
21 -6.62438922704797
22 -8.60341747085392
23 -10.4702193041189
24 -12.4595210025208
25 -14.3557682070264
26 -16.2449860501642
27 -17.6549053532839
28 -18.7171135249919
29 -19.4211195442353
30 -19.797758775947
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.51233578035908
1 2.69152524558698
2 1.8128555851992
3 0.846530011733334
4 -0.120423880372282
5 -0.89140921503968
6 -1.03658940923368
7 -0.955999075747818
8 -0.685517120271553
9 -0.520961111781141
10 -0.829243742151407
11 -1.19485727801962
12 -1.39383633720745
13 -1.61009579664416
14 -1.75809469120879
15 -1.9477717033946
16 -2.51869219347607
17 -3.41736855070398
18 -4.71803248890693
19 -6.20273806733664
20 -7.85921620612521
21 -9.63929352407397
22 -11.4330510228573
23 -13.0291537930435
24 -14.6668670793681
25 -16.3801292559419
26 -17.9085328602391
27 -19.0820364149121
28 -19.9239833923601
29 -20.3879027997845
30 -20.771247896425
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.46483398440732
1 2.83420629108085
2 1.92910292002227
3 0.975711533295488
4 -0.0496512885616791
5 -0.697615349412005
6 -0.591003216667729
7 -0.439207879915822
8 -0.260781384291553
9 0.0136211008055114
10 -0.0887116917720754
11 -0.130927531764294
12 -0.0926035854312564
13 0.0137205676847019
14 0.0910322863794939
15 0.197916894798744
16 0.28442203692049
17 0.396705094637616
18 0.61006407323301
19 0.655746476764781
20 0.660654176786912
21 0.661386387333988
22 0.703077177739646
23 0.747746593694208
24 0.926408085090624
25 0.958076173088681
26 0.986304565368303
27 1.08588397706013
28 1.2630177626756
29 1.30256081754939
30 1.33970137646702
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.5204938058607
1 2.73368862284648
2 1.76910177393651
3 0.84826652080683
4 -0.1770121392617
5 -0.839464760808811
6 -0.994930411516552
7 -0.823892766596174
8 -0.506793623330203
9 0.0797487796329026
10 0.408337377194906
11 0.67341349597366
12 1.04729198482523
13 1.34156418397607
14 1.48095156575666
15 1.60726289805974
16 1.65084671624109
17 1.56128350351635
18 1.60583084379271
19 1.62155615890896
20 1.72537720518245
21 1.98077235004157
22 2.16836877067784
23 2.34770569528012
24 2.56132877320576
25 2.83721189197145
26 2.98233664424746
27 2.97413817451899
28 3.00445969910689
29 3.06850327741239
30 3.21708427133712
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.46691420989852
1 2.67346230397271
2 1.685115260944
3 0.737212082227736
4 -0.258813356515965
5 -0.876390387448704
6 -0.98015229972339
7 -0.7158252708623
8 -0.125568609921558
9 0.147152634871702
10 0.24943040993051
11 0.142093571451779
12 -0.0434344907550357
13 -0.00778486827741109
14 -0.0302138059168082
15 -0.0540212956274038
16 -0.265717251327898
17 -0.490163420330729
18 -1.0296078757757
19 -1.61960503803166
20 -2.43783480605234
21 -3.41092122402479
22 -4.68211624700722
23 -6.23624006433424
24 -7.89557860868096
25 -9.5169393514995
26 -11.3242274468496
27 -13.212119880564
28 -14.9472193960593
29 -16.7236677276511
30 -18.26768728178
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.44722561378566
1 2.84842132044257
2 2.07385578603104
3 1.11315835296006
4 0.227761610985333
5 -0.215523744088387
6 0.0633155870470314
7 0.488965414433675
8 1.17668400060173
9 1.62675022000161
10 1.93851168905276
11 1.99511736199431
12 2.02000169940805
13 2.21198068602583
14 2.34929231066497
15 2.33632768780943
16 2.23588129896491
17 2.1723870914564
18 2.07420532638903
19 2.00552536139296
20 1.98888941088972
21 2.0706643362188
22 1.76003064606347
23 1.35904318559356
24 0.939219135139805
25 0.64139246578727
26 0.186163990010019
27 -0.253635697929627
28 -0.73170890564781
29 -1.51920698314348
30 -2.75309793125192
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.49373166917883
1 2.71750800614626
2 2.00157878852671
3 1.20915573623727
4 0.306710302757392
5 -0.123142881568614
6 0.15070877793113
7 0.823255969587722
8 1.57012920038716
9 2.54412509510421
10 3.3496782757452
11 3.94007575181338
12 4.80524872953311
13 5.628474979285
14 6.06787709376624
15 6.10807157142338
16 5.92295690348771
17 5.51568518200198
18 5.04889089144648
19 4.50961130559159
20 3.71710281984892
21 3.12234049430292
22 2.52625856046354
23 1.77956266674408
24 1.04004569566876
25 0.343213223033746
26 -0.156616932217282
27 -0.667745013241181
28 -1.23603779735747
29 -2.17687313251024
30 -3.26368092227637
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.49059214839782
1 2.68237887079104
2 1.68749819753651
3 0.96320549515932
4 -0.153334455930521
5 -0.825029427480158
6 -0.91476420270608
7 -0.742706314062949
8 -0.370689850570351
9 0.0158081742287568
10 0.141806535633226
11 0.255394740447337
12 0.412059016662627
13 0.601167404674396
14 0.670148715891707
15 0.445521562202977
16 0.0282518289526787
17 -0.71213746620363
18 -1.69577926940123
19 -3.06078282384517
20 -4.80750725010157
21 -6.69437732343035
22 -8.61880104900578
23 -10.574340679287
24 -12.5534113683727
25 -14.367743869693
26 -16.1110479674219
27 -17.7243515110496
28 -19.159916405825
29 -20.2157286048958
30 -20.8716499601977
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.49457822622192
1 2.84018919820442
2 2.07814068428851
3 1.14967200659701
4 0.371364972181219
5 0.0327837250748315
6 0.281926710774054
7 0.889747937929725
8 1.75133730073992
9 2.59018214317499
10 3.19942295359872
11 3.47768142355673
12 4.11948573986941
13 4.64510909579906
14 5.0698876492197
15 5.29789491286679
16 5.36357961284882
17 5.39990576835299
18 5.1265213516425
19 4.58645381092781
20 4.07298726612843
21 3.42436188704508
22 2.74963528482978
23 2.2893869477802
24 1.70132989581771
25 0.894717128561113
26 0.0645073606380442
27 -0.638962595574254
28 -1.29855431494855
29 -1.8533778255018
30 -2.71071895992084
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.50189238701916
1 2.4175809027385
2 1.38639710407249
3 0.367631930542458
4 -0.783955951956121
5 -1.57051626748749
6 -2.01938189264785
7 -2.34401538796649
8 -2.20509637681266
9 -1.94597859747157
10 -1.69287705325498
11 -1.39379022625907
12 -1.14045173887298
13 -0.471575280699914
14 -0.0985400347273317
15 0.12914541914511
16 0.311534715550396
17 0.551298507947174
18 0.662955272148134
19 0.725186149292756
20 1.02111707258561
21 1.4899266035693
22 1.96244040612191
23 2.43957069966589
24 2.65368139784903
25 2.8765847442279
26 3.08195191032051
27 3.18988840275291
28 3.16174286682383
29 3.15287332765285
30 3.23179313839638
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.48619571480438
1 2.74377532740777
2 1.84475475380564
3 0.747780511663999
4 -0.484738771146058
5 -1.1488044093555
6 -1.25286982258791
7 -1.12436791893281
8 -0.84938670507356
9 -0.372982612360877
10 -0.180140460958302
11 0.0255231490737404
12 0.183076593660735
13 0.448654894067258
14 0.555679021042304
15 0.568019829158079
16 0.439836766338253
17 0.293203073387581
18 -0.128122981865519
19 -0.524607585865401
20 -0.991752245528563
21 -1.5884978470459
22 -2.52061208685226
23 -3.66961531752933
24 -5.09376126022025
25 -7.02315467271412
26 -8.91071922694181
27 -10.5367567336887
28 -12.1636822472145
29 -13.7393379763462
30 -15.194559353528
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.52542825632338
1 2.62586165795092
2 1.87242280458873
3 0.945481294452808
4 0.135095368875034
5 -0.414681066771761
6 -0.35846375272454
7 0.122674521452083
8 0.738100340343794
9 1.12235702505427
10 1.35313373549755
11 1.46777127990147
12 1.43379145177468
13 1.48517198963771
14 1.4792724477355
15 1.47529067814742
16 1.39932004701414
17 1.19811340160528
18 1.11063353471649
19 1.05541389204682
20 0.823514199396885
21 0.646329438491427
22 0.614510978967542
23 0.481837447694162
24 0.479314188339021
25 0.46343771150471
26 0.456727510818987
27 0.395687554612626
28 0.365122915499857
29 0.470387347712136
30 0.457561214806112
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.51242752279148
1 2.83149536896737
2 1.9507908934459
3 1.05910574918877
4 0.220402607372565
5 -0.243057734809875
6 0.0592227708798143
7 0.619564158630959
8 1.3601469645664
9 2.29533136044335
10 3.03156557223775
11 3.50250629531213
12 4.29047485995009
13 4.74622198215894
14 5.07943486550147
15 4.916842210647
16 4.50011756900332
17 3.85438318999271
18 3.42440947991953
19 2.89136981410895
20 2.5980694400845
21 2.47406060798462
22 2.34437015804851
23 2.21637745715988
24 2.0645744913625
25 1.94099430807398
26 1.72072923951087
27 1.52712448855174
28 1.61585192039182
29 1.76032076561129
30 1.86884677148365
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.49177578422361
1 2.80004352578547
2 2.1218528341201
3 1.50823870392101
4 0.756057207813403
5 0.377682765769105
6 0.623376191635792
7 1.45160866434574
8 2.42217869269257
9 3.29231660230458
10 3.71954906466838
11 3.98029300927225
12 4.20353106174347
13 4.68467952142814
14 5.19122177176466
15 5.62560607680028
16 5.89726113794635
17 6.08243830791954
18 5.92906710281001
19 5.41626316459484
20 4.70613551237278
21 4.1090583271861
22 3.4891571685098
23 3.00741282383747
24 2.55256964179982
25 1.97802043597149
26 1.61875739207715
27 1.35997557424177
28 1.23699031214971
29 1.25405269714137
30 1.24606266598808
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.49190525158992
1 2.74568131010104
2 1.82404427383258
3 0.80411131728853
4 -0.215501028370968
5 -0.799612682120291
6 -0.760424810699911
7 -0.537716008707693
8 0.0121251074360307
9 0.239278061339089
10 0.166355927622082
11 0.0152080891083219
12 -0.337158046112248
13 -0.495699251697565
14 -0.715688781055087
15 -1.13980666424031
16 -1.7244094015778
17 -2.51731340263981
18 -3.39038782085003
19 -4.63301958684128
20 -6.01954526447065
21 -7.54454401685507
22 -9.23970412885339
23 -11.0357383063506
24 -12.7831032131561
25 -14.708431861282
26 -16.6639594912742
27 -18.1672074192501
28 -19.3095400988979
29 -19.8957206450998
30 -20.1925368817487
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.49273756241961
1 2.6838405511848
2 1.77872540416175
3 0.870164040744171
4 -0.347379570076074
5 -1.03468166692367
6 -1.26916520599937
7 -1.68647198190978
8 -1.77382425357813
9 -1.67757593241524
10 -1.80458311543103
11 -1.60591347900694
12 -1.49277306521739
13 -1.11734249872625
14 -0.777920861669858
15 -0.565694859654236
16 -0.56383405329889
17 -0.575551699202509
18 -0.622542693977044
19 -0.737918313709461
20 -0.705811699498409
21 -0.707881168152216
22 -0.845456317593276
23 -0.9465059986501
24 -1.03555978446685
25 -1.17164479327443
26 -1.23201014249354
27 -1.24806882940621
28 -1.2942166246888
29 -1.40848483546903
30 -1.54198672988473
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.46459767294732
1 2.70367012510185
2 1.74666326459849
3 0.911131849498814
4 -0.047338877490676
5 -0.753080224834958
6 -0.973350200595211
7 -1.12440716717083
8 -1.13146903489193
9 -0.886596374334187
10 -0.964403602131855
11 -1.045267688607
12 -1.02149504002538
13 -1.18954194777274
14 -1.29724458298887
15 -1.48029104895651
16 -1.88720298026133
17 -2.5913184502702
18 -3.67625892426485
19 -5.02308694030995
20 -6.64218406884888
21 -8.39646894965739
22 -10.458631606201
23 -12.5618850461512
24 -14.5864252922814
25 -16.5601405423619
26 -18.3439264034211
27 -19.7177994926194
28 -20.6562677305953
29 -21.3827539111506
30 -21.7639111609617
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.50068719269398
1 2.56538877299193
2 1.64585868098564
3 0.835794387296116
4 -0.22893435011516
5 -1.00118849006887
6 -1.25938445186953
7 -1.19763505606815
8 -0.980906472955256
9 -0.749455228426312
10 -0.811716739140353
11 -0.912559686959141
12 -1.20496438845213
13 -1.30854188415224
14 -1.26498633328341
15 -1.45282774977602
16 -1.6558063589236
17 -2.14426546868501
18 -2.8223654986314
19 -4.05797406197896
20 -5.71531858832637
21 -7.6457360519603
22 -9.63229742806955
23 -11.5511352738728
24 -13.2601546407023
25 -15.1068975318721
26 -16.9547926113174
27 -18.3406698182438
28 -19.4499261197722
29 -20.4068886587898
30 -21.029847342841
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.52292638017596
1 2.71272198320536
2 1.70505768271842
3 0.875254308377121
4 -0.23630755092011
5 -0.959692593067096
6 -1.23244822061399
7 -1.18152707351906
8 -0.706376380451477
9 -0.56398671041444
10 -0.76276255597081
11 -1.0290213578947
12 -1.39121290770395
13 -1.83197398924576
14 -2.32448013886695
15 -3.05403511715816
16 -4.15358875231647
17 -5.61960518783552
18 -7.1088402746843
19 -8.84669387486436
20 -10.5246214133128
21 -12.6002693375371
22 -14.6546811411297
23 -16.4242066497557
24 -18.0642145127386
25 -19.6207178808547
26 -20.7107904247576
27 -21.5734811607566
28 -22.2490457497867
29 -22.7512341717985
30 -22.9276394165085
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.49406344722077
1 2.69792102541723
2 1.66203017354812
3 0.444812909454554
4 -0.654515432938489
5 -1.77912904108749
6 -2.50789905887427
7 -3.04807870318736
8 -2.98775377826083
9 -3.07545443891471
10 -3.39542642223428
11 -3.7919386555022
12 -4.27985568446777
13 -4.72822498607858
14 -5.43943937760893
15 -6.60886048274296
16 -8.03231872422147
17 -9.98462965813899
18 -11.9597902273385
19 -13.8458397647455
20 -15.5427492445685
21 -17.1181810160338
22 -18.6336623007074
23 -19.8735154928147
24 -20.9517651012863
25 -21.7415925669657
26 -22.3106959258246
27 -22.6960201644297
28 -22.7670636965139
29 -22.5140807889708
30 -21.9316177558739
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.51426084100411
1 2.61133861450303
2 1.69908830648898
3 0.826480200648942
4 -0.0343998567693968
5 -0.621786459200136
6 -0.498218493702215
7 -0.180110363552737
8 0.364805377449172
9 0.692013901191469
10 0.943458451776331
11 0.959457441030721
12 0.938579089290795
13 1.07942833293946
14 1.25165642186407
15 1.558639624995
16 1.7283904678226
17 1.70111781648091
18 1.70489946239966
19 1.62865726738379
20 1.35759586809143
21 0.974520599326638
22 0.501045135350562
23 -0.292108981955195
24 -1.30965925975326
25 -2.74394626840349
26 -4.5347483724796
27 -6.48597364016255
28 -8.27395565160942
29 -10.1754682999132
30 -12.110187686908
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.51263205006388
1 2.7592607262848
2 1.90558029371393
3 1.1143151942217
4 0.0774575497682473
5 -0.569090528306696
6 -0.612003599125171
7 -0.342479089269405
8 0.0200044980864413
9 0.435548663201796
10 0.315842512754152
11 0.111153204237322
12 -0.139759058894263
13 -0.332183283981752
14 -0.440264760567382
15 -0.731714742300212
16 -1.05356864959001
17 -1.33341101253898
18 -1.64212670244282
19 -2.07876755953946
20 -2.7130937048978
21 -3.62942845657625
22 -4.8732810385279
23 -6.57509070578724
24 -8.42188363376963
25 -10.3744895970929
26 -12.3209424651356
27 -14.0007385053274
28 -15.5681655954646
29 -17.0873150794364
30 -18.564821632739
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.49332717168653
1 2.71928215757822
2 1.96251330185309
3 1.1673460525911
4 0.342102333550022
5 -0.294910046892645
6 -0.283225958634212
7 -0.0528376003707587
8 0.335748556046924
9 0.668502208518842
10 0.738077365642562
11 0.780426609148859
12 0.891571113853075
13 1.27595761992225
14 1.67206839172423
15 2.0461143381878
16 2.31764448503292
17 2.27064994260709
18 2.06816029481894
19 1.82573497058719
20 1.41630765481503
21 1.01070879441992
22 0.606483968756911
23 0.204443707615757
24 -0.0346901949593927
25 -0.283986628131535
26 -0.448363477392164
27 -0.452253187639776
28 -0.464808782670719
29 -0.307733219766769
30 -0.221944938390469
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.52585320175772
1 2.64287682741283
2 1.73132979288916
3 0.819270893859775
4 -0.0786876472766589
5 -0.553458762058244
6 -0.324081838058129
7 -0.0602209365838098
8 0.452524657190453
9 0.90517723799412
10 1.17003720040854
11 1.41666190744246
12 1.73013787528861
13 2.19971758031716
14 2.89148349387936
15 3.27761545526252
16 3.45866255662616
17 3.54974007857028
18 3.67628112960608
19 3.68425866317304
20 3.73996900734505
21 3.75389253652552
22 3.73354009138553
23 3.59016437158945
24 3.33032852714266
25 3.08696112048023
26 2.93007330839891
27 2.81535146186624
28 2.46890755827834
29 2.01652447399011
30 1.52995621066317
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.4444656344699
1 2.79494550031326
2 1.97234001824864
3 1.09275182957379
4 0.0822784153557983
5 -0.534675696249584
6 -0.314468627076314
7 0.123058952429414
8 0.671647074382837
9 1.30434176346469
10 1.79692650988943
11 2.1805099970902
12 2.58940316173619
13 3.2008757347906
14 3.5779267650228
15 4.03554905828644
16 4.35199551537417
17 4.54777520620558
18 4.44398909985577
19 4.01814513580189
20 3.19942114828418
21 2.71181497197312
22 1.97565724492492
23 1.39876407984978
24 0.846203280165665
25 0.399672028411025
26 -0.0782523583861074
27 -0.655029531916512
28 -1.25502807789165
29 -2.12993677158456
30 -3.38590712785857
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.48112486911012
1 2.75904238680265
2 1.80250704279506
3 0.937915632111688
4 0.0487484113828027
5 -0.459700451024093
6 -0.304952515172964
7 0.252911232761743
8 0.925426168546646
9 1.30237768484088
10 1.48668287359103
11 1.3619493081451
12 1.12047622446686
13 1.22204707252814
14 1.38255800913004
15 1.45065692370382
16 1.39077276725127
17 1.18998352699209
18 0.894115570744826
19 0.44193799208892
20 -0.537360461016672
21 -1.66757037541696
22 -3.26896886663558
23 -5.25002081817887
24 -7.13593789262451
25 -9.29218951040396
26 -11.3091833715583
27 -13.0108689698941
28 -14.5388135360062
29 -16.04064558103
30 -17.3463028593583
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.50265754364965
1 2.5937786312685
2 1.6700643611869
3 0.907263865325785
4 -0.17342271755123
5 -0.672438961768382
6 -0.675533952353629
7 -0.315234877976113
8 0.112887251937204
9 0.377815629488416
10 0.448436334566956
11 0.375378634151306
12 0.146677577989745
13 0.063349646257953
14 -0.0870789579642635
15 -0.300053297114894
16 -0.786868221777181
17 -1.66778546994729
18 -2.81611386233214
19 -4.3713992202075
20 -6.12970478678297
21 -7.8786017977343
22 -9.69481131917597
23 -11.5801907497381
24 -13.4996251217688
25 -15.3640345213251
26 -16.919742391318
27 -18.2944424169902
28 -19.3058460783912
29 -20.2668199432466
30 -20.6737800426069
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.48257533593527
1 2.86724748612702
2 2.02740779470611
3 1.09086816225122
4 0.19235982640235
5 -0.496463124187302
6 -0.316182251758097
7 0.201830622497126
8 0.513730818843634
9 0.888752627658332
10 1.0501176484474
11 1.16872762671804
12 1.16558136199097
13 1.37345728236832
14 1.80129851887943
15 2.19049735156624
16 2.4860750548317
17 2.54941668065938
18 2.57857695235647
19 2.33141653116276
20 2.02394989108361
21 1.70530716751604
22 1.29328478937916
23 0.884147920960469
24 0.405084289543433
25 0.0241137174713677
26 -0.241474827808515
27 -0.255335770697231
28 -0.420059456008284
29 -0.807574991913453
30 -1.40345374147562
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.50496504533617
1 2.75953229332363
2 1.80475335845468
3 0.867215012572626
4 -0.0172441527401861
5 -0.587666581061152
6 -0.637066956322699
7 -0.454756196362132
8 0.0109978704404918
9 0.300422140092109
10 0.214559883022963
11 0.170572428802008
12 0.423000522744022
13 1.03815211307301
14 1.55641347437678
15 2.08851373542431
16 2.44323825229468
17 2.71321922935067
18 3.1031687349906
19 3.36369040967521
20 3.69328446976015
21 3.87645039963068
22 4.07056206553479
23 4.17730074785958
24 4.00012234511203
25 3.64336002844112
26 3.24931015376273
27 2.75274787156678
28 2.19095742902186
29 1.53917882201141
30 1.18665337397163
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.46072729406249
1 2.68655279925997
2 1.8535310695829
3 0.987965125225591
4 0.0325129901773671
5 -0.518847999060241
6 -0.343508191742577
7 -0.0825959839534356
8 0.430374064127319
9 0.8801847344416
10 1.02405026444781
11 1.02002060044902
12 0.975162466818573
13 1.07023154186633
14 1.20797557286672
15 1.29864975822987
16 1.24339930886092
17 1.16163740258152
18 1.050651171409
19 0.69476859526999
20 0.0601426341354194
21 -0.77671823953144
22 -1.87669767944539
23 -3.78224681363668
24 -5.72733287647518
25 -7.69615408781225
26 -9.79429092963737
27 -11.9805049837431
28 -13.8047068632745
29 -15.6817225552468
30 -17.2466267486675
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.48844093948175
1 2.63698336535492
2 1.68504059679592
3 0.671758213455814
4 -0.268676675106038
5 -1.07458375594939
6 -1.54026723353145
7 -1.63736372609134
8 -1.25734996366459
9 -0.77338470323767
10 -0.363982805709731
11 0.0064071757457338
12 0.297261243423777
13 0.632842533038911
14 0.89213836433763
15 0.912603728433623
16 0.640961664027759
17 0.223066100411958
18 -0.124098633416564
19 -0.55194349030239
20 -1.15491249180555
21 -1.74457106884849
22 -2.27426094020521
23 -3.02513492427521
24 -4.03664873001199
25 -5.37314297342086
26 -6.96920870315643
27 -8.65384132158611
28 -10.347217744574
29 -12.2215858952851
30 -14.1665721441721
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.47726382198592
1 2.55826685257611
2 1.55212545863355
3 0.527375472942159
4 -0.771589618507695
5 -1.89430569120849
6 -2.86205018400478
7 -3.57577909845646
8 -3.85808325728285
9 -3.97749747928343
10 -4.5283342102349
11 -5.31519699616535
12 -6.54342776700502
13 -8.21732736493576
14 -10.0723286545405
15 -12.1378095347965
16 -14.3730630142274
17 -16.2491309403117
18 -17.9014327235244
19 -19.361864783457
20 -20.6223841298921
21 -21.5359061720766
22 -22.2405833816128
23 -22.5495749220072
24 -22.5696053085557
25 -22.4877720688096
26 -22.2400643727085
27 -21.8957165530678
28 -21.5282563236092
29 -21.0380601415472
30 -20.4606830955452
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.48682502862962
1 2.74278708446226
2 1.94031136884041
3 1.13776596312884
4 0.234304151279721
5 -0.369484689526868
6 -0.165231768745113
7 0.348448330256211
8 0.997392318499985
9 1.77443953772275
10 2.17663631149036
11 2.52503729677491
12 2.7656118652891
13 3.06871702131877
14 3.28695000036047
15 3.3381991262958
16 3.40471907413482
17 3.30028931430514
18 2.98312466923354
19 2.6485923874777
20 2.37265487383266
21 2.05239321897354
22 1.72828912651237
23 1.40666430395077
24 1.06013883494495
25 0.485125199510577
26 -0.185460735551583
27 -0.736331807388229
28 -1.37544870550624
29 -2.24029418346234
30 -3.73938908932509
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.44680464930548
1 2.64134766809581
2 1.77396676934655
3 0.844460808091831
4 -0.0650322679093751
5 -0.679070047731277
6 -0.694778037914806
7 -0.367480384842197
8 0.163243789532175
9 0.528481609957628
10 0.886142812192
11 1.4022364154743
12 1.90729575005777
13 2.33258147109873
14 2.59063730759788
15 2.63482914495408
16 2.66045270738449
17 2.51086772822761
18 2.4228796517714
19 2.41164767010555
20 2.32853645259663
21 2.33185135250486
22 2.36260019092462
23 2.35472097348259
24 2.35511752525822
25 2.45533137756234
26 2.5527192468597
27 2.73764494782881
28 2.92712255470733
29 3.23083812710436
30 3.38163596505534
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.52032846511856
1 2.72401572280799
2 1.87882409455563
3 0.945428122917143
4 0.0511573540957828
5 -0.347826842629247
6 -0.0360145113111769
7 0.6993588190828
8 1.39996749468238
9 1.99849010414211
10 2.29337159128353
11 2.59830486760909
12 2.83208062243874
13 3.15456685098293
14 3.37525301016846
15 3.55376602473814
16 3.64693475468392
17 3.68380797591892
18 3.63849791249603
19 3.36114075608564
20 3.20317385744159
21 2.96864056289278
22 2.69745442757454
23 2.26834528291498
24 1.47423644468338
25 0.944910503377997
26 0.487996000426012
27 0.186842292286147
28 -0.0865651437690942
29 -0.519625431788564
30 -1.18794109444897
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.47425083317802
1 2.77621605672203
2 1.95352872732957
3 1.12091618173491
4 0.300616547646187
5 -0.228478471072697
6 0.0428193524386262
7 0.637858958561756
8 1.46348160018295
9 2.26744794532799
10 2.57616289375595
11 2.78276225093441
12 3.16671439618035
13 3.7923228148653
14 4.12436092780307
15 4.28386803625238
16 4.13342457198343
17 3.98736612752749
18 3.89729730751324
19 3.59272000056143
20 3.06079506164762
21 2.57349283615117
22 2.01998428496231
23 1.41815840795041
24 0.937842795742216
25 0.694352335539217
26 0.567479765658522
27 0.329672095070039
28 -0.0289801675766355
29 -0.744017488740452
30 -1.60959085006457
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.4692710727833
1 2.73501694090378
2 1.8254545140814
3 0.935965932174709
4 0.0121347223543569
5 -0.661519384976355
6 -0.475893566278944
7 -0.0771318370991891
8 0.499325274743331
9 0.652921967155873
10 0.605276370514415
11 0.567421377498075
12 0.51744253169518
13 0.620907709125698
14 0.676454943473404
15 0.738067595861644
16 0.772942053911596
17 0.669182045388534
18 0.663081315730073
19 0.608945127945429
20 0.350006760822229
21 0.220103324843001
22 0.140615757878616
23 -0.00965624811557531
24 -0.200194729667431
25 -0.160475161556609
26 -0.140074968099188
27 -0.203905732948845
28 -0.338177703644352
29 -0.577183096981774
30 -0.966316884434441
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.51028455041431
1 2.6631364670351
2 1.75481750066333
3 0.903620828470877
4 -0.236360544547146
5 -0.786361310716929
6 -0.867071581945301
7 -0.865182699385048
8 -0.563422092753275
9 -0.256595927874751
10 -0.146607386451128
11 -0.203217568911738
12 -0.154509278628699
13 -0.0938271487497895
14 -0.0962501142945724
15 -0.249550449340397
16 -0.582627348374866
17 -1.30717009545434
18 -2.1863064604828
19 -3.40754010152705
20 -4.98601237852016
21 -6.55889008404348
22 -8.30423719745112
23 -10.2254352031826
24 -11.9292627231693
25 -13.6388607604432
26 -15.2837331090681
27 -16.8060963655305
28 -17.9527644615627
29 -18.6522239719562
30 -19.2538480379388
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.46923960883825
1 2.81428136525594
2 1.8880326198058
3 1.01059898249878
4 0.12877727882596
5 -0.342960425042397
6 -0.0595092706897473
7 0.365780862846984
8 1.13184451610218
9 1.99617058707489
10 2.782307850788
11 3.49349876292557
12 3.94189523803804
13 4.52845888041649
14 5.02944070398022
15 5.02852941588344
16 4.70779635674767
17 4.24519092211542
18 3.75949288170911
19 3.0010589172808
20 2.36755366266163
21 1.69393973651559
22 1.06796326233749
23 0.518392045030084
24 0.0862870790032979
25 -0.417170654546617
26 -1.05982340860117
27 -2.04202112915841
28 -3.3859618720441
29 -4.96833033546897
30 -6.63085666956595
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.51583751133081
1 2.70044717244252
2 1.88293590155546
3 1.08960653864103
4 0.0907201445243748
5 -0.34200415752205
6 -0.0930977319188602
7 0.148454588069713
8 0.565388502599315
9 0.831551869039012
10 1.00382491340488
11 0.932673925568304
12 1.02572638404903
13 1.35817517713446
14 1.53368001960517
15 1.37762480761492
16 1.21306015433095
17 0.979917354172753
18 0.375860220394194
19 -0.202774881362392
20 -0.928311840167245
21 -1.88235484859311
22 -3.05896969690943
23 -4.74129479531416
24 -6.23968924613549
25 -7.70369368083273
26 -9.25414537622153
27 -10.9952352791195
28 -12.729341623955
29 -14.5152150664946
30 -16.0844260471088
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.48285072267799
1 2.54821747859068
2 1.63738294089737
3 0.704225665546061
4 -0.342022138566251
5 -0.963051270939426
6 -0.90432733276957
7 -0.888285292610498
8 -0.6700143696809
9 -0.620935501547593
10 -0.636794531947993
11 -0.364844049681978
12 0.247011547210293
13 0.856368330699553
14 1.54433360786259
15 1.94117689630236
16 2.18480754188437
17 2.19752100192346
18 2.07533870605697
19 1.78403749930869
20 1.35754488752675
21 1.07023195761113
22 0.740543784449225
23 0.307769444947911
24 -0.254012925242524
25 -0.912643251063563
26 -1.56376730525824
27 -2.37756425681888
28 -3.26181148324083
29 -4.52773851716944
30 -6.03830221983193
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.49178672817567
1 2.70608934468081
2 1.70301560454297
3 0.702207075808646
4 -0.387898957434853
5 -1.0256541153308
6 -1.37459452728514
7 -1.52639846739787
8 -1.31673118784792
9 -1.02867904949835
10 -0.760031250394511
11 -0.654474539520408
12 -0.360058480633505
13 0.133596499910327
14 0.688489910538094
15 1.244794091762
16 1.77064899902619
17 2.13065072602346
18 2.41913857445481
19 2.46531066893043
20 2.56355098529563
21 2.55220506154278
22 2.36527495196631
23 2.06113641267321
24 1.82793014754113
25 1.59939415313971
26 1.24917955149765
27 0.854398610305283
28 0.469446266375823
29 0.0300680116541376
30 -0.523518036107047
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.48943620963901
1 2.64209769929695
2 1.83563120517934
3 1.02665239549416
4 0.178617062057158
5 -0.396137955988904
6 -0.298966283017733
7 0.0218782257100498
8 0.609154397047675
9 1.18541443319529
10 1.45160410792642
11 1.63014584093308
12 1.65418218404703
13 1.77323499982359
14 1.66491599332218
15 1.3978187185013
16 1.01722869590527
17 0.202539069876472
18 -0.460758989672089
19 -1.25814581151641
20 -2.36227696980452
21 -4.04009835935824
22 -5.79628544521215
23 -7.50189267946344
24 -9.39106190476866
25 -11.2657250657822
26 -12.893597763871
27 -14.4805094802329
28 -15.8454907579088
29 -17.0594297231358
30 -18.1655601107638
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.49062996015019
1 2.71954940392716
2 1.94734506643626
3 1.13143609850084
4 0.390499925301135
5 -0.0951985464117098
6 0.0606656640943588
7 0.696766621510131
8 1.44583897578777
9 2.11072168678706
10 2.35093937383694
11 2.42776130135139
12 2.53750224638324
13 2.79771845040839
14 2.97793540286027
15 3.04684557340852
16 2.94757905992037
17 2.82596666623493
18 2.90601376617518
19 3.14445047163931
20 3.19152180997732
21 3.12796222454616
22 2.5758591363424
23 1.89496389842945
24 1.23771668712001
25 0.523806446374619
26 -0.147687239413644
27 -0.556900088317145
28 -0.952912746747188
29 -1.76488587785491
30 -2.7870853367139
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.47856934731152
1 2.6929958620728
2 1.90143092542244
3 1.0411725200303
4 0.0883462220938134
5 -0.361247142936034
6 -0.0805506329979213
7 0.385286993578741
8 0.890859599797205
9 1.55890310694824
10 1.92734581421758
11 2.05687657586243
12 1.9104891516325
13 2.21564766901749
14 2.26231139895579
15 2.40428267089404
16 2.54233556204087
17 2.68833519451806
18 2.81234699302256
19 2.56293244196768
20 2.20839390647554
21 1.60961310961298
22 0.866075616539982
23 0.342956733627513
24 0.23184407551191
25 -0.133788429946072
26 -0.441694715475081
27 -0.799691442808557
28 -1.49817760010064
29 -2.34850764868026
30 -3.51699531715312
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.49028867464765
1 2.72242869451448
2 1.80403985478482
3 0.72531731664997
4 -0.614416862496423
5 -1.40032556722965
6 -1.68362108364412
7 -1.87214544493167
8 -1.63890956176064
9 -1.55706513703417
10 -1.44070690558802
11 -1.55632399340055
12 -1.678180383628
13 -1.83513201532839
14 -2.25779124655687
15 -3.09766308360502
16 -4.55214324196578
17 -6.39171363678076
18 -8.28656681831731
19 -10.2037689060334
20 -12.0446356553297
21 -13.8132349036187
22 -15.7777904092792
23 -17.5142802541026
24 -18.8156342512668
25 -19.7465166933666
26 -20.3489866941948
27 -20.5526354676362
28 -20.4209424056573
29 -20.1711997463277
30 -19.8584291168027
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.52478317617998
1 2.59616446976847
2 1.6781808791158
3 0.793864903874733
4 -0.234230569273731
5 -0.945046649056292
6 -0.909700481085315
7 -0.765777180610955
8 -0.330193259443725
9 0.00135902182925784
10 0.170431951876269
11 0.217276844766341
12 0.0352142289981388
13 0.159442560087014
14 0.264079250861425
15 0.256951410496955
16 0.130277643464473
17 -0.150973576058317
18 -0.762827700291448
19 -1.64699990162149
20 -2.94627226704465
21 -4.99925252033929
22 -6.6613103933621
23 -8.42597221552596
24 -10.2279169456474
25 -12.2828277583109
26 -14.1804558514149
27 -15.955031435392
28 -17.4622890912737
29 -18.6302700013591
30 -19.3220240794747
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.49301254951792
1 2.7763530036616
2 1.90062500244647
3 1.08037559768591
4 0.11861890919055
5 -0.426085676705217
6 -0.120513571296964
7 0.314870882979235
8 0.956253994773118
9 1.55976520585635
10 1.82977045525313
11 2.18038229296517
12 2.5796799709973
13 3.18113227815747
14 3.57747774294365
15 3.93221122604232
16 4.00101050333835
17 3.91281962767276
18 3.74988731059229
19 3.48811752560136
20 2.94372260022124
21 2.61851086561846
22 2.24283183011822
23 1.80394417606898
24 1.53358245667619
25 1.17740239363335
26 0.693205353467155
27 0.309416864726708
28 0.00763944918056136
29 -0.306692642899852
30 -0.662267587209009
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.49288774164908
1 2.6857998268069
2 1.80350231374129
3 0.87193159619224
4 -0.135698295003934
5 -0.764310651410449
6 -0.874660374279761
7 -0.647808581301673
8 -0.16435929897303
9 0.342691764004972
10 0.682971401942709
11 0.883827712335709
12 1.03934572766116
13 1.19644360376353
14 1.35037477540827
15 1.37753436555355
16 1.38767781425211
17 1.09324794227387
18 0.773752059834717
19 0.183252450726488
20 -0.254065830329243
21 -0.662786135044137
22 -0.979388474625433
23 -1.54922699702303
24 -2.31703658158333
25 -3.36694126705716
26 -4.57221606014572
27 -5.67015686055553
28 -7.14729348236606
29 -8.77801319056015
30 -10.5316002524002
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.49030963030559
1 2.80408601611641
2 1.90357180394203
3 1.12015611714715
4 0.317393745952126
5 -0.108041425727905
6 0.337846693334508
7 0.790970921501072
8 1.42121966100371
9 1.9152291879318
10 1.91246561793033
11 1.87835024747193
12 1.96760520746323
13 2.18667112589967
14 2.47141443779962
15 2.48666322737042
16 2.4071181284525
17 2.02808088070928
18 1.60457001560887
19 1.03114376116694
20 0.410635417457076
21 -0.243274256556369
22 -0.877837531793446
23 -1.42092802784414
24 -1.83063371059868
25 -2.39584912516756
26 -2.9137621186663
27 -3.66027691350564
28 -4.52951655022175
29 -5.58244486426806
30 -7.1071292976819
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.48560692471117
1 2.553848056319
2 1.70221443229588
3 0.905810576643991
4 -0.0764352038740659
5 -0.659916935024578
6 -0.623438354509753
7 -0.240802436542022
8 0.370830389278191
9 0.97395695671663
10 1.2638137396553
11 1.6684304066995
12 1.81754976068895
13 1.8924570219093
14 1.82208541504311
15 1.48113100810864
16 0.943184069227225
17 0.355476402575756
18 -0.256634734267509
19 -1.09781358875844
20 -1.87337054013852
21 -2.45263241002153
22 -3.13030322002115
23 -4.42324031772543
24 -5.79135498279087
25 -7.40409100478289
26 -9.01776344891272
27 -10.6754445164662
28 -12.2829969381296
29 -13.8618708131085
30 -15.7520968532775
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.46162579563109
1 2.80581602198825
2 1.96747359611156
3 1.16228569037097
4 0.348051379766966
5 -0.178055582623037
6 0.0480709016964012
7 0.597998686758868
8 1.40358377395015
9 2.35202873429684
10 3.11257527320222
11 3.70482010613368
12 4.37772680977693
13 4.98126539779161
14 5.17761156097873
15 5.05134710185386
16 4.72268960838518
17 4.36247789980451
18 3.84008369261276
19 3.060174207981
20 2.73901950853128
21 2.21246155524725
22 1.60930178761611
23 1.10227145523025
24 0.515984982062609
25 -0.0876138121672347
26 -0.849001345468421
27 -1.72902284884281
28 -2.92094971411101
29 -4.06721084182952
30 -5.31379147507443
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.48302080353988
1 2.75450732156744
2 1.97018905864348
3 1.00469219856083
4 0.000741584958047437
5 -0.549821713352402
6 -0.489433043097921
7 -0.178937749427054
8 0.235523127954063
9 0.646442677400894
10 0.684691216300838
11 0.5310430177851
12 0.496843355093875
13 0.417523318110394
14 0.453270461816496
15 0.411196092332041
16 0.237657573329579
17 0.0230687821163522
18 -0.352678701430346
19 -1.13468054000604
20 -2.00219921726275
21 -3.48082679647331
22 -5.30694848892631
23 -6.99611606958332
24 -8.69104277035775
25 -10.6506435819663
26 -12.4128674527993
27 -14.1418181948049
28 -15.6686252187323
29 -16.8801766966399
30 -17.8492773009057
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.50141159040747
1 2.58470563615321
2 1.6505762285003
3 0.780753700056138
4 -0.269749953922894
5 -0.947260782971132
6 -0.947506208280427
7 -0.726297587147682
8 -0.334392189124459
9 0.0557925010098479
10 0.339928830926736
11 0.277727425318822
12 0.193629205738
13 0.189832229783472
14 0.16463858443274
15 -0.223204550662811
16 -0.73572285051537
17 -1.46629525793707
18 -2.7358298458263
19 -4.47262603386384
20 -6.73443679436936
21 -8.60987525252867
22 -10.6995084294828
23 -12.6545590635942
24 -14.4782100639041
25 -16.1694662819817
26 -17.7874466806374
27 -19.0397069801107
28 -19.9712827384576
29 -20.7562061497387
30 -21.0398086921237
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.50392260809156
1 2.74029012051009
2 1.62073921865878
3 0.68269487685764
4 -0.466222619417467
5 -1.43059455586455
6 -2.00665912470898
7 -2.39600448594869
8 -2.54625549467924
9 -2.56543901792944
10 -2.85755892545318
11 -3.32704506094186
12 -3.88707244561333
13 -4.92737477354427
14 -6.44127520462661
15 -8.44670857522703
16 -10.3831236568667
17 -12.2235289736969
18 -13.8680513293349
19 -15.1741375737579
20 -16.2651254573618
21 -17.3232696451691
22 -17.8712497695563
23 -18.0271516957004
24 -18.016856325955
25 -18.0598344820417
26 -17.9306982440581
27 -17.7001948953761
28 -17.3509299201891
29 -17.0736528889028
30 -16.6990303391503
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.48648430731778
1 2.68860774069719
2 1.74894092439285
3 0.858601528434254
4 -0.034938935265848
5 -0.75777760099764
6 -0.76171350208166
7 -0.617123540016107
8 0.0542766821685003
9 0.519154979219031
10 0.784902602175982
11 0.71019910684254
12 0.764287624895315
13 0.73173406924255
14 0.755884545973284
15 0.518239442827565
16 0.042532267680476
17 -0.655556275961859
18 -1.71622145119905
19 -3.30591901736118
20 -5.25700418688629
21 -7.10179180575241
22 -9.03239024951285
23 -10.9414971142881
24 -12.7865226457531
25 -14.782070295576
26 -16.4541041105128
27 -17.875466979216
28 -19.0537554475398
29 -20.055278975413
30 -20.8030847315798
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.47108740484166
1 2.73451229248894
2 2.0008573550383
3 1.10490100681228
4 0.173775159379638
5 -0.311097389101164
6 -0.136051501733203
7 0.308830230991933
8 0.802985936822675
9 1.25098587862591
10 1.35400282068471
11 1.46019088557862
12 1.70443165723542
13 2.16463582179103
14 2.5404245436033
15 2.79338419741926
16 2.93971010384141
17 2.99991521288855
18 2.90554762716214
19 2.63598796237014
20 2.27115703991403
21 1.95213264240157
22 1.49952925288918
23 1.04494818877951
24 0.47328607766298
25 -0.015867925646599
26 -0.353012115319157
27 -0.581616255742101
28 -0.807314311422886
29 -1.3434183970815
30 -2.13168376053317
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.51811014116807
1 2.6405772400345
2 1.7060465092943
3 0.689598404503093
4 -0.445779986077088
5 -1.10750165937436
6 -1.55648482754325
7 -1.7413520550796
8 -1.5773474903149
9 -1.21331190158698
10 -0.898258396175363
11 -0.527465162031205
12 -0.120923831244545
13 0.557389529255314
14 1.18441460615701
15 1.60998520919077
16 1.72560763715191
17 1.65992947370019
18 1.34400619522796
19 0.943134199357449
20 0.596655839795636
21 0.306087769999325
22 -0.0187778009457991
23 -0.246879245169838
24 -0.387364198243081
25 -0.567799671828433
26 -0.662137488862995
27 -0.664386405003568
28 -0.592636329448246
29 -0.503477261465962
30 -0.23445947378322
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.48880900565183
1 2.87227688806702
2 2.08044092723365
3 1.20305517190559
4 0.299167880411311
5 -0.229429491661922
6 -0.214101463321397
7 0.209172954558751
8 0.92932911396671
9 1.13170046403039
10 1.32385313400342
11 1.26211021107231
12 1.38550185017913
13 1.61375609347606
14 1.99840611842606
15 2.55531634134972
16 3.05726191997144
17 3.27726720930876
18 3.28517694384631
19 3.23113127579013
20 3.12550688622129
21 2.96935353170257
22 2.58854005917019
23 2.28817469195074
24 1.8840309949657
25 1.56842533421891
26 1.17151332413944
27 0.882919191399818
28 0.616562477376505
29 0.233544868528939
30 -0.355060750371555
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.49683442950868
1 2.7944283352459
2 1.91497088749589
3 1.15546830215233
4 0.158384478494593
5 -0.236691525676602
6 -0.169488466519906
7 0.332967939397449
8 0.926590245398219
9 1.47802088423369
10 1.9577164444691
11 2.2528334820996
12 2.50828719412177
13 3.15955946511628
14 3.57925530655424
15 3.96032184299172
16 4.07480304700859
17 4.20001666725812
18 4.31806112900277
19 4.0289751066423
20 3.62060785817207
21 3.1003317275567
22 2.56763940389316
23 2.075776011712
24 1.75517641475354
25 1.31555095856615
26 0.757246734261596
27 0.322096923604584
28 0.0393097088831833
29 -0.327949813819893
30 -0.876026419586848
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.50747845884962
1 2.55687696880833
2 1.6721538868898
3 0.775719099953119
4 -0.29810752084336
5 -1.18810732977996
6 -1.72874024084452
7 -1.94660819383811
8 -1.72409501462015
9 -1.55348740932375
10 -1.49625876627714
11 -1.39938493968661
12 -1.16158306025726
13 -0.942110686314829
14 -0.833254901926311
15 -0.929356109183664
16 -1.05152796660578
17 -1.15295227949297
18 -1.37159433691995
19 -1.73734995398091
20 -2.09421860837035
21 -2.48779421051125
22 -2.92296024180767
23 -3.54897539335111
24 -4.47483316330423
25 -5.63276444333211
26 -7.26520393380801
27 -9.06480292100426
28 -10.9167931159985
29 -12.8891368117775
30 -14.6765401696479
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.47795202003928
1 2.60530993928782
2 1.71235142774742
3 0.902727012883714
4 -0.0081794533526709
5 -0.59292388656944
6 -0.477760443699348
7 -0.176506069706283
8 0.208126047518447
9 0.533780148908443
10 0.69311056819987
11 0.73507162240682
12 0.787552932324717
13 0.909902611880861
14 1.03032981336528
15 1.09821697761442
16 1.20518494863143
17 1.15677755812036
18 1.16318123753624
19 1.13918611404004
20 1.13581627462512
21 1.18577995983345
22 1.29353474887402
23 1.37482476526874
24 1.5747512805777
25 1.86332829919516
26 2.05794307422816
27 2.2601654697176
28 2.53793526361587
29 2.81087747599901
30 3.04904447109033
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.46811981242584
1 2.65998577995005
2 1.75977518151931
3 0.746518891494055
4 -0.243221881359962
5 -0.852937895612923
6 -0.860850392960931
7 -0.717661172972867
8 -0.446401257463919
9 -0.240504849446005
10 -0.0735741766299189
11 -0.0969931247872637
12 -0.0933821030191879
13 0.157073502513642
14 0.295845726074361
15 0.490537809932206
16 0.544243038173617
17 0.604405663600337
18 0.722325145432529
19 0.831660543537814
20 1.00494263187799
21 1.07959422299947
22 1.21906611567963
23 1.35574777083711
24 1.32330735481138
25 1.17510885272235
26 1.16156134363761
27 1.10303943460036
28 1.05405309028537
29 1.07490545576922
30 1.07255911519934
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.51384163335417
1 2.68714222688351
2 1.65244602152931
3 0.746439729761304
4 -0.138835307953849
5 -0.694470327061728
6 -0.665380573291952
7 -0.454345096900317
8 0.0852620287725787
9 0.481378538558991
10 0.605014577240121
11 0.635176597543772
12 0.476682665179615
13 0.254573974268704
14 -0.101122537927653
15 -0.658673307496431
16 -1.71294053781117
17 -3.22195154922122
18 -5.00746378966291
19 -7.01836547292244
20 -9.12846256742673
21 -11.1500495598543
22 -13.2337224356989
23 -15.0609090579605
24 -16.623537230855
25 -17.9038997261826
26 -18.9660252133975
27 -19.489592012834
28 -19.9408951188654
29 -20.3079177632632
30 -20.3394612966048
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.50142987293631
1 2.74034514704821
2 1.87076445672712
3 1.15236663983754
4 0.224567534755481
5 -0.0904992156261304
6 0.165249751510566
7 0.905012087908576
8 1.72692137279296
9 2.45844943129032
10 2.95388288207632
11 3.37331356897247
12 3.92812799353901
13 4.46821818234917
14 4.73638345713684
15 4.65752228561609
16 4.44079747360235
17 4.16903057172908
18 4.03323709240377
19 3.658715404648
20 3.26803221714883
21 2.86721773239489
22 2.28490794445709
23 1.78692604499056
24 1.29900850158317
25 0.826615279089509
26 0.441057238096025
27 0.115164606162083
28 -0.038375244390485
29 -0.487978258265131
30 -1.06394703630857
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.45996551264541
1 2.72367313620455
2 1.86054833805602
3 0.96557296487537
4 -0.0321208376423645
5 -0.642890066848601
6 -0.726944567391794
7 -0.379401983158175
8 0.0206410811571813
9 0.220602714800435
10 0.157698220363087
11 -0.113467582951593
12 -0.424488899154178
13 -0.579872486333143
14 -0.823307166313412
15 -1.20917660358935
16 -1.61490092916472
17 -2.29410762982647
18 -3.0802674232438
19 -4.00592330771744
20 -5.27289366287222
21 -6.65893613255043
22 -8.20713670464007
23 -9.60262886317719
24 -11.3243356623916
25 -13.2495602000723
26 -15.0507140174543
27 -16.8460842269731
28 -18.46762111093
29 -19.7941111587433
30 -20.4949370808265
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 3.46908612200809
1 2.82009101700113
2 1.95208740561066
3 1.11459238940909
4 0.303420921287629
5 -0.102036347149998
6 0.150685747526986
7 0.551642706820922
8 1.09655106456671
9 1.46022191873189
10 1.56471777448535
11 1.54602077580402
12 1.48114031132823
13 1.58267151159206
14 1.6687447103707
15 1.73930408779914
16 1.85419327741086
17 1.82122054874584
18 2.00932776764307
19 2.4139707291308
20 2.71494033506285
21 2.79298780159685
22 2.8145007971984
23 2.79425255210913
24 2.42318073165545
25 1.96391930520444
26 1.42349139554246
27 0.973630468981912
28 0.628520939045737
29 0.4502034065555
30 0.360981164993407
};
\addplot [line width=0.01pt, color1, mark=*, mark size=2, mark options={solid, draw=black}]
table {%
1 2.65103446372252
2 1.87298481713709
3 1.03310235020523
4 -0.0349224785257646
5 -0.681923979276541
6 -0.614035490335335
7 -0.208100847346677
8 0.33428430837777
9 0.710486243049944
10 0.726233644866842
11 0.520411660737353
12 0.347599665643602
13 0.244300607278545
14 0.195112904269273
15 0.20629800498181
16 0.161911176310666
17 0.161283251423433
18 0.247899352697984
19 0.208651205023874
20 0.171253015388636
21 0.20029198108343
22 0.172890109571832
23 0.187770311286831
24 0.213147053788955
25 0.185796243819713
26 0.165625930691843
27 0.187584184388062
28 0.20252014981221
29 0.179459395114634
30 0.2013127196102
};
\end{groupplot}


==> experiments/figs/double_pendulum/tikz_samples_ep-2-all.tex <==
\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}

\begin{groupplot}[group style={group size=1 by 3}]
\nextgroupplot[
xshift=-8,
title={2 episodes},
title style={font=\large},
ylabel={\textcolor{color0}{inner angle}},
ylabel style={font=\large},
xmin=-1.45, xmax=30.45,
%ymin=-5.18312483023826, ymax=6.87015257507078,
ymin=2.7, ymax=6.7,
width=\figurewidth,
height=\figureheight,
xtick={},
xticklabels={},
tick align=outside,
tick pos=left,
x grid style={white!69.019607843137251!black},
y grid style={white!69.019607843137251!black}
]
\addplot [semithick, color0, opacity=0.1]
table {%
0 2.99645252475745
1 2.59799875123799
2 2.9355365826807
3 3.24341145731169
4 3.25687949966615
5 3.53023037381882
6 3.73059949022062
7 4.04959501579868
8 4.60288041697881
9 4.57341369639449
10 4.48179884196027
11 4.66609993346037
12 4.48239930027858
13 4.54102950125497
14 5.00290646173193
15 5.54750548797208
16 5.94724930431024
17 6.19890127358825
18 6.03889784716788
19 5.97115667346985
20 5.85154672775038
21 5.38000727307072
22 5.50456701614241
23 5.46861963536631
24 5.18253347545986
25 5.40519021554219
26 5.80703624217496
27 5.70025964779112
28 5.40210569941033
29 5.29998769197492
30 5.53949078273043
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.01780319717589
1 2.64727765368762
2 2.85345918189928
3 2.34879753632435
4 2.66001250889336
5 2.18227468149846
6 1.98102538689299
7 2.23457535112792
8 2.71212791695408
9 2.91000544367913
10 3.11122605338365
11 3.09588345686598
12 3.63974896777234
13 4.58949019735021
14 5.18716969068454
15 5.86315496933276
16 6.5751592829428
17 6.94334510862391
18 7.51393202542129
19 7.5200584797946
20 7.86855269433773
21 7.85883572285994
22 8.00951645026308
23 8.18272903784185
24 8.10248097334342
25 7.91049630417811
26 7.89857126180446
27 7.97295642985681
28 7.44864318102702
29 7.39961321611837
30 7.29044656091555
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.02931790408055
1 3.10401287423945
2 3.07636384697946
3 2.5271172652508
4 2.32135420585101
5 1.88813352822158
6 2.14038537746624
7 2.35404296100222
8 2.55044543842369
9 3.04476800510525
10 3.30714477507962
11 3.75215958409811
12 4.44820250355189
13 4.4989995194394
14 4.29090815057825
15 4.14553556028996
16 4.3140579975132
17 4.54273324867439
18 4.18507601017984
19 4.22712823135662
20 4.18774752562825
21 4.1600303849048
22 3.85852603387599
23 3.86995950481027
24 3.67566693363698
25 3.787321115782
26 4.08819743139543
27 4.16330800671282
28 3.97763903346473
29 4.17809370278473
30 4.37907826919217
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.00716140479953
1 3.00635919612387
2 3.15109519818716
3 3.36192444469434
4 3.9295260796996
5 3.54070457107573
6 3.62848180326415
7 3.63294288445093
8 3.39167909678403
9 3.30123459783797
10 3.25648985270355
11 3.49581466178134
12 4.186682831271
13 4.97881449867316
14 5.71514272319287
15 6.62159171878279
16 7.52607835540853
17 8.26593976690203
18 8.94138011534569
19 9.19387316830569
20 9.61241598144946
21 9.97493576187978
22 10.3545883994006
23 10.5707045368923
24 10.9432017157088
25 11.2330955480354
26 11.3830849148621
27 11.864942464396
28 12.284677243588
29 12.8922095215608
30 13.088535614849
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.03312759535966
1 2.92649803666616
2 2.94847813696948
3 3.21892211937654
4 3.03442718242964
5 3.25718686939921
6 3.56580670432692
7 4.18649010386344
8 4.71108016883375
9 5.00444795102776
10 5.30322302549738
11 5.30531441566642
12 4.52362873183173
13 5.00115111429772
14 5.0472565807142
15 5.24000150057561
16 4.96791517025458
17 4.74520003727236
18 4.23188437043172
19 3.97277614700405
20 3.54654697718828
21 2.96433770334018
22 2.35504574795239
23 2.0801853696486
24 1.34050844650718
25 0.778024872909265
26 0.358127930673261
27 0.222420011528655
28 -0.539611872368724
29 -0.792628986883884
30 -0.97177582181262
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.03706970503173
1 2.43811398507405
2 1.95740153789069
3 1.83128550434652
4 1.40028979393141
5 1.09266828339204
6 0.80168210059165
7 0.98527353180244
8 1.18079968996865
9 1.14113639068464
10 1.61711636308691
11 1.60076742465482
12 1.42064496750817
13 1.88684141297805
14 1.95115283109291
15 2.42053676264275
16 2.39808992666487
17 2.28347673199531
18 1.81169056433795
19 1.49355103428285
20 1.36735546864669
21 0.993632981367638
22 0.497316403609553
23 0.141622443229811
24 -0.33660817348645
25 -0.913117541487771
26 -1.3037480407319
27 -1.76110780516401
28 -2.32179384685676
29 -2.89581831654431
30 -3.21332956056634
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.01807237206453
1 3.45554889376243
2 4.18556030170002
3 4.75048816736734
4 5.34036509208596
5 6.02162339886018
6 6.54999587632203
7 7.20537423517771
8 7.72206078895529
9 8.51434861187902
10 9.01744974050099
11 9.18581815402759
12 9.02505511349623
13 8.85093992218198
14 9.57454236309034
15 9.58682766030989
16 9.87940565524809
17 10.1673209336364
18 10.4850409346822
19 10.8248960841617
20 10.6571483374352
21 10.9113173769459
22 10.7649455136075
23 10.3524211490262
24 10.436321539059
25 10.1255817397685
26 9.55729388846729
27 8.97436546884329
28 9.3414193221536
29 9.01246601311937
30 8.32966326413045
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 2.99542592323086
1 3.51841289284803
2 3.44357784598669
3 3.69551855898578
4 4.21459913535153
5 4.29449760556798
6 4.73430991187715
7 5.18726256516281
8 5.87576303110047
9 5.86830017916375
10 5.79507953700317
11 6.09260224094323
12 6.40260501102254
13 6.41733573812151
14 6.43164332716171
15 6.23622821854649
16 6.10056250725338
17 5.92124283787071
18 6.41507190209643
19 6.7953575095079
20 6.77789042700427
21 7.61791347387473
22 8.02679268056211
23 8.19470313549511
24 8.73781993535644
25 8.67432202742077
26 8.80172749498299
27 8.95640949097345
28 9.25550636382578
29 9.3400621817195
30 9.66321440215368
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 2.99525140927671
1 3.29761557261265
2 2.78569565681403
3 2.45937449235747
4 2.72849740184804
5 2.9998034195879
6 2.7246337574541
7 2.76014197575517
8 3.18032877141459
9 3.44354315438152
10 3.3572348627444
11 3.09812605060048
12 3.02464714700631
13 3.54804082399552
14 3.34289816412897
15 3.67084989985741
16 3.7431738032229
17 3.37258083763936
18 3.0771714429701
19 3.09424925475374
20 2.99538612559437
21 2.66066388699656
22 2.44758405242445
23 2.47931919022297
24 2.36700485904444
25 2.04647549501164
26 1.85615878788348
27 1.79542720064117
28 2.0116794155152
29 2.03891165139302
30 1.94569713910807
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.02755800569357
1 2.97410288156293
2 2.95843817239545
3 2.98595591298848
4 2.50711650770861
5 2.68974505138814
6 3.39554001846979
7 3.61672031803854
8 4.20911389228592
9 4.85722041330585
10 5.07948650720509
11 5.38797151669382
12 5.28829980712386
13 5.86098545591916
14 6.4062712611512
15 6.99761308272523
16 7.06276934435364
17 7.36101067896611
18 7.24906200082776
19 6.75430105175815
20 6.92307661355738
21 6.75233841099356
22 6.48192070024514
23 6.36906126931017
24 6.21160308960651
25 5.77593359626371
26 5.25602077865192
27 4.87791107139959
28 4.5536443861352
29 4.2396249533171
30 3.8973352679504
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.00266148213299
1 2.95170552413132
2 2.64094300687438
3 2.11809781553155
4 2.07206980125448
5 2.57783519844561
6 3.09311648710207
7 3.81609436481661
8 4.532255962306
9 4.84581102276092
10 4.83829808083495
11 5.00284877425308
12 4.85981900584532
13 4.6995723683186
14 4.55306724917197
15 4.59944146666175
16 4.53936117983758
17 4.37355263289338
18 4.13729705100873
19 4.02436546415516
20 4.0655983254547
21 4.09710552096806
22 4.40091639663977
23 4.25525680591416
24 4.33745705852453
25 4.22930072351172
26 3.93822315695767
27 3.91704675913767
28 3.68332381708331
29 3.65772760627675
30 3.57097872945546
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 2.99503703370153
1 2.41064660278389
2 2.50656232563302
3 2.58357933395275
4 2.34995298144948
5 2.6504608106367
6 2.38986176127758
7 2.42752995126094
8 3.02832922872784
9 3.11978719581066
10 3.30358212358921
11 2.90286163355626
12 2.76627872362973
13 2.32573674792186
14 2.47950453530363
15 2.27062880950374
16 2.21550954037806
17 2.3088975031685
18 1.88030439309708
19 1.37007208122048
20 1.23613587248693
21 1.22697812359327
22 0.972393065176123
23 0.635816222406297
24 0.323596416368862
25 0.0510049623866835
26 0.0664013856399701
27 -0.226903643737057
28 -0.31427821265409
29 -0.585218696829805
30 -0.754694405158642
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 2.99348599446338
1 2.95456008523909
2 2.83383690589451
3 2.86183912147682
4 2.93573856568332
5 2.9913396996786
6 3.64979860244962
7 4.02256760572367
8 4.38529718198227
9 4.96192094488659
10 4.88784421897924
11 5.23336604136572
12 5.45582722186482
13 5.87374513041896
14 6.11475031518447
15 6.30161877312043
16 6.38889345823295
17 6.1524715162436
18 6.47330976921026
19 6.3558423212936
20 6.72256950116764
21 7.12343572282349
22 7.23807714103869
23 7.16672652720874
24 7.42409200076871
25 7.12521729862627
26 6.99134906329079
27 6.5835828706951
28 6.59949321625556
29 6.4385555426996
30 6.29820741306077
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.01024042371685
1 3.24999411972551
2 3.83403386009344
3 4.28295562967651
4 5.25022837063677
5 5.04025807517352
6 4.8573434710969
7 4.95913076085219
8 4.94301634154342
9 5.3678899386862
10 5.25813878672788
11 5.07319355229644
12 5.03701180579179
13 5.10331881829183
14 5.75856723788328
15 6.05049254091112
16 6.69160900867217
17 6.6892635623696
18 6.79536113501551
19 6.88600341615057
20 7.26562074272513
21 7.35482485368086
22 7.78745056490251
23 8.08221835694519
24 8.39660042517852
25 8.69107839707405
26 8.94394615196128
27 9.07473044751576
28 9.26398611644056
29 9.43373488924672
30 9.44693146656079
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.00299826997831
1 3.19899935186941
2 3.18959485265591
3 3.09351585981511
4 3.45129358912377
5 3.4418599329027
6 3.34130253770597
7 2.73200707786948
8 2.05685082746416
9 2.3843734666842
10 2.2606369605372
11 2.38819049229676
12 2.87896708280908
13 3.79109294847057
14 4.87261499711824
15 5.83250653148489
16 6.29922670318082
17 6.83111962436355
18 7.03877476732967
19 6.84175713263935
20 7.40421635866291
21 7.23709031220068
22 7.59923310111069
23 7.91220168625296
24 7.85264642125224
25 8.2681106865487
26 8.97435334776571
27 9.13178948631964
28 8.74390883379592
29 8.84115093806913
30 9.3232405244618
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.02350579723812
1 2.89286212928907
2 2.80471882801496
3 2.96993114637353
4 3.41977228528802
5 3.62203066760175
6 3.7560465876763
7 4.15306687379194
8 4.68052898497633
9 4.84817821887756
10 4.60698728813467
11 4.59767715896137
12 4.89386181024579
13 5.33038454326285
14 5.50980348194575
15 5.88085161414391
16 6.24188240949666
17 6.20140397486571
18 6.39187884094372
19 6.30384845568399
20 5.88496005678668
21 5.85986818423539
22 5.30262812813822
23 4.80614494295989
24 4.57329555009573
25 4.2386397493872
26 3.86006526223831
27 3.28636814200288
28 3.08294886169584
29 2.30064308114171
30 1.96861866806805
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.04313603937096
1 3.11720961654226
2 3.03835499715994
3 3.38030427289754
4 3.45946957426851
5 3.98115433397691
6 4.9446278338925
7 5.97024648417226
8 7.19970749797592
9 7.31619349578263
10 7.19493385846627
11 7.47915883111901
12 7.43530565914332
13 7.63362958159471
14 8.06739268551102
15 8.32718659207473
16 8.49741112701784
17 8.46258369425065
18 8.55346893325473
19 8.76103263845276
20 8.84422759063034
21 8.72435587211097
22 8.38271972017609
23 8.46235100425603
24 8.44552264304827
25 8.10483715663251
26 7.79486336381376
27 7.73896731082519
28 7.77377416812198
29 7.45266992971255
30 7.0704451119534
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.0091393720439
1 2.73817070491551
2 2.8441623143268
3 2.96421615892359
4 2.66772589957933
5 3.07265465171855
6 3.49098969862419
7 3.38341633557896
8 3.32840657556719
9 3.87765440115021
10 4.08936714823849
11 4.15169516997032
12 4.31070773273307
13 4.5039494347564
14 5.19655545251725
15 5.63116605415951
16 6.34828165292642
17 7.10165511149397
18 7.29740900965308
19 6.95994031204642
20 6.98935851118225
21 7.14031633478278
22 7.69482235292709
23 8.03510992257007
24 8.04972250720605
25 8.39927623493959
26 8.68995953061259
27 9.15431886405638
28 9.00071131005873
29 9.45386176830727
30 9.72316823012773
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.01949039635972
1 2.88114015232197
2 2.91195925792552
3 2.76100045710067
4 3.1532505932418
5 3.01834691918291
6 3.22946564084363
7 3.24419747991866
8 3.43489874837014
9 3.71456803794541
10 3.84739183694472
11 4.11555851662796
12 4.2579576537416
13 4.60242771558879
14 4.48314563315231
15 4.7748432610471
16 4.7744586077042
17 4.81881671248615
18 4.85850664407873
19 4.48710623639677
20 4.75501194304943
21 4.83889078936509
22 5.14355156801497
23 5.66097320200927
24 6.01408335957416
25 6.00039036685741
26 5.88490383555741
27 6.35374013390181
28 6.57820291531451
29 6.92547790276204
30 6.98998949609539
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.00564876618314
1 2.78590685960383
2 2.9541973973913
3 3.13199985338989
4 2.84988736375488
5 3.21896227340892
6 3.4373376007989
7 3.84382536930247
8 4.37701831697019
9 4.52298148291014
10 4.67131187503284
11 4.68431302091104
12 4.69175392695625
13 5.5673728883385
14 6.04131703144643
15 6.36950542534899
16 6.62096668386382
17 6.46928609145263
18 6.63484448883711
19 6.8132345253161
20 7.06050944741934
21 7.08215710393997
22 7.20769729576649
23 7.42090603971434
24 7.31569524227183
25 7.30339906640048
26 7.30170952825534
27 7.49348947702113
28 7.71771771301621
29 8.09171066638213
30 8.42302654351046
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.02532259057392
1 3.31163794649111
2 3.312873275727
3 3.21877352937208
4 2.89065983207687
5 3.06098414284785
6 3.24644459608724
7 3.86041014329603
8 4.38144143907326
9 4.47351301609117
10 5.02762590199811
11 5.09981371604045
12 5.16027157517828
13 5.36463577436223
14 5.85824795739898
15 6.28852300829484
16 6.66871102508049
17 7.18829760139597
18 7.58379644406993
19 8.00564809662986
20 8.19049660781643
21 8.23873281618133
22 8.10835791375346
23 7.95893313671226
24 7.62150863578477
25 7.52466540693323
26 7.45503461819676
27 7.54113523815404
28 7.16939179925614
29 7.16616257466098
30 7.31838583533834
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.01462797368036
1 2.62906184665173
2 2.3317585871317
3 2.11651552774211
4 1.80608390080904
5 1.84015246656811
6 1.86161012806353
7 1.88254920558322
8 2.14232055464902
9 2.23517148725711
10 2.67203464522089
11 2.66966339155559
12 2.35174982782041
13 2.87503917526959
14 3.27307199200006
15 3.425703571149
16 3.03158036875181
17 2.51094326616672
18 2.29197302386688
19 2.16804956071775
20 2.1296560533169
21 1.70703991283155
22 1.19738216652389
23 0.937670053394652
24 0.539733717456546
25 0.511347542406242
26 0.26299448009896
27 0.0423393312259175
28 -0.226492320303763
29 -0.292208178728844
30 -0.0973370206749351
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.0298080046332
1 3.09299717520994
2 2.54419487783801
3 2.26766891717
4 1.93865436169038
5 1.64121739688407
6 1.88966617240503
7 1.83437160705295
8 1.48511016161316
9 1.82849369251737
10 2.4007866890489
11 2.76827354282747
12 2.5516945630415
13 3.46868771948672
14 3.50911400979611
15 3.87402711707329
16 4.04426703614508
17 3.96591305159455
18 3.30878884125816
19 2.71019857579485
20 2.60243613919151
21 2.20468610660518
22 1.91946039995952
23 1.92636026489672
24 1.86516509943512
25 1.56476136487984
26 1.17948765959646
27 1.08801655771054
28 0.682923756191786
29 0.745907217680812
30 0.579701721650924
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 2.99034655852295
1 3.49825707663621
2 3.75119789363788
3 3.70480593456965
4 3.61151153129255
5 2.68923221948624
6 2.22401426111129
7 1.81882866897668
8 1.32703226611651
9 1.7429841021261
10 1.93813787442624
11 2.41481577649643
12 3.102477817878
13 3.78576841139817
14 4.56032734489644
15 4.98867550267911
16 5.39023520563557
17 5.6279171294591
18 6.05405087317314
19 6.33083076780155
20 6.6427160364814
21 6.96891279496725
22 6.83671949682725
23 6.91777288024726
24 7.14701685932279
25 7.07704356247164
26 6.90331559174568
27 6.97744166203324
28 7.24990743656141
29 7.33159115697026
30 7.23351331376703
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.0451974173611
1 3.13078558343591
2 2.84129747100947
3 1.92686221331394
4 1.41050547521691
5 1.66149206267005
6 1.66705325473628
7 2.26559448222955
8 2.57491833782077
9 2.63056188628372
10 2.49762992431
11 2.95103034692161
12 3.02387090703148
13 3.77348547879547
14 4.0705152526485
15 4.37088497194848
16 4.4417082680102
17 4.52374826621524
18 3.98636779262439
19 3.52962782019208
20 3.44539160074958
21 3.15133434089966
22 2.87152476155502
23 2.49831680600521
24 2.22270408870339
25 1.99890381764841
26 1.87580286975012
27 1.64753308760217
28 1.27191733496516
29 1.15855884880863
30 0.836857568365386
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.02537518647782
1 3.16837839121776
2 2.78856712533976
3 3.30618770564302
4 3.80490373953792
5 4.16335591329506
6 3.94530739217952
7 3.98015426635511
8 3.75320079321141
9 4.32856423179712
10 4.93771821470969
11 5.55549502409647
12 5.9298848599456
13 6.61972650370752
14 6.65975954295501
15 7.27819247753176
16 7.4002765907247
17 7.7411097875459
18 7.94017588434715
19 8.10046671252976
20 8.54791218336961
21 8.99433489324001
22 8.8308591652262
23 8.78047164627942
24 8.25129757312749
25 8.04383268307856
26 7.680137506303
27 7.31509554627871
28 6.95353653076079
29 6.29523511802608
30 5.66461018048374
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.02522513818247
1 2.95692293599107
2 2.49049482506672
3 2.78931082270067
4 3.09500606811382
5 3.36668347859683
6 3.35658752549871
7 3.37715813006359
8 2.96216651856852
9 2.5956016444346
10 2.89043398708495
11 3.17860903500625
12 3.787202793296
13 4.11095929725006
14 4.30806151240989
15 4.67320839929809
16 5.18531135142405
17 5.79497891605154
18 6.47315593097384
19 6.58818133703873
20 6.92447746716128
21 7.4031217734786
22 7.72895444509955
23 8.09494624613306
24 8.46723958529509
25 8.68928265828071
26 8.92429052100484
27 9.09037786375068
28 9.12671650715167
29 9.41132207391923
30 9.36239763825356
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.00289511846949
1 2.98856162302088
2 3.18857785524573
3 3.00197547414564
4 2.6666595612424
5 3.08288715595912
6 2.77528193554514
7 2.64894248649817
8 3.00675141075288
9 3.29440783417274
10 3.55195529363794
11 3.47539838293781
12 3.97944426472199
13 4.7662631728044
14 5.08978002955736
15 5.618684452231
16 5.78190508836008
17 5.69075510682916
18 5.72306381937752
19 5.76835367128635
20 5.95458502581359
21 6.21027802895667
22 6.09172351138995
23 6.03482521924318
24 6.03473501405814
25 6.0843163709417
26 5.9652362035801
27 5.77657412879412
28 6.0314975813527
29 6.04979365914105
30 5.99622481977187
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 2.99747247627481
1 2.37965488002577
2 1.98111988469452
3 2.15913704497623
4 1.55930972570038
5 2.68122989630341
6 3.22262019388255
7 3.95788916448811
8 4.7680836400962
9 5.39982519864332
10 5.58386556269802
11 5.767140845425
12 5.65418567855196
13 5.57996986824246
14 5.66909204209407
15 5.72118711338027
16 5.75943028777977
17 5.68460594165309
18 5.55035140267071
19 5.422410589333
20 5.81865102158006
21 5.54799436719147
22 5.38509397314426
23 5.39467106728173
24 5.51583974485651
25 5.70441262541617
26 5.80284472281705
27 5.91330688007399
28 6.03648725168472
29 6.13263468203355
30 6.27827180867932
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.010791615347
1 2.74489929287868
2 2.40587091667218
3 2.84396734242515
4 2.59633258305878
5 2.16868511001952
6 2.49905322539005
7 2.1837805072589
8 2.27821852837239
9 2.37612119311911
10 2.73149618271156
11 2.60787925558239
12 2.45928244028744
13 2.85472487958978
14 3.50913338864736
15 3.79563490761247
16 3.8841789048989
17 3.99738467736012
18 4.02114636823824
19 4.30748371519639
20 4.68134021431707
21 4.88767085310537
22 4.87709826551223
23 5.02350490336823
24 4.98109610124602
25 4.78738188591724
26 4.61575421424611
27 4.26012009841671
28 4.2338988049107
29 4.13954733175887
30 4.25572663854382
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.02027865682919
1 2.96671792040108
2 3.41722934631556
3 3.45459549320976
4 3.85100728084899
5 3.76484235760729
6 3.84826782863294
7 3.83485012504923
8 3.88098244170111
9 3.88343361130957
10 4.12995980786346
11 4.22115717892722
12 4.76339666440614
13 5.21410372406332
14 5.61147682766342
15 5.6350414735366
16 6.12117725396189
17 5.97817333809531
18 5.99849806646687
19 6.1814509952593
20 5.87361599576923
21 5.67606644061242
22 5.47957271989538
23 5.47316467110101
24 5.11930335937814
25 4.90962043277533
26 4.86263106286982
27 4.84446806914989
28 4.56091767131067
29 4.52175542422789
30 4.60999464608193
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.01683497913197
1 2.54573381206973
2 2.77393748791766
3 3.49217355993195
4 3.84298934155026
5 3.45704739331458
6 2.55324230556351
7 1.82087373849876
8 1.31340696104907
9 1.32477904815648
10 1.24826422262266
11 1.18307735846758
12 1.68629568079556
13 2.14231739732026
14 2.7978779873729
15 2.67894011080618
16 2.67717731275541
17 2.79693757038459
18 3.00768356677132
19 3.22684826474837
20 3.3081751115924
21 3.28917681753522
22 3.30470624902065
23 3.41828766217996
24 3.21386363105442
25 3.1055321995526
26 2.99054995416888
27 2.67174600533205
28 2.70199142402342
29 2.6855569677318
30 2.54864507693989
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.04495967833223
1 3.22758755465938
2 3.51817175930868
3 4.02655165452578
4 4.07176835805383
5 3.9997469808216
6 3.97851920555269
7 4.35572727423125
8 5.00326858502203
9 4.91142042812303
10 4.85005480751356
11 4.99141981634636
12 4.71478523702478
13 5.45431311266092
14 5.96079564768675
15 6.40790149260917
16 6.2913357574478
17 6.65243626889076
18 6.06366529371306
19 5.9063714838511
20 5.74203642288553
21 5.45075719278625
22 5.09348696321373
23 4.66173168718538
24 4.05417777043273
25 3.55748325334953
26 3.20055677935812
27 2.76333212993567
28 2.54304610907697
29 2.24646837051815
30 1.93740513577026
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.00095714431021
1 3.4015994230777
2 3.52660778361509
3 3.55576781976135
4 3.85877547583894
5 3.97044416853843
6 4.26384026805388
7 4.25603644848574
8 4.30419380747906
9 4.78508793938022
10 4.81915710546292
11 4.80678260172478
12 5.09362246127139
13 5.40523351981697
14 5.37412000926243
15 6.00402322062634
16 5.81183319152126
17 5.88872822699714
18 6.14325634955703
19 6.16224340833591
20 6.26440299175604
21 6.0756810772766
22 5.8843987403207
23 5.8209432154202
24 5.66134369713468
25 5.60235800782425
26 5.45921984223445
27 5.38003919047892
28 4.95226907269364
29 4.83996670292295
30 4.47165315477233
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.03266714587724
1 2.99770355598574
2 3.1123808619059
3 3.26326896434227
4 3.18491986205602
5 2.96855266125628
6 2.55309006973621
7 2.22074107146023
8 2.1532258537007
9 2.47013917338288
10 2.54717891311661
11 3.1422409536327
12 3.29288927874041
13 3.73642559194722
14 4.15816231879166
15 4.84122631037037
16 4.91917287726314
17 4.95979702918334
18 4.67241576424403
19 4.57932942109957
20 4.75232296602726
21 4.40567694391028
22 4.45229111205198
23 4.4378000959687
24 4.0337214066596
25 3.78756637731203
26 3.46830662689631
27 3.31764862781254
28 3.03805013216204
29 2.87581545101177
30 2.70935012446605
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.01703571473147
1 3.04683878858014
2 3.25124261894935
3 3.57135733527163
4 3.25874252971852
5 3.06084120051336
6 3.03190890929612
7 2.78082313450119
8 2.08921599097092
9 2.40769594601953
10 2.7452850396971
11 2.91422669516547
12 3.15755849169441
13 3.51320394020668
14 3.89611546202095
15 4.13037175846058
16 4.3466897532681
17 4.75547836863975
18 4.62139361712837
19 4.19122275168607
20 4.31770255691737
21 3.88394380288371
22 3.61541057215611
23 3.34915454902058
24 3.01464325375695
25 2.3536025206913
26 1.53599932803
27 1.0487201200585
28 0.624443497511921
29 0.099872242837574
30 -0.585077052044619
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.01651441970601
1 2.62258308211837
2 2.09959450932116
3 2.04854835571259
4 1.34725429674689
5 1.58975885498648
6 2.29868068192155
7 2.68213287026166
8 3.21264786961377
9 3.48714932779779
10 3.53270821807843
11 3.49645662837204
12 3.71947682296228
13 4.33871710036964
14 4.57713273214206
15 4.69323803507949
16 4.44638594630277
17 4.45005610327129
18 4.21979113994737
19 4.02010973248821
20 3.84000300006062
21 3.75179115577656
22 3.19343459978636
23 2.90899679638581
24 2.54911158349713
25 2.02940516586571
26 1.71537285795793
27 1.2577289426004
28 1.02716616961426
29 0.545409526097979
30 0.127149674548241
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.00522885049921
1 3.10601620155461
2 2.73758200566931
3 2.18045872523501
4 1.86280722088273
5 1.66909794000868
6 1.72588641976325
7 1.43396902081789
8 1.37410723374995
9 1.22052872330304
10 1.09339684771062
11 1.33044921613683
12 1.86123726377858
13 2.12439166942121
14 1.98218725464228
15 2.15187917256877
16 2.08500819922407
17 1.91097913764259
18 1.76349395683606
19 1.53711683286225
20 1.51397963188739
21 1.12729372026042
22 1.18221393323192
23 1.00754641934713
24 0.776641313811583
25 0.555572555594586
26 0.31710218107023
27 -0.0120417130932067
28 -0.285321492857664
29 -0.583252363217853
30 -1.02922269500959
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 2.98467120940056
1 3.55986324840698
2 3.77864557869309
3 4.18091173933431
4 4.3534245322802
5 4.67364163211358
6 5.35639289145823
7 6.14235187240548
8 7.07192752012219
9 6.76934067682335
10 6.65150610899334
11 6.62988309494909
12 6.6259038434214
13 6.92962775028048
14 6.89099422056093
15 6.69239981699848
16 6.83817047478618
17 7.24413444607327
18 6.92744096085073
19 6.69960117525277
20 6.62060000251995
21 6.52440870776779
22 6.53386394017686
23 6.20337096149787
24 5.82195551270638
25 5.90591621603955
26 5.94873580011446
27 5.50248788133517
28 5.48367327519842
29 5.13011708250418
30 5.05141910928726
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.01685736550235
1 3.1890327720065
2 3.52711245210348
3 3.15079214748567
4 2.94600684915463
5 3.22479613275548
6 3.26389089982956
7 3.52619591748878
8 3.59841153295746
9 3.82209467317987
10 3.92960109244949
11 4.28941555953265
12 4.27223578631223
13 4.71105386826771
14 4.59912373798385
15 4.72402952524996
16 4.67452169353232
17 4.68253417755997
18 4.32778532527028
19 3.99250321641798
20 3.80322851545235
21 3.64285686053648
22 3.77335058875699
23 3.39016109871922
24 3.05400772895103
25 2.61365823222506
26 2.1477418966362
27 1.74539152620966
28 1.08190225155413
29 0.929981573644965
30 0.618460638516122
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.03715419423321
1 3.07760563185382
2 2.98273454726434
3 3.09682840273121
4 3.24793370546017
5 4.5180150594435
6 5.05571673984498
7 5.47355038749811
8 5.93359217728324
9 5.85449734891347
10 6.59616933405231
11 6.52243003611972
12 7.64322606160503
13 7.91580604483546
14 8.26681701711221
15 8.16176676456238
16 8.65291033452007
17 8.712697844312
18 9.37980046244649
19 10.0280471587608
20 10.0266568369359
21 10.6235309843883
22 10.6138525623431
23 10.5421683145498
24 10.9005914012495
25 10.9794269800951
26 10.9437044569762
27 10.9745575539412
28 11.269122099918
29 11.29617770975
30 11.2079272878729
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.00389527673249
1 2.78243287155419
2 3.03808462088861
3 3.86367424751017
4 4.20216716564637
5 4.45810640557223
6 4.71605153666023
7 4.7420706649081
8 4.86447958540004
9 5.03221107130291
10 4.66599000727837
11 4.98454764286898
12 5.00957114711323
13 5.35025872662751
14 5.8233010092081
15 5.84661821748546
16 6.07253440769177
17 6.28997548395047
18 6.37231028478585
19 6.68786969118587
20 6.48126366416524
21 6.63373067999315
22 6.68254482737157
23 6.79420979701465
24 6.87630628601243
25 6.93700552869597
26 6.77510394185394
27 6.85988599302661
28 7.08221202514368
29 7.03361650795297
30 6.94197565313003
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 2.99344646479877
1 2.62171414583869
2 2.66275094107177
3 2.94535185588043
4 3.15389619316347
5 3.22588701680046
6 3.26820267984135
7 3.73752335939248
8 4.20339734540492
9 4.34672123297882
10 4.59397099855655
11 4.84724060172196
12 4.79947026969493
13 4.43137923523376
14 4.20192501523106
15 3.95261727222714
16 3.75891852800502
17 3.40620547192033
18 2.92369729981142
19 2.79205129377899
20 2.26660951866806
21 1.86776208911019
22 1.08886291189995
23 0.823034479132294
24 0.479310124660083
25 0.172091656524135
26 -0.285178025451351
27 -0.808346793340291
28 -0.753531307646221
29 -1.15758259216712
30 -1.57852242797905
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.02909995357784
1 3.35819272264653
2 3.91087947946435
3 3.91901207012543
4 4.15993072136157
5 3.87280808842903
6 3.74998541535792
7 3.57520404796944
8 3.42867424012057
9 3.3433756385387
10 3.18314365511722
11 3.06833147587785
12 3.15270117907338
13 3.68745703710642
14 4.37614470263107
15 4.43336931254462
16 4.94292147243122
17 5.56250280498803
18 6.33099905793625
19 6.67484004241176
20 7.06612252429917
21 7.32014330686055
22 7.4152671950458
23 7.64487681871754
24 7.52702772364218
25 7.23616994864952
26 7.22893669046421
27 7.32878494320962
28 7.32826623283079
29 7.03955295864037
30 7.00293006425001
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.02653703740301
1 3.00457218113833
2 3.07061254914965
3 3.03218010562198
4 3.10910005482499
5 2.75800051527173
6 2.74734185017486
7 3.05063008161944
8 3.45985548286582
9 4.37747301428235
10 4.75582939954139
11 5.15566265885644
12 5.46801451802931
13 5.62090355933553
14 5.97030889208879
15 5.90018163578996
16 6.0256927979143
17 6.63130644351416
18 6.92965925337805
19 6.99185002001733
20 7.0283999886296
21 7.25870890985214
22 7.33970933229623
23 7.47043227595053
24 7.61594199855886
25 7.75267407545494
26 8.0776002187674
27 8.40752886111293
28 8.48830465770263
29 8.89183871421912
30 9.276309751622
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.032620704444
1 2.7899996746589
2 2.94209712476566
3 3.21520368592481
4 3.08277654209594
5 4.10368557042909
6 4.43655944003373
7 5.25482801485859
8 6.0842033008565
9 6.11443376918941
10 6.26841363434307
11 6.27326124226585
12 5.51335505961148
13 5.66541523962362
14 5.82083953450106
15 6.19490604650753
16 5.9149454209129
17 5.97098768555135
18 5.0184943838181
19 4.5638557064012
20 3.51021064306673
21 2.87573754979079
22 2.46609883372715
23 1.90994624341945
24 1.55392855455914
25 1.45227418391522
26 1.13173347241439
27 0.500449329329836
28 0.53476259748577
29 0.181581167215136
30 -0.213534657304748
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.00462305565416
1 2.79720462537911
2 2.76704964451978
3 2.64400150682398
4 3.04631803524491
5 2.74771796703857
6 2.93304043341514
7 3.21952667789968
8 3.50557165988283
9 3.57487163775632
10 3.4392970859123
11 3.1952797833279
12 3.47959234758386
13 4.06454951535068
14 4.62712131756844
15 5.7129421764966
16 6.51686874958264
17 7.07764786120668
18 7.4420370673594
19 7.68475554245737
20 7.96619582420885
21 8.32045364739742
22 8.09712702150284
23 8.09588647557084
24 8.15590093945097
25 8.27661416600412
26 8.52886609047521
27 8.64710807095468
28 8.54520071774081
29 8.74494214181475
30 8.84214860304948
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.03755139771031
1 3.2081014509093
2 3.38833443256847
3 3.52141078254884
4 3.70654999343926
5 4.18232675807985
6 4.5406047393693
7 4.53916138211079
8 5.01959651714405
9 5.21843786780177
10 5.27126544188826
11 5.47471626311504
12 5.68080130263108
13 6.20625546384088
14 6.85619734364439
15 7.24503371955562
16 7.53820016460045
17 7.91239559706955
18 8.28995065701378
19 8.33782426446169
20 8.76130305225309
21 8.81451782536827
22 8.90366264934869
23 9.19866004000875
24 9.11590442942319
25 9.4122369374359
26 9.63142434730867
27 9.8452227517822
28 10.0613582475782
29 10.1066292594466
30 10.3934179509517
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.03264109153816
1 2.69647361726186
2 2.60999921185265
3 3.40360754311381
4 3.47607657504108
5 3.64591190950354
6 4.35739351816493
7 4.82475559755655
8 5.0439304069518
9 5.04321042862451
10 5.21446687680148
11 5.19205887083018
12 5.12598462494301
13 5.74442048018632
14 5.84728614278016
15 6.18174360100394
16 6.4657283081749
17 6.33342586277285
18 6.11988048623493
19 5.94166383017963
20 6.11153472283216
21 5.85439043436715
22 5.7357916422348
23 5.74749150655696
24 5.73559842502786
25 5.65946256807051
26 5.72939672456644
27 5.68137170613745
28 5.85692539159672
29 5.87763765450095
30 5.62161128068483
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.01933711058395
1 3.22072662982493
2 2.66585065588633
3 2.60201451879743
4 2.63037192481657
5 2.79211846293096
6 3.0814496218575
7 3.31826762036879
8 3.77160050975332
9 4.63420313632561
10 5.03763373967306
11 5.22480622327696
12 5.35408391755431
13 5.80714546315172
14 6.46578531127688
15 6.80801883011463
16 7.11182286014538
17 7.50787363281089
18 7.57928052965804
19 7.97504682781005
20 7.93058206176802
21 8.08928100790658
22 7.99722314343373
23 7.77224311895897
24 7.89743273049905
25 7.71964075164187
26 7.68531690400552
27 7.68321871614628
28 7.88273488349906
29 7.49628291991962
30 7.25297958545955
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.00217349776158
1 2.97332880715035
2 3.0960226894095
3 3.17355238650375
4 3.16175909033518
5 3.44146486075353
6 3.64494568713694
7 3.73246690849512
8 3.76729864948826
9 4.00819838077914
10 4.10629519169748
11 3.69070053119389
12 3.72627731845847
13 3.79770228601192
14 4.18008334608468
15 4.68879497605752
16 4.98387220385499
17 5.31374123868334
18 5.11699356434465
19 4.74581400328395
20 4.86904288125604
21 4.67548441239415
22 4.70729986585395
23 4.72225431229775
24 4.60026137735629
25 4.44678102884315
26 4.36473373342521
27 4.38322105629265
28 3.87832241498933
29 3.8100908315765
30 3.63882716429539
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.01777433301985
1 3.06492017297389
2 2.75449730115468
3 2.47041005648153
4 1.84924098922645
5 1.96799449912357
6 1.90309459873748
7 1.89754492233036
8 1.93108570210858
9 1.57094245905004
10 1.39911998683495
11 1.22560496733381
12 1.22746418731814
13 2.31036613653656
14 3.19923471995278
15 3.83530867334252
16 3.94389127788771
17 4.35950516753119
18 4.43029875198976
19 4.41891161253645
20 4.37724212822451
21 4.52466326918386
22 4.50583053403135
23 4.45310725512051
24 4.54809636377201
25 4.23413654292013
26 3.89915850865566
27 3.60833481969181
28 3.73783148468721
29 3.62883907678193
30 3.57569467110161
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.01344201226362
1 3.66731239591245
2 4.15698124844918
3 4.09801061782416
4 4.07127142103263
5 4.51559939258231
6 4.84089747987923
7 4.96915330041562
8 4.79731451081716
9 4.82704667240273
10 4.82473042374602
11 4.6868600495079
12 5.2939458219754
13 5.02215669314993
14 5.30131820408098
15 5.6092550345844
16 6.34047391877803
17 6.86851562649931
18 6.77952541528659
19 6.60302043894551
20 6.56693699606685
21 6.03759620858436
22 6.04740688170674
23 6.20676992801697
24 5.98452667604762
25 6.23884088402032
26 6.17442550160014
27 6.06410191690556
28 5.91627626685916
29 5.71823576359012
30 5.88855545707355
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.01369916653578
1 4.23370189574443
2 4.66803444570241
3 4.98332057227117
4 5.33924970446904
5 5.19677088757355
6 5.55227788165966
7 5.81777507955395
8 6.24834206124489
9 6.39075469975623
10 5.98899633353431
11 6.07400917900278
12 6.5082672827998
13 6.81228026342609
14 7.46488158487263
15 7.54592511721682
16 7.48475375025298
17 7.58038556133323
18 7.86545634257792
19 8.03408211505521
20 7.82575309272464
21 7.9337026767731
22 7.89222210573463
23 7.75013185445277
24 8.14348380860901
25 8.0878021977669
26 8.0168349590987
27 7.96695503333213
28 8.21109748501066
29 8.54837180319529
30 8.41276573343537
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.04240312027982
1 2.91395964260171
2 2.17019982183855
3 1.4853501969202
4 0.656547418960717
5 0.14217696034298
6 -0.207458873682758
7 -0.97730087060517
8 -1.65150723097575
9 -1.33788236245525
10 -1.14864502121363
11 -0.684381268393002
12 -1.23554654968595
13 -0.652810658851457
14 -0.492431942512515
15 -0.367085469510784
16 -0.693898569891139
17 -0.966141583548903
18 -1.39987644081882
19 -1.66072319909976
20 -2.18485611961489
21 -2.49598744280231
22 -2.74209975891194
23 -3.07496679874339
24 -3.51353658269276
25 -3.6672440922185
26 -4.07833582096948
27 -4.11242157578121
28 -4.23180745466877
29 -4.22100698803435
30 -4.55033927067458
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 2.98956143706802
1 2.91584094893636
2 2.77312919301988
3 2.14100182139225
4 1.60599201890188
5 2.31875249094969
6 2.54199953135873
7 3.13997839103653
8 3.86412592189844
9 4.20550990061843
10 4.36061358306487
11 4.80592014034097
12 4.65692523353466
13 5.53690863038784
14 6.18695751796526
15 7.01529943108401
16 7.17148417996832
17 8.04925845773089
18 8.04696038029527
19 8.08635872124935
20 8.07907190278133
21 7.96214686664081
22 8.06548301028771
23 7.90063011548975
24 7.75120721073428
25 8.03254973434771
26 7.98213609107107
27 7.93577477094911
28 7.57983946219628
29 7.29298056791945
30 6.83447782456756
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.0062664267731
1 3.18391837559272
2 3.49077744502565
3 4.02407753408001
4 4.08131039516071
5 4.0714306462626
6 3.76362310468392
7 3.69547338936637
8 3.95840877435164
9 3.97705868253639
10 4.00137754106539
11 4.3426357465922
12 4.33736787130739
13 4.68125847237102
14 4.98325447094238
15 5.32166274608464
16 5.04606095986363
17 5.16204955816832
18 4.61067138099507
19 4.19744105736623
20 3.75036428990418
21 3.31165875686005
22 2.65083445483358
23 2.33376037936739
24 1.86891967234028
25 1.64450426702092
26 1.14218929642641
27 0.710012056241665
28 0.0967566340354971
29 -0.645894510828718
30 -0.952453665363494
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 2.99840514204902
1 3.31711233590641
2 3.48329236057507
3 3.59131269847876
4 3.54142268194944
5 4.39810719415995
6 5.18517679658238
7 6.28083064120447
8 7.07576245361501
9 7.6645720672646
10 8.13695003987235
11 8.21379573214773
12 8.55204853815161
13 8.90362515329391
14 8.93009110675466
15 9.29902301548591
16 9.26429915549422
17 9.44355856020238
18 9.38991099876899
19 9.21260294440111
20 9.67606794749821
21 9.66665688541248
22 9.74189466589767
23 10.2299512999536
24 10.2171996434303
25 10.6147025949088
26 11.2342640131996
27 11.7453494556717
28 11.9416157483089
29 12.672970364095
30 13.3819481898019
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.00242085698851
1 2.37582532030837
2 1.98029187371872
3 1.66059348188922
4 1.19523967999107
5 0.957502794917843
6 0.415301276648934
7 0.69453424629572
8 1.02492662377935
9 0.948676178898963
10 0.866998321951984
11 0.972008854157576
12 0.566134119782545
13 1.169327586419
14 0.941039944129499
15 0.878146645346603
16 1.03623582764638
17 0.890280517049931
18 0.514343136869889
19 0.371171238425266
20 0.295216931751369
21 0.159588622762117
22 -0.0295266307391175
23 -0.40730122066027
24 -0.463964881506691
25 -0.487021285854705
26 -0.771941319551296
27 -1.19694841762808
28 -1.35418678305674
29 -1.70658657325176
30 -1.88458919515163
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.00078534136301
1 2.48900188846252
2 2.18520993690977
3 1.94240768401931
4 2.07208679702405
5 2.50766251804762
6 3.50174124129356
7 4.62522064777715
8 5.65151582062767
9 6.35060816466614
10 6.45661617405986
11 6.69029890536491
12 7.05696262994287
13 7.30482495495207
14 7.45548256750009
15 7.52711528083029
16 7.28429365146498
17 7.44183284432053
18 7.9492526394921
19 8.23473642500298
20 8.1176181688785
21 8.56821292664106
22 8.50218190681043
23 8.64614181625643
24 8.73082568885859
25 8.65498748030337
26 8.83626084814756
27 8.56523337471977
28 8.54987756178649
29 8.42586185493332
30 8.13289528252795
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.02175337403206
1 3.04607009906597
2 3.74332105481798
3 3.43963239564328
4 2.97288208193014
5 2.87524155914615
6 2.07437348247674
7 2.10505678127629
8 2.41174507857842
9 2.74477586558826
10 2.7926736737889
11 2.88823374189921
12 3.04740970761171
13 3.45283573944006
14 3.88456202236941
15 4.27171593382025
16 4.30567058894628
17 4.24748426615804
18 4.4437505986173
19 4.38791421229809
20 4.23352331349184
21 3.96506650169436
22 3.79794853454722
23 3.50802030907475
24 3.12867808988474
25 3.17991745616714
26 3.21460033181938
27 2.7688824276525
28 2.43525577028572
29 2.41324873683964
30 2.34165422567532
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.0210168663449
1 3.62051125551547
2 4.45013176303405
3 5.59668298475475
4 6.38422361964482
5 6.81884232963447
6 6.75570166712956
7 7.18957650629615
8 7.27104513386159
9 7.19347500304552
10 7.42407465867995
11 7.70979984380219
12 7.86016392069986
13 8.58212921044423
14 9.3237551507659
15 9.67166824623176
16 10.3606365328944
17 10.7899558916245
18 11.6307834160374
19 12.2370611667701
20 12.6821827819901
21 13.1769659776381
22 13.8691371089507
23 14.5180453847413
24 15.2208258314048
25 16.3306707963675
26 16.8706408672606
27 17.1813802534949
28 17.8234254135591
29 18.1918474839657
30 18.8665781182976
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.01631520314882
1 3.09630594803704
2 2.95032496437885
3 2.65843213004107
4 2.01558758545249
5 1.73340826798947
6 1.33987643098888
7 1.5259425156701
8 1.43183267944022
9 2.07807667737358
10 2.34386408428532
11 2.3904749211141
12 2.48996659070073
13 3.25580253846238
14 3.68051551031909
15 4.04171594058281
16 4.12763359624683
17 4.64665135080971
18 4.50056152724019
19 4.46030187715056
20 3.9063587313735
21 3.57045828558874
22 3.13421304214532
23 2.44615958789375
24 1.71845455792181
25 1.05641005120093
26 0.417022169336935
27 -0.218423608536644
28 -1.08421621741178
29 -2.04617876501008
30 -3.21419916133105
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.00873342316332
1 2.91221607797978
2 2.42290662111736
3 1.87618391850517
4 1.49696076750148
5 1.3225332693244
6 1.56172407317852
7 1.83786269738182
8 2.48872075047508
9 2.41542655330928
10 2.66360398399692
11 3.10974660334864
12 3.37449248958583
13 3.62754148336341
14 3.75608643981137
15 4.10397849537811
16 3.74250902523313
17 3.58750138180806
18 3.65572811866297
19 3.55002641636626
20 3.70295135496825
21 3.56704494215748
22 3.52329876572771
23 3.56642286766557
24 3.65176732125551
25 3.61405955100795
26 3.53454751119305
27 3.7032448882207
28 3.89207918299113
29 4.02297734907562
30 4.03896805273629
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.00697547698926
1 3.45528319578583
2 3.88582014234965
3 3.84874206276376
4 3.79602415783301
5 3.51445454646918
6 3.94437434472576
7 3.61947231212523
8 3.47377771792741
9 3.81086838520577
10 4.36219595349566
11 4.79025943010791
12 4.33627632957563
13 5.0147048196344
14 5.04658932279717
15 5.55505296341678
16 5.69300592558084
17 5.71136458656273
18 5.27709434299783
19 4.90132239719256
20 4.75332336634049
21 4.47583474299285
22 4.04916626115305
23 3.77742781721256
24 3.26448630792376
25 3.4680096603005
26 3.31033565953407
27 2.91625517227787
28 2.9368971726046
29 2.64833183244839
30 2.55871745988337
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 2.9957136705374
1 3.23849216552657
2 3.94286038487053
3 4.18487548090199
4 4.35931525015692
5 4.79602123863333
6 5.12840912937009
7 5.50307377472911
8 5.53312216531624
9 6.00803661160482
10 6.46983962760719
11 7.17316078732662
12 7.40163246992681
13 7.72762389572771
14 8.21063400607182
15 8.39862330726802
16 9.14275003981938
17 9.39575052680364
18 9.30974627524332
19 9.40878266102004
20 9.51490790353362
21 9.70781126979447
22 10.0021739513487
23 10.0463473350187
24 10.198060650185
25 10.4584313771044
26 10.8611639812442
27 10.9064690087069
28 11.0377725074323
29 11.2081518714248
30 11.2309542369913
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.02037228138797
1 2.93160523130628
2 3.15580928589382
3 3.16443410156872
4 2.99972684251795
5 2.70790224450458
6 2.0834683204691
7 1.72321309393691
8 1.22342610219275
9 1.36212422464444
10 1.70406581413384
11 1.49213101736875
12 1.38957319546082
13 2.01553312393679
14 2.24262370392876
15 2.94648156163799
16 2.43264375851242
17 2.24883496258407
18 1.89279233344042
19 1.76861430326628
20 1.78604651936482
21 1.33944101621015
22 1.23483158879557
23 1.57705714872655
24 1.05255576850431
25 0.897603614127141
26 0.897176358199378
27 0.844434244712157
28 0.588392965466159
29 0.400894901576708
30 0.399073582209271
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.00167303568522
1 3.24932691970063
2 3.33465426397578
3 3.3549751260787
4 3.05384149367823
5 3.56372512851479
6 3.77805196066088
7 4.15815751219871
8 4.36203782980785
9 4.35487171667579
10 4.60418754359019
11 4.87196831521423
12 5.13803342548612
13 5.14033159882369
14 5.48635675745652
15 5.92961095221169
16 5.76173865712488
17 6.15539603590651
18 6.35091973833701
19 6.28426885836015
20 6.28723131561382
21 6.38838986179609
22 6.47548136026666
23 6.61729179228687
24 6.49562470143835
25 6.52423291159638
26 6.4462343680957
27 6.55332146404228
28 6.17504662541152
29 6.29006594763255
30 6.33440040835034
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 2.99504318524129
1 3.06567626590261
2 3.36308261505364
3 3.53630708094582
4 3.33324906429447
5 3.07397338304552
6 2.77774804575357
7 2.28727925955998
8 1.5740414678706
9 1.33527662500563
10 1.03002368089675
11 1.20394776430451
12 1.12234485511731
13 1.65212631380348
14 2.27765953341026
15 2.8859570524794
16 3.25844000095418
17 3.82659804253545
18 3.64184855121641
19 3.61551315004111
20 3.70393129486094
21 3.67305942015583
22 3.80959980554159
23 3.79971736559709
24 3.82537829678164
25 4.36378908377321
26 4.71460370482813
27 5.04649749635134
28 5.06637919270244
29 5.35423581153093
30 5.82730893746507
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.00891588531358
1 2.41190976967497
2 2.98476694757089
3 3.15300885261074
4 3.21377990237454
5 3.92373401862481
6 3.84209504819631
7 4.33807878756756
8 5.01989523935275
9 4.93909512070715
10 4.77681556821647
11 4.75147514441401
12 4.9956209135531
13 5.45309003724162
14 6.17802283152103
15 7.00201220430785
16 7.43710563615166
17 7.57362482350317
18 7.52453787710489
19 7.55780460089238
20 7.40611403913564
21 7.16910954503055
22 6.79917420638926
23 6.49084627745213
24 6.35957387722534
25 6.29403952674996
26 6.25238219512097
27 6.11127077913035
28 6.14234978277603
29 6.08473532612589
30 5.76293332505715
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.02500130424312
1 3.03886976838017
2 2.82538423787987
3 1.86150450452448
4 1.27462695394855
5 1.32371769363538
6 1.30192804175155
7 1.3841181812996
8 1.20706485215753
9 1.4510148521778
10 1.31991328005626
11 1.10621956157018
12 1.44578816641073
13 1.80418969097303
14 1.8718712180796
15 2.10141637370223
16 2.1064753897474
17 2.58160201146506
18 2.25592265571914
19 2.09073169198812
20 2.11316380563039
21 1.89270395575332
22 1.81185878697447
23 1.83934179759345
24 1.42216426825056
25 1.29522473418605
26 0.970821586346329
27 0.478214056466293
28 -0.44551482268853
29 -0.830492337036186
30 -1.37259525002297
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.00279506592037
1 3.02984220852491
2 3.22480616046362
3 3.20335012064112
4 2.97355463654529
5 3.35038419697106
6 3.61325860659677
7 3.88047784841854
8 4.36206621427776
9 4.40382682866545
10 4.3837951817443
11 4.15025189119371
12 4.21593202146261
13 4.99633907867523
14 5.81756544670287
15 6.5886862835621
16 7.03478305634248
17 7.47457039494377
18 7.50539727816745
19 7.36156575710439
20 7.46283104376903
21 7.33492785325269
22 7.31176230600101
23 7.31528762728856
24 7.2343393017741
25 7.36625591069873
26 7.26299788812106
27 7.18842683978672
28 7.29732318819476
29 7.10825489388795
30 6.62507035591689
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.01380946962269
1 3.4480948815528
2 4.02886380661367
3 4.60883829982544
4 4.76881281279416
5 5.11298976363896
6 5.30477865421935
7 5.92224306207545
8 6.60587096893113
9 6.61928692764323
10 6.78024741844964
11 6.69072110369515
12 6.9394766638952
13 7.29575658382426
14 7.73398355673988
15 8.1860443276048
16 8.20957782235987
17 8.36830962510881
18 8.35740815404291
19 8.09932439561901
20 7.92558972459897
21 7.55028505066101
22 7.39330970384678
23 7.27259858870139
24 7.01870232058594
25 6.80549729049219
26 6.76138588008947
27 6.86819250757279
28 6.57048402016761
29 6.49254845845956
30 6.40263988497457
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.01317233046298
1 2.94154281524364
2 2.8816951339107
3 3.48316954465089
4 3.57853892829804
5 3.71300849484237
6 3.74043149903171
7 3.74300333306517
8 3.96175980671288
9 4.09971938771196
10 4.2718793407399
11 4.78930283603126
12 4.7315244184959
13 5.29380075715903
14 5.65202417489168
15 5.94614388635902
16 5.93678524591887
17 5.970933691537
18 5.91884721212251
19 6.00237089987291
20 6.28350772352651
21 6.4422497935795
22 6.43643113809558
23 6.36266540655547
24 6.29008716275964
25 6.21751839321872
26 6.51953105369941
27 6.34096650748663
28 6.11772474911101
29 5.95370681193321
30 5.71725543320576
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.02035459438763
1 2.818134220548
2 1.97924645662312
3 1.57606316364058
4 0.48148809335791
5 -0.175870117362856
6 -0.309472382102769
7 -0.298768652060324
8 -0.559028746230343
9 -0.852643376135318
10 -0.949733716509711
11 -1.24307923912869
12 -1.43819758101961
13 -1.01710334903876
14 -0.921477130761893
15 -0.609005159992508
16 -1.05782566641011
17 -1.53554416993318
18 -2.11653935555431
19 -2.66651914311497
20 -3.266651802507
21 -3.92063134678204
22 -4.13273192473461
23 -4.68674730013422
24 -5.40734513388464
25 -5.53268376867998
26 -5.82956173148862
27 -6.3232446965789
28 -6.99561976984089
29 -7.43574023852641
30 -7.61706397705488
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.03677183208807
1 3.11653451672968
2 3.46873390370454
3 3.28133301136513
4 3.13028764235724
5 3.86731287953256
6 4.8522195235291
7 5.71741637298921
8 6.14357442595899
9 6.08960970232646
10 6.15754654595206
11 6.16640280881763
12 6.67210755665534
13 7.01080461641735
14 7.03292654736079
15 7.2071982097643
16 7.01091251429826
17 6.93324655047632
18 6.89558833747729
19 6.99420307568161
20 7.01257895619357
21 7.14381216064471
22 7.12422478060886
23 7.11559747524697
24 7.05513914546068
25 6.72698065395672
26 6.52411987956292
27 6.41185853144906
28 6.65353461802964
29 6.66062963183542
30 6.79401121717825
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.0230975383613
1 2.6984116899373
2 2.21901873391463
3 2.17617832469483
4 2.16002827645527
5 2.08694208163587
6 2.1436126573416
7 2.41452096631595
8 2.76110470359965
9 2.64211208621881
10 2.67781092601408
11 2.83514829250592
12 2.51019924292759
13 3.42071342459702
14 3.37625724000155
15 3.68832602454179
16 3.47333300227966
17 3.28235574144942
18 3.07054235750616
19 2.85079040933259
20 2.89518087836292
21 2.9035904607649
22 3.19512180151609
23 3.22936588048973
24 2.98095870133832
25 2.98073850271021
26 3.10909658387849
27 3.1605424232527
28 3.00605045746338
29 2.83546612045569
30 2.52650614165583
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.02986928001549
1 3.01361667563304
2 3.34618665235279
3 3.8077162312095
4 4.1140251070442
5 4.02947062772383
6 4.8682491108018
7 5.4313076633466
8 5.58492463659431
9 5.5957311321481
10 5.56072058080561
11 5.80091767871353
12 6.46609280591671
13 6.3877773712236
14 6.45407892201337
15 6.57715538000531
16 6.49482521409886
17 6.2577921450062
18 6.54460950146628
19 6.46656496519901
20 6.42046928851704
21 6.54273420820351
22 6.75488513667627
23 6.895036291313
24 6.96118123141225
25 6.78176087327263
26 6.41876481689186
27 6.74249426854667
28 6.39813518000482
29 6.34519229196868
30 5.8351179052112
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.00341274974579
1 3.37703509957028
2 3.97305427838669
3 3.86308371758393
4 4.53260382346792
5 5.37209591990926
6 5.8802245155375
7 6.65534755416762
8 7.58152141680228
9 7.2399096221777
10 7.08346512211599
11 6.9222653432142
12 7.16894323137222
13 7.24473018903376
14 7.10119581392568
15 7.36556741199042
16 7.64866305673783
17 7.74161273574343
18 7.92911239339543
19 8.04620813382467
20 7.97534328911283
21 7.81697413827751
22 7.87475418515182
23 7.81557117387847
24 7.45915007874652
25 7.04114694474123
26 6.73221046346375
27 6.48717135234956
28 6.19963098950035
29 5.7279128256808
30 5.30946970529545
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.01803567186767
1 3.47060621305658
2 3.78752532248702
3 4.3066159478049
4 4.28457738266047
5 4.62860463212458
6 4.6880159390877
7 5.06934617345314
8 5.43593715175142
9 5.66761846275418
10 6.45627831106669
11 6.66631066187167
12 7.20404428285451
13 7.69839791249379
14 7.79920413641601
15 8.06752912571186
16 7.91127732196067
17 7.3340214847301
18 7.53597250095554
19 7.67417000736195
20 7.60998915335604
21 7.38547092596321
22 7.66358037641735
23 7.69181289501067
24 7.61298782099207
25 7.88380768387546
26 7.96511008832015
27 8.13360902117244
28 8.27376261170597
29 8.24946595442563
30 8.33452593727765
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.00239185287895
1 3.98925502327143
2 4.21336575926787
3 4.28316715818903
4 4.03979525067058
5 3.77923660146066
6 3.46317752741682
7 3.24590102068171
8 3.25100030951185
9 3.51905389510881
10 3.39826525658455
11 3.44262330037824
12 3.18449629830507
13 3.74011432983187
14 3.88917268930518
15 4.15109430338392
16 4.45368792089081
17 4.56975252934471
18 4.17363514323077
19 3.70357560891817
20 3.29711663462997
21 2.66745631293791
22 2.4263906531591
23 2.38339611419311
24 2.11083897736096
25 2.25363180714408
26 2.22430594671456
27 1.96967020609499
28 1.64601015125636
29 1.39611929766361
30 1.36062826294129
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.02078223308707
1 2.50583509230496
2 1.77473534978849
3 1.74289320490165
4 1.49338445135086
5 1.79844297122311
6 2.39432400823398
7 2.3838065839462
8 2.26173335795248
9 2.47877608306516
10 2.9134019121536
11 3.39587001306567
12 3.56887047205212
13 4.29490670430885
14 4.45469705746941
15 5.19722639384672
16 5.45530372385822
17 5.48363460842539
18 4.8358045041469
19 4.467848365794
20 4.60458060421538
21 4.29450147253846
22 4.04059279592579
23 4.07693140686678
24 3.42860911200251
25 3.49809399650756
26 3.35578272344307
27 3.38986545342611
28 3.18903479682166
29 2.99431315515667
30 2.65245427329755
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.02492103965739
1 3.49181629101497
2 3.72108058941035
3 4.28161775694315
4 4.41958420756812
5 3.89177564034524
6 3.7452575970753
7 3.53395769512351
8 3.388877723074
9 3.37228312005705
10 3.24326092856604
11 3.29125085397982
12 3.71644134154656
13 4.61995801505433
14 5.14596595024332
15 5.71289737369424
16 5.23109978763672
17 5.29427496497788
18 5.77409226167243
19 6.23543946518607
20 6.21370725242778
21 6.28519876388543
22 5.87006846768481
23 5.23236849738045
24 5.28446375770224
25 5.0807997964155
26 4.64020232023036
27 3.90411135726686
28 3.995125593242
29 3.52711319718453
30 3.1534624859677
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.02270863785487
1 3.23769375208154
2 3.53367525311385
3 3.98919698447069
4 4.01656620114411
5 4.17279458281262
6 4.78432712127526
7 5.01254149596244
8 4.67734279479859
9 4.79573086243965
10 4.95551629929096
11 4.95771671265689
12 4.82753026675713
13 4.9048370836252
14 5.2831700556216
15 5.42315725533501
16 5.73807026512413
17 6.05849215974258
18 6.27187960286461
19 6.40198312288459
20 6.54058969715617
21 6.72789329461555
22 7.19538188504364
23 7.56053311323272
24 7.69274347020144
25 7.91680645940122
26 8.29499381560516
27 8.71911383193063
28 8.7453760234377
29 8.98597805616347
30 9.68580133033614
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 2.98943748699303
1 3.44463249558119
2 3.64048976401512
3 3.80899855318498
4 3.75654033254755
5 4.60929144891047
6 5.36151517238922
7 6.14822936511807
8 7.09553843796139
9 7.12909594865057
10 7.04205638517569
11 7.09366439222127
12 7.19507326730601
13 7.74336048195885
14 8.34516213105729
15 8.75438757393164
16 9.14443974736489
17 9.7223610242587
18 9.89020055217608
19 10.1670849616263
20 10.1661922812241
21 10.5185645175056
22 10.7630914990186
23 10.979166517351
24 11.288505301985
25 11.2611042556219
26 11.4091274402423
27 11.9044119443773
28 12.2527395153913
29 12.6638784396352
30 13.0183563424616
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.01223978191559
1 3.23844158139591
2 3.25845353593574
3 2.59916572728257
4 2.251817121532
5 2.90874772735629
6 3.04470889849872
7 3.53019825874508
8 3.99799700803228
9 4.30865882008918
10 4.4677904032029
11 4.67862171155766
12 5.34612429255582
13 5.9570947446365
14 6.29476983773711
15 7.26540593215003
16 7.57952386939339
17 8.06344195346088
18 8.36532743272144
19 8.30728469338627
20 8.29836948427385
21 8.24508165061998
22 8.41441890840447
23 8.17485757093241
24 8.55874990266062
25 8.74660197265554
26 8.80760836657
27 9.01631914559364
28 9.12661363500559
29 9.39733855354173
30 9.48040054361709
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.0217927186132
1 2.93614234103981
2 3.11756243514597
3 3.0303260167464
4 2.71643824136907
5 2.81685847992701
6 3.25212607824768
7 3.59100255412314
8 3.90458809571419
9 4.17860236673191
10 4.56137020118765
11 4.55052031640559
12 3.62068848859185
13 3.65382384605465
14 3.574024373034
15 3.72596347373351
16 3.28617727475126
17 3.13068719544273
18 2.56871921992936
19 2.05590655697604
20 1.32495891018266
21 0.683822177123022
22 0.18219197670508
23 -0.449118896829278
24 -0.893093076238936
25 -1.22057114872157
26 -1.50080812674392
27 -2.31640006477376
28 -3.01913930842568
29 -3.65719377147879
30 -3.76691036743768
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.02316131215125
1 2.66735117397945
2 2.5430166686201
3 2.92539757560328
4 3.0598542945293
5 3.04387816048626
6 3.2444734819886
7 3.478447309038
8 3.82619667750496
9 4.34877519580714
10 4.72522000641552
11 5.00070113697183
12 4.92891256586754
13 5.66186368351634
14 6.11043357726877
15 6.62303206575142
16 6.80610641078063
17 7.33058539612097
18 7.63924618149857
19 7.71520001919089
20 8.26298552890839
21 8.16729384760528
22 8.43178633434666
23 8.68916382871811
24 8.62393459135299
25 8.53148074380781
26 8.91176265960895
27 9.06047619634263
28 8.96236945061236
29 9.08748776212021
30 9.22443529439374
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.00819573580649
1 3.52030112935593
2 3.70111259596853
3 3.88711065064137
4 3.54273895830493
5 3.57040605208932
6 3.39402247090188
7 3.22357514536393
8 3.12239363206406
9 3.1410556900549
10 3.58888432404682
11 3.90705744681331
12 3.72331019013583
13 4.81089422029919
14 5.27390042177408
15 5.93520367054155
16 5.91122106628174
17 5.93203431629255
18 5.55505193103291
19 5.19662579284362
20 4.82581785373241
21 4.54408903341271
22 3.96857019130545
23 3.74911390275676
24 3.22426537347565
25 3.20282131425628
26 3.21727841406648
27 3.18060481067288
28 2.89684194819986
29 2.90022065143391
30 3.21569713057093
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.00850635592396
1 2.95332415459152
2 2.57954500330748
3 2.21935263298145
4 1.04066574568995
5 1.06899368520002
6 1.16062036882182
7 1.56748110006933
8 2.11012677985935
9 2.27446875367224
10 2.31508784487139
11 2.61849854885403
12 3.09855718215201
13 3.76041406321353
14 3.95155469543454
15 3.98216587371206
16 3.48821662913839
17 3.66110896456357
18 3.5447101620725
19 3.76161142823476
20 3.82325605338441
21 4.03220473179725
22 3.69899511992938
23 3.70767862569055
24 3.93079983667685
25 3.00674875189946
26 2.3704956828232
27 2.1702553541739
28 2.35655318904785
29 2.2320534747941
30 1.8600223893622
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.03489069079733
1 2.71719230915695
2 2.28651908120652
3 2.24905732208167
4 2.89438167922857
5 3.07630947976095
6 3.06801447346272
7 3.60064173535993
8 4.36626339856771
9 4.87059242699828
10 5.03091809794321
11 5.62139336164143
12 6.14633714932654
13 7.02063247329786
14 7.42090242366192
15 8.23841591482221
16 8.41844502879487
17 8.60668242281605
18 8.94673598694071
19 8.96092196860858
20 9.53737129766838
21 9.92195392650502
22 10.2902600255484
23 10.7825161692296
24 11.3342864974151
25 11.6396910508169
26 12.2144791170276
27 12.7012329322552
28 12.7220620309251
29 13.4482381298647
30 14.2087582171942
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.01260368133636
1 2.59091010436632
2 2.46632990561185
3 2.50426533480219
4 3.0471551744399
5 3.09845729538987
6 3.01375020762637
7 3.53736718608557
8 4.08282078356876
9 4.25711108885302
10 4.30826375874499
11 4.86004794824341
12 5.36498451563567
13 5.70283120383815
14 6.02852155771242
15 5.99455533325145
16 6.00907317958926
17 6.05143145211603
18 6.51826670804722
19 6.7905177520797
20 6.71531586576732
21 6.8230850740726
22 6.80933311501728
23 6.82058982361253
24 6.87790599479869
25 6.78399992740936
26 6.70938184812646
27 6.89516040135737
28 6.93919014877582
29 7.0977303556578
30 6.9820181627697
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.00627506674401
1 2.75804589877228
2 2.21216430869068
3 2.13983127106945
4 1.46776849727663
5 1.98873746958309
6 2.34482872667799
7 2.28544842124494
8 2.24819773390036
9 2.63509589771811
10 2.75639081709723
11 2.9056965663332
12 2.81601894015823
13 3.24617314576348
14 3.24321481706254
15 3.65620786347295
16 3.59613705549998
17 3.52242080834847
18 3.59955543350901
19 3.33628112964501
20 3.27947650269228
21 3.16957603259067
22 3.08406490465892
23 3.15207256347276
24 2.75563083974478
25 2.41443717444313
26 1.98926594554245
27 1.53882284160881
28 1.3477676090909
29 0.982541792951454
30 0.616450739589363
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.03859886678711
1 3.03942444592922
2 3.59504103271016
3 3.7074290835576
4 3.68670301736537
5 3.72549683000222
6 3.97286888771642
7 4.06578516470207
8 4.01353089784377
9 4.31236998392167
10 4.61060931720744
11 4.95925846990825
12 5.10672066591392
13 6.01720012766647
14 6.85420332753264
15 7.72440023226097
16 8.36107684587956
17 8.7442241675637
18 9.06301349000761
19 9.17007060044165
20 9.32660512839609
21 9.19782571233393
22 8.78009247108191
23 8.57149335711923
24 8.26083935903747
25 8.0127299904536
26 7.56985428322667
27 7.22974322617008
28 6.74489416287039
29 6.40913399062169
30 5.955644358483
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.01135957927677
1 2.64930861356111
2 2.59386993460737
3 3.01723918914469
4 2.90887028066208
5 1.97816933040575
6 1.80317180266758
7 1.97283641881558
8 2.183939256031
9 3.13300328960689
10 3.64788735977118
11 4.25007852212212
12 4.54162262015873
13 4.61489109024161
14 4.47792600617288
15 4.54929140590925
16 4.53982515126241
17 4.73857542938661
18 4.86147103056782
19 5.42313398977464
20 5.46303395403718
21 5.68124756853811
22 5.97255384074117
23 5.93430855527753
24 6.20721541982936
25 6.34843213034192
26 6.57056111256587
27 6.70075943703092
28 6.69551185830958
29 6.85174521654849
30 7.432444322776
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.02306002573555
1 2.51440860151782
2 2.13024675849948
3 2.37966106437358
4 1.60800944374541
5 1.89859981769147
6 2.200466514412
7 2.26480678023993
8 2.38522310786691
9 2.25212891182612
10 2.66837860371673
11 2.82916438995296
12 2.73599509473514
13 2.83924660053965
14 2.41082554743886
15 2.11782659882029
16 1.47401246807483
17 0.802066527949894
18 0.442366021805363
19 0.74067115830819
20 0.450183243800272
21 0.315115370229258
22 0.0699448797428488
23 -0.0948710636234802
24 -0.0546107602139756
25 -0.413941609607163
26 -0.582838400701391
27 -0.984199771530966
28 -1.42482180618023
29 -1.7787652267076
30 -2.00834632793886
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.02639113029334
1 2.74515066121711
2 2.63025637937448
3 2.85374737810012
4 2.56089089486253
5 2.37921126127892
6 2.20880580751718
7 1.69951621377679
8 1.56833888393015
9 1.43793063201703
10 1.15201400960383
11 0.977555232652358
12 1.09700290823294
13 1.69964083997007
14 1.78917912332823
15 1.96312084705985
16 1.65571744049285
17 1.59924595569634
18 1.35684962823636
19 1.53794217337717
20 1.33999698456753
21 1.45888167132567
22 1.30319002879099
23 1.51475906575152
24 1.73830942475159
25 1.78992336460331
26 2.10739018840097
27 2.21393027067475
28 2.34899637198945
29 2.23717243025366
30 2.56027446692564
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.03259497418499
1 3.3205890367307
2 3.22369223996454
3 3.17834328924133
4 2.84260690033354
5 3.84846444848488
6 4.1006137454401
7 4.63765512743322
8 5.00508386489724
9 5.29224594644448
10 5.13396484125022
11 5.24262939882002
12 5.2651134060122
13 5.59311864709305
14 6.02352318609442
15 6.0889316071544
16 6.52382191577752
17 6.64246366640995
18 6.86179081737887
19 6.8348217600986
20 6.76989873092025
21 6.93698074888633
22 6.98846385896763
23 7.08912752087887
24 7.16882324331372
25 7.77804994259322
26 8.02839153214313
27 8.43231281148118
28 8.467671214295
29 8.72448302498812
30 8.97187011825276
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 2.99185322911999
1 2.68929618907427
2 3.00292942956023
3 3.29233172578881
4 3.34995473912379
5 3.5959018133142
6 4.13276189653731
7 4.71049326137472
8 5.07593359722164
9 4.94785527484698
10 5.03709715080736
11 4.88646025109968
12 5.13289105175919
13 5.67201905019971
14 6.05518710023321
15 6.68710957537397
16 6.58150902512464
17 6.84756102646691
18 7.10384132241914
19 7.78914374630171
20 8.22110317680009
21 8.5242785150374
22 8.85359763482247
23 9.45613837718814
24 9.73364704641787
25 9.81676820926562
26 9.97073972414973
27 10.2936300140058
28 10.7659247015322
29 11.0044618541286
30 11.1165719193324
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.03447410055907
1 3.10625110697603
2 3.32820100040868
3 3.59996575710139
4 3.95202117591923
5 3.919788987878
6 3.5275821962485
7 2.9913746805376
8 2.48163052328561
9 2.74513407509042
10 3.08489843702251
11 3.40028672733124
12 3.95724605813064
13 4.54563498394729
14 5.44748113516209
15 6.18420000669792
16 6.86518995333788
17 7.84722151574906
18 8.66147672751049
19 9.38230353666328
20 10.3011099373461
21 11.0996827602178
22 11.9272928616015
23 12.6712926454186
24 13.3877270973633
25 13.8085492617063
26 14.4125131793186
27 14.9652378113743
28 15.5503116361479
29 16.4482821021479
30 17.0862873204517
};
\addplot [line width=0.01pt, color0, mark=*, mark size=2, mark options={solid, draw=black}]
table {%
1 3.31996634253658
2 3.45443899460193
3 3.38784218387077
4 3.01931286439371
5 2.82906626173755
6 3.09427938765557
7 3.60416870184349
8 4.24596487007442
9 4.84338888587772
10 5.27994908427636
11 5.61004074039071
12 5.90268352537916
13 6.05852129333431
14 6.16858387553312
15 6.19509636026208
16 6.21485180933973
17 6.20378189365436
18 6.1468591562609
19 6.14787992255152
20 6.14579317317396
21 6.15283082950704
22 6.15412613868876
23 6.14366281427887
24 6.16587792193215
25 6.18223254289368
26 6.18638821201769
27 6.14794417270148
28 6.14179954980725
29 6.15812095860932
30 6.16746194810668
};
\end{groupplot}

\begin{groupplot}[group style={group size=1 by 3}]
\nextgroupplot[
xshift=-8,
xmin=-1.45, xmax=30.45,
%ymin=-0.0317332990665444, ymax=27.9914686596272,
ymin=-0.85, ymax=5.85,
width=\figurewidth,
height=\figureheight,
xtick={},
xticklabels={},
yticklabels={},
axis y line=right,
tick align=outside,
xtick pos=left,
ytick pos=right,
x grid style={white!69.019607843137251!black},
y grid style={white!69.019607843137251!black}
]
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.94865660015306
1 3.13340699414994
2 2.75015589465113
3 1.94116995773251
4 1.38422671155463
5 0.735312356680259
6 0.544713355423342
7 0.486556857050413
8 0.841628342306892
9 1.51682176522083
10 2.02694412101109
11 2.39487136017482
12 2.49575970677226
13 2.30885446400016
14 2.00165533258343
15 1.65484464328116
16 1.14502993275588
17 0.631058818785574
18 0.102521861197557
19 -0.498124750471931
20 -0.997870505300968
21 -1.4579972503584
22 -1.95377634907935
23 -2.29411477562811
24 -2.78645639676717
25 -3.27071334548282
26 -3.78266653252337
27 -4.32441094054793
28 -4.68268950751212
29 -5.3026795210147
30 -5.92242508103055
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.89333977891547
1 2.5454317736473
2 1.81050745696012
3 1.31226827347551
4 0.249092011347495
5 0.0979803525508345
6 -0.298928238235563
7 -0.434589594351792
8 0.0396118840124853
9 0.656826311185014
10 0.922125203386635
11 1.12063272292336
12 1.23754478900552
13 1.07512112478739
14 0.478115085141681
15 -0.337823271257356
16 -1.27489457415525
17 -2.10807982747194
18 -2.84239198980343
19 -3.54470036651672
20 -4.24809211209862
21 -4.84916868582503
22 -5.38233537863976
23 -6.17479042375027
24 -6.5918026436387
25 -7.35399796558518
26 -8.21700648855946
27 -8.69550997330657
28 -9.01062141877979
29 -9.25742177154214
30 -9.8880664209774
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.86350666776257
1 1.98008596201231
2 1.11409326200674
3 0.249019619961251
4 -0.690213121718964
5 -0.627511890060454
6 -1.10188533221634
7 -0.836718316420837
8 -0.457500335903116
9 -0.595429040244852
10 -0.762632948211687
11 -1.08194690056156
12 -1.32481196040679
13 -1.83321162044772
14 -2.34570789265059
15 -3.09693778148012
16 -3.88353837011262
17 -4.62995903418109
18 -5.25250503540476
19 -6.18655889479952
20 -6.75136706924895
21 -7.26884496800832
22 -7.70173931465806
23 -8.14328597265919
24 -8.62518033557577
25 -9.31322479486567
26 -9.90313016792267
27 -10.2919373658385
28 -10.5954427370764
29 -11.1194580991773
30 -11.6714336784675
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.92091128181682
1 2.97741467483149
2 2.54604626473998
3 1.74980299949688
4 0.639982389463313
5 0.168090772778543
6 -0.0310521579464833
7 0.677225328157498
8 2.11523082092156
9 2.4960750689427
10 3.27230556060312
11 3.328951221148
12 3.33900026355374
13 3.08998178785242
14 2.28398103102697
15 1.29180270113995
16 0.41806891974151
17 -0.455470270758594
18 -1.52107051878783
19 -2.72758448617714
20 -3.48337418901859
21 -4.59264182786715
22 -5.50036360090794
23 -6.26883101524281
24 -7.31027886327231
25 -7.66874855369495
26 -8.29119339076357
27 -9.06678237871808
28 -9.85915259765506
29 -10.5492006247545
30 -10.9760573985717
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.85363625209946
1 2.69566132721944
2 2.04676178745253
3 1.12025475794337
4 0.104774230941228
5 -0.252620833838678
6 -0.573088292637335
7 -0.858058826190412
8 -0.86144060620056
9 -0.611537546007694
10 -0.562678455834606
11 -0.67506686043809
12 -0.935370827956874
13 -1.32156714673004
14 -1.73421774328675
15 -2.19983064249737
16 -3.05113014203507
17 -3.76890839237425
18 -4.19691588621971
19 -4.68108993945575
20 -5.16174797409843
21 -5.49500670059355
22 -5.84991816166933
23 -6.15766075007254
24 -6.51368486622255
25 -7.03832817356339
26 -7.58288186331303
27 -8.00047948673823
28 -8.39541882764302
29 -8.79003626020482
30 -9.38696978963028
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.84342275756613
1 2.61417180799182
2 2.05723949581675
3 1.10262996562699
4 0.441142508566742
5 -0.262082360053158
6 -0.682206162422169
7 -1.05538461204035
8 -1.30437036247729
9 -0.821276832902409
10 -0.47622184998813
11 -0.226256262135873
12 -0.0276777320217025
13 -0.233644406633244
14 -0.694641796053915
15 -1.20695427204738
16 -1.72068110833646
17 -2.39950074087443
18 -2.86274523554652
19 -3.29354810009477
20 -4.0012925313593
21 -4.6180049439883
22 -5.25370103585528
23 -5.9604227225583
24 -6.51982841752381
25 -7.2076961267528
26 -8.20926259917516
27 -9.02205807895692
28 -9.3431535042557
29 -9.86333939451223
30 -10.5538406259605
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.89264238171389
1 2.47412722692272
2 1.71036620100956
3 0.90337932641021
4 -0.0672211497308783
5 -0.392353831440904
6 -0.675561638894887
7 -0.229482108270249
8 0.457017105705486
9 0.169260965966606
10 0.122570303735753
11 -0.12823206011697
12 -0.296790514812059
13 -0.0958438379334119
14 -0.460034414804083
15 -0.766245236659444
16 -1.32987513336919
17 -1.91097517253672
18 -2.30534213661582
19 -2.71970102105513
20 -3.39244947123883
21 -3.85475907683483
22 -4.67966032087879
23 -5.3355871529191
24 -5.93256263376762
25 -6.59481466259876
26 -7.1932325946679
27 -7.78183508249812
28 -8.36774572694372
29 -9.13939147107539
30 -9.70041003440614
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.9513163914709
1 2.72274988922112
2 2.00389710183054
3 0.792986058394375
4 -0.340472899934049
5 -0.74160931839767
6 -1.34303993388978
7 -1.41355164361365
8 -1.07353340012383
9 -1.23090532676507
10 -1.16439716928033
11 -1.54856941359854
12 -1.87942848562654
13 -2.59219942487648
14 -3.20248467765656
15 -3.99015231143206
16 -4.75688958388131
17 -5.54427115612389
18 -5.98215005436854
19 -6.54482036655223
20 -7.18572522627964
21 -7.77937224815338
22 -8.44215003960696
23 -9.24885575791419
24 -9.72530185513031
25 -10.913283596228
26 -12.1643211427708
27 -12.989095428382
28 -13.808293444073
29 -14.5673534210243
30 -15.7265952151585
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.95176853447682
1 2.64274588718599
2 2.13842607738693
3 1.15290468506889
4 0.283565869417744
5 -0.0242431328214572
6 -0.186344651728586
7 0.180293752483069
8 1.05145969227118
9 1.77903818872961
10 2.63656986962264
11 3.00120547644702
12 3.02281894461987
13 3.14788533857924
14 2.86648702917425
15 2.45910314623624
16 1.88192154831423
17 1.50058411764314
18 1.21606709354769
19 0.931072630625218
20 0.487941995182167
21 0.0399663120058928
22 -0.376215686927248
23 -0.874819357428793
24 -1.22508755073348
25 -1.680303150746
26 -2.11733389221621
27 -2.51994853368548
28 -2.69606983888115
29 -3.02327303259412
30 -3.54528436890428
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.8680663360747
1 2.724733522637
2 1.90474760106422
3 1.05810519977182
4 0.0419976022201904
5 0.173041417168436
6 0.00439664015848784
7 0.591696954842423
8 1.31758639489078
9 1.71121421608184
10 1.93364489686902
11 1.89757612483956
12 2.17510085732309
13 1.85527071212471
14 1.49399238818742
15 0.913356900641535
16 0.0536030343127756
17 -0.803155780171769
18 -1.48463242668524
19 -2.06267201560026
20 -2.75649859550141
21 -3.39883767688785
22 -4.0455263229763
23 -4.93613275385462
24 -5.36017215674688
25 -6.08938559552626
26 -6.63291771705269
27 -7.28820832077822
28 -7.82154314416058
29 -8.39768124096141
30 -8.94462456932241
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.93256999742304
1 2.68501615123366
2 2.08427674352374
3 1.26658143261286
4 0.339966561806381
5 -0.115067761990426
6 -0.550105345597125
7 -0.812759740141605
8 -1.03305362074498
9 -0.932084987927952
10 -0.578344685797726
11 -0.652404518289664
12 -0.851938056517879
13 -1.23559421087098
14 -1.83897236918644
15 -2.7221643618778
16 -3.55757718269504
17 -4.44466582030006
18 -5.38128670894151
19 -6.20432280310068
20 -6.84436028368408
21 -7.66343256246316
22 -8.66055284937276
23 -9.72631364106087
24 -10.611274907083
25 -11.4218831808429
26 -12.2939283804292
27 -13.3225074328471
28 -13.7822953324842
29 -14.7330016427176
30 -15.6811756816468
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.95232395376933
1 2.73183440605455
2 1.51729229321915
3 0.184092573679253
4 -0.841630705971776
5 -1.65222018813439
6 -2.06376608705373
7 -2.05095062262062
8 -1.46642818162852
9 -1.16252576876693
10 -0.863231363734105
11 -0.537713579959728
12 -0.363793759381366
13 -0.382911259316028
14 -0.801259813241581
15 -1.25771289825617
16 -1.67381443071632
17 -2.24746333374115
18 -3.06752192452091
19 -3.94557464768755
20 -4.48044540964112
21 -5.1533664241723
22 -5.58766131783561
23 -5.99303864928198
24 -6.72062090851228
25 -6.97636255221926
26 -7.32181086275606
27 -8.06112751731796
28 -8.99394907936726
29 -9.59351923151738
30 -9.87411951195802
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.95634249513366
1 3.04794631774436
2 2.83887438974716
3 1.77344439485022
4 0.878152865708032
5 1.20318548647751
6 1.30463371913165
7 1.82250046606824
8 2.54081950446782
9 3.02656040374064
10 3.53800150416278
11 3.69516863482531
12 3.75206891000765
13 3.70113542774651
14 3.64982071691967
15 3.27786020725649
16 2.96602870528396
17 2.38415719268452
18 1.93942772777336
19 1.21222715547242
20 0.677197102540831
21 0.267465269325902
22 0.0518814017968996
23 -0.190728567696295
24 -0.596178909142091
25 -0.652708185011873
26 -0.886073388077092
27 -1.01261451564482
28 -1.26575061662772
29 -1.35067965932438
30 -1.38435870422806
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.91293394341273
1 2.71052676432243
2 1.88398698026329
3 1.07744783315073
4 0.29644032647742
5 -0.22133318885235
6 -0.608977484730978
7 -0.897174179791056
8 -0.672582489681201
9 -0.108159350739825
10 0.109557374956717
11 0.222744215166472
12 0.542737436665181
13 0.51098083043547
14 0.305460568534194
15 -0.0824182257855348
16 -0.367105065013099
17 -1.04631891024444
18 -1.77287023631955
19 -2.23666207625163
20 -3.16535911772833
21 -3.58950676805944
22 -4.45012286218689
23 -5.26747288778108
24 -5.70060048666036
25 -6.2646628368066
26 -6.87838728622649
27 -7.68846851856715
28 -8.02696403960782
29 -8.69340955918475
30 -9.35024719501972
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.93169742382586
1 2.82076516820814
2 2.40042538239168
3 1.71294375482906
4 0.955255291477592
5 0.468562141860724
6 0.222439716201409
7 0.370422970069159
8 0.978408567754752
9 1.56961057641343
10 2.16915928284252
11 2.53958152453427
12 2.62430575743941
13 2.37594256491132
14 1.88258079486912
15 1.3410777570038
16 0.669948316739045
17 0.247892939066761
18 -0.41678116497428
19 -0.958763513968783
20 -1.51656977250244
21 -2.04582896967887
22 -2.52886538489699
23 -2.99277829841211
24 -3.44441888235192
25 -4.06096990470914
26 -4.72918674656526
27 -5.39859016247937
28 -5.72292389253897
29 -6.32926536693093
30 -7.01293411663359
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.8785650822666
1 2.79695016873421
2 2.30667999127944
3 1.28056429938225
4 0.421589825242002
5 -0.53867730138604
6 -0.969089188187986
7 -1.19643930507345
8 -1.20588826291049
9 -0.906922127297213
10 -0.59957281019015
11 -0.511184428968697
12 -0.489781404708966
13 -0.997141163086157
14 -1.78048806051785
15 -2.95275493505453
16 -4.09766115237637
17 -4.90608766869123
18 -5.77232927665532
19 -6.49933521356712
20 -7.58760736908349
21 -8.2198419012486
22 -8.74530992096287
23 -9.43174299234156
24 -9.92011689255731
25 -10.6590974337849
26 -11.2990105335324
27 -11.5413874114551
28 -11.8972924833706
29 -12.205820004128
30 -12.581588175648
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.82770567261282
1 2.49007440548868
2 1.72814122410988
3 0.839911624461424
4 -0.17163364716432
5 -0.40647221658574
6 -0.598699138073489
7 -1.02177912578992
8 -1.19805347469959
9 -0.909005534189504
10 -0.667223128548923
11 -0.701115331425532
12 -0.855854381715424
13 -1.3095625202391
14 -1.71453675723634
15 -2.22132248655996
16 -2.8277530603928
17 -3.60277047146569
18 -4.09209657770435
19 -4.61757805817349
20 -5.51499063458087
21 -6.05156224468817
22 -6.44788347907947
23 -7.13834116012976
24 -7.65484801907958
25 -7.9439097840368
26 -8.36374665497975
27 -9.05645168540312
28 -9.40212296713305
29 -10.0538382265182
30 -10.6248457756975
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.91578662539728
1 2.84533561429581
2 1.97457266491105
3 0.937605205665458
4 0.0746237288931955
5 -0.465957093000384
6 -1.04318723140592
7 -0.895085227607176
8 -0.459753017525006
9 0.400089628249413
10 1.19364885794636
11 1.88193016880061
12 2.3576644239733
13 2.26148955151588
14 1.5357094241851
15 0.912076092601191
16 0.346622601952301
17 -0.269220119371079
18 -0.798557133910803
19 -1.46847908322349
20 -1.94192149139083
21 -2.48065869457688
22 -3.02059364980393
23 -3.65219157112708
24 -4.26695255677657
25 -4.8863667474678
26 -5.60697174583446
27 -6.01588960030401
28 -6.46258491025432
29 -6.9855946549132
30 -7.5293211113677
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.88896846480343
1 2.64399110096993
2 2.23951912695676
3 1.6243228225626
4 0.442554991793111
5 0.486640392484562
6 0.224425473315767
7 0.65229606121747
8 0.948195948668271
9 1.3707107477329
10 1.814818562235
11 2.01468859973024
12 1.75227238396652
13 1.45716753590424
14 1.07979832737104
15 0.402051827400216
16 -0.222591830731002
17 -1.08568402218425
18 -1.95760950285731
19 -2.82026330789445
20 -3.57789388692407
21 -4.47894078072418
22 -5.39925748090955
23 -6.1074973933106
24 -7.01686231400959
25 -7.75463416599301
26 -8.34007629939281
27 -9.00836251874755
28 -9.58846202286399
29 -10.244806479499
30 -10.9134310391477
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.92483033215397
1 2.33833796845437
2 1.40326563770052
3 0.360813157232492
4 -0.789954069488997
5 -0.988342093653349
6 -1.15170100307027
7 -1.24484186239144
8 -1.06948387363284
9 -0.554496584135654
10 -0.134820117833238
11 -0.14546161254939
12 -0.271549063636952
13 -0.605091148777747
14 -1.36368118413787
15 -1.94650087887887
16 -2.62244819288118
17 -3.25678205199387
18 -3.93151201866405
19 -4.45288695149405
20 -5.13991380595003
21 -5.49067176382722
22 -6.15245355810925
23 -6.90388857506511
24 -7.42846903064488
25 -8.16037979566961
26 -8.85949850229099
27 -9.33759456957364
28 -9.71777273235869
29 -10.1044495617088
30 -10.6236529491052
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.8738580065262
1 2.71945914688571
2 2.13069208514136
3 0.946485413422796
4 0.159099822577513
5 0.00891489677327684
6 -0.220016903731862
7 -0.225910608511148
8 0.164245750023026
9 0.539554602948169
10 0.633704753287462
11 0.902766733084865
12 1.22823990662864
13 1.07933590712664
14 1.02510550316433
15 0.537446449090245
16 0.0399140469890806
17 -0.488509787987546
18 -1.10019300018466
19 -1.72675777789475
20 -2.3526200249988
21 -2.62381878624228
22 -3.20280528714603
23 -3.54001925800971
24 -3.62136658147659
25 -3.83554034250497
26 -3.87943436968645
27 -3.90411965236135
28 -3.63624283512051
29 -3.75130461989948
30 -3.85806131161143
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.90156637089577
1 2.78871310539072
2 2.38530905227871
3 1.65133949708385
4 1.09290665570493
5 0.6630517193886
6 0.514001290818637
7 0.876182375573636
8 1.53279736770212
9 1.6171106714427
10 1.34733841388383
11 1.33683504968727
12 1.28948226900401
13 0.755187682000086
14 0.280467961134558
15 -0.440511454464646
16 -0.82790224174745
17 -1.40633701635703
18 -1.91742466255604
19 -2.26064968010633
20 -2.85860237344608
21 -3.39552566159007
22 -3.95472927548823
23 -4.8476196761826
24 -5.27353113220873
25 -6.13575278844616
26 -7.12735488712483
27 -7.90179980794524
28 -8.2441526399272
29 -8.93564809797535
30 -9.71860928367098
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.86223688083839
1 2.3877090850113
2 1.77794501910252
3 0.665710094243318
4 -0.491206310533522
5 -0.916394388024361
6 -1.24493430525402
7 -1.16454527470096
8 -0.507933457496927
9 -0.496801693596909
10 -0.384077491296312
11 -0.452223054643918
12 -0.555911542913268
13 -1.3294218505363
14 -2.18803088905408
15 -3.38333733886986
16 -4.36276039384707
17 -5.3059141249682
18 -6.0207654322611
19 -6.54551550209424
20 -7.36416632893268
21 -8.11649043279795
22 -9.13719158989989
23 -10.208322452615
24 -10.9493358807805
25 -11.7321062620827
26 -12.6154381974025
27 -13.2787901242706
28 -13.6928199347696
29 -14.1607322908555
30 -14.5733248057953
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.96447636620339
1 2.45111136039297
2 2.04894845424222
3 1.21630812786569
4 0.545761861408826
5 0.0553046636239394
6 -0.533082607823147
7 -1.10012559264048
8 -1.2387452242544
9 -0.840396126013875
10 -0.447328067973318
11 -0.539699064108566
12 -0.892025639119522
13 -1.18198691710687
14 -1.84096974306897
15 -2.37869286817656
16 -3.13718012390203
17 -3.72125396935986
18 -4.4331226669693
19 -5.08361776502581
20 -6.1123345917017
21 -6.82977900914063
22 -7.68989006803041
23 -8.59958678047077
24 -9.07711892240389
25 -10.0632397995958
26 -10.9094522776483
27 -11.7050071497015
28 -12.28993016566
29 -12.8167929443639
30 -13.3907891131628
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.82236490977647
1 2.71038028187188
2 2.15805459881499
3 1.22669861578948
4 0.228563242652577
5 -0.411159999716078
6 -0.608184754290003
7 -0.786960402402332
8 -0.495203466935742
9 -0.0867753177903872
10 0.571649582897395
11 0.986859873852413
12 1.27653638900675
13 1.03742918048375
14 0.571238294787355
15 -0.26526037438803
16 -0.672397516483681
17 -1.42708085040969
18 -2.24883584311336
19 -2.9492584967607
20 -3.62277843817589
21 -4.19024200833952
22 -4.79937486224909
23 -5.20983785332992
24 -5.76394037085739
25 -6.02333451812444
26 -6.41829495417155
27 -7.00277686838688
28 -7.69693871726016
29 -8.27976566705983
30 -8.62196735279679
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.87372173736535
1 2.77132385668489
2 2.4196199517861
3 1.92893500637746
4 1.01300583098564
5 0.255391006294049
6 0.111171417791725
7 0.277710259126209
8 0.842979351916842
9 1.3004162526662
10 1.59448526064818
11 1.77885889342286
12 1.9390573319351
13 1.3650056021202
14 1.07138355125854
15 0.439686497353978
16 -0.0632250164596169
17 -0.737593559847401
18 -1.37575900889269
19 -1.85489082424204
20 -2.65660834391595
21 -3.47759308956983
22 -4.19851710993386
23 -4.70623580964567
24 -5.24111782387758
25 -5.6473863598143
26 -6.0685990018817
27 -6.75136292566993
28 -7.1865585377185
29 -7.75356889656682
30 -8.17749380602874
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.87411049302458
1 2.84166492787831
2 2.50968426982028
3 1.57885973623512
4 0.641377015712861
5 0.451544586308428
6 0.148001933274791
7 0.135312594310189
8 0.50954253846866
9 1.19313364805118
10 1.6133795296788
11 1.95828361082956
12 1.9342221732492
13 1.98177750319447
14 1.87757357947965
15 1.43995096246821
16 0.94035224755822
17 0.482713588385218
18 -0.309168631656597
19 -1.21960631796454
20 -2.34546919098015
21 -3.02363672410408
22 -3.92412852009477
23 -4.78580502304921
24 -5.78652452998617
25 -6.72355641941711
26 -7.70002200287006
27 -8.62121205226805
28 -9.40845637789718
29 -10.271901626475
30 -10.7956032665568
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.93196467599767
1 2.8089336497358
2 2.33491421971435
3 1.57182858428715
4 0.716922490535678
5 0.493483199383592
6 0.119551182955576
7 0.0726619512734263
8 0.454924270744183
9 0.687316417502279
10 0.903010251339618
11 0.948951902856829
12 0.861806543325615
13 0.139620072485707
14 -0.482198507603737
15 -1.40554172058918
16 -1.98250922928575
17 -2.7164499985611
18 -3.25553305918301
19 -4.01580247003879
20 -4.87931802726561
21 -5.60643338395607
22 -6.16056190568992
23 -6.73079707780534
24 -7.37050169321392
25 -8.11068689752602
26 -8.60313110245316
27 -9.12023182509429
28 -9.65864852171079
29 -10.1686321428424
30 -10.6904873751145
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.94601403814608
1 2.92262937130842
2 2.63544891627446
3 1.59684769205743
4 0.933827164799
5 0.697853805674209
6 0.563550687505442
7 0.817293784464383
8 1.48249103906249
9 1.56057933808134
10 1.80949853587133
11 1.7911150497149
12 2.11785790103737
13 1.81620525633678
14 1.28873941850068
15 0.137753105825649
16 -0.412925751191635
17 -1.2428801856012
18 -1.57039506159051
19 -1.95938243786595
20 -2.38557542706767
21 -2.56125123638942
22 -2.94532944106598
23 -3.43130518347976
24 -3.79520657335511
25 -4.63188094767717
26 -5.1394918735731
27 -5.66505500162254
28 -6.42058076101742
29 -7.09829865033797
30 -7.5924181187831
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.91150587743547
1 2.5379529878683
2 2.03552092853444
3 1.04373207278751
4 0.03393224505351
5 -0.190443389825747
6 -0.679803152984224
7 -0.432916022711465
8 -0.121226972966156
9 0.0256169424296875
10 0.384821337282048
11 0.409641430310348
12 0.507976153758166
13 0.414067133076164
14 0.230174802456602
15 -0.184459785407464
16 -0.702444185786518
17 -1.38218352427367
18 -1.92719092712119
19 -2.75339512988443
20 -3.1426813512874
21 -3.64014721260555
22 -4.29096184155301
23 -4.65520339658203
24 -5.12073190070055
25 -5.64867382852761
26 -6.10917331805961
27 -6.44221196225713
28 -6.85312513388861
29 -7.23710343820854
30 -7.58387031265695
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.88692618423149
1 2.67188681679674
2 1.9619060226374
3 1.13314793087933
4 0.0374253973861176
5 -0.555147464515951
6 -0.9951889648428
7 -1.17545322751642
8 -0.88448590303622
9 -0.449799519475764
10 0.0501335033243802
11 0.135030303734307
12 0.109859831894488
13 -0.480853884368184
14 -1.06335109624677
15 -1.97810244469762
16 -2.85090858158572
17 -3.62901487902647
18 -4.51793529003346
19 -5.4477257560791
20 -6.51068292929481
21 -7.45756485818456
22 -8.49108107721244
23 -9.62041327939252
24 -10.311918707775
25 -11.3635421586301
26 -12.5715265024723
27 -13.479884648124
28 -13.9945091167278
29 -14.6381146242347
30 -15.3491768343471
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.89584830620703
1 2.67445264231202
2 1.96094600631401
3 0.888905757156994
4 -0.345918661892602
5 -0.903170581575051
6 -1.12391617047488
7 -0.658970243303854
8 0.270101055511848
9 1.31135284857207
10 1.91767363714424
11 2.52378402062715
12 2.77202039941802
13 2.57442820981385
14 2.27862001327424
15 1.53276713137174
16 1.21512857846237
17 0.67359136584149
18 -0.225734775061159
19 -0.939215602628467
20 -1.58913750236998
21 -2.21431648666798
22 -2.96185388597934
23 -3.71852787892503
24 -4.68227665103029
25 -5.56436912513964
26 -6.43337957256639
27 -7.07548998375542
28 -7.5288416422168
29 -8.05100831627442
30 -8.59462347343706
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.82298086074529
1 2.87579756203565
2 2.21088160667229
3 0.951089084312983
4 -0.263829898517384
5 -0.803331034146719
6 -0.904631312291555
7 -0.788124691563899
8 -0.299728640896648
9 0.37368897403201
10 0.861696417741062
11 1.60325864366533
12 2.04422395774588
13 1.85012976806017
14 1.18962750228063
15 0.551011264885684
16 -0.39188484042362
17 -1.4745384150592
18 -2.29642417820565
19 -3.12351823307407
20 -3.96792747894203
21 -4.69719755779065
22 -5.2291950375203
23 -5.74327224372591
24 -6.24602929878994
25 -6.67824649179526
26 -7.09450791524906
27 -7.61127150525499
28 -8.0341510742135
29 -8.49798263524868
30 -8.81771218405762
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.93698571552425
1 2.89325891396854
2 2.18787550239799
3 1.34290601206005
4 0.397394121740351
5 -0.299996374803163
6 -0.87930913876168
7 -1.34314897714862
8 -1.40491324549392
9 -1.27111063239155
10 -1.06179484928519
11 -1.10443004514923
12 -1.21904634485713
13 -1.76702572922637
14 -2.08338048627802
15 -2.71517939979141
16 -2.86102424785959
17 -3.09359747804085
18 -3.50037918218279
19 -4.1887408212058
20 -4.83598574009752
21 -5.23867210988808
22 -5.74948390411429
23 -6.47697873478286
24 -7.0505817518021
25 -7.47694627931992
26 -8.00120867773429
27 -8.80791150061865
28 -9.41046021960254
29 -10.0554945940819
30 -10.7714354573719
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.85482921694894
1 2.70717454938433
2 1.86557251769501
3 1.05518605772084
4 0.317549051849719
5 -0.119516381514336
6 -0.372396987144446
7 -0.343071386283894
8 -0.0870742498268573
9 -0.224796263229617
10 -0.079287992012981
11 -0.251879481169045
12 -0.41442327317308
13 -1.03232172713544
14 -1.67920862228883
15 -2.52267443972119
16 -3.31632158299512
17 -3.90491058624262
18 -4.37963713610168
19 -4.94205541064909
20 -5.30746757438379
21 -5.72821300989507
22 -6.29706377589037
23 -6.69208916558833
24 -7.26391112968214
25 -7.83268128331524
26 -8.16422880262286
27 -8.53534533127772
28 -8.76232502370095
29 -9.37848669008079
30 -9.829814441856
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.89532822632121
1 2.39819801887894
2 1.71951034552563
3 0.607942829805909
4 -0.369035969371287
5 -0.328660095225723
6 -0.469914413082737
7 -0.115575350374735
8 0.6728015555017
9 0.577371750745243
10 0.463179598646429
11 0.108311333587706
12 -0.127954651159516
13 -0.382333557485614
14 -0.84884157703353
15 -1.34273709080907
16 -2.12654982629904
17 -2.91468393247945
18 -3.84685944399635
19 -4.61531575162753
20 -5.5825650599581
21 -6.45623942504661
22 -7.58097299268208
23 -8.55443499120066
24 -9.37272744983665
25 -10.1314257702629
26 -10.7256707326853
27 -11.1518425266193
28 -11.2909601255115
29 -11.6261429612762
30 -12.0222531474764
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.89667883407585
1 2.30764748983242
2 1.62664568053073
3 1.01062131476784
4 0.369500764428571
5 -0.257152202151763
6 -0.633910181275635
7 -0.64686446464048
8 -0.709366297522832
9 -0.26190743697439
10 -0.00317551637496294
11 0.0555889190319974
12 0.422133306571592
13 0.0522704108394247
14 -0.508504486479268
15 -1.15761598740255
16 -1.83605568565966
17 -2.36465060905008
18 -2.64635521023096
19 -2.9658964118937
20 -3.27594363273038
21 -3.60796834487008
22 -4.00562813424464
23 -4.19138518338039
24 -4.50946190553608
25 -4.82413840945472
26 -5.13510172668338
27 -5.41653419918971
28 -5.67186542859103
29 -6.13244724215739
30 -6.62606561850232
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.92591827919226
1 2.68748288257195
2 2.22416827715267
3 1.18845630817802
4 0.077662387228786
5 0.0702976435757776
6 -0.0806594793145941
7 0.331083173969523
8 0.907510955795573
9 1.59699655755303
10 2.20323564665863
11 2.43627778887467
12 2.33068751220348
13 2.26939284945263
14 1.92082721796189
15 1.35131771015342
16 0.14591732712069
17 -0.525655061592651
18 -1.67128656075758
19 -2.48326895229278
20 -3.30917385488095
21 -4.22423034136396
22 -5.24464521690228
23 -5.98263389852529
24 -6.89675247425119
25 -7.44475129750711
26 -8.16375182569699
27 -8.91503231161704
28 -9.64119043878284
29 -10.3523842785595
30 -11.077652552434
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.9791804592039
1 2.89598958865985
2 2.32242744158406
3 1.73129169872696
4 0.624875419360963
5 0.522483923240099
6 0.0742435416746048
7 0.316070768172045
8 0.603874684074844
9 0.896719722386429
10 1.42029318709458
11 1.40612877144837
12 1.31851209154918
13 1.07765413629224
14 0.74215209052211
15 -0.149421289138331
16 -0.675898870330261
17 -1.39007099798667
18 -1.78286780644248
19 -2.09677096208028
20 -2.50791536287831
21 -2.78775645625487
22 -3.28680220808232
23 -3.68215843168614
24 -4.16357740522381
25 -4.67516895021761
26 -5.25825504754178
27 -5.70640432000609
28 -6.04523826928828
29 -6.53509394131238
30 -7.02722770477611
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.89579030602678
1 2.77839163024206
2 2.15537586365432
3 1.23148461390334
4 0.228786273694052
5 -0.292112958556949
6 -0.600319015059746
7 -0.575789794265262
8 0.10873172646957
9 0.530432438204146
10 0.939103203939705
11 0.880196138811495
12 0.562397457121936
13 -0.0868551252627121
14 -0.692849650003112
15 -1.610917799286
16 -2.48116247149974
17 -3.3743314001557
18 -3.88557280943429
19 -4.31823081939361
20 -4.82380503378823
21 -5.34363564018318
22 -6.03162361584091
23 -6.71282399622968
24 -7.07039762614443
25 -7.59260647929995
26 -8.11619748696724
27 -8.77080423116925
28 -9.06549390863658
29 -9.50929386461083
30 -10.0626323257879
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.84320385701053
1 2.48127177274629
2 1.83019113801543
3 0.775315126707577
4 -0.539851659271754
5 -1.24576252007384
6 -1.91133660653741
7 -2.21973784992314
8 -2.02712650875163
9 -2.04587152445555
10 -2.17392602012675
11 -2.35329703611144
12 -2.52871801777424
13 -2.91833134839779
14 -3.37458913770572
15 -4.00956165095799
16 -4.68682908210349
17 -5.11644245440227
18 -5.87748964965535
19 -6.35622950227753
20 -6.869141963163
21 -7.38877077230725
22 -7.95475696854859
23 -8.52520359034564
24 -8.86250679129535
25 -9.77111418177811
26 -10.75377601155
27 -11.3927184727797
28 -12.0253391032769
29 -12.7537658991924
30 -13.6556414851565
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.92937339574384
1 2.26748313573918
2 1.43016661944541
3 0.382340858512567
4 -0.86129530349463
5 -1.33420688936452
6 -1.97554206408677
7 -2.17815412742841
8 -1.9137906441461
9 -1.60861031823718
10 -1.28258588689592
11 -1.07271854308232
12 -1.28022371096041
13 -1.69211038002305
14 -2.16724595152951
15 -2.84662381616203
16 -3.64913318236227
17 -4.21855408130387
18 -5.02883098415059
19 -6.00446421954074
20 -6.87324516301835
21 -7.73801942858837
22 -8.28529857108666
23 -8.98262210026351
24 -9.75434981945866
25 -10.5752011796959
26 -11.4015907561598
27 -12.3956641513159
28 -13.3002640069908
29 -14.2392189015295
30 -15.1688314614336
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.95644491136429
1 2.40073102124255
2 1.42578182065094
3 0.0873086935090992
4 -0.949705641000163
5 -1.87091003467269
6 -2.39910883129235
7 -2.59607899832059
8 -2.4342727566664
9 -1.96336465959823
10 -1.50681330282132
11 -1.51178703515928
12 -1.87126414355523
13 -2.2153425509988
14 -2.86568942849966
15 -3.60909841982899
16 -4.41875554827238
17 -5.08578753632753
18 -5.54255136952918
19 -6.0628716403549
20 -6.57882883763897
21 -7.11815353853025
22 -7.65526043237935
23 -8.21643964864273
24 -8.71002598740758
25 -9.20790175507805
26 -9.54513633160083
27 -10.071279124556
28 -10.8072003571156
29 -11.4348662992817
30 -11.8590997814835
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.86407134922837
1 2.70851645363252
2 1.91347036891226
3 0.818903547885611
4 -0.568136658599656
5 -1.13148199785413
6 -1.52302990812547
7 -1.53697628268282
8 -1.58674741486234
9 -1.14189513350424
10 -0.587032916533362
11 -0.141600319072026
12 -0.0761927423885158
13 -0.44592568390647
14 -1.02943630293665
15 -1.41011313726938
16 -2.24956324312702
17 -3.36175432331642
18 -4.62216316200411
19 -6.05687320188819
20 -7.14391187563921
21 -8.11649113950968
22 -9.0548910983877
23 -10.0200590022994
24 -10.6391651221055
25 -11.5043595664555
26 -12.2996169459682
27 -13.1053155818297
28 -13.5701483978403
29 -14.0933829796112
30 -14.9023764902992
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.8707115324091
1 2.44364672718236
2 1.80167028583198
3 0.770769154572806
4 -0.224391613793397
5 0.115538237901646
6 0.073286097262379
7 0.443278004012862
8 1.23210116776498
9 1.122193285582
10 1.02338573164274
11 1.0819797971394
12 1.01809275856849
13 0.58930843284363
14 0.113796536252268
15 -0.489848523453288
16 -1.06816029757585
17 -1.70302616411899
18 -2.58645996687928
19 -3.36140225750254
20 -3.90516916596362
21 -4.7254679135097
22 -5.24271576889543
23 -5.83791721943349
24 -6.66053225666444
25 -7.13352091225676
26 -7.61124892486059
27 -8.08769348480079
28 -8.85358888963269
29 -9.40736980180257
30 -9.89617434317996
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.85494954067507
1 2.63961395771456
2 2.0376989830074
3 1.48396026054396
4 0.884358287704648
5 0.217361931506758
6 -0.118941632789438
7 -0.427811474143809
8 -0.527712637324351
9 -0.773356628502054
10 -0.782848130745876
11 -1.0728707950331
12 -1.38771630659718
13 -2.27129537531429
14 -2.96928691407257
15 -3.69687514549332
16 -4.32635080214699
17 -5.02632429372997
18 -5.74788818481433
19 -6.5987961823927
20 -7.07709426002339
21 -7.64178389629236
22 -8.20620979731542
23 -8.64271876528555
24 -9.18280729234134
25 -9.83639390432333
26 -10.3402576771352
27 -10.8203966316633
28 -11.2145114133363
29 -11.7289684789519
30 -12.183720849359
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.92748781501263
1 2.20770054340256
2 1.59789858555941
3 0.654792438887668
4 -0.237564052681281
5 -0.54570697725665
6 -0.634261858558565
7 -0.726900666517801
8 -0.62104396812949
9 -0.138213086136783
10 0.288096348608917
11 0.877970232304577
12 1.31725619206845
13 1.3912824448001
14 1.46324594542753
15 0.802636638512674
16 0.164109971949831
17 -0.369045255977982
18 -1.3821841571594
19 -2.2320187907899
20 -3.16540451492673
21 -4.1633786872835
22 -5.03961121146677
23 -5.82062347199301
24 -6.73702887256595
25 -7.45891653893247
26 -8.30309870401157
27 -8.97019371766067
28 -9.6030471697441
29 -10.1690507771208
30 -10.8917894760435
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.84217475435245
1 2.76982475768673
2 2.30446251953867
3 1.33454936339686
4 0.164461603292189
5 -0.491096422594035
6 -0.893436129192072
7 -0.907161091526211
8 -0.686452206820633
9 -0.0972566247897841
10 0.281726457384956
11 0.71156883597833
12 0.82557841771678
13 0.442977223116134
14 -0.547532813970866
15 -1.34131118461875
16 -1.9815827555743
17 -3.1348639091548
18 -3.96598010873171
19 -4.75738768932547
20 -5.21812414130141
21 -6.02785694142943
22 -6.50024652907758
23 -6.95049860205596
24 -7.71912484851444
25 -8.00262150028692
26 -8.33563911660141
27 -8.75633235179932
28 -9.47868191645714
29 -10.0223449327225
30 -10.3467689663129
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.85489672036004
1 2.73652263531578
2 2.25603107894719
3 1.23566468297195
4 0.305820064724831
5 0.122413881214145
6 0.0678841766774614
7 0.582386804155457
8 1.28986999912471
9 1.69063994060089
10 1.98201036447207
11 2.21374906502847
12 2.53906237934167
13 2.3899896334305
14 2.12653465115067
15 1.49669334129832
16 0.952876131382475
17 0.469881970176413
18 -0.126888759546391
19 -0.732675194907651
20 -1.15276971828336
21 -1.67953102594482
22 -2.10806742788009
23 -2.58999821638561
24 -3.04409210222729
25 -3.36174054772516
26 -3.71854297984309
27 -4.32735049221903
28 -4.92384462555325
29 -5.49052940692642
30 -5.84702905670285
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.88936560835425
1 2.79430044188761
2 2.70039511131769
3 2.18821738666513
4 1.65553215264235
5 1.75601868395726
6 1.96899765241064
7 2.46843285965707
8 3.00556111596662
9 2.871452157255
10 2.88813109372186
11 2.78411358697836
12 2.84516624769496
13 2.57446080803145
14 2.37874722286191
15 2.0475720130177
16 1.62526826534135
17 0.973670438150149
18 0.54541200538921
19 0.0749207376018095
20 -0.630925909220972
21 -1.39784813747946
22 -2.05311623322902
23 -2.59269840421321
24 -3.27994662975641
25 -3.62595457451573
26 -4.23769528678414
27 -4.87713533236676
28 -5.68263577745156
29 -6.38632805939384
30 -7.13981369565389
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.93383430159628
1 2.75860244379275
2 1.92121050362222
3 0.734339336562217
4 -0.623449534853069
5 -1.27480176049624
6 -1.55040269483529
7 -1.49690850336206
8 -1.03405847477615
9 -0.422521115432618
10 -0.120055546143
11 0.179493026775184
12 0.178757917875753
13 -0.115783241576885
14 -0.59509129037651
15 -1.3437542252066
16 -1.97969335256236
17 -2.78802724841377
18 -3.47237306849868
19 -4.09366634031314
20 -4.71075493923521
21 -5.34450847987966
22 -6.14403137876661
23 -6.79055393688877
24 -7.40831867876232
25 -7.87194754045101
26 -8.38417439229596
27 -8.87669774470171
28 -9.27252081575339
29 -9.61202232986079
30 -9.905617222387
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.89341456219764
1 2.71792296704089
2 1.97528393505521
3 1.18559600093606
4 0.126765307944739
5 -0.0114974996004147
6 -0.561767788035537
7 -0.517522127150624
8 -0.136924737574414
9 0.240398177091187
10 0.637104354244526
11 0.756413703264892
12 0.563790011615467
13 0.39428121187885
14 -0.0118914454643679
15 -0.764932209096042
16 -1.47022632962515
17 -2.1693621099649
18 -3.27861228242064
19 -4.27141273643752
20 -5.00530136704334
21 -5.94203059927737
22 -6.82957651433568
23 -7.56020239910437
24 -8.74732543231028
25 -9.29524804669865
26 -9.825126068269
27 -10.535692517815
28 -11.5569240765866
29 -12.4129647459339
30 -13.0533567771527
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.90463904300646
1 2.63216181613502
2 2.2334785362466
3 1.44067404948243
4 0.954213910975067
5 0.268423077259767
6 -0.443747984406642
7 -0.84590183784014
8 -1.034117188434
9 -0.653560249151255
10 -0.334424805941049
11 -0.459771634196589
12 -0.545538632682728
13 -0.834984972938551
14 -0.942872703952329
15 -1.45883760018217
16 -2.08954054507553
17 -2.80691132226345
18 -3.45051943232819
19 -4.13219620867357
20 -4.52305028277036
21 -4.95932325089213
22 -5.55318407285504
23 -6.14169343259176
24 -6.5678648596184
25 -7.07566626115642
26 -7.48597941629886
27 -7.99335760994033
28 -8.41251666096312
29 -8.85761518188477
30 -9.35717565742489
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.90397278966207
1 2.79530803788925
2 2.3195034190932
3 1.11245101590759
4 0.306714838546226
5 0.447884960810413
6 0.185683604086925
7 -0.00285414055570499
8 0.0915332643392333
9 -0.718344700916507
10 -0.977798754394716
11 -1.71005072224477
12 -2.42677827953595
13 -2.9439136417274
14 -3.99046870371733
15 -4.66318483363221
16 -5.53361950440559
17 -6.41633352348271
18 -6.81477845337404
19 -7.3278087392868
20 -7.83551684747993
21 -8.26973647702126
22 -8.76788231888973
23 -9.12544830111365
24 -9.49691002856054
25 -10.252837024019
26 -10.8521872631205
27 -11.1759027662349
28 -11.8647670065771
29 -12.2186328723949
30 -12.5938786908415
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.82960457085602
1 2.49408746812809
2 2.15895344137492
3 1.74432339047484
4 1.30842473820471
5 1.03330065033967
6 0.988511673071844
7 1.27170402429057
8 2.07192396629817
9 2.71414006015494
10 3.47598675690514
11 3.60114008566558
12 3.67126852971291
13 3.42184510872203
14 3.18618971817047
15 2.47996446280879
16 1.88116504844261
17 1.35164002875724
18 0.889611247508157
19 0.271581133270699
20 -0.305096384139596
21 -0.87115509092224
22 -1.42495908888035
23 -2.05994833809783
24 -2.69302737307555
25 -3.51547055031162
26 -4.23594974392061
27 -5.04665224474211
28 -5.65083611151806
29 -6.39107209275501
30 -7.13076572560418
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.96651051399606
1 2.61098682758631
2 2.02818169402592
3 1.2943335642757
4 0.311484162278729
5 -0.278729239664456
6 -0.720361061016616
7 -1.0807619292652
8 -1.21543207850764
9 -1.17440809166267
10 -0.876924503059282
11 -0.910293639857366
12 -1.39744980244383
13 -1.96399512659593
14 -2.79022807250705
15 -3.6174403994351
16 -4.42539161552351
17 -5.3290558457015
18 -6.3123738793018
19 -7.34263247527863
20 -8.01434851846692
21 -8.90329106413821
22 -9.62309682459507
23 -10.4354640804057
24 -11.2927237804257
25 -11.9674528549781
26 -12.6308507641773
27 -13.3716457116297
28 -13.9845572411846
29 -14.7107796385597
30 -15.5064728072502
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.92323005372852
1 2.8385865732959
2 2.43775324084132
3 1.55084169997451
4 0.349043762891833
5 0.0696114496148699
6 -0.129495523138125
7 0.319413967283282
8 0.810263481492047
9 1.14970431405883
10 1.34412749027052
11 1.39726847410919
12 0.818198682962102
13 -0.0743022793044457
14 -0.572140432842321
15 -1.61182355702458
16 -2.13697225029644
17 -2.87146488485125
18 -3.51122562476858
19 -3.87431853611337
20 -4.38687986877699
21 -4.76129028604839
22 -5.11621253367295
23 -5.53784788419322
24 -5.83924866941049
25 -6.11670644239442
26 -6.2393957248285
27 -6.5019364808354
28 -6.92983731883817
29 -7.1085929505323
30 -7.34938902721106
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.9435976221712
1 2.60434640396296
2 1.82531944122752
3 0.915436025197645
4 -0.20253823008235
5 -0.996477443312562
6 -1.51754398729509
7 -1.77049759798548
8 -1.9385542298273
9 -1.56591956519139
10 -1.01181794782326
11 -0.64288000450366
12 -0.335017927747101
13 -0.658011944729953
14 -1.18089823544264
15 -1.82178681308893
16 -2.71281034761956
17 -3.49169300601809
18 -4.25764459101841
19 -4.96944061111127
20 -5.69892080746051
21 -6.47686466411992
22 -7.4489321292192
23 -8.38777304396719
24 -9.29145367585666
25 -10.238213800163
26 -11.3142800741209
27 -12.4381565337616
28 -13.210567611412
29 -14.2265005841731
30 -15.1736997904836
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.93319342594283
1 2.78175133650157
2 2.07072687408619
3 0.809314197849055
4 -0.471314747072839
5 -0.325643261659565
6 -0.518865188779872
7 -0.47217221695135
8 -0.0774795413904528
9 0.411845406390039
10 0.640146888723354
11 0.687693066532059
12 0.619901535139169
13 0.33283327598158
14 -0.208557176326821
15 -0.859913468768362
16 -1.6889564542041
17 -2.27994612991458
18 -2.95841230675417
19 -3.71577512937591
20 -4.35865465907462
21 -5.13491476582201
22 -5.88334255304879
23 -6.50995600535579
24 -7.17502678887057
25 -7.74360835317096
26 -8.30228145335666
27 -8.84385723361144
28 -9.22363781754923
29 -9.84853203814344
30 -10.3392655370049
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.93743083466299
1 2.4618667505381
2 1.90877631229131
3 0.809551927824241
4 -0.21503615471261
5 -1.01649028028315
6 -1.77278420777936
7 -1.9831937429708
8 -1.86216456434405
9 -1.82511717453144
10 -1.77043075160794
11 -1.99854178084841
12 -1.96278991707541
13 -2.34853251895596
14 -2.68615724942901
15 -3.13881349276035
16 -3.80478546629946
17 -4.35911696968099
18 -4.95526720535159
19 -5.7222239986125
20 -6.36683258435973
21 -7.19440803242158
22 -7.90740369494987
23 -8.47190004529271
24 -9.38240183770504
25 -10.1192583183662
26 -10.8441829682568
27 -11.4316944769191
28 -12.1098003116621
29 -12.7683633854228
30 -13.3224432428212
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.88310538335514
1 2.55926314341934
2 1.77916207914626
3 0.496922495545396
4 -0.605135884960303
5 -1.59537015218532
6 -2.10378564061297
7 -2.29523303556155
8 -2.54410753918477
9 -2.30575397175805
10 -2.2117842328846
11 -2.22479731648984
12 -2.31198057712861
13 -2.8622911242503
14 -3.50161782144431
15 -4.28356986728664
16 -5.26045375045567
17 -6.00114145870232
18 -6.88114647956575
19 -7.59747235459221
20 -8.19605111747942
21 -8.72471768656091
22 -9.22336185383707
23 -9.67274046637905
24 -10.1484861102361
25 -10.9432862786341
26 -11.5504594982176
27 -12.1177176575398
28 -12.6173378815727
29 -13.0863425532142
30 -13.6941697536453
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.88501357918485
1 2.15305833866845
2 0.945881195178439
3 -0.354270727923874
4 -1.79857045933571
5 -2.09834555248273
6 -2.33846348017841
7 -2.55563140255559
8 -2.58159554047167
9 -2.21141232536116
10 -1.87449102896611
11 -1.9303093655007
12 -1.83715658066218
13 -2.26807732866261
14 -2.71922501509768
15 -3.2534016566151
16 -3.7509344555716
17 -4.33384791785951
18 -4.93597633075317
19 -5.40751547268532
20 -5.66449427613441
21 -6.13692240364059
22 -6.45415574661563
23 -6.94442635311361
24 -7.43711547214253
25 -8.28615847110485
26 -9.08423449012573
27 -9.53533038768601
28 -9.9349761136346
29 -10.3827868870261
30 -11.1419586025403
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.89719497832019
1 2.74455440811125
2 2.47280587183004
3 2.12769021427278
4 1.64124082746463
5 1.7425819613028
6 1.52764636734248
7 1.42453093302357
8 1.82273673967213
9 2.21402392167337
10 2.61911281800675
11 2.88366923100713
12 3.11788132621245
13 2.97465451021719
14 2.91692435309664
15 2.39745993010175
16 1.93275579208787
17 1.31848448989418
18 0.766669082629081
19 0.290587090568954
20 -0.313809410014201
21 -1.05800302822386
22 -1.67658721309076
23 -2.27385900180073
24 -2.76961998700828
25 -3.20212467346623
26 -3.46492860863419
27 -3.87978695380789
28 -4.44832856895323
29 -4.68194858821135
30 -4.8933029556824
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.91683838626076
1 2.77211096106391
2 2.01378138200327
3 1.13005700772266
4 0.35855185841268
5 -0.0229159321377121
6 -0.697857522401966
7 -0.676880364537165
8 -0.52384385456422
9 -0.358597758983931
10 -0.228695317089414
11 -0.224082484699323
12 -0.515393033983855
13 -1.11679164536899
14 -1.70003842538725
15 -2.45335627830135
16 -2.92196536294861
17 -3.29786658925145
18 -3.80970348436106
19 -4.36517943690114
20 -4.44241712128907
21 -4.80349821261641
22 -5.01966344002693
23 -5.17789179448255
24 -5.53178855377629
25 -6.01974738325377
26 -6.2099820668153
27 -6.26851884331501
28 -6.6221133395825
29 -6.75486894014544
30 -6.92549170345542
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.92139299664258
1 2.43224254773937
2 1.74923972186752
3 0.800456043299581
4 0.0522081750311507
5 0.198485761995361
6 0.0544516133548232
7 0.387724529963222
8 1.07376492237801
9 1.43910644467963
10 1.62712285391588
11 1.68861196048561
12 1.68233326552281
13 1.30522212545402
14 0.595554215845278
15 -0.45573816876469
16 -1.44543149255044
17 -2.30271455772976
18 -2.72799160038608
19 -3.32323830560492
20 -3.97358302439439
21 -4.61153003781302
22 -5.26275350766972
23 -5.97846234657599
24 -6.42311989666815
25 -7.19858895938061
26 -7.91311951811163
27 -8.51584218824517
28 -9.1321774634689
29 -9.74719055486082
30 -10.400630085569
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.95057087554497
1 2.54309477218288
2 1.70288691457008
3 0.682059395500373
4 -0.237009599769628
5 -0.783798161458455
6 -1.03570153448547
7 -0.611248577784032
8 0.215569938829159
9 0.795641622277618
10 1.29431084547389
11 1.66415317995659
12 2.09763706958025
13 2.09166325734223
14 1.61772954321654
15 1.36792384501073
16 0.959977992269836
17 0.271034583456791
18 -0.0126187549556551
19 -0.341648005718032
20 -0.779491413489637
21 -1.10946420312917
22 -1.28625187480422
23 -1.58625687630223
24 -1.73020100527534
25 -2.04088914640019
26 -2.37233299765707
27 -2.62936512846716
28 -3.08550604481458
29 -3.30162854497115
30 -3.55006310915089
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.88668361515075
1 2.54834311996417
2 1.88526130207818
3 0.99441788194928
4 -0.079849413496424
5 -0.789808055770324
6 -0.84843161810049
7 -0.526763018207248
8 0.128393675591917
9 0.7960612894243
10 1.51534701810741
11 1.88734649438743
12 2.03099501902577
13 1.7357683050114
14 1.28082812700067
15 0.403180219055249
16 -0.380605032781245
17 -0.932461313746701
18 -1.6546390176469
19 -2.16171696141281
20 -2.6617140072688
21 -3.2877004081727
22 -3.79885695006269
23 -4.34202701638191
24 -5.04150913007045
25 -5.74441511141299
26 -6.53950008640157
27 -7.13105549564666
28 -7.77241987680185
29 -8.50092098167287
30 -9.38552671162828
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.9351309338836
1 2.43389659398219
2 1.53732518899365
3 0.761806258786812
4 -0.380467352065601
5 -0.716960045605191
6 -1.4247830070388
7 -1.60876339572054
8 -1.4655146631347
9 -1.10423161445438
10 -0.544046290140312
11 -0.34205161177025
12 -0.182424770489739
13 -0.0406085280915125
14 -0.222401717506978
15 -0.721193672511506
16 -0.842951724109449
17 -1.27318545117389
18 -1.88050935458558
19 -2.48355443989532
20 -2.79794835472521
21 -3.28503798317215
22 -3.54481480484169
23 -3.86197945959031
24 -4.32427521100361
25 -4.78243072265084
26 -5.23661142636361
27 -5.87758043432511
28 -6.52524271834919
29 -6.99550977096823
30 -7.41424460201803
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.95230801592821
1 2.76017062396994
2 2.05474536517638
3 1.07193223624455
4 0.350439778328354
5 -0.133813486753242
6 -0.714172772392025
7 -0.450179714287499
8 -0.0378471871026917
9 -0.327410290190253
10 -0.683872279702417
11 -0.990286936244599
12 -1.11085540741657
13 -1.60030232986074
14 -2.33746470094731
15 -2.89733932412869
16 -3.6658663121361
17 -4.38258759066539
18 -4.94175432558113
19 -6.00022443696733
20 -6.93713834917761
21 -7.9481883632298
22 -8.87029510026318
23 -9.69880111474272
24 -10.5208131786297
25 -11.193633911597
26 -11.9416613017038
27 -12.819023548258
28 -13.5584950660274
29 -14.4113826179418
30 -15.1456807477156
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.9163656505103
1 2.68586883748621
2 2.12252795347083
3 1.1485352159901
4 0.144334211604553
5 0.0402759740773213
6 0.0390199128116162
7 0.114766861793544
8 0.325255080655166
9 0.574895863524606
10 0.641414726709062
11 0.635908194096181
12 0.450164572184379
13 0.205351062536343
14 -0.56709473995649
15 -1.26973993860093
16 -1.7601424605429
17 -2.13575635816962
18 -2.94401113695299
19 -3.79860829707417
20 -4.06034387913342
21 -4.61578407193496
22 -5.10865947183532
23 -5.26648162260049
24 -5.72442860526442
25 -6.07109977735533
26 -6.34406094568701
27 -6.56486338994617
28 -7.06746997010809
29 -7.38744147516443
30 -7.44448182671903
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.87469041771114
1 3.0427021651964
2 2.46847169678202
3 1.49188756361272
4 0.719557709241114
5 -0.10545324980022
6 -0.511128009028532
7 -0.550155624676551
8 -0.594512222876773
9 -0.831541808397979
10 -0.692265907536832
11 -0.950382498796118
12 -1.10876332027876
13 -1.68427692840214
14 -2.31262568862311
15 -3.24096432037378
16 -4.35799886560152
17 -5.52134192674043
18 -6.45634993477837
19 -7.39570451530766
20 -8.4308637188379
21 -9.32613358149408
22 -10.3280294770401
23 -11.3791175663251
24 -12.3971874147889
25 -13.4101308562818
26 -14.5588553189179
27 -15.626888155649
28 -16.4677565188331
29 -17.3188292809976
30 -18.250837998956
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.93222389916711
1 2.2353514881659
2 1.32466878054561
3 0.343077952618877
4 -0.715870063514991
5 -1.0165745121685
6 -1.39235434559338
7 -1.53762548418794
8 -1.27572437263959
9 -1.19111913772485
10 -1.54612027622187
11 -1.72904091788884
12 -1.94136432039493
13 -2.36169637837895
14 -3.07409739842788
15 -3.88496650041701
16 -4.86648823882041
17 -5.87620516330587
18 -6.70693198030865
19 -7.59518343137015
20 -8.45124781320617
21 -9.37752348296379
22 -10.3486014775057
23 -11.3162531412773
24 -12.1701267371024
25 -12.9437058836286
26 -13.7608545014151
27 -14.7546664771975
28 -15.5352174680512
29 -16.4193326967595
30 -17.0964008393699
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.90368700867959
1 2.64164456175367
2 1.70889808567389
3 0.503894091152679
4 -0.211995633495881
5 -1.00581221831788
6 -1.59438690975468
7 -1.84240504163568
8 -2.060247114225
9 -1.95537199325463
10 -1.76060297011821
11 -1.70870572065197
12 -1.75496883120775
13 -2.2783445070499
14 -2.65013912510738
15 -3.44984186834777
16 -3.84339993589455
17 -4.60310229000094
18 -5.18369211249331
19 -5.45935846993161
20 -5.92785733340336
21 -6.46609637417034
22 -6.96627376966991
23 -7.35831380192248
24 -7.92806857970136
25 -8.14606776870304
26 -8.50106930341831
27 -8.73413488765762
28 -9.06909380834202
29 -9.35813844508131
30 -9.45232770667346
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.90533775355124
1 2.70259750834927
2 2.25708676282388
3 1.28284015138423
4 0.528853673981329
5 -0.185326900871603
6 -0.305090151158833
7 -0.348718720089856
8 0.208970272856877
9 0.509137308225576
10 0.638566211494348
11 0.828149993333824
12 1.32496083486837
13 1.34248350718896
14 1.15275972036486
15 0.463467860033219
16 0.00969593240208333
17 -0.676540492041672
18 -1.31246395942587
19 -2.03548839034448
20 -2.4823900012247
21 -3.07205275477529
22 -3.53706430581011
23 -4.02815708823552
24 -4.71077064345469
25 -5.481380897726
26 -6.2418825736633
27 -6.76956383484589
28 -7.39111063901938
29 -8.04896862756466
30 -8.42404293989061
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.88672943987313
1 2.51368123049979
2 1.89887055185809
3 0.990011475431272
4 0.302260942190658
5 0.12344836496559
6 -0.321323666538838
7 -0.343903572904473
8 0.0822034530646185
9 0.387936243178236
10 0.56732560703764
11 0.467174210341453
12 0.488457874788358
13 0.34408453148893
14 0.110748289645624
15 -0.472702032717061
16 -0.866887219442779
17 -1.23790101336304
18 -1.88002796238632
19 -2.25434579676274
20 -2.63093091578906
21 -2.86166916857833
22 -3.34934908636885
23 -3.65691234286551
24 -3.95464571300611
25 -4.43346707605641
26 -4.77625087650489
27 -5.20539784515385
28 -5.51011857355901
29 -5.96386964715581
30 -6.23092439591705
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.8441945077037
1 2.69092262968877
2 2.0143672598188
3 1.03868276011035
4 0.0306367734802997
5 -0.354277572327103
6 -0.569828429808721
7 -0.806637435404628
8 -0.627029473661509
9 -0.0917628995458646
10 0.485164453428009
11 0.603983178828411
12 0.675453007511168
13 0.276822918218029
14 0.193462733409758
15 -0.0338626135557636
16 -0.562923619365421
17 -0.9899982453194
18 -2.03661834866046
19 -2.96385100504626
20 -3.5262152956492
21 -4.26219840968522
22 -4.84060953521612
23 -5.23707310479008
24 -6.00003598323538
25 -6.65857248565263
26 -7.13363164608578
27 -7.78604465652294
28 -8.47642343348257
29 -9.18127253183169
30 -9.75240738999906
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.87962282803052
1 2.53989286784146
2 1.74017786019655
3 0.756851471779926
4 -0.579995660542959
5 -0.773352762652465
6 -1.25148450962846
7 -1.25457405547875
8 -1.0396867590498
9 -0.729659318132892
10 -0.410490908184432
11 -0.314593687255982
12 -0.563939712199781
13 -1.16516192845848
14 -1.86786107730572
15 -2.84386716973339
16 -3.81172601787874
17 -4.77961781032246
18 -5.87890628429099
19 -6.76302746031576
20 -7.64767665579922
21 -8.60678590175466
22 -9.3979011446079
23 -9.91289377597575
24 -10.4839525374776
25 -10.8861623902059
26 -11.4432986158605
27 -11.9687160649784
28 -12.7967309976893
29 -13.0860024694994
30 -13.4104117993453
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.86207812427552
1 3.01740213897603
2 2.46735634242805
3 1.44555214112267
4 0.503568249712176
5 -0.0441186794773252
6 -0.610669686605934
7 -0.978843242667395
8 -0.757170968659606
9 -0.526967298103159
10 -0.0832727632815278
11 0.112660673213457
12 -0.111906894740244
13 -0.560015369317242
14 -0.876763682452465
15 -1.49286221300316
16 -2.01220775485626
17 -2.53624266127879
18 -2.9982599693805
19 -3.49878370378009
20 -4.03347171131936
21 -4.6295379592002
22 -5.11625243618575
23 -5.71385027129857
24 -6.28796270845455
25 -6.82116146946221
26 -7.32361945081929
27 -7.84456053094064
28 -8.06871126366167
29 -8.47969878961718
30 -8.76241441935436
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.9306235605416
1 2.39711925443337
2 1.47148723371615
3 0.393967457411952
4 -0.401367392201136
5 -1.24474468669347
6 -1.81548364296116
7 -2.2508842033958
8 -2.42106331413894
9 -2.25968472448889
10 -1.97106619537728
11 -1.83086119311804
12 -1.52904505300935
13 -1.88365617260717
14 -2.21945156709456
15 -2.64736084228455
16 -3.23344040729508
17 -3.66461749453864
18 -4.14923818478625
19 -4.70522969699692
20 -5.36513818714834
21 -5.70230926236404
22 -6.06751578912711
23 -6.54561190029483
24 -6.88506081683024
25 -7.0289359446978
26 -7.21105459132528
27 -7.30862456376615
28 -7.7446935130467
29 -7.86257833846456
30 -7.8118721152978
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.89273746716082
1 2.62552963283675
2 2.06712290419479
3 1.32752272364737
4 0.411974220275759
5 0.240216775401795
6 -0.2674751456425
7 -0.309017907367661
8 0.164071248734569
9 0.474267868560235
10 0.66798431037294
11 0.766259823518952
12 0.846956309239095
13 0.345611097531307
14 -0.50986640235835
15 -1.59573540872202
16 -2.61095264496214
17 -3.49833606002447
18 -4.04537908900364
19 -4.74548093146493
20 -5.53990818748372
21 -5.83765774893723
22 -6.46997995256931
23 -7.28219370762983
24 -7.80923148153181
25 -8.74337489445296
26 -9.39859348785585
27 -9.92349113458279
28 -10.3201341098308
29 -10.790289195402
30 -11.3742661197671
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.93326857182641
1 2.49060603601579
2 1.75281668179393
3 0.47831520096851
4 -0.543569979360244
5 -0.753893157968223
6 -1.34094436322266
7 -1.2970892864799
8 -1.05997891800093
9 -0.378400848317051
10 0.344235442698116
11 0.73257074931392
12 1.04211714463586
13 0.754635324345486
14 0.358973539168963
15 -0.395874826658371
16 -1.16359753738985
17 -2.1967037663511
18 -2.77344085508458
19 -3.28534055301187
20 -3.74997265688529
21 -4.05151835017014
22 -4.29086998712929
23 -4.49884294183626
24 -4.79397530797068
25 -4.83971833611852
26 -4.95944880112658
27 -5.24336133826116
28 -5.42313673546534
29 -5.70725496966593
30 -6.00346102846886
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.885621483504
1 2.3421513481962
2 1.63614562187013
3 0.711569533844795
4 -0.0384361719803525
5 -0.425938546415511
6 -0.770179282334214
7 -0.807889644430999
8 -0.437642828392974
9 -0.319992890602919
10 -0.0812486223790714
11 -0.25827427462886
12 -0.445707656621551
13 -1.13011422680819
14 -1.66473525251532
15 -2.55570591683483
16 -3.32971405948217
17 -4.26325569509786
18 -4.59660742379533
19 -4.99934781075133
20 -5.81714440841726
21 -6.26945649123103
22 -6.6530475062401
23 -7.31222576204296
24 -7.75599843417717
25 -8.25293773166372
26 -8.62589001343835
27 -9.05500892296582
28 -9.65222762725888
29 -10.140105766441
30 -10.4646454983649
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.87489837283561
1 2.46998032986789
2 1.58796518396016
3 0.525007882965985
4 -0.440532708330451
5 -0.647068178616641
6 -0.873056834179453
7 -0.79490882687227
8 -0.33532774234787
9 -0.107530234617466
10 0.216080491223607
11 0.314812469120627
12 0.0461856663152513
13 -0.531456697504176
14 -1.32583076066285
15 -2.40631608157178
16 -3.29073121433133
17 -4.68787483691006
18 -5.90116768060246
19 -7.09513026042861
20 -8.1480651567823
21 -9.32771589192829
22 -10.3870689612495
23 -11.2730677879548
24 -12.4203868382568
25 -13.5712584820713
26 -14.5910245085471
27 -15.2489219565261
28 -16.2852444968067
29 -17.0400022567868
30 -18.050646309321
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.88063041876922
1 2.06062320719403
2 1.38545337500439
3 0.404964712276138
4 -0.714556768875271
5 -1.19190724953428
6 -1.54126346654363
7 -1.55181928305322
8 -1.30975810087287
9 -0.646566319483879
10 -0.312128426309384
11 0.326689639225226
12 0.570939211704232
13 0.37562781580923
14 0.321553083998898
15 0.0687206856776523
16 -0.425537785434425
17 -1.02224688985074
18 -1.81704452345544
19 -2.57524866992176
20 -2.83428094347399
21 -3.39687837582469
22 -3.62436497791703
23 -3.82920371429539
24 -4.3336418390876
25 -4.78515580210048
26 -5.18975473798393
27 -5.50308154115356
28 -5.97436255256646
29 -6.43325516716572
30 -6.85448750873077
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.96683165255349
1 2.33142161663912
2 1.596558597381
3 0.86743622718317
4 0.0957538081443996
5 -0.106778821170932
6 -0.321097021354605
7 -0.319832127360577
8 -0.327032528813477
9 -0.0368561140236832
10 0.172809422749882
11 0.186059812178989
12 -0.00272918339639006
13 -0.391806561872626
14 -0.957108466729004
15 -1.68632172044719
16 -2.23907309396854
17 -2.76281841646923
18 -3.3324920350913
19 -3.99618077968809
20 -4.61923025039852
21 -5.1711437471948
22 -5.71632303657642
23 -6.44998622149366
24 -7.02402244625768
25 -7.85632300861337
26 -8.75778417982209
27 -9.31230459552383
28 -9.937519491019
29 -10.4650023617615
30 -11.0596077821035
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.90775386580665
1 2.34640678950752
2 1.79973586685699
3 0.7290399966232
4 0.0166650909946533
5 -0.48448106620066
6 -0.924956928526523
7 -1.19363680115957
8 -1.22387328759711
9 -0.915527058346004
10 -0.465500014221414
11 -0.423241182621284
12 -0.594547637690889
13 -1.20742006296219
14 -1.87970824174251
15 -3.0044728863374
16 -3.96346243121843
17 -5.07708382756081
18 -5.88923894262123
19 -6.76671183137674
20 -7.75999369565723
21 -8.50893903451347
22 -9.43228974821513
23 -10.3774863529246
24 -11.0726838327784
25 -12.1279153191095
26 -12.9183603439757
27 -13.8437508273672
28 -14.5712190345138
29 -15.3112095408504
30 -16.1035103103076
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.88300344665172
1 2.42028036672892
2 1.64698607004821
3 0.859595253182352
4 -0.146924411400066
5 -0.476175971228306
6 -0.933027218979561
7 -1.22815692619697
8 -1.23563843263588
9 -1.15414034740192
10 -0.815183747985003
11 -1.04256753933913
12 -1.27375493072141
13 -1.62147499601215
14 -2.13153314187305
15 -2.64237937028257
16 -3.554617252792
17 -4.39587468832812
18 -5.20811114286748
19 -5.81656579421621
20 -6.66643359017033
21 -7.26300486987502
22 -8.23226330299902
23 -9.12327709403224
24 -9.72649033128453
25 -10.6180654677704
26 -11.3988363167742
27 -12.4108429529484
28 -12.9480881911669
29 -13.8587714357431
30 -14.5499511923359
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.87945759841766
1 2.62489174575565
2 1.9382014743368
3 0.848269948840503
4 -0.514509700786029
5 -0.831062941686504
6 -1.16566183211802
7 -1.25931028772089
8 -1.48119544603101
9 -1.90353785325669
10 -2.10179855587832
11 -2.76055545448002
12 -2.96059103660421
13 -3.35072764242516
14 -3.88050940154942
15 -4.6087203709246
16 -5.39758453211682
17 -6.35030669758046
18 -7.25067364390654
19 -7.95695611162059
20 -9.06362495509841
21 -9.76224822417096
22 -10.6199698456718
23 -11.4270731968068
24 -12.1922794697488
25 -12.9461187702136
26 -13.8115448978499
27 -14.4330905693111
28 -14.8392672198997
29 -15.4844684298924
30 -16.0160427817017
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.91823146441852
1 2.35404750003665
2 1.59906446529649
3 0.587044006060879
4 0.0675971612829951
5 -0.304207498360746
6 -0.416833437725767
7 -0.608548839830927
8 0.164696591246045
9 1.01520622831066
10 1.31842068658443
11 1.77389447415294
12 1.96234452248132
13 1.32619450366607
14 0.75734166728356
15 -0.387580902806885
16 -1.16880922791175
17 -2.31825948044658
18 -2.94794689510919
19 -3.42581022852164
20 -4.16898776278193
21 -4.70418598144123
22 -5.32086966960536
23 -5.87375593632433
24 -6.33465067992929
25 -7.17067676095183
26 -8.00533310940205
27 -8.53794747716496
28 -8.6765063958927
29 -9.18694732448815
30 -10.0845563017117
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.917426688008
1 2.59601876365814
2 1.79712037065875
3 0.750006756598966
4 -0.217984494048467
5 -0.400245869229526
6 -0.721089445591499
7 -0.556621150203684
8 -0.104940980080032
9 0.0334480138070319
10 0.214438568669994
11 0.234583768928054
12 0.00432001668250237
13 -0.483350813621165
14 -1.19115759431094
15 -2.16209141948237
16 -2.80115507405302
17 -3.83266095517842
18 -4.80151931769405
19 -5.70290770406296
20 -6.83707340170079
21 -7.81107054020208
22 -8.67015882383783
23 -9.45888565591461
24 -10.3955650631255
25 -11.1412459978533
26 -11.8874887946632
27 -12.6971594020064
28 -13.3971872333065
29 -14.2615706573774
30 -15.0779089309405
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.84906830064393
1 2.62263776259587
2 1.996987192646
3 1.11926128722095
4 0.0472426277323557
5 0.00893527499733793
6 -0.089988611372414
7 -0.0420104671500763
8 0.243283645034392
9 0.895950418872724
10 1.31239892596395
11 1.24997129776256
12 1.28098680649181
13 0.887246428638591
14 0.270475162366459
15 -0.453751932938509
16 -1.28234022816592
17 -2.18954856871757
18 -2.65610665810434
19 -3.24363662561639
20 -3.80734579325322
21 -4.18283851336959
22 -4.42675157170457
23 -5.04366067777547
24 -5.51453512869013
25 -6.05553484702918
26 -6.50512442657301
27 -6.77188558360079
28 -7.03289317902279
29 -7.32236339123169
30 -7.67662146934012
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.90681104963615
1 2.62000003246492
2 1.84710636634498
3 1.4453112698791
4 0.613484576931164
5 0.141683599502347
6 -0.215917792412212
7 -0.410432307889593
8 -0.388346807186585
9 -0.439553189146856
10 -0.396697294775027
11 -0.623807399705706
12 -0.487902100928435
13 -0.925284319137669
14 -1.18888700278817
15 -1.58016126134366
16 -1.80438647249304
17 -2.30903008553876
18 -3.0347947972213
19 -3.82665281068844
20 -4.52999003783479
21 -5.19601970585825
22 -5.5701839814754
23 -6.13134581931704
24 -6.65106771693333
25 -7.39367201937856
26 -7.96850668888374
27 -8.62400985447228
28 -9.04366315052126
29 -9.521102446466
30 -10.0019183843121
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.92320766868523
1 2.70787002729755
2 2.40200643245474
3 1.93463130292033
4 0.959236191425932
5 0.650479421244567
6 0.485832027402198
7 0.656164257879734
8 0.906443893144878
9 1.35218535441605
10 1.53239300648055
11 1.47057368561036
12 1.48855422653216
13 1.12614237060431
14 0.643711323699369
15 -0.170322165430212
16 -0.853398454704463
17 -1.39693103545895
18 -2.30558687015716
19 -3.23262427253605
20 -3.76094297558658
21 -4.55645515337259
22 -5.43794068450257
23 -6.06554808955012
24 -6.7337970483797
25 -7.33678227930361
26 -7.75685801059532
27 -8.42173500981503
28 -9.04211279057304
29 -9.67678681744877
30 -10.1464666119394
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.8394608979203
1 2.69364721800836
2 1.93121757361941
3 1.07999497697324
4 0.0377538917411631
5 0.111997590407448
6 0.175789517174048
7 0.587511941529803
8 1.24864728332919
9 2.01372430922182
10 2.56356737922986
11 3.35622760598555
12 3.64485767671733
13 3.37010665113774
14 2.92564553531561
15 1.97834489896375
16 1.22856557003623
17 0.226550548772851
18 -0.413352844735437
19 -1.18698196731726
20 -1.99843473976777
21 -2.54416930206327
22 -2.96583793989272
23 -3.41918909847207
24 -3.74846452885985
25 -4.1601146019029
26 -4.52016013272502
27 -4.76644776066923
28 -4.76176528492952
29 -4.71853640022925
30 -4.76101808722894
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.91003435660666
1 2.84507886703042
2 2.41583435487418
3 1.50540647929607
4 0.934668478230034
5 0.561983098351002
6 0.172769088249069
7 0.395547919592397
8 1.00793812798393
9 1.14849048009412
10 1.26057649530311
11 1.39115402093496
12 1.05206826497784
13 0.357923588688159
14 -0.472339440779828
15 -1.54964729704175
16 -2.50627763892776
17 -3.33798385737244
18 -3.82087004514753
19 -4.35850935289171
20 -4.86401954638083
21 -5.18857166366692
22 -5.84639613082911
23 -6.37592177908454
24 -6.78477027446328
25 -7.69067436188056
26 -8.52289678404514
27 -9.13195785862068
28 -9.55275926960859
29 -10.1749955205856
30 -11.1041163862538
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.87972001837527
1 2.95631230944783
2 2.3643413788157
3 1.48095126326867
4 0.267382090324654
5 -0.696563161456696
6 -0.914622017729602
7 -1.2008387497189
8 -1.06910989056169
9 -0.781476002930722
10 -0.513340361586923
11 -0.463365029714936
12 -0.557674645477846
13 -0.960147767046854
14 -1.51540240905151
15 -2.26610391355573
16 -3.10029182158061
17 -3.9624003121486
18 -4.55964374439051
19 -5.51058149371369
20 -6.37955510400754
21 -6.91971682978884
22 -7.36320862495613
23 -8.10778393236593
24 -8.96795479028571
25 -10.0443967875556
26 -10.9975941865328
27 -11.7181218135782
28 -12.2720155254804
29 -12.9968477051697
30 -13.7127048962388
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.8710895587937
1 2.64285993931721
2 1.79391283869023
3 0.699744520450478
4 -0.441751192804706
5 -0.721217604461721
6 -1.04194965487128
7 -0.656969243901568
8 -0.224573170868783
9 0.28728849971905
10 0.656800272257312
11 0.747529423473251
12 0.896896167108219
13 0.902702470070659
14 0.67721852221578
15 -0.15412201593703
16 -0.571455333602445
17 -1.16982715451956
18 -1.83647920992649
19 -2.50582568361967
20 -3.14824888908927
21 -3.80210605157423
22 -4.34306600798397
23 -5.02059071122754
24 -5.59982234320422
25 -6.20259476721988
26 -6.89983834521265
27 -7.69933061525167
28 -8.18656463230953
29 -8.939107861061
30 -9.64728772290094
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.85501620443676
1 2.33859602420311
2 1.56234543912385
3 0.931894974091662
4 -0.147823616768491
5 -0.596932620609998
6 -1.17143926766722
7 -1.23259487866583
8 -1.13723120841399
9 -0.667624206661449
10 -0.306261754213928
11 -0.111133796717981
12 -0.0680820329026481
13 -0.525691528027306
14 -0.99229876053441
15 -1.86070687174253
16 -2.41007859737882
17 -3.14451161044444
18 -3.88914010190668
19 -4.57110014878169
20 -5.53379156682963
21 -6.1523909660072
22 -7.12723279534815
23 -8.11189349612681
24 -8.85558830033195
25 -9.88659065492068
26 -10.9770930604808
27 -11.8055616733386
28 -12.5770048076574
29 -13.5815779242024
30 -14.6095612817162
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.9605727782298
1 2.70846372225408
2 1.77906237664719
3 0.580898504445212
4 -0.613636223319459
5 -0.94748781380758
6 -1.3035450284196
7 -1.10617227883556
8 -0.410787081954853
9 -0.166012499695404
10 0.229570753933439
11 0.391154633940365
12 0.589069973405879
13 0.123728627273453
14 -0.617410085141108
15 -1.57562805320835
16 -2.20217638974573
17 -2.93489716126403
18 -3.77254353751495
19 -4.7688971877627
20 -5.50273699838341
21 -6.32268159596196
22 -7.05341908816807
23 -7.6625710835475
24 -8.55792249498313
25 -9.14930264520187
26 -9.65407695473734
27 -10.037963271201
28 -10.3583078522892
29 -11.0006543356046
30 -11.4789965464226
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.85014763188408
1 2.57399639130531
2 1.62596777010032
3 0.397693575989896
4 -0.741985341551901
5 -1.32870121197151
6 -1.47795494480569
7 -1.21119306939838
8 -0.608210581655362
9 -0.188818638164628
10 -0.0637277944387638
11 -0.0713710424378924
12 -0.407857310100232
13 -0.66164048515
14 -1.12767157680877
15 -2.16196120697162
16 -3.29659976997317
17 -4.47203566079936
18 -5.67876475924363
19 -6.66783239162739
20 -7.85449928597131
21 -9.03861925472188
22 -10.2679027107336
23 -11.4968516681285
24 -12.4521610110976
25 -13.5216297115766
26 -14.7208103957494
27 -15.9633280238415
28 -16.79790817808
29 -18.136632495742
30 -19.4621323921727
};
\addplot [line width=0.01pt, color1, mark=*, mark size=2, mark options={solid, draw=black}]
table {%
1 2.65103446372252
2 1.87298481713709
3 1.03310235020523
4 -0.0349224785257646
5 -0.681923979276541
6 -0.614035490335335
7 -0.208100847346677
8 0.33428430837777
9 0.710486243049944
10 0.726233644866842
11 0.520411660737353
12 0.347599665643602
13 0.244300607278545
14 0.195112904269273
15 0.20629800498181
16 0.161911176310666
17 0.161283251423433
18 0.247899352697984
19 0.208651205023874
20 0.171253015388636
21 0.20029198108343
22 0.172890109571832
23 0.187770311286831
24 0.213147053788955
25 0.185796243819713
26 0.165625930691843
27 0.187584184388062
28 0.20252014981221
29 0.179459395114634
30 0.2013127196102
};

\end{groupplot}


==> experiments/figs/double_pendulum/tikz_samples_ep-8-all.tex <==
\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}

\begin{groupplot}[group style={group size=1 by 3}]
\nextgroupplot[
xshift=-8,
title={8 episodes},
title style={font=\large},
xmin=-1.45, xmax=30.45,
%ymin=1.45279922629327, ymax=6.59122540478087,
ymin=2.7, ymax=6.7,
width=\figurewidth,
height=\figureheight,
xtick={},
xticklabels={},
yticklabels={},
tick align=outside,
tick pos=left,
x grid style={white!69.019607843137251!black},
y grid style={white!69.019607843137251!black}
]
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.09181717025381
1 3.26433761326292
2 3.21335791116766
3 2.98043246214825
4 2.79861367479082
5 3.01575891435463
6 3.1843997749744
7 3.1402246909847
8 2.83330358219165
9 2.46829114347869
10 2.07050525611437
11 1.62513735443336
12 1.16060178293092
13 0.800829018997597
14 0.176618397019231
15 -0.166067584645345
16 -0.475633284420923
17 -0.861179255348848
18 -1.12785253446476
19 -1.42168391132546
20 -1.78992093742078
21 -2.27920521379678
22 -2.58345318005847
23 -2.95135537497888
24 -3.40070121868806
25 -3.87132841201935
26 -4.28275522363522
27 -4.60340426370748
28 -4.87267814856092
29 -5.10134340058613
30 -5.2504967659125
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.18526912578385
1 3.42347850171755
2 3.47634249843012
3 3.2770035984891
4 3.04748521576749
5 3.16923639928785
6 3.36165011191692
7 3.41522545616921
8 3.34500024001809
9 2.82329136438717
10 2.24035135555178
11 1.64072396778315
12 0.913090684928871
13 0.520334546719145
14 0.145260263971574
15 -0.15846177174148
16 -0.589432517050669
17 -0.846824268556173
18 -1.04106896716278
19 -1.18202794690124
20 -1.37030028668705
21 -1.56613501735211
22 -1.72868729246926
23 -1.9286042044241
24 -2.13851712009566
25 -2.37411782692574
26 -2.64052433613419
27 -2.80786382442835
28 -3.0373059690177
29 -3.16816875164586
30 -3.17664635862295
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.31136414675513
1 3.62856447615133
2 3.45547868047449
3 3.07543035700938
4 2.77008000271001
5 3.14932834963223
6 3.31369525470689
7 3.51770070954131
8 3.47887458573494
9 3.06520120991979
10 2.53793136875865
11 2.11558515823165
12 1.7095842619452
13 1.32573815918246
14 0.868727738724568
15 0.353609440934894
16 -0.1757612187604
17 -0.569815344769399
18 -1.12756940581015
19 -1.63184535756022
20 -1.93704889972412
21 -2.28129548086891
22 -2.6183044446613
23 -2.89834990924794
24 -3.14278713027099
25 -3.48574447411395
26 -3.72185103263021
27 -3.98057409655994
28 -4.22554342739971
29 -4.4266572870091
30 -4.69878185811778
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.08933589272699
1 3.41556270810353
2 3.30082774863135
3 3.10359375041496
4 2.9028558688164
5 3.11180168557654
6 3.17546183752112
7 3.21692984610798
8 2.89289650259928
9 2.62777969994412
10 2.38755026673446
11 2.2015450789738
12 2.01640689498628
13 1.79751664646451
14 1.41386704395956
15 0.897873340825308
16 0.614425773617285
17 0.234912895396828
18 -0.015326819902624
19 -0.258353351904899
20 -0.622614762794273
21 -0.90118623109683
22 -1.20673894072553
23 -1.62216056978157
24 -2.00686936844187
25 -2.38670778418189
26 -2.81121876507193
27 -3.32777699346442
28 -3.79904621896078
29 -4.26774168271267
30 -4.77220276806501
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.24695391041536
1 3.4372891319353
2 3.34726087438465
3 2.94466413764118
4 2.46927069179518
5 2.47380979118702
6 2.58442913824526
7 2.79678167941762
8 2.79522239496111
9 2.53943267150384
10 2.28234144607709
11 2.18550589876962
12 1.85641287598675
13 1.67724011951219
14 1.30414701743131
15 0.982148221317759
16 0.644958316785035
17 0.380556629118718
18 0.0229928249132474
19 -0.349314905330203
20 -0.692091492374752
21 -1.12326435453718
22 -1.59396252902308
23 -2.03361640201816
24 -2.41606930326657
25 -2.61136485995127
26 -2.73263497263907
27 -2.83906256292075
28 -2.87891002433676
29 -2.80315864649956
30 -2.58452359016943
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.23836336370171
1 3.57096270246955
2 3.36489403902768
3 2.92333964948468
4 2.43758155617994
5 2.49390930554793
6 2.84148026767052
7 3.09967773639633
8 3.00080785550192
9 2.90322261962759
10 2.6788366910967
11 2.30501638565923
12 1.83659257570526
13 1.60599480047125
14 1.44811098686309
15 1.38750925256855
16 1.21920848871207
17 1.05219632736133
18 0.895612576495971
19 0.735245399802453
20 0.522858533714187
21 0.268565219741001
22 0.101604642599762
23 -0.0947058952141671
24 -0.209656634533719
25 -0.310669398041419
26 -0.424804187102746
27 -0.516728396169777
28 -0.657515985241863
29 -0.810604386841765
30 -0.996109271904558
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.10263793495394
1 3.29787943130897
2 3.22110521734943
3 2.65640308291741
4 2.07056063121958
5 2.13091903559281
6 2.31548987329776
7 2.66675769302061
8 2.91099721452565
9 2.73169573336687
10 2.2871784084853
11 2.0396934564786
12 1.72008824009763
13 1.3197474628178
14 0.951135925120324
15 0.654757940997278
16 0.493039018635017
17 0.250233770041421
18 0.0254704486299975
19 -0.343432712165008
20 -0.665281800279937
21 -1.00661868486592
22 -1.32656045043467
23 -1.67658987791278
24 -1.96526501552491
25 -2.35224957850214
26 -2.62797642350247
27 -2.75214112885767
28 -2.87235555271017
29 -3.01625909475871
30 -3.03649352728145
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.16749367737468
1 3.24314660123996
2 3.20548254225579
3 3.09355939476751
4 2.88754468000039
5 3.15535257312749
6 3.51652554570775
7 3.86193114005424
8 4.0652647468541
9 4.18243235159311
10 3.86283180538173
11 3.47958871797238
12 2.91183959181487
13 2.43798405468395
14 1.95576986891378
15 1.53247864451528
16 1.10719070829855
17 0.804143276981128
18 0.53726070728934
19 0.206293987352138
20 -0.0553724916523759
21 -0.312519724292358
22 -0.484566488755156
23 -0.641998732448959
24 -0.916931627628173
25 -1.21564743347022
26 -1.43148023177601
27 -1.64513859504579
28 -1.87116957994648
29 -2.03135370340875
30 -2.26132567181119
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.19023144320537
1 3.37305122937865
2 3.34718277380933
3 2.96007615967591
4 2.57559385002001
5 2.63851803887363
6 2.78102854227027
7 2.89338314415446
8 2.94913297790344
9 2.54522005182674
10 1.91738388913343
11 1.27331176216109
12 0.735806251677838
13 0.239566480665623
14 -0.285358472897176
15 -0.786282347516195
16 -1.28083873122012
17 -1.69508119571943
18 -2.10111237638372
19 -2.48206090857351
20 -3.03962951251509
21 -3.49875334072108
22 -3.87730260188274
23 -4.17366346046544
24 -4.53234946663551
25 -4.86755365230878
26 -5.22419325232656
27 -5.6140211519146
28 -5.85802211336957
29 -6.11310028420721
30 -6.3638752729285
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.20071158602178
1 3.43908993027455
2 3.3692827426027
3 3.21053286537994
4 2.80328715382896
5 2.84476903775921
6 3.24970991022379
7 3.64368525461512
8 3.88349396782919
9 4.01858628342188
10 3.71277576024668
11 3.41642199291688
12 3.03896160236265
13 2.2995038542924
14 1.46005247893901
15 0.649155617377911
16 -0.0215474568158882
17 -0.460012926265614
18 -0.661760403610414
19 -0.905148581115162
20 -1.30012021735226
21 -1.80043079628738
22 -2.43340901686297
23 -2.90669859340724
24 -3.47185980133338
25 -4.11353449303349
26 -4.67523454779391
27 -5.49405041556349
28 -6.15496895458227
29 -6.65396015271121
30 -7.23698038946156
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.18257084805207
1 3.52339584012743
2 3.35653432298624
3 2.9623816324969
4 2.52937797767443
5 2.79394542622825
6 3.00046866769239
7 3.17700371286396
8 3.26040120499912
9 3.14769672409511
10 2.75369526305215
11 2.34522738969776
12 2.30325728909273
13 2.17014296956825
14 2.02111072081234
15 1.73203321370482
16 1.32822580572247
17 1.05904141683431
18 0.805397632423727
19 0.547408718794289
20 0.017634878593789
21 -0.49510637111276
22 -1.18855250907301
23 -1.7959098027239
24 -2.38965414791848
25 -2.91946187302547
26 -3.44005249853395
27 -3.89418200852808
28 -4.25454685945926
29 -4.56380422963996
30 -4.95826778418314
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.18867270303462
1 3.58541687293996
2 3.49056063025055
3 3.27386708344263
4 2.81931279076928
5 2.95540572938961
6 3.35373749162656
7 3.60881652966986
8 3.77044196961317
9 3.36136910923578
10 2.48115894707601
11 1.78036085484448
12 1.27190781405124
13 0.855253172050922
14 0.448314301804674
15 0.178717353812914
16 -0.15931897400673
17 -0.44757818582724
18 -0.768003726175069
19 -1.02697708383228
20 -1.2144119488007
21 -1.50914562548932
22 -1.73072712464116
23 -2.00697150217114
24 -2.31446655272023
25 -2.72705612081887
26 -3.01238347245125
27 -3.26823076805715
28 -3.38656979873753
29 -3.34128187834605
30 -3.28732190414005
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.24728230480185
1 3.56217958045357
2 3.28061953757334
3 2.73819938895678
4 2.48094774549575
5 2.80923328482647
6 3.10225974247042
7 3.23203799891456
8 3.24849367287121
9 2.87694824694187
10 2.16389389686034
11 1.46606049465341
12 0.883644952865286
13 0.0754749464595417
14 -0.663489272885114
15 -1.47310840938973
16 -2.27452816919252
17 -3.05974364533624
18 -3.87987429865571
19 -4.72613832514982
20 -5.62218152937971
21 -6.54894256311977
22 -7.53161557687472
23 -8.47826497790424
24 -9.34369818882392
25 -10.1038488878463
26 -10.9014796179842
27 -11.6574105769599
28 -12.4578836470611
29 -13.2898184367124
30 -14.0542811293109
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.17594972908783
1 3.26598368263449
2 3.17828587270552
3 2.86219244368742
4 2.60189735775275
5 2.6762748133405
6 2.84725682918307
7 2.92036360368658
8 2.76550345394461
9 2.27816855356931
10 1.69855846527239
11 1.0229590683106
12 0.479958952599052
13 0.122768585503882
14 -0.378194503548588
15 -0.828844246939193
16 -1.32614740231054
17 -1.6056182078136
18 -1.98271250865969
19 -2.27023116355695
20 -2.59750363269372
21 -3.06633100969377
22 -3.51852769036724
23 -4.00597010408543
24 -4.58313226477771
25 -5.00841254212553
26 -5.44092756470542
27 -5.84498631401539
28 -6.24903972483011
29 -6.49703178477412
30 -6.62852039021315
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.1471706609141
1 3.51539438440282
2 3.64435064421349
3 3.60896952152205
4 3.25617386575913
5 3.52892069316441
6 3.82793233628832
7 4.20599849048635
8 4.21319042179485
9 3.8523756009872
10 3.27194626068075
11 2.6007377175432
12 2.05931932549475
13 1.6384497694053
14 1.17711362672764
15 0.694062667073549
16 0.127366940212983
17 -0.484451379038601
18 -1.13701814012514
19 -1.59429127328359
20 -2.02015375536049
21 -2.37472949100823
22 -2.63244025875285
23 -3.01180068777272
24 -3.5715893479059
25 -4.09532725813891
26 -4.60443218573339
27 -5.07022024714398
28 -5.53385632010399
29 -6.00450779207297
30 -6.40923950213778
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.21225279878247
1 3.45360580210673
2 3.3453186226945
3 2.96839787511137
4 2.57457933759363
5 2.79486308847931
6 3.17187901066598
7 3.2921670602504
8 3.32513173557279
9 3.04523581095121
10 2.42182664861377
11 1.48753009716254
12 0.709214925404043
13 0.174914185952971
14 -0.389997898957914
15 -0.82691205694274
16 -1.23053649567932
17 -1.56010267423285
18 -1.93268940655259
19 -2.27680176447911
20 -2.65478166933244
21 -2.96302189279687
22 -3.30658517820139
23 -3.70180571191814
24 -4.08625015989258
25 -4.57567966909358
26 -5.17720075872927
27 -5.63752012932346
28 -5.95861482330606
29 -6.11662934777053
30 -6.29065135214519
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.30504335901021
1 3.55018026079729
2 3.50953800981822
3 3.22050704713977
4 3.0449908302986
5 3.3285134486166
6 3.60874619017057
7 3.70975389703408
8 3.81540005889544
9 3.76477126664896
10 3.50944218494756
11 2.88179480567844
12 2.05685743144242
13 1.17395141432394
14 0.38824922572179
15 -0.320665702919177
16 -0.810380070535029
17 -1.12561169740906
18 -1.48167187456949
19 -1.62194777667917
20 -2.04600070729573
21 -2.41733788790583
22 -2.71671797988666
23 -3.02678301084159
24 -3.27885510993402
25 -3.43371599428712
26 -3.75359572822111
27 -4.02464564005558
28 -4.26488138897884
29 -4.40592261950729
30 -4.42553650723244
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.20345343032751
1 3.464350420382
2 3.56111948281954
3 3.22409524995011
4 2.7954571691677
5 2.97253494345611
6 3.05908293878831
7 3.16532898506809
8 3.0541808988132
9 2.90764447847027
10 2.54341737848869
11 2.07373868182782
12 1.74493590567592
13 1.44468823687344
14 1.0471518020813
15 0.75863752621464
16 0.439121556978245
17 0.337629409564375
18 0.0503650667829518
19 -0.00180807984912157
20 -0.027982038491194
21 -0.0602737909442776
22 -0.0793422324978845
23 0.0168317259593618
24 -0.0326912437299711
25 0.0957503842246403
26 0.26756025531996
27 0.458864276843919
28 0.569729441594472
29 0.996287625261473
30 1.51831937722812
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.19003008525881
1 3.38769431917336
2 3.30422275138175
3 2.94981022894076
4 2.62197019727923
5 2.83508446543831
6 3.174900316431
7 3.60384204079915
8 3.92478862551269
9 3.65066278711092
10 3.20590987365765
11 2.80645728317654
12 2.22444027513004
13 1.64033023368235
14 1.00033460994206
15 0.376192766779454
16 -0.215490190923234
17 -0.8562159474402
18 -1.19929527005796
19 -1.40688161275733
20 -1.71485740814452
21 -1.83861761048186
22 -2.07084954183742
23 -2.14230855857828
24 -2.30816010297638
25 -2.54590097709879
26 -2.82080366165232
27 -3.07832969045168
28 -3.3763179502419
29 -3.85771326674262
30 -4.16767963659379
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.22148323543619
1 3.624654038783
2 3.59180393781826
3 3.35981141357482
4 2.888642072201
5 2.83962638225668
6 3.05629243306505
7 3.17131029054877
8 3.1351112845348
9 2.75989271150348
10 2.26232421171523
11 1.60603957714114
12 1.13012053809832
13 0.699141879567321
14 0.314860091783634
15 -0.0964770872199203
16 -0.506377082364924
17 -0.837675037341393
18 -1.34804589867318
19 -1.97193325286919
20 -2.52645938264377
21 -3.09931647176945
22 -3.6800484121525
23 -4.16565258369068
24 -4.63953914881153
25 -5.05863860249609
26 -5.51629974532679
27 -5.87874268225666
28 -6.28195882059583
29 -6.67518150112647
30 -7.07958653302954
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.29236349931218
1 3.5999142515781
2 3.41740036459404
3 2.86314163007309
4 2.27571735417069
5 2.51539740471623
6 2.62257098188262
7 2.86412932110173
8 2.97270425431672
9 2.57770376294302
10 2.01738242197201
11 1.36340824242867
12 0.695432062893639
13 0.0552027358224123
14 -0.497007292177651
15 -0.932156207091975
16 -1.24556733465524
17 -1.47804214752654
18 -1.73002118776528
19 -1.87718088909243
20 -2.07210763707602
21 -2.25923492948193
22 -2.5335632899317
23 -2.65955854813056
24 -2.81756279544134
25 -3.05630924142608
26 -3.20153038332154
27 -3.28292963876332
28 -3.28250747101092
29 -3.19326995065376
30 -2.82190014298023
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.19747644648137
1 3.56188377264743
2 3.73162433236986
3 3.62233309887201
4 3.27333501147664
5 3.47935335735101
6 3.64643747580119
7 3.61912738882679
8 3.61483408033078
9 3.3595221626464
10 2.85816720337486
11 2.33015187480342
12 1.62052728346305
13 1.01585111512817
14 0.219652383332448
15 -0.537211206073938
16 -1.25999580758964
17 -1.93811688497134
18 -2.59739797091654
19 -3.18971062414939
20 -3.73404315982302
21 -4.38898059792792
22 -4.95478890462615
23 -5.53606960394033
24 -6.10888370129149
25 -6.53593044149227
26 -6.8631904186469
27 -7.03221297677458
28 -7.02300511245718
29 -6.99267527205718
30 -6.98941748258777
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.27235665625399
1 3.48731388648863
2 3.44895213987448
3 3.07247898845007
4 2.69293147309517
5 2.83064025477771
6 3.18498873802112
7 3.53111504739946
8 3.85964477750783
9 3.86819168270936
10 3.54629497874108
11 3.18263871177521
12 2.77572964691896
13 2.01870612116628
14 1.23466143918998
15 0.447671732471068
16 -0.236538178955458
17 -0.974938623608944
18 -1.57481562834484
19 -2.25805825022322
20 -3.01232748020402
21 -3.6566110175089
22 -4.34367686604822
23 -5.00086774381048
24 -5.63359107096029
25 -6.28786175276675
26 -6.91317279854238
27 -7.54280957758277
28 -8.12941707471315
29 -8.65517783335387
30 -9.15196991149471
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.15900021427219
1 3.50131606044441
2 3.49475157225075
3 3.48274598221838
4 3.22751940855089
5 3.30997157903329
6 3.5941817048898
7 3.90111477701382
8 4.13889156503974
9 4.07364446980929
10 3.67143757105534
11 3.18481387161063
12 2.68075841672099
13 2.04692972946452
14 1.52404727180962
15 1.0489008522544
16 0.733510225176447
17 0.627025638768529
18 0.289375285407425
19 -0.015373566442225
20 -0.104843393828382
21 -0.280628417628568
22 -0.450192028496234
23 -0.672858149309572
24 -0.904764042417673
25 -1.05951083627853
26 -1.28074184026882
27 -1.47888058656924
28 -1.73476825429059
29 -1.83639038959852
30 -1.7867496417226
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.30743720255056
1 3.58082625213491
2 3.50315433805717
3 3.01610385131588
4 2.68360044004426
5 2.71784760287764
6 3.07998284066264
7 3.11009333650181
8 3.00389026080518
9 2.72912651698347
10 2.23376273686798
11 1.6671914607707
12 1.11683646587346
13 0.546668167325418
14 -0.0128867308494716
15 -0.598228881194428
16 -1.20744073487672
17 -1.66122450929332
18 -2.10887581768505
19 -2.50123559383777
20 -2.90943515771185
21 -3.34474408986385
22 -3.74433213905204
23 -4.06629067370337
24 -4.29091401018858
25 -4.43983404670865
26 -4.5410542027781
27 -4.58587503183663
28 -4.55791957957384
29 -4.56153300486558
30 -4.58839957060387
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.15971734248469
1 3.43631681304463
2 3.52214995052491
3 3.48884567543138
4 3.55864673637109
5 3.86569942844185
6 4.39376295870077
7 4.58632035668749
8 4.24715203215455
9 3.60110802330973
10 2.78667848797344
11 2.19092550769133
12 1.75607917956343
13 1.50762777545593
14 1.20737889447147
15 0.79863718747457
16 0.332058813841936
17 -0.297744908763752
18 -0.970123775777489
19 -1.61248275743039
20 -2.15340021598663
21 -2.63767533540717
22 -3.01494497932359
23 -3.25376296150401
24 -3.54517011336481
25 -3.68478055038506
26 -3.81850068645979
27 -3.64819342679067
28 -3.32441882848524
29 -2.96622106433195
30 -2.4804623600436
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.18236830805734
1 3.60591837376914
2 3.43494652255405
3 2.96556083583157
4 2.44797028961418
5 2.78588010968551
6 2.9535050443262
7 3.21502690365318
8 3.40301587635375
9 3.25670267137562
10 2.93658658874431
11 2.67341420033525
12 2.52684627544498
13 2.52562616853564
14 2.37136918837538
15 2.23744087351721
16 1.90676288282831
17 1.64839432087686
18 1.28668959816896
19 0.830683016816169
20 0.371816041419423
21 -0.12554104290764
22 -0.51868798946647
23 -0.913265785115039
24 -1.3333960487742
25 -1.68836739035447
26 -2.00004711378656
27 -2.33967515325499
28 -2.67383657090725
29 -3.01560049964795
30 -3.32417927580019
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.16324788416005
1 3.33727676623347
2 3.28357765281393
3 3.08169586806479
4 2.85472818078129
5 3.03603803028654
6 3.33809403622476
7 3.48678893346966
8 3.43093739279622
9 3.07417079914504
10 2.53993552095355
11 1.9950404520638
12 1.40405686586404
13 0.749415628265824
14 -0.0254521928980527
15 -0.635803451717051
16 -1.21663775285042
17 -1.68462005636761
18 -2.25192646523125
19 -2.8563358568304
20 -3.40497290272789
21 -3.89204062934179
22 -4.34152953591255
23 -4.90293097969072
24 -5.43454089927481
25 -6.08355321402044
26 -6.63832544682322
27 -7.27658245674952
28 -7.79471560745224
29 -8.28896596492956
30 -8.69549872796066
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.15552402954046
1 3.30617222099564
2 3.28710627269732
3 2.84162169832865
4 2.35288302606125
5 2.42876576632933
6 2.85134707730503
7 3.06634598207316
8 3.0617419951007
9 2.94430501816059
10 2.60094146615661
11 2.23515875603842
12 1.74271043661541
13 1.54250449156651
14 1.41907468440006
15 1.2374650386004
16 1.0080347551655
17 0.813847778570333
18 0.794682948818833
19 0.678104756514436
20 0.5902678219141
21 0.31204310000107
22 0.0710534919907282
23 -0.24432097970826
24 -0.546097895396864
25 -0.891308379901659
26 -1.17511864869977
27 -1.2670674848378
28 -1.39470104576504
29 -1.38755788223195
30 -1.45798864214565
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.20592486757385
1 3.70053093605731
2 3.91981006559983
3 3.71588465289841
4 3.33220924773299
5 3.53924906367611
6 3.96533757669683
7 4.03522573189177
8 3.90796319898742
9 3.65331593118673
10 3.43013234267601
11 2.94923992542948
12 2.47402155928846
13 2.21945671409904
14 2.0468156196888
15 1.8003537327481
16 1.49593227541784
17 1.14196545285625
18 0.67889274364372
19 0.209064419044454
20 -0.351463333040799
21 -0.921889791729331
22 -1.59465410915456
23 -2.12381996518187
24 -2.59412507403086
25 -3.16270946187215
26 -3.58250046852006
27 -3.88015336061995
28 -4.056354521847
29 -4.25623876198173
30 -4.42745253703196
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.19615808451591
1 3.46492902344227
2 3.63648820723134
3 3.28013143168514
4 2.77769345427
5 2.75550728631558
6 2.91823996756328
7 3.22790533124633
8 3.35034302257191
9 3.21763122254509
10 2.55001126784635
11 1.90185560757571
12 1.47061072631432
13 1.26810327590489
14 0.996904281359633
15 0.786033176439725
16 0.484860560781314
17 0.194301469537546
18 -0.122725117210232
19 -0.443896281061875
20 -0.787073695864887
21 -1.08915259691076
22 -1.36285624676139
23 -1.62821580543145
24 -1.78281729273337
25 -2.04704133663426
26 -2.36096648658061
27 -2.8115365496988
28 -3.24265533420487
29 -3.7043697379633
30 -4.14996909472335
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.14192543122278
1 3.54986674910523
2 3.65750558889465
3 3.51718612994615
4 3.23239930956354
5 3.65681978814857
6 3.95555676108845
7 3.9859807866112
8 4.04670939617814
9 3.81631240086577
10 3.31111430792319
11 2.79741081073426
12 2.20764455741034
13 1.6431384783209
14 1.01689005577138
15 0.49060097998783
16 -0.0355384016612739
17 -0.400068226473557
18 -0.833397399332828
19 -1.20560408220292
20 -1.53081662982135
21 -1.76283577108975
22 -2.09497997309443
23 -2.33846974244813
24 -2.48575081829219
25 -2.52544629412209
26 -2.37622215691852
27 -2.1609144738677
28 -1.99323060942778
29 -1.72599652339685
30 -1.32867446186322
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.19749016228122
1 3.51378019813834
2 3.4861802092133
3 3.19141821761272
4 2.64691263650349
5 2.83456757775363
6 3.02914599420624
7 3.65829400979093
8 4.12036538998164
9 4.02367851897517
10 3.77413924826297
11 3.43344110214686
12 3.0460168732772
13 2.53709567843392
14 2.00048335977506
15 1.44618635477152
16 0.865713245205502
17 0.554749665973477
18 0.418772550600428
19 0.372976597223278
20 0.0376865255755536
21 -0.230050353265161
22 -0.569703727083578
23 -0.82861722881861
24 -1.06703309448832
25 -1.35166280507178
26 -1.6927000080584
27 -2.14729836993064
28 -2.62155069046874
29 -3.03031721489345
30 -3.49404264922495
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.14024525898101
1 3.50508737511135
2 3.58533929813173
3 3.2763227468624
4 2.84645014292263
5 2.92392498168181
6 3.17729650601709
7 3.42406598803465
8 3.52051605696797
9 3.22336224776597
10 2.83017057237698
11 2.51325476423384
12 2.11384140708765
13 1.77481216333843
14 1.46723517817499
15 1.17101113721786
16 0.928279995291625
17 0.630402326621592
18 0.297160141878445
19 -0.00772911307535473
20 -0.234978532671722
21 -0.554814933743792
22 -0.910106762548104
23 -1.26346199801596
24 -1.58081444205505
25 -1.84136683661213
26 -2.09808109098323
27 -2.30789049695353
28 -2.45249631176332
29 -2.58050542384644
30 -2.68791163141305
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.297576441558
1 3.58530527998065
2 3.54906749044109
3 3.13493754080783
4 2.77685862505186
5 2.83347539252954
6 3.04051859461789
7 2.91804069366523
8 2.73159573538923
9 2.42594578069676
10 1.8920367822382
11 1.35827286825906
12 0.861947123981425
13 0.524315949885146
14 0.114005982142963
15 -0.218944900179467
16 -0.501762656706781
17 -0.790619096398387
18 -1.20041595866733
19 -1.47176947638277
20 -1.76303729613325
21 -1.83801446389926
22 -1.96243065910797
23 -1.95513559272187
24 -1.61407805198499
25 -1.12315458901753
26 -0.45924212381499
27 0.15628656238769
28 0.719698354748347
29 1.27710040156339
30 1.94108554168122
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.26260363091365
1 3.52223075824414
2 3.60048149389217
3 3.32858614663295
4 2.89576593795448
5 3.14917879844985
6 3.34074742559132
7 3.44568755663025
8 3.28353312940133
9 2.99957095079521
10 2.54470651902277
11 2.35364256351762
12 2.05435273802858
13 1.68598879263853
14 1.29404440488923
15 0.916805263290346
16 0.638528577022877
17 0.328400033199573
18 0.0776512973306094
19 -0.150204075551457
20 -0.594993613783481
21 -1.07125311203353
22 -1.53028150720028
23 -1.83226631434059
24 -2.31327166541135
25 -2.40101574255385
26 -2.527828207099
27 -2.7909639822884
28 -3.18207171950109
29 -3.43079896722793
30 -3.57236435635028
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.17619337355697
1 3.41300984233741
2 3.32529747209464
3 3.13794193539374
4 2.95915320001895
5 3.27840346387133
6 3.7669068234144
7 3.89195581828661
8 3.74093247719533
9 3.10587202677153
10 2.37857805616077
11 1.6899825956326
12 1.14926326880205
13 0.783353172378439
14 0.399210439324413
15 -0.152709330015867
16 -0.644538516468456
17 -1.25138846862369
18 -1.64362163069398
19 -2.0571132262926
20 -2.52472966771518
21 -2.84958338056977
22 -3.24538688957392
23 -3.5848573833407
24 -4.04722645515617
25 -4.51362070038684
26 -5.05769584892818
27 -5.54195469318632
28 -5.96469073159124
29 -6.50469460454975
30 -7.03309423031099
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.22182822800266
1 3.5358182970543
2 3.48945828581842
3 3.12852150010081
4 2.71573499199141
5 3.02642036639345
6 3.33607968869075
7 3.64185644194134
8 3.55666015718624
9 3.15441752020475
10 2.53171269410897
11 1.77228787694595
12 1.18697411579767
13 0.839105140031275
14 0.614374781943297
15 0.454535372971755
16 0.302511287695749
17 0.125397280914218
18 -0.10568781593677
19 -0.296743870214595
20 -0.586443250172229
21 -0.964757917061386
22 -1.30192009232615
23 -1.62546308827148
24 -2.02187929041301
25 -2.2360043384275
26 -2.5022687354805
27 -2.81729884964638
28 -3.12142620156005
29 -3.39678648056747
30 -3.63863355294511
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.18593697916499
1 3.57772186857364
2 3.68810464936389
3 3.54897854538066
4 3.37764852177317
5 3.32277718016246
6 3.40490996150839
7 3.5318625046779
8 3.61319616228
9 3.23729420697272
10 2.73002845802808
11 2.24738075717285
12 1.80401855013148
13 1.09368109453418
14 0.37075542790538
15 -0.269067122044294
16 -0.913344815475011
17 -1.56957888029176
18 -2.21402213249897
19 -2.81714518801252
20 -3.51312066705275
21 -4.49191165317866
22 -5.4482212495478
23 -6.30450349285845
24 -7.04788063271696
25 -7.85519014461573
26 -8.61058966272473
27 -9.23200609915845
28 -9.68948017600804
29 -10.1931947322936
30 -10.6748611997309
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.11740885465685
1 3.52399538579999
2 3.52135233702854
3 3.25799652240504
4 2.85404389402577
5 2.88079243052741
6 3.08068010325505
7 3.39572427082151
8 3.47187705255184
9 3.210313637999
10 2.7166047021688
11 2.11355388983079
12 1.56651216526721
13 1.40886893131095
14 1.16583768944948
15 0.878481969308032
16 0.534911539642865
17 0.171084232144965
18 -0.164148638344956
19 -0.511843622416997
20 -0.875540890563444
21 -1.15295322599313
22 -1.30607400117506
23 -1.47525044858342
24 -1.50341566355548
25 -1.42392405135202
26 -1.24266210835187
27 -1.03588007848582
28 -0.794998981587826
29 -0.341313874765383
30 0.0669532957273589
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.24877077298323
1 3.54349595352044
2 3.28026680296259
3 2.56797890503036
4 1.94122655260413
5 1.88480774126879
6 2.22074472771084
7 2.91135117154016
8 3.20070103367757
9 3.05147098765805
10 2.87258670549632
11 2.66600691878261
12 2.45711864230411
13 2.24379782192076
14 1.89049973717341
15 1.54232524254387
16 1.30866841469028
17 1.01539934737612
18 0.732379438911231
19 0.423775735505782
20 -0.100840448236799
21 -0.570271582152186
22 -1.12102178505761
23 -1.73145208456576
24 -2.15120181974202
25 -2.52506658140016
26 -2.90964322118562
27 -3.25653764473701
28 -3.57277051532166
29 -3.98437972859981
30 -4.46065454542365
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.24721523742708
1 3.6118125049295
2 3.73354180163194
3 3.74123085709502
4 3.57349524017092
5 3.74730668419843
6 4.089118063817
7 4.14172659710229
8 4.01450122404774
9 3.94502612114962
10 3.61240386060045
11 3.20083632255741
12 2.7741917210648
13 2.33557682247239
14 1.8485815468192
15 1.24427747218486
16 0.720693905210233
17 0.235389344137152
18 -0.313177455847608
19 -0.790601306771402
20 -1.23686604389191
21 -1.53565873718966
22 -1.78199089627964
23 -2.08395690564556
24 -2.50296806224901
25 -2.76337844455008
26 -2.91457910003169
27 -3.0784653586792
28 -3.21992836145053
29 -3.51142211387678
30 -3.82720915470354
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.143246780191
1 3.46696416012118
2 3.52721354136616
3 3.27874177180542
4 2.8915861170242
5 2.78526946133222
6 2.89057479673792
7 2.88559000988863
8 2.96398884115795
9 2.52974698422707
10 2.05102014275265
11 1.57508591714215
12 1.17284067546351
13 0.736550790218951
14 0.0632915894412669
15 -0.620420201553426
16 -1.27271372565546
17 -1.70479745218856
18 -2.27059963423005
19 -2.79947401543509
20 -3.19882005926239
21 -3.57029036217388
22 -3.7017546240347
23 -3.83382280421712
24 -3.90452560601807
25 -3.86164362330001
26 -3.9875106575752
27 -4.16529347296852
28 -4.46876422701627
29 -4.86031921581467
30 -5.16677533366341
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.22451927721345
1 3.55501936665512
2 3.54892553542044
3 3.28014752432306
4 3.10200355619514
5 3.13945434276761
6 3.17363288275956
7 2.98285231898873
8 2.59731093408754
9 2.07098747342404
10 1.31317573765585
11 0.357433581500569
12 -0.397145669744077
13 -1.19876944982367
14 -2.00551707354922
15 -2.76411853141012
16 -3.65042382890629
17 -4.4402252094096
18 -5.34863556667717
19 -6.17829646234541
20 -6.96681045809308
21 -7.66391265763552
22 -8.35652082517683
23 -9.03476882636191
24 -9.71621685280687
25 -10.569427593049
26 -11.1994322550078
27 -11.7054897725918
28 -12.2100645764022
29 -12.5539138567601
30 -12.8866367906715
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.20884549673435
1 3.53743325828331
2 3.51952529541916
3 3.30816995596095
4 3.26088503293198
5 3.62025172496509
6 3.75606414923615
7 3.79891205428855
8 3.7308535809982
9 3.19242436191827
10 2.57087298802083
11 1.95797824175314
12 1.29464578153262
13 0.861373086258622
14 0.269189015477371
15 -0.270133415294239
16 -0.883293713969257
17 -1.62015728369688
18 -2.31812573462269
19 -2.87438548760534
20 -3.42976762309325
21 -3.79495326771338
22 -4.25632349802494
23 -4.7782485974826
24 -5.21212991063433
25 -5.67110738445794
26 -6.2545832021022
27 -6.68110382035398
28 -6.88701285471245
29 -6.98708141883192
30 -6.95171624823876
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.15672726049691
1 3.48476433693207
2 3.64352526940663
3 3.1646828012003
4 2.69627257950396
5 2.82924885247957
6 2.85960603577768
7 2.98339959055398
8 2.95742886443493
9 2.89817126003854
10 2.77116247370424
11 2.52092620331617
12 2.20855549429144
13 1.84432981084735
14 1.28929210107618
15 0.875182487262235
16 0.399558354356182
17 0.00951476190926748
18 -0.372465555061735
19 -0.696775354307011
20 -0.766793024610502
21 -1.01323104423427
22 -1.26442814993951
23 -1.53790906830235
24 -1.71754832292761
25 -1.9228481704626
26 -2.28875871354786
27 -2.62050462511183
28 -3.04047069607677
29 -3.36591753334371
30 -3.5388927683062
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.17180521676025
1 3.44569653722493
2 3.48965519982145
3 3.19383798418475
4 2.63046854515065
5 2.57042892879648
6 2.80967387284532
7 3.17334734065721
8 3.46516641703542
9 3.53575541901495
10 3.34741802358004
11 3.05597242524847
12 2.75368141770407
13 2.37787401446449
14 1.96373421868251
15 1.40294378565253
16 0.835860748548406
17 0.25961108209324
18 -0.218045859798265
19 -0.609388088684172
20 -1.02545262399604
21 -1.41388898950888
22 -1.74811758238937
23 -2.17600037377118
24 -2.64164656641372
25 -3.14983682358037
26 -3.62298470808618
27 -4.03870776201693
28 -4.28877080185365
29 -4.67828968314243
30 -4.94806589146137
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.20359261924865
1 3.54870677249656
2 3.52760584077912
3 3.16996601351818
4 2.78869956030409
5 2.83418459475225
6 2.91886139513687
7 3.17627742200661
8 3.64522972756195
9 3.72136014682761
10 3.37166315508966
11 2.83229828958143
12 2.17356565262155
13 1.44821500852428
14 0.724548388555776
15 0.143211855180031
16 -0.351023603415996
17 -0.741692735705517
18 -0.974247881678963
19 -1.14697981526522
20 -1.56148472782162
21 -2.08207522378105
22 -2.81665888562907
23 -3.63177323105198
24 -4.46051900493294
25 -5.14141248636489
26 -5.81642123043867
27 -6.52758386687663
28 -7.12326461239678
29 -7.58531689377393
30 -7.89931392506023
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.25182066654492
1 3.48747029230775
2 3.54040068288078
3 3.39180516843871
4 3.06779678727379
5 3.40389771090818
6 3.64942055864865
7 3.43316403094773
8 2.96843732212707
9 2.23710104683572
10 1.4687141504148
11 0.840482670155716
12 0.187280233115763
13 -0.281083016115497
14 -0.744220869911677
15 -1.30499971237714
16 -1.86915770237189
17 -2.31085449412248
18 -2.85996317744002
19 -3.32374662945955
20 -3.64359769547843
21 -3.92610815112358
22 -4.1318590039291
23 -4.29161276798885
24 -4.54556125319664
25 -4.76096839670601
26 -4.95039228017164
27 -5.1410839591922
28 -5.33100601472755
29 -5.47289790121427
30 -5.5389170854341
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.24132699550811
1 3.36392300177804
2 3.1955271740077
3 2.98264801790056
4 2.56984546098134
5 2.48479228433337
6 2.87756858961993
7 2.97424026031443
8 2.86153165499921
9 2.61253401907627
10 2.13402842034567
11 1.81134622973339
12 1.49929819279433
13 1.04822804819066
14 0.672936723376438
15 0.221659742069717
16 -0.244473774895628
17 -0.902863716881024
18 -1.46100290829772
19 -2.01320442005639
20 -2.50510774802161
21 -3.03920184439763
22 -3.6020599009413
23 -4.02729794953356
24 -4.58981595667755
25 -5.05785981371604
26 -5.34898208563257
27 -5.65635396374652
28 -5.8949030418519
29 -5.96505674354486
30 -5.96241459041233
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.18646188622393
1 3.57414114344172
2 3.47865784123056
3 3.20436848804614
4 2.88429839697461
5 3.03690448872268
6 3.29233666390316
7 3.6931183956252
8 3.82848793760308
9 3.68324997186741
10 3.25032231549304
11 2.76874453736289
12 2.15174177876422
13 1.77385402239465
14 1.38227345965659
15 0.90935810782103
16 0.383185911808114
17 -0.173608329931231
18 -0.799104659204382
19 -1.38296356749085
20 -1.91451350606829
21 -2.49834677925025
22 -3.15170861274379
23 -3.81058327829831
24 -4.3479254207879
25 -4.9355375839871
26 -5.55676114495228
27 -6.19083850209969
28 -6.71648935518963
29 -7.29450507397426
30 -7.7800184584077
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.2090792337642
1 3.57803681833091
2 3.42488738566317
3 3.05039389455541
4 2.5881159736733
5 2.541716262837
6 2.61676830763924
7 3.02242807812499
8 3.19621807779529
9 2.93022364539252
10 2.5853530137485
11 2.17723945873797
12 1.90143690464535
13 1.96883813325822
14 1.9360179509731
15 1.74032647746381
16 1.54550920457717
17 1.27655816091712
18 0.865983380823707
19 0.413135562933256
20 0.0811539179846985
21 -0.482147197417062
22 -0.978822834143401
23 -1.52762102479447
24 -2.03464568059764
25 -2.42333317613294
26 -2.76598051610078
27 -2.99442183192984
28 -3.39434945557791
29 -3.71918013866946
30 -4.02171913201289
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.17840504460295
1 3.32806872346497
2 3.21287126510826
3 2.84164383195563
4 2.4094748768541
5 2.66631252046734
6 3.04605829631778
7 3.21671706976004
8 3.21013899888012
9 2.99755835066798
10 2.57057178280824
11 1.99414558102586
12 1.53557751263941
13 1.03378548671837
14 0.644273882552918
15 0.126668355083849
16 -0.4260863968858
17 -0.888706025675811
18 -1.47822159933613
19 -2.13400420169159
20 -2.86699819005482
21 -3.44519700058304
22 -3.91392492691997
23 -4.27331999186066
24 -4.69065032100262
25 -5.06542464625595
26 -5.48142831770259
27 -5.90176655432054
28 -6.35770185071481
29 -6.81077426255114
30 -7.26021899610745
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.21840352883872
1 3.70698696350594
2 3.67587204997295
3 3.17162395778123
4 2.66086634402351
5 2.70932383984612
6 2.87600801452574
7 3.10561350017084
8 3.01501954200547
9 2.78075767781054
10 2.41326375854953
11 1.84352868064971
12 1.29125132468223
13 0.905482581181875
14 0.527824977916501
15 0.154090617272384
16 -0.25142650047667
17 -0.565167172125539
18 -0.882083402562184
19 -1.18135143586495
20 -1.63638644285811
21 -2.15624707317419
22 -2.74593937735648
23 -3.08320794593598
24 -3.44393522195908
25 -3.95511988317075
26 -4.25043485710164
27 -4.6409976195129
28 -4.99697181438441
29 -5.41028571822271
30 -5.87804814604961
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.24788602592023
1 3.67539695154164
2 3.90119671243514
3 3.98360513071176
4 4.04581780258038
5 4.22793328416073
6 4.27869161949785
7 4.18866058293433
8 4.07339208350999
9 3.6828592609451
10 3.32746017342238
11 2.89933137940896
12 2.68582040262332
13 2.21767503075228
14 1.78651971194843
15 1.36257969565842
16 0.782939600760987
17 0.249353812611009
18 -0.264529307308827
19 -0.7041181298554
20 -1.39440589853989
21 -2.03414500782573
22 -2.72953823480691
23 -3.45677751426055
24 -4.29526343876135
25 -4.83155861052874
26 -5.32135926348187
27 -5.65295471122999
28 -5.81174946688292
29 -5.87394017058125
30 -5.80570592242433
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.20149425305545
1 3.50043569002809
2 3.59691809346248
3 3.28954658976211
4 2.92525173173142
5 3.06485104589227
6 3.45459811978192
7 3.67427513797445
8 3.90313338105925
9 3.70633457330721
10 2.99532638017098
11 2.253866195297
12 1.66629713384426
13 1.07781881980452
14 0.244883782396672
15 -0.555270908277276
16 -1.39574030880566
17 -2.0479911944179
18 -2.7040371010269
19 -3.26896128304305
20 -3.98319076761499
21 -4.61494963694786
22 -5.17020818543964
23 -5.65847103991751
24 -6.11038146557429
25 -6.44096619033952
26 -6.76704412174021
27 -7.17873006976956
28 -7.57625503997545
29 -8.03950280338174
30 -8.45116275108579
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.2311621654838
1 3.51970000680733
2 3.46141006162553
3 3.26173118944674
4 2.93844372780531
5 3.34911631987415
6 3.81565370845805
7 3.84165698059908
8 3.70751913141303
9 3.3974915766671
10 3.1881548028063
11 2.87054921925217
12 2.53931707957669
13 2.20647100899784
14 1.85487491791778
15 1.46978247793196
16 1.18545167691915
17 0.78601352038033
18 0.42772207916628
19 0.171809915477805
20 -0.0703806251172825
21 -0.371516616168458
22 -0.683345403046715
23 -1.02759944563736
24 -1.27690236604497
25 -1.61698812643907
26 -1.93402750859225
27 -2.23816366173614
28 -2.49760054302233
29 -2.72635813403797
30 -3.06378450633352
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.11320768988861
1 3.2158728898098
2 2.95217768685882
3 2.57906105420217
4 2.00611276891584
5 2.08985565826562
6 2.22437029493966
7 2.66308526972196
8 2.72729194577514
9 2.49863274432443
10 2.08819433050191
11 1.79343025158835
12 1.60824004871797
13 1.29148759606773
14 0.923736659371798
15 0.579336352189413
16 0.217182641209863
17 -0.0451927965737031
18 -0.345886961239392
19 -0.583825892195705
20 -0.860838690467768
21 -1.13171085102124
22 -1.52969386707573
23 -1.96579726216666
24 -2.4302776294191
25 -2.84898664805625
26 -3.27128338043212
27 -3.74843071228979
28 -4.23932882063055
29 -4.58640686825927
30 -4.92681886582287
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.17014161654052
1 3.60649044400978
2 3.72868929799272
3 3.76856475683068
4 3.66685725561271
5 4.09106262739799
6 4.33900089915192
7 4.19433624816575
8 3.65705643932051
9 2.89700093200921
10 2.00366570086351
11 1.13681188158244
12 0.407956270781575
13 -0.329318620510616
14 -1.07450829421555
15 -1.93108022980167
16 -2.87676666625137
17 -3.72973166425141
18 -4.57971404492252
19 -5.46450911356941
20 -6.39408073072267
21 -7.40127608953073
22 -8.50608810948683
23 -9.54387801293885
24 -10.4531081339948
25 -11.3827410209466
26 -12.2752560934354
27 -13.0189512510273
28 -13.9160756213868
29 -14.6206208917331
30 -15.3614939672944
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.16923268760946
1 3.4520838421203
2 3.27625967217584
3 2.9409295510852
4 2.53789879838113
5 2.65453970840728
6 2.84340704076509
7 2.86711864308718
8 2.76650082210725
9 2.1130386011797
10 1.38715738067517
11 0.780472762890565
12 0.424326498027337
13 -0.0280365661838342
14 -0.581817195794326
15 -1.1154923215907
16 -1.56293818103323
17 -1.83822791506217
18 -2.38322193820842
19 -2.7915601323401
20 -3.11998155951605
21 -3.50629960234522
22 -3.93220686031863
23 -4.29183296723218
24 -4.43954844957618
25 -4.43641409702653
26 -4.47991281688727
27 -4.30037242052549
28 -4.02700819821235
29 -3.81977245323858
30 -3.38584076181253
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.14013402767114
1 3.53626060055387
2 3.26443424834254
3 2.82191286489187
4 2.35266169711674
5 2.42636265150986
6 2.8260314966826
7 3.18810100445391
8 3.37086577832293
9 3.15950836344205
10 2.64034276015565
11 2.03271135854303
12 1.4287390135761
13 1.00943246931251
14 0.546883659245639
15 0.168403758785953
16 -0.229723084764556
17 -0.565920263659274
18 -0.926021170755609
19 -1.2320491642595
20 -1.38882508220427
21 -1.60011941466223
22 -1.82262442593966
23 -2.00026898094444
24 -2.13536318644125
25 -2.27038255645602
26 -2.28267506381373
27 -2.30018736170534
28 -2.42432958518203
29 -2.4760848493453
30 -2.4804381769719
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.21523924467289
1 3.30955390648106
2 3.20160991712012
3 2.86346798708471
4 2.49075254568913
5 2.79999312600326
6 3.24868749433717
7 3.39668706767121
8 3.41866642603618
9 3.29038159985642
10 2.86797368430083
11 2.27343458933819
12 1.81350413171814
13 1.46817604171364
14 1.08820088563917
15 0.664986891631123
16 0.249903764087033
17 -0.0957723864883899
18 -0.255036040446956
19 -0.415513217847682
20 -0.577742520499909
21 -0.813054983119963
22 -1.08792707852085
23 -1.38211880707361
24 -1.69299088457673
25 -1.97422276187016
26 -2.10184845659424
27 -2.10807999419193
28 -2.00988371646983
29 -1.91453865013298
30 -1.76885875646939
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.11569676893092
1 3.61760576435556
2 3.81809306885829
3 3.67894194469433
4 3.51302591987501
5 3.70106313593907
6 4.18823376180651
7 4.42435180252668
8 4.5299835132197
9 3.90899733705099
10 3.29941481917928
11 2.50988117033462
12 1.97870465969107
13 1.55654624362329
14 0.950066749915235
15 0.348285959347361
16 -0.330227731467966
17 -0.892469814541107
18 -1.61948321063439
19 -2.36912764835637
20 -2.92256053739423
21 -3.42456952901446
22 -4.08827763195447
23 -4.62828222404164
24 -5.09413638962342
25 -5.64522195935124
26 -6.17813981316803
27 -6.72788591554393
28 -7.02146101154279
29 -7.08708515268886
30 -7.22035671038646
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.20673896809416
1 3.54362274200776
2 3.59782987920562
3 3.24392231144752
4 2.8634498981406
5 3.19922435741863
6 3.5405391037771
7 3.92583139999585
8 3.87356735060487
9 3.51615158644124
10 2.97251693915456
11 2.52299409067875
12 1.98069893935129
13 1.36407030313588
14 0.718956970748247
15 0.151923783530677
16 -0.296013458806422
17 -0.723908547645815
18 -1.10299723399531
19 -1.49740324571385
20 -1.93533079471818
21 -2.29882233767934
22 -2.67276001437672
23 -3.09729391063186
24 -3.3745483598887
25 -3.64000190531206
26 -3.85429170739475
27 -4.03436116786603
28 -4.22328689319617
29 -4.42222476571991
30 -4.58995008404754
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.1648032645655
1 3.52624412895107
2 3.52851580250501
3 3.25696105755471
4 2.91835835255127
5 2.99679538229072
6 3.29292841599657
7 3.54261278288233
8 3.68004555800632
9 3.41194732501078
10 2.99171846072406
11 2.43337579421137
12 1.90169982268488
13 1.34638439519952
14 0.789445274878886
15 0.309443180200708
16 -0.254812707461802
17 -0.767425878532531
18 -1.25315093373143
19 -1.57003761238242
20 -1.87109446712353
21 -2.08592208914504
22 -2.25426148577242
23 -2.49397805267057
24 -2.71855792783326
25 -2.80686636914912
26 -2.89643987190278
27 -2.94883129394025
28 -3.01141159814637
29 -3.0309221514341
30 -3.13873402164628
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.09732224737969
1 3.41782261696993
2 3.44360992693307
3 3.15367754492395
4 2.64944379307916
5 2.86382087136825
6 3.101554008096
7 3.44025094983191
8 3.5912076581211
9 3.58077263149857
10 3.39728954080452
11 3.09726333822429
12 2.597682824865
13 2.24122445270035
14 1.9389219987219
15 1.58383259917741
16 1.31582941367153
17 1.04934874552463
18 0.913724100991109
19 0.671913820245955
20 0.520409824264574
21 0.351079683224183
22 0.197713006400676
23 0.108084292284548
24 -0.0187220015992047
25 -0.0608165272251728
26 -0.0980031509738879
27 -0.124486610881227
28 -0.084867442238199
29 0.0218078266300417
30 0.0618590032563002
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.19528732614673
1 3.38186592587526
2 3.41184328769518
3 3.26542166509785
4 3.06414091040165
5 3.41095843422918
6 4.18949449565726
7 4.36829733614167
8 4.0096721227765
9 3.58947165389437
10 3.08866000460511
11 2.40648010051009
12 1.90508391191649
13 1.57209641940941
14 1.38352436040455
15 1.30584906754045
16 1.19068222808659
17 1.17920004116312
18 0.95997645731215
19 0.843311550944335
20 0.777344700358135
21 0.741592791663042
22 0.749498761698119
23 0.810293548511575
24 0.715852891832141
25 0.749487260497297
26 0.824544702059717
27 0.900563094330463
28 1.05668573426045
29 1.18176561138044
30 1.35030713961538
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.15539711701348
1 3.42744914166596
2 3.21016425593751
3 2.62128935880363
4 2.08120533899013
5 2.27343915193964
6 2.74086030170291
7 2.9990783614145
8 3.17049253892265
9 3.10335409806379
10 2.95401457773299
11 2.77751786514565
12 2.39492875766998
13 1.97714263935761
14 1.33592515649599
15 0.690311992928997
16 0.20075404574899
17 0.0694999727884227
18 -0.0391988727680772
19 -0.194529920891373
20 -0.220363757160067
21 -0.384558383959829
22 -0.661062101749408
23 -0.759648056894507
24 -0.997834947850388
25 -1.26996368555816
26 -1.43528281150139
27 -1.57460200808476
28 -1.64058924341493
29 -1.77403664190026
30 -1.78970188705753
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.24279634225108
1 3.48113423094873
2 3.31498680176784
3 2.97874435045267
4 2.54790716662613
5 2.83857754596782
6 3.30301631786512
7 3.69255026396004
8 3.75647911181248
9 3.361474235877
10 2.626963333806
11 1.93682940144677
12 1.28545832698223
13 0.770639739998034
14 0.432742368150945
15 -0.172747305732187
16 -0.756970410439493
17 -1.50223547362721
18 -2.0971278059629
19 -2.6369515973323
20 -3.11837617102406
21 -3.52493564869804
22 -3.89197333375937
23 -4.24323056679397
24 -4.54643340474472
25 -4.82762953096777
26 -5.02968742675212
27 -5.28278096897714
28 -5.42359408774209
29 -5.49508732143531
30 -5.52485324152086
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.11676021558269
1 3.43438279995534
2 3.39277511171444
3 3.24928796290841
4 2.78947801958457
5 2.88481992264006
6 3.13297533287096
7 3.13618871540614
8 3.09942502653999
9 2.70533019844105
10 1.93632560210824
11 1.31687940559367
12 0.826799384965916
13 0.268907501042547
14 -0.377355946701357
15 -1.01001727650826
16 -1.62380098985418
17 -2.30189216920787
18 -2.91146559808972
19 -3.53243699452085
20 -4.05503350606028
21 -4.57981128828639
22 -5.10647309910559
23 -5.52647705095106
24 -5.90637776016932
25 -6.31471361235975
26 -6.60280753871382
27 -6.92847855906467
28 -7.34584772871129
29 -7.82727408860975
30 -8.39731653872072
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.25400235117537
1 3.36100636383284
2 3.23047889179469
3 2.83198072946668
4 2.38120672627208
5 2.71159634510013
6 3.1073491571238
7 3.26782246854925
8 3.26213402556996
9 3.02763883574505
10 2.53042107373378
11 2.11877968502937
12 1.5940324253693
13 1.02659577639332
14 0.544250611080543
15 0.0262257232519527
16 -0.416922200579418
17 -0.731320914635415
18 -0.826252628820209
19 -0.923423370745288
20 -0.99349785823838
21 -1.07662785284958
22 -1.24611966889492
23 -1.25370633066553
24 -1.4024969548559
25 -1.55979659570507
26 -1.58874466569963
27 -1.64200837420383
28 -1.65900825811686
29 -1.57542235165575
30 -1.51613395896609
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.24515551679364
1 3.41905089213498
2 3.56158135079513
3 3.2897546044063
4 2.79910498151256
5 2.96117555551415
6 3.16566357681798
7 3.75053074115278
8 4.32224193980735
9 4.32810124670141
10 4.07628981167387
11 3.70210604274077
12 3.3260058732531
13 2.94172889778062
14 2.44222763645704
15 2.14432884509601
16 1.97921940028971
17 1.81697804312
18 1.73969054483361
19 1.59649184028349
20 1.32492033801521
21 1.09960960366562
22 0.809162875110522
23 0.364198575803629
24 -0.071279862186806
25 -0.425142387196988
26 -0.759013522493964
27 -1.15532639284946
28 -1.49859465748121
29 -1.81672589121045
30 -2.16390690440374
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.22266812776453
1 3.62461862189458
2 3.60574860809971
3 3.40559019050131
4 3.00498265464041
5 2.97669112872086
6 3.19518408220593
7 3.36548435869734
8 3.61684391978339
9 3.42189728090015
10 3.04050416076897
11 2.5715023231583
12 2.04136434624217
13 1.68802946440837
14 1.23700187768708
15 0.7955995601274
16 0.404201467041888
17 0.081761804541836
18 -0.175009734624489
19 -0.50713922763156
20 -0.866336830913379
21 -1.2342406469936
22 -1.48460792948
23 -1.68389279194141
24 -1.902571533075
25 -1.99071820658101
26 -2.11100837490149
27 -2.16720864558918
28 -2.07075778586362
29 -1.91219489606991
30 -1.66006480262437
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.26396197814688
1 3.57600253513847
2 3.44471379344617
3 2.99492399516444
4 2.60866070339965
5 2.75033476680158
6 3.20350685606467
7 3.64966995280207
8 3.80768345105602
9 3.33791514597472
10 2.81607724546363
11 2.18266652706167
12 1.53553832163274
13 1.05874623168367
14 0.57851088878955
15 0.122573255648058
16 -0.49982041191978
17 -1.12053054481262
18 -1.82752230877439
19 -2.53213196847178
20 -3.15395978893392
21 -3.70279106015082
22 -4.19213514982333
23 -4.69425483775106
24 -5.14422445323838
25 -5.64624432727036
26 -5.98649514933794
27 -6.27555376856279
28 -6.66612921467815
29 -6.89074255160098
30 -6.93081511359027
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.20626864750971
1 3.37080495624393
2 3.21001941019976
3 2.83781535216832
4 2.33630255338212
5 2.53715000010235
6 2.90834609334115
7 2.92280885408904
8 2.98018898071804
9 3.72321073005365
10 4.78496821683344
11 6.09762717316984
12 6.72961257084411
13 6.88229239848012
14 6.8075410138898
15 6.3714297063147
16 5.99281454882343
17 5.64847009689515
18 5.37372333120839
19 5.33001448601313
20 5.18654780512801
21 5.03638069441389
22 4.85336551097712
23 4.55780589820743
24 4.19853729357738
25 3.77799958822755
26 3.26294238405377
27 2.88886909347758
28 2.77128756851889
29 2.92862567296108
30 3.07351446385142
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.25658552898495
1 3.47082710476685
2 3.39649896865899
3 2.98525477837032
4 2.72503971482698
5 3.08422889920362
6 3.46109075656148
7 3.65434003185238
8 3.6446289525014
9 3.48816545405291
10 3.14057451442003
11 2.70221111980623
12 2.13194834516091
13 1.58128804824086
14 1.14555582066121
15 0.744328623878937
16 0.365148532244774
17 -0.00479056715273884
18 -0.268382930798465
19 -0.519140464965114
20 -0.818233385383529
21 -1.21264398222676
22 -1.64593544670449
23 -2.01834815914692
24 -2.27631492123501
25 -2.73987835671156
26 -3.05653643280576
27 -3.40972912317373
28 -3.65108602961805
29 -4.03584266229477
30 -4.44058490459767
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.23127489287905
1 3.42733482227055
2 3.27842563412258
3 2.81660137320982
4 2.42365820313253
5 2.53884000255261
6 2.72027100754178
7 2.88899310538793
8 2.74485772366976
9 2.18772190664949
10 1.407865187313
11 0.433208844465993
12 -0.382608983203772
13 -1.17881478444453
14 -1.92092602575355
15 -2.39487409115371
16 -2.93533713882337
17 -3.54746215990092
18 -4.22431286913905
19 -5.06300298377673
20 -5.83887745835473
21 -6.57300255045581
22 -7.20840040752345
23 -7.76147017171969
24 -8.31482625401014
25 -8.49263156297313
26 -8.65593615392406
27 -8.70366489692298
28 -8.72966795560858
29 -8.36123115226065
30 -7.91476555893067
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.15203926743035
1 3.23145754018118
2 3.22358571377887
3 2.98662146014905
4 2.71431434498369
5 3.03058072350052
6 3.5725992645021
7 3.78296915591414
8 3.7047548067111
9 3.62194580015807
10 3.32044905392989
11 2.59941416767834
12 2.00639636350814
13 1.54363589493789
14 0.903862068981276
15 0.50963366085306
16 -0.134441670246311
17 -0.60314367679953
18 -1.028575267783
19 -1.48322872377538
20 -1.83810386507012
21 -2.07278756218209
22 -2.3281344381084
23 -2.44553214065189
24 -2.59847893557541
25 -2.68601284864418
26 -2.80184107435504
27 -2.90794678546441
28 -3.07275352262527
29 -2.96930489274153
30 -2.86230911269907
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.19345123614707
1 3.52318057485349
2 3.5595193497851
3 3.43260000332081
4 3.48894704108705
5 3.5873535544968
6 4.11888700035211
7 4.40363021202148
8 4.58868534549353
9 4.58503397216482
10 4.34949610016399
11 3.88571838591946
12 3.31647799720714
13 2.70480569372267
14 1.92404499276971
15 1.32169475201326
16 0.713156853527813
17 0.242787116569035
18 -0.159295282858729
19 -0.695287040280366
20 -1.11529001225341
21 -1.63924013289847
22 -2.26756015958512
23 -2.93094061242483
24 -3.55824042844672
25 -4.25562706022705
26 -4.98362121472368
27 -5.67355121782141
28 -6.44442524399633
29 -7.15603455983772
30 -7.69608796606064
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.19581302396698
1 3.53013332273547
2 3.48500965218349
3 3.02711446265838
4 2.68981155218295
5 2.9197288806767
6 3.07996472023508
7 3.31132607400077
8 3.57650583554878
9 3.59417813483966
10 3.41996211420367
11 3.17473415742568
12 2.88344621412411
13 2.59756273222934
14 2.27737843670518
15 2.01805024132695
16 1.62108363588279
17 1.15480029872784
18 0.890316860906028
19 0.553300952612174
20 0.135528895824603
21 -0.0890115288177107
22 -0.317957827231323
23 -0.48928604425619
24 -0.56202419142547
25 -0.7811597872932
26 -1.05341123019124
27 -1.30916398956255
28 -1.5809845746081
29 -1.89634264062881
30 -2.3457491353263
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.17066578060565
1 3.49293722026837
2 3.478644446576
3 3.15150335218057
4 2.80109239098629
5 2.83332580599022
6 3.23091078603794
7 3.5898439062304
8 3.81471071995744
9 3.59627003866184
10 3.10399884538732
11 2.40005444352402
12 1.72446907672077
13 0.966352242629624
14 0.325443695237988
15 -0.272555830149615
16 -0.920448930729311
17 -1.37529690606616
18 -1.71649391869937
19 -2.01732121760529
20 -2.3292491728206
21 -2.54224329805898
22 -2.78899035577883
23 -3.06816211455468
24 -3.35716124145144
25 -3.59635458655269
26 -3.85655509771915
27 -4.11858134573002
28 -4.23063876442022
29 -4.4784893368023
30 -4.65913243335121
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.19566632315881
1 3.35939547736712
2 3.19905289559579
3 2.87508116243679
4 2.57590664422103
5 2.83516515837489
6 2.99198088893639
7 3.04414118300971
8 2.78014859572346
9 2.42622338534576
10 1.94520304103644
11 1.33750250308323
12 0.768731222919719
13 0.103198624705941
14 -0.737446049714624
15 -1.5252588925808
16 -2.26355615202737
17 -2.90283656904232
18 -3.47315450893513
19 -3.91578942435974
20 -4.42669896204231
21 -4.86401553142431
22 -5.3285265279219
23 -5.82677768105354
24 -6.29320967187771
25 -6.83877509445361
26 -7.35737919913037
27 -8.05219954265816
28 -8.71250561564416
29 -9.34698758485045
30 -9.91785382107426
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.30205634079708
1 3.75587508888006
2 3.86114410984164
3 3.70248324270239
4 3.47964486610684
5 3.66137929139227
6 3.68859299259094
7 3.68577275050164
8 3.49473105762965
9 3.05792594720422
10 2.43804789080452
11 1.73045956935148
12 1.08395558453325
13 0.406910453100409
14 -0.33129486751065
15 -1.10300637246697
16 -1.85670476661139
17 -2.45608569399112
18 -2.95066416541834
19 -3.41550747947835
20 -3.96950073688354
21 -4.44644781138255
22 -4.8747574496518
23 -5.32153346306606
24 -5.7587297929454
25 -6.03494383934292
26 -6.28445741090888
27 -6.61919719412013
28 -7.01694832039184
29 -7.280012638247
30 -7.54386312098706
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.22192615199638
1 3.45337215229915
2 3.38660149847349
3 3.22939260747109
4 3.10866319825019
5 3.46161036562278
6 3.96381922943298
7 4.30103320194001
8 4.47567711720786
9 4.27156789389789
10 3.79895788337572
11 3.31073949291411
12 2.92074661982231
13 2.40745640897878
14 1.93200384474803
15 1.52464214320868
16 1.27238607506506
17 1.10995834301624
18 0.994191800767464
19 0.774510230065305
20 0.362010759315297
21 0.00857695692426041
22 -0.436689185331439
23 -0.748882305182555
24 -1.14809726865126
25 -1.45001216325548
26 -1.69464502762028
27 -1.93393669556764
28 -2.06379203794587
29 -2.03831179773477
30 -1.90902038508278
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.10928192834369
1 3.14604545075734
2 3.00922938217309
3 2.83898694083525
4 2.77432041777775
5 3.16988199420289
6 3.70588687288451
7 3.99916539266336
8 4.14115565967612
9 3.83718445705935
10 3.3045068572262
11 2.77008098634386
12 2.32525621811617
13 1.90015715424904
14 1.53358332929385
15 1.23584253954551
16 0.961487431653483
17 0.793530822431189
18 0.689170254332947
19 0.613869391308574
20 0.635921900362824
21 0.6870395994662
22 0.662333081035532
23 0.471330161849506
24 0.239400790223467
25 -0.0528169393845168
26 -0.285916867457212
27 -0.54106905476724
28 -0.803115969584791
29 -1.1422760659448
30 -1.33545262323105
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.14261454190101
1 3.2947391002232
2 3.23808011485701
3 3.07641778650888
4 2.85353273908623
5 3.13463861541903
6 3.33491738084159
7 3.74932508030855
8 4.0761442123317
9 3.91257860658019
10 3.73065799380068
11 3.585877535091
12 3.63328697719099
13 3.51362731452779
14 3.26019723487866
15 2.96683971470936
16 2.7098673257116
17 2.45760767438141
18 2.31917179831158
19 2.20481644117802
20 2.02542099644008
21 1.80504210628003
22 1.54331282434013
23 1.23041132802468
24 1.00133215591937
25 0.803782399108062
26 0.611360820272653
27 0.444187089095765
28 0.390811690432358
29 0.35836213459684
30 0.275224489048291
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.22172597295269
1 3.54399091243196
2 3.47183275737187
3 3.13369055922876
4 2.51289225638517
5 2.4712790141886
6 2.52727052319984
7 2.49446317940294
8 2.16098202927523
9 1.52109903818821
10 0.93878293374225
11 0.268745336775634
12 -0.44907672332679
13 -1.18923394505388
14 -1.92448592604468
15 -2.5798839980436
16 -3.28568547024972
17 -3.85576133723876
18 -4.43837338648984
19 -5.23013355405704
20 -5.95848861652389
21 -6.65809662546459
22 -7.42823526597962
23 -8.12610423711097
24 -8.77171154361247
25 -9.50611177040219
26 -10.4042142687731
27 -11.3511063035021
28 -12.2111315845669
29 -13.0212734833518
30 -13.8315943938956
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.23106796891857
1 3.38322370976058
2 3.22887388076879
3 2.84615183585188
4 2.40393942565777
5 2.62415915525222
6 2.89943025963975
7 3.29803084431365
8 3.4866614048781
9 3.41081422063859
10 3.16689899873607
11 3.03690461250042
12 2.80115308584727
13 2.48394342595234
14 2.13576023399141
15 1.73244856273757
16 1.31149706005285
17 0.843795625973678
18 0.40858033387374
19 -0.0100437928304782
20 -0.27671490401252
21 -0.683316841674944
22 -1.14358942440485
23 -1.62927522752946
24 -2.25520203097018
25 -2.74531601059548
26 -3.27582811271592
27 -3.73518184879623
28 -4.02125953354347
29 -4.30758550621999
30 -4.68095324592481
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.24664508155294
1 3.65959467830722
2 3.63713958766891
3 3.44074016973767
4 3.05559612022943
5 3.27160036844655
6 3.79689147607656
7 4.24042490649362
8 4.53840897034118
9 4.59058985393819
10 4.45262577593119
11 4.07263327704283
12 3.62782559796291
13 3.20468669922935
14 2.80091989207914
15 2.45760449660343
16 2.07344796561844
17 1.80431750202626
18 1.59936694276239
19 1.33680509625064
20 1.03790867007955
21 0.814232506141863
22 0.397713551601253
23 0.0500039683548348
24 -0.329789847161138
25 -0.708175814404537
26 -1.03467835632661
27 -1.45126828911235
28 -2.04489140362818
29 -2.54383002791296
30 -2.88461133126669
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.1750505702714
1 3.47018017920363
2 3.47357949514793
3 3.0518926402751
4 2.55624013201938
5 2.68854297761989
6 3.23847728655885
7 3.59882284294196
8 3.90174324392626
9 3.92531526678376
10 3.58586927164411
11 3.07117331740041
12 2.57943641483005
13 1.96578312073724
14 1.39212341580541
15 0.849688377675916
16 0.376704045653053
17 0.0401618568648878
18 -0.415096263895164
19 -0.823546804753498
20 -1.17835186984405
21 -1.62577539497797
22 -2.14707231852313
23 -2.69656041443118
24 -3.3447910283963
25 -3.9972994182957
26 -4.74487569762686
27 -5.46235320385572
28 -6.19418484636383
29 -6.95275937551349
30 -7.64349325192884
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.22113885797057
1 3.42891436863364
2 3.576070494845
3 3.37646645108944
4 3.04166886175004
5 3.18891476346478
6 3.4195716230952
7 3.84732877019971
8 3.82467223033009
9 3.58067908685114
10 3.10608570035093
11 2.5425841549247
12 2.03929473919406
13 1.71584204545326
14 1.3117754086081
15 1.02241434957463
16 0.683637438938378
17 0.383858607851106
18 0.0176619052331812
19 -0.554432667261027
20 -1.15598394367692
21 -1.70725343624384
22 -2.49346207075699
23 -3.26137770521498
24 -4.0451409142769
25 -4.76579975665191
26 -5.43970237735309
27 -6.05843076121071
28 -6.6744917398467
29 -7.24545364940876
30 -7.86570364597909
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.23291715949417
1 3.49007233580315
2 3.3047318184822
3 2.77529613499405
4 2.2830176583855
5 2.1730444224702
6 2.33303931796849
7 2.57318415608919
8 2.94773182102658
9 3.17034365912309
10 3.05561036148235
11 2.70360918139949
12 2.24296797295287
13 1.85683264499969
14 1.68845004898115
15 1.54779087813024
16 1.23903646879986
17 0.930959786979248
18 0.392169309468706
19 -0.142848955497374
20 -0.575255590363245
21 -0.94028639795822
22 -1.32564104602175
23 -1.5869149222618
24 -1.85974006004509
25 -2.04005479470764
26 -2.28119878312447
27 -2.55970530505602
28 -3.06759014258584
29 -3.50248827614174
30 -3.84407317826551
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.19153873765365
1 3.54535199367033
2 3.47349868491138
3 2.9677279964905
4 2.32851797175141
5 2.51746781796289
6 2.75942085638844
7 3.03037747273863
8 2.88171619463515
9 2.4247919882018
10 1.84404488405209
11 1.20508497815988
12 0.655202466242965
13 0.0842353290780125
14 -0.426255952113372
15 -0.961872721450003
16 -1.56683672631036
17 -2.09252224098078
18 -2.73880076892097
19 -3.32798251335979
20 -3.9914227670912
21 -4.63693844714839
22 -5.23523441337981
23 -5.68145185482421
24 -6.15268288951068
25 -6.48148751170134
26 -6.66489573338887
27 -6.78541006330077
28 -6.79495687943077
29 -6.68456179377051
30 -6.63436611891242
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.26974800628749
1 3.49735921200084
2 3.47565316705439
3 3.3276866077256
4 3.13854406553306
5 3.47641336279241
6 3.70936461390823
7 3.74657531623389
8 3.86986488820112
9 3.64362334384542
10 3.35155112983813
11 2.97555149916115
12 2.49123983490032
13 1.74886612166103
14 1.1330795129164
15 0.461240501275228
16 -0.0898178274752048
17 -0.70711683642357
18 -1.24373822922412
19 -1.79598240693382
20 -2.38355871588872
21 -2.80338216164657
22 -3.15381365864409
23 -3.4670513866293
24 -3.72973152226953
25 -4.13873349778642
26 -4.49355122322634
27 -4.82928562742025
28 -5.07942423353981
29 -5.36858515315824
30 -5.70610985064012
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.18617062714679
1 3.41309071654777
2 3.36086544908115
3 2.917406804117
4 2.40481098204154
5 2.65743218086407
6 2.83926999005887
7 3.14772459056623
8 3.4566633830606
9 3.15450020349288
10 2.86411902641571
11 2.46098890281461
12 1.9739857788403
13 1.46413470015487
14 1.02217684972992
15 0.720377719025546
16 0.446916377364355
17 0.12921266277535
18 -0.151345850171198
19 -0.470521204470078
20 -0.720140755645883
21 -0.923900170892949
22 -1.22985442710014
23 -1.61658359415181
24 -1.99731924350572
25 -2.42334669653206
26 -2.80301687930946
27 -3.19406342219438
28 -3.42048368557234
29 -3.49162415412034
30 -3.46245205254132
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.22631525789151
1 3.60281350989068
2 3.58514345919358
3 3.45214735648766
4 3.07114758072427
5 3.19280723582792
6 3.47506587305143
7 3.69101155551264
8 3.70632402918634
9 3.36438817953619
10 2.83101204403887
11 2.36189824409678
12 1.91527111316161
13 1.53539459635278
14 1.12531850904228
15 0.713229087345082
16 0.0660586047692711
17 -0.558394890038185
18 -1.2336427364738
19 -1.89146341803301
20 -2.38206587555951
21 -2.88754527113905
22 -3.34058167372423
23 -3.75272545415629
24 -4.20987788998263
25 -4.50863435523848
26 -4.97167328665505
27 -5.34085986236463
28 -5.74263304481461
29 -6.05607176975849
30 -6.40287185398585
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.20830759390929
1 3.51976553019202
2 3.55371485202857
3 3.24442730718812
4 3.04966455851418
5 2.92147822786849
6 3.29043003421703
7 3.61099425821359
8 3.826294657065
9 3.69312416457916
10 3.33163606632404
11 2.88607596584144
12 2.5156943143211
13 2.16589246269017
14 1.83736561449754
15 1.435643102767
16 1.02227607578475
17 0.571173067620938
18 0.00741664598242053
19 -0.63649976815368
20 -1.29858124979929
21 -1.96539416285695
22 -2.6529600229409
23 -3.32514907000195
24 -3.93746926583403
25 -4.53410366121907
26 -5.10959574782258
27 -5.60489214232581
28 -6.11762386685435
29 -6.67346085545942
30 -7.25726292623434
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.24998380303157
1 3.57965078425139
2 3.64324172892621
3 3.42796565728906
4 3.09730049997882
5 3.09574610121376
6 3.23153937670925
7 3.47237329610208
8 3.57657022954298
9 3.63363155028977
10 3.47789264815539
11 3.5300091263422
12 3.42375842459309
13 3.13265938671259
14 2.83778341103898
15 2.435629676724
16 2.09739245141335
17 1.76408305941773
18 1.31750946897552
19 0.913312519085549
20 0.645371472497599
21 0.467749463205541
22 0.174939902929905
23 -0.133636553085555
24 -0.423183872636519
25 -0.841102359495498
26 -1.25084703624105
27 -1.5786237086085
28 -1.94782533308856
29 -2.29249647360182
30 -2.61727496728601
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.19028520664698
1 3.43369356691053
2 3.30957519475349
3 2.84932990752641
4 2.53832871374211
5 2.68576488042211
6 3.29740771997387
7 3.42626549809915
8 3.37758690373237
9 3.03070582206222
10 2.67987603958486
11 2.10222214903119
12 1.77226476591493
13 1.59229949041822
14 1.27583843688549
15 0.973998409244492
16 0.767705703282873
17 0.6634025549582
18 0.548880023277585
19 0.398621552954406
20 0.14751415712394
21 -0.181527151747758
22 -0.600578541055176
23 -0.948897885631444
24 -1.18028140740208
25 -1.38011519524096
26 -1.58063684128357
27 -1.82576485246005
28 -1.93397655822546
29 -2.08345062074367
30 -2.22097164288953
};
\addplot [semithick, color0, opacity=0.1]
table {%
0 3.17916995438733
1 3.3605695525045
2 3.25536481489402
3 2.86645694104324
4 2.56317931876636
5 2.73959455708613
6 3.07713002765344
7 3.45379502613828
8 3.52771316409367
9 3.08062660363449
10 2.48880573403233
11 1.74950416349055
12 1.00744047901534
13 0.286566778207433
14 -0.313151038764696
15 -0.86771890518407
16 -1.42529740164273
17 -1.89578436862621
18 -2.50151111294332
19 -3.13894453715736
20 -3.66384624679654
21 -4.23858918404441
22 -4.69522265857561
23 -5.07843881654385
24 -5.51022708678854
25 -6.00507208591472
26 -6.50352373458341
27 -6.90412206533221
28 -7.3547990340105
29 -7.76426728769923
30 -7.99828123850161
};
\addplot [line width=0.01pt, color0, mark=*, mark size=2, mark options={solid, draw=black}]
table {%
1 3.31996634253658
2 3.45443899460193
3 3.38784218387077
4 3.01931286439371
5 2.82906626173755
6 3.09427938765557
7 3.60416870184349
8 4.24596487007442
9 4.84338888587772
10 5.27994908427636
11 5.61004074039071
12 5.90268352537916
13 6.05852129333431
14 6.16858387553312
15 6.19509636026208
16 6.21485180933973
17 6.20378189365436
18 6.1468591562609
19 6.14787992255152
20 6.14579317317396
21 6.15283082950704
22 6.15412613868876
23 6.14366281427887
24 6.16587792193215
25 6.18223254289368
26 6.18638821201769
27 6.14794417270148
28 6.14179954980725
29 6.15812095860932
30 6.16746194810668
};
\end{groupplot}

\begin{groupplot}[group style={group size=1 by 3}]
\nextgroupplot[
xshift=-8,
xmin=-1.45, xmax=30.45,
%ymin=-2.46891241301875, ymax=46.6986447843329,
ymin=-0.85, ymax=5.85,
width=\figurewidth,
height=\figureheight,
xtick={},
xticklabels={},
yticklabels={},
axis y line=right,
tick align=outside,
xtick pos=left,
ytick pos=right,
x grid style={white!69.019607843137251!black},
y grid style={white!69.019607843137251!black}
]
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.51449527600915
1 1.65263797282671
2 0.885698784509295
3 -0.0512125163318231
4 -1.58941429259235
5 -3.21002832104077
6 -4.20112336893458
7 -4.64673038635938
8 -4.7190146987115
9 -4.7954538062244
10 -4.94600813204799
11 -5.30284464754359
12 -5.83473576619159
13 -6.25137666924403
14 -6.9019327067286
15 -7.67347224075089
16 -8.45494997176789
17 -9.09001541362697
18 -9.73692294889496
19 -10.1531595161162
20 -10.4482491806604
21 -10.5434884900814
22 -10.4730934113126
23 -10.3113301988494
24 -9.85084405908331
25 -9.61899201585684
26 -9.4470505266509
27 -9.32978199748259
28 -9.19573506299622
29 -9.02325231895288
30 -8.6967795371946
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.5716012564685
1 1.90849753859415
2 1.12997340240984
3 0.0461854517528923
4 -1.31014233361252
5 -3.03703180527415
6 -3.94833101083549
7 -4.88625670011353
8 -5.62223731358372
9 -5.84667385778093
10 -5.8394990748953
11 -6.08547692030767
12 -6.60074491733129
13 -6.91167848206354
14 -7.23776963820285
15 -7.55771385308158
16 -8.12260121806778
17 -8.52691229566092
18 -8.8731618071383
19 -9.16575041596174
20 -9.18798050105856
21 -9.2686255879525
22 -9.3719419332199
23 -9.41044692223241
24 -9.23854628260447
25 -9.17573929235782
26 -9.08721118964464
27 -9.20113504471775
28 -9.2552841731436
29 -9.14594104124239
30 -8.96228012702035
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.64865453761992
1 1.7658029473426
2 0.731788462243454
3 -0.365815087641042
4 -1.73493406804507
5 -3.36058522629768
6 -4.23374810548713
7 -4.90573071215242
8 -5.05564908912445
9 -4.7245816364592
10 -4.37712921758876
11 -4.56546143433136
12 -5.29575802456364
13 -5.8535214922921
14 -6.61581071945406
15 -7.28531057809896
16 -7.93744373600414
17 -8.51833739681303
18 -9.01827438522947
19 -9.41606661835351
20 -9.85490465684756
21 -10.0233568813886
22 -10.2730631629692
23 -10.5450527153875
24 -10.6196241064852
25 -10.5080765901172
26 -10.6926344119322
27 -10.7067620431909
28 -10.549653321033
29 -10.6086712225462
30 -10.471847001489
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.5129790339449
1 1.81592890038052
2 1.01665683562056
3 -0.118240614007441
4 -1.52640099354567
5 -3.03398909573744
6 -3.89205721011055
7 -4.19705673387757
8 -4.07136794906639
9 -3.80630459350282
10 -4.11081796407738
11 -4.48671654246506
12 -5.17188394760026
13 -5.57770400207888
14 -6.08782021304833
15 -6.41744870922028
16 -6.96011594392432
17 -7.39908090924486
18 -7.86564124211917
19 -8.44187940112985
20 -8.90094395062235
21 -9.59308568811729
22 -10.1543418931253
23 -10.716403324715
24 -11.3646987133191
25 -11.725514268913
26 -12.1151408439449
27 -12.5794328411089
28 -13.0584147983161
29 -13.2370025789015
30 -13.3046263319953
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.60929517186948
1 1.87255197417621
2 1.21131004962823
3 0.496768909347221
4 -0.44861299487015
5 -1.80838706229821
6 -2.93044854261516
7 -3.72195085185438
8 -4.05676126890104
9 -4.11002598812304
10 -4.21949239186794
11 -4.45323924317472
12 -5.25374749920361
13 -5.8105356377878
14 -6.38486076299855
15 -6.76772559217868
16 -7.32358796237284
17 -7.66735970853272
18 -8.05797112663158
19 -8.38171466473713
20 -8.87533273504362
21 -8.92884336996474
22 -9.13723236207702
23 -9.10899746166783
24 -9.05623278751623
25 -8.82309658581298
26 -8.64372133732298
27 -8.43655207101149
28 -8.19362558017027
29 -7.84322932486747
30 -7.39973146260973
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.60404571946389
1 1.84650792032551
2 0.969034188003345
3 -0.0909553333183535
4 -1.3788610571133
5 -3.36426564816446
6 -4.7796853244434
7 -5.39357313485526
8 -5.71112856241842
9 -5.8742406508702
10 -6.00077197751831
11 -6.26715166137148
12 -6.76109910138819
13 -6.84182056180709
14 -7.34815202392726
15 -7.59271676900144
16 -8.11620776241827
17 -8.63042078127141
18 -9.03849966554968
19 -9.34944407464707
20 -9.66738810754494
21 -10.128806076093
22 -10.5235351207299
23 -10.8876313243261
24 -10.9988575023898
25 -11.4440595985885
26 -11.6624710622563
27 -11.7047510105078
28 -11.8838015056592
29 -11.9842406284134
30 -12.1888903914988
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.52110755473586
1 1.95211727268939
2 1.19044650424943
3 0.402450951310819
4 -0.854498860635269
5 -2.12646533387313
6 -3.10059609212389
7 -3.6788733419172
8 -4.10972878835738
9 -4.24456879544846
10 -4.26105112479276
11 -4.2281870013914
12 -4.39544695105231
13 -4.62562397715431
14 -5.26574757180786
15 -5.93241885851241
16 -6.49211464668623
17 -6.98528057701251
18 -7.30911462727422
19 -7.5469191595585
20 -7.88687666708995
21 -8.1640824907125
22 -8.56733139612586
23 -8.94461778939437
24 -9.30705962601986
25 -9.68001044794227
26 -9.85888133187012
27 -9.87713407407766
28 -9.99083703002539
29 -10.0265172324736
30 -9.97788492275007
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.56073915728873
1 1.7716371734757
2 0.949171141251592
3 0.030507787547446
4 -1.13214342287936
5 -2.85201186345927
6 -4.08872625706204
7 -4.25447086625473
8 -4.28545728727538
9 -3.95553426899793
10 -3.86881839363419
11 -3.76278763880077
12 -4.24892346100187
13 -4.47964654976869
14 -5.12108618722325
15 -5.93339794738508
16 -7.04452749318923
17 -8.42782915130958
18 -9.58199630472468
19 -10.7046061718146
20 -11.8304480688218
21 -12.5534377102001
22 -13.252004717588
23 -13.8743252232323
24 -14.5643157043903
25 -15.4741608595705
26 -16.2384693315261
27 -16.9140215732312
28 -17.7271297042252
29 -18.3273115954273
30 -18.739105144627
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.57463359538638
1 1.78833796889662
2 0.966519423371322
3 0.0423958049996305
4 -1.17353576478616
5 -2.88125736913909
6 -3.85230381087767
7 -4.34087993161836
8 -4.38730983074341
9 -4.45990497847001
10 -4.42286281328376
11 -4.8454116472974
12 -5.68300769997566
13 -6.66948442993604
14 -7.45861799994532
15 -8.13974310890752
16 -9.11141844360188
17 -9.73622137623092
18 -10.2567573206084
19 -10.618039298182
20 -11.0765717904315
21 -11.4869322823914
22 -11.9072491141772
23 -12.1838902554736
24 -12.6019679610168
25 -12.9993381569997
26 -13.3260491552319
27 -13.5751391055576
28 -13.7910909964491
29 -14.0015463192277
30 -14.13721016077
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.58103772922703
1 2.17599135569361
2 1.62341594950044
3 0.795988302074278
4 -0.505725004472627
5 -2.11842189635734
6 -3.46582051126459
7 -4.17225683260382
8 -4.42367476463499
9 -4.46745973496526
10 -4.52574287877303
11 -4.85796703734536
12 -5.13480994895812
13 -5.48592756134111
14 -5.96468517178117
15 -6.54617755703076
16 -7.34600995006448
17 -8.1967921026277
18 -9.08196288369225
19 -10.2177134104657
20 -11.0301734939037
21 -11.7441786011871
22 -12.2387817135557
23 -12.9835867441468
24 -13.2731165464716
25 -13.6870538522699
26 -13.8280310743294
27 -14.1399295387643
28 -14.2627987487054
29 -14.2644049573265
30 -14.0948645039523
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.56995241140633
1 2.16373326344519
2 1.7742651626691
3 0.864101198630292
4 -0.249313131479012
5 -1.22661081285849
6 -1.89752519594261
7 -2.81395896036533
8 -3.06915816432447
9 -2.59963033582582
10 -2.28780162809645
11 -2.25695089510183
12 -2.45801040420859
13 -2.82398847267009
14 -3.4036819234573
15 -4.01516664669403
16 -4.86630837934762
17 -5.70862703212554
18 -6.32222685858232
19 -7.01120660317895
20 -7.70351315289437
21 -8.38531565769164
22 -8.80867892318689
23 -9.23086114196951
24 -9.69230501085739
25 -10.1679111067108
26 -10.5647758685675
27 -11.0138436728436
28 -11.4213271589856
29 -11.7402927474332
30 -12.0082896269663
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.57368109112655
1 2.00535342490571
2 1.51277499835559
3 0.666005815093898
4 -0.374470852395683
5 -1.74648343649645
6 -2.94752051486071
7 -3.57919267053517
8 -4.03106754626075
9 -3.54054839047481
10 -3.66072780649939
11 -3.81358496320932
12 -4.24857919059363
13 -4.81916386308287
14 -5.42638093029776
15 -5.86638571398658
16 -6.34637026011626
17 -6.7875325455549
18 -7.14446706375539
19 -7.58653627441641
20 -7.7666513118782
21 -8.11548435382201
22 -8.26408746832599
23 -8.43228604854207
24 -8.47381998572801
25 -8.47046581730711
26 -8.41213460021655
27 -8.2259814757913
28 -8.10896849457872
29 -7.87364745364884
30 -7.25002302215816
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.60949584486034
1 1.89872057120653
2 0.925796733261921
3 -0.143282590807409
4 -1.54819148824288
5 -3.5697670209211
6 -4.4303956959926
7 -5.31443650604653
8 -5.97001221266595
9 -6.27069016157227
10 -6.71599731840749
11 -7.3046693159541
12 -7.94817093273367
13 -8.82056665236959
14 -9.51551990572591
15 -10.4992299948794
16 -11.2617240933986
17 -12.1710007258347
18 -13.1291221317765
19 -13.8422497694066
20 -14.3975672849936
21 -15.1357050525727
22 -15.8961789626523
23 -16.4092245604841
24 -16.9822949698716
25 -17.6012894695333
26 -18.0850494000524
27 -18.4574942949035
28 -18.8236459107386
29 -19.2037076556345
30 -19.3774880675168
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.56590642341126
1 1.79312028900875
2 0.73023804762747
3 -0.329018885899615
4 -1.78589399995495
5 -3.39758981224589
6 -4.62674107527045
7 -5.4665866211312
8 -5.74257734808656
9 -5.65481325429706
10 -5.7874798348967
11 -6.2713094621147
12 -6.51911118233616
13 -6.8304692402593
14 -7.36055402166436
15 -7.93439001317977
16 -8.88570806550804
17 -9.65466566701263
18 -10.2695759509347
19 -10.5780544274484
20 -10.8513832406387
21 -11.3031231350157
22 -11.6918729759119
23 -12.0026082366556
24 -12.5059984210894
25 -12.9423528568818
26 -13.2491550541202
27 -13.4540466662148
28 -13.7718234464507
29 -13.9093224562205
30 -14.128683771821
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.54832030768531
1 1.92471063412862
2 1.37984587863143
3 0.865653963850505
4 -0.0763632476845189
5 -1.30033789084727
6 -2.65160990068264
7 -3.3497473199968
8 -3.84441074608509
9 -4.06445907020971
10 -4.25881844942129
11 -4.70545156508871
12 -5.00956076293044
13 -5.64803607752252
14 -6.37577146676847
15 -6.91570120988594
16 -7.47504886334082
17 -7.86361657209192
18 -8.38563130457179
19 -8.84734199768677
20 -9.3751469031701
21 -9.75692137433162
22 -10.3629022342789
23 -10.6997650960274
24 -11.2809427803393
25 -11.8881892397705
26 -12.4797524779083
27 -13.0629273770121
28 -13.6430299670711
29 -14.0473620424809
30 -14.3843525254055
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.58809025441659
1 1.85895947819974
2 1.30557444624526
3 0.314413918431431
4 -1.08603565550158
5 -2.61747896482378
6 -4.26534832951205
7 -5.16717458262901
8 -5.52727887717657
9 -5.54096517301544
10 -5.64727637039488
11 -5.78542047827909
12 -6.04908152918421
13 -6.77439149409715
14 -7.26854378420681
15 -7.99589267202322
16 -8.8415851490031
17 -9.54319075976575
18 -10.2554544570657
19 -10.8728491345234
20 -11.3470716808449
21 -11.9440506162399
22 -12.3393034565582
23 -12.6833304361485
24 -12.8808324473558
25 -12.9169518957139
26 -12.8374386695237
27 -12.6351113383873
28 -12.471847139303
29 -12.5639397038992
30 -12.4185978336934
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.64479207396786
1 1.82602595290967
2 1.07584603855297
3 0.122118686717108
4 -1.19678211944412
5 -2.70823511261436
6 -3.59244980107854
7 -4.27350263369991
8 -4.66961657941249
9 -4.86334729700132
10 -4.78936929728388
11 -4.71654847339111
12 -4.82348889080654
13 -5.24570524376503
14 -5.85802816070902
15 -6.43952293166294
16 -7.30040758665402
17 -8.17308768252145
18 -9.02543068217143
19 -9.66387636668742
20 -10.0888425327941
21 -10.4458286713058
22 -10.7355291325685
23 -11.0372315394122
24 -11.3250415753527
25 -11.1918994375932
26 -11.3500483515216
27 -11.4916892386171
28 -11.6796698008771
29 -11.4587327273289
30 -11.2312464854932
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.5827131966526
1 1.64520054187233
2 0.743547856365407
3 -0.481220481443781
4 -2.21658752855551
5 -3.69188250406935
6 -4.76062611940951
7 -5.60933165093203
8 -5.73345554391359
9 -6.11760158216573
10 -6.32035539343492
11 -6.35994338566766
12 -6.61479058686947
13 -6.73453235965338
14 -6.74425061020818
15 -6.59096852747089
16 -6.57792630108207
17 -6.69760446642325
18 -6.70526426832876
19 -6.77633018265932
20 -6.79134922043223
21 -6.71930409525481
22 -6.56643994996205
23 -6.38838532687521
24 -6.06697155656393
25 -5.58045743348722
26 -4.97430973740346
27 -4.14467207874855
28 -3.10620619218522
29 -2.06087237900585
30 -0.918020815948809
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.57451055095252
1 2.04140586871198
2 1.38301142784969
3 0.604060854253456
4 -0.669969209872409
5 -1.98654123103059
6 -3.23540331288158
7 -3.9153559941812
8 -4.25293155962184
9 -4.42406316983222
10 -4.4576290316861
11 -4.79503197012942
12 -5.14687338405477
13 -5.74711991784321
14 -6.49068024109207
15 -7.28979835704755
16 -8.13647982216191
17 -8.94863603801998
18 -9.6537612517575
19 -10.3096783300818
20 -10.6694341454699
21 -11.0598678048789
22 -11.316468079284
23 -11.4668376588664
24 -11.5434693481727
25 -11.5998138192533
26 -11.7642937465051
27 -11.9774733849691
28 -12.2489463099125
29 -12.4964661044155
30 -12.4039910094853
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.59373072638092
1 2.17616074021265
2 1.34430987412983
3 0.487026592326188
4 -0.830225481549158
5 -2.2996267062042
6 -3.71922795562627
7 -4.41149273849205
8 -4.90334634886588
9 -4.6504052862717
10 -4.65988144806499
11 -4.98231569389239
12 -5.52902080034534
13 -6.18154203254578
14 -6.81842990527147
15 -7.55961904812489
16 -8.31548247569635
17 -8.74343480077778
18 -9.19954971121056
19 -9.71303766150645
20 -10.2650293585786
21 -10.7812091108882
22 -11.2130719790755
23 -11.8035389844174
24 -12.2468274339976
25 -12.8908943274008
26 -13.1859131914382
27 -13.5445610982364
28 -13.9119760709189
29 -14.1515860847472
30 -14.4351520701871
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.63704375221219
1 1.77638095427202
2 1.04439814493956
3 0.131574351821898
4 -1.10250657216259
5 -2.62356670594351
6 -4.10405375550981
7 -5.01781457867981
8 -5.50849102035109
9 -6.00493584827713
10 -6.35233264642319
11 -6.39312187857464
12 -6.66026836037919
13 -7.17554811909938
14 -7.59623900946843
15 -8.20960605542312
16 -8.76990645335426
17 -9.30026140297119
18 -9.87120743116865
19 -10.4539004634969
20 -10.9716259505454
21 -10.8809653680451
22 -10.7181229882014
23 -10.5695126987458
24 -10.4231137555588
25 -10.1680511939634
26 -9.70877123357087
27 -9.03962955175495
28 -8.47823049813234
29 -7.755109135492
30 -7.11335878988957
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.57906082233055
1 1.78277574798254
2 1.03209117653827
3 0.165069381731268
4 -0.907049371013958
5 -2.22089602966234
6 -3.37314850546641
7 -4.27963442086537
8 -4.83415903491697
9 -5.09481370695292
10 -5.55078659539397
11 -6.03948495067287
12 -6.96886713819779
13 -7.69199775889597
14 -8.53241153416298
15 -9.38931742920702
16 -10.1755014247282
17 -10.9578773763028
18 -11.5900579694774
19 -12.2254877908556
20 -12.6589475919776
21 -12.9889834972841
22 -13.3329970168797
23 -13.5945593248949
24 -13.8088943671415
25 -14.0463453074516
26 -14.0870475320655
27 -14.2509991592861
28 -14.2386268379065
29 -13.9717577038892
30 -13.7607494254209
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.62481810768444
1 1.90771068037758
2 1.25448479979402
3 0.52994963778116
4 -0.713694438226479
5 -2.16702766028971
6 -3.22115336594814
7 -3.88103996115226
8 -4.17829807694983
9 -4.49127722401223
10 -4.95375995036936
11 -5.48932508367073
12 -6.03681228345301
13 -6.62552013356136
14 -7.28051584837351
15 -8.12453934593942
16 -9.10007170626315
17 -9.92522229911955
18 -10.5490519854334
19 -11.0712632360068
20 -11.7640437974704
21 -12.3244517352107
22 -12.9393161136905
23 -13.4924657438656
24 -14.058016974737
25 -14.6495315442838
26 -15.0067672408783
27 -15.4151089584132
28 -15.7938248388293
29 -16.0473812764862
30 -16.2949678242578
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.55554903007083
1 1.92280947228583
2 1.33092108554785
3 0.41503520200043
4 -0.877746638374211
5 -2.40668412607417
6 -3.38853624407668
7 -4.01535832827203
8 -4.50850591958362
9 -4.91669196099394
10 -4.88252053340881
11 -4.90479131116891
12 -5.16955049331286
13 -5.69489171062575
14 -6.19712252669134
15 -6.81326421700803
16 -7.34246143772628
17 -7.84657168395573
18 -8.22668891328925
19 -8.51955362457978
20 -8.67585794249022
21 -8.70761722396225
22 -8.85624836952358
23 -9.00898982294401
24 -9.1629959544807
25 -9.30712068329164
26 -9.1647444739622
27 -9.12714085388064
28 -8.99916494306808
29 -8.66283434970836
30 -8.02308487705372
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.64625488747093
1 1.9303198473398
2 0.980631182538163
3 0.107602499634204
4 -1.12299097371012
5 -2.58050450312352
6 -3.91899208839663
7 -4.90985538962998
8 -5.4789900295581
9 -5.93151438292082
10 -6.41924840220011
11 -7.05442146691736
12 -7.77050548748202
13 -8.51525519745039
14 -9.15741697254189
15 -9.73924815439518
16 -10.3809264006186
17 -10.9649965350035
18 -11.4646565137733
19 -11.9697788765249
20 -12.2640734405377
21 -12.5005486357524
22 -12.7895792733318
23 -12.9802335205401
24 -13.2464786188239
25 -13.2499255613363
26 -13.3132438214819
27 -13.2772253500382
28 -13.1881618270674
29 -12.8712351487147
30 -12.4258101281851
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.55598724786367
1 1.80415890353646
2 0.973586911203702
3 0.156839301139923
4 -0.799023389909406
5 -2.39323615665365
6 -3.33646468402638
7 -3.62687597117088
8 -3.73259732668655
9 -3.65736728083773
10 -3.78105409091059
11 -4.13234456968528
12 -4.76121819147963
13 -5.80514989789391
14 -6.706289256495
15 -7.80816170627951
16 -8.83927232477325
17 -9.53991958463798
18 -9.96989905968487
19 -10.1003924192777
20 -10.3199561695739
21 -10.4981064693861
22 -10.5577875683349
23 -10.5576974368404
24 -10.3311732384934
25 -9.68796149732102
26 -8.94194125572406
27 -8.3434372625701
28 -7.64433321625759
29 -6.74866757314562
30 -6.01464562492587
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.56982864465458
1 1.907676652179
2 1.27188496113747
3 0.484121783264344
4 -0.485908141629043
5 -1.49689086051704
6 -2.17288956848871
7 -2.97705758624349
8 -3.21192903779581
9 -2.8405141064555
10 -2.62915543451681
11 -2.58979250434028
12 -2.97772734927789
13 -3.49914897258171
14 -4.07865926529492
15 -4.55868819019506
16 -5.146623257868
17 -5.44635997012331
18 -5.92134724721585
19 -6.3177726806684
20 -6.86578134856775
21 -7.62076497001152
22 -8.03088453523659
23 -8.41862124294093
24 -8.98472968661688
25 -9.86234851045631
26 -10.4999405551953
27 -11.0290368899145
28 -11.5630648438109
29 -12.0541655275901
30 -12.5868257042576
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.55814466707209
1 1.60561864195964
2 0.761940292242642
3 -0.187661621521098
4 -1.51943873911642
5 -3.3324650073359
6 -4.47724680802849
7 -5.36482793571182
8 -5.60715545427677
9 -5.56583126068235
10 -5.92075628740219
11 -6.41204022372822
12 -6.79247236017224
13 -6.94706205521808
14 -7.44513233284519
15 -7.99419621318487
16 -8.57670358432994
17 -9.0486306334706
18 -9.54655511479283
19 -10.0326444637932
20 -10.5303703155002
21 -10.9866363918699
22 -11.2658665537534
23 -11.5467817976171
24 -11.9970904509717
25 -12.2294649676084
26 -12.5459959823084
27 -12.6987683615796
28 -12.8974992073456
29 -13.3319102559388
30 -13.334614326452
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.55342482693096
1 1.86541330115544
2 1.09326777275746
3 -0.0573205767070029
4 -1.57193886905987
5 -3.15953441281944
6 -4.17875369124871
7 -5.01069993903617
8 -5.52630314928279
9 -5.10791315030488
10 -4.58451492162657
11 -4.19453180309638
12 -4.42864966217465
13 -4.87378497152127
14 -5.53731562411448
15 -6.10949911049101
16 -6.67575218134027
17 -7.1559577382977
18 -7.75421012360328
19 -8.36645078836662
20 -8.90146568955998
21 -9.27525403482219
22 -9.68098953115125
23 -9.93475757675888
24 -10.1993726133268
25 -10.3202902474594
26 -10.3174673799896
27 -10.2008392745044
28 -10.0879585877125
29 -9.77454912398034
30 -9.31719450772515
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.58422342558569
1 1.96629228473795
2 1.44942351846507
3 0.595802893841428
4 -0.585689325684042
5 -2.19143747772718
6 -3.04675631265196
7 -3.49387498550403
8 -3.43982726473817
9 -3.48871597995449
10 -3.30339600098521
11 -3.49741086628175
12 -3.88012880586109
13 -4.54414181249654
14 -5.42652905392478
15 -6.08996515485356
16 -6.53474252764514
17 -7.2326730441528
18 -7.73860488275414
19 -8.32391766877415
20 -8.96470267887383
21 -9.66200656807269
22 -10.307231929961
23 -10.8744580032951
24 -11.3026990388513
25 -11.8919782939396
26 -12.4524046912619
27 -12.8902202289743
28 -13.1176055115173
29 -13.4004549214719
30 -13.6964383121351
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.57825520673683
1 2.02151291249588
2 1.20333172494635
3 0.376107701690986
4 -0.833682564174731
5 -2.3762750771527
6 -3.72088250592215
7 -4.33082841857919
8 -4.66167135820462
9 -4.38344602755142
10 -4.06980193301766
11 -3.98274438647912
12 -4.12935093657177
13 -4.42370947253653
14 -4.81875972612656
15 -5.29141711392131
16 -5.86296430153124
17 -6.57304279248122
18 -7.06332829630733
19 -7.56996178543776
20 -8.02408491611772
21 -8.50061262402434
22 -9.25460351508127
23 -9.79327929615139
24 -10.134131979494
25 -10.4338763558713
26 -10.5277345993001
27 -10.383427507103
28 -10.3313414727811
29 -10.2363821957089
30 -10.0141684586755
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.5451150886767
1 1.92756866974606
2 0.916675888603223
3 -0.182008863369566
4 -1.36553974611429
5 -2.85611649552127
6 -3.76131036732932
7 -4.02483828574743
8 -4.26514942833686
9 -4.40188970445426
10 -4.32028236478297
11 -4.80216661449055
12 -5.23580241737333
13 -5.53438532769195
14 -5.82450238363842
15 -6.10873774001971
16 -6.53913561360792
17 -7.06756421169751
18 -7.82991010725716
19 -8.2414552809646
20 -8.51488718360348
21 -8.52155672194641
22 -8.65488953213011
23 -8.84478463931631
24 -8.63332900434845
25 -8.30959982513566
26 -7.98211525366272
27 -7.76436761696103
28 -7.47826309079588
29 -7.04853776595276
30 -6.46873272986531
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.57906920368751
1 2.00435572719284
2 1.2977036798031
3 0.301854903395336
4 -0.765448794534064
5 -2.17406006142207
6 -3.4631677032819
7 -3.87639249246275
8 -4.02978319490847
9 -4.22240283237486
10 -4.62964591966163
11 -4.9246633228268
12 -5.13986676403659
13 -5.46350602205846
14 -5.55030869450603
15 -5.64472447684471
16 -6.18163839496976
17 -6.87404681936672
18 -7.77599966722983
19 -8.42769411207501
20 -8.96179852352736
21 -9.6759613728361
22 -10.4042376749109
23 -10.9655428010698
24 -11.5185183781646
25 -12.0815371051557
26 -12.4014506477374
27 -12.7622864622926
28 -13.3592043928024
29 -13.8166191767935
30 -14.4572475381281
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.54408838053921
1 1.96590775715546
2 1.27673186965971
3 0.377101564736972
4 -0.761412686708535
5 -2.20967611406487
6 -3.71128205797414
7 -4.71317816345169
8 -5.03870130997606
9 -4.77626256803834
10 -4.63653806731441
11 -4.91952025257111
12 -5.39895577026637
13 -5.81526355772368
14 -6.34297790854057
15 -6.76335984165432
16 -7.17518201850917
17 -7.53409926614429
18 -8.00168314239638
19 -8.57636225427499
20 -8.8204359468072
21 -9.08286999031105
22 -9.19675074701505
23 -9.37522806143484
24 -9.72245516706625
25 -10.0400834702179
26 -10.2542573561906
27 -10.535813240014
28 -10.9069447479676
29 -11.2835100707955
30 -11.5048162588212
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.64022924122991
1 1.71327811106128
2 0.72236796313423
3 -0.294869747144288
4 -1.8938633535007
5 -3.43772083153393
6 -4.11401701353481
7 -4.57043747458774
8 -4.64505705055513
9 -4.99000494781279
10 -5.30090427326296
11 -5.89291121572403
12 -6.38767135930591
13 -6.73594020363016
14 -7.2604552677618
15 -7.60380811319157
16 -7.95954765315816
17 -8.24503100955795
18 -8.44516642336718
19 -8.50797612225042
20 -8.52361110231801
21 -8.13838237453051
22 -7.39478461269795
23 -6.62664339837971
24 -5.57486363586674
25 -4.80066397813377
26 -4.14311151075357
27 -3.23700812135997
28 -2.22032725317634
29 -1.60627193961401
30 -1.15021933193843
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.61885829580734
1 1.94915805760456
2 1.22383352414391
3 -0.02216403307653
4 -1.49072249942405
5 -3.07030812619425
6 -4.16579099122566
7 -4.73700105371939
8 -4.90590773297878
9 -4.8529658688856
10 -5.23130013471488
11 -5.58566103167539
12 -6.06087444279252
13 -6.73546428420346
14 -7.17597661710051
15 -7.82514559604774
16 -8.24315834509948
17 -8.44184966482311
18 -8.75100135242973
19 -9.17419157580833
20 -9.53526849960473
21 -9.98438393732612
22 -10.4326283034993
23 -10.9076855286004
24 -11.4603596827756
25 -11.772948178673
26 -12.012556761347
27 -12.1951747572752
28 -12.3441005547996
29 -12.4854737354639
30 -12.6399429122095
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.5660553080035
1 1.67638873050204
2 0.979705601883692
3 0.047898154446731
4 -1.46152873118941
5 -2.88037285629644
6 -3.98439846776902
7 -4.49134046335721
8 -4.45891576068768
9 -4.43954819835715
10 -4.7862289968677
11 -5.11692777686383
12 -5.69495799796698
13 -6.82540863015498
14 -7.902242042914
15 -8.69620839328299
16 -9.49985114838904
17 -10.1592760691149
18 -10.6185977940261
19 -11.261585020098
20 -11.7445220650359
21 -12.2419895027088
22 -12.6231547231476
23 -13.0994370094633
24 -13.4247235470261
25 -13.8261531207256
26 -14.2879673834573
27 -14.6947964555125
28 -15.1498975569324
29 -15.5808777552515
30 -15.9399857942012
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.59394154207384
1 1.83881873617905
2 0.94854560171281
3 0.0888701752565666
4 -1.24824773144074
5 -2.66033870712803
6 -3.87414705629032
7 -4.46531344948202
8 -5.01874621930662
9 -4.90171751049015
10 -5.04993338367951
11 -5.19334975883146
12 -5.2550609703491
13 -5.48658476487609
14 -5.66022614598145
15 -5.89814253490656
16 -6.13495328099924
17 -6.40931124436788
18 -6.83611986952017
19 -7.41512007364672
20 -7.57987541534788
21 -7.87957689868959
22 -8.07804053916899
23 -8.2623423477492
24 -8.62965826012577
25 -8.69178552424647
26 -8.92251774241569
27 -9.20289919507434
28 -9.43920266888743
29 -9.63472491330856
30 -9.85242770908508
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.57200936373513
1 1.67258234437459
2 0.779418405326091
3 -0.122591645818881
4 -1.37160991212387
5 -2.90106418644842
6 -4.16700922104597
7 -5.06238070627042
8 -5.38629682221757
9 -6.03335857946981
10 -6.81811368954928
11 -7.51779861646795
12 -8.15126985388349
13 -8.51488164148909
14 -9.11484086886143
15 -9.71047357069765
16 -10.4939631218315
17 -11.373781989494
18 -12.2662628135837
19 -13.0002049158246
20 -13.6675279943728
21 -14.1905979009257
22 -14.7393581093252
23 -15.2782968090476
24 -15.8250580587836
25 -16.1043241099269
26 -16.1589780502557
27 -15.8929701289468
28 -15.4958357584489
29 -14.8827159348656
30 -14.1788448665454
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.53013366710704
1 1.8644187199645
2 1.22292829878969
3 0.486265980506715
4 -0.773931206557283
5 -2.36427873386626
6 -3.87467028126259
7 -4.66419440851283
8 -5.17653249490913
9 -4.97167666449373
10 -4.54472450300785
11 -4.45518077411423
12 -4.55722356015043
13 -4.87993921408091
14 -5.3760028086219
15 -6.10038655396756
16 -6.73786285309607
17 -7.24235705432774
18 -7.45555337932801
19 -7.61078414350021
20 -7.60956585062644
21 -7.62610012053305
22 -7.55288840942831
23 -7.46317098605489
24 -7.27373950957709
25 -6.95300115421731
26 -6.450814311284
27 -5.89562160758557
28 -5.11020997469218
29 -4.14658623238152
30 -3.25314382052713
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.61040540779456
1 1.72507843582792
2 0.870678187774201
3 -0.211065030544736
4 -1.84159726136151
5 -3.50418559621706
6 -5.06615403713118
7 -5.77470233719864
8 -6.2004456703783
9 -6.36862729978168
10 -6.77041353109837
11 -7.22845929720133
12 -7.85360256891871
13 -8.67303653048413
14 -9.55125483523689
15 -10.2536695034096
16 -11.0714165417716
17 -11.5828848618951
18 -12.2219834868271
19 -12.7548511054524
20 -13.1331511547966
21 -13.5629893671033
22 -13.9909710634463
23 -14.2277215928993
24 -14.3950360850906
25 -14.635340923044
26 -14.9118407831019
27 -15.3200349120836
28 -15.7307417439259
29 -15.9802269176349
30 -16.3631875729478
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.60945486178865
1 2.01438982443939
2 1.39467293508276
3 0.31652486176902
4 -0.950263430615133
5 -2.39283770568486
6 -3.51087624938754
7 -4.05309854268936
8 -4.07511872217808
9 -4.04375383812741
10 -4.20826474971564
11 -4.33460319975261
12 -4.96310098563407
13 -5.84346890024524
14 -6.78492448527968
15 -7.55575054755473
16 -8.30665976610762
17 -8.98033669302752
18 -9.82896859471241
19 -10.4680213639546
20 -11.1528882240776
21 -11.8988350591872
22 -12.6969942314038
23 -13.1225045370278
24 -13.5588599587751
25 -14.0556967560758
26 -14.44666638153
27 -14.6828128396505
28 -14.5422206219301
29 -14.2565274427912
30 -14.2607609976672
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.54592252954759
1 1.73854730145679
2 0.624386141236043
3 -0.51655893971904
4 -1.86036711308073
5 -3.49931330876999
6 -4.81300106877705
7 -5.82054816952367
8 -6.53754199230276
9 -7.24941884903201
10 -7.72880214654928
11 -8.21864630864783
12 -8.57959990784021
13 -8.8938310735785
14 -9.32866527312564
15 -9.90310988085877
16 -10.3889169994475
17 -11.009812831906
18 -11.5829822769339
19 -12.2339334630837
20 -12.8913579582871
21 -13.5209547107773
22 -14.0253850074499
23 -14.4754329333193
24 -14.8992034043015
25 -15.2295606670596
26 -15.3182740174564
27 -15.3948060767647
28 -15.2254061784071
29 -15.0534992727044
30 -14.9095365686755
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.59558596998093
1 2.07310258098645
2 1.35327157814671
3 0.171114044234605
4 -1.19028035395825
5 -3.21713057148563
6 -4.46715406490941
7 -5.39533600399174
8 -6.14488650314776
9 -6.94339891944041
10 -7.80251834367276
11 -8.65911257666652
12 -9.55774265424772
13 -10.3505272789363
14 -11.1822840818556
15 -11.9235134102776
16 -12.6605619800695
17 -13.3204181276121
18 -13.9541850879283
19 -14.7442367893559
20 -15.5637709718065
21 -16.405031876233
22 -17.2252786095018
23 -17.9471296264357
24 -18.5309820413101
25 -19.062751556369
26 -19.5647195028073
27 -19.7602821901287
28 -19.8815081135255
29 -19.8660536043617
30 -19.6027956828397
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.5860081436349
1 1.75039932991718
2 0.815018190899819
3 -0.108229674316817
4 -1.1645316757472
5 -2.42713198986528
6 -3.34369165419961
7 -4.11241046392647
8 -4.52489146518634
9 -4.29914131921372
10 -4.18087609728892
11 -4.6125505623661
12 -5.11500860210078
13 -5.7703028073595
14 -6.55191396958981
15 -7.34762938095819
16 -8.13157290222169
17 -8.81324860384118
18 -9.06710712783205
19 -9.26489638514648
20 -9.72078495077195
21 -10.0392981975602
22 -10.4868187085106
23 -10.8783071188764
24 -11.0300301291456
25 -10.9054392714306
26 -10.6835998537599
27 -10.414871937279
28 -10.2050109840343
29 -10.0142400066684
30 -9.82477636696313
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.55416008905681
1 1.8231625699226
2 1.41651291468662
3 0.686520533391571
4 -0.511123345777545
5 -1.72074447439543
6 -2.8282932740101
7 -3.80618977015496
8 -4.08968642981282
9 -3.98263766414825
10 -3.87194809799167
11 -4.15836100983958
12 -4.45350832164445
13 -4.80743639641552
14 -5.14979616673702
15 -5.46131293796231
16 -5.96350326017177
17 -6.64462736605806
18 -7.41218015454881
19 -8.13369469650331
20 -8.7703516486602
21 -9.42018570014056
22 -9.90359941895344
23 -10.2549794443907
24 -10.582811372724
25 -10.8206630143044
26 -10.9941286990972
27 -10.8570869157363
28 -10.4904778266449
29 -9.92685267613351
30 -9.22040972999438
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.56337382322489
1 1.86739710289082
2 1.41537253263694
3 0.629472717771842
4 -0.489439402023976
5 -1.84173526556786
6 -3.20652789422512
7 -3.98136383199228
8 -4.36208423302221
9 -4.63620087532029
10 -5.06998831504304
11 -5.51093245565584
12 -5.97000953781828
13 -6.24471214210068
14 -6.62669641902644
15 -6.95215560227079
16 -7.26505821982665
17 -7.83150872779532
18 -8.60534579371598
19 -9.59648677283473
20 -10.2102274563018
21 -11.0240581087763
22 -12.0251591957092
23 -12.9517010237457
24 -13.7535859572503
25 -14.4827024021774
26 -15.0040353460015
27 -15.5058070704764
28 -15.9241348922557
29 -16.3043389813668
30 -16.4685619046939
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.58279825126452
1 1.97912281817446
2 1.18224631379708
3 0.168327999041118
4 -1.07992795541594
5 -2.38835315236267
6 -3.62199190286905
7 -4.58714909608253
8 -5.13400107801532
9 -5.33380877004227
10 -5.27969348835128
11 -5.52559677971796
12 -5.83701330779433
13 -6.1647780449166
14 -6.66577972172053
15 -7.19765512220496
16 -7.86698994370687
17 -8.83766122978245
18 -9.77950212877446
19 -10.6989767661986
20 -11.533830304667
21 -12.4126967703688
22 -13.1467829123651
23 -13.6110345000817
24 -14.2425940379731
25 -14.4774725057816
26 -14.3828934093444
27 -14.4652294374476
28 -14.6792139230506
29 -15.0628372265488
30 -15.4848324215849
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.61226911584806
1 2.08981534017867
2 1.27718317185143
3 0.234359947370434
4 -1.25593667598221
5 -2.84375808566015
6 -4.12442909824855
7 -4.78378006497338
8 -5.24186395493657
9 -5.4650919697746
10 -5.92590519395024
11 -6.58083140554713
12 -7.62698924876384
13 -8.12237651022022
14 -8.97300600500206
15 -9.45538422603641
16 -9.86848497969742
17 -10.2265781538402
18 -10.6575194549299
19 -11.2247429838118
20 -11.3364949379949
21 -11.5309334347765
22 -11.7846653301258
23 -12.0442917276224
24 -12.3060492883677
25 -12.2561960337556
26 -12.1071190314398
27 -11.8822345819203
28 -11.8703747723502
29 -11.7131883126832
30 -11.4626098363699
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.60585671527521
1 1.84060334148066
2 0.959811804001355
3 0.0781984748099447
4 -0.98580327810477
5 -2.83441606850514
6 -4.15210543024566
7 -5.10864134426013
8 -5.19767822896957
9 -4.82708461951647
10 -4.68099754093411
11 -4.84793793959128
12 -5.02077067643265
13 -5.43024542843853
14 -5.99330534444548
15 -6.6307114802205
16 -7.37048323945361
17 -7.93186060405975
18 -8.61544695062754
19 -9.08499244839995
20 -9.75922196692838
21 -10.3870573003201
22 -10.841650728344
23 -11.2124799324731
24 -11.422503059293
25 -11.4149621778544
26 -11.5952090467637
27 -11.6118230714413
28 -11.602700455988
29 -11.4577011865678
30 -11.2561777113771
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.57233012034296
1 1.76093139844058
2 0.726476298274019
3 -0.0128933069567569
4 -1.06370225766743
5 -2.57442362368768
6 -3.6908869235263
7 -4.41830627542883
8 -4.72598100201902
9 -4.79399087811361
10 -4.73160584488231
11 -4.88840148468194
12 -5.36687596765798
13 -6.10771113058559
14 -6.69422083846685
15 -7.38711257142676
16 -7.97265895834303
17 -8.65702382015743
18 -9.49669319703298
19 -10.2130409137715
20 -11.0602144660126
21 -11.8877998304252
22 -12.68794961229
23 -13.3585573168389
24 -13.8691810351601
25 -14.2660921541273
26 -14.7296031121588
27 -15.0246541896373
28 -15.2151130505302
29 -15.1617233038633
30 -15.204087749462
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.58615097405705
1 2.10389985948933
2 1.35944745321327
3 0.668826244758089
4 -0.627659858638149
5 -1.91544269447236
6 -3.05214056608043
7 -3.44087622507753
8 -3.44615816654637
9 -3.29355447658974
10 -2.99904231442512
11 -3.13522079203021
12 -3.4843690839587
13 -3.72302265195102
14 -4.00095813961766
15 -4.62272885856743
16 -5.1680612012666
17 -5.7423991568758
18 -6.37442997940476
19 -6.97504432356798
20 -7.66150647856451
21 -8.1502054834072
22 -8.58199623907391
23 -9.10864130570422
24 -9.47010608505875
25 -9.68692121678595
26 -9.97593883499557
27 -10.111589021334
28 -10.324202779849
29 -10.3302197821941
30 -10.3988475613486
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.56740680078734
1 1.68346527364392
2 0.879254592728131
3 0.237807576723297
4 -0.791654730500936
5 -2.2044070155871
6 -3.37173324294389
7 -4.05441928518716
8 -4.65538559100846
9 -5.08438038172289
10 -5.19304712980571
11 -5.54127158172864
12 -6.14874837233265
13 -6.88192979798752
14 -7.75096543871421
15 -8.73528459942136
16 -10.0002273548627
17 -11.1856152767142
18 -12.2286044806637
19 -13.0404059575558
20 -13.9241382083368
21 -14.7254214608546
22 -15.4364254364397
23 -15.9610042552867
24 -16.2559389289833
25 -16.7512566589514
26 -17.2360691500722
27 -17.7116992217583
28 -17.979379001383
29 -18.3346909328943
30 -18.8758575002469
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.59184880038185
1 1.88412191279165
2 1.2085416127928
3 0.152001326177508
4 -1.2392276836931
5 -2.52728396244372
6 -3.56470282720577
7 -4.37131928269212
8 -4.70505400187733
9 -4.79719157099768
10 -4.91104981005472
11 -5.19158505031976
12 -5.78028795266254
13 -6.70641269749384
14 -7.57226739590083
15 -8.16168675812041
16 -8.73564367337157
17 -9.45321924849287
18 -10.0808514197299
19 -10.7682217629451
20 -11.2749277410322
21 -11.7517584197827
22 -12.3144671503362
23 -12.8836981321712
24 -13.4642624298389
25 -13.9950978417816
26 -14.4292807556863
27 -14.8318701750037
28 -15.2154116929025
29 -15.5697294330081
30 -15.8189084868799
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.60986476262342
1 1.98685123487091
2 1.3514281340634
3 0.586439908031849
4 -0.534697646704139
5 -1.78234481652427
6 -2.4548693792049
7 -3.01124425109099
8 -3.19377317023513
9 -3.28706712709819
10 -3.23884088223974
11 -3.54386404418856
12 -3.79322849157443
13 -4.20806930155226
14 -4.77652622498622
15 -5.71720167229893
16 -6.43762517895829
17 -7.4277471561512
18 -8.22652758427814
19 -9.06068415157229
20 -9.64198277453975
21 -10.264364810827
22 -10.7772356458152
23 -10.9848458837001
24 -11.0780777047967
25 -10.9708421225861
26 -10.6400931815723
27 -10.2073924793149
28 -9.65660347555152
29 -8.83475092597075
30 -7.69182359608852
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.58151599603352
1 1.63116891505541
2 0.967745642280551
3 0.184172689430484
4 -0.804934366488949
5 -2.29999522633651
6 -3.20231717015071
7 -3.59352813263587
8 -3.72896211695002
9 -4.05986448654618
10 -4.63274101692962
11 -5.11424006910302
12 -5.96647261015809
13 -6.44835586007135
14 -7.16481115085801
15 -7.92636274767276
16 -8.79045403043243
17 -9.60112210988002
18 -10.3910391748896
19 -10.7949714346158
20 -11.4407836085492
21 -11.8423746588827
22 -12.1880559930319
23 -12.576257450935
24 -12.7605242571441
25 -13.0564230582513
26 -13.2891878843285
27 -13.7368583860306
28 -14.1347876045634
29 -14.3337365071518
30 -14.637469882548
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.59964526061438
1 2.0208164203378
2 0.989345382852148
3 -0.335917861261089
4 -1.54806761964086
5 -3.36919408220308
6 -4.11423064698049
7 -4.77662137116491
8 -5.10965099390934
9 -5.32618834529792
10 -5.36094336809398
11 -5.75520437531639
12 -6.30550199529044
13 -6.85837869768342
14 -7.40735285098066
15 -7.75860731407163
16 -8.19814720518718
17 -8.39857948791274
18 -8.96627112141615
19 -9.46811045251059
20 -9.66300571786397
21 -9.95884413841505
22 -10.1933058085163
23 -10.5180875076103
24 -10.8425637274549
25 -11.0912992720252
26 -11.4038957773396
27 -11.7845592154742
28 -12.1456478724725
29 -12.3837231979828
30 -12.7024905202935
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.52756644813553
1 2.06177919606358
2 1.33313648687384
3 0.39101801634556
4 -0.869472061210624
5 -2.08209740887194
6 -3.00691337181187
7 -3.51317780454296
8 -3.63137504572215
9 -3.39543711020286
10 -3.2117411599448
11 -3.37780145127953
12 -3.6363484056773
13 -4.05283271403519
14 -4.6292755322788
15 -5.24066110583613
16 -5.73757568409107
17 -6.28512433043765
18 -6.8256369970534
19 -7.26423505626463
20 -7.99106566134386
21 -8.44366572669676
22 -8.96167835748522
23 -9.38528546890184
24 -9.92603116418912
25 -10.3570579166268
26 -10.7889713419245
27 -11.1941588629608
28 -11.6345422713029
29 -11.9858873735547
30 -12.2688517582632
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.56235724180504
1 1.83636253947758
2 0.943184831394264
3 -0.0985167426319862
4 -1.60113209268935
5 -2.9122987030068
6 -3.78837979200262
7 -4.28424253526838
8 -4.52293651241294
9 -4.77664215641606
10 -5.33959533488346
11 -5.97502056585393
12 -6.86738918302042
13 -7.87343939386061
14 -8.70462905440877
15 -9.76315118088608
16 -10.9990205303167
17 -12.160384324867
18 -13.3313251771797
19 -14.4814101513374
20 -15.4075707820587
21 -16.1750994902325
22 -17.0007584594083
23 -17.5723259507396
24 -18.1569047581433
25 -18.8271685995431
26 -19.4465361630146
27 -20.0378544040739
28 -20.8728459732175
29 -21.478164520077
30 -21.8723154193949
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.56180181974371
1 1.91226484827307
2 0.98063827456161
3 -0.0710377986119202
4 -1.33819627295682
5 -3.03207337781169
6 -4.05359173760407
7 -4.66442725300196
8 -4.94187845888051
9 -4.89185619942363
10 -5.08983123762046
11 -5.58169198496982
12 -6.26418939980375
13 -6.84963076568974
14 -7.54324525231415
15 -8.19745457399098
16 -8.70528360730402
17 -9.18608241643248
18 -9.5603402955011
19 -9.79391898255693
20 -9.82202345975399
21 -9.89523591577292
22 -9.75875971656389
23 -9.47278252717508
24 -9.26531557560499
25 -9.06215470624731
26 -8.7329950152741
27 -8.38056630686481
28 -7.82633897754652
29 -7.03926163755221
30 -6.17387891603136
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.54402041007276
1 1.95615872827082
2 1.0382526245972
3 -0.0281881407386262
4 -1.25648001934781
5 -2.8972780379064
6 -4.08410044768992
7 -4.50635760457118
8 -4.69190718506054
9 -4.74188800158716
10 -4.62830587274641
11 -4.52504763745873
12 -4.51772338276115
13 -4.91828041581863
14 -5.53554702634147
15 -6.07091515998927
16 -6.46436716138568
17 -6.75096449481834
18 -6.78077006106773
19 -7.02836200458708
20 -7.24331497343596
21 -7.42036548799136
22 -7.62690418227454
23 -7.67755233892925
24 -7.79046600366669
25 -8.17881980381256
26 -8.18540805394667
27 -8.0590201576216
28 -7.83783808664226
29 -7.640678677273
30 -7.30632090161254
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.58991519130201
1 1.94424333451902
2 1.00984963482983
3 -0.159937705684165
4 -1.69932623543248
5 -3.22422335179774
6 -4.30425202167625
7 -4.74291209490619
8 -4.88064702367361
9 -4.81792126552447
10 -4.63402376074769
11 -4.41909051681253
12 -4.62758868765728
13 -4.65860334536315
14 -5.01842838918616
15 -5.63628294787081
16 -6.27143178933649
17 -7.03151439917189
18 -7.51851778055329
19 -7.84991846369585
20 -8.13265451396195
21 -8.28349888995252
22 -8.38470941178066
23 -8.4815147402143
24 -8.52571498619406
25 -8.78251790724761
26 -8.8491276473464
27 -8.90678364185006
28 -8.66920363067448
29 -8.44697068431976
30 -8.38709164663563
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.52908745749639
1 1.8488104082524
2 1.21887486227418
3 0.41360290756838
4 -0.848018155651273
5 -2.18339603088356
6 -3.11362571748913
7 -3.93513384122541
8 -4.09836032223066
9 -4.03723486538661
10 -4.01864790499895
11 -4.11581318583278
12 -4.31780196709949
13 -4.61993940068042
14 -5.50591599291495
15 -6.60290815973373
16 -7.67034093128196
17 -8.67465878406591
18 -9.76565141768878
19 -10.8080325854813
20 -11.676009989837
21 -12.4256516117847
22 -13.1641228753517
23 -13.7393826267433
24 -14.2209423316069
25 -14.4786150295521
26 -14.5098300618081
27 -14.4853274592774
28 -14.3334179999039
29 -13.8806245344138
30 -13.2663478576151
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.58472090055175
1 1.89399592310526
2 1.06914252624795
3 0.115974444324793
4 -1.24161469108026
5 -2.53007684623845
6 -3.87066803779173
7 -4.62552499597895
8 -4.81638623452528
9 -5.01968243028775
10 -5.24857690916606
11 -5.57381158630775
12 -6.00578423447895
13 -6.61009447582213
14 -7.39362627111143
15 -8.081403748902
16 -8.92867930914557
17 -9.5515695244179
18 -10.1970907118469
19 -10.6985269037472
20 -11.2286793350081
21 -11.7098414759466
22 -12.2597000462008
23 -12.5604227924979
24 -12.8052319278379
25 -13.0303205426142
26 -13.0644832425529
27 -13.1163481034092
28 -13.198266321413
29 -13.3322479165975
30 -13.5328905098907
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.55909511826957
1 2.18316662106576
2 1.69111888285364
3 0.993342874529313
4 -0.243468119698422
5 -1.72377807942131
6 -3.00714984016732
7 -3.93256492932155
8 -4.5508887438158
9 -4.66981313549091
10 -4.7437522364129
11 -5.19895667619832
12 -5.71958219387985
13 -6.29104068490918
14 -6.98007392919469
15 -7.63622141582892
16 -8.59005918623335
17 -9.21936920272106
18 -9.81703658321515
19 -10.4278328916119
20 -10.7980508488866
21 -10.8612740225274
22 -10.8180715843251
23 -10.8406430581814
24 -10.9574317359777
25 -10.9605052147919
26 -10.693838443506
27 -10.3876147645112
28 -10.1079999558702
29 -9.44809974673022
30 -8.81509028918225
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.51785928080706
1 2.02413794693784
2 1.34563412140293
3 0.453332522617611
4 -0.680442610981112
5 -1.73511230782846
6 -3.2499737545974
7 -3.99961511662813
8 -4.50032346344179
9 -4.72525288393383
10 -4.78658706113132
11 -4.77706355413433
12 -4.86509407291713
13 -5.08433179133555
14 -5.39082548020095
15 -5.60279752354434
16 -5.84028040878586
17 -6.01513593410836
18 -6.29120836341089
19 -6.65604280477246
20 -6.8318101805913
21 -6.95924346655023
22 -6.97516502901132
23 -6.91757062213201
24 -6.86641984565527
25 -6.85943502619008
26 -6.82288885309283
27 -6.64880754176003
28 -6.53729237633627
29 -6.32862770005886
30 -5.93160706098313
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.57772310968083
1 1.87868529017138
2 1.10413135282698
3 0.242991505525691
4 -0.922013349469598
5 -2.72144356519903
6 -3.57814809847398
7 -4.21653610849847
8 -4.46237465790717
9 -4.31865336780478
10 -4.28790638792036
11 -4.15309386081955
12 -4.34877210197381
13 -4.44042680738473
14 -4.70163241885488
15 -4.9508513795039
16 -5.12480163752217
17 -5.39887006877671
18 -5.48391212044468
19 -5.39288052000059
20 -5.53992787329638
21 -5.58890952395302
22 -5.5440630371288
23 -5.42735929028421
24 -5.27934407520024
25 -5.03040764895198
26 -4.88616243718616
27 -4.64642037959826
28 -4.39076999691624
29 -4.0669397866078
30 -3.66203923451014
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.55334727409384
1 1.8138709267691
2 1.21410667684099
3 0.192112362957518
4 -0.950013900521926
5 -2.36495511692116
6 -3.68430331875495
7 -4.75464788353567
8 -5.55377149997651
9 -5.27440048153996
10 -4.89775983471512
11 -4.80650015466048
12 -5.0082286522864
13 -5.35790063241102
14 -5.82790836582809
15 -6.47989278371536
16 -7.25337251950255
17 -8.02296864204558
18 -8.51388487466437
19 -8.82620432700475
20 -8.98048341385852
21 -9.08832462588177
22 -9.39861811507339
23 -9.50700562748511
24 -9.70849926113758
25 -10.1605982339289
26 -10.3945893164626
27 -10.5936172969765
28 -10.7304422319348
29 -10.8322689943914
30 -10.9639303657083
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.6067545936119
1 2.0693794065412
2 1.32483083204958
3 0.0967088105126823
4 -1.04282984730772
5 -2.31883080671319
6 -3.2632432594221
7 -4.07714574216057
8 -4.24072304888573
9 -4.04650091027536
10 -3.94342975051507
11 -4.17790056529243
12 -5.01382173843982
13 -5.83861817550497
14 -6.84200451112848
15 -7.73984957986624
16 -8.62809021871571
17 -9.43996547251643
18 -10.2814416029381
19 -10.9069713086157
20 -11.4101198027893
21 -11.8170466405479
22 -11.8760234260056
23 -11.9683464054143
24 -11.9854342455971
25 -11.7915901204393
26 -11.5614540089026
27 -11.4540043496169
28 -11.1194168031403
29 -10.7256002105539
30 -10.1555008715472
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.52973730118742
1 1.85036875598391
2 1.15470727873849
3 0.230362940872702
4 -1.32648795880722
5 -3.22932402118461
6 -4.58371812892138
7 -5.4116940388743
8 -5.9847953510542
9 -6.24093266760177
10 -6.81542629073253
11 -7.2277194298545
12 -7.72149306053902
13 -8.38314188612024
14 -9.12099645163753
15 -9.77706523286952
16 -10.2024360997968
17 -10.704498306281
18 -11.0786454139072
19 -11.4989424216665
20 -11.9075416500476
21 -12.4631009674171
22 -13.1224142373053
23 -13.8730249974237
24 -14.5688028156184
25 -15.1066190058782
26 -15.5404075437294
27 -15.9020583184853
28 -16.1319141149196
29 -16.1461204549811
30 -16.0359506018227
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.61360228473863
1 2.04998770912212
2 1.38432919194333
3 0.40943372375858
4 -0.755772373603804
5 -2.35543577482133
6 -3.40130901743378
7 -4.16255714924794
8 -4.54845753790424
9 -4.59528919587192
10 -4.48004445781154
11 -4.68720367843167
12 -5.22040855833858
13 -5.95720530711591
14 -6.4803733284041
15 -7.0165296386079
16 -7.40985063323924
17 -7.93340266910379
18 -8.32203154152124
19 -8.69035453468878
20 -9.04456256040242
21 -9.18982281884043
22 -9.36545392216959
23 -9.42337844952406
24 -9.27826256335005
25 -9.46273121288722
26 -9.37105564561544
27 -9.24823526759545
28 -9.12047724059878
29 -9.0226940058087
30 -9.08252846379234
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.60819622182143
1 2.04664938253157
2 1.26929070277044
3 0.495105991873009
4 -0.657603201351099
5 -1.95827248262261
6 -2.56392243328977
7 -2.86178490932492
8 -2.82916708239537
9 -2.28854972756114
10 -2.07974397431591
11 -2.22324841625815
12 -2.58001972397548
13 -3.34777052632488
14 -4.29611396907461
15 -5.35061460201422
16 -6.08784089639542
17 -6.73276694719209
18 -7.13929186240844
19 -7.5587582109048
20 -8.26987688681209
21 -8.91577775163705
22 -9.45188088719898
23 -9.69307359079292
24 -9.85357419702944
25 -10.2278740098909
26 -10.46335932216
27 -10.6076817120729
28 -10.8254677097793
29 -11.1505885037907
30 -11.4757071667667
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.59445478226359
1 1.88909419485651
2 1.19010584780113
3 0.161191850666093
4 -1.13927702820339
5 -2.71563726194457
6 -3.70072802971115
7 -4.33403961539811
8 -4.60041205891728
9 -4.56957023520504
10 -4.63189876568919
11 -4.59986670900174
12 -4.74365722373605
13 -4.99603658006675
14 -5.31164443944144
15 -5.88710493072442
16 -6.34378658533087
17 -6.79312721031558
18 -7.31716543964376
19 -7.64368184387036
20 -7.88528030158383
21 -8.12319405223628
22 -8.34272625787484
23 -8.58800116591692
24 -8.69413987457172
25 -8.73858805370606
26 -8.64034155446474
27 -8.69095439903616
28 -8.62584491547664
29 -8.3480793747668
30 -8.13957990246867
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.61968834532443
1 2.06575605918304
2 1.23030087630818
3 0.188866027892473
4 -1.00853557146363
5 -2.24736970305401
6 -3.52485865147437
7 -4.18412915040984
8 -4.35550732959577
9 -4.30134324437263
10 -4.30363444679331
11 -4.41239915553579
12 -4.79223382067713
13 -5.49787498388087
14 -6.16243571743898
15 -6.76861577631014
16 -7.57844050820961
17 -8.23207062359585
18 -8.83791451237601
19 -9.37344417661017
20 -9.64825664883723
21 -9.97331038865418
22 -10.3089986252916
23 -10.5717482400698
24 -10.8947991881329
25 -11.1408308638286
26 -11.1563635440409
27 -11.1723155151061
28 -11.0696867926735
29 -10.6923384261979
30 -10.2188916082268
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.58443350027261
1 2.26620446083673
2 1.88347058213828
3 1.17419462320222
4 0.38503143666699
5 -0.011413709059088
6 0.813877518799844
7 1.9486200013745
8 3.96770801284738
9 5.2074719712305
10 5.20835879798391
11 4.35386425048564
12 4.31229385803566
13 4.60810869258249
14 4.91698075838841
15 5.46060673572289
16 5.51501671016019
17 5.31295331926782
18 4.9403817009534
19 4.5540414663256
20 4.32816302776938
21 4.19178247027943
22 4.07334645151515
23 3.90254584527311
24 3.61920404750846
25 3.50425461044949
26 3.46320066631873
27 3.31222237726664
28 2.88423265834417
29 2.23422315614371
30 1.64933640064382
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.61518079532923
1 1.87903933693803
2 0.984693796751293
3 -0.0957021373525198
4 -1.67236256347655
5 -3.40051322496984
6 -4.43800939792141
7 -5.07704269788831
8 -5.38473736185427
9 -5.60104426078059
10 -6.02655892045709
11 -6.24650818151336
12 -6.2051285808236
13 -6.12217684985462
14 -6.37365079313689
15 -6.76762270072764
16 -7.1053755942849
17 -7.90427657554297
18 -8.65800144886719
19 -9.2054155841655
20 -9.45724542908365
21 -9.95957174186266
22 -10.2847976850566
23 -10.662933183069
24 -11.0151810296452
25 -11.3992479977225
26 -11.8519085465815
27 -12.2172282523108
28 -12.6109443177335
29 -13.0088342287361
30 -13.3374507682192
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.59971414529843
1 1.89790475725714
2 0.942846292090106
3 -0.111204636714193
4 -1.47797684040556
5 -3.09099861627684
6 -4.84274245884554
7 -5.78901352255955
8 -6.14003029800488
9 -6.53372506460287
10 -6.65579653773192
11 -6.98426098221321
12 -7.30922387717778
13 -7.67482889386112
14 -8.45821908397691
15 -9.26072796990963
16 -10.0663137074851
17 -10.6121862290543
18 -11.1909923535588
19 -11.7161362611303
20 -11.7573358455432
21 -11.6451122379924
22 -11.6006932459398
23 -11.575151118645
24 -11.2600279397276
25 -10.5552672081041
26 -9.5493513465663
27 -8.53829546977372
28 -7.2053593157052
29 -5.96545655506008
30 -4.70201840001173
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.55129538238551
1 1.92966312486983
2 0.928670448211498
3 -0.314339874892589
4 -1.53578117985538
5 -3.09456547594655
6 -3.97004724416641
7 -4.38515334923883
8 -5.04901053565459
9 -5.16751716034294
10 -4.92215776942701
11 -5.34529670130773
12 -5.96454795474966
13 -6.60772442011017
14 -7.12095467845544
15 -7.79028623817143
16 -8.33896600840944
17 -9.08533731116715
18 -9.21788822232873
19 -9.42915045704448
20 -9.78799270531732
21 -9.88508399969377
22 -9.88599056206102
23 -9.92947066779491
24 -10.006021756784
25 -9.87997380307714
26 -9.96041681327151
27 -9.79099675392318
28 -9.63992149974572
29 -9.56201257912993
30 -9.39595959687294
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.57660112438852
1 1.89576427766026
2 1.04149827532577
3 0.0860615746727564
4 -1.1021754082977
5 -2.53678536377072
6 -3.48053321821665
7 -3.83425907705938
8 -4.30530704085182
9 -4.51935946586397
10 -4.95128912439943
11 -5.33078837739585
12 -5.39849458780149
13 -5.56123791391275
14 -6.10631609722486
15 -6.49594060178899
16 -7.18257694499574
17 -7.94008094251271
18 -8.93745794530673
19 -9.98259225887411
20 -10.9139597721133
21 -11.6857306373477
22 -12.4660813901242
23 -13.363660951458
24 -14.0145440836112
25 -14.5324438907929
26 -14.9329699746305
27 -15.2830562119544
28 -16.0235142398353
29 -16.6195503198351
30 -17.2216552560419
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.57804434950166
1 1.98958998154364
2 1.65754930311521
3 0.894092609111162
4 -0.0978884288575834
5 -0.96470997516581
6 -2.15502777756998
7 -2.88521004747108
8 -3.33572385858063
9 -3.33993701480905
10 -3.41122040346366
11 -3.67352732933198
12 -3.85839683771649
13 -4.11427840239057
14 -4.3640782631462
15 -4.82535030251561
16 -5.37401832839077
17 -6.03965198735737
18 -6.68420332628908
19 -7.39057259993945
20 -8.2654858570859
21 -9.04753455301828
22 -9.77449692098893
23 -10.5013324720525
24 -11.1662704683324
25 -11.5023138121469
26 -12.0520126863205
27 -12.6108418023769
28 -13.0865358179406
29 -13.4395706360791
30 -13.5936896322283
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.5626775443893
1 1.92323000410951
2 1.05271048691007
3 -0.186886685587575
4 -1.21711369334827
5 -2.48559083784284
6 -3.77354681095777
7 -4.68990295769572
8 -5.13153110004592
9 -5.23347194318242
10 -5.14836665488427
11 -5.24195247303729
12 -5.70527914278038
13 -6.05672228712577
14 -6.56757277750801
15 -6.98506846212832
16 -7.43857191911945
17 -8.03074126606215
18 -8.4997926514516
19 -8.76815043969443
20 -9.27051415306204
21 -9.71661114432597
22 -10.0929220574776
23 -10.4817852968376
24 -10.7594515347628
25 -11.1077374894137
26 -11.46945202311
27 -11.7938881745741
28 -11.941007660053
29 -12.1811426146832
30 -12.3587326069851
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.5779547045773
1 1.93447943652996
2 1.07632926245993
3 -0.0402366702388139
4 -1.78173933980767
5 -3.38446723614536
6 -4.79477861317916
7 -5.76033776623877
8 -6.27099212838661
9 -6.52561429841106
10 -7.11260661756477
11 -7.61179735045966
12 -7.97110254742056
13 -8.31584708856752
14 -8.63404874105012
15 -9.19910880820475
16 -9.84595814894142
17 -10.4473167627182
18 -11.30361805497
19 -12.2152765779149
20 -12.9886876445992
21 -13.7033479004799
22 -14.1790162679644
23 -14.7498645553713
24 -15.3502950691639
25 -15.8794859334625
26 -16.3841394522617
27 -16.7378103645816
28 -17.088816550178
29 -17.5252910372638
30 -17.9499802310671
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.6429667873514
1 2.09351748747166
2 1.34773858378286
3 0.147113214064698
4 -0.960951485899226
5 -2.41373899276415
6 -3.32013433416935
7 -3.95874125194639
8 -4.45292678591248
9 -4.6803549157261
10 -4.66213920625499
11 -4.88310501942612
12 -5.87255005916794
13 -6.67588683200285
14 -7.2677872138801
15 -7.88371613624785
16 -8.62417462375884
17 -9.44712128616225
18 -10.2289819004658
19 -10.9522519327127
20 -11.6630224008846
21 -12.3809403375366
22 -12.9280383541086
23 -13.6230171321876
24 -14.138812870361
25 -14.6367873620066
26 -14.9508358909936
27 -15.2531868340629
28 -15.6763284252451
29 -16.0767490519549
30 -16.27003690999
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.59400138079674
1 1.96817361207128
2 1.37661862256756
3 0.464264739790638
4 -0.706419393333032
5 -2.4510938968449
6 -3.11017898248319
7 -3.49812326177136
8 -2.9729459080635
9 -2.4333562233138
10 -1.96936864987522
11 -1.68025605077503
12 -1.6815277361165
13 -2.26483823385045
14 -2.94645215743316
15 -4.11637488050902
16 -4.94538660675174
17 -5.62516950521987
18 -6.09143046748146
19 -6.47425766219463
20 -6.86300399024302
21 -7.30643945206717
22 -7.58833685347204
23 -8.10137427143721
24 -8.6895330749823
25 -9.19161096960573
26 -9.59503082968837
27 -9.86206760210578
28 -10.2305014113756
29 -10.5274799146894
30 -10.783796179904
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.52516752067809
1 1.85483321783949
2 0.884359776398567
3 -0.126342986952016
4 -1.25468872907194
5 -3.0221376516792
6 -3.74920892732618
7 -4.76089798393448
8 -4.9984234133399
9 -4.75465732348309
10 -4.36341271903514
11 -3.93564333848753
12 -3.74321459216112
13 -3.79685444302686
14 -4.07435522048609
15 -4.71872465088695
16 -5.72278062232199
17 -6.55851271651152
18 -7.42810150864871
19 -8.17592532325311
20 -8.84723246657974
21 -9.37041335761668
22 -9.6788219796761
23 -9.70649588931695
24 -9.92143459105059
25 -10.2669662962329
26 -10.6833555158935
27 -10.8952971329145
28 -11.1529798328655
29 -11.2514539319333
30 -11.3321746055869
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.54553618570674
1 2.0269075650876
2 1.47351512970387
3 0.986964255147821
4 -0.03106661862296
5 -1.36599151602079
6 -2.27925653617659
7 -3.16258059988925
8 -3.49477236048334
9 -3.41882426741459
10 -3.19459826085922
11 -3.07152938372999
12 -3.14180965072087
13 -3.02575586195005
14 -2.868724821185
15 -3.02241646852796
16 -3.39117602711752
17 -3.79346502091664
18 -4.18899659113561
19 -4.83269564628836
20 -5.41848564369526
21 -5.70443994254825
22 -6.0522680739925
23 -6.24665561590917
24 -6.47064975493709
25 -6.81182147516382
26 -7.08823524542376
27 -7.23581046732262
28 -7.34588494944238
29 -7.37009916257278
30 -7.31650383272452
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.59387905675876
1 1.8960635391129
2 1.0246590581235
3 -0.254338027816242
4 -1.97489138277323
5 -3.80810786619815
6 -5.22151971698885
7 -6.19103943573547
8 -6.99982395776772
9 -7.83679575704528
10 -8.44829208184212
11 -9.05734967768798
12 -9.52013923616307
13 -10.2241453035122
14 -10.9471785517594
15 -11.7482325001107
16 -12.653473555105
17 -13.5739623656868
18 -14.1461741669782
19 -14.7631939334536
20 -15.6195301791877
21 -16.4716204849132
22 -17.4121012528584
23 -18.4791414405891
24 -19.3747884578368
25 -20.2423327404941
26 -20.7991633153636
27 -21.1734124403749
28 -21.6248867801424
29 -21.8000238772587
30 -21.906312738515
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.59958769962293
1 2.15007068932733
2 1.51609886833207
3 0.804009260267897
4 -0.281464384276978
5 -1.49965750030188
6 -2.34751654118479
7 -3.25669065792852
8 -3.4184774307419
9 -3.15395859371996
10 -3.06270932507831
11 -3.14745600288646
12 -3.57352945403129
13 -3.93253094098529
14 -4.42823548002331
15 -5.02178375557241
16 -5.72053467685244
17 -6.52434341322824
18 -7.41084377867488
19 -8.42793856119638
20 -9.24440970081736
21 -10.0652049047216
22 -10.7583125019046
23 -11.2325310411379
24 -11.7156509656349
25 -12.1539176353049
26 -12.779371886291
27 -13.4723815467475
28 -14.0818068184063
29 -14.6269767071342
30 -15.2476326761063
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.60910645484497
1 2.28194083009546
2 1.66940070978104
3 0.987339400148084
4 0.0371319430609311
5 -1.43358247841043
6 -2.15858250197119
7 -2.27797069750735
8 -1.9617789141908
9 -2.14091121980679
10 -2.37779792854881
11 -2.84387586341744
12 -3.40571070606552
13 -4.07896422093802
14 -4.65029694729221
15 -5.19405206335253
16 -6.01217398277625
17 -7.05912998072174
18 -7.87774586162665
19 -8.584620380981
20 -9.02401034629543
21 -9.67774919502764
22 -10.3529895885358
23 -10.8494331464863
24 -11.4787417458473
25 -12.0180026118524
26 -12.4129205354772
27 -12.8386777610604
28 -13.4987418952746
29 -13.9692307372515
30 -14.4506235609784
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.56535697160461
1 2.0434843149427
2 1.35083570947635
3 0.381066514603049
4 -1.00001571657461
5 -2.46769424391122
6 -3.53689497980666
7 -4.00427515768305
8 -4.312528246965
9 -4.27563725448858
10 -3.99571912676801
11 -4.18045206428131
12 -4.88884548936888
13 -5.51831861972014
14 -6.33581366442414
15 -6.91041373802206
16 -7.57230496679131
17 -8.45851480557603
18 -9.11509104797816
19 -9.79975154832061
20 -10.4552987677564
21 -11.2277347497818
22 -11.8627072322639
23 -12.6305223286147
24 -13.4690584252648
25 -14.0743196711367
26 -14.8766510729111
27 -15.5546610621525
28 -16.0040628827942
29 -16.338290182761
30 -16.6387250393335
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.59352028655961
1 2.26973476935844
2 1.79049243898577
3 1.05870089713797
4 0.0646698335632774
5 -1.2449136908647
6 -2.45321775569741
7 -3.17674616110784
8 -3.47585592999844
9 -3.53423147867374
10 -3.55115323109104
11 -3.73670345244182
12 -4.2405679717854
13 -4.68704158276389
14 -5.369026473628
15 -6.26021714547497
16 -7.07708205860974
17 -7.76011451245008
18 -8.30405978575118
19 -8.67060449030138
20 -9.07439695823984
21 -9.37605529079406
22 -9.92592961790488
23 -10.4055095018898
24 -11.0299270527494
25 -11.795482021851
26 -12.2440332811245
27 -12.5733091635236
28 -13.0198108904019
29 -13.4177557160083
30 -13.716248548253
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.60071769032539
1 2.13719686205316
2 1.49875132495082
3 0.671949145070643
4 -0.438938230349727
5 -1.33863289555693
6 -2.42998431438838
7 -3.14438126782689
8 -3.64580324824587
9 -3.93286287870817
10 -3.83525329730395
11 -3.55249555567193
12 -3.58062987742252
13 -4.10560644115189
14 -4.7091813652333
15 -5.47277802228841
16 -6.24781129764861
17 -6.76125014176294
18 -7.44662138455177
19 -7.9715769669908
20 -8.38260390198339
21 -8.9667807069358
22 -9.47082201589483
23 -10.0067432604752
24 -10.7951858467851
25 -11.254777086307
26 -11.653665704375
27 -11.8100637653375
28 -12.0301433628577
29 -12.3197566569903
30 -12.5192129879667
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.57543244791755
1 1.74246994125064
2 0.927315642374261
3 -0.330458288070616
4 -1.82071351053884
5 -3.11225141877527
6 -4.38732534207158
7 -5.05691536610458
8 -5.43762700232124
9 -5.82857294964546
10 -6.24257932346857
11 -6.77628833096415
12 -7.19045517126679
13 -7.64379378839586
14 -8.1754326931491
15 -8.68269828811842
16 -9.08602251526771
17 -9.62947275582865
18 -10.2718486338416
19 -11.1212359410596
20 -11.7575201991874
21 -12.3443371967999
22 -12.4851666960888
23 -12.6400832729879
24 -12.5904418412265
25 -12.5251243752164
26 -12.2898729086145
27 -11.863272806082
28 -11.4643038750222
29 -10.9296148582686
30 -10.2021553375575
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.62322403174277
1 1.72608272865772
2 1.00115686362671
3 0.274372018892564
4 -0.837600655151387
5 -2.4634675143449
6 -3.38638171714515
7 -4.02389322747159
8 -4.23145204696068
9 -4.34706110071602
10 -4.45616400732981
11 -4.77321031928531
12 -5.30783609566148
13 -5.88559691411552
14 -6.43825580659762
15 -7.01923125093501
16 -7.68539174485934
17 -8.37536462029749
18 -9.15789477897943
19 -9.81450009218178
20 -10.4223933213441
21 -11.0934336556508
22 -11.4953040893686
23 -12.1582420439948
24 -12.7330152894775
25 -13.1293948402275
26 -13.5125204202943
27 -13.664588336317
28 -13.7621320155342
29 -13.5469662893111
30 -13.2268455617268
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.57215213974241
1 1.6745945573036
2 0.826401316565846
3 -0.364898919441302
4 -1.69725008764092
5 -3.19937663657011
6 -4.35512631530838
7 -4.87157331673136
8 -5.19009367136473
9 -5.2137248578873
10 -5.04492534504358
11 -5.06966312122932
12 -5.28174394159703
13 -5.7612647896554
14 -6.47702550642145
15 -7.41372535363127
16 -8.32374777534521
17 -9.01797682538716
18 -9.73176057808543
19 -10.2959964634513
20 -10.9147112056426
21 -11.3158159693939
22 -11.4490604678369
23 -11.2832129531659
24 -11.0900394554239
25 -10.8821750395159
26 -10.3742279960404
27 -9.99951132903309
28 -9.81951120795417
29 -9.6294733921513
30 -9.19702452478487
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.59668344554391
1 1.92917066682434
2 1.11816981882059
3 0.384785403698734
4 -0.781826109223976
5 -2.19767650952821
6 -3.08499836441799
7 -3.66143135473484
8 -4.07819859356573
9 -3.97079469091955
10 -4.06929684094188
11 -4.537699184082
12 -5.55749547215079
13 -6.43798820791006
14 -7.38463495326351
15 -8.02688867550927
16 -8.69533476613094
17 -9.10548535046273
18 -9.69911062232888
19 -10.38566501555
20 -10.9237844490359
21 -11.4557392001565
22 -11.9493872082846
23 -12.3648588955473
24 -13.0128854800688
25 -13.4049689562624
26 -13.6468463458867
27 -13.9951025520059
28 -14.3660663894174
29 -14.7051034536837
30 -14.905458761307
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.58567944566339
1 1.76180717694452
2 1.13925289154986
3 0.0739332333092779
4 -1.22472665875627
5 -2.85206192519988
6 -4.14161162286193
7 -5.02730776736422
8 -5.25341603907153
9 -5.37417889808461
10 -5.4340877436559
11 -5.58963566456359
12 -6.13122958907642
13 -6.86513858624279
14 -7.68486278723395
15 -8.44330653307983
16 -9.01892462962706
17 -9.72401499433973
18 -10.4437826246541
19 -11.13287966084
20 -12.0395967368653
21 -12.8740444212838
22 -13.7783895909167
23 -14.6302560647059
24 -15.4220524144411
25 -15.9589202208214
26 -16.5976295019953
27 -17.053132373267
28 -17.2721582352039
29 -17.6394593460613
30 -17.9710892313426
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.61114665788231
1 1.91179012432249
2 1.41550488385306
3 0.897090214103795
4 -0.0490525547464848
5 -1.20980470309531
6 -2.0891646587285
7 -2.83418171660935
8 -2.86752249503474
9 -2.64840760682387
10 -2.44799473706646
11 -2.53000826191342
12 -2.75633139582433
13 -3.1454665567781
14 -3.89729497723775
15 -4.71230627732686
16 -5.58882059067806
17 -6.12934097584115
18 -6.81545759591785
19 -7.56525978199709
20 -8.12915364034662
21 -8.45724315179657
22 -9.07145552333619
23 -9.43019727509905
24 -9.95216045375072
25 -10.273232227938
26 -10.7426945560069
27 -11.2224861889972
28 -11.6040556097025
29 -11.9402549794384
30 -12.3171373762951
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.57466644878178
1 1.85746884641836
2 0.989003962715707
3 0.0502756169671663
4 -0.868119804628053
5 -2.34028965889462
6 -3.85712526210431
7 -4.69348064486441
8 -4.95854323469158
9 -4.83273334227057
10 -4.72162281461044
11 -4.95869882080286
12 -5.44358698813538
13 -5.93693719335428
14 -6.60237305979747
15 -7.22312740773771
16 -7.66432427484624
17 -8.01829794240652
18 -8.48037874388455
19 -8.8033833631199
20 -9.05362030134579
21 -9.30435824536887
22 -9.54079864870883
23 -9.60161712719083
24 -9.60845220364064
25 -9.76221883557132
26 -9.79549445290951
27 -9.64174875407516
28 -9.40740146564029
29 -9.19724006357493
30 -8.81573819732799
};
\addplot [semithick, color1, opacity=0.1]
table {%
0 2.56787421661564
1 1.54716950246189
2 0.772082626097472
3 -0.241397108429098
4 -1.5258960165528
5 -3.17232563486689
6 -4.20837429012615
7 -4.75085641210706
8 -5.07667010803181
9 -5.25991944804235
10 -5.60151939421267
11 -5.79716311921165
12 -6.23946660169519
13 -6.76593744544288
14 -7.30936205534404
15 -7.92697222756711
16 -8.57679458532047
17 -9.48902518267016
18 -10.0469773252685
19 -10.4668559468078
20 -11.1232861983
21 -11.876418963395
22 -12.4595963192367
23 -13.0244268896388
24 -13.4952310777203
25 -13.8819481029346
26 -14.2976478342099
27 -14.4790347708254
28 -14.6744720588521
29 -14.6078519723777
30 -14.3710895419064
};
\addplot [line width=0.01pt, color1, mark=*, mark size=2, mark options={solid, draw=black}]
table {%
1 2.65103446372252
2 1.87298481713709
3 1.03310235020523
4 -0.0349224785257646
5 -0.681923979276541
6 -0.614035490335335
7 -0.208100847346677
8 0.33428430837777
9 0.710486243049944
10 0.726233644866842
11 0.520411660737353
12 0.347599665643602
13 0.244300607278545
14 0.195112904269273
15 0.20629800498181
16 0.161911176310666
17 0.161283251423433
18 0.247899352697984
19 0.208651205023874
20 0.171253015388636
21 0.20029198108343
22 0.172890109571832
23 0.187770311286831
24 0.213147053788955
25 0.185796243819713
26 0.165625930691843
27 0.187584184388062
28 0.20252014981221
29 0.179459395114634
30 0.2013127196102
};
\end{groupplot}



==> experiments/figs/sup_mat/tikz_samples_ep-14-all.tex <==
\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}

\begin{groupplot}[group style={group size=1 by 3}]
\nextgroupplot[
xshift=-8,
title={14 episodes},
title style={font=\large},
xmin=-1.45, xmax=30.45,
%ymin=1.15124371169553, ymax=6.91115994797861,
ymin=2.7, ymax=6.7,
width=\figurewidth,
height=\figureheight,
xtick={},
xticklabels={},
yticklabels={},
tick align=outside,
tick pos=left,
x grid style={white!69.019607843137251!black},
y grid style={white!69.019607843137251!black}
]
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.40958979204541
1 3.50167738560338
2 3.46529177834903
3 3.17787007728519
4 2.96321605330536
5 3.25713313015265
6 4.02396255002326
7 4.71678585673224
8 5.02128474732438
9 5.10964208769495
10 5.18783930452376
11 5.07931112500971
12 4.63434035448156
13 4.26531348004429
14 3.64034226099943
15 3.15325890209546
16 2.48823453461459
17 2.01620910123989
18 2.15800268261965
19 2.56798940848056
20 2.94205950842422
21 3.1773958046763
22 3.45997202785605
23 3.39455919879405
24 3.3109822116968
25 2.91119484821375
26 2.44161033553841
27 1.92131263264334
28 1.38746441779804
29 0.75519039884928
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.42699982278861
1 3.57593501289551
2 3.54534445536686
3 3.16367232221292
4 2.89351097212513
5 3.22218827523777
6 3.77073000432696
7 4.19101251472082
8 4.83605807107464
9 5.07627474763137
10 5.38041354711774
11 5.70704345516276
12 5.56890809893928
13 5.23652033163488
14 4.82532051004374
15 4.30221247932572
16 3.73612093299553
17 3.17291588113259
18 2.7751145676743
19 2.39383450738712
20 2.04066982978872
21 2.05616701364223
22 2.24607249272239
23 2.59993370777652
24 2.89567842867222
25 3.13308556715328
26 3.18435125092283
27 2.98279560978564
28 2.7226253621437
29 2.50549064296298
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.5687793361235
1 3.64864890144533
2 3.5933144178986
3 3.50631783126456
4 3.3013657346245
5 3.36022913618829
6 3.73008479237651
7 4.2078025262175
8 4.3763448626275
9 4.41568338759936
10 4.31530013183546
11 4.06378541772542
12 3.64266811269897
13 2.93488408642009
14 2.5640596666683
15 2.30803504839574
16 2.07463970749525
17 2.21824033185909
18 2.40603900497724
19 2.64991840812583
20 2.91788603047588
21 3.08886079762311
22 2.95231695772735
23 2.85365665656592
24 2.69799567369068
25 2.55340066617682
26 2.47771400217981
27 2.35030501211684
28 2.17714289447303
29 1.96319759835024
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.50917617071343
1 3.62459349701745
2 3.49396195733172
3 3.24063668113275
4 3.03062280404505
5 3.35643676415249
6 3.79378220187777
7 4.34715290371863
8 4.55098428982971
9 4.79778215364053
10 4.88394197786883
11 5.11705167689105
12 4.80260044262643
13 4.40039399738037
14 3.89560085116205
15 3.25011802334636
16 2.63692328489166
17 2.2685214930776
18 2.13343057373282
19 2.2468995387567
20 2.39657794434582
21 2.52704508780836
22 2.62597683642972
23 2.63096126868406
24 2.55799294603502
25 2.39697287668125
26 2.3986920101605
27 2.53716701546458
28 2.51916559554652
29 2.65806924831059
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.42957721061187
1 3.62810576110068
2 3.55968106700103
3 3.28028350211976
4 3.08687389624361
5 3.36676063828493
6 3.96470643520351
7 4.65591528259081
8 4.99846550391255
9 5.30379766487492
10 5.40157529643755
11 5.46628451230192
12 5.33315546923832
13 5.16378133734166
14 4.98861257430269
15 4.84269327495638
16 4.56072850362137
17 4.39380200845374
18 4.15652909436142
19 3.86919750811954
20 3.43091537227068
21 2.86869094222625
22 2.4194864777625
23 2.70543330960008
24 3.07318577441776
25 3.27653620149313
26 3.44512794155084
27 3.43301343242384
28 3.19955749072628
29 2.88273362664525
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.58271448972532
1 3.60798917542732
2 3.53327194281838
3 3.22550264354267
4 2.93239925116926
5 3.13378987770534
6 3.56026218442165
7 4.01085482849916
8 4.4503807873019
9 4.69027957152752
10 4.95166631659382
11 5.09406065618158
12 5.04044946682854
13 4.82127636248569
14 4.45886796783539
15 4.0002986327193
16 3.61433263260617
17 3.12004475871068
18 2.82427737644011
19 2.81629727830065
20 3.14825632041384
21 3.83175862899455
22 3.99643732888913
23 3.72675738427075
24 3.54434129826608
25 3.33356819409522
26 3.12689446742286
27 2.89450163441023
28 2.583749172733
29 2.29130262076071
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.48415351143306
1 3.69972213871165
2 3.60863876418089
3 3.27977813785367
4 3.01928790917842
5 3.23955851527913
6 3.73084252403738
7 4.33828781336935
8 4.77128626926186
9 5.09549283510469
10 5.15793281815051
11 5.13966043308529
12 4.87167117391483
13 4.3480569999695
14 3.70381667178058
15 3.07766671420779
16 2.52045799120353
17 2.65879870516345
18 3.24965094703607
19 3.50899520346757
20 3.72580005897546
21 3.69180057485025
22 3.54799234215003
23 3.443186137911
24 3.02563596850535
25 2.46909977435114
26 2.00560309657981
27 1.75143731878086
28 1.47603284002685
29 1.06218083530241
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.43161912746504
1 3.54484184017913
2 3.59141419837195
3 3.36363944965745
4 3.17510763125831
5 3.41696478838067
6 3.87457581291773
7 4.34643643901908
8 4.56820852015325
9 4.56009828529957
10 4.64177392361453
11 4.49484515725723
12 4.32085992532612
13 3.9319482609581
14 3.57007948550353
15 3.13256334463826
16 2.8422667989331
17 2.63788966348012
18 2.77276768827155
19 2.85390266958506
20 2.96744371562682
21 2.96336963929044
22 2.98770548130435
23 3.14725504602689
24 3.21146022586526
25 3.16156047427682
26 3.00467079835681
27 2.98540330491536
28 3.11491803687528
29 3.07835950349473
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.33605404983952
1 3.56439158272457
2 3.51708511909016
3 3.27068313491807
4 3.17137612479015
5 3.68281002382575
6 4.06067365583184
7 4.48273406115369
8 4.82036263651631
9 5.30046352927838
10 5.52215848100765
11 5.75901359028889
12 5.59028097901986
13 5.36116049514103
14 4.99096712490994
15 4.74858362995726
16 4.2034230843411
17 3.71952379691762
18 3.17478082829064
19 2.63396781954658
20 2.21992691162308
21 2.12191488803207
22 2.16284916392714
23 2.51070599737012
24 2.97920858690039
25 3.31523809336664
26 3.70491098621841
27 4.05627482797773
28 4.21963114526042
29 4.22066580163399
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.46336915001094
1 3.53038469539622
2 3.52998643596527
3 3.23371263929224
4 3.07933815049259
5 3.31888891442268
6 3.65610640818181
7 4.07739885168013
8 4.65275934351464
9 4.94536934880634
10 5.09265397344609
11 5.06960717688256
12 4.99233401632597
13 4.75203411866488
14 4.29119631733133
15 3.81192158284231
16 3.30838290890127
17 2.85336652330844
18 2.47074774235091
19 2.145801813159
20 2.2273660251196
21 2.49072661795598
22 2.66318186803857
23 2.69788449822174
24 2.72931841394354
25 2.70659127776794
26 2.79616357672266
27 2.97716538884947
28 3.10540706991302
29 3.03364674479842
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.53496756841957
1 3.56034187986796
2 3.40262732914903
3 3.12040043576985
4 2.88552583796395
5 3.1137579230493
6 3.67439630730181
7 4.40219251039965
8 4.83375417051393
9 5.10671503836854
10 5.39851714206191
11 5.60469927171015
12 5.40417051841031
13 5.04515343249897
14 4.53528449364367
15 4.12448350068549
16 3.53647258659583
17 3.04104635821709
18 2.44967273578677
19 2.37291066719273
20 2.70115695185881
21 3.35877625943297
22 3.77205020156736
23 4.1359008910423
24 4.11818441076248
25 3.71918482457841
26 3.18856037747679
27 2.93524438102415
28 2.84223152088975
29 2.74211676410325
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.57723853219815
1 3.64461222088334
2 3.54422972960468
3 3.25335534999685
4 3.01792515943877
5 3.24021075741999
6 3.79533166481725
7 4.2775989696996
8 4.48947022639733
9 4.83603668598167
10 5.15140580824879
11 5.30613266090862
12 5.28016493118252
13 5.09575168745022
14 4.85165643195846
15 4.49776177376517
16 3.97332604828076
17 3.53650837478922
18 3.03860544288437
19 2.59852019065673
20 2.33839654529921
21 2.24734855205693
22 2.30470256670445
23 2.46683530000033
24 2.70187193117278
25 2.91749507634543
26 3.177016513719
27 3.39789017816101
28 3.58257825779772
29 3.70075382299488
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.45788150351057
1 3.58260928347073
2 3.55040424469944
3 3.14987196647987
4 2.87388247671143
5 3.20378615967059
6 3.81319001589523
7 4.31885196784951
8 4.71369307129097
9 4.95035073572447
10 5.12625449058206
11 5.1774700412903
12 5.11415568495357
13 4.83054457929057
14 4.35535369769227
15 3.86398803332505
16 3.11979485809499
17 2.66063133985397
18 2.21926426382951
19 1.9276083140064
20 2.03359131031629
21 2.43928492096895
22 2.6361438922939
23 3.03507879723474
24 3.49417298493087
25 3.56864678688882
26 3.38175338508222
27 3.13643408135737
28 2.91989199875588
29 2.81100214629535
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.52452840394355
1 3.6273685535714
2 3.59245583826381
3 3.3860817348298
4 3.11939401441888
5 3.37805730359909
6 3.63739594442011
7 4.22811791598782
8 4.6482932763342
9 4.8443751612986
10 4.97310667903284
11 5.01144556212842
12 4.67351456677622
13 4.15877172820943
14 3.56210928315804
15 3.19034088076277
16 2.91609447178834
17 2.78544676508509
18 2.73899893297792
19 2.4211168835752
20 2.41946912111582
21 2.28157613926022
22 2.09267019444061
23 2.0872878666946
24 1.96498115492984
25 1.85535075049173
26 1.82206245246314
27 2.02284756569506
28 2.25494159928231
29 2.42989319404186
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.35637863255996
1 3.36216217660825
2 3.34940860800271
3 3.34711210563087
4 3.3266218861233
5 3.74211459011387
6 4.13179184777371
7 4.74267616795271
8 5.01932052516097
9 5.20397403833988
10 5.25709744005045
11 5.22784411783838
12 4.98668500672597
13 4.71367504960847
14 4.28184690905127
15 3.7158716354221
16 2.91836028552944
17 2.38751734587209
18 1.96041879415623
19 1.91084865797238
20 2.09437544295215
21 2.47412454907152
22 2.95033858417615
23 3.3987577804247
24 3.90668933383761
25 4.35528806114354
26 4.85327593235943
27 5.3383424884028
28 5.58403178113307
29 5.53620865125299
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.34173262931867
1 3.39616626309407
2 3.45238583701502
3 3.23476082616964
4 3.00699102783686
5 3.34967279483688
6 3.86336478814748
7 4.32007054793967
8 4.70502725844047
9 4.90227876063992
10 5.08207158350405
11 5.27291391989595
12 5.09105195979769
13 4.79832099504562
14 4.44294991036586
15 3.89834945654336
16 3.34362820388035
17 2.63683976854457
18 2.12788623199487
19 1.75141203332049
20 1.86976821981295
21 1.9287453635944
22 1.7411444114892
23 1.64827829401234
24 1.69551007970155
25 1.66688002242658
26 1.76927834413021
27 2.08974137489323
28 2.38001200580064
29 2.6798501432915
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.4727565989944
1 3.59212211393626
2 3.55656808566513
3 3.32244351357801
4 3.15066464053262
5 3.47365815672578
6 3.85219171727764
7 4.30027875932756
8 4.67724004291945
9 4.95848367040633
10 5.13177538218669
11 5.07052625763579
12 4.78574740489643
13 4.45350652372691
14 3.97082035719707
15 3.38223761872617
16 2.93920057778572
17 2.52584553779145
18 2.48623929195584
19 2.27287543689205
20 2.17695449254416
21 2.29575022573634
22 2.42593647503975
23 2.65592863610426
24 2.93002477734018
25 3.28057682597
26 3.54660292678242
27 3.50950508560071
28 3.38965374165132
29 3.06332913360303
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.5226730614876
1 3.67819535495896
2 3.56064868782486
3 3.37627560537572
4 3.23295205884374
5 3.38168795158182
6 3.7245969299391
7 4.34426243622987
8 4.66094760592777
9 4.80931156708923
10 5.09942708034875
11 5.21864104679499
12 5.05481182732709
13 4.87731353558015
14 4.41416579999151
15 3.84427969182576
16 3.31968479063718
17 2.81163009372428
18 2.43184330684941
19 2.31048236688403
20 2.59259529197681
21 2.83888096320068
22 3.05759249386225
23 3.12223250311312
24 3.09103680948809
25 2.99405654530868
26 2.86369306150339
27 2.8763072204216
28 2.79792095622363
29 2.64884676415549
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.39364426181671
1 3.47413328457966
2 3.49362760125915
3 3.24008108035346
4 3.1006712204054
5 3.40197692055845
6 3.82590999308315
7 4.1851766205521
8 4.36664853183473
9 4.3500463297975
10 4.36635043023066
11 4.15733904983708
12 3.6671244674459
13 3.14835163507273
14 2.79866959064448
15 2.89270654720283
16 3.0980365138289
17 3.40975753217359
18 3.43516166921741
19 3.02968585013081
20 2.62011122408992
21 2.24856499412322
22 1.92667716567979
23 1.59181345736477
24 1.10179605246205
25 0.495003527909471
26 0.00510557693512903
27 -0.497628060904772
28 -0.962641228612844
29 -1.34989406804224
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.56428910426952
1 3.62753948813066
2 3.6012296674432
3 3.34783056207007
4 3.17139812075359
5 3.38798494095095
6 3.74103799329436
7 4.18804695415637
8 4.50568294184482
9 4.75632990392272
10 4.85227560572255
11 4.76616069931286
12 4.50189105784974
13 4.29203439571891
14 3.87286930701427
15 3.46404535136722
16 2.89090707394049
17 2.96263966312852
18 3.39711335931247
19 3.61507705904507
20 3.83193793655913
21 3.8207033335463
22 3.60536261330908
23 3.3945425319951
24 3.11788370269859
25 2.66156410173256
26 2.16603264545423
27 1.7339041336675
28 1.30880798353469
29 0.829829989876998
};
\end{groupplot}

\begin{groupplot}[group style={group size=1 by 3}]
\nextgroupplot[
xshift=-8,
ylabel={\textcolor{color1}{outer angle}},
ylabel style={font=\large},
xmin=-1.45, xmax=30.45,
%ymin=-9.72718755361779, ymax=3.33959760594388,
ymin=-0.85, ymax=5.85,
width=\figurewidth,
height=\figureheight,
xtick={},
xticklabels={},
axis y line=right,
tick align=outside,
xtick pos=left,
ytick pos=right,
x grid style={white!69.019607843137251!black},
y grid style={white!69.019607843137251!black}
]
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.61950555933346
1 1.91148679239511
2 0.9800599415482
3 -0.217110188560676
4 -0.867938973890784
5 -1.11685381671571
6 -1.20685092292884
7 -1.19612553657888
8 -1.09849275847532
9 -1.22161495066757
10 -1.32089172912551
11 -1.45559669811115
12 -1.5796514358526
13 -1.77294581432246
14 -2.00530639458671
15 -2.33832105154502
16 -2.89903126769385
17 -3.83727763442437
18 -5.18556807874986
19 -6.61730458334486
20 -8.24332283885249
21 -10.0558252037028
22 -11.8572153892428
23 -13.5412363791027
24 -15.0978715384313
25 -16.458287541734
26 -17.5315984062954
27 -18.5145920015132
28 -19.5502557072706
29 -20.583796882955
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.70366195954305
1 1.95192946033404
2 1.13611862315948
3 0.0312135857822664
4 -0.455039583803375
5 -0.19343002847393
6 0.210365110981824
7 0.684407858538638
8 1.15116348310388
9 1.40665318043748
10 1.76461633807848
11 2.2135930637623
12 2.6349964010358
13 2.9786465917974
14 3.32315368434731
15 3.86634255199684
16 4.62781252356072
17 5.49054764416003
18 6.45449747792796
19 7.49478543201697
20 8.2139942433306
21 8.69255829975891
22 8.90045843587562
23 8.58642782801775
24 7.88949778944482
25 7.42241221819782
26 6.98744292427548
27 6.61151242161375
28 6.25692265412422
29 5.79436466937483
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.70390879274813
1 2.06284230654488
2 1.28751107423576
3 0.274353723261973
4 -0.0865557225496474
5 0.295962518934486
6 0.82939207218058
7 1.61045327291199
8 2.49379316041754
9 3.25239498632427
10 3.90616161022503
11 4.78519522656865
12 5.82762140468566
13 6.89052927723638
14 8.13614108133533
15 9.38969573024471
16 10.2894264871838
17 10.807981771013
18 10.8125222198279
19 10.5091332752195
20 10.0739937923252
21 9.61402070839407
22 9.25898209386927
23 8.84496897556997
24 8.42914294626332
25 7.93971749910984
26 7.40816056071359
27 6.84700900047766
28 6.22201599296404
29 5.62273005197862
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.67010882481419
1 1.96971617363226
2 1.0879214302868
3 -0.0250319135090891
4 -0.500412832942605
5 -0.321329141444542
6 -0.00575915189395637
7 0.511539236761362
8 1.1776389592071
9 1.76519461598089
10 2.31720514248705
11 2.91942089619786
12 3.6217733550031
13 4.22682037172477
14 4.92322974999604
15 5.76396485468781
16 6.48248442467833
17 7.27781067245593
18 7.77921595837448
19 7.96555997751913
20 7.67660895670639
21 7.12204355074224
22 6.46216009157125
23 5.86035949037874
24 5.39442329948425
25 4.94720446969553
26 4.49595499649515
27 4.12055658963365
28 3.72112283640161
29 3.46648283097718
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.65997650251569
1 1.92589144222464
2 0.921825048974528
3 -0.328802060930487
4 -0.941797019056832
5 -1.15064576742635
6 -1.24325377375617
7 -1.15334418321814
8 -0.898802106032687
9 -0.724402089397287
10 -0.721697429710296
11 -0.865395080713608
12 -0.803854659088975
13 -0.653967499733005
14 -0.496369888803027
15 -0.515904944829673
16 -0.450232923255214
17 -0.530844763160092
18 -0.634495963416866
19 -0.9722508790364
20 -1.49224017170138
21 -2.3135112224469
22 -3.39939413924866
23 -5.04462182538667
24 -6.92053413719749
25 -8.71375229842016
26 -10.1956001471665
27 -11.5487413657754
28 -12.8930749128593
29 -14.2292992635356
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.65832762655855
1 1.95238661210138
2 1.07830301722588
3 -0.0809431247682895
4 -0.734380345852921
5 -0.739237205424505
6 -0.364082873522854
7 0.154063570556856
8 0.5007391592552
9 0.558390850601498
10 0.453976559704749
11 0.472280795979543
12 0.412821145954014
13 0.288625904254683
14 0.153289707453371
15 -0.0415383377197749
16 -0.607086688388051
17 -1.24413173763841
18 -2.31036696214161
19 -3.50635170018696
20 -4.94113445818772
21 -6.58017703763813
22 -8.10193501075269
23 -9.38611563014286
24 -10.9232710880828
25 -12.3503827982775
26 -13.6748681506935
27 -14.7720879650724
28 -15.8018972045729
29 -16.8194503971283
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.68908658090228
1 1.9866101182228
2 1.02335758240891
3 -0.177687370247217
4 -0.79557846187798
5 -0.969001479273851
6 -0.917666950322799
7 -0.830450243126437
8 -0.660565826748769
9 -0.875583526569837
10 -1.19225680628012
11 -1.53249711665814
12 -1.96980610138735
13 -2.30534583319865
14 -2.66899949140462
15 -3.41463944832244
16 -4.48993518633083
17 -5.86821026229962
18 -7.49339831740616
19 -9.04165624045782
20 -10.3589189050045
21 -11.5126731806801
22 -12.6744354090701
23 -13.597527306352
24 -14.5156369058044
25 -15.434799106369
26 -16.2757645032981
27 -17.0443735435649
28 -18.0466235421681
29 -19.1946845400588
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.70034432565367
1 1.91815227713715
2 1.05888452887444
3 -0.128435900420797
4 -0.707089006984893
5 -0.555616737030856
6 -0.266657482988242
7 0.112639927001092
8 0.68383847416667
9 1.09806461418472
10 1.65326427126743
11 2.3600477773853
12 3.07752231796578
13 3.79244572456685
14 4.44813768747766
15 5.02293054344296
16 5.43917563893448
17 5.69975959302294
18 5.49752585962218
19 5.16190514627513
20 4.90355401032716
21 4.71294168545542
22 4.56470658059431
23 4.31529979662424
24 4.18731912641586
25 4.09689233889289
26 4.13737153048105
27 4.17683653372312
28 4.09376298108756
29 4.0049537638829
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.71658173713363
1 1.97993606578676
2 1.07751901397388
3 0.11609356817725
4 -0.336880036744819
5 -0.344185543896684
6 -0.077563704627595
7 0.355650008184243
8 0.777087794936465
9 0.939133757315444
10 1.00273952272854
11 1.12232044505616
12 1.19670716682378
13 1.24956744351313
14 1.3397297440672
15 1.40205496292544
16 1.35413185204454
17 1.08656111223944
18 0.676401649997525
19 0.204175465405358
20 -0.30778032875533
21 -0.900318252660627
22 -1.60585835165582
23 -2.6789686645089
24 -4.00113450678989
25 -5.41507036199837
26 -6.99074280913071
27 -8.44735221601767
28 -9.80145240998491
29 -10.9913723532458
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.67011013489685
1 1.97662279961282
2 1.11573139660623
3 0.0711341755914727
4 -0.402881776117843
5 -0.1989782886185
6 0.302110175707403
7 0.99096876576559
8 1.64104030426092
9 2.18800614217009
10 2.75915358280556
11 3.20990829065438
12 3.65365791765799
13 4.07640863232632
14 4.55966324150235
15 5.01564077151604
16 5.85745142017754
17 6.65866178264024
18 7.39148105236416
19 7.83732601560301
20 8.00187674086911
21 7.60222373816667
22 6.92283403916472
23 6.38303232214282
24 5.91993563250916
25 5.52394252590441
26 5.27432482671008
27 4.98478174538813
28 4.73997978500852
29 4.56490030171607
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.69931929891135
1 2.04327575440857
2 1.09729020147018
3 -0.130440371583397
4 -0.76392456946169
5 -0.829068728739642
6 -0.882218723737957
7 -0.744449530429421
8 -0.733747008773348
9 -0.878547239524565
10 -1.13799505491403
11 -1.34777790980008
12 -1.46368752430491
13 -1.49869743069785
14 -1.51385041001301
15 -1.64547070088193
16 -2.02189197246906
17 -2.48246255204929
18 -3.18641781562074
19 -4.32252439575824
20 -5.7961978323028
21 -7.53487752772209
22 -9.09678979624358
23 -10.5469933044745
24 -11.8687666940607
25 -13.2872946492867
26 -14.681018335819
27 -16.0035407055027
28 -17.2380235149141
29 -18.3979798932416
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.71874874449566
1 1.90870947692094
2 0.954972179524646
3 -0.241440202594633
4 -0.765009031151694
5 -0.614933063237388
6 -0.341658214281512
7 0.243930380481588
8 0.643599050521889
9 1.02852206978183
10 1.39134238296373
11 1.82886236099631
12 2.35361230654323
13 2.76414987935601
14 3.14953820112423
15 3.35194393332045
16 3.71598993433066
17 3.97912689879375
18 4.28397038361005
19 4.52478922261925
20 4.53250251625193
21 4.38575861350261
22 4.12274965948743
23 3.78166887354183
24 3.401681851434
25 3.15841283838882
26 3.14391584439841
27 3.1437778234799
28 3.21832399970171
29 3.35382486605699
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.75939031503598
1 2.02419390432946
2 1.12910421995586
3 0.0166649474640952
4 -0.452526750052577
5 -0.39641378180986
6 -0.188435141521952
7 0.180008571131856
8 0.533395050695045
9 0.735569692174236
10 0.853283158404512
11 0.851429416357581
12 0.816319173688099
13 0.724471184788452
14 0.578533238423789
15 0.285773168182738
16 -0.126936492345934
17 -0.929404443835654
18 -1.77748823884474
19 -2.63580444078069
20 -3.85605839612981
21 -5.59234328959522
22 -7.42151632162512
23 -8.9982374933401
24 -10.8790421129046
25 -12.5758204264116
26 -14.0185931186653
27 -15.3477187434521
28 -16.5013960261498
29 -17.5426094809126
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.71924842644924
1 2.03859558637315
2 1.12573213725142
3 -0.0577873701944203
4 -0.515403613313016
5 -0.374351477034669
6 0.102432996574302
7 0.675037602231672
8 1.46041276191885
9 2.03650647418261
10 2.52545065148001
11 3.01667659750414
12 3.69303998753685
13 4.43887373044344
14 5.17188885910687
15 5.87629607419456
16 6.41184350637486
17 7.04032347394163
18 7.3346588140222
19 7.29830891737191
20 6.84778686524645
21 6.10316513983111
22 5.45632235397477
23 4.72050522787223
24 3.92311316591121
25 3.15813176561599
26 2.42390604169781
27 1.64048140264421
28 0.90057636938216
29 0.202120258449025
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.65526014053647
1 1.85517483459315
2 0.985685869014805
3 -0.060768320739859
4 -0.540573836473101
5 -0.602864318605002
6 -0.427679343043136
7 -0.123189153001626
8 0.137119806337182
9 0.335130279630519
10 0.537130333751049
11 0.719007462949817
12 0.917113095996545
13 0.920741350461604
14 1.05641545402256
15 1.08949653742901
16 1.06271460623789
17 1.00350667513697
18 0.792430373301746
19 0.61455059555384
20 0.352612621519111
21 0.0325011008008573
22 -0.658464650639983
23 -1.50675721803775
24 -2.73541561082051
25 -3.98611568836952
26 -5.13823546541345
27 -6.14148819671492
28 -6.96672332270359
29 -7.64867611759768
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.76336696606541
1 2.04605211759736
2 1.02786002479152
3 -0.0359973006641621
4 -0.459112767449328
5 -0.287424392187367
6 0.0727008898271713
7 0.524211176053537
8 1.0885444316172
9 1.58424093945323
10 2.17209992259071
11 2.70792207166001
12 3.20108736791907
13 3.74362976203599
14 4.23575198072281
15 4.72020569340462
16 5.3364484112357
17 6.02154318326474
18 6.44638032474696
19 6.42995117657615
20 6.1313117455974
21 5.43093535800986
22 4.4944482532858
23 3.38758201666803
24 2.27995354591862
25 1.1468287382976
26 0.0543549874340847
27 -1.20005218886987
28 -2.73492729243505
29 -4.34575578800237
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.6438696788416
1 1.95494662805965
2 1.17874477997851
3 0.0107602224075478
4 -0.463510649136339
5 -0.323440218797318
6 0.116731175300474
7 0.754523879879287
8 1.55384531824679
9 2.2155320612566
10 2.82578068937977
11 3.16096220508723
12 3.67303834627354
13 4.131189822515
14 4.51856659472794
15 4.72992695315545
16 5.09234551785523
17 5.21860938463463
18 5.12380442440485
19 4.68664936932345
20 4.28495452039381
21 3.82337198871203
22 3.36038806928208
23 3.00120156772647
24 2.62995224415271
25 2.54105382067012
26 2.62378542291716
27 2.99984559541183
28 3.30169102922334
29 3.62184572941589
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.60653024531803
1 1.94080048573905
2 1.07585814963554
3 -0.0481287829233601
4 -0.371718423155386
5 -0.251021824958604
6 0.165533111831325
7 0.714843105377374
8 1.24074103923867
9 1.78050077178606
10 2.28654031234596
11 2.85900041753506
12 3.53818415057052
13 4.13194412766205
14 4.82694058388631
15 5.56671943100244
16 6.42719836421484
17 7.45814790364078
18 8.42231558974862
19 9.08108824470672
20 9.51499401233623
21 9.55434040822239
22 9.39430276939061
23 9.01285134442753
24 8.66073440326231
25 8.25775116797665
26 7.91042985220174
27 7.47662214581804
28 7.07999407809354
29 6.64574289250792
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.67183990042016
1 1.84370965436382
2 0.814246429200148
3 -0.411152003290594
4 -1.05639214215467
5 -1.25414290380762
6 -1.32455753618744
7 -1.15989931597173
8 -0.997192006612343
9 -0.968623119947724
10 -1.2577889237272
11 -1.90044949309599
12 -2.57546469449507
13 -3.45840878758611
14 -4.63175376961487
15 -6.22615138200982
16 -7.85049837504954
17 -9.57761740953963
18 -11.3150617451513
19 -12.9138874361152
20 -14.2252982996066
21 -15.7402960554981
22 -17.1584445471529
23 -18.501767202864
24 -19.9109911634331
25 -21.3078082794771
26 -22.6189582349959
27 -23.921268412845
28 -25.3697199200122
29 -26.7141143229504
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.65664401364741
1 1.84253305646656
2 0.921420455390553
3 -0.25903913630545
4 -0.772184237165224
5 -0.840837594589338
6 -0.527949977445145
7 -0.144856361747088
8 0.167201999690958
9 0.129355763124455
10 0.047970005733605
11 -0.202195256439902
12 -0.342032272588746
13 -0.733005464283316
14 -1.44160400367792
15 -2.39128611581866
16 -3.59769911076977
17 -5.32798514697426
18 -6.93319997465418
19 -8.47033027154955
20 -9.82201969515057
21 -11.1860119142424
22 -12.5159229128398
23 -13.884492995388
24 -15.2610479716388
25 -16.7085803799235
26 -17.9812851650804
27 -19.2564423545319
28 -20.5174624298462
29 -21.9691376049799
};
\end{groupplot}

\begin{groupplot}[group style={group size=1 by 3}]
\nextgroupplot[
xshift=-8,
xmin=-1.45, xmax=30.45,
%ymin=2.65977698435744, ymax=6.38414108671984,
ymin=2.7, ymax=6.7,
width=\figurewidth,
height=\figureheight,
xtick={},
xticklabels={},
yticklabels={},
tick align=outside,
tick pos=left,
x grid style={white!69.019607843137251!black},
y grid style={white!69.019607843137251!black}
]
\addplot [line width=0.06pt, color0, mark=*, mark size=2, mark options={solid,draw=black}]
table {%
0 3.31996634253658
1 3.45443899460193
2 3.38784218387077
3 3.01931286439371
4 2.82906626173755
5 3.09427938765557
6 3.60416870184349
7 4.24596487007442
8 4.84338888587772
9 5.27994908427636
10 5.61004074039071
11 5.90268352537916
12 6.05852129333431
13 6.16858387553312
14 6.19509636026208
15 6.21485180933973
16 6.20378189365436
17 6.1468591562609
18 6.14787992255152
19 6.14579317317396
20 6.15283082950704
21 6.15412613868876
22 6.14366281427887
23 6.16587792193215
24 6.18223254289368
25 6.18638821201769
26 6.14794417270148
27 6.14179954980725
28 6.15812095860932
29 6.16746194810668
};
\end{groupplot}

\begin{groupplot}[group style={group size=1 by 3}]
\nextgroupplot[
xshift=-8,
xmin=-1.45, xmax=30.45,
%ymin=-0.848571901426494, ymax=2.81768238587247,
ymin=-0.85, ymax=5.85,
width=\figurewidth,
height=\figureheight,
xtick={},
xticklabels={},
yticklabels={},
axis y line=right,
tick align=outside,
xtick pos=left,
ytick pos=right,
x grid style={white!69.019607843137251!black},
y grid style={white!69.019607843137251!black}
]
\addplot [line width=0.06pt, color1, mark=*, mark size=2, mark options={solid,draw=black}]
table {%
0 2.65103446372252
1 1.87298481713709
2 1.03310235020523
3 -0.0349224785257646
4 -0.681923979276541
5 -0.614035490335335
6 -0.208100847346677
7 0.33428430837777
8 0.710486243049944
9 0.726233644866842
10 0.520411660737353
11 0.347599665643602
12 0.244300607278545
13 0.195112904269273
14 0.20629800498181
15 0.161911176310666
16 0.161283251423433
17 0.247899352697984
18 0.208651205023874
19 0.171253015388636
20 0.20029198108343
21 0.172890109571832
22 0.187770311286831
23 0.213147053788955
24 0.185796243819713
25 0.165625930691843
26 0.187584184388062
27 0.20252014981221
28 0.179459395114634
29 0.2013127196102
};
\end{groupplot}


==> experiments/figs/sup_mat/tikz_samples_ep-2-all.tex <==
\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}

\begin{groupplot}[group style={group size=1 by 3}]
\nextgroupplot[
xshift=-8,
title={2 episodes},
title style={font=\large},
ylabel={\textcolor{color0}{inner angle}},
ylabel style={font=\large},
xmin=-1.45, xmax=30.45,
%ymin=-5.18312483023826, ymax=6.87015257507078,
ymin=2.7, ymax=6.7,
width=\figurewidth,
height=\figureheight,
xtick={},
xticklabels={},
tick align=outside,
tick pos=left,
x grid style={white!69.019607843137251!black},
y grid style={white!69.019607843137251!black}
]
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.41289310163331
1 3.05051687853909
2 3.09932099612203
3 3.18769350278898
4 3.24552780666672
5 3.16750664224544
6 3.00911921170606
7 2.77901212901609
8 3.0379600792271
9 3.37765183287035
10 3.61249801177389
11 4.09212460456359
12 4.49405002386523
13 4.89425079130043
14 5.14834302592042
15 5.22811732691164
16 5.1709354410081
17 5.20652795110208
18 5.29609598327113
19 5.08648505446709
20 5.15643644452188
21 5.20950239927538
22 5.13170088578445
23 5.2139785755416
24 5.25817689210719
25 5.29775693994264
26 5.34611319746027
27 5.55754004293797
28 5.70258893992972
29 5.62892835404119
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.62675117947097
1 3.30438159022828
2 3.24496304542662
3 3.15831259869557
4 2.85631320277671
5 2.72961164148492
6 2.59719963915924
7 2.13877549047287
8 2.1917911773713
9 2.32262268464628
10 2.27705974013039
11 2.49243116370972
12 2.94868424780364
13 3.19410479407622
14 3.43685232435551
15 3.79737713322084
16 4.03431545575104
17 4.0524222547038
18 4.03441281886615
19 4.02117971725268
20 3.96018349781977
21 4.1388030388022
22 4.10861723799349
23 4.10230030947739
24 4.28815427295851
25 4.24343432586917
26 4.30048799706524
27 4.2675985212859
28 4.29603386662686
29 4.29772959282216
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.51920735780842
1 3.48691390425132
2 3.38983396189592
3 3.23430553727682
4 3.07195134039274
5 3.17285105888252
6 3.44767391806781
7 3.34321895047491
8 3.47420585899804
9 3.57065838086876
10 3.72594495414718
11 4.02819338560428
12 4.63758033404928
13 4.89284830350272
14 5.16048716835963
15 5.03660601788048
16 5.11990922347906
17 5.1152404713927
18 5.06110089302616
19 5.07143687783987
20 4.88036080709466
21 4.75699423161772
22 4.76174232666134
23 4.61760263230762
24 4.51985382243341
25 4.47649833095254
26 4.31614150761705
27 4.20984454305424
28 4.02773055713415
29 3.96065949201223
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.45386092242128
1 3.48785816760023
2 3.44484026463111
3 3.21473825385762
4 2.73305974499629
5 2.819741822446
6 2.68993416948298
7 2.30989830657704
8 2.6970870435561
9 2.9336500451896
10 3.33888358594897
11 3.44512235018261
12 3.97707432925544
13 4.45961698016017
14 4.82666939252971
15 4.91836188817522
16 5.1288635742437
17 5.40367778775085
18 5.44210086249605
19 5.53934750436078
20 5.71085602216982
21 5.96716459913452
22 6.14952249689501
23 6.26049630026405
24 6.4379299483277
25 6.53000985960386
26 6.57251006607482
27 6.54923969186839
28 6.57789931997358
29 6.62262525518004
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.75113967083616
1 3.61013021652081
2 3.51511750035992
3 3.6352489190781
4 2.9288019592271
5 2.71047392138709
6 2.63220810993761
7 2.35053094452881
8 2.8951364671782
9 3.31474634035035
10 3.84407996221008
11 4.15211989754515
12 4.65558302176165
13 4.81871414123971
14 5.23283362574843
15 5.46633245126215
16 5.47059267939886
17 5.63130262688719
18 5.92271451286946
19 5.85545826806387
20 6.05301380313106
21 6.12016000672075
22 6.11549902050237
23 6.28455490703889
24 6.34619483358154
25 6.43365538139582
26 6.40105305527574
27 6.55481521126226
28 6.49068321460378
29 6.60511535174508
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.65425466628332
1 3.52933030260276
2 3.63854288748125
3 3.36048177474356
4 2.99586141430448
5 2.71308591585516
6 2.51689930622233
7 2.25277023941729
8 2.5335158555683
9 2.68839888870116
10 2.6609162967361
11 2.58616625855091
12 3.05272820594346
13 3.12309426329273
14 3.2121808590703
15 3.07552727748617
16 2.9189785356645
17 2.82291399280707
18 2.82351125927817
19 2.74825638727305
20 2.61597433227212
21 2.56675260427609
22 2.48256851956328
23 2.46553050473178
24 2.37180397660978
25 2.29850864495608
26 2.2334323668424
27 2.17046102821872
28 2.10337310441086
29 2.1309345218947
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.47926468719603
1 3.25104162179219
2 3.12331942759417
3 3.31832333465087
4 2.94850105584201
5 2.97739610730939
6 2.85491275374917
7 2.45571927373938
8 2.52720037774265
9 2.67712432215892
10 2.92913178536277
11 3.02802391355047
12 3.44189203898254
13 3.72892684726738
14 4.03901785699453
15 4.13560475231204
16 3.95051918917776
17 3.82133170011931
18 3.79497283342966
19 3.81401651248842
20 3.65929781046563
21 3.69401958553862
22 3.56464296376372
23 3.6418027433405
24 3.72784778863905
25 3.87012879308984
26 3.74206355069309
27 3.79525027576085
28 3.76613662852949
29 3.85794307688957
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.18055302886721
1 3.13405225361342
2 3.31943398626576
3 3.40561337021024
4 3.31991724794387
5 3.54017251988422
6 3.31855795141351
7 2.9163178492169
8 3.24182363582723
9 3.82304993816413
10 4.01161796692156
11 4.16212845570058
12 4.48454829881319
13 4.64014697573353
14 4.89345224049462
15 4.87437809490021
16 4.88425309973117
17 4.98319576839412
18 5.10688083987627
19 5.14791330110702
20 5.2798077644698
21 5.27085163391758
22 5.14119621408158
23 5.23897893884893
24 5.18564980714668
25 5.2648594980428
26 5.30413762428235
27 5.39436393026073
28 5.36850351397679
29 5.3100243340421
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.5579296617354
1 3.5689905343398
2 3.63687483813142
3 3.37876340664492
4 2.98807306346975
5 2.93629666198573
6 2.75841349294657
7 2.33796891452453
8 2.47656697418567
9 2.7721244036664
10 2.92285009575676
11 2.95793833906682
12 3.2724550962092
13 3.65385482216081
14 3.89241309165458
15 3.96795709997901
16 3.93319143713262
17 3.80350124431383
18 3.83111685328305
19 3.72165334252428
20 3.67886543022167
21 3.4499539204686
22 3.31176369587767
23 3.24844369598971
24 3.32401795248082
25 3.31585534230585
26 3.14794509376642
27 3.10664300935888
28 3.0995864125112
29 3.02574863326737
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.44873839294622
1 3.37770145945011
2 3.15420234412274
3 3.01515415823868
4 2.55935031559012
5 2.33017306496655
6 2.14394942620106
7 1.82476887072867
8 2.01764420117516
9 2.29427807053407
10 2.61501821669817
11 2.93057825880766
12 3.16621714430747
13 3.29459566726943
14 3.40321102904514
15 3.3622237556343
16 3.25090869586216
17 3.28752186836531
18 3.46725346483945
19 3.29755865648523
20 3.1980836075574
21 3.28721380283712
22 3.2833563967269
23 3.18687777178133
24 3.13036299876715
25 3.09884306764517
26 3.11052897217013
27 3.03286822695524
28 2.96884439001992
29 2.97808586553909
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.58420164627459
1 3.56315172847734
2 3.64422783393182
3 3.56908436746244
4 3.1676671523747
5 3.29502773115027
6 3.18100256178842
7 3.11709712220186
8 3.41142009774581
9 3.71009787876651
10 3.95164082104152
11 4.03041507918881
12 4.49453722306205
13 5.07429942414232
14 5.54146379230816
15 5.82293931536836
16 5.80643435364313
17 5.69136909598622
18 5.6015705945571
19 5.69833808867281
20 5.52783121780868
21 5.52788003684648
22 5.49253398790466
23 5.42866232007745
24 5.54844973899828
25 5.49018686550279
26 5.35912565105571
27 5.16956051847261
28 5.09456279495788
29 5.00543042866399
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.78448160283413
1 3.57543583331358
2 3.59729187969974
3 3.51355023652996
4 3.17622273069857
5 3.1609219490948
6 2.96222372609489
7 2.55688092342085
8 2.89796638695417
9 3.33488056487879
10 3.6130526125903
11 3.75940263216863
12 4.15746034119415
13 4.4575144615604
14 4.57248453857018
15 4.66444679395009
16 4.85702339423463
17 4.80699040215944
18 4.83476414752294
19 5.05570705876371
20 5.00215479213775
21 5.03038497096954
22 5.19468029399138
23 5.16030938882612
24 5.24934701625999
25 5.27982649639944
26 5.36577315780855
27 5.23047785763323
28 5.26439741567414
29 5.35723917567154
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.50896874149356
1 3.08184782933726
2 2.88331324877944
3 2.63132424333118
4 2.37192298813664
5 2.32581503732485
6 2.2460852425436
7 2.16290459580621
8 2.30610429067988
9 2.67384441830331
10 2.80743506375509
11 2.95234414286827
12 3.52092328635497
13 3.86845687376568
14 4.35746502702342
15 4.17016070403898
16 4.03326566191116
17 3.85515004157744
18 3.55650054259544
19 3.17237454728917
20 2.9840264332989
21 2.84833868096806
22 2.61658382923273
23 2.63755145291391
24 2.59700770234444
25 2.44036159809733
26 2.34772037747675
27 2.35593248654693
28 2.24796941278073
29 2.1122190650888
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.37903160453369
1 3.34791338095471
2 3.21253666599565
3 2.8364156535121
4 2.79741837440454
5 2.6531941367424
6 2.66088530772564
7 2.64736997555185
8 2.9940322683173
9 3.41194804001864
10 3.53639039460047
11 3.66212458478583
12 4.09033011211297
13 4.27641100484995
14 4.53066665938552
15 4.36229463703081
16 4.0413710243163
17 3.71032759951987
18 3.38683720338181
19 3.13093188213943
20 2.84267286244253
21 2.5575011903187
22 2.33113118809841
23 2.09602902373151
24 2.00087831417838
25 1.80821756218347
26 1.46570008919404
27 1.17524758761581
28 0.929503033255491
29 0.605402801973965
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.63352026726901
1 3.59284484400665
2 3.49960555564545
3 3.31117996451623
4 2.80743576720903
5 2.90449073097887
6 2.66469669683802
7 2.63760924593396
8 3.04905738018359
9 3.21031678152213
10 3.25900042058241
11 3.37787760294867
12 3.87621614616002
13 4.1516636503025
14 4.39092933046316
15 4.4433262899484
16 4.40098881970106
17 4.28812303357948
18 4.29506434212242
19 4.30067896720977
20 4.27119544766952
21 4.28425698986412
22 4.3639117856862
23 4.40439327282304
24 4.5002550120115
25 4.66360158074249
26 4.71968746569307
27 4.8169522443589
28 4.87683389196641
29 4.97113800416688
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.52660760083237
1 3.37595425791963
2 3.31513279183825
3 3.19482915292183
4 3.11199098191601
5 3.17867527795835
6 3.26195850862421
7 3.17300992301324
8 3.40505346497058
9 3.67022830442675
10 4.01426209864774
11 4.04499262788198
12 4.57885893004965
13 4.69046269466621
14 4.88611083746756
15 4.82120058358255
16 4.76931829117432
17 4.49991172844968
18 4.17454188200033
19 3.94698551680106
20 3.75445801218215
21 3.55549477475807
22 3.43215256050371
23 3.20695579216881
24 3.06632330246036
25 2.92187387645647
26 2.9270352417562
27 2.65328228294354
28 2.63271831102881
29 2.64100940007448
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.76207290852536
1 3.73728978376529
2 3.49985425744116
3 3.4440824291077
4 3.01449563479132
5 2.99246394771615
6 2.76974579776704
7 2.18560805697497
8 2.55959273294485
9 2.66550449477737
10 2.99249281909692
11 3.14010190160737
12 3.60326320926003
13 3.93246371796845
14 4.29307222293505
15 4.40152011396058
16 4.45851644815144
17 4.6184567377893
18 4.65899347584473
19 4.65120844835968
20 4.65132583622642
21 4.76590746714972
22 4.84289738979881
23 5.03472381739981
24 5.1714487725008
25 5.15761121976826
26 5.13343910943851
27 5.30488068931868
28 5.35857108376541
29 5.31978249292032
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.47792189592837
1 3.61059092176214
2 3.72327987498364
3 3.58796219866349
4 2.94904056420882
5 2.92249459157107
6 2.48135833150399
7 2.16963953105363
8 2.59223045008482
9 2.894751870194
10 3.29037824253779
11 3.389674905328
12 3.79154397780932
13 3.82566129133623
14 4.02598480306737
15 3.93692668193681
16 3.82781205056498
17 3.6415181762927
18 3.30255725365307
19 3.17246326400874
20 2.90200189317053
21 2.7787525375912
22 2.74729498138522
23 2.49734659802284
24 2.58508777745006
25 2.48306683134125
26 2.44746402609748
27 2.26562133283082
28 2.14332005753292
29 2.12420892469049
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.52731888958683
1 3.28265758936634
2 3.13792883733901
3 3.01988751027391
4 2.69605161897985
5 2.50763670457837
6 1.91889145798881
7 1.41973380349385
8 1.69473385768298
9 2.11818759639376
10 2.32250137386641
11 2.6325720266764
12 3.20346326230072
13 3.59858669233028
14 4.03874862953272
15 4.36950721483386
16 4.31469390242844
17 4.47352781465091
18 4.67637574129423
19 4.9119721495136
20 4.96941453584157
21 4.94920019497943
22 5.09296616934162
23 5.09690641447952
24 4.94328929880438
25 4.85741585817567
26 4.89121338094728
27 4.93530665602228
28 4.85582632465361
29 4.81999110735648
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.57710055848102
1 3.39083371735406
2 3.41994549868665
3 3.19117139248922
4 2.87425345933613
5 2.74638737395543
6 2.47930868670814
7 1.7785974742086
8 1.71487960220785
9 1.55716952684092
10 1.81538144662967
11 1.99027400823401
12 2.46528141889312
13 2.50776971779713
14 2.80492421425351
15 2.74509679498134
16 2.54119904229191
17 2.42856615815067
18 2.2323594611436
19 2.06158823520603
20 1.80839644204182
21 1.86482721922895
22 1.76970641540005
23 1.57871017639856
24 1.57331862925958
25 1.53151809843888
26 1.55428275133155
27 1.5740974917409
28 1.60028775334599
29 1.60465494260825
};
\end{groupplot}

\begin{groupplot}[group style={group size=1 by 3}]
\nextgroupplot[
xshift=-8,
xmin=-1.45, xmax=30.45,
%ymin=-0.0317332990665444, ymax=27.9914686596272,
ymin=-0.85, ymax=5.85,
width=\figurewidth,
height=\figureheight,
xtick={},
xticklabels={},
yticklabels={},
axis y line=right,
tick align=outside,
xtick pos=left,
ytick pos=right,
x grid style={white!69.019607843137251!black},
y grid style={white!69.019607843137251!black}
]
\addplot [semithick, color1, opacity=0.3]
table {%
0 1.94549092899313
1 1.37177223531952
2 0.412717598122349
3 -0.523252845725859
4 -0.243139010335787
5 0.188910096735247
6 1.06091144148161
7 2.37064404878736
8 3.38744937047385
9 3.920869110506
10 4.42517324786769
11 4.79401740816412
12 4.50002150162083
13 3.82784008234888
14 3.0988845678135
15 2.17659858293533
16 1.7126988508748
17 1.56636219204187
18 0.92529232179119
19 0.436160068106805
20 0.226780826664505
21 -0.389839304251671
22 -0.665198732354115
23 -1.06572580829257
24 -1.69103895793317
25 -2.3080142210969
26 -2.74518868755263
27 -3.06456054982019
28 -3.51578894217637
29 -4.04899035429859
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.84687027260119
1 2.288118242207
2 1.45845994451595
3 0.839253205234309
4 0.744946252032781
5 0.93673565430066
6 1.75038498943345
7 3.16648804293795
8 4.21291333868069
9 5.2424427766175
10 5.31921629165915
11 5.79204465073737
12 5.99140157887772
13 5.90991341132755
14 5.66866571980713
15 5.23140954883776
16 4.50815458565231
17 4.18628913719635
18 3.80816122895569
19 3.40331413195662
20 3.32329458280975
21 2.72523665246598
22 2.27478176635914
23 1.8181953573383
24 1.19158659757106
25 0.339940101734422
26 -0.493278287122497
27 -0.761851562539364
28 -1.44870833403248
29 -2.07136265021478
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.69508830974404
1 1.70091722022634
2 0.791696450288661
3 -0.150633115074564
4 0.0626785859429422
5 0.237994914266014
6 0.522864534539394
7 1.59826279047895
8 2.28852757056264
9 3.27929515463339
10 3.60978886372121
11 3.5762060702587
12 3.68134143197285
13 3.49114826756662
14 3.47753322503737
15 3.33553900354105
16 2.82939077289031
17 2.11269131167194
18 1.43121624135182
19 1.04451534088733
20 0.610706588927771
21 0.312199690140952
22 -0.157197810366569
23 -0.752585182974636
24 -1.05119142833877
25 -1.46717877129575
26 -1.8598432656766
27 -2.66899150956853
28 -3.08763403066465
29 -3.60649807707768
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.69230092314131
1 2.56486346598884
2 2.11093246068557
3 1.70531743438374
4 1.86688702467328
5 1.85763881920301
6 2.36606673513379
7 3.43361807303447
8 4.27544041185034
9 4.53439990586508
10 4.67287957319237
11 5.7115009987293
12 5.12465972976976
13 4.44230858938624
14 3.54177204012692
15 3.13207209085047
16 2.571956254758
17 2.22084332611218
18 1.7711524415123
19 1.80966841667274
20 1.89715792032971
21 1.87342249158379
22 1.90729155820859
23 1.70826821743243
24 1.26216297737045
25 0.859086622424631
26 1.0004421500603
27 1.31271935306676
28 1.56458163296335
29 1.57548400705722
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 1.77451900689785
1 0.862401505050924
2 -0.220266948357239
3 -1.18175572523456
4 -1.41623852353719
5 -1.13008055305302
6 -1.06225939527273
7 -0.481330285096492
8 0.388285922702984
9 1.09883724030976
10 1.54360742756199
11 1.88449813935754
12 1.42717395957824
13 1.38421633653801
14 0.461112796072094
15 -0.19681057481526
16 -0.611038748135121
17 -0.950241234587875
18 -1.52717566820953
19 -1.67692023517892
20 -2.08086091704153
21 -2.39716652215811
22 -2.81838463732152
23 -3.42292691011127
24 -4.01703653618905
25 -4.66480511679705
26 -5.21532018527776
27 -5.83663196447709
28 -6.40744848888199
29 -7.07474232021871
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.71596271260996
1 1.70788152860271
2 0.710406389485083
3 -0.11731980101106
4 -0.215330133240434
5 -0.45222473890032
6 -0.0466179643478863
7 0.487831709271797
8 1.23350793860979
9 2.02633481529244
10 2.36488702147274
11 2.88219840502784
12 2.59114812832771
13 2.17580152690233
14 1.5728483063935
15 1.07541171620259
16 0.2483964844394
17 -0.0859944006870084
18 -0.753629884821363
19 -1.33483716087173
20 -1.69526454150128
21 -2.12487618822936
22 -2.60912103362679
23 -3.02590418833541
24 -3.94857366577763
25 -4.83047585845764
26 -5.37602580857545
27 -5.98852132574754
28 -6.51619699113763
29 -7.40708497492976
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.54671592861176
1 2.06054097777691
2 0.512673924139882
3 -0.286398885747877
4 -0.130494844085645
5 0.171789055945121
6 0.608342400239675
7 1.41516656828755
8 1.95274218538215
9 2.06324885167157
10 2.35003909989709
11 2.58426672781206
12 2.33840850110493
13 1.88413759681775
14 1.29481524382834
15 0.609431670139619
16 -0.252143381958623
17 -1.22079545988178
18 -2.09653714236772
19 -2.68875011729857
20 -3.68542509227806
21 -4.38473798877582
22 -5.0678211153084
23 -5.88892917652605
24 -6.74549449332986
25 -7.73479875122551
26 -8.64236593535736
27 -9.703605776425
28 -10.7733944682924
29 -11.9116616069673
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.67118869304877
1 1.83753894171216
2 0.607510421824559
3 -0.388789476691997
4 -0.15044557208733
5 -0.192546975079857
6 0.358821773446499
7 1.33364397480292
8 1.8817752254605
9 2.53439759875412
10 2.89488231627589
11 3.38181482622037
12 3.28375266891966
13 3.16729619192449
14 2.91333078147511
15 2.96579842208352
16 2.71820543273191
17 2.91488969861856
18 2.87880397926511
19 2.77806129418871
20 2.95268356567587
21 3.08049977971707
22 3.20616249712534
23 3.53314834578866
24 3.94567769550544
25 4.15392934959092
26 4.17576947728335
27 4.5780236257267
28 4.78984387188506
29 4.93497796678828
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.45947585557125
1 1.63853409511091
2 0.640296462113346
3 -0.100054699815461
4 0.114813968291017
5 0.395637923379864
6 1.42175067908173
7 2.61234393940969
8 3.35650835973777
9 3.91859843460002
10 4.04370809725658
11 4.46921656162688
12 4.24661160692368
13 3.7467628433151
14 2.88093589617227
15 2.04912570211525
16 1.37013216934515
17 1.0162202287984
18 0.514169331604135
19 -0.0336534922078489
20 -0.539624068984248
21 -0.875394080936944
22 -1.34664841763573
23 -1.49545493024725
24 -2.07182087590276
25 -2.6102519522664
26 -3.24895503796615
27 -3.67310752400727
28 -4.31560377202445
29 -5.09946364826232
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.49702527979295
1 2.05009011998423
2 0.889846155399146
3 0.0582686712932183
4 -0.0113720555080032
5 0.0685438951508104
6 0.331914989689293
7 0.966230425781768
8 1.63049104911505
9 2.0434105411191
10 1.83368446585219
11 1.55910749509825
12 0.91021337569069
13 0.414143825197426
14 -0.63758147813299
15 -1.45240935578932
16 -2.32017074945537
17 -3.31657282571002
18 -4.42570517310707
19 -5.3869070467823
20 -6.46844850966612
21 -7.63238660826853
22 -8.70352906713266
23 -9.70350171282728
24 -10.6380000157036
25 -11.7574410541693
26 -12.800707017022
27 -13.9311477323909
28 -14.9655041557577
29 -16.025908899447
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.70298495124686
1 2.19091409279405
2 0.846818266945375
3 -0.144098146873482
4 -0.199969088259067
5 -0.118235055831022
6 -0.00459135412549827
7 0.502843039813873
8 1.60894786401401
9 2.32401101575662
10 2.94212746948758
11 3.19065442065359
12 2.90890350352211
13 2.53289929512278
14 1.66531106016028
15 0.654811721064792
16 0.0224003458941837
17 -0.622556708566231
18 -1.29121840030001
19 -1.93424667169132
20 -2.36140679577779
21 -3.23365485755812
22 -3.69846429318353
23 -4.26445358658943
24 -5.02261113193519
25 -5.80373628325836
26 -6.0849627866531
27 -6.46496395391233
28 -7.09586699699206
29 -7.70643273002027
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.41266196250574
1 1.68881885527506
2 0.920641378713913
3 0.205290632368779
4 0.476259697848308
5 0.394898784335377
6 0.529146744064716
7 1.27253952840538
8 2.05184277062962
9 2.59092072238814
10 2.80741922485377
11 3.18639388907344
12 3.19657610420445
13 3.1484917911609
14 2.90339036989602
15 2.93188133153763
16 2.52571206133937
17 2.59689398008367
18 2.34545069964998
19 2.32221856330443
20 2.29257754886331
21 2.22099142792132
22 2.16594649775422
23 1.92062830770661
24 1.79078031801938
25 1.93301509450337
26 1.87926355292309
27 1.43966695433823
28 1.28349449117789
29 1.26077189026528
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.61708714695282
1 2.6039888575128
2 1.38189282020365
3 0.54759363997664
4 0.396223588833246
5 0.60395701433689
6 1.27907661769211
7 2.33046223416323
8 3.52019030481296
9 4.44395003708997
10 4.91615020160898
11 5.39973855653283
12 5.04366345701147
13 4.79671442387463
14 3.96166280586158
15 3.51298384902709
16 2.93914756810941
17 2.23067968191719
18 1.56631792836957
19 1.15745371430301
20 0.526188636157793
21 0.00468461526536146
22 -0.470892843081955
23 -0.997902933570799
24 -1.43408610086183
25 -1.88221669141607
26 -2.47120631467357
27 -3.33786866881699
28 -3.99664620340802
29 -4.47618063159133
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.21879099613857
1 1.6154299270273
2 0.600883987963034
3 -0.256130589906091
4 -0.641966870389455
5 -0.545012423392697
6 -0.290997733915841
7 0.941986997629682
8 1.70848885848761
9 2.54706733125846
10 2.68280914008794
11 3.03836006023276
12 2.97587855246912
13 2.33742548847382
14 1.6707853644491
15 0.890169824566778
16 0.470820173063712
17 -0.249657367634093
18 -0.949598688946624
19 -1.28977649422348
20 -1.74415558918916
21 -2.0989513156621
22 -2.57805246226989
23 -3.28089910172165
24 -4.0633131140578
25 -4.76322410476811
26 -5.28518670439999
27 -5.82559461636148
28 -6.37178329402157
29 -7.04366315558309
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.5580886040598
1 2.05050299682174
2 0.847305849562487
3 0.275190515052861
4 0.366950746757768
5 0.284062018291825
6 0.924666698642934
7 2.02269330602111
8 3.29365111694727
9 4.37403232711213
10 5.07814402481453
11 5.09571793518911
12 4.68406353714561
13 4.17485982245585
14 3.30300432263486
15 2.66784308697929
16 1.82389689920837
17 1.16314746224602
18 0.609422091887255
19 -0.295952359600266
20 -0.968389308322893
21 -1.50177547770001
22 -2.18035839050538
23 -2.86868794945984
24 -3.58367840060782
25 -4.3391752620356
26 -5.14406863963293
27 -5.81308439349446
28 -6.66324079639169
29 -7.47345429664766
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.18580511457684
1 1.33590704498062
2 0.0457505938324569
3 -0.624997860664665
4 -0.785059151072595
5 -1.09156770646567
6 -1.25096876405481
7 -0.499318713627915
8 0.298399885267777
9 0.935245817784919
10 1.0486318229443
11 1.48323634865919
12 1.14068201264867
13 1.07021570771394
14 0.757704382184178
15 0.169733361260159
16 -0.325675562695025
17 -0.60460362127097
18 -1.10765978500892
19 -1.49797524033272
20 -1.77891282510287
21 -2.06891205860326
22 -2.54857680700819
23 -2.82639740102089
24 -3.30681326763118
25 -3.89024932902147
26 -4.36782182689735
27 -4.80204794876986
28 -5.30525321589301
29 -5.957711816799
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.47304667391637
1 1.68062254004544
2 0.649524694665191
3 -0.202394465895555
4 0.0918701584306074
5 0.0832258855982424
6 0.223745130063396
7 0.726596057600378
8 1.76096927582822
9 2.84158747712249
10 3.55581721606261
11 4.22164584145776
12 3.63451347056828
13 2.96503423549254
14 1.9336174990139
15 1.06817454073297
16 0.102471154523364
17 -0.806743666234567
18 -1.74993088143967
19 -2.48582410965282
20 -3.18524392537601
21 -3.85724088240602
22 -4.72102813598256
23 -5.30417671784578
24 -6.15588790717525
25 -7.29246338509665
26 -8.17122887843664
27 -8.85881345499617
28 -9.64784536790648
29 -10.5220338861082
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.71180745484452
1 2.13327849584911
2 0.962815638489248
3 0.102670427157252
4 0.390486774376294
5 0.513050201105806
6 1.37843963333861
7 2.39271652110924
8 3.39582954529271
9 4.23939991215617
10 4.56199907826469
11 4.51313852953463
12 4.29548046032312
13 3.97912552209978
14 3.32635510241958
15 2.74421997750359
16 1.873862121793
17 1.28223475335211
18 0.860889035211358
19 0.0453110621840835
20 -0.540301251623044
21 -1.30155181756695
22 -2.29992285553088
23 -3.04680102311592
24 -4.03201658415171
25 -5.069718277824
26 -6.08729718353822
27 -7.13830699056134
28 -8.10892743023669
29 -9.22717693360346
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.6318276695961
1 1.96288238028836
2 0.915866241023757
3 0.406831109611323
4 0.801981944913969
5 1.40876703911327
6 2.43842265875765
7 3.70162939102626
8 4.71182030846206
9 5.49079531856058
10 6.27292169445496
11 6.86693778150386
12 6.69076733859369
13 6.41585531730658
14 6.07746476885682
15 5.77697672473427
16 5.76796859281252
17 5.91729156106864
18 5.83268919829703
19 6.04737954810041
20 6.28557449647825
21 6.42150842119987
22 6.74948269018679
23 7.05552824752717
24 7.10572437073244
25 7.47260506530455
26 7.93734909945906
27 8.06229963023739
28 8.4525692132425
29 8.74841219932729
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.67953268899794
1 2.10772921570662
2 1.17859165476992
3 0.692929299844977
4 1.35335448850732
5 1.62381417829932
6 1.96130322774569
7 3.32093791030863
8 4.36826111689517
9 5.22277891702188
10 5.44027830948928
11 6.03542213980876
12 5.80857946988982
13 5.08827144202809
14 4.46939932312814
15 3.87166518090771
16 3.07902652792793
17 2.69790672034229
18 2.29441207586672
19 1.65411525755188
20 1.33248486307257
21 0.708084973493079
22 0.112857735630183
23 -0.287795506081338
24 -1.18871614006775
25 -1.82530989620391
26 -2.50472068424581
27 -3.21203104063378
28 -3.85729963044603
29 -4.55744174555877
};
\end{groupplot}

\begin{groupplot}[group style={group size=1 by 3}]
\nextgroupplot[
xshift=-8,
xmin=-1.45, xmax=30.45,
%ymin=2.65977698435744, ymax=6.38414108671984,
ymin=2.7, ymax=6.7,
width=\figurewidth,
height=\figureheight,
xtick={},
xticklabels={},
yticklabels={},
tick align=outside,
tick pos=left,
x grid style={white!69.019607843137251!black},
y grid style={white!69.019607843137251!black}
]
\addplot [line width=0.06pt, color0, mark=*, mark size=2, mark options={solid,draw=black}]
table {%
0 3.31996634253658
1 3.45443899460193
2 3.38784218387077
3 3.01931286439371
4 2.82906626173755
5 3.09427938765557
6 3.60416870184349
7 4.24596487007442
8 4.84338888587772
9 5.27994908427636
10 5.61004074039071
11 5.90268352537916
12 6.05852129333431
13 6.16858387553312
14 6.19509636026208
15 6.21485180933973
16 6.20378189365436
17 6.1468591562609
18 6.14787992255152
19 6.14579317317396
20 6.15283082950704
21 6.15412613868876
22 6.14366281427887
23 6.16587792193215
24 6.18223254289368
25 6.18638821201769
26 6.14794417270148
27 6.14179954980725
28 6.15812095860932
29 6.16746194810668
};
\end{groupplot}

\begin{groupplot}[group style={group size=1 by 3}]
\nextgroupplot[
xshift=-8,
xmin=-1.45, xmax=30.45,
%ymin=-0.848571901426494, ymax=2.81768238587247,
ymin=-0.85, ymax=5.85,
width=\figurewidth,
height=\figureheight,
xtick={},
xticklabels={},
yticklabels={},
axis y line=right,
tick align=outside,
xtick pos=left,
ytick pos=right,
x grid style={white!69.019607843137251!black},
y grid style={white!69.019607843137251!black}
]
\addplot [line width=0.06pt, color1, mark=*, mark size=2, mark options={solid,draw=black}]
table {%
0 2.65103446372252
1 1.87298481713709
2 1.03310235020523
3 -0.0349224785257646
4 -0.681923979276541
5 -0.614035490335335
6 -0.208100847346677
7 0.33428430837777
8 0.710486243049944
9 0.726233644866842
10 0.520411660737353
11 0.347599665643602
12 0.244300607278545
13 0.195112904269273
14 0.20629800498181
15 0.161911176310666
16 0.161283251423433
17 0.247899352697984
18 0.208651205023874
19 0.171253015388636
20 0.20029198108343
21 0.172890109571832
22 0.187770311286831
23 0.213147053788955
24 0.185796243819713
25 0.165625930691843
26 0.187584184388062
27 0.20252014981221
28 0.179459395114634
29 0.2013127196102
};
\end{groupplot}

==> experiments/figs/sup_mat/tikz_samples_ep-8-all.tex <==
\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}

\begin{groupplot}[group style={group size=1 by 3}]
\nextgroupplot[
xshift=-8,
title={8 episodes},
title style={font=\large},
xmin=-1.45, xmax=30.45,
%ymin=1.45279922629327, ymax=6.59122540478087,
ymin=2.7, ymax=6.7,
width=\figurewidth,
height=\figureheight,
xtick={},
xticklabels={},
yticklabels={},
tick align=outside,
tick pos=left,
x grid style={white!69.019607843137251!black},
y grid style={white!69.019607843137251!black}
]
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.48337875869527
1 3.6442202037301
2 3.66282466808451
3 3.36453350774775
4 3.27965046788557
5 3.29208727891878
6 3.39261136185822
7 3.45003434238356
8 3.28031762306548
9 2.98757875182044
10 2.78244171044778
11 2.72029312396403
12 2.48995444583512
13 2.26150669313712
14 2.05177589427387
15 1.84316686578503
16 1.64678010962233
17 1.48731584272048
18 1.26190536714608
19 1.10980469739296
20 0.796799009314428
21 0.679425175258739
22 0.373051054486364
23 0.0659012195365154
24 -0.182576403015553
25 -0.564756018533565
26 -0.953884405591626
27 -1.2728656887166
28 -1.71057071845999
29 -2.14930639957504
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.75692694683593
1 4.01014900262247
2 3.84176781894086
3 3.47793920274067
4 3.38911663383903
5 3.63948850617803
6 3.88004880307313
7 3.98895927965018
8 3.87870065992497
9 3.93332641368873
10 3.79027531766603
11 3.83766111162598
12 3.64323390690747
13 3.43222694513809
14 3.20386024669403
15 2.97112072254271
16 2.73532236190239
17 2.79499737448877
18 3.08226953384808
19 3.50520445560815
20 3.83785745327285
21 4.06772072217622
22 4.12065818974769
23 3.99816253559129
24 3.74832459086682
25 3.33470852038491
26 3.10118519038182
27 3.10661933782059
28 3.19068114809326
29 3.47441749704563
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.65234732581682
1 3.90010842653655
2 3.63938621913213
3 3.36216327308807
4 3.32203809417704
5 3.63120797879368
6 3.9928402058386
7 4.07817832344486
8 4.23180001394492
9 4.40839427054663
10 4.51243257420724
11 4.56874205781971
12 4.41662005422091
13 4.38088843028637
14 4.38447991144576
15 4.41665054810174
16 4.30117435453017
17 4.18020512972514
18 4.14805723336751
19 3.95851209545402
20 3.8557265033704
21 3.98884736350419
22 4.12402241911154
23 4.33147122547376
24 4.50298236677333
25 4.60929015112806
26 4.5918796656371
27 4.45418341405489
28 4.2941886562424
29 4.16389658239248
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.75122655419372
1 4.07901111583593
2 3.8984151782181
3 3.61417579327541
4 3.48566880818386
5 3.6979929692895
6 3.98859862505109
7 4.00313004113371
8 3.92224789987416
9 4.14703322285152
10 4.4331853079169
11 4.91805343191512
12 5.4003906763876
13 5.81160735787195
14 5.95016323116149
15 6.08444721693215
16 5.79036059685789
17 5.50478027071253
18 5.19288623253458
19 5.07790749538615
20 4.93931117889542
21 4.98050369649413
22 5.18343388000498
23 5.37599817667426
24 5.61256760108844
25 5.84456361250139
26 5.89711292267137
27 5.97847317601459
28 5.92382737928073
29 5.8989496494955
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.6568350896717
1 4.02176498329454
2 4.05344731636131
3 3.74774990808631
4 3.67932077661175
5 3.75331385075798
6 3.74208352467637
7 3.60409617440468
8 3.53846299141638
9 3.47710327277611
10 3.23195537667875
11 3.17478822566972
12 2.91958263313008
13 2.45672519236248
14 1.90549630231465
15 1.25486578675158
16 0.807087184272254
17 0.291396411928766
18 0.00064833090104699
19 -0.363798879794606
20 -0.570911397091843
21 -0.912194161316233
22 -1.40494077120224
23 -1.92064285974698
24 -2.47878285434533
25 -2.98364535849569
26 -3.4509188483338
27 -3.78892201317439
28 -4.16632372416114
29 -4.57639451005674
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.87098666412201
1 4.12093277573055
2 3.98626372845992
3 3.82698242426428
4 3.76036070108147
5 3.82944860022407
6 3.76362125608429
7 3.68189982114874
8 3.47336439679899
9 3.85813465387593
10 4.26266344937843
11 4.68812783526384
12 4.98562372080937
13 5.12711303054221
14 5.23147767073895
15 5.02608680465105
16 4.74697212501896
17 4.4848599318816
18 4.30556152782077
19 4.08820107866623
20 3.87440167315797
21 3.94087801353455
22 4.10863244160597
23 4.2820411330909
24 4.51494352332015
25 4.69024004908491
26 4.71061148432857
27 4.77384674269846
28 4.81829433956539
29 4.91505539191804
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.53945268349674
1 3.7370250177998
2 3.68028427583068
3 3.64278633528485
4 3.69759559145772
5 3.84883842628306
6 3.98228073317847
7 4.00170976660768
8 4.11107631725844
9 4.30248595941989
10 4.30968685920947
11 4.25912925325406
12 4.13381932570561
13 3.840099870979
14 3.62609213468741
15 3.41363410695543
16 3.13743502739556
17 3.06650851868855
18 3.23579179701332
19 3.49623781782729
20 3.8919297974781
21 4.24568418796184
22 4.58389358413321
23 4.73877594357643
24 4.72321095988689
25 4.54276335747558
26 4.319444191326
27 4.19624900353447
28 4.12218697444437
29 4.19400406398713
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.73574178546096
1 4.01898640462085
2 3.97435821108532
3 3.78860290919008
4 3.72443461978893
5 3.99558092297967
6 4.14504007228924
7 4.25032624223739
8 4.32940692966766
9 4.5331160994636
10 4.63553918079801
11 4.72117706494963
12 4.65596791231052
13 4.34970658445617
14 4.43074221078944
15 4.46937307417792
16 4.4302042920591
17 4.39232182210118
18 4.38447372454579
19 4.38271915111191
20 4.25407018154569
21 4.25723872422524
22 4.40287483881216
23 4.54507908619838
24 4.55557864473132
25 4.58373300239576
26 4.52423415306044
27 4.45531896393169
28 4.48153041254366
29 4.57918336539489
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.75485920290594
1 3.96842605176422
2 3.80900874237053
3 3.67144964057277
4 3.53701625967359
5 3.70182056516957
6 3.74456148580934
7 3.88169332084518
8 4.08262721583412
9 4.29454231544214
10 4.44244093324172
11 4.61186135261001
12 4.4676483576001
13 4.26831067437921
14 4.06192383422567
15 3.98394533792294
16 3.85617648780099
17 3.95910019502746
18 4.21436553140894
19 4.45294936824948
20 4.68299498329539
21 4.91428368556922
22 5.12172771363984
23 5.12133269429512
24 5.22824201419339
25 5.33394286079186
26 5.30985192593281
27 5.27382060165261
28 5.27268445194817
29 5.25289193551714
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.69581243955628
1 3.91887573365133
2 3.87355098313053
3 3.53003109168975
4 3.48337107751317
5 3.73233264825417
6 3.91737820902166
7 3.75168074706782
8 3.56900913848411
9 3.42263408566148
10 3.22737774852689
11 2.82983146349931
12 2.39860326926466
13 1.93102289003277
14 1.54121694104587
15 1.17581164637895
16 0.997737779186016
17 0.644961519609529
18 0.380081086889344
19 -0.052271940784701
20 -0.572752593366785
21 -1.09203909161029
22 -1.60500772762445
23 -2.15046281788578
24 -2.70473998409462
25 -3.30946770521974
26 -3.84737504233836
27 -4.35473942952219
28 -4.90375584205518
29 -5.36077982413389
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.7856298254202
1 4.09630485351153
2 4.08807681540183
3 3.88651958075562
4 3.87183050240927
5 4.02412001602768
6 4.05030855418972
7 3.97514465244214
8 3.84120715810627
9 3.78155396382583
10 3.59643393078013
11 3.53863554949776
12 3.04598396354397
13 2.52456652994421
14 1.98818312964271
15 1.54888723283305
16 1.25733960870063
17 1.09578124516476
18 1.04394400759814
19 1.26512378284637
20 1.3880493830703
21 1.50354769614053
22 1.53277698941767
23 1.28199883492338
24 1.03871081771662
25 0.532317805528981
26 0.0781959945317521
27 -0.309353433490054
28 -0.894413262014664
29 -1.57284514716435
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.64573686481737
1 3.78479644012612
2 3.75901502677705
3 3.66378648182119
4 3.67290209807681
5 4.03135821590982
6 4.15136894290023
7 4.01247280852929
8 3.92282489750376
9 3.80499433663094
10 3.88970247250222
11 3.91506837853817
12 3.87490231586382
13 3.85250290953584
14 3.860039844322
15 3.88171267365335
16 3.75335582017392
17 3.58179325539474
18 3.28797457128038
19 2.9332741259104
20 2.61218971624792
21 2.54116643642831
22 2.53828301484527
23 2.53805660596948
24 2.67163961361724
25 2.74805339078508
26 2.82904708945047
27 2.81904394945592
28 2.84575252593818
29 2.83783689860793
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.71763152540294
1 3.94605377228024
2 3.57434577967726
3 3.08827707115009
4 2.90157722278035
5 3.05261601262763
6 3.21223813928705
7 3.45599048309542
8 3.44898015216311
9 3.5824886263218
10 3.81327465312553
11 3.99714693215204
12 3.84115332463437
13 3.77098343302155
14 3.58834515695817
15 3.47451379665512
16 3.17809394347855
17 3.00091365021702
18 2.8963732222488
19 2.92421569406842
20 2.98605587128072
21 3.1748592334647
22 3.35298842338556
23 3.51828345761705
24 3.51492586433345
25 3.52824549606665
26 3.51787899330005
27 3.42194571217321
28 3.41270635041167
29 3.3535310767473
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.92980368462784
1 4.15241060259077
2 3.90172987815915
3 3.66475666036754
4 3.30507022544961
5 3.357641997975
6 3.55206162297724
7 3.9116867954236
8 4.10419848614916
9 4.35367103534581
10 4.6227383789132
11 4.62185851001647
12 4.43356851381904
13 4.25250268985707
14 3.93726871410397
15 3.73991025176629
16 3.61441611335777
17 3.61813900023431
18 3.68221689399896
19 4.16111406013854
20 4.45168793674757
21 4.85080669672653
22 5.2668314934224
23 5.5150248465053
24 5.73160684788407
25 5.85624776741652
26 5.88191360876757
27 5.84502060973749
28 5.9267994373716
29 5.8496709670095
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.87541415708238
1 4.08993418870803
2 3.89007595517407
3 3.6310241125162
4 3.47161634574683
5 3.47562892044868
6 3.56878422847304
7 3.56202867533099
8 3.51883732818689
9 3.61514470518779
10 3.9013164792277
11 4.13197184761291
12 4.39868122377741
13 4.48162402988892
14 4.55060530801949
15 4.653854028617
16 4.78185489540605
17 4.95556724952147
18 5.03780537232518
19 4.9234087081531
20 4.85457549910474
21 4.95426343560363
22 4.94507110878404
23 5.039250050742
24 5.3380246735513
25 5.62880775370637
26 5.71056846373902
27 5.72706488201095
28 5.57354318609019
29 5.4780129749678
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.64242913543583
1 3.96247246668598
2 3.97072102534323
3 3.95465564375668
4 3.87088855458676
5 4.05911801007885
6 4.37459654142961
7 4.49434582700594
8 4.28262598082436
9 4.28054974233086
10 4.35451886161533
11 4.45626355116605
12 4.47763722476805
13 4.55406385398167
14 4.71153092192055
15 5.02889564673771
16 5.14992632579977
17 5.06680425515105
18 4.98444755585941
19 4.86475602048422
20 4.84508077642069
21 4.90957164005385
22 4.93391910464057
23 5.17727019515626
24 5.39718387152821
25 5.67522479801721
26 5.78519524786402
27 5.87470225566531
28 5.94729254902164
29 5.94398573843628
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.7456656750272
1 3.98084573429858
2 3.9296144290903
3 3.73484504914595
4 3.61867234557538
5 3.84451748054673
6 4.0348780224517
7 4.2962093783034
8 4.38990889151089
9 4.44354752581499
10 4.51218109274764
11 4.47223181956849
12 4.30392685969749
13 4.41064217800854
14 4.57823613268433
15 4.87551822424888
16 5.09090140723769
17 5.26958621080005
18 5.44557232971366
19 5.57430796679935
20 5.63337246923994
21 5.58948045633056
22 5.64778943384696
23 5.77819391547392
24 5.89577373898171
25 6.00972748227465
26 6.2193326050542
27 6.47318808559541
28 6.59146714210536
29 6.72948702875354
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.87288789603665
1 4.17483681681896
2 4.17654543231314
3 3.89192263230608
4 3.68899188935305
5 3.83030574414674
6 3.95993059621402
7 4.16920489951448
8 4.35464511489283
9 4.56620365645315
10 4.60299826153757
11 4.41666146905337
12 4.10182197078316
13 3.58485562097327
14 2.9564504615239
15 2.57991697073926
16 2.47810896146473
17 2.49475192443373
18 2.77479784294432
19 3.3011060565353
20 3.65054397658144
21 4.12763154281841
22 4.39023998964417
23 4.23750570425577
24 3.9932291138581
25 3.54114971315715
26 3.23682900952312
27 3.08468640088209
28 3.11253884174229
29 3.3776434988986
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.86026056634126
1 4.28954618265937
2 4.31331348028386
3 4.34915544162042
4 4.25169277820764
5 4.31180610780142
6 4.27292372548523
7 4.16590675858998
8 4.06560010306182
9 4.10801917742977
10 4.07055872339201
11 3.96181968366082
12 3.64938985951848
13 3.51517454070201
14 3.39227779562857
15 3.48092321318838
16 3.53291887738918
17 3.6609868213714
18 3.85217669065652
19 3.9784678862473
20 3.99998827425934
21 4.09290629574085
22 4.2508733701415
23 4.24897287735535
24 4.50461026137931
25 4.63366439529667
26 4.80312787783364
27 4.81577093102074
28 4.9506379945922
29 5.18886836218157
};
\addplot [semithick, color0, opacity=0.3]
table {%
0 3.69712382969966
1 3.92212007735063
2 3.82703785211794
3 3.71092597942983
4 3.74075887807424
5 3.80974547115642
6 3.86134445003896
7 3.71046819196614
8 3.36498374618602
9 3.10754142822998
10 2.89982910841615
11 2.63175301397082
12 2.12231827583077
13 1.51655739657703
14 1.05028941892878
15 0.432784400725952
16 -0.032415520205074
17 -0.516637340562635
18 -1.08757342130684
19 -1.69080507993
20 -2.27253035985337
21 -2.76849265246961
22 -3.33529575350975
23 -3.73400561520718
24 -4.21803253716014
25 -4.73043950328871
26 -5.28384382850145
27 -5.76341763501967
28 -6.23442454821156
29 -6.69810738871337
};
\end{groupplot}

\begin{groupplot}[group style={group size=1 by 3}]
\nextgroupplot[
xshift=-8,
xmin=-1.45, xmax=30.45,
%ymin=-2.46891241301875, ymax=46.6986447843329,
ymin=-0.85, ymax=5.85,
width=\figurewidth,
height=\figureheight,
xtick={},
xticklabels={},
yticklabels={},
axis y line=right,
tick align=outside,
xtick pos=left,
ytick pos=right,
x grid style={white!69.019607843137251!black},
y grid style={white!69.019607843137251!black}
]
\addplot [semithick, color1, opacity=0.3]
table {%
0 1.99461017672552
1 0.827397330337661
2 -0.377487921631158
3 -1.64492547155563
4 -2.67206975415198
5 -3.69021788830489
6 -3.74518413527199
7 -2.99427166820469
8 -2.06917161658307
9 -1.39218209477295
10 -1.21058707882414
11 -0.999428943155051
12 -1.02640819823377
13 -1.22678118019291
14 -1.43760087933121
15 -1.94543140707707
16 -2.50283519333045
17 -3.43898295261109
18 -4.58058081199334
19 -5.80160665527764
20 -7.2526037237346
21 -8.59529989589816
22 -9.8473458968948
23 -10.7755097979289
24 -11.7731676881498
25 -12.5747008248684
26 -13.0842068585951
27 -13.6985481759729
28 -14.1931084595232
29 -14.6971176429522
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.39885257478199
1 1.55443614941206
2 0.363775882548737
3 -0.715888628494877
4 -1.41098340476658
5 -1.79131499472773
6 -1.75987184283016
7 -1.07424956211091
8 0.0294015827155558
9 0.760981984249575
10 1.13992533208294
11 1.70952542120269
12 1.96812308357942
13 2.10346420866903
14 2.10002176401301
15 2.40504847763257
16 2.48853501838962
17 2.72327801194155
18 2.41254642598856
19 2.03966301170832
20 1.73135152742586
21 1.53896462944886
22 1.58965481522817
23 1.88414214001336
24 2.03060655753461
25 2.32300074684652
26 2.66529131036937
27 2.78458313951143
28 2.86213343524897
29 2.89731874313489
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.45453667866042
1 1.56836218173971
2 0.437027028580443
3 -0.250968720457816
4 -0.850396281877552
5 -0.887731136219344
6 -0.695649682254547
7 0.18295530252189
8 1.49829773060017
9 2.01038624121872
10 2.64452353647915
11 3.32965000511349
12 3.47231365988185
13 3.52977177435953
14 3.22968726230891
15 3.30866852167292
16 3.27779550663195
17 3.34369546361843
18 3.3626177961707
19 3.54406863515322
20 3.61243556870935
21 3.411023115105
22 3.43992837487628
23 3.30100753664147
24 3.24215446229016
25 3.23071933553916
26 3.25986540329249
27 3.39333146121557
28 3.43120747256236
29 3.4842488375827
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.69278778085465
1 1.93847872297612
2 1.08393553059563
3 0.370487022229572
4 -0.000395202589444921
5 0.199780089976102
6 0.80598326953789
7 2.0642637708215
8 3.48396042277964
9 4.01199124517597
10 4.38612333467757
11 4.49218518940418
12 4.27722473596879
13 4.21668129641129
14 4.12173800000473
15 3.99160592307866
16 4.33232089623921
17 4.56597259430976
18 4.7832323668745
19 4.9495786645893
20 5.05304518773267
21 4.80779822101048
22 4.63961280789511
23 4.5838666461479
24 4.50931229560942
25 4.573450127647
26 4.7615920736987
27 4.85399115580068
28 5.03508577085903
29 5.3866927420163
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.35216456807257
1 1.24327038488901
2 -0.0163412927321858
3 -1.25186424740748
4 -2.18334113346784
5 -2.81567564037371
6 -3.01421923451723
7 -2.80932471740986
8 -1.89986718714576
9 -1.51502945525684
10 -1.61947417153253
11 -1.77520147002146
12 -2.3950257260827
13 -3.00909083582242
14 -3.74049262718714
15 -4.67108780532389
16 -5.74323480664615
17 -7.29677061422106
18 -8.58509214482359
19 -9.8117957230651
20 -10.9919059736211
21 -12.125924946692
22 -13.3323290490169
23 -14.3469684935679
24 -15.2632391852358
25 -16.2806101153986
26 -16.9399298358848
27 -17.4050907132992
28 -17.8163687153338
29 -18.4991648773121
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.30959573012918
1 1.71001221143436
2 1.07792430693352
3 0.630574984997118
4 0.238518206383945
5 0.55458898592436
6 1.28765230673705
7 2.43499858847068
8 3.8359970248021
9 4.38673216308278
10 4.55980538581475
11 4.39370559018588
12 4.06441473371834
13 3.76393128808139
14 3.44103223303614
15 3.41296758731246
16 3.6918680470943
17 3.74401876843425
18 3.94912980136757
19 4.12312268376747
20 4.21150206604718
21 4.33613158699382
22 4.57374589311995
23 4.64175408549407
24 4.66109880833776
25 4.69239736275476
26 4.80210300178135
27 4.84328517702675
28 4.88064707792347
29 5.01074844574788
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.43537759705551
1 1.42770184040541
2 0.531578421509849
3 -0.258310275883611
4 -1.02814237389804
5 -1.1794671908212
6 -0.863403138503735
7 -0.241837028697741
8 0.506012988701126
9 1.13750094304367
10 1.50177798788923
11 1.92651926148077
12 2.37060297888604
13 2.47140928565647
14 2.53518533232527
15 2.79748562464407
16 2.9904419924704
17 3.21683854092459
18 3.28987769294083
19 3.08117457845938
20 2.9687271346252
21 2.73474373412524
22 2.60560417673512
23 2.68175781865171
24 2.78344654034236
25 2.93578554935012
26 3.29794851398456
27 3.61367019420044
28 4.00912280959897
29 4.30070449146154
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.52021851563423
1 1.74057020148982
2 0.70178589580803
3 -0.216971289859018
4 -0.688047392577126
5 -0.757927881514766
6 -0.446378266058659
7 0.624642292694491
8 1.8676978421172
9 2.71377397681399
10 3.40427192225047
11 3.94256248929903
12 4.13363532725283
13 4.06122607914693
14 3.87980434338915
15 3.56447828113606
16 3.56562801946567
17 3.7254204997124
18 3.72541252003617
19 3.79984256048527
20 4.03452139612418
21 3.98312822768021
22 4.1269054438837
23 4.23883179550966
24 4.11575846823425
25 4.20356512308793
26 4.26187888183372
27 4.44056774113485
28 4.4640294542653
29 4.4737999475353
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.2622638127073
1 1.31457929488215
2 0.149301934569104
3 -0.631879977314568
4 -1.06243692984532
5 -0.963550801353517
6 -0.761578516401904
7 -0.0652961704663078
8 0.903469093868605
9 1.59417778421812
10 2.34375470677474
11 2.88262834619849
12 3.19917768620117
13 3.41043355739356
14 3.56354029160057
15 3.57409217186134
16 3.71271186645883
17 3.91317294518803
18 3.75479286026351
19 3.76597359900927
20 3.84959483790308
21 3.98566172861346
22 4.20409209925658
23 4.4116043987448
24 4.47473863800988
25 4.58485086627765
26 4.8869841909284
27 5.02316143460424
28 5.07075439318583
29 5.20799963162311
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.0096791884375
1 0.991040172776348
2 -0.349900104366517
3 -1.69591702568425
4 -2.6480725993295
5 -3.15119800940822
6 -3.11063539331121
7 -2.3491935521829
8 -1.47333738704934
9 -1.08285199741858
10 -1.02890678144074
11 -0.978053782451926
12 -1.32633995053428
13 -1.81315707372143
14 -2.50290578209164
15 -3.73739643229942
16 -4.86934974312708
17 -6.31942612840846
18 -7.8210633487278
19 -9.66724467069437
20 -11.1738707487261
21 -12.4662530491203
22 -13.6519861296607
23 -14.7908742181902
24 -15.6714679033192
25 -16.4654488967341
26 -17.0486489423882
27 -17.951383902638
28 -18.5518655748988
29 -18.873797965001
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.36765378651552
1 1.38499440579082
2 0.352797392947577
3 -0.348362883308786
4 -1.08861964138042
5 -1.60678911772122
6 -2.08234970138046
7 -1.92193626485633
8 -0.961391333835175
9 -0.578765012153761
10 -0.329685360363662
11 -0.0952719997615414
12 -0.404077637513396
13 -0.822431956061342
14 -1.1548590729542
15 -1.55913240732626
16 -1.87474737016176
17 -2.04942789997101
18 -2.42167226596014
19 -2.83377062773073
20 -3.44409749497884
21 -4.0801649931814
22 -4.76395739210256
23 -5.89806115295164
24 -6.84710702604742
25 -7.95998801140924
26 -9.08726140834647
27 -10.1368964012825
28 -11.1354449978007
29 -12.1443297476642
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.19343832813298
1 1.41863170980538
2 0.661251604152236
3 -0.132150962436018
4 -0.864338689445006
5 -1.21238449552417
6 -1.24577358153776
7 -0.583723388590824
8 0.55931500134024
9 1.16795499352602
10 1.8198345539299
11 2.26705237508012
12 2.29866624137685
13 2.14546857633499
14 1.89232471670018
15 1.67957613114191
16 1.5200406815462
17 1.51876825311286
18 1.44519131607588
19 1.5304428144022
20 1.50580497370789
21 1.49813635383157
22 1.52930810094324
23 1.34711794947988
24 1.2858503073271
25 1.11465652030522
26 0.819498176471054
27 0.714513842417864
28 0.498256467901353
29 0.166702256362214
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.42506003689749
1 1.43668541112496
2 0.244011318021105
3 -0.691783203000709
4 -1.21728588065206
5 -1.50031501692393
6 -1.39058077128278
7 -0.789821543144868
8 0.0584214923778799
9 0.776473799667331
10 1.25753318674992
11 1.65176227783974
12 1.70195584692446
13 1.8586433336953
14 1.92322666054159
15 1.84486559602889
16 1.71571280180357
17 1.6934161056575
18 1.5768235822147
19 1.79725469992804
20 1.8225383859363
21 1.82149847089649
22 1.79780594102779
23 1.83747040264958
24 1.56629636391772
25 1.3281376145392
26 1.28567937271598
27 1.35485683917309
28 1.41161687823879
29 1.42005945078185
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.30798502231453
1 1.30414353422589
2 0.275243571559624
3 -0.557516364962629
4 -1.01907860176867
5 -1.25320946117963
6 -1.0852305206993
7 -0.490600230746743
8 0.62923826594894
9 1.2079251631749
10 1.87720002025102
11 2.28429159778494
12 2.77743825153589
13 3.10638991955788
14 3.55088136076224
15 3.77043008321806
16 4.13469151530509
17 4.45436182057677
18 4.59188842445298
19 4.77968126547275
20 5.09485810486102
21 5.36199972523518
22 5.60259516830553
23 5.88816389569383
24 6.03643253986177
25 6.30199957581043
26 6.67312346677868
27 7.02153230872913
28 7.39415096620553
29 7.76134983280909
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.2555166824542
1 1.4348837961966
2 0.349149177428572
3 -0.528626257165866
4 -1.0981389727185
5 -1.33261845365992
6 -1.10266382602354
7 -0.279496660733933
8 0.865199620078856
9 1.68341059486656
10 2.31960372513849
11 2.82674821635305
12 3.24974316588945
13 3.3362305517646
14 3.29799938364185
15 3.28907604885197
16 3.33535274324892
17 3.49007050826604
18 3.74417707055337
19 3.83849310220018
20 3.98814655522294
21 4.07926757252283
22 4.02780291432875
23 4.17888143103723
24 4.17286931698469
25 4.16455450289857
26 4.24507579101065
27 4.53451530083713
28 4.81511401957661
29 4.64666442088688
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.53103163672522
1 1.83836639874313
2 0.805356670882457
3 0.182583293226992
4 -0.470411576220197
5 -0.571610502126893
6 -0.310167164136525
7 0.686287971969948
8 1.63440760004951
9 2.24900961746523
10 2.96742552859612
11 3.57163649790504
12 3.93524804073968
13 3.98882913545796
14 3.94255597960029
15 3.72717690591525
16 3.43862615455369
17 3.5666049709496
18 3.67663364364145
19 4.03406729742686
20 4.37514276378681
21 4.58649666897098
22 4.72927104777996
23 4.56473184178637
24 4.59125224615829
25 4.5273121612386
26 4.66302610674861
27 4.98645046997916
28 5.22790664614146
29 5.53383020046095
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.68280213935676
1 1.90706140164081
2 1.01140599143988
3 0.350375216488683
4 -0.21337077865048
5 -0.135720179443565
6 0.265368413986351
7 1.15964252765423
8 2.31877084567818
9 2.96627418066009
10 3.53499161860014
11 4.13680939013969
12 4.73204768491517
13 4.81848540919144
14 4.49890515135081
15 4.42220453541445
16 4.67096089718402
17 4.84817211290194
18 4.9238336531802
19 5.18324308632239
20 5.38521439166348
21 5.5388659531573
22 5.65927350812602
23 5.93501056848117
24 6.17358397513354
25 6.46077202887095
26 6.7999408390064
27 7.00146107459028
28 7.12500284439427
29 7.4487854443086
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.21444776014574
1 1.25556248820565
2 0.174639571103585
3 -0.640205734851516
4 -1.17961810884137
5 -1.06674292348844
6 -0.953049654448522
7 -0.349873507361893
8 0.205086394942443
9 0.598082630230902
10 0.969233044158347
11 1.46400749992559
12 1.64555600296063
13 1.92583270680584
14 2.08485696277695
15 2.1397145218112
16 2.3253153020055
17 2.38293768560135
18 2.30295684638456
19 2.23979805435575
20 2.2980117145038
21 2.25201320591605
22 2.2868659239179
23 2.44636192511403
24 2.65001017696619
25 2.72552172224684
26 2.80597952860173
27 2.81577872680342
28 2.79337010199495
29 2.86979817244769
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 2.59578321115962
1 1.72003968291617
2 0.626366092718737
3 -0.151492935504921
4 -0.521001734217201
5 -0.777923050102341
6 -0.523794431534583
7 0.209646787092883
8 0.72562588380293
9 1.1600816713637
10 1.36305400823716
11 1.84755551056985
12 2.23351264192174
13 2.45964565463916
14 2.46732187746045
15 2.50051131676197
16 2.53834745789506
17 2.6759130475762
18 2.67696710219255
19 2.85071609596967
20 3.11257769103067
21 3.21529961429664
22 3.39652038955742
23 3.62964390053373
24 3.83244486499634
25 4.02337913154487
26 4.23143070511489
27 4.5000985954228
28 4.78272447801652
29 4.89276955577757
};
\addplot [semithick, color1, opacity=0.3]
table {%
0 1.90667953803294
1 0.756842711263184
2 -0.418048861923085
3 -1.72528167493683
4 -2.68285990688276
5 -3.57643581221407
6 -4.30971526018273
7 -4.20978809447368
8 -4.05000035344417
9 -4.19600565569071
10 -4.36321779593588
11 -4.7127940364656
12 -5.61082881135376
13 -6.56961664142302
14 -7.61643774724871
15 -8.75620937105619
16 -9.92817796598784
17 -10.8966593935777
18 -11.7790841128455
19 -12.7648066926123
20 -13.4648461113987
21 -14.1321506768745
22 -14.7648404852256
23 -15.2034038572113
24 -15.9628795011629
25 -16.6666734665683
26 -17.1834911352629
27 -17.6404355430797
28 -18.0881163954135
29 -18.6795022254001
};
\end{groupplot}

\begin{groupplot}[group style={group size=1 by 3}]
\nextgroupplot[
xshift=-8,
xmin=-1.45, xmax=30.45,
%ymin=2.65977698435744, ymax=6.38414108671984,
ymin=2.7, ymax=6.7,
width=\figurewidth,
height=\figureheight,
xtick={},
xticklabels={},
yticklabels={},
tick align=outside,
tick pos=left,
x grid style={white!69.019607843137251!black},
y grid style={white!69.019607843137251!black}
]
\addplot [line width=0.06pt, color0, mark=*, mark size=2, mark options={solid,draw=black}]
table {%
0 3.31996634253658
1 3.45443899460193
2 3.38784218387077
3 3.01931286439371
4 2.82906626173755
5 3.09427938765557
6 3.60416870184349
7 4.24596487007442
8 4.84338888587772
9 5.27994908427636
10 5.61004074039071
11 5.90268352537916
12 6.05852129333431
13 6.16858387553312
14 6.19509636026208
15 6.21485180933973
16 6.20378189365436
17 6.1468591562609
18 6.14787992255152
19 6.14579317317396
20 6.15283082950704
21 6.15412613868876
22 6.14366281427887
23 6.16587792193215
24 6.18223254289368
25 6.18638821201769
26 6.14794417270148
27 6.14179954980725
28 6.15812095860932
29 6.16746194810668
};
\end{groupplot}

\begin{groupplot}[group style={group size=1 by 3}]
\nextgroupplot[
xshift=-8,
xmin=-1.45, xmax=30.45,
%ymin=-0.848571901426494, ymax=2.81768238587247,
ymin=-0.85, ymax=5.85,
width=\figurewidth,
height=\figureheight,
xtick={},
xticklabels={},
yticklabels={},
axis y line=right,
tick align=outside,
xtick pos=left,
ytick pos=right,
x grid style={white!69.019607843137251!black},
y grid style={white!69.019607843137251!black}
]
\addplot [line width=0.06pt, color1, mark=*, mark size=2, mark options={solid,draw=black}]
table {%
0 2.65103446372252
1 1.87298481713709
2 1.03310235020523
3 -0.0349224785257646
4 -0.681923979276541
5 -0.614035490335335
6 -0.208100847346677
7 0.33428430837777
8 0.710486243049944
9 0.726233644866842
10 0.520411660737353
11 0.347599665643602
12 0.244300607278545
13 0.195112904269273
14 0.20629800498181
15 0.161911176310666
16 0.161283251423433
17 0.247899352697984
18 0.208651205023874
19 0.171253015388636
20 0.20029198108343
21 0.172890109571832
22 0.187770311286831
23 0.213147053788955
24 0.185796243819713
25 0.165625930691843
26 0.187584184388062
27 0.20252014981221
28 0.179459395114634
29 0.2013127196102
};
\end{groupplot}

